Approaching 100% Confidence in Stream Summary through ReliableSketch

To approximate sums of values in key-value data streams, sketches are widely used in databases and networking systems. They offer high-confidence approximations for any given key while ensuring low time and space overhead. While existing sketches are proficient in estimating individual keys, they struggle to maintain this high confidence across all keys collectively, an objective that is critically important in both algorithm theory and its practical applications. We propose ReliableSketch, the first to control the error of all keys to less than $\Lambda$ with a small failure probability $\Delta$, requiring only $O(1 + \Delta\ln\ln(\frac{N}{\Lambda}))$ amortized time and $O(\frac{N}{\Lambda} + \ln(\frac{1}{\Delta}))$ space. Furthermore, its simplicity makes it hardware-friendly, and we implement it on CPU servers, FPGAs, and programmable switches. Our experiments show that under the same small space, ReliableSketch not only keeps all keys' errors below $\Lambda$ but also achieves near-optimal throughput, outperforming competitors with thousands of uncontrolled estimations. We have made our source code publicly available.

==> vldb/Body/Extensions.tex <==
\presec
\section{Optimizations and Extensions} \postsec
\label{sec:extensions}



% \subsection{Turn the Accuracy of Priority Flows}


% The extended Priority \anamelong{} can adjust the estimation accuracy of any flow. We can improve the accuracy of a high-priority flow (\eg, a flow with high SLA requirement) by giving it a weight. The weight of flow $e_i$, denoted as $w_i$, is an user-defined positive integer and it can improve the guaranteed accuracy from the old $\Lambda$ to $\floor{ \frac{\Lambda}{w_i}}$. Therefore, when $w_i$ is set to $\lfloor w_i \rfloor$, the estimation of flow $e_i$ must be correct.
% The key idea of inserting a packet $e_i$ with weight $w_i$ is to insert a packet for $w_i$ times by common insert operation. 
% Instead of spending $w_i$ times of time, we can achieve the same insertion speed as usual by some reasonable modifications. 
% Increasing the accuracy of partial flow will consume more memory. For example, if we reduce the error of 10\% flow by 50\%, we need 10\% more memory. 




% The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 
% The new \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. 

% The extended priority TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 

\subsection{Network-wide Deployment}

In a network, \anamelong{} can be deployed on user specified switches to measure the traffic. On the one hand, the accuracy can be improved by multiple sketches. On the other hand, we can find abnormal flow size changes without false positives.

\ppp{Accuracy improvement by multiple sketches.}
When a flow passes through multiple sketches on multiple switches, we can query its flow size in these sketches. Each sketch reports a possible flow size interval, \ie, $[\widehat{f_e}-MPE, \widehat{f_e}]$. The intersection of these intervals is a more accurate answer.

\ppp{Anomaly detection.} When a same flow passes through two sketches and they report two flow size intervals without intersection, we know that the flow size must have changed, without false positive.
In this case, we report potential packet drops if the flow size decreased, and report potential loops if the flow size increased.
More details are in \cref{sec:extensions:appendix:packetdrop}.


\subsection{A Mice Filter for Better Accuracy}
After achieving good theoretical results, the memory efficiency of \anamelong{} can be further optimized in practice.
The first layer of \anamelong{} is the largest layer, but it is inefficient when a large number of mice flows arrive and lock most buckets in the first layer. To handle the mice flows, we replace the first layer with a small mice-flow filter and still controlling the error well. 
Since that the mice flow filter only works for mice flows, we can optimize existing sketches based on this. We replace the basic unit of CU sketch \cite{estan2002cusketch} from 32-bit counter to 8-bit counter, as our mice filter. When inserting a packet to \anamelong{}, we insert it to the mice filter and query its over-estimated flow size at mice filter simultaneously. If the flow size exceeds the error threshold $\lambda_1$, we will insert the packet into the second layer. Otherwise, we do nothing and discard it. In real datasets, a mice filter usually improves the accuracy. More details in \cref{sec:extensions:appendix:micefilter}.





\presub
\subsection{Emergency Solution} \postsub
\label{extension:emergency}
In rare cases (\eg, probability $\delta=0.1^{10}$), we cannot insert a packet in the \anamelong{}, \ie, a packet reaches the last layer and meets an unavailable bucket, but we can still handle it with a CPU control plane or a small additional data structure like a hash table or a SpaceSaving \cite{spacesaving}. 
% When \anamelong{} is deployed on the switch (P4 platform), it is placed on the data plane. We just send these small amount of packets to the control plane, and use the CPU in control plane to count the flow size with no error. We can also use a small additional data structure like a hash table or a SpaceSaving \cite{spacesaving}. 
We implemented emergency solutions but did not add it to our accuracy evaluation (\cref{sec:experiments}), in order to clearly show \anamelong{} itself.
% \ppp{Stash for Emergency:}
% In rare cases, the last layer is not available for some flows, so we put a special \textit{stash} after the last layer to store these flows. The size of the stash can be regarded as a small constant. In our experiments, the stash does not have sensible impact on the experimental results, but it is important for our mathematical complexity analysis.
% We choose the classic SpaceSaving \cite{spacesaving} algorithm as our stash structure (We can also use others, including Misra–Gries algorithm \cite{misra1982finding} and Frequent \cite{demaine2002frequency}). 
% When there exists one flow's estimation error is greater than $\lambda$, we call it algorithm failure.
% Assuming that the probability of algorithm failure is $\delta$, \eg, $\delta=10^{-100}$. According to Theorem \ref{theo:main}, we set the size of SpaceSaving to $\Delta_2 \ln(\frac{1}{\delta})$.
% Although we cannot guarantee that there is no algorithm failure, we can make it small enough and become tolerable with small cost, \ie, $O(\ln(\frac{1}{\delta}))$.
% $\delta$ can be small enough to be less than the probability of hardware platform failure/damage (\eg, $\delta=10^{-100}$).




% \presub
% \subsection{More Functions of \anamelong{}} \postsub
% \label{extend}


% Our \anamelong{} has good versatility for various scenarios. We take the two most concernful tasks as examples, weighted counting and unbiased frequency estimation. We only introduce the key idea of how to achieve them.

% \ppp{Weighted Counting.} The extended Weighted TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 

==> vldb/Body/Framework.tex <==
% % % \presec
% % % \section{Framework of Error-Sensing} \postsec
% % % \label{sec:Framework}

% We first show the framework, followed by how it covers existing election operations. Then we show how we sense the error by the framework. 

% \ppp{Abstract Data Structure.} 
% The bucket has three fields, one ID field recording the ID of a candidate flow, and two counters recording the positive votes and negative votes, denoted as $ID$, $YES$ and $NO$, respectively. Initially, $ID$ is $null$ and both counters are $0$. The bucket supports two operations, insert and query as follows:

% \ppp{Insert a packet.}
% To insert a packet with flow ID $e$ into bucket $B$, we first decide whether to perform the replacement, \ie, replace the old $ID$ with new $e$ as the candidate frequent flow. 
% The criterion is whether $YES \leqslant F(NO)$, where $F: N |->N $ is a monotonically increasing function ($F(i)<F(i+1) \forall i$).
% If so, we believe there are too many NO votes and we replace the recorded flow. 
% In this case, $ID$ is not frequent enough to be kept and we can give other flows a chance to enter.
% After that, we vote whether the recorded flow $ID$ is $e$ or not. If so, we vote YES by incrementing $YES$ by $1$.
% Otherwise, we vote NO by incrementing the number of $NO$ by $1$.


% \ppp{Query the flow size.} 
% To query the flow size of $e$ in bucket $B$, we first check whether the recorded winner $B.winner$ is the queried flow $e$. If so, our estimation of the flow size $\widehat{f_e}$ is $B.YES$. Otherwise, $\widehat{f_e}$ is $B.NO$. The estimation is guaranteed to be no less than the true flow size (Proved by induction).
% % In both cases, MPE is $B.NO$. \wyh{This is our key technique I called Error-Sensing. 
% % At a high level, $B.NO$ works because it can \textit{reflect the intensity of conflict between different flows.

% \ppp{existing }
% elastic
% majority 
% space saving

% In fact, the novelty of our basic unit is not to design a structure that have never seen before, but to modify and use the reasonable part of the traditional structure as our basic unit. For the first time, we focus on and use the sensed error in other parts of the data structure, rather than just use it for the algorithm analysis.



% % % \ppp{Insert a packet.} 
% % % \wyh{To insert a packet with flow ID $e$ into bucket $B$, we first decide whether to perform the replacement, \ie, replace the old $B.winner$ with new $e$ as the candidate frequent flow. 
% % % The criterion is whether $B.YES \leqslant B.NO$.
% % % If so, we believe there are too many NO votes and we replace the recorded flow. In this case, $B.winner$ is not frequent enough to be kept and we can give other flows a chance to enter.
% % % % We will strictly explain the condition later.
% % % After that, we vote whether the recorded flow $B.winner$ is $e$ or not.
% % % If so, we vote YES by incrementing $B.YES$ by $1$.
% % % Otherwise, we vote NO by incrementing the number of $B.NO$ by $1$.}


% % % \ppp{Query the flow size and MPE. } 
% % % To query the flow size of $e$ in bucket $B$, we first check whether the recorded winner $B.winner$ is the queried flow $e$. If so, our estimation of the flow size $\widehat{f_e}$ is $B.YES$. Otherwise, $\widehat{f_e}$ is $B.NO$. The estimation is guaranteed to be no less than the true flow size (Proved by induction).
% % % In both cases, MPE is $B.NO$. \wyh{This is our key technique I called Error-Sensing. 
% % % At a high level, $B.NO$ works because it can \textit{reflect the intensity of conflict between different flows.}}



==> vldb/Body/Implementation.tex <==

\presec
\section{Implementations} \postsec
\label{sec:Implementations}

In this section, we introduce the implementation of \anamelong{} on P4 and FPGA platforms. We release our source code at GitHub anonymously \cite{opensource}.

% \subsection{Implementation on RMT switches}
% \label{sec:p4:deploy}
% We first briefly describe the architecture of RMT (recofigurable match-action table) switches \cite{??}, then we present the implementation of \aname{} on a typical kind of RMT switch, \ie, Tofino switch \cite{?} in P4 language. 

% \subsubsection{Architecture of RMT Switches}
% We take Tofino switch, a typical kind of RMT switch as example.
% %
% Figure \ref{?} shows the pipeline architecture of Tofino switches.
% %
% It mainly consists of three components: an Ingress pipeline, a traffic manager (TM), and an Egress pipeline.
% %
% Each incoming packet undergoes these three components in sequence.
% %
% %
% Each pipeline consists of a parser, a deparser, and multiple stages, and each of the stage has independent memory resources (\eg, SRAM, TCAM) and computing resources (\eg, SALU, hash units).
% %
% In the pipeline, Each incoming packet first undergoes the parser, which extracts packet header from the packet for forwarding logic.
% %
% Then, the packet access the stages in sequence.
% %
% %
% Finally, the packet undergoes the deparser, which reconstructs the packet with the extracted packet header, and then leaves the pipeline.
% %
% The TM forwards each packet that leave the Ingress pipeline to the egress pipeline, and the forwarded packet undergoes another pipeline before leaving the switch.
% %

% Such RMT architecture is constrained by its limited accessibility: In each stage, the packet can only access the resources in the stage itself.
% %
% In other words, the packet can never access the prior stages again.
% %
% Usually, this constraint requires the workflow of algorithms to be unidirectional. 
% %
% In order to circumvent this constraint, some prior solutions \cite{?} resubmit, mirror, or recirculate packets to access the prior stages at the cost of pipeline forwarding capacity.

\subsection{P4 Implementation}

To implement \aname{} on programmable switches (\eg, Tofino), we need to solve the following three challenges.

\ppp{Challenge I: Circular Dependency.}
%
Programmable switches require programmers to implement arrays as multiple SRAM blocks for data store and several SALUs for data operation.
%
A SALU in a stage can at most access a pair of 32-bit data from the SRAM in that stage.
%
However, each bucket of \aname{} has three fields: \texttt{ID}, \texttt{YES}, and \texttt{NO}, and there are two dependencies: (1) packets need to access \texttt{ID} before updating \texttt{YES} and \texttt{NO}; (2) packets need to access \texttt{YES} and \texttt{NO} before deciding whether to replace the \texttt{ID}.
%
These dependencies require the same SALU to operate on three fields, which are unachievable.
%
To address the problem, we need to reduce the interdependent fields to two.
%
We find that the replacement can be decided by only the difference between \texttt{YES} and \texttt{NO}, \ie, the replacement happens only when \texttt{NO}$\geqslant$\texttt{YES}.
%
Here, we can eliminate the dependency between \texttt{ID} and \texttt{NO}, and break the aforementioned dependency (2).
% , because the replacement (\ie, the update of \texttt{ID}) is decided by one field (\ie, \texttt{DIFF}) instead of two (\ie, \texttt{YES} and \texttt{NO})
%
\texttt{DIFF} and \texttt{ID} are interdependent. \texttt{NO} depends on \texttt{DIFF} and \texttt{ID}, but both \texttt{DIFF} and \texttt{ID} do not depend on \texttt{NO}.
%
Therefore, we replace \texttt{YES} with \texttt{DIFF}=\texttt{YES}-\texttt{NO}, put \texttt{DIFF} and \texttt{ID} in the first stage, and put \texttt{NO} in the second stage.


% \ppp{Challenge I: Circular Dependency.}
% %
% Programmable switches require programmers to implement arrays as multiple SRAM blocks for data store and several SALUs for data operation.
% %
% A SALU in a stage can at most access a pair of 32-bit data from the SRAM in that stage.
% %
% However, each bucket of \aname{} has three fields: \texttt{ID}, \texttt{YES}, and \texttt{NO}, and there are two dependencies: 1) packets need to access \texttt{ID} before updating \texttt{YES} and \texttt{NO}; 2) packets need to access \texttt{YES} and \texttt{NO} before deciding whether to replace the \texttt{ID}.
% %
% These dependencies require the same SALU to operate on three fields, which is unachieveable.
% %
% Therefore, we replace \texttt{YES} with \texttt{TOTAL}=\texttt{YES}+\texttt{NO}, thus eliminating the dependency between \texttt{ID} and \texttt{TOTAL}.
% %
% Specifically, we put \texttt{TOTAL} in one stage, and put \texttt{ID} and \texttt{NO} in the next stage.


\ppp{Challenge II: Backward Modification.}
%
% \zyk{
When \texttt{NO} exceeds the user-defined threshold, we need to lock the bucket, so that the flows other than \texttt{ID} can enter other buckets.
%
Since it is too late to know whether the bucket is locked when accessing \texttt{NO}, we put a flag \texttt{LOCKED} before \texttt{ID}.
%
However, due to the pipeline architecture of programmable switches, when a packet finds that \texttt{NO} exceeds the threshold, the flag cannot be modified in its life cycle.
%
Therefore, in this case, we will mirror the packet that first exceeds the threshold, and recirculate it, so that it can enter the pipeline again to modify the flag.
% }

\ppp{Challenge III: Three Branches Update and Output Limitation.}
%
When performing weighted update that inserts a flow with weight $w$, \texttt{DIFF} could be updated to three different values, but the switch can only support two of them: 
(1) When the \texttt{ID} matches and \texttt{YES} is increased by $w$, \texttt{DIFF} should be updated to \texttt{DIFF}+$w$; 
(2) When the replacement happens, \texttt{DIFF} should be updated to $w$-\texttt{DIFF}; 
(3) When \texttt{ID} does not match and the replacement does not happen, we just increase \texttt{NO} by $w$ and update \texttt{DIFF} to \texttt{DIFF}-$w$.
%
The tofino switch has two slices and each slice has two ALUs (Arithmetic Logic Unit). Since one slice should be used for updating \texttt{ID}, the other slice only supports two different result values for \texttt{DIFF}.
%
Besides, the output limitation requires that one stage can only output a $32$-bit value. For the first stage including \texttt{ID} and \texttt{DIFF}, its output value should not only tell the next stage whether and how to update \texttt{NO}, but also provide the estimation result when \texttt{ID} matches.
%
Therefore, when updating \texttt{DIFF}, we simplify the second case where the replacement happens. Specifically, if not in the first case (ID matches), we update \texttt{DIFF} to \texttt{DIFF} $|-| w$, where $|-|$ is the saturated subtract that will not subtract \texttt{DIFF} to a negative number (at most 0).
In the second case (replacement), \texttt{DIFF} will be subtracted to $0$ and we do not replace \texttt{ID} immediately. We will replace \texttt{ID} when the next packet comes and finds \texttt{DIFF} is $0$. 


% \ppp{Challenge III: Backward Update.}
% %
% Although we eliminate the dependency between \texttt{ID} and \texttt{NO} in the unlocked bucket, for a locked bucket, packets still need to access the \texttt{ID} before deciding whether to update \texttt{TOTAL}.
% %
% Since frequent mirroring and recirculation will significantly consume the switch bandwidth, after locking a bucket, we increment \texttt{NO} instead of \texttt{TOTAL} for each packet with flow ID matching \texttt{ID}.
% %
% By comparing \texttt{NO} and threshold, we can restore the number of packets with flow ID matching \texttt{ID} received after the bucket is locked.

% \begin{comment}


% At a high level, we abstract the implementation of \aname{} as a workflow consisting of several modules.
% %

% \ppp{Workflow:}
% The workflow consists of a cold filter \cite{coldfilter} module, \aname{} module, and a lock module, and the traffic undergoes them in turn.
% %

% \bbb{1) Cold filter module:}
% This module consists of several pairs of hash function and array.
% %, and each pair of hash function and 8-bit counter array is placed in one stage.
% %
% For each incoming packet, it find a counter in every array, and increase the values by one.
% %
% %
% % When the value of the hashed counter in the first array reaches $u$, it will further enter the second array, and repeats the same operation as in the first array.
% %
% %
% Only the packet that its counter in each array reaches $u$ can further enter the \aname{} module.

% \bbb{2) Lock module:}
% This module consists of several pairs of hash function and array.
% %
% For each packet enter a layer of \aname{} module, they need to get status of the lock, and then decide how to work in \aname{} module.
% %
% Besides, \aname{} module could also mirror a packet back here to lock the bucket.

% \bbb{3) \aname{} module:}
% This module consists of several pairs of hash function and array.
% %
% For each array, we build two registers.
% %
% The first consists of 32-bit counters, counting the total number of packets.
% %
% The second consists of 64-bit counters, each of which is split into two field, first field is to store the ID, and second field counts the collision number of packets.
% %
% For each incoming packet, it gets the status from the lock module, determined by the status, the work of a layer will be divided into two classes:
% %

% \bbb{Unlocked}: First, the packet will find a bucket in the first register and increase the value of the total counter.
% %
% Second, the packet will find the bucket in the second register, checking whether it needs to change the ID storing in the ID field, and then compare the ID, if different, increase the value of collision field. 
% %
% Third, the packet will check whether the collision value reaches threshold of the layer, if so, we mirror the packet to lock the bucket.
% %

% \bbb{Locked:}In a locked bucket, packet will only find the bucket in second register, and then check whether the ID is match, increasing the value of collision field if matches, if not, the packet will enter the next layer.

% \ppp{Hardware Resources Utilization:}
% We show the utilization of different types of hardware resources in Table \ref{table:resource}. We can see that the average usage is less than 25\% across all resources. We implement \aname{} in 9 stages on Tofino switch: 1 stage for cold filter module, 7 stages for three layers of \aname{} module and 1 stage for lock module.

% \end{comment}

% \ppp{Workflow:}
% The workflow consists of a cold filter \cite{coldfilter} module, \aname{} module, and a lock module, and the traffic undergoes them in turn.
% %

% \bbb{1) Cold filter module:}
% The cold filter module consists of several pairs of hash function and 8-bit counter array.
% %, and each pair of hash function and 8-bit counter array is placed in one stage.
% %
% Specifically, for each array, we build a register consists of $w$ 8-bit register elements, and use one stateful ALU (SALU) to set a constant upper bound $u$ for each counter.
% %
% For each incoming packet, it is first hashed to one counter in the first array, and the SALU increments the value of the hashed counter by one.
% %
% %
% % When the value of the hashed counter in the first array reaches $u$, it will further enter the second array, and repeats the same operation as in the first array.
% The same operation will be repeat in the second array as that in the first one.
% %
% Only the packet that its hashed counter in each array reaches $u$ can further enter the \aname{} module.

% \bbb{2) Lock module:}
% The lock module consists of several pairs of hash function and array made of error-sensibel buckets.
% %
% For each array, we build one register consist of 8-bit register elements, used as lock.
% %
% For each packet enter a layer of \aname{} module, they first need to get the status of the hashed lock register, then decide how to work with the layer of \aname{} module, when the status is locked, the packet will possibly enter the next layer of \aname{} module.
% %
% Besides, \aname{} module will also mirror a packet back to the ingress pipeline to lock the corresponding bucket, while receiving the packet, lock module will find the register and lock the corresponding bucket, and then drop the mirrored packet.

% \bbb{3) \aname{} module:}
% The \aname{} module consists of several pairs of hash function and array made of error-sensible buckets.
% %
% Specifically, for each array, we build two registers.
% %
% The first register consists of 32-bit counters, each of which counts the total number of packets hashed to it.
% %
% The second register consists of 64-bit counters, each of which is split into two field, the first field is to store the packet ID, which we called ID field, and the second field is to count (twice of) the collision number of packets hashed to it, which we called collision field.
% %
% For each incoming packet, it is first hashed to the lock module to get the status, determined by the status, the work of layer will be divided into two class:
% %

% \bbb{Unlocked}: First, the packet will be hashed to one bucket in the first register, increasing the value of the total counter, and get the increased value into our metadata.
% %
% Second, the packet will use the same hash to a bucket in the second register, getting the collision field to check whether it needs to change the ID storing in the ID field(if $total - 2 * collision < 0$), and then compare the ID in the ID field with that in metadata, if not the same, increase the value of collision by two(convenient for computing $total - 2 * collision$), then we get the increased value into metadata. 
% %
% Third, the packet will compare the collision value in metadata with the threshold of the corresponding layer, if equal, we mirror the packet to lock module. The packet hashed into an unlocked bucket will not enter the next layer.  
% %

% \bbb{Locked:}The packet hashed into a locked bucket will be only hashed to a bucket in the second register, and then compare whether the ID is match that in the ID field, increasing the value of collision field if matches. When the bucket is locked, the collision number will not exceed the threshold, so we use the collision counter as an additional total counter, if it does not match, the packet enter the next layer.

% \ppp{Hardware Resources Utilization:}
% We show the utilization of different types of hardware resources in Table \ref{table:P4}. We can see that the average resources usage is less than 25\% across all resources. The most resource usage is Stateful ALUs, which is used for accessing registers and performing transactional read-test-write operations on \aname{}. We implement \aname{} in 9 stages on Tofino switch: 1 stage for the Cold Filter module, 7 stages for the three layer of \aname{} module pipeline and 1 stage for the lock module. In addition, we use 1 stage to implement the basic functions of the switch, such as route matching and packet forwarding.


\vspace{-0.2cm}
\begin{table}[H]
\caption{H/W Resources Used by \aname{}. }
%\vspace{0.05in}
\label{table:resource} 
\vspace{-0.3cm}
\begin{tabular}{m{0.35\columnwidth}|m{0.25\columnwidth}<{\raggedleft}|m{0.27\columnwidth}<{\raggedleft}}
% \hline
\bottomrule[1pt]
\textbf{Resource}   & \textbf{Usage} & \textbf{Percentage} \\ \hline
Hash Bits  & 541 & 10.84\% \\
SRAM  & 138 & 14.37\% \\
Map RAM  & 119 & 20.66\% \\
TCAM  & 0 & 0\% \\
Stateful ALU  & 12 & 25.00\% \\
VLIW Instr  & 23 & 5.99\% \\
Match Xbar  & 109 & 7.10\% \\
% \hline
 \toprule[1pt]
\end{tabular}
\vspace{-0.05in}
\end{table}

\ppp{Hardware resource utilization:}
%
% \zyk{
After solving the above three challenges, we have fully implemented \aname{} on Edgecore Wedge 100BF-32X switch (with Tofino ASIC).
%
Table \ref{table:resource} lists the utilization of various hardware resources on the switch.
%
The two most used resources of \aname{} are Map RAM and Stateful ALU, which are used 20.66\% and 25\% of the total quota, respectively.
%
These two resources are mainly used by the multi-level bucket arrays in \aname{}.
%
For other kinds of sources, \aname{} uses up to 14.37\% of the total quota.
% }

\begin{table}[H]
\caption{Time Consumption of Aggregation.}
%\vspace{0.05in}
\label{table:time} 
\vspace{-0.3cm}
\begin{tabular}{m{0.21\columnwidth}<{\centering}|m{0.21\columnwidth}<{\centering}|m{0.21\columnwidth}<{\centering}|m{0.21\columnwidth}<{\centering}}
\bottomrule[1pt]
% \hline
\textbf{Total}   & \textbf{Sync.} & \textbf{Collection} & \textbf{Analysis} \\ \hline
$1.005\ sec$ & $995.566\ msec$ & $3.612\ msec$ & $5.387\ msec$ \\
% \hline
\toprule[1pt]
\end{tabular}
\vspace{-0.05in}
\end{table}

\ppp{Network-wide aggregation mechanism:}
%
We have also implemented a set of aggregations mechanism for collecting data structures on each switch in the whole network.
%
The mechanism includes some \texttt{sender} agents and an \texttt{aggregator} agent.
%
The \texttt{sender} runs on the control plane of each switch deployed with \aname{}, periodically synchronizes the data of the \aname{} from the data plane, and sends the synchronized \aname{} to the \texttt{aggregator}.
%
The \texttt{aggregator} runs on a server, collects the \aname{}es sent by all switches, and performs data analysis.
%
Table \ref{table:time} lists the time consumption of each part of the aggregation process.






\presub
\subsection{FPGA Implementation} \postsub
\label{sec:FPGA:deploy}
We implement the \aname{} on an FPGA network experimental platform (Virtex-7 VC709). The FPGA integrated with the platform is xc7vx690tffg1761-2 with 433200 Slice LUTs, 866400 Slice Register, and 1470 Block RAM Tile. The implementation mainly consists of three hardware modules: calculating hash values (hash), Error-Sensible Buckets (ESbucket), and a stack for emergency solution (Emergency). \anamelong{} is fully pipelined, which can input one key in every clock, and complete the insertion after 41 clocks. According to the synthesis report (see Table 1), the clock frequency of our implementation in FPGA is 340 MHz, meaning the throughput of the system can be 340 million insertions per second.

\begin{table} [h]
\renewcommand\arraystretch{1.05}
    % \begin{center}
    % \vspace{-0.05in}
    \caption{FPGA Implementation Results.}
    \label{tb:FPGA}
    \vspace{-0.15in}
    \begin{tabular}{m{0.2\columnwidth}|m{0.12\columnwidth}<{\raggedleft}|m{0.15\columnwidth}<{\raggedleft}|m{0.12\columnwidth}<{\raggedleft}|m{0.2\columnwidth}<{\raggedleft}}
\bottomrule[1pt]
    % \hline
    \textbf{Module} & \centering \makecell{\textbf{CLB}\\\textbf{LUTS}} & \makecell{\textbf{CLB}\\\textbf{Register}} &\makecell{\textbf{Block}\\\textbf{RAM}} &\makecell{\textbf{Frequency}\\\textbf{(MHz)}}\\
    \hline
    Hash & 85 & 130 & 0 & 339\\
    % \hline
    ESbucket &  2521 &  2592 & 258 & 339\\
    % \hline
    Emergency &  48 &  112 & 1 & 339\\ \hline
     \specialrule{0em}{1pt}{1pt} \hline
    % \hline
    Total &  2654 &  2834 & 259 & 339\\
    % \hline
    Usage &  0.61\% &  0.33\% & 17.62\% & \\
    % \hline
\toprule[1pt]
    \end{tabular}

    % \end{center}
\end{table}

==> vldb/Body/abstract.tex <==

\begin{abstract}
    To estimate the frequency of every item in a data stream, the sketch is the most promising solution due to its fast speed and small average estimation error.
    Some estimations have small errors but some have large errors greater than the user-defined threshold.
    The key problem is that no existing sketch can sense the error for each estimation, let alone controlling the error of all estimations below the user-defined threshold.
    We devise TrustySketch that can report differentiated/personalized error bound for each estimation and control all errors below any user-defined threshold.
    Further, after 16 years without progress,
    we reduce the space complexity of frequency estimation from $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ to $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$, where $\varepsilon$ and $\delta$ are the parameters of accuracy and confidence, respectively.
\end{abstract}

%\keywords{data stream mining, top-k item, unbiased estimation, waving counter}

==> vldb/Body/abstractV2.tex <==

\begin{abstract}
    In network measurement, sketches become the most promising solution due to the fast speed, memory efficiency, and small average estimation error.
    However, existing sketches are not reliable enough in practice, because they cannot sense and control the per-flow error.
    We devise ReliableSketch that can report maximum possible error for each estimation, and control the error of all flows below small user-defined threshold $\Lambda$ at line rate.
    In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$.
    We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform.
    Under the same small memory, ReliableSketch not only controls the error of all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows.
\end{abstract}

%\keywords{data stream mining, top-k item, unbiased estimation, waving counter}

==> vldb/Body/abstractV3.tex <==

\begin{abstract}



    % For the network measurement on the switch data plane, sketches achieve the smallest average estimation error using small memory. 
    % However, the estimation error of a flow is not definitely small and there are always some flows with large errors. 
    % Therefore, the operator can never 100\% trust the sketch, especially during troubleshooting. We devise ReliableSketch that can control the estimation error of all flows below a small threshold $\Lambda$ at line rate. In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$. We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform. Under the same small memory, ReliableSketch not only controls the error of all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows. We open our source code anonymously.
    
    
    \wyh{For network measurements on the switch data plane, the sketch can estimate the sizes of all flows with high overall accuracy using small memory. }
    However, \wyh{the estimation error of each flow is not definitely small} and there are \wyh{almost} always some flows with large errors. 
    \wyh{Therefore, the operator can hardly trust every estimated flow size with 100\% confidence, especially during troubleshooting.} 
    We devise ReliableSketch that can control the estimation error of all flows below a small threshold $\Lambda$ at line rate. 
    In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$, \wyh{where $N$ is the total flow size and $\delta$ is the proportion of out-of-control flows with errors greater than $\Lambda$. 
    Thanks to the change of $\ln(\frac{1}{\delta})$ from multiplier to adder, under small memory constraints, our $\delta$ is small enough (far less than $\frac{1}{N}$) to eliminate out-of-control flow with extremely high probablity.}
    We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform. Under the same small memory, ReliableSketch not only controls the error of all flows \wyh{of less than $\Lambda$}, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows. We open our source code anonymously.
\end{abstract}

%\keywords{data stream mining, top-k item, unbiased estimation, waving counter}

==> vldb/Body/abstractV4.tex <==

\begin{abstract}



    % For the network measurement on the switch data plane, sketches achieve the smallest average estimation error using small memory. 
    % However, the estimation error of a flow is not definitely small and there are always some flows with large errors. 
    % Therefore, the operator can never 100\% trust the sketch, especially during troubleshooting. We devise ReliableSketch that can control the estimation error of all flows below a small threshold $\Lambda$ at line rate. In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$. We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform. Under the same small memory, ReliableSketch not only controls the error of all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows. We open our source code anonymously.
    
    
    \wyh{For network measurements on the switch data plane, the sketch can estimate the sizes of all flows with high overall accuracy using small memory. }
    However, \wyh{the estimation error of each flow is not definitely small} and there are \wyh{almost} always some flows with large errors. 
    \wyh{Therefore, the operator can hardly trust every estimated flow size with 100\% confidence, especially during troubleshooting.} 
    We devise ReliableSketch that can control the estimation error of all flows below a small threshold $\Lambda$ at line rate. 
    In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$, \wyh{where $N$ is the total flow size and $\delta$ is the proportion of out-of-control flows with errors greater than $\Lambda$. 
    Thanks to the change of $\ln(\frac{1}{\delta})$ from multiplier to adder, under small memory constraints, our $\delta$ is small enough (far less than $\frac{1}{N}$) to eliminate out-of-control flow with extremely high probablity.}
    We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform. Under the same small memory, ReliableSketch not only controls the error of all flows \wyh{of less than $\Lambda$}, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows. We open our source code anonymously.
\end{abstract}

%\keywords{data stream mining, top-k item, unbiased estimation, waving counter}

==> vldb/Body/abstractV5.tex <==

\begin{abstract}

        
    % \wyh{For network measurements on the switch data plane, the sketch can estimate the sizes of all flows with high overall accuracy using small memory. }
    However, \wyh{the estimation error of each flow is not definitely small} and there are \wyh{almost} always some flows with large errors. 
    \wyh{Therefore, the operator can hardly trust every estimated flow size with 100\% confidence, especially during troubleshooting.} 
    We devise ReliableSketch that can control the estimation error of all flows below a small threshold $\Lambda$ at line rate. 
    In theory, we reduce existing space complexity from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$, \wyh{where $N$ is the total flow size and $\delta$ is the proportion of out-of-control flows with errors greater than $\Lambda$. 
    Thanks to the change of $\ln(\frac{1}{\delta})$ from multiplier to adder, under small memory constraints, our $\delta$ is small enough (far less than $\frac{1}{N}$) to eliminate out-of-control flow with extremely high probablity.}
    We implement ReliableSketch on CPU, FPGA, and P4, and conduct experiments on a testbed and an event-level simulation platform. Under the same small memory, ReliableSketch not only controls the error of all flows \wyh{of less than $\Lambda$}, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows. We open our source code anonymously.
\end{abstract}

%\keywords{data stream mining, top-k item, unbiased estimation, waving counter}

==> vldb/Body/algo.tex <==
\presec
\section{The Versatile Sketch} \postsec
\label{SEC:Algorithm}


In this section, we first present the data structure of \aname{}, then we show its operations.
%Finally, as a case study, we show how to use \aname{} to find frequent items.
We list the symbols frequently used in this paper and their meanings in Table \ref{table:symbol}.

\begin{table} [!ht]
\begin{center}
\vspace{-0.1in}
\caption{Symbols frequently used in this paper.}
\label{table:symbol}
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}&\textbf{Meaning}\\
\hline
$\mathcal{S}$&a data stream\\
\hline
%$N$& number of distinct items in $\mathcal{S}$\\
%\hline
$e_i$& $i_{th}$ item in $\mathcal{S}$\\
\hline
$f_i$&frequency of $e_i$\\
\hline
$\widehat{f^{up}_i}$& the upper bound of the frequency of item $e_i$\\
\hline
$\widehat{f^{lo}_i}$& the lower bound of the frequency of item $e_i$\\
\hline
$d$&number of arrays/hash functions\\
\hline
$w$&number of buckets in each array\\
\hline
$h_j(.)$&hash functions from items to $\{1, \ldots ,w\}$\\
\hline
%$\mathcal{T}$&a predefined threshold\\
%\hline
$B_j[t]$& the $i_{th}$ bucket of the $j$-th array\\
\hline
$B_j[t].high$& high counter of $B_j[t]$\\
\hline
$B_j[t].low$\;\,& low counter of $B_j[t]$\\
\hline
$B_j[t].ID$\;\;& ID of the defender in $B_j[t]$\\
\hline
\end{tabular}
\vspace{-0.2in}
\end{center}
\end{table}
\vspace{-0.05in}

\presub
\subsection{Data Structure} \postsub
\label{subsec:alg:struct}

\ppp{Data Stream:} a data stream $\mathcal{S}=\{e_1,e_2,e_3,\dots\}$ is a sequence of items, each of which could appear more than once. The number of times that an item $e$ appears is $e$'s \textit{frequency}.

The \aname{} consists of $d$ arrays, $B_1, B_2, \dots, B_d$, and each array consists of $w$ buckets. 
% There are $k$ hash functions, $h_1(.), h_2(.), \dots, h_k(.)$,  and their outputs are integers in range $[0,w)$.
There are $d$ hash functions related to the $d$ arrays respectively, $h_1(.), h_2(.),\dots, h_d(.)$, mapping an item $e_i$ into bucket $B_j[t], t=h_j(e)$, where $j$ is the index of a hash function.
A bucket $B_j[t]$ consists of three parts: an ID field $B_j[t].ID$ recording the ID of the defender item, a low counter recording the health point of the defender item $B_j[t].low$, and a high counter recording the total number of the inserting items in this bucket $B_j[t].high$.

\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.48\textwidth]{vldb/GraphPPT/algo_graph1.pdf}
	\vspace{0.02in}
    \caption{Data structure and insertion examples of \aname{}.}
    \vspace{-0.1in}
	\label{ppt:struct}
\end{figure}


\begin{algorithm}
    
    \caption{\aname{}.}
    \label{alg:pseudo:v1}
    \KwIn{an item $e_i$}
    
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e_i$}}{
        \For{$j=1,2,\dots,d$}{
            $t \gets h_j(e_i)$\;
            $B_j[t].high\gets B_j[t].high+1$\;
            \If{$B_j[t].ID=NULL$}{
                $B_j[t].ID \gets e_i$\;
            }
            \eIf{$e_i=B_j[t].ID$}{
                $B_j[t].low\gets B_j[t].low+1$\;
            }
            {
                $B_j[t].low\gets B_j[t].low-1$\;
            }
            \If{$B_j[t].low=0$}{
                $B_j[t].ID\gets NULL$\;
            }
        }
    }
    
    % \SetKwFunction{FMain}{Query}
    % \SetKwProg{Fn}{Function}{:}{}
    % \Fn{\FMain{$f$, $p_i$}}{
    %     $Answer\gets MAX\_NUM$\;
    %     \For{$j=0$ to $K-1?$}{
    %         $c_j\gets C_j[h_j(f)\%d]$\;
    %         \If{$\lfloor\frac{c_j}{w_{p_i}}\rfloor<Answer$}{
    %             $Answer\gets \lfloor\frac{c_j}{w_{p_i}}\rfloor$\;
    %         }
    %     }
    %     \Return $Answer$\;
    % }
\end{algorithm}

\presub
\subsection{Standard Operations of \aname{}} \postsub
\label{subsec:alg:vote}

\ppp{Initialization.} 
Initially, all fields in the data structure are $0$ or $null$. If an item $e_i$ goes into a bucket $B_j[t]$ with a $null$ ID field. The ID field $B_j[t].ID$ will be set to $e_i$.

\ppp{Insertion (Figure \ref{ppt:struct}).} 
We show the pseudocode of inserting an item $e_i$ in Algorithm \ref{alg:pseudo:v1}.
%
To insert $e_i$, for each hash function $h_j(.)$, we find the bucket $B_j[t], t=h_j(e_i),$ and insert $e_i$ to it.
There are three steps to insert $e_i$ into bucket $B_j[t]$. First we increment the high counter $B_j[t].high$ by $1$ and set $B_j[t].ID$ to $e_i$ if it is $null$.
Then we check wheth to er $e_i$ is the same as the defender $B_j[t].ID$ or not. If so, we increment the low counter $B_j[t].low$ by $1$. Otherwise, we decrease $B_j[t].low$ by $1$. Finally, we check if $B_j[t].low$ is equal to $0$. If so we set $B_j[t].ID$ to $e_i$. 

\ppp{Frequency Estimation.}
To estimate the frequency of item $e_i$, the \aname{} can give both the upper bound $\widehat{f^{up}_i}$ and the lower bound $\widehat{f^{lo}_i}$.
An item $e_i$ is mapped to $d$ buckets $B_j[h_j(e_i)], j=1,2,\dots,d$. The \aname{} estimate the frequency in different buckets independently and then summarise the result from different buckets.
To estimate the upper bound of the frequency of item $e_i$ in bucket $B_j[t], t=h_j(e_i)$, we first check whether $e_i$ is the same as $B_j[t].ID$ and calculate the upper bound of the $j$-th hashed bucket $c$ by the following formula:
\begin{align}
    f^{up}_{i,j} & = \left\{
    \begin{aligned}
    \frac{1}{2}\cdot(B_j[t].high+B_j[t].low) & , & e=B_j[t].ID, \\
    \frac{1}{2}\cdot(B_j[t].high\hspace{-0.3mm}-B_j[t].low) & , & e\neq B_j[t].ID.
    \end{aligned}
    \right.\label{equation:upperbound:bucket}\\
\intertext{The upper bound of $e_i$'s frequency:} 
    \widehat{f^{up}_i} & =\min_{j=1}^{d}{\left\{f^{up}_{i,j}\right\}}\label{equation:upperbound}\\
\intertext{We can also get the lower bound of $e_i$'s frequency:}
    % \label{eq2}
    f^{lo}_{i,j} & = \left\{
    \begin{aligned}
    B_j[t].low & , & e_i=B_j[t].ID, \\
    0 & , & e_i\neq B_j[t].ID.
    \end{aligned}
    \right.\\
    \widehat{f^{lo}_i} & = \max_{j=1}^{d}{\left\{f^{lo}_{i,j}\right\}}
\end{align}

\subsection{Extra Operations of \aname{}}

\ppp{Expansion of the \aname{}.} We can double the size of each array of \aname{} so that it can contains more items. Since the methods of the expansion for each array are the same, without loss of generality, we assume that the $j$-th array be the expanded array.
Suppose that the $j$-th array before expansion is denoted by $\mathcal{P}$ with size $w$ and the result of the expansion is denoted by $\mathcal{Q}$ with size $2*w$.
% Suppose that the $i$-th bucket of \aname{} $\mathcal{P}$ was denoted by $\mathcal{P}[t]$.
The hash functions of $\mathcal{P}$ were implemented by $h^{(\mathcal{P})}_j(e)=(H_j(e) \mod l)$, where $H_j(.)$ is an hash function whose output is a $32$-bit integer. And the hash functions of $\mathcal{Q}$ were implemented by $h^{(\mathcal{Q})}_j(e)=(H_j(e) \mod 2*w)$.
To expand $\mathcal{P}$, we copy $\mathcal{P}$ to get a new \aname{} $\mathcal{P'}$ and concatenate $\mathcal{P}$ and $\mathcal{P'}$ to get an \aname{} $\mathcal{Q}_0$ with size $2*w$. Both the first $w$ buckets of $\mathcal{Q}_0$ and the other $w$ buckets of $\mathcal{Q}_0$ are the same as $\mathcal{P}$. Then we scan each bucket of $\mathcal{Q}_0$ to check each bucket by hash the IDs again. Specifically, for each bucket $\mathcal{Q}_0[t]$, we check if $h^{(\mathcal{Q})}_j(\mathcal{Q}_0[t].ID)$ equals to $t$. If not, we set $\mathcal{Q}_0[t].ID$ to $null$ , subtract $\mathcal{Q}_0[t].high$ from $\mathcal{Q}_0[t].low$, and set $\mathcal{Q}_0[t].low$ to $0$.
After that, we get the result of the expansion $\mathcal{Q}=\mathcal{Q}_0$.
\begin{align}
   \left[
 \begin{matrix*}[l]
   \mathcal{Q}[t].high \\
   \mathcal{Q}[t].low \\
   \mathcal{Q}[t].ID
  \end{matrix*}
  \right]
   = \left\{
    \begin{aligned}
    &\left[\begin{matrix*}[l]
   \mathcal{P}[\lfloor t/2\rfloor].high \\
   \mathcal{P}[\lfloor t/2\rfloor].low \\
   \mathcal{P}[\lfloor t/2\rfloor].ID
  \end{matrix*}\right]  ,\hspace{-1.90cm}  & h^{(\mathcal{Q})}_j(\mathcal{P}[\lfloor t/2\rfloor].ID) = t, \\
  %
  &\left[\begin{matrix}
   \mathcal{P}[\hspace{-0.0mm}\lfloor \!t/2\!\rfloor\hspace{-0.0mm}].high\!-\!\mathcal{P}[\hspace{-0.0mm}\lfloor \!t/2\!\rfloor\hspace{-0.0mm}].low \\
   0 \\
   null
  \end{matrix}\right]\!
   , \hspace{-1.93cm} &  otherwise .
    \end{aligned}
    \right.
\end{align}

\ppp{Compression of  \aname{}.} We can compress the size of each array of \aname{} by half to save memory. Suppose that the $j$-th array before compression is $\mathcal{P}$ with size $w$ and the result of compression is $Q$ with size $w/2$, where $w$ is an even number.
The hash functions of $\mathcal{Q}$ were implemented by $h^{(\mathcal{P})}_j(e)=(H_j(e) \mod w/2)$.
We calculate each bucket of $\mathcal{Q}$ according to the following two formulas:
\begin{align}
    \mathcal{Q}[t].high
   &= \max{(\mathcal{P}[t].high,\mathcal{P}[t+w/2].high)}\notag
   \\
   \left[
 \begin{matrix*}[l]
   \mathcal{Q}[t].low \\
   \mathcal{Q}[t].ID
  \end{matrix*}
  \right]
   &= \left\{
    \begin{aligned}
    \left[\begin{matrix*}[l]
   \hspace{0.37cm}\mathcal{P}[t].low\hspace{0.38cm}\\
   \hspace{0.37cm}\mathcal{P}[t].ID
  \end{matrix*}\right] & , &\!\!
   %
  \mathcal{P}[t].low\!>\!\mathcal{P}[t\!+\!w/2].low, \\
  %
  \left[\begin{matrix}
   \mathcal{P}[t\!+\!w/2].low\!\\
   \mathcal{P}[t\!+\!w/2].ID\;\,\! 
  \end{matrix}\right] & , &\!\!
   %
  \mathcal{P}[t].low\!\leq\!\mathcal{P}[ t\!+\!w/2].low.
    \end{aligned}
    \right.
\end{align}

\ppp{Mergence of \aname{}.} We can merge two \aname{}es to get a new \aname{}.
The two \aname{} and the new \aname{} have same number of arrays, same size of each array, and same hash functions. We merge the same index array from the two groups. Without loss of generality,  let $\mathcal{P}$ and $\mathcal{Q}$ denote the $j$-th array of the two \aname{}es respectively. The result of the merger of $\mathcal{P}$ and $\mathcal{Q}$, denoted by $\mathcal{R}$, can be calculated by the following two formulas:
\begin{align}
    \mathcal{R}[t].high
   &= \mathcal{P}[t].high+\mathcal{Q}[t].high\notag
   \\
   \left[
 \begin{matrix*}[l]
   \mathcal{R}[t].low \\
   \mathcal{R}[t].ID
  \end{matrix*}
  \right]
   &= \left\{
        \begin{aligned}
        %
        &\left[\begin{matrix}
       \mathcal{P}[t].low\!+\!\mathcal{Q}[t].low\\
       \mathcal{P}[t].ID
      \end{matrix}\right] ,\hspace{-0.8cm}& 
       \mathcal{P}[t].ID = \mathcal{Q}[t].ID,& \\
        %
        &\left[\begin{matrix*}[l]
       \mathcal{P}[t].low\\
       \mathcal{P}[t].ID
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].ID \neq \mathcal{Q}[t].ID\\
       \land \\
       \mathcal{P}[t].low\!>\!\mathcal{Q}[t].low
      \end{matrix}\right),& \\
      %
      &\left[\begin{matrix*}[l]
       \mathcal{Q}[t].low\\
       \mathcal{Q}[t].ID 
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].ID \neq \mathcal{Q}[t].ID\\
       \land\\
       \mathcal{P}[t].low\!\leq\!\mathcal{Q}[t].low
      \end{matrix}\right).&                                         
      %
        \end{aligned}
    \right.
\end{align}


\ppp{Refining \aname{}} %Refined \aname{}.
We can refine an \aname{} to get a simple sketch by deleting IDs and merging the High part with the Low part. The simple sketch $X$ was called \textit{Heavy \aname{}} and it can be used to estimate the frequency without recording IDs.
Let $\mathcal{P}$ denote the $j$-th array of the \aname{}.
The $j$-th array of Heavy \aname{}, $X_j$, is calculated by the following formula:
\begin{align}
    X_j[t] = (\mathcal{P}[t].high+\mathcal{P}[t].low)/2,\;\; t=0,1,\dots,l-1.
\end{align}

\ppp{Flow Classification.} To estimate the frequency of infrequent items, we can generate a \textit{Light \aname{}} $Y$. Together with Heavy \aname{} $X$, the Light \aname{} $Y$ can estimate the distribution/entropy of all items accurately.
Let $\mathcal{P}$ denote the $j$-th array of the \aname{}. 
The $j$-th array of Light \aname{}, $Y_j$, is calculated by the following formula:
\begin{align}
    Y_j[t] = (\mathcal{P}[t].high-\mathcal{P}[t].low)/2,\;\; t=0,1,\dots,l-1.
    \label{formula:light}
\end{align}

\ppp{An Option: Conservative Update.} The \textit{Conservative Update} is a different method of inserting an item. Although the \aname{} is quite accurate, we can further improve its accuracy by Conservative Update at the cost of its hardware friendliness. The \aname{} is compatible with all above operations. The \aname{} with Conservative Update is named of \textit{VCU Sketch}. 
Instead of inserting an incoming item $e_i$ to all hashed buckets, VCU Sketch only insert $e_i$ to the bucket with the smallest $f^{up}_{i,j}$. VCU Sketch insert
$e_i$ by two steps, accessing all hashed buckets to compute $f^{up}_{i,j}$ and inserting $e_i$ to every bucket $B_j[t]$ which satisfies both $t=h_j(e_i)$ and $f^{up}_{i,j}=\widehat{f^{up}_{i}}$. The methods of inserting an item to a bucket are the same for both VCU Sketch and \aname{}.

EXAMPLE:????





















The \aname{} reports both the upper bound $\widehat{f^{up}_i}$ and the lower bound $\widehat{f^{lo}_i}$ of the answer $f_i$ simultaneously.
An item $e_i$ is mapped into $d$ buckets $B_j[h_j(e_i)], j=1,2,\dots,d$. The \aname{} estimate the frequency in different buckets independently and then summarise the result from different buckets.
To estimate the upper bound of the frequency of item $e_i$ in bucket $B_i[j]$, where $t=h_j(e_i)$, we first check whether $e_i$ matches $B_i[j].record$ and calculate the upper bound of the $j^{th}$ hashed bucket $c$ by the following formula:
\begin{align}
    \hat{f}^{up}_{i,j} & = \left\{
    \begin{aligned}
    \frac{1}{2}\cdot(B_i[j].high+B_i[j].low) & , & e_i=B_i[j].record, \\
    \frac{1}{2}\cdot(B_i[j].high\hspace{-0.3mm}-B_i[j].low) & , & e_i\neq B_i[j].record.
    \end{aligned}
    \right.\label{equation:upperbound:bucket}\\
\intertext{The upper bound of the frequency of $e_i$:} 
    \widehat{f^{up}_i} & =\min{\left\{\hat{f}^{up}_{i,1}, \hat{f}^{up}_{i,2}, \dots, \hat{f}^{up}_{i,d}\right\}}\label{equation:upperbound}\\
\intertext{We can also calculate the lower bound of the frequency of $e_i$:}
    % \label{eq2}
    \hat{f}^{lo}_{i,j} & = \left\{
    \begin{aligned}
    B_i[j].low & , & e_i=B_i[j].record, \\
    0 & , & e_i\neq B_i[j].record.
    \end{aligned}
    \right.\\
    \widehat{f^{lo}_i} & = \max{\left\{\hat{f}^{lo}_{i,1}, \hat{f}^{lo}_{i,2}, \dots, \hat{f}^{lo}_{i,d}\right\}}
\end{align}

Correctness is shown later in Section \ref{subsec:math:cuoverestimation}.





\subsection{Extra Operations of \aname{}}
\label{subsec:alg:extra}
The extra operations include expansion, compression, aggregation, refinement, and flow classification. The first three operations are used for distributed systems. And the refining operation can compose a simplified sketch for incremental deployment. As the $d$ arrays in \aname{} are homogeneous, without loss of generality, we only describe the operation of one array in \aname{} (\ie, $d=1$) in the following parts. So we denote \aname{} as $B_j$.

\presubsub
\subsubsection{Expansion of the \aname{}.} We can double the size of \aname{} so that it contains more items. 
Suppose that the \aname{} before expansion is denoted by $B_j$ with size $w$ and the \aname{} after expansion is denoted by $B'_j$ with size $2*w$.
The hash functions of $B_j$ were implemented by $h_j(e)=(H_j(e) \mod w)$, where $H_j(.)$ is a hash function whose output is a $32$-bit integer. And the hash function of $B'_j$ is implemented by $h_j(e)=(H_j(e) \mod 2*w)$.
We calculate the expanded \aname{} $B'_j$ by the following formula:

\vspace{-0.15in}
\begin{align}
  \left[
 \begin{matrix*}[l]
  B'_j[t'].high \\
  B'_j[t'].low \\
  B'_j[t'].record
  \end{matrix*}
  \right]
  = \left\{
    \begin{aligned}
    &\left[\begin{matrix*}[l]
  B_i[j].high \\
  B_i[j].low \\
  B_i[j].record
  \end{matrix*}\right]  ,\hspace{0cm}  & \left(H_j(B_i[j].record) \bmod 2*w\right) = t, \\
  %
  &\left[\begin{matrix}
  B_i[j].high-B_i[j].low \\
  0 \\
  null
  \end{matrix}\right]
  , \hspace{-2.9cm} &  otherwise .
    \end{aligned}
    \right.
    \label{formula:expand}
\end{align}
\vspace{-0.2in}

\noindent where $t'=0, 1, \dots, 2w-1$ and $t= (t' \bmod w)$.


% \subsubsection{Expansion of the \aname{}.} We can double the size of each array of \aname{} so that it contains more items. 
% % Since the expansion methods for each array are the same, without loss of generality, we assume that the $j^{th}$ array be the expanded array.
% Suppose that the $j^{th}$ array before expansion is denoted by $\mathcal{P}$ with size $w$ and the result of the expansion is denoted by $\mathcal{Q}$ with size $2*w$.
% % Suppose that the $i$-th bucket of \aname{} $\mathcal{P}$ was denoted by $\mathcal{P}[t]$.
% The hash functions of $\mathcal{P}$ were implemented by $h^{(\mathcal{P})}_j(e)=(H_j(e) \mod w)$, where $H_j(.)$ is a hash function whose output is a $32$-bit integer. And the hash function of $\mathcal{Q}$ is implemented by $h^{(\mathcal{Q})}_j(e)=(H_j(e) \mod 2*w)$.
% To expand $\mathcal{P}$, we copy $\mathcal{P}$ to get a new \aname{} $\mathcal{P'}$ and concatenate $\mathcal{P}$ and $\mathcal{P'}$ to get a \aname{} $\mathcal{Q}_0$ with size $2*w$. In other words, both the first $w$ buckets of $\mathcal{Q}_0$ and the other $w$ buckets of $\mathcal{Q}_0$ are the same as $\mathcal{P}$. Then we scan each bucket of $\mathcal{Q}_0$ to check the IDs by hashing. Specifically, for each bucket $\mathcal{Q}_0[t]$, we check if $h^{(\mathcal{Q})}_j(\mathcal{Q}_0[t].record)$ equals to $t$. If not, we set $\mathcal{Q}_0[t].record$ to $null$, subtract $\mathcal{Q}_0[t].high$ from $\mathcal{Q}_0[t].low$, and set $\mathcal{Q}_0[t].low$ to $0$.
% After that, we get the result of the expansion $\mathcal{Q}=\mathcal{Q}_0$.
% % \newcommand{\divtwo}[1]{\left\lfloor\frac{t}{2}\right\rfloor}
% \begin{align}
%   \left[
%  \begin{matrix*}[l]
%   \mathcal{Q}[t].high \\
%   \mathcal{Q}[t].low \\
%   \mathcal{Q}[t].record
%   \end{matrix*}
%   \right]
%   = \left\{
%     \begin{aligned}
%     &\left[\begin{matrix*}[l]
%   \mathcal{Q}_0[t].high \\
%   \mathcal{Q}_0[t].low \\
%   \mathcal{Q}_0[t].record
%   \end{matrix*}\right]  ,\hspace{0cm}  & h^{(\mathcal{Q})}_j(\mathcal{Q}_0[t].record) = t, \\
%   %
%   &\left[\begin{matrix}
%   \mathcal{Q}_0[t].high-\mathcal{Q}_0[t].low \\
%   0 \\
%   null
%   \end{matrix}\right]
%   , \hspace{-1.2cm} &  otherwise .
%     \end{aligned}
%     \right.
%     \label{formula:expand}
% \end{align}

\presubsub
\subsubsection{Compression of  \aname{}.} We can compress the size of \aname{} by half to save memory. 
Suppose that the \aname{} before compression is denoted by $B_j$ with size $w$ and the \aname{} after compression is denoted by $B'_j$ with size $\frac{w}{2}$.
The hash function of $B'_j$ is implemented by $h_j(e)=(H_j(e) \bmod \frac{w}{2})$.
We calculate each bucket of $B'_j$ according to the following two formulas:

\vspace{-0.15in}
\begin{align}
    \mathcal{Q}[t].high
   &= \max{(\mathcal{P}[t].high,\mathcal{P}[t+\frac{w}{2}].high)}\notag
   \\
   \left[
 \begin{matrix*}[l]
   \mathcal{Q}[t].low \\
   \mathcal{Q}[t].record
  \end{matrix*}
  \right]
   &= \left\{
    \begin{aligned}
    \left[\begin{matrix*}[l]
   \hspace{0.30cm}\mathcal{P}[t].low\hspace{0.28cm}\\
   \hspace{0.30cm}\mathcal{P}[t].record
  \end{matrix*}\right] & , &
   %
  \mathcal{P}[t].low>\mathcal{P}[t+\frac{w}{2}].low, \\
  %
  \left[\begin{matrix}
   \mathcal{P}[t+\frac{w}{2}].low\\
   \mathcal{P}[t+\frac{w}{2}].record\;\,
  \end{matrix}\right] & , &
   %
  \mathcal{P}[t].low\leq\mathcal{P}[ t+\frac{w}{2}].low.
    \end{aligned}
    \right.
    \label{formula:compress}
\end{align}

\vspace{-0.2in}
\noindent where $t=0, 1, \dots, w/2-1$.

% \subsubsection{Compression of  \aname{}.} We can compress the size of each array of \aname{} by half to save memory. Suppose that the $j^{th}$ array before compression is $\mathcal{P}$ with size $w$ and the result of compression is $\mathcal{Q}$ with size $\frac{w}{2}$, where $w$ is an even number.
% The hash function of $\mathcal{Q}$ is implemented by $h^{(\mathcal{Q})}_j(e)=(H_j(e) \mod \frac{w}{2})$ which equals $(h^{(\mathcal{P})}_j(e) \mod \frac{w}{2})$.
% We calculate each bucket of $\mathcal{Q}$ according to the following two formulas:
% \begin{align}
%     \mathcal{Q}[t].high
%   &= \max{(\mathcal{P}[t].high,\mathcal{P}[t+\frac{w}{2}].high)}\notag
%   \\
%   \left[
%  \begin{matrix*}[l]
%   \mathcal{Q}[t].low \\
%   \mathcal{Q}[t].record
%   \end{matrix*}
%   \right]
%   &= \left\{
%     \begin{aligned}
%     \left[\begin{matrix*}[l]
%   \hspace{0.30cm}\mathcal{P}[t].low\hspace{0.28cm}\\
%   \hspace{0.30cm}\mathcal{P}[t].record
%   \end{matrix*}\right] & , &
%   %
%   \mathcal{P}[t].low>\mathcal{P}[t+\frac{w}{2}].low, \\
%   %
%   \left[\begin{matrix}
%   \mathcal{P}[t+\frac{w}{2}].low\\
%   \mathcal{P}[t+\frac{w}{2}].record\;\,
%   \end{matrix}\right] & , &
%   %
%   \mathcal{P}[t].low\leq\mathcal{P}[ t+\frac{w}{2}].low.
%     \end{aligned}
%     \right.
%     \label{formula:compress}
% \end{align}

\subsubsection{Aggregation of \aname{}.} 
When aggregating all \aname{}es of distributed data streams, the aggregation can be simplified to the mergence of two \aname{}es.
As each \aname{} corresponds to a data stream and depicts a multiple set of inserted items, there are two kinds of merging results: the union set and the sum set.

When we want the union of the two sets corresponding to two \aname{}es, we use \textbf{Union Mergence}. In other words, the resulting sketch reports item's maximum frequency in the two sets.
We demand that the two \aname{}es have the same sizes and the same hash functions. We merge each pair of arrays in parallel. 
Without loss of generality, let $\mathcal{P}$ and $\mathcal{Q}$ denote the $j^{th}$ array of the two \aname{}es, respectively. 
The aggregated sketch $\mathcal{R}$ can be calculated by the following two formulas:

\vspace{-0.15in}
\begin{align}
    \mathcal{R}[t].high
   &= \max{(\mathcal{P}[t].high,\mathcal{Q}[t].high)}\notag
   \\
   \left[
 \begin{matrix*}[l]
   \mathcal{R}[t].low \\
   \mathcal{R}[t].record
  \end{matrix*}
  \right]
   &= \left\{
        \begin{aligned}
        %
        &\left[\begin{matrix}
      \max{(\mathcal{P}[t].low,\mathcal{Q}[t].low)}\\
       \mathcal{P}[t].record
      \end{matrix}\right] ,\hspace{-0.8cm}& 
       \mathcal{P}[t].record = \mathcal{Q}[t].record,& \\
        %
        &\left[\begin{matrix*}[l]
       \mathcal{P}[t].low\\
       \mathcal{P}[t].record 
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].record \neq \mathcal{Q}[t].record\\
       and \\
       \mathcal{P}[t].low\!>\!\mathcal{Q}[t].low
      \end{matrix}\right),& \\
      %
      &\left[\begin{matrix*}[l]
       \mathcal{Q}[t].low\\
       \mathcal{Q}[t].record 
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].record \neq \mathcal{Q}[t].record\\
       and\\
       \mathcal{P}[t].low\!\leq\!\mathcal{Q}[t].low
      \end{matrix}\right).&                                         
      %
        \end{aligned}
    \right.
    \label{formula:merge}
\end{align}

When we want the sum of the two multisets, we use \textbf{Sum Mergence}.
In other words, the resulting sketch reports the sum of the frequencies of an item in the two sets.
The aggregated sketch $\mathcal{R}$ can be calculated by the following two formulas:

\vspace{-0.15in}
\begin{align}
    \mathcal{R}[t].high
   &= \mathcal{P}[t].high+\mathcal{Q}[t].high\notag
   \\
   \left[
 \begin{matrix*}[l]
   \mathcal{R}[t].low \\
   \mathcal{R}[t].record
  \end{matrix*}
  \right]
   &= \left\{
        \begin{aligned}
        %
        &\left[\begin{matrix}
       \mathcal{P}[t].low\!+\!\mathcal{Q}[t].low\\
       \mathcal{P}[t].record
      \end{matrix}\right] ,\hspace{-0.8cm}& 
       \mathcal{P}[t].record = \mathcal{Q}[t].record,& \\
        %
        &\left[\begin{matrix*}[l]
       \mathcal{P}[t].low\\
       \mathcal{P}[t].record
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].record \neq \mathcal{Q}[t].record\\
       and \\
       \mathcal{P}[t].low\!>\!\mathcal{Q}[t].low
      \end{matrix}\right),& \\
      %
      &\left[\begin{matrix*}[l]
       \mathcal{Q}[t].low\\
       \mathcal{Q}[t].record 
      \end{matrix*}\right] , \hspace{-1.0cm}&
      \left(\begin{matrix}
       \mathcal{P}[t].record \neq \mathcal{Q}[t].record\\
       and\\
       \mathcal{P}[t].low\!\leq\!\mathcal{Q}[t].low
      \end{matrix}\right).&                                         
      %
        \end{aligned}
    \right.
    \label{formula:merge}
\end{align}

\presubsub
\subsubsection{Refinement of \aname{}} %Refined \aname{}.
We can refine a \aname{} to get a simple sketch (defined as $X$) by deleting IDs and merging the high counter with the low counter. The simple sketch $X$ was called \textit{Heavy \aname{}} and it can be used to estimate the frequency without recording IDs.
The $j^{th}$ array of Heavy \aname{}, $X_j$, is calculated by the following formula:
\begin{align}
    X_j[t] = (B_i[j].high+B_i[j].low)/2,\;\; t=0,1,\dots,w-1.
    \label{formula:heavy}
\end{align}

\presubsub
\subsubsection{Flow Classification.} To estimate the frequency of infrequent items, we can generate a \textit{Light \aname{}} (defined as $Y$). Together with the Heavy \aname{} $X$, the Light \aname{} $Y$ can estimate the distribution/entropy of all items accurately.
The $j^{th}$ array of Light \aname{}, $Y_j$, is calculated by the following formula:
\begin{align}
    Y_j[t] = (B_i[j].high-B_i[j].low)/2,\;\; t=0,1,\dots,w-1.
    \label{formula:light}
\end{align}



\presub
\subsection{Scalability} \postsub
\label{subsec:alg:scalability}
Previously in the paper, we have presented a \aname{} only with an ID and a PairCounter (high and low). Here, we present our \aname{} with more diverse fields and other designs of the PairCounter.

\vspace{-0.07in}
\subsubsection{Diverse fields in the bucket.} 
We discuss what other tasks we can achieve when we attach more fields.

\ppp{Finding DDoS attack.} In this scenario, each item is a network packet, which includes a source IP (sIP) and a destination IP (dIP). 
A key step in finding DDoS attack is to find the victim, \ie, the dIPs that connect to large numbers of sIPs. The above number of distinct sources is called cardinality. We append an extra Bitmap (Section \ref{subsec:relate:}) as a cardinality estimator to each ID/bucket. When inserting a packet, we use the dIP as the ID of the packet. If the dIP is the same as the recorded dIP, we additionally insert the source to the bitmap. Otherwise, we do not modify the bitmap. When the recorded dIP changes, we clear the bitmap. Every time we insert an item into the bitmap, we calculate the cardinality. If the cardinality exceeds a given threshold $\Delta$, we alarm that the dIP might be a victim.
% Only when the destination is frequently accessed (\ie, be recorded in the ID field) will we estimate its connected sources' cardinality.
This approach is memory efficient because it ignores those packets with infrequent dIPs when estimating cardinality. Also, this approach benefits from its time awareness---dIPs having intensive visits in a short time are more likely to record.
In addition, when the above threshold $\Delta$ is huge, we can replace the bitmap with a HyperLogLog \cite{hyperloglog} as a cardinality estimator.
% 5)bitmap-> super spreaders graph stream

\ppp{Data attributes summary.} In many data stream scenarios, an item includes not only an identifier (ID) but also many attributes. The supervisor may want to count the sum/mean/variance of some attributes for frequent items. Suppose there is only one attribute $x_i$ of item $e_i$. We can attach three counters $C_0, C_1, C_2$ to each bucket/ID.
In a bucket, when the ID of incoming item $e_i$ matches the recorded ID, we increment $C_0$ by $1$, increment $C_1$ by $x_i$, and increment $C_2$ by $x_i^2$. When the recorded ID changes, we clear the three counters.
A bucket report $C_1$, $\frac{C_1}{C_0}$, and $\frac{1}{C_0-1}\left(C_2-\frac{C_1^2}{C_0}\right)$ as the sum, mean, and variance of attribute $x$. When querying an item, among its $d$ mapped buckets, we choose the bucket with both the matched ID and the largest $C_0$, and we answer the report from the chosen bucket.
% RDF图 排名 地理位置 各种属性 学生的分数 银行汇款 
% -> sum/ mean value/ variance

\ppp{Data aging.} When we need to remove old items, we can attach a timer (\eg, a timestamp) to each bucket/ID. Every time the inserted ID matches the recorded ID, we update the timer. When the inserted ID does not match the recorded ID, we check the timer whether the recorded item has not appeared for a long time. If so, we record the new inserted ID and reset the timer.

% timer 定时器 timestamp 删掉太老的
%2)timestamp->counter array->flowlet/aging  sliding window/hopping window


% ???
% eviction, freezing counter?
% \ppp{Circular counter array for sliding window/hopping window.}
% 1)

% 4)flag-> used to be a large flow/ Special monitor mark, total correct, freezing bit

% 5)bitmap-> super spreaders graph stream




\vspace{-0.07in}
\subsubsection{Design choices of PairCounter.}
We use a high counter and a low counter (high-and-low) as the PairCounter above, but besides, there are other designs of PairCounter with different features.
\ppp{1) Pure-and-low.} We replace the high counter of high-and-low with a counter called \textit{pure}. Unlike the high counter increases by $1$ at every time an item is inserted to the bucket, the pure counter increases by $1$ only when the inserted item matches the recorded ID. Every time the recorded ID changes, the pure counter is reset to $0$. The pure counter provides a more accurate under-estimation frequency than \textit{low} counter.
\ppp{2) Positive-and-native.} We can also use a positive counter and a negative counter to count the times that the incoming item matches and not matches the recorded ID, respectively. This strategy is similar to a high counter with a pure counter. 

==> vldb/Body/algo_v2.tex <==


\begin{table} [!ht]
\begin{center}
\caption{Symbols frequently used in this paper.}
\vspace{-0.1in}
\label{table:symbol}
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}&\textbf{Meaning}\\
\hline
% $\mathcal{S}$&a data stream\\
% \hline
$N$ & the size of stream $\mathcal{S}$\\
\hline
% $e_t$& $t^{th}$ item in $\mathcal{S}$\\
% \hline
% $f_t$&frequency of $e_t$\\
% \hline
$d$&the number of layers\\
\hline
$w_i$&the number of buckets in the $i^{th}$ layer\\
\hline
$R_w$& the portion that $w_i$ decreases\\
\hline
$\lambda_i$&the error threshold in the $i^{th}$ layer\\
\hline
$R_\lambda$& the portion that $\lambda_i$ decreases\\
\hline
$h_i(.)$& hashing location function in the $i^{th}$ layer\\
\hline
$S(.)$& sign hash function\\
\hline
$B_i[j]$& the $j^{th}$ bucket of the $i^{th}$ layer\\
\hline
$B_i[j].high$& the high counter of bucket $B_i[j]$\\
\hline
$B_i[j].unbias$ & the unbiased counter of bucket $B_i[j]$\\
\hline
$B_i[j].low$\;\,& the low counter of bucket $B_i[j]$\\
\hline
$B_i[j].record$\;\;& the recorded item in $B_i[j]$\\
\hline
\end{tabular}
\vspace{-0.2in}
\end{center}
\end{table}
\vspace{-0.05in}


\presec
\section{The Versatile Sketch} \postsec
\label{SEC:Algorithm}


% In this section, we present our Versatile Sketch (\aname{}).
% First, we describe the data structure (Section Section \ref{subsec:alg:struct}) and the standard operations of \aname{} including the interval estimation (Section \ref{subsec:alg:Standard}).
% Then, we show its extra operations which are used for distributed systems and incremental deployment (Section \ref{subsec:alg:extra}).
% For easy understanding, the \aname{} presented above is a simple version. In the final Section \ref{subsec:alg:scalability}, we show more features that \aname{} can achieve and discuss more design choices.
% To clarify \aname{}, we list essential symbols used in this paper and their meanings in Table \ref{table:symbol}.

\ppp{Data Stream Model:} A data stream $\mathcal{S}=\{\langle e_1, w_1\rangle , \langle e_2, w_2\rangle, \dots$, $\langle e_t, w_t\rangle, \dots, \langle e_N, w_N\rangle\}$ is a sequence of pairs following time order. Each pair has an item identifier $e_t$ and a weight $w_t$ ($w_t>0$). An identifier $e$ may appear more than once in different pairs. The frequency of an item $e$ is the number of times that it appears, \ie, $f(e)\coloneqq \sum_{\forall e_t=e} 1$. The weighted frequency of item $e$ is the total weight, \ie, $w(e)\coloneqq \sum_{\forall e_t=e} w_t$. A data streaming algorithm (\eg, sketches) can only process the data stream in single pass. Our \aname{} is to estimate $f(e)$ and $w(e)$ for arbitrary queried item $e$ ($e$ may not appear in the data stream).

% Our \aname{} provides two estimators for each query. One is an one-sided estimator including an estimated frequency that is not less than the answer
% \begin{figure}[!ht]
%     % \prefig
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{vldb/GraphPPT/algo_graph1.pdf}
% 	\prefigcaption
%     \caption{Data structure and insertion examples. There is a \aname{} with $d=2$ arrays, and each array has $w=5$ buckets. The figure shows how to insert a new item $e_i$.}
% 	\label{ppt:struct}
% 	\postfig
% \end{figure}


\newcommand\floor[1]{{\lfloor #1 \rfloor}}

\presub
\subsection{Data Structure} \postsub
\label{subsec:alg:struct}

The structure of \aname{} consists of $d$ layers. The $i^{th}$ layer is an array consists of $w_i$ buckets, denoted by $B_i[1], B_i[2], \dots, B_i[w_i], i\in\{1, 2, \dots, d\}$. The size of each layer decreases in proportion to $R_{w}=2$, \ie, $ w_i=\frac{W}{2^i}$.
Each layer has an location function $h_i(\cdot)$, which maps each item (denote by $e$) into a random bucket (the $j^{th}$ bucket $B_i[j], j=h_i(e)$) uniformly by hashing. Each layer has an error threshold $\lambda_i$, where \aname{} can ensure that the estimation error of $i^{th}$ layer is less than $\floor{\lambda_i}$. Each error threshold also decreases in proportion to $R_{\lambda}=2$, \ie, $ \lambda_i=\frac{\Lambda}{2^i}$.

The structure of all buckets is the same: Bucket $B_i[j]$ records an item identifier $B_i[j].record$ and three counters $B_i[j].high$, $B_i[j].unbias$, and $B_i[j].low$. 
$B_i[j].high$ is the total frequency of all items inserted into the bucket. Among these items, the frequency of item $B_i[j].record$ is at least $B_i[j].low$. $B_i[j].unbias$ is a counter that helps provide unbiased estimation.

% recording the ID of the defender item, a low counter $B_i[j].low$ recording the health point of the defender item, and a high counter $B_i[j].high$ recording the total number of the inserting items in this bucket .


\presub
\subsection{Standard Operations of \aname{}} \postsub
\label{subsec:alg:Standard}

\ppp{Initialization.} 
Initially, all counters in the data structure are $0$ and the recorded item identifiers are $null$.

\begin{algorithm}[!h]
    \SetAlgoNoLine
    \caption{\aname{} Insertion.}
    \label{alg:pseudo:v1}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $i\gets 1$ \Comment{Start finding first available bucket}
    
        \While{$i<d$}{
            $j\gets h_i(e)$  \Comment{Locate a bucket}
            
            \If{$(\frac{1}{2}\cdot(B_i[j].high-B_i[j].low) < \floor{\lambda_i}$\textbf{or} $B_i[j].record=e)$}{
                \textbf{break} \Comment{Stop at the first available bucket}
            }
            $i\gets i+1$ \Comment{Go to next layer}
        }
            $j\gets h_i(e)$ \Comment{Will insert $e$ into bucket $B_i[j]$}
            
            \If{$B_i[j].low=0$}{ 
                $B_i[j].record\gets e$ \Comment{Perform item replacement}
            }
                                \Comment{Update counters}
                                
            \eIf{$B_i[j].record=e$}{
                $B_i[j].low\gets B_i[j].low+1$
            }{
                $B_i[j].low\gets B_i[j].low-1$
            }
            $B_i[j].high\gets B_i[j].high+1$
            
            $B_i[j].unbias\gets B_i[j].unbias+S(e)$
    
    
    }
\end{algorithm}

\begin{algorithm}[!h]
    \SetAlgoNoLine
    \caption{\aname{} Query Frequency.}
    \label{alg:pseudo:v1}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{QueryFrequency}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $ UP\gets 0$  \Comment{Upper Estimator}
        
        $ Ub\gets 0$ \Comment{Unbiased Estimator}
        
        $ TotalError\gets 0$ \Comment{Maximum Possible Error}
    
        $i\gets 1$ 
        
        \While{$i\leqslant d$}{
            $j\gets h_i(e)$  \Comment{Locate the bucket}
            
            \eIf{$B_i[j].record=e$}{
                $UP\gets UP +\frac{1}{2}\cdot(B_i[j].high+B_i[j].low)$
                
                $Ub\gets Ub+B_i[j].unbias$
            }{
                $UP\gets UP + \frac{1}{2}\cdot(B_i[j].high-B_i[j].low)$
                
                $Ub\gets Ub+B_i[j].unbias-B_i[j].low\cdot S(B_i[j].record)$
            }
            
            
            $TotalError\gets \frac{1}{2}\cdot(B_i[j].high-B_i[j].low)$
            
            \If{$\frac{1}{2}\cdot(B_i[j].high-B_i[j].low)  < \floor{\lambda_i}$ \textbf{or} $B_i[j].record=e$}{
                \textbf{break} \Comment{Stop collecting frequency}
            }
            $i\gets i+1$ \Comment{Go to next layer}
        }
        
        $Ub\gets Ub*S(e)$
        
        \Return{$<UP, Ub, TotalError>$}
    }
\end{algorithm}

\ppp{Insertion (Figure \ref{ppt:struct} and pseudocode Algorithm \ref{alg:pseudo:v1}).} 
We insert an item $e$ with weight $1$ by two steps.
\textbf{Step 1: Finding an available bucket.} We start from the first layer and locate $e$ to a bucket, called mapped bucket $B_i[j], j=h_i(e)$. Then we check whether $B_i[j]$ is an available bucket. The bucket is available if one of the following two conditions holds: 
\textit{(i)} $B_i[j].record=e$, which means $e$ is an unlimited item in this bucket; 
% 2) $B_i[j].low=0$, which means the new item $e$ can replace the old item $B_i[j].record$; 
\textit{(ii)} $\frac{1}{2}(B_i[j].high-B_i[j].low)< \floor{\lambda_i}$, which means the error of this bucket is tolerable.
If the bucket is not available, we keep finding an available bucket in the next layer. Otherwise, we insert $e$ into current available bucket and accomplish the insertion without accessing next layer.
\textbf{Step 2: Insert the item into the available bucket.} To insert $e$ into bucket $B_i[j]$, we first replace the recorded item if $B_i[j].low=0$. Then we check where the recorded item is $e$. If so, we increment $B_i[j].low$ by $1$. Otherwise, there is a \textbf{collision} and we decrement $B_i[j].low$ by $1$, so that other items may replace it in the future. Second, anyway, we increment $B_i[j].high$ by $1$, and add $B_i[j].unbiased$ by $S(e)$, where $S(\cdot)$ is a hash function mapping items to $\{+1, -1\}$. So far, we have completed the insertion. 


\ppp{Query---Frequency estimation.} When query the frequency of an arbitrary item $e$, \aname{} can report two kinds of estimators (a one-sided error estimator and an unbiased estimator) and the maximal possible error of the two estimators.
Recall that, every time inserting an item, we only insert it into one bucket.
To estimate the total frequency, we just need to add up the frequencies in different buckets. 
Starting from the first layer, we access the mapped bucket $B_i[j], j=h_i(e)$ in each layer. 
If a bucket is available for $e$ (\ie, $B_i[j].record=e$ \textbf{or} $\frac{1}{2}(B_i[j].high-B_i[j].low)< \floor{\lambda_i}$), we know that $e$ must never be inserted into the following layers, and therefore we stop at current layer. 
%

For each mapped bucket $B_i[j]$, we estimate the frequency that $e$ insert into it, denoted as $f_i(e)$.
The number of collisions is at most $C=\frac{1}{2}\cdot(B_i[j].high-B_i[j].low)$.
If $e$ is the recorded item $B_i[j].record$, $f_i(e)$ is at most $B_i[j].high-C=\frac{1}{2}\cdot(B_i[j].high+B_i[j].low)$. Because if not ($f_i(e)>B_i[j].high-C$), there is less than $C$ items other than $e$, which is contradict to the $C$ collisions between different items. 
If $e$ is not the recorded item $B_i[j].record$, $f_i(e)$ is at most $C$. Because if not ($f_i(e)>C$), $e$ must not collide with $B_i[j].record$, which induces a contraction.
If $e$ is the recorded item $B_i[j].record$, its unbiased estimator of the frequency is $B_i[j].unbias*S(e)$. Otherwise, the unbiased estimator is $(B_i[j].unbias-B_i[j].low\cdot S(B_i[j].record))*S(e)$.
The maximum possible error of the above estimators is at most $C$.
Finally, we add up the estimators and the maximum possible error in different bucket, respectively. 
We get a one-sided error estimator $UP$ that is no less than $f(e)$, an unbiased estimator $Ub$ that $E(Ub)=f(e)$, and the maximum possible error of the two estimator $TotalError$.


==> vldb/Body/algo_v3.tex <==

\newcommand\floor[1]{{\lfloor #1 \rfloor}}


\begin{table} [!ht]
\begin{center}
\vspace{-0.3cm}
\caption{Symbols.}
\vspace{-0.2cm}
\label{table:symbol}
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}&\textbf{Meaning}\\
\hline
% $\mathcal{S}$&a data stream\\
% \hline
$N$ & the size of stream $\mathcal{S}$\\
\hline
% $e_t$& $t^{th}$ item in $\mathcal{S}$\\
% \hline
% $f_t$&frequency of $e_t$\\
% \hline
$d$&the number of layers\\
\hline
% $B_i$&the $i$-th layer\\
% \hline
$w_i$&the number of buckets in the $i$-th layer\\
\hline
$R_w$& the proportion that $w_i$ decreases\\
\hline
$\Lambda_i$&the warning threshold in the $i$-th layer\\
\hline
$\lambda_i$&the error threshold in the $i$-th layer\\
\hline
$R_\lambda$& the proportion that $\lambda_i$ decreases\\
\hline
$h_i(.)$& hash function in the $i$-th layer\\
% \hline
% $S(.)$& sign hash function\\
\hline
$B_i[j]$& the $j$-th bucket of the $i$-th layer\\
\hline
$B_i[j].total $& the total number of items in $B_i[j]$\\
\hline
% $B_i[j].unbias$ & the unbiased estimator in $B_i[j]$\\
% \hline
$B_i[j].collision$\;\,& the number of collisions in $B_i[j]$\\
\hline
$B_i[j].winner$\;\;& the recorded frequent item in $B_i[j]$\\
\hline
\end{tabular}
\vspace{-0.2in}
\end{center}
\end{table}
\vspace{-0.05in}


% 3.1 Rationale
% 3.2 key 
%  data
%  insertion
%  query
% 3.3 key techniques
%  1.
%  2.
% 3.4 dis

% 3.1 rationale
% 3.2 key technique1: collision sensible bucket
%     过渡
% 3.3 key technique2: double exp.. control
% 3.4 Weighted counting version
% 3.5 Unbiased version
% 3.6 handling the worst case


% \presec
%这个 Trusty Sketch 必须分开
\section{The Trusty Sketch} \postsec
\label{SEC:Algorithm}

In this section, we present \anamelong{}. 
It is made of many buckets. 
After showing the data structure, we first show how one bucket senses collisions and errors in Section \ref{subsec:alg:struct}. 
Then, we show how to organize these buckets and set thresholds to control the error of every item to the user-defined threshold in Section \ref{subsec:alg:Standard}.
Last, we extend \anamelong{} to support weighted-counting task and the unbiased estimation in Section \ref{extend}.
Essential symbols used in this paper and their meanings are listed in Table \ref{table:symbol}.


%We present \anamelong{} in this section. First, we present our rationale and the data structure of \anamelong{}. Then we present our two key techniques in the following two sections \ref{?}-\ref{?}. 
%Finally, we extend \anamelong{} to support weighted-counting task and the unbiased estimation.
% in Section \ref{?} and \ref{?}.
% Finally, 
% In this section, we present our Versatile Sketch (\anamelong{}).
% First, we describe the data structure (Section Section \ref{subsec:alg:struct}) and the standard operations of \anamelong{} including the interval estimation (Section \ref{subsec:alg:Standard}).
% Then, we show its extra operations which are used for distributed systems and incremental deployment (Section \ref{subsec:alg:extra}).
% For easy understanding, the \anamelong{} presented above is a simple version. In the final Section \ref{subsec:alg:scalability}, we show more features that \anamelong{} can achieve and discuss more design choices.
% To clarify \anamelong{}, we list essential symbols used in this paper and their meanings in Table \ref{table:symbol}.


\ppp{Overview:}
Given an user-defined error threshold $\Lambda$, our goal is to control the error of any item's estimated frequency below $\Lambda$.
The \anamelong{} consists of multiple layers, and each layer has an increasing warning threshold. These thresholds are at most $\Lambda$.
When an item’s error boundary (\ie, the maximum possible error) reaches the warning threshold in one layer, it will be inserted to the next layer. 
There are two key challenges: (1) finding all items whose error bounds reach the warning threshold with little false positive error; (2) handling items with large error bounds efficiently with small space and a small number of layers.
To tackle the first challenge, we devise the Collision-Sensing technique. To tackle the second challenge, we devise the Double Exponential Control technique based on a multi-layer structure.




\begin{figure}[htbp]
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graphnew1.pdf}
    \vspace{-0.15in}
    \caption{The structure of \anamelong{}.}
    \label{fig:algo:structure}
    \postfig
\end{figure}
\vspace{-0.6cm}

\presub
\subsection{Data Structure} \postsub
\label{sec:algo:structure}


As shown in Figure \ref{fig:algo:structure}, the data structure of \anamelong{} consists of $d$ layers, $B_1,$ $B_2,$ $\dots,$ $B_d$. The $i$-th layer $B_i$ is an array consists of $w_i$ \textit{collision-sensible buckets}, denoted as $B_i[1],$ $B_i[2],$ $\dots,$ $B_i[w_i]$. 
The size of layer $B_i$, denoted as $w_i$, decreases in proportion to $R_{w} (R_{w}>1)$ as $i$ increases.
Each layer $B_i$ has an error threshold, denoted as $\lambda_i$. $\lambda_i$ decreases in proportion to $R_{\lambda} (R_{\lambda}>1)$ as $i$ increases.
The warning threshold in layer $B_i$, denoted as $\Lambda_i$, is the sum of the error thresholds of the first $i$ layers, \ie, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i$ must be no more than user-defined threshold $\Lambda$.
Each layer is associated with a pair-wisely independent hash function $h_i(\cdot)$, which maps each item (denoted by $e$) into a random bucket (the $j$-th bucket $B_i[j], j=h_i(e)$) uniformly.
% , \ie, $ w_i=\left\lceil\frac{W_0}{R_{w}^i}\right\rceil$.
% To control all errors below $\Lambda$, each layer has an increasing error warning threshold, denoted as $\Lambda_i$ ($\Lambda_i\leqslant \Lambda$) in the $i$-th layer.
% The difference between the warning thresholds in adjacent layers is the amount of error that one layer can accommodate.
% For the $i$-th layer, it has an error threshold  $\lambda_i=\Lambda_i-\Lambda_{i-1}$, which represents the maximum error it can accommodate.
% The error threshold $\lambda_i$ guarantees that the estimation error of any bucket in $i$-th layer is less than $\lambda_i$.
% In the i-th layer, we set the error threshold to $\lambda_i=\left\lfloor\frac{\Lambda}{R_{\lambda}^i}\right\rfloor$, which decrease in proportion to $R_{\lambda}=2$. 
% Therefore, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i\leqslant\Lambda$.
% $\Lambda_i$ and $\Lambda_{i-1}$ represents the amount of error that the $i$-th layer can accommodate.
% Each layer has an error threshold $\lambda_i$, where \anamelong{} can guarantee that the estimation error of $i$-th layer is less than $\floor{\lambda_i}$.

\ppp{Parameter Configurations:} 
Let $W$ denote the total number of buckets. We set $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$. 
In our proofs (Theorem \ref{theo:main}), we set $W=\frac{4(R_w R_\lambda)^{6}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, which is with large constant.
But based on our experimental results, we recommend to set $W=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, $R_w\in[2, 10]$, $R_l\in[2, 10]$, and $d\geqslant 7$.
When then memory size is given without given $\Lambda$, we set 
\begin{align}
    \Lambda=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{W}
    \label{formula:setLambda}
\end{align}








\presub
\subsection{Technique I: Collision-Sensing} \postsub
\label{subsec:alg:struct}
In this section, we present the \textit{Collision-Sensing} technique.
%We focus on one bucket, and describe how it senses the error when one item is mapped into it.
% In this part, we present Collision-Sensing technique that can estimate the error boundary of each estimation. 
\textit{Collision-Sensing} is based on our special bucket design, named as collision-sensible bucket.
As shown in Figure \ref{collision_sensible}, a collision-sensible bucket supports two operations: (1) insertion of an item; (2) query of an item for its estimated frequency and error boundary.
%of an item together with its maximum possible error.
The structures of all collision-sensible buckets are the same. The bucket $B_i[j]$ contains one item identifier $B_i[j].winner$ and two counters, $B_i[j].total$ and $B_i[j].collision$.
$B_i[j].winner$ records the identifier of an elected frequent item.
$B_i[j].total$ records the total frequency of all items inserted into the bucket. 
$B_i[j].collision$ records the number of times that the inserted item differs from $B_i[j].winner$, called collisions.
Initially, all counters are set to $0$ and $B_i[j].winner$ is $null$.

\begin{figure}[htbp]
    % \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graphnew2.pdf}
    \vspace{-0.15in}
    \caption{The operations of the collision-sensible bucket.}
    \label{collision_sensible}
    \postfig
\end{figure}

\ppp{Insert an item (Algorithm \ref{alg:pseudo:bucketinsert}).} When inserting $e$ into bucket $B_i[j]$, we first decide whether the new item $e$ can replace the recorded item $B_i[j].winner$ as the elected frequent item. 
We perform the replacement only when $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$. 
The intuition of this condition is that, when too many collisions happen, $B_i[j].winner$ is not frequent enough to be kept and we can give other items a chance to be recorded.
% We will strictly explain the condition later.
After that, we check whether the recorded item $B_i[j].winner$ is $e$. If not, we increment the number of collisions $B_i[j].collision$ by $1$.
Finally, we increment $B_i[j].total$ by $1$.
From our replacement strategy, we have the following theorem:
\begin{theorem}
    The majority item that with a frequency more than half of $B_i[j].total$ must be the $B_i[j].winner$.
\end{theorem}


\vspace{-0.4cm}
\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.8}\selectfont
    \SetAlgoNoLine
    \caption{Insertion of Collision-Sensible Bucket.}
    \label{alg:pseudo:bucketinsert}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{InsertToBucket}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e, B_i[j]$}}{
            
        \If{$B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$}{ 
            $B_i[j].winner\gets e$ \Comment{Item replacement}
        }
                            % \Comment{Update counters}
                            
        \If{$B_i[j].winner\neq e$}{
            $B_i[j].collision\gets B_i[j].collision+1$
        }
        $B_i[j].total\gets B_i[j].total+1$
    }
\end{algorithm}
\vspace{-0.6cm}
\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.8}\selectfont
    \SetAlgoNoLine
    \caption{Query of Collision-Sensible Bucket.}
    \label{alg:pseudo:bucketquery}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{QueryBucket}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e, B_i[j]$}}{
        % $InsertionSuccess\gets False$
        
            \eIf{$B_i[j].winner=e$}{
                $Freq\gets  B_i[j].total-B_i[j].collision$
                
            }{
                $Freq\gets  B_i[j].collision$
                
            }
            $MaxError\gets B_i[j].collision$
            
        \Return{$\langle Freq, MaxError\rangle $}
    }
\end{algorithm}
\vspace{-0.4cm}

\ppp{Query an item with error feedback (Algorithm \ref{alg:pseudo:bucketquery}). } When querying the frequency of $e$ in bucket $B_i[j]$, we check whether the recorded winner $B_i[j].winner$ is $e$. If so, we report that the estimated frequency is $B_i[j].total-B_i[j].collision$. Otherwise, the estimated frequency is $B_i[j].collision$. In both cases, the maximum possible error is $B_i[j].collision$ and the estimated frequency is guaranteed to be no less than the true frequency.
The above query algorithm is based on the following theorem:
% Let $T$ and $C$ denote $B_i[j].total$ and $B_i[j].collision$ respectively, we have
\begin{theorem} The frequency of the winner is at most $B_i[j].total-B_i[j].collision$ and it is at least $B_i[j].total-2\cdot B_i[j].collision$. The frequency of any item other than the winner is at most $B_i[j].collision$.
\end{theorem}


\ppp{Lock the bucket to control the error.} When the maximum possible error (\ie, the number of collisions $B_i[j].collision$) reaches a threshold $\lambda_i$, to control the error, we lock the bucket, which means we only allow $B_i[j].winner$ to insert so that we can avoid more collisions. 
The other items will be inserted to other buckets in the next layer. 
We hope that the bucket will not be locked as far as possible, so as to reduce additional time and space overhead.
Before a bucket is locked, we have the following theorem:
\begin{theorem} 
    \label{alg:theorem:collision}
    $B_i[j].collision$ is no greater than the total frequency of all items except for the most frequent item.
\end{theorem}
\ppp{Bounded lock probability for any item.} Base on Theorem \ref{alg:theorem:collision}, the bucket can ensure that, when we know that an arbitrarily frequent item will be inserted to the bucket, whatever its arriving time, the probability of the bucket being locked is small and bounded.
This is the key point that our algorithm can achieve better theoretical complexity in both time and space (detailed in Section \ref{sec:math}).
When we lock the bucket, some items will be inserted into the next layer. We use the next technique to handle these items.




\presub
\subsection{Technique II: Double Exponential Control} \postsub
\label{subsec:alg:Standard}



In this part, we show how to organize and leverage collision-sensible buckets to accurately control the error of every item.
% \wyh{Then, we show how to combine these buckets and set thresholds to control the error of every item to the user-defined threshold in Section.}
% We present Double Exponential Control technique to handle all items with large error boundaries.
As mentioned in Section \ref{subsec:alg:struct}, \anamelong{} has multiple layers, and each layer has a number of buckets.
Every collision-sensible bucket in layer $i$ will not be locked until the error boundary reaches $\lambda_i$.
The size of each layer decreases $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and the error threshold of each layer also decreases $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$.
An ideal case is that the amount of items entering each layer decreases much faster than $w_i$ and $\lambda_i$. But it is not easy to reach the ideal case.
Now, we fully introduce the Double Exponential Control starting from the operations of \anamelong{}: Insertion and Query.


\vspace{-0.2cm}
\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Insertion.}
    \label{alg:pseudo:Insertion:all}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        % $i\gets 1$ \Comment{Start finding first available bucket}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
                        
            \If{$(B_i[j].collision < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0)$}{
                % \Comment{Stop at the first available bucket}
                $InsertToBucket(e, B_i[j])$
                
                \textbf{break} 
            }
            % $i\gets i+1$ 
            % \Comment{Go to next layer}
        }
            % $j\gets h_i(e)$ 
            % \Comment{Start inserting $e$ into bucket $B_i[j]$}
            % \If{$B_i[j].total=2\cdot B_i[j].collision$}{ 
            %     $B_i[j].winner\gets e$ \Comment{Perform item replacement}
            % }
            %                     \Comment{Update counters}
                                
            % \If{$B_i[j].winner\neq e$}{
            %     $B_i[j].collision\gets B_i[j].collision+1$
            % }
            % $B_i[j].total\gets B_i[j].total+1$
            
            % $B_i[j].unbias\gets B_i[j].unbias+S(e)$
    
    
    }
\end{algorithm}
\vspace{-0.2cm}


\ppp{Insertion (Algorithm \ref{alg:pseudo:Insertion:all}).} 
%
We insert an item $e$ into \anamelong{} by two steps, finding an available bucket and insert the item to it. 
For the first step, we start from the first layer and hash $e$ into a random bucket of this layer, called \textit{mapped bucket} ($B_i[j], j=h_i(e), i=1$). 
Then we check whether $B_i[j]$ is an available bucket, where $e$ will not incur collisions to make the error greater than $\lambda_i$ (\ie, the error threshold of this layer).
The mapped bucket is available if any of the following three conditions holds: 
\vspace{-0.1cm}
\begin{itemize}[leftmargin=*]
    \item $B_i[j].collision < \floor{\lambda_i}$, which means the maximum possible error of this bucket is tolerable.
    \item $B_i[j].winner=e$, which means $e$ will not incur collision.
    \item $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$, which means we can replace the $B_i[j].winner$ by $e$.
\end{itemize}
\vspace{-0.1cm}
% \textit{(i)} $B_i[j].winner=e$, which means $e$ is an unlimited item in this bucket; 
% 2) $B_i[j].low=0$, which means the new item $e$ can replace the old item $B_i[j].winner$; 
% \textit{(ii)} $\frac{1}{2}(B_i[j].total-B_i[j].low)< \floor{\lambda_i}$, which means the error of this bucket is tolerable.
If the mapped bucket is available, we insert $e$ into the bucket and completed the insertion.
Otherwise, when the bucket is not available, we keep finding an available bucket in the next layer until the last layer.
In a few cases, the mapped bucket in the last layer is unavailable and we insert $e$ to a small stash to handle these items. We will detail the stash later.

\vspace{-0.3cm}

\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Query Frequency.}
    \label{alg:pseudo:query:all}
    % \KwIn{an item $e$}
    \SetKwFunction{FMain}{QueryFrequency}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $ Freq\gets 0$  \Comment{Frequency Estimator}
        
        % $ Ub\gets 0$ \Comment{Unbiased Estimator}
        
        $ MaxError\gets 0$ \Comment{Maximum Possible Error}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the bucket}
            
            \eIf{$B_i[j].winner=e$}{
                $Freq\gets Freq + B_i[j].total-B_i[j].collision$
                
                % $Ub\gets Ub+B_i[j].unbias$
            }{
                $Freq\gets Freq + B_i[j].collision$
                
                % $Ub\gets Ub+B_i[j].unbias-B_i[j].low\cdot S(B_i[j].winner)$
            }
            
            
            $MaxError\gets MaxError + B_i[j].collision$
            
                        
            \If{$(B_i[j].collision  < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0)$}{
                \textbf{break} \Comment{Stop collecting frequency}
            }
        }
        
        \Return{$\langle Freq, MaxError\rangle$}
    }
\end{algorithm}

\vspace{-0.3cm}

\ppp{Query (Algorithm \ref{alg:pseudo:query:all}).} When query the frequency of an arbitrary item $e$, \anamelong{} reports an over-estimated frequency with its maximal possible error.
As every time inserting an item, we only insert it into one mapped bucket.
When estimating the total frequency, we just add up the frequencies in these mapped buckets. 
Starting from the first layer, we access the mapped bucket $B_i[j], j=h_i(e)$ layer by layer and add up the estimated frequencies and the maximum possible errors in these buckets, respectively. We stop at layer $B_i$ if a mapped bucket in layer $B_i$ is available for $e$ (\ie, $B_i[j].collision  < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$), because in this case, $e$ must never be inserted to its following layers.
We do not access all layers because if a mapped bucket in layer $B_i$ is available for $e$ (\ie, $B_i[j].collision  < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$), $e$ must never be inserted to its following layers and we stop at the $i$-th layer.
In a few cases, we do not stop at the last layer. We estimate the frequency in the stash and add it to the total frequency.


\ppp{Stash for Emergency:}
In rare cases, the last layer is not available for some items, so we put a special \textit{stash} after the last layer to store these items. The size of the stash can be regarded as a small constant. In our experiments, the stash does not have sensible impact on the experimental results, but it is important for our mathematical complexity analysis.
We choose the classic SpaceSaving \cite{spacesaving} algorithm as our stash structure (We can also use others, including Misra–Gries algorithm \cite{misra1982finding} and Frequent \cite{demaine2002frequency}). 
When there exists one item's estimation error is greater than $\lambda$, we call it algorithm failure.
Assuming that the probability of algorithm failure is $\delta$, \eg, $\delta=10^{-100}$. According to Theorem \ref{theo:main}, we set the size of SpaceSaving to $\Delta_2 \ln(\frac{1}{\delta})$.
Although we cannot guarantee that there is no algorithm failure, we can make it small enough and become tolerable with small cost, \ie, $O(\ln(\frac{1}{\delta}))$.
$\delta$ can be small enough to be less than the probability of hardware platform failure/damage (\eg, $\delta=10^{-100}$).


\presub
\subsection{More Functions of \anamelong{}} \postsub
\label{extend}
% \subsection{\anamelong{} for Weighted-Counting and Unbiased Estimation} \postsub

Our \anamelong{} has good versatility for various scenarios. We take the two most concernful tasks as examples, weighted counting and unbiased frequency estimation. We only introduce the key idea of how to achieve them.

\ppp{Weighted Counting.} The extended Weighted TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting an item $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting item $e$ for $w_e$ times in \anamelong{}. 
\anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 
% \wyh{ Due to space limitations, we leave the detailed \anamesum{} algorithm to the reader, which is not the primary focus of this paper.}

\ppp{Unbiased Frequency Estimation.} 
Rather than guaranteeing one-side error\footnote{The estimations from \anamelong{} must be no less than the true frequency}, we can extend \anamelong{} to provide the unbiased estimated frequency whose expected value is the true frequency.
We only introduce how to provide unbiased frequencies in one Collision-Sensible Bucket.
It can be directly extended to the entire algorithm.
To provide unbiased estimation, for each Collision-Sensible Bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. Initially, $B_i[j].unbias$ is $0$. For each item $e$ to be inserted, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping items to $\{+1, -1\}$ randomly. 
When queried item $e$, a simple but correct approach is to report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency. That is because $E[S(e)\cdot B_i[j].unbias]=E[f(e)]+\sum_{x\in U \setminus {e}} E[S(x)]\cdot E[S(e)f(x)]=f(e)$, where $U$ is the universe of all items. But in this case, we cannot sense the error and control it below $B_i[j].collision$.
Actually, we can subtract the frequency of $B_i[j].winner$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{winner}\big)$, where $F_{winner}=S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].collision)$.
In this case, the error boundary is $2\cdot B_i[j].collision$.


% \ppp{Insertion (Algorithm \ref{?}).}
% In the task of SUM (Defined in Section \ref{??}), each inserted item includes an identifier $e$ and weight $w_e (w_e>0)$.
% The insertion of \anamesum{} is similar to inserting $e$ by \anamecount{} for $w_e$ times.
% Let variable $W$ represent the remaining weight to be inserted. Its initial value is $w_e$. Every time we find an available bucket, we try to insert into it. First, we calculate how much weight (denoted as $W_0$) can be inserted into the current bucket at most. The $W_0$ is the minimum value of the remaining weight ($W$) and the maximum weight that the bucket can hold $\floor{\lambda_i}-B_i[j].collision$ before being locked. 
% Next, we insert $e$ with weight $W_0$ to the bucket directly.
% We add up the total items by $W_0$ and then add up the collision number if needed.
% If the item replacement is triggered, we replace the item and correct the number of collisions to $B_i[j].total-B_i[j].collision$.

% % similar to xxx to insert w0 into the bucket. Next, continue to find the next feasible bucket for insertion until the frequency W to be inserted is equal to 0.

% \ppp{Query.}
% The query asks the total weight of an given item identifier $e$. 
% The query of \anamesum{} is the same as that of \anamecount{}.

% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Insertion in Sum Task}
%     \KwIn{an item $e$ and its weight $w_e$}
%     \SetKwFunction{FMain}{Insert???}
%     % \SetKwProg{Fn}{Procedure}{:}{}
%     % \Fn{\FMain{$e, w_e$}}{
            
%         $W\gets w_e$ \Comment{The total amount to be inserted}
        
%         \For{Layer $i=1,2,\dots, d$}
%         {
%             $j\gets h_i(e)$  \Comment{Locate the bucket $B_i[j]$}
                        
%             \If{$(B_i[j].collision < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].total- 2\cdot B_i[j].collision\leqslant 0)$}{
                
%                 \If{$B_i[j].winner = null$}{ 
%                     $B_i[j].winner\gets e$ 
%                 }
%                                             \Comment{The amount to be inserted into this bucket}
                                            
%                 $W_0\gets min(W, \floor{\lambda_i}-B_i[j].collision)$
                
%                 $W\gets W-W_0$
                
%                 $B_i[j].total\gets B_i[j].total+W_0$ 
                
%                 \If{$B_i[j].winner\neq e$}{
%                     $B_i[j].collision\gets B_i[j].collision+W_0$
%                 }
                
%                 \If{$B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$}{
%                     $B_i[j].winner\gets e$ \Comment{Item replacement}
                    
%                     $B_i[j].collision\gets B_i[j].total-B_i[j].collision$
%                 }
%                 \If{$W = 0$}{
%                     \textbf{break}
%                 }
%             }
%         }
        
%     % }
% \end{algorithm}



% \presub
% \subsection{\anamelong{} for Unbiased Estimation} \postsub
% \label{}


% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Unbiased Estimation in Collision-Sensible Bucket}
%     \label{alg:pseudo:bucketinsert}
%     % \KwIn{an item $e$}
%     \SetKwFunction{FMain}{InsertToBucket}
%     \SetKwProg{Fn}{Procedure}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         $B_i[j].unbias\gets B_i[j].unbias+S(e)$
        
%         \If{$B_i[j].total- 2\cdot B_i[j].collision\leqslant 0$}{ 
%             $B_i[j].winner\gets e$ \Comment{Item replacement}
%         }
%                             % \Comment{Update counters}
%         \If{$B_i[j].winner\neq e$}{
%             $B_i[j].collision\gets B_i[j].collision+1$
%         }
%         $B_i[j].total\gets B_i[j].total+1$
%     }
    
%     \SetKwFunction{FMain}{QueryBucket}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         % $InsertionSuccess\gets False$
            
%             \eIf{$B_i[j].winner=e$}{
%                 $UbFreq\gets  S(e)\cdot B_i[j].unbias$
                
%             }{
%                 $UbFreq\gets   S(e)\cdot \big(B_i[j].unbias-S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].collision)\big)$
                
%             }
            
%             $MaxError\gets 2\cdot B_i[j].collision$
            
%         \Return{$\langle UbFreq, MaxError\rangle $}
%     }
% \end{algorithm}


% The \anamelong{} introduced above provides an estimated frequency that must be greater than the true frequency. In this part, we provide an unbiased frequency whose expected value is equal to the true frequency. We only introduce how to provide unbiased frequencies in one Collision-Sensible Bucket. It can be directly extended to the entire algorithm. To provide unbiased estimation, for each Collision-Sensible Bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. The initial value of $B_i[j].unbias$ is $0$.

% \ppp{Insertion.} For each item $e$, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping items to $\{+1, -1\}$ randomly. Then we update the bucket in the same way as the basic version.

% \ppp{Query.} Given the queried item $e$. If it is $B_i[j].winner$, we report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency ($UbFreq$). Otherwise, we subtract the frequency of $B_i[j].winner$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{winner}\big)$, where $F_{winner}=S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].collision)$.
% Here we explain why the result is unbiased. Let $U$ be all items that are inserted to this bucket, and let $f(\cdot)$ denote the frequency in this bucket.
% The $B_i[j].unbias$ equals to $\sum_{x\in U} S(x)f(x)$. 
% For the first case that $e=B_i[j].winner$, we have $E[S(e)\cdot B_i[j].unbias]=E[S^2(e)f(e)]+\sum_{x\in U \setminus {e}} E[S(e)S(x)f(x)]$. As $E[S(e)S(x)f(x)]=E[S(x)]E[S(s)f(x)]$ and $E[S(x)]=0$, we have $E[S(e)\cdot B_i[j].unbias]= f(e)$. Similarly, we can proof that the result in the second case ($e\neq B_i[j].winner$) is unbiased. In this case, we substract $F_{winner}$ from $B_i[j].unbias$ is to reduce the variance. 
% Particularly, the maximum possible error is $2\cdot B_i[j].collision$, which is slightly different from the basic algorithm with one-side error.

% \presub
% \subsection{Protective Measure for Emergency} \postsub




% \presub
% \subsection{Practical Configurations and Discussions} \postsub

% Given a goal, we estimate the resources required.

% Given resources, we estimate the best performance.

% strength and weakness?


==> vldb/Body/algo_v4.tex <==

\newcommand\floor[1]{{\lfloor #1 \rfloor}}

\newcommand{\hit}{hit}
\newcommand{\miss}{miss}

\begin{table} [!ht]
\begin{center}
\vspace{-0.3cm}
\caption{Symbols.}
\vspace{-0.2cm}
\label{table:symbol}
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}&\textbf{Meaning}\\
\hline
% $\mathcal{S}$&a data stream\\
% \hline
$N$ & the total number of packets\\
\hline
% $e_t$& $t^{th}$ flow in $\mathcal{S}$\\
% \hline
% $f_t$&frequency of $e_t$\\
% \hline
$d$&the number of layers\\
\hline
% $B_i$&the $i$-th layer\\
% \hline
$w_i$&the number of buckets in the $i$-th layer\\
\hline
$R_w$& the proportion that $w_i$ decreases\\
\hline
$\Lambda$& the user-defined error threshold\\
\hline
$\Lambda_i$&the warning threshold in the $i$-th layer\\
\hline
$\lambda_i$&the error threshold in the $i$-th layer\\
\hline
$R_\lambda$& the proportion that $\lambda_i$ decreases\\
\hline
$h_i(.)$& hash function in the $i$-th layer\\
% \hline
% $S(.)$& sign hash function\\
\hline
$B_i[j]$& the $j$-th bucket of the $i$-th layer\\
\hline
$B_i[j].\hit $& the number of hits in $B_i[j]$\\
\hline
% $B_i[j].unbias$ & the unbiased estimator in $B_i[j]$\\
% \hline
$B_i[j].\miss{}$\;\,& the number of \miss{}es in $B_i[j]$\\
\hline
$B_i[j].winner$\;\;& the recorded frequent flow in $B_i[j]$\\
\hline
\end{tabular}
\vspace{-0.05in}
\end{center}
\end{table}
%\vspace{-0.05in}


% 3.1 Rationale
% 3.2 key 
%  data
%  insertion
%  query
% 3.3 key techniques
%  1.
%  2.
% 3.4 dis

% 3.1 rationale
% 3.2 key technique1: \miss{} sensible bucket
%     过渡
% 3.3 key technique2: double exp.. control
% 3.4 Weighted counting version
% 3.5 Unbiased version
% 3.6 handling the worst case


% \presec
%这个 Trusty Sketch 必须分开
\section{The Trusty Sketch} \postsec
\label{SEC:Algorithm}

In this section, we present \anamelong{}. 
After showing the data structure, we show how one bucket senses the error in Section \ref{subsec:alg:struct}. 
% After showing the data structure, we first show how one bucket senses \miss{}es and errors in Section \ref{subsec:alg:struct}. 
Then, we show how to organize these buckets and set appropriate thresholds to control the error of every flow under the user-defined threshold in Section \ref{subsec:alg:Standard}.
Symbols frequently used are listed in Table \ref{table:symbol}.
% Last, we extend \anamelong{} to support weighted-counting task and the unbiased estimation in Section \ref{extend}.
% Essential symbols used in this paper and their meanings are listed in Table \ref{table:symbol}.


%We present \anamelong{} in this section. First, we present our rationale and the data structure of \anamelong{}. Then we present our two key techniques in the following two sections \ref{?}-\ref{?}. 
%Finally, we extend \anamelong{} to support weighted-counting task and the unbiased estimation.
% in Section \ref{?} and \ref{?}.
% Finally, 
% In this section, we present our Versatile Sketch (\anamelong{}).
% First, we describe the data structure (Section Section \ref{subsec:alg:struct}) and the standard operations of \anamelong{} including the interval estimation (Section \ref{subsec:alg:Standard}).
% Then, we show its extra operations which are used for distributed systems and incremental deployment (Section \ref{subsec:alg:extra}).
% For easy understanding, the \anamelong{} presented above is a simple version. In the final Section \ref{subsec:alg:scalability}, we show more features that \anamelong{} can achieve and discuss more design choices.
% To clarify \anamelong{}, we list essential symbols used in this paper and their meanings in Table \ref{table:symbol}.

\ppp{Problem Definition:}
Given an user-defined error threshold $\Lambda$, our goal is to control the absolute error of every flow's estimated frequency below $\Lambda$ ($\Lambda$ is small):
$$\widehat{f_e}-\Lambda\leqslant f_e\leqslant \widehat{f_e},\ \forall\ flow\ e,$$where $\widehat{f_e}$ is the estimated frequency and $f_e$ is the true frequency.

%不重复展示
\ppp{Rationale:}
The \anamelong{} consists of multiple layers, and each layer has an increasing warning threshold. These thresholds are at most $\Lambda$.
When a flow’s error boundary (\ie, the maximum possible error) reaches the warning threshold in one layer, it will be inserted to the next layer. There are two key challenges: (1) Accurately Sensing. Find high-risk flows whose error bounds reach the warning threshold; (2) Effectively Control. Reduce high-risk flows efficiently//effectively with small space and a small number of layers.
We devise the Error-Sensing technique (Sec. \ref{subsec:alg:tech1}) and the Double Exponential Composition (Sec. \ref{subsec:alg:tech2}) to tackle above two challenges respectively.
% To tackle the first challenge, we devise the Error-Sensing technique. To tackle the second challenge, we devise the Double Exponential Control technique based on a multi-layer structure.

\begin{figure}[htbp]
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph1V2.pdf}
    \vspace{-0.15in}
    \caption{The structure of \anamelong{}.}
    \label{fig:algo:structure}
    \postfig
\end{figure}

\presub
\subsection{Data Structure} \postsub
\label{sec:algo:structure}



As shown in Figure \ref{fig:algo:structure}, the data structure of \anamelong{} consists of $d$ layers, $B_1,$ $B_2,$ $\dots,$ $B_d$. The $i$-th layer $B_i$ is an array consists of $w_i$ \textit{error-sensible buckets}, denoted as $B_i[1],$ $B_i[2],$ $\dots,$ $B_i[w_i]$. 
The size of layer $B_i$, denoted as $w_i$, decreases in proportion to $R_{w} (R_{w}>1)$ as $i$ increases.
Each layer $B_i$ has an error threshold, denoted as $\lambda_i$. $\lambda_i$ decreases in proportion to $R_{\lambda} (R_{\lambda}>1)$ as $i$ increases.
The warning threshold in layer $B_i$, denoted as $\Lambda_i$, is the sum of the error thresholds of the first $i$ layers, \ie, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i$ must be no more than user-defined threshold $\Lambda$.
Each layer is associated with a pair-wisely independent hash function $h_i(\cdot)$, which maps each flow (denoted by $e$) into a random bucket (the $j$-th bucket $B_i[j], j=h_i(e)$) uniformly.
% , \ie, $ w_i=\left\lceil\frac{W_0}{R_{w}^i}\right\rceil$.
% To control all errors below $\Lambda$, each layer has an increasing error warning threshold, denoted as $\Lambda_i$ ($\Lambda_i\leqslant \Lambda$) in the $i$-th layer.
% The difference between the warning thresholds in adjacent layers is the amount of error that one layer can accommodate.
% For the $i$-th layer, it has an error threshold  $\lambda_i=\Lambda_i-\Lambda_{i-1}$, which represents the maximum error it can accommodate.
% The error threshold $\lambda_i$ guarantees that the estimation error of any bucket in $i$-th layer is less than $\lambda_i$.
% In the i-th layer, we set the error threshold to $\lambda_i=\left\lfloor\frac{\Lambda}{R_{\lambda}^i}\right\rfloor$, which decrease in proportion to $R_{\lambda}=2$. 
% Therefore, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i\leqslant\Lambda$.
% $\Lambda_i$ and $\Lambda_{i-1}$ represents the amount of error that the $i$-th layer can accommodate.
% Each layer has an error threshold $\lambda_i$, where \anamelong{} can guarantee that the estimation error of $i$-th layer is less than $\floor{\lambda_i}$.

\ppp{Parameter Configurations:} 
Let $W$ denote the total number of buckets. We set $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$. 
In our proofs (Theorem \ref{theo:main}), we set $W=\frac{4(R_w R_\lambda)^{6}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, which is with large constant.
But based on our experimental results, we recommend to set $W=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, $R_w\in[2, 10]$, $R_l\in[2, 10]$, and $d\geqslant 7$.
When then memory size is given without given $\Lambda$, we set 
\begin{align}
    \Lambda=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{W}
    \label{formula:setLambda}
\end{align}








\presub
\subsection{Technique I: Error-Sensing} \postsub
\label{subsec:alg:tech1}
In this section, we present the \textit{Error-Sensing} technique, based on the error-sensible bucket.
The key idea is to bound the error by the number of "nays" when electing the most frequent flow.
As shown in Figure \ref{\miss{}_sensible}, the error-sensible bucket supports two operations: (1) insert a packet; (2) query of a flow for its estimated size and the error boundary.
%of a flow together with its maximum possible error.
% The structures of all error-sensible buckets are the same.
One error-sensible bucket $B_i[j]$ contains one flow ID $B_i[j].winner$ and two counters, $B_i[j].\hit$ and $B_i[j].\miss{}$.
$B_i[j].winner$ records the identifier of an elected frequent flow.
$B_i[j].\hit$ records the hit times and $B_i[j].\miss{}$ records the miss times (detailed later).
% total frequency of all flows inserted into the bucket. 
% $B_i[j].\miss{}$ records the number of times that the inserted flow differs from $B_i[j].winner$, called \miss{}es.
Initially, all counters are set to $0$ and $B_i[j].winner$ is $null$.

\begin{figure}[htbp]
    % \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph2V2.pdf}
    \vspace{-0.15in}
    \caption{The operations of the error-sensible bucket.}
    \label{\miss{}_sensible}
    \postfig
\end{figure}

\ppp{Insert a packet (Algorithm \ref{alg:pseudo:bucketinsert}).} When inserting a packet with flow ID $e$ into bucket $B_i[j]$, we first decide whether the new flow $e$ can replace the recorded flow $B_i[j].winner$ as the elected frequent flow. 
When $B_i[j].\hit = B_i[j].\miss{}$, we replace the recorded flow.
The intuition of this condition is that, when too many \miss{}es happen, $B_i[j].winner$ is not frequent enough to be kept and we can give other flows a chance to be recorded.
% We will strictly explain the condition later.
After that, we check whether the recorded flow $B_i[j].winner$ is $e$. If not, we increment the number of \miss{}es $B_i[j].\miss{}$ by $1$.
Otherwise, we increment $B_i[j].\hit{}$ by $1$.
% From our replacement strategy, we have the following theorem:
% \begin{theorem}
%     The majority flow that with a frequency more than half of $B_i[j].total$ must be the $B_i[j].winner$.
% \end{theorem}


\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.8}\selectfont
    \SetAlgoNoLine
    \caption{Insertion of Error-Sensible Bucket.}
    \label{alg:pseudo:bucketinsert}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{InsertToBucket}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e, B_i[j]$}}{
            
        \If{$B_i[j].\hit = B_i[j].\miss{}$}{ 
            $B_i[j].winner\gets e$ \Comment{flow replacement}
        }
                            % \Comment{Update counters}
                            
        \eIf{$B_i[j].winner\neq e$}{
            $B_i[j].\miss{}\gets B_i[j].\miss{}+1$
        }{
            $B_i[j].\hit\gets B_i[j].\hit+1$
        }
    }
\end{algorithm}
\vspace{-0.6cm}
\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.8}\selectfont
    \SetAlgoNoLine
    \caption{Query of Error-Sensible Bucket.}
    \label{alg:pseudo:bucketquery}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{QueryBucket}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e, B_i[j]$}}{
        % $InsertionSuccess\gets False$
        
            \eIf{$B_i[j].winner=e$}{
                $Freq\gets  B_i[j].\hit{}$
                
            }{
                $Freq\gets  B_i[j].\miss{}$
                
            }
            $MaxError\gets B_i[j].\miss{}$
            
        \Return{$\langle Freq, MaxError\rangle $}
    }
\end{algorithm}

\ppp{Query a flow with error feedback (Algorithm \ref{alg:pseudo:bucketquery}). } When querying the frequency of $e$ in bucket $B_i[j]$, we check whether the recorded winner $B_i[j].winner$ is $e$. If so, we report that the estimated frequency is $B_i[j].\hit{}$. Otherwise, the estimated frequency is $B_i[j].\miss{}$. In both cases, the maximum possible error is $B_i[j].\miss{}$ and the estimated frequency is guaranteed to be no less than the true frequency.
The frequency of $B_i[j].winner$ is at least  $B_i[j].\hit-B_i[j].\miss$ because $.\hit-\miss$ increments by 1 only when $B_i[j].winner$ comes.
% The above query algorithm is based on the following theorem:
% % Let $T$ and $C$ denote $B_i[j].total$ and $B_i[j].\miss{}$ respectively, we have
% \begin{theorem} The frequency of the winner is at most $B_i[j].\hit{}$ and it is at least $B_i[j].total-2\cdot B_i[j].\miss{}$. The frequency of any flow other than the winner is at most $B_i[j].\miss{}$.
% \end{theorem}


\ppp{Lock the bucket to control the error.} When the maximum possible error (\ie, the number of \miss{}es $B_i[j].\miss{}$) reaches a threshold $\lambda_i$, in order to control the error, we lock current bucket.
When we lock the bucket, we we only allow $B_i[j].winner$ to insert because it does not incur more \miss{}es. 
The other flows will be inserted to other buckets in the next layer. 


\begin{figure}[htbp]
    % \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph3V2.pdf}
    \vspace{-0.15in}
    \caption{An example of the error-sensible bucket. The packets "c,a,b,a,a,b,a,a" are inserted into a bucket in turn, and their estimation results are shown in the right.}
    \label{\miss{}_sensible}
    \postfig
\end{figure}

\presub
\subsection{Technique II: Double Exponential Control} \postsub
\label{subsec:alg:tech2}



In this part, we show how to organize and leverage error-sensible buckets to accurately control the error of every flow.
% \wyh{Then, we show how to combine these buckets and set thresholds to control the error of every flow to the user-defined threshold in Section.}
% We present Double Exponential Control technique to handle all flows with large error boundaries.
As mentioned in Section \ref{subsec:alg:struct}, \anamelong{} has multiple layers, and each layer has a number of buckets.
Every error-sensible bucket in layer $i$ will not be locked until the error boundary reaches $\lambda_i$.
The size of each layer decreases $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and the error threshold of each layer also decreases $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$.
An ideal case is that the amount of flows entering each layer decreases much faster than $w_i$ and $\lambda_i$. But it is not easy to reach the ideal case.
Now, we fully introduce the Double Exponential Control starting from the operations of \anamelong{}: Insertion and Query.


\vspace{-0.2cm}
\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Insertion.}
    \label{alg:pseudo:Insertion:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        % $i\gets 1$ \Comment{Start finding first available bucket}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
                        
            \If{$(B_i[j].winner=e$ \textbf{or} $B_i[j].\miss{}  < \floor{\lambda_i}$ \textbf{or} $B_i[j].\hit{} = B_i[j].\miss{})$}{
                % \Comment{Stop at the first available bucket}
                $InsertToBucket(e, B_i[j])$
                
                \textbf{break} 
            }
            % $i\gets i+1$ 
            % \Comment{Go to next layer}
        }
            % $j\gets h_i(e)$ 
            % \Comment{Start inserting $e$ into bucket $B_i[j]$}
            % \If{$B_i[j].total=2\cdot B_i[j].\miss{}$}{ 
            %     $B_i[j].winner\gets e$ \Comment{Perform flow replacement}
            % }
            %                     \Comment{Update counters}
                                
            % \If{$B_i[j].winner\neq e$}{
            %     $B_i[j].\miss{}\gets B_i[j].\miss{}+1$
            % }
            % $B_i[j].total\gets B_i[j].total+1$
            
            % $B_i[j].unbias\gets B_i[j].unbias+S(e)$
    
    
    }
\end{algorithm}
\vspace{-0.2cm}


\ppp{Insertion (Algorithm \ref{alg:pseudo:Insertion:all}).} 
%
We insert a flow $e$ into \anamelong{} by two steps, finding an available bucket and insert the flow to it. 
For the first step, we start from the first layer and hash $e$ into a random bucket of this layer, called \textit{mapped bucket} ($B_i[j], j=h_i(e), i=1$). 
Then we check whether $B_i[j]$ is an available bucket, where $e$ will not incur \miss{}es to make the error greater than $\lambda_i$ (\ie, the error threshold of this layer).
The mapped bucket is available if any of the following three conditions holds: 
\vspace{-0.1cm}
\begin{itemize}[leftmargin=*]
    \item $B_i[j].winner=e$, which means $e$ will not incur \miss{}.
    \item $B_i[j].\miss{} < \floor{\lambda_i}$, which means the maximum possible error of this bucket is tolerable.
    \item $B_i[j].\hit{} = B_i[j].\miss{}$, which means we can replace the $B_i[j].winner$ by $e$.
\end{itemize}
\vspace{-0.1cm}
% \textit{(i)} $B_i[j].winner=e$, which means $e$ is an unlimited flow in this bucket; 
% 2) $B_i[j].low=0$, which means the new flow $e$ can replace the old flow $B_i[j].winner$; 
% \textit{(ii)} $\frac{1}{2}(B_i[j].total-B_i[j].low)< \floor{\lambda_i}$, which means the error of this bucket is tolerable.
If the mapped bucket is available, we insert $e$ into the bucket and completed the insertion.
Otherwise, when the bucket is not available, we keep finding an available bucket in the next layer until the last layer.
In a few cases, the mapped bucket in the last layer is unavailable. The insertion in the data plane is failed. We will discuss our emergency solution later.
% and we insert $e$ to a small stash to handle these flows. We will detail the stash later.


\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Query Frequency.}
    \label{alg:pseudo:query:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{QueryFrequency}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $ Freq\gets 0$  \Comment{Frequency Estimator}
        
        % $ Ub\gets 0$ \Comment{Unbiased Estimator}
        
        $ MaxError\gets 0$ \Comment{Maximum Possible Error}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the bucket}
            
            \eIf{$B_i[j].winner=e$}{
                $Freq\gets Freq + B_i[j].\hit{}$
                
                % $Ub\gets Ub+B_i[j].unbias$
            }{
                $Freq\gets Freq + B_i[j].\miss{}$
                
                % $Ub\gets Ub+B_i[j].unbias-B_i[j].low\cdot S(B_i[j].winner)$
            }
            
            
            $MaxError\gets MaxError + B_i[j].\miss{}$
            
                        
            \If{ $(B_i[j].winner=e$ \textbf{or} $B_i[j].\miss{}  < \floor{\lambda_i}$ \textbf{or} $B_i[j].\hit{} = B_i[j].\miss{})$}{
                \textbf{break} \Comment{Stop collecting frequency}
            }
        }
        
        \Return{$\langle Freq, MaxError\rangle$}
    }
\end{algorithm}

% \vspace{-0.3cm}

\ppp{Query (Algorithm \ref{alg:pseudo:query:all}).} When query the frequency of an arbitrary flow $e$, \anamelong{} reports an over-estimated frequency with its maximal possible error.
As every time inserting a flow, we only insert it into one mapped bucket.
When estimating the total frequency, we just add up the frequencies in these mapped buckets. 
Starting from the first layer, we access the mapped bucket $B_i[j], j=h_i(e)$ layer by layer and add up the estimated frequencies and the maximum possible errors in these buckets, respectively. We stop at layer $B_i$ if a mapped bucket in layer $B_i$ is available for $e$ (\ie, $B_i[j].winner=e$ \textbf{or} $B_i[j].\miss{}  < \floor{\lambda_i}$ \textbf{or} $B_i[j].\hit{} = B_i[j].\miss{}$), because in this case, $e$ must never be inserted to its following layers.
We do not access all layers because if a mapped bucket in layer $B_i$ is available for $e$, $e$ must never be inserted to its following layers and we stop at the $i$-th layer.
% In a few cases, we do not stop at the last layer. We estimate the frequency in the stash and add it to the total frequency.


\ppp{Emergency Solution:}
In rare cases (\eg, probability $\delta=0.1^{10}$), we failed to insert a packet in the \anamelong{}, \ie, a packet reaches the last layer and meets an unavailable bucket. 
When \anamelong{} is deployed on the switch (P4 platform), it is placed on the data plane. We just send these small amount of packets to the control plane, and use the CPU in control plane to count the flow size with no error. We can also use a small additional data structure like a hash table or a SpaceSaving \cite{spacesaving}. 
We implemented emergency solutions on CPU, FPGA and P4 to prove its feasibility. But we did not add it to our main accuracy evaluation (Sec. \ref{}), in order to clearly show \anamelong{} it self.
% \ppp{Stash for Emergency:}
% In rare cases, the last layer is not available for some flows, so we put a special \textit{stash} after the last layer to store these flows. The size of the stash can be regarded as a small constant. In our experiments, the stash does not have sensible impact on the experimental results, but it is important for our mathematical complexity analysis.
% We choose the classic SpaceSaving \cite{spacesaving} algorithm as our stash structure (We can also use others, including Misra–Gries algorithm \cite{misra1982finding} and Frequent \cite{demaine2002frequency}). 
% When there exists one flow's estimation error is greater than $\lambda$, we call it algorithm failure.
% Assuming that the probability of algorithm failure is $\delta$, \eg, $\delta=10^{-100}$. According to Theorem \ref{theo:main}, we set the size of SpaceSaving to $\Delta_2 \ln(\frac{1}{\delta})$.
% Although we cannot guarantee that there is no algorithm failure, we can make it small enough and become tolerable with small cost, \ie, $O(\ln(\frac{1}{\delta}))$.
% $\delta$ can be small enough to be less than the probability of hardware platform failure/damage (\eg, $\delta=10^{-100}$).




\presub
\subsection{Extensions} \postsub

\subsubsection{Freely turning the accuracy of priority flows.}


The extended Priority TrustySketch (\anamesum{} for short) can adjust the estimation accuracy of any flow. We can improve the accuracy of a high-priority flow (\eg, a flow with high SLA requirement) by giving it a weight. The weight of flow $e_i$, denoted as $w_i$, is an user-defined positive integer and it can improve the guaranteed accuracy from the old $\Lambda$ to $\lfloor \frac{\Lambda}{w_i} \rfloor$. Therefore, when $w_i$ is set to $\lfloor w_i \rfloor$, the estimation of flow $e_i$ must be correct.
The key idea of inserting a packet $e_i$ with weight $w_i$ is to insert a packet for $w_i$ times by common insert operation. 
Instead of spending $w_i$ times of time, we can achieve the same insertion speed as usual by some reasonable modifications. 
Increasing the accuracy of partial flow will consume more memory. For example, if we reduce the error of 10\% flow by 50\%, we need 10\% more memory. 
% The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 
% The new \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. 

% The extended priority TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 


\subsubsection{Improving the overall accuracy by a mice filter.}
After achieving good theoretical results, the memory efficiency of \anamelong{} can be further optimized in practice.
% In a switch, the memory reserved for the measurement function is scarce 
The first layer of \anamelong{} is the largest layer and it takes more than $50\%$ space of the whole \anamelong{}. But the first layer is in efficient when there are quite a few mice flows in the traffic. The mice flows will increment the 'miss' counters sharply and lock most buckets in the first layers. In this case, many buckets are wasted to record the mice flows. 

To tackle the mice flows, we replace the first layer with a small mice-flow filter and still controlling the error well. Specifically, inspired by CU \cite{estan2002cusketch}, the filter consists of two arrays ($F_1[]$ and $F_2[]$) and each array has $\frac{1}{2} w_1$ $L$-bit counters. For every flow ID $e$, we use two hash functions $h_1^{(1)}(.)$ and $h_1^{(2)}(.)$ to select two mapped counters $C_1=F_1[h_1^{(1)}(e)]$ and $C_2=F_1[h_1^{(1)}(e)]$. To insert a packet with flow ID $e$, if 
any of its two mapped counters is less than $\lambda_1$, we regard it as a mice flow. For a mice flow, we drop it and increment the minimal mapped counter(s) less than $\lambda_1$ by one. Otherwise, when both mapped counters equal to $\lambda_1$, we regard it as a non-mice flow, and pass the packet to the second layer.
In practice, 8-bit counters are sufficient for the filter. Compared to a layer composed of 72-bit error-sensible buckets, the filter can reduce the space cost of layer-1 nearly $10$ times while incurring small controllable errors. The overall accuracy will be significantly improved when we move the space saved by the filter to the other layers. But we cannot replace other layers by the filter because the filter cannot estimate elephant flows well.

% \presub
% \subsection{More Functions of \anamelong{}} \postsub
% \label{extend}


% Our \anamelong{} has good versatility for various scenarios. We take the two most concernful tasks as examples, weighted counting and unbiased frequency estimation. We only introduce the key idea of how to achieve them.

% \ppp{Weighted Counting.} The extended Weighted TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 

\presub
\subsection{Discussion} \postsub

We shortly review the design and discuss the design choices.
In \anamelong{}, we devise Error-Sensible buckets that can sense the error of both mice and elephant flows, and combine them into a multi-layer structure to eliminate the flows at the risk of losing control.

\noindent\textbf{How we design the error-sensible bucket?} We try to design the most simple error-sensible structure so that it can implemented in various platforms, especially the programmable switch. The bucket has only two counters and one ID, which can hardly be further simplified.

\noindent\textbf{Compared with a simple counter, what is the disadvantage of the error-sensible bucket as a basic unit?} The recorded ID consumes a lot of space, and the insertion becomes more complex and time-consuming. These costs are worth paying, in order to get the ability to sense the error. The time consumption is not significant because the main cost lies in memory access and hash calculation, rather than the insertion within the basic unit. 
Based on the ability to sense the error, we devise the Double Exponential Composition technique, which not only covers the disadvantages of the error-sensible bucket but also performs much better than existing sketches.

\noindent\textbf{What is the difference of the multi-layer structure of \anamelong{} and the traditional multi-layer structure?} The key difference is that we have no copy and can quickly reduce flows layer by layer.
Existing sketches, including CM, CU, and Count, have multi-layers and may update multiple counters when inserting one packet, which is called copy. We only update one counter for each packet, which makes \anamelong{} accurate and memory-efficient.
Our multi-layer buckets can reduce both elephant flows and mice flows. In contrast, traditional methods \cite{coldfilter,lu2008counterbraids} insert all remaining flows to the next layer when a counter is large, which method will insert most elephant flows to the next layer and cannot reduce elephant flows effectively.
Thanks to efficiently reducing flows, every packet only needs to access $1\sim 2$ layers in average, which makes \anamelong{} fast. Never seen before, \anamelong{} can reduce flows at the double exponential speed (proved mathematically in Sec \ref{?} and experimentally in Sec \ref{?}).


% Before a bucket is locked, we have the following theorem:
% \begin{theorem} 
%     \label{alg:theorem:\miss{}}
%     $B_i[j].\miss{}$ is no greater than the total frequency of all flows except for the most frequent flow.
% \end{theorem}
% \ppp{Bounded lock probability for any flow.} Base on Theorem \ref{alg:theorem:\miss{}}, the bucket can ensure that, when we know that an arbitrarily frequent flow will be inserted to the bucket, whatever its arriving time, the probability of the bucket being locked is small and bounded.
% This is the key point that our algorithm can achieve better theoretical complexity in both time and space (detailed in Section \ref{sec:math}).
% When we lock the bucket, some flows will be inserted into the next layer. We use the next technique to handle these flows.




% \wyh{ Due to space limitations, we leave the detailed \anamesum{} algorithm to the reader, which is not the primary focus of this paper.}

% \ppp{Unbiased Frequency Estimation.} 
% Rather than guaranteeing one-side error\footnote{The estimations from \anamelong{} must be no less than the true frequency}, we can extend \anamelong{} to provide the unbiased estimated frequency whose expected value is the true frequency.
% We only introduce how to provide unbiased frequencies in one Error-Sensible Bucket.
% It can be directly extended to the entire algorithm.
% To provide unbiased estimation, for each Error-Sensible Bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. Initially, $B_i[j].unbias$ is $0$. For each flow $e$ to be inserted, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. 
% When queried flow $e$, a simple but correct approach is to report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency. That is because $E[S(e)\cdot B_i[j].unbias]=E[f(e)]+\sum_{x\in U \setminus {e}} E[S(x)]\cdot E[S(e)f(x)]=f(e)$, where $U$ is the universe of all flows. But in this case, we cannot sense the error and control it below $B_i[j].\miss{}$.
% Actually, we can subtract the frequency of $B_i[j].winner$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{winner}\big)$, where $F_{winner}=S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})$.
% In this case, the error boundary is $2\cdot B_i[j].\miss{}$.


% \ppp{Insertion (Algorithm \ref{?}).}
% In the task of SUM (Defined in Section \ref{??}), each inserted flow includes an identifier $e$ and weight $w_e (w_e>0)$.
% The insertion of \anamesum{} is similar to inserting $e$ by \anamecount{} for $w_e$ times.
% Let variable $W$ represent the remaining weight to be inserted. Its initial value is $w_e$. Every time we find an available bucket, we try to insert into it. First, we calculate how much weight (denoted as $W_0$) can be inserted into the current bucket at most. The $W_0$ is the minimum value of the remaining weight ($W$) and the maximum weight that the bucket can hold $\floor{\lambda_i}-B_i[j].\miss{}$ before being locked. 
% Next, we insert $e$ with weight $W_0$ to the bucket directly.
% We add up the total flows by $W_0$ and then add up the \miss{} number if needed.
% If the flow replacement is triggered, we replace the flow and correct the number of \miss{}es to $B_i[j].\hit{}$.

% % similar to xxx to insert w0 into the bucket. Next, continue to find the next feasible bucket for insertion until the frequency W to be inserted is equal to 0.

% \ppp{Query.}
% The query asks the total weight of an given flow identifier $e$. 
% The query of \anamesum{} is the same as that of \anamecount{}.

% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Insertion in Sum Task}
%     \KwIn{a flow $e$ and its weight $w_e$}
%     \SetKwFunction{FMain}{Insert???}
%     % \SetKwProg{Fn}{Procedure}{:}{}
%     % \Fn{\FMain{$e, w_e$}}{
            
%         $W\gets w_e$ \Comment{The total amount to be inserted}
        
%         \For{Layer $i=1,2,\dots, d$}
%         {
%             $j\gets h_i(e)$  \Comment{Locate the bucket $B_i[j]$}
                        
%             \If{$(B_i[j].\miss{} < \floor{\lambda_i}$ \textbf{or} $B_i[j].winner=e$ \textbf{or} $B_i[j].\hit{} = B_i[j].\miss{})$}{
                
%                 \If{$B_i[j].winner = null$}{ 
%                     $B_i[j].winner\gets e$ 
%                 }
%                                             \Comment{The amount to be inserted into this bucket}
                                            
%                 $W_0\gets min(W, \floor{\lambda_i}-B_i[j].\miss{})$
                
%                 $W\gets W-W_0$
                
%                 $B_i[j].total\gets B_i[j].total+W_0$ 
                
%                 \If{$B_i[j].winner\neq e$}{
%                     $B_i[j].\miss{}\gets B_i[j].\miss{}+W_0$
%                 }
                
%                 \If{$B_i[j].\hit{} = B_i[j].\miss{}$}{
%                     $B_i[j].winner\gets e$ \Comment{flow replacement}
                    
%                     $B_i[j].\miss{}\gets B_i[j].\hit{}$
%                 }
%                 \If{$W = 0$}{
%                     \textbf{break}
%                 }
%             }
%         }
        
%     % }
% \end{algorithm}



% \presub
% \subsection{\anamelong{} for Unbiased Estimation} \postsub
% \label{}


% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Unbiased Estimation in Error-Sensible Bucket}
%     \label{alg:pseudo:bucketinsert}
%     % \KwIn{a flow $e$}
%     \SetKwFunction{FMain}{InsertToBucket}
%     \SetKwProg{Fn}{Procedure}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         $B_i[j].unbias\gets B_i[j].unbias+S(e)$
        
%         \If{$B_i[j].\hit{} = B_i[j].\miss{}$}{ 
%             $B_i[j].winner\gets e$ \Comment{flow replacement}
%         }
%                             % \Comment{Update counters}
%         \If{$B_i[j].winner\neq e$}{
%             $B_i[j].\miss{}\gets B_i[j].\miss{}+1$
%         }
%         $B_i[j].total\gets B_i[j].total+1$
%     }
    
%     \SetKwFunction{FMain}{QueryBucket}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         % $InsertionSuccess\gets False$
            
%             \eIf{$B_i[j].winner=e$}{
%                 $UbFreq\gets  S(e)\cdot B_i[j].unbias$
                
%             }{
%                 $UbFreq\gets   S(e)\cdot \big(B_i[j].unbias-S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})\big)$
                
%             }
            
%             $MaxError\gets 2\cdot B_i[j].\miss{}$
            
%         \Return{$\langle UbFreq, MaxError\rangle $}
%     }
% \end{algorithm}


% The \anamelong{} introduced above provides an estimated frequency that must be greater than the true frequency. In this part, we provide an unbiased frequency whose expected value is equal to the true frequency. We only introduce how to provide unbiased frequencies in one Error-Sensible Bucket. It can be directly extended to the entire algorithm. To provide unbiased estimation, for each Error-Sensible Bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. The initial value of $B_i[j].unbias$ is $0$.

% \ppp{Insertion.} For each flow $e$, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. Then we update the bucket in the same way as the basic version.

% \ppp{Query.} Given the queried flow $e$. If it is $B_i[j].winner$, we report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency ($UbFreq$). Otherwise, we subtract the frequency of $B_i[j].winner$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{winner}\big)$, where $F_{winner}=S(B_i[j].winner)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})$.
% Here we explain why the result is unbiased. Let $U$ be all flows that are inserted to this bucket, and let $f(\cdot)$ denote the frequency in this bucket.
% The $B_i[j].unbias$ equals to $\sum_{x\in U} S(x)f(x)$. 
% For the first case that $e=B_i[j].winner$, we have $E[S(e)\cdot B_i[j].unbias]=E[S^2(e)f(e)]+\sum_{x\in U \setminus {e}} E[S(e)S(x)f(x)]$. As $E[S(e)S(x)f(x)]=E[S(x)]E[S(s)f(x)]$ and $E[S(x)]=0$, we have $E[S(e)\cdot B_i[j].unbias]= f(e)$. Similarly, we can proof that the result in the second case ($e\neq B_i[j].winner$) is unbiased. In this case, we substract $F_{winner}$ from $B_i[j].unbias$ is to reduce the variance. 
% Particularly, the maximum possible error is $2\cdot B_i[j].\miss{}$, which is slightly different from the basic algorithm with one-side error.

% \presub
% \subsection{Protective Measure for Emergency} \postsub




% \presub
% \subsection{Practical Configurations and Discussions} \postsub

% Given a goal, we estimate the resources required.

% Given resources, we estimate the best performance.

% strength and weakness?


==> vldb/Body/algo_v5.tex <==

\newcommand\floor[1]{{\lfloor #1 \rfloor}}

\newcommand{\hit}{YES}
\newcommand{\miss}{NO}

% \begin{table} [!ht]
% \begin{center}
% \vspace{-0.3cm}
% \caption{Symbols.}
% \vspace{-0.2cm}
% \label{table:symbol}
% \begin{tabular}{c|l}
% \hline
% \textbf{Notation}&\textbf{Meaning}\\
% \hline
% % $\mathcal{S}$&a data stream\\
% % \hline
% $N$ & the total number of packets\\
% % \hline
% % $e_t$& $t^{th}$ flow in $\mathcal{S}$\\
% % \hline
% % $f_t$&frequency of $e_t$\\
% % \hline
% $d$&the number of layers\\
% % \hline
% % $B_i$&the $i$-th layer\\
% % \hline
% $w_i$&the number of buckets in the $i$-th layer\\
% % \hline
% $R_w$& the proportion that $w_i$ decreases\\
% % \hline
% $\Lambda$& the user-defined error threshold\\
% % \hline
% $\Lambda_i$&the warning threshold in the $i$-th layer\\
% % \hline
% $\lambda_i$&the error threshold in the $i$-th layer\\
% % \hline
% $R_\lambda$& the proportion that $\lambda_i$ decreases\\
% % \hline
% $h_i(.)$& hash function in the $i$-th layer\\
% % \hline
% % $S(.)$& sign hash function\\
% % \hline
% $B_i[j]$& the $j$-th bucket of the $i$-th layer\\
% % \hline
% $B_i[j].\hit $& the number of hits in $B_i[j]$\\
% % \hline
% % $B_i[j].unbias$ & the unbiased estimator in $B_i[j]$\\
% % \hline
% $B_i[j].\miss{}$\;\,& the number of \miss{}es in $B_i[j]$\\
% % \hline
% $B_i[j].ID$\;\;& the recorded frequent flow in $B_i[j]$\\
% \hline
% \end{tabular}
% \vspace{-0.05in}
% \end{center}
% \end{table}
%\vspace{-0.05in}


% 3.1 Rationale
% 3.2 key 
%  data
%  insertion
%  query
% 3.3 key techniques
%  1.
%  2.
% 3.4 dis

% 3.1 rationale
% 3.2 key technique1: \miss{} sensible bucket
%     过渡
% 3.3 key technique2: double exp.. control
% 3.4 Weighted counting version
% 3.5 Unbiased version
% 3.6 handling the worst case


% \presec
%这个 Trusty Sketch 必须分开
\section{The Reliable Sketch} \postsec
\label{SEC:Algorithm}

% \wyh{Overview.} 
In this section, we present \anamelong{}, which consists of multiple layers of buckets. 
We first show how one bucket works in \cref{subsec:alg:onebucket}. Then, we show how to organize these buckets and set appropriate thresholds to control the error of every flow under the user-defined threshold in \cref{subsec:alg:formal:tech2}.
% Finally, we discuss our design choices in \cref{subsec:alg:discussion}.
% Symbols frequently used are listed in Table \ref{table:symbol}.}

% %不重复展示
% \ppp{Rationale:}
% The \anamelong{} consists of multiple layers, and each layer has an increasing warning threshold. These thresholds are at most $\Lambda$.
% When a flow’s error boundary (\ie, the maximum possible error) reaches the warning threshold in one layer, it will be inserted to the next layer. There are two key challenges: (1) Accurately Sensing. Find high-risk flows whose error bounds reach the warning threshold; (2) Effectively Control. Reduce high-risk flows efficiently//effectively with small space and a small number of layers.
% We devise the Error-Sensing technique (Sec. \ref{subsec:alg:tech1}) and the Double Exponential Composition (Sec. \ref{subsec:alg:tech2}) to tackle above two challenges respectively.

% \presub
% \subsection{Data Structure} \postsub
% \label{sec:algo:structure}



% As shown in Figure \ref{fig:algo:structure}, the data structure of \anamelong{} consists of $d$ layers, $B_1,$ $B_2,$ $\dots,$ $B_d$. The $i$-th layer $B_i$ is an array consists of $w_i$ \textit{Error-Sensible buckets}, denoted as $B_i[1],$ $B_i[2],$ $\dots,$ $B_i[w_i]$. 
% The size of layer $B_i$, denoted as $w_i$, decreases in proportion to $R_{w} (R_{w}>1)$ as $i$ increases.
% Each layer $B_i$ has an error threshold, denoted as $\lambda_i$. $\lambda_i$ decreases in proportion to $R_{\lambda} (R_{\lambda}>1)$ as $i$ increases.
% The warning threshold in layer $B_i$, denoted as $\Lambda_i$, is the sum of the error thresholds of the first $i$ layers, \ie, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i$ must be no more than user-defined threshold $\Lambda$.
% Each layer is associated with a pair-wisely independent hash function $h_i(\cdot)$, which maps each flow (denoted by $e$) into a random bucket (the $j$-th bucket $B_i[j], j=h_i(e)$) uniformly.







\presub
\subsection{Basic Unit: the Error-Sensible Bucket } \postsub
\label{subsec:alg:onebucket}
We show how the basic unit of \anamelong{}, called \textit{Error-Sensible bucket}, works on the packet stream and senses the error. 
First, we introduce the Error-Sensible bucket as a framework that covers many election designs. Then, through our analysis, we recommend one specific design.
% The Error-Sensible bucket supports two operations: (1) Insert a packet; (2) Query the flow size and its MPE.

% The key idea is to sense the error through the number of NO votes in the process of electing frequent flows.
% In this section, we present the \textit{Error-Sensing} technique, based on the Error-Sensible bucket.
% The key idea is to bound the error by the number of "nays" when electing the most frequent flow.
%of a flow together with its maximum possible error.
% The structures of all Error-Sensible buckets are the same.
\ppp{Structure:}
Specifically, the bucket has three fields, one ID field recording the ID of a candidate flow, and two counters recording the positive votes and negative votes, denoted as $ID$, $YES$ and $NO$, respectively. Initially, $ID$ is $null$ and both counters are $0$. The bucket supports two operations: (1) Insert a packet; (2) Query the flow size and its MPE.

% one Error-Sensible bucket $B$ contains one flow ID $B.ID$ and two counters, $B.\hit$ and $B.\miss{}$.
% $B.ID$ records the flow ID of an elected frequent flow.
% $B.\hit$ records the number of positive votes and $B.\miss{}$ records the number of negative votes.
% % total frequency of all flows inserted into the bucket. 
% % $B.\miss{}$ records the number of times that the inserted flow differs from $B.ID$, called \miss{}es.
% Initially, $B.ID$ is $null$ and both two counters are set to $0$. 



\subsubsection{\textbf{Insert a packet}} $\ $

\noindent{}When inserting a packet with flow ID $e$, there are two stages: Replacement and Votes Voting.
First, we first examine the criteria for whether replacement occurs: whether $YES \leqslant F(NO)$, where $F: N \mapsto N $ is a monotonically increasing function satisfying $F(i)<F(i+1)\ \forall i$.
If so, we believe there are too many $NO$ votes, replace the recorded flow $ID$ with $e$, and swap the value of $YES$ and $NO$.
In this case, $ID$ is not frequent enough to be kept and we can give other flows a chance to enter.
After the replacement stage, we vote whether the recorded flow $ID$ is $e$ or not. If so, we vote YES by incrementing $YES$ by $1$.
Otherwise, we vote NO by incrementing the number of $NO$ by $1$.

\textit{The coverage of the framework.} This framework can cover the operations from Elastic, Majority, SpaceSaving and more \cite{frequent,tang2019mvsketch}. For Elastic, it is a case of $F(i)=\lambda\times i, \lambda\in[4,128]$. For Majority, it only records one counter whose value is $YES-NO$, and it is a case of $F(i)=i$. For SpaceSaving, when it is of size $2$, it records two IDs and two counters and it is a case of $F(i)=\lambda\times i, \lambda\in[4,128]$.


\textit{Analysis results.} 
From complex proofs, we can derive that the flow size of $ID$ must be in interval $[YES-NO-\Delta_n, YES+\sum_{i=1}^{n-1}\Delta_i]$, where $\Delta_i$ is the value of $F(NO)-YES$ at the moment before the $i$-th replacement occurs and $\Delta_n$ is that of the latest replacement.
And the flow size of any other flow must be in interval $[0, NO+\sum_{i=1}^{n}\Delta_i]$.
An ideal design scheme can minimize the above two intervals at the same time through a simple structure. After detailed analysis, we choose the best $F(i)=i$ as our specific design. Its workflow of insertion and query is shown in Figure \ref{fig:operations:bucket}.


\subsubsection{\textbf{Query the flow size and MPE}} $\ $
% \ppp{Query the flow size and MPE. } 

\noindent{}To query the flow size of $e$ in a bucket, we first check whether the recorded ID is the queried flow $e$. If so, our estimation of the flow size $\widehat{f_e}$ is $\hit{}$. Otherwise, $\widehat{f_e}$ is $\miss{}$. The estimation is guaranteed to be no less than the true flow size (Proved by induction).
In both cases, MPE is $\miss{}$. 
At a high level, $\miss{}$ works because it can reflect the intensity of conflict between different flows.


\subsubsection{\textbf{Discussions.}} $\ $
% \ppp{Discussions.}

\ppp{Key technique I: Error-Sensing.} To sense the error, our technical approach is to replace the basic unit of sketches with the Error-Sensible bucket. 
Instead of designing a completely new basic unit, we stand on the shoulders of giants to devise the basic bucket. We modify and use the beneficial parts of the prior work as our basic unit for error-sensing. For the first time, we focus on and utilize the sensed error in other parts of the data structure, rather than only use it for the theoretical analysis.



\begin{figure}[tbp]
    \prefig
    \centering  
    \includegraphics[width=0.98\linewidth]{vldb/Figures/algo/algo_graph1V2.pdf}
    \vspace{-0.15in}
    \caption{An Overview of \anamelong{}.}
    \label{fig:algo:structure}
    \postfig
\end{figure}

\begin{figure}[tbp]
    % \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph2V2.pdf}
    \vspace{-0.15in}
    \caption{Operation Workflow.}
    \label{fig:operations:bucket}
    \postfig
\end{figure}


\noindent\textit{Compared with a simple counter, what is the disadvantage of the Error-Sensible bucket as a basic unit?}
The recorded ID is space-consuming and the insertion becomes more complex and time-consuming. These costs are worth paying, in order to get the ability to sense the error. The time consumption is not significant because the main cost lies in memory access and hash calculation, rather than the insertion within the basic unit. 
Based on the ability to sense the error, we devise the Double Exponential Composition technique, which not only covers the Error-Sensible bucket's disadvantages in both time and space but also performs much better than existing sketches.






% \ppp{Insert a packet.} 
% \wyh{To insert a packet with flow ID $e$ into bucket $B$, we first decide whether to perform the replacement, \ie, replace the old $B.ID$ with new $e$ as the candidate frequent flow. 
% The criterion is whether $B.\hit \leqslant B.\miss{}$.
% If so, we believe there are too many \miss{} votes and we replace the recorded flow. In this case, $B.ID$ is not frequent enough to be kept and we can give other flows a chance to enter.
% % We will strictly explain the condition later.
% After that, we vote whether the recorded flow $B.ID$ is $e$ or not.
% If so, we vote YES by incrementing $B.\hit{}$ by $1$.
% Otherwise, we vote NO by incrementing the number of $B.\miss{}$ by $1$.}
% \ppp{Query the flow size and MPE. } 
% To query the flow size of $e$ in bucket $B$, we first check whether the recorded ID $B.ID$ is the queried flow $e$. If so, our estimation of the flow size $\widehat{f_e}$ is $B.\hit{}$. Otherwise, $\widehat{f_e}$ is $B.\miss{}$. The estimation is guaranteed to be no less than the true flow size (Proved by induction).
% In both cases, MPE is $B.\miss{}$. \wyh{This is our key technique I called Error-Sensing. 
% At a high level, $B.\miss{}$ works because it can \textit{reflect the intensity of conflict between different flows.}}





% As MPE is $B.\miss{}$, the true flow size of $B.ID$ must be in interval $\left[B.\hit-B.\miss, B.\hit\right]$.

% \begin{theorem} 
% The outputs of Error-Sensible buckets satisfies: $$\widehat{f_e}-MPE\leqslant f_e\leqslant \widehat{f_e}$$
% \end{theorem}

% can be prove that $\hit-\miss$ increments by 1 only when $ID$ comes.
% The true flow size of $B.ID$ 

% The above query algorithm is based on the following theorem:
% % Let $T$ and $C$ denote $B.total$ and $B.\miss{}$ respectively, we have
% \begin{theorem} The frequency of the ID is at most $B.\hit{}$ and it is at least $B.total-2\cdot B.\miss{}$. The frequency of any flow other than the ID is at most $B.\miss{}$.
% \end{theorem}




% \begin{figure}[htbp]
%     % \prefig
%     \centering  
%     \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph3V2.pdf}
%     \vspace{-0.15in}
%     \caption{An example of the Error-Sensible bucket. The packets "c,a,b,a,a,b,a,a" are inserted into a bucket in turn, and their estimation results are shown in the right.}
%     \label{\miss{}_sensible}
%     \postfig
% \end{figure}



\presub
\subsection{Formal \aname{}: Error Control} \postsub
\label{subsec:alg:formal:tech2}



% The \anamelong{} consists of multiple layers, and each layer has an increasing warning threshold. These thresholds are at most $\Lambda$.
% When a flow’s error boundary (\ie, the maximum possible error) reaches the warning threshold in one layer, it will be inserted to the next layer. 



In this part, we show how to organize Error-Sensible buckets and assemble them into a \anamelong{}, in order to control per-flow error. The overview of \anamelong{} is shown in Figure \ref{fig:algo:structure}.
First, we introduce a new mechanism called ``lock'' to the bucket in order to control the error in the bucket.
Then, we show the data structure of the \anamelong{}, followed by the operations of insertion and query.



% \subsubsection{\textbf{Lock Mechanism}} $\ $

% \tex{Lock a bucket to control the error when necessary.}
\ppp{Lock Mechanism.}
When MPE of a bucket reaches a threshold, \ie, $B.\miss{}=\lambda$, in order to stop the growth of MPE, we lock the bucket.
When we lock the bucket, only two cases of insertion are allowed, and they will not increase MPE (\ie, $B.\miss{}$) :
\begin{itemize}[leftmargin=*]
    \item $B.ID=e$, which only increment $B.\hit$
    \item $B.\hit{}\leqslant B.\miss{}$, where a replacement happens and we increment $B.\hit$.
\end{itemize}
In other cases, packets cannot be inserted to the locked bucket. These packets are at higher risk of losing control and we will find other buckets for them.


\ppp{Data structure of \anamelong{}:}
As shown in Figure \ref{fig:algo:structure}, \anamelong{} has $d$ layers and each layer has many Error-Sensible buckets. The $j$-th bucket in the $i$-th layer is denoted as $B_i[j]$.
The width of the $i$-th layer (denoted as $w_i$) decreases as $i$ increases.
Each layer has a layer threshold to determine whether to lock the bucket, denoted as $\lambda_i$. 
$\lambda_i$ also decreases as $i$ increases and their sum does not exceed the user-defined error threshold, \ie, $\sum_i \lambda_i \leqslant \Lambda$.
Each layer has a independent hash function $h_i(\cdot)$, which uniformly maps each flow to one bucket in the layer. Detailed parameter settings are in \cref{subsec:math:parametersetting}.

% The warning threshold in layer $B_i$, denoted as $\Lambda_i$, is the sum of the layer thresholds of the first $i$ layers, \ie, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i$.
% Each layer is associated with a pair-wisely independent hash function $h_i(\cdot)$, which maps each flow (denoted by $e$) into a random bucket (the $j$-th bucket $B_i[j], j=h_i(e)$) uniformly.




% The \anamelong{} consists of multiple layers, and each layer has many buckets.
% % \wyh{Then, we show how to combine these buckets and set thresholds to control the error of every flow to the user-defined threshold in Section.}
% % We present Double Exponential Control technique to handle all flows with large error boundaries.
% As mentioned in Section \ref{subsec:alg:struct}, \anamelong{} has multiple layers, and each layer has a number of buckets.
% Every Error-Sensible bucket in layer $i$ will not be locked until the error boundary reaches $\lambda_i$.
% The size of each layer decreases $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and the error threshold of each layer also decreases $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$.
% An ideal case is that the amount of flows entering each layer decreases much faster than $w_i$ and $\lambda_i$. But it is not easy to reach the ideal case.
% Now, we fully introduce the Double Exponential Control starting from the operations of \anamelong{}: Insertion and Query.




\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Insertion.}
    \label{alg:pseudo:Insertion:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e$}}{
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
                        
            \If{($B_i[j].\miss{}  < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].\hit{} \leqslant B_i[j].\miss{}$)}{
                \Comment{Insert to the first available bucket}
                % \Comment{}
                
                \If{$B_i[j].\hit \leqslant B_i[j].\miss{}$}{ 
                    $B_i[j].ID\gets e$ \Comment{flow replacement}
                }
                                    % \Comment{Update counters}
                                    
                \eIf{$B_i[j].ID=  e$}{
                    $B_i[j].\hit\gets B_i[j].\hit+1$
                }{
                    $B_i[j].\miss{}\gets B_i[j].\miss{}+1$
                }
                % $InsertToBucket(e, B_i[j])$
                
                \textbf{break} \Comment{Succeed and Stop.}
            }
            % $i\gets i+1$ 
            % \Comment{Go to next layer}
        }
    
    }
\end{algorithm}

\subsubsection{\textbf{Insertion}} $\ $

\noindent{}We insert a packet $e$ to \anamelong{} by two steps, finding an available bucket and insert the packet to it. The pseudo-code is shown in Algorithm \ref{alg:pseudo:Insertion:all}.
For the first step, we start from the first layer and hash $e$ to a bucket of this layer, called \textit{mapped bucket} ($B_i[j], j=h_i(e), i=1$). 
Then we check whether $B_i[j]$ is an available bucket that can be inserted by $e$.
% where $e$ will not incur \miss{}es to make the error greater than $\lambda_i$ (\ie, the error threshold of this layer).
The bucket is available in any of the following three cases: 
\vspace{-0.1cm}
\begin{itemize}[leftmargin=*]
    \item $B_i[j].\miss{} < \lambda_i$: The bucket is not locked.
    \item $B_i[j].ID=e$: Only increment $B_i[j].\hit$
    \item $B_i[j].\hit{}\leqslant B_i[j].\miss{}$: A replacement happens and we increment $B_i[j].\hit$.
    % \item $B_i[j].ID=e$, which means $e$ will not incur \miss{}.
    % \item $B_i[j].\hit{} = B_i[j].\miss{}$, which means we can replace the $B_i[j].ID$ by $e$.
\end{itemize}
\vspace{-0.1cm}
% \textit{(i)} $B_i[j].ID=e$, which means $e$ is an unlimited flow in this bucket; 
% 2) $B_i[j].low=0$, which means the new flow $e$ can replace the old flow $B_i[j].ID$; 
% \textit{(ii)} $\frac{1}{2}(B_i[j].total-B_i[j].low)< \lambda_i$, which means the error of this bucket is tolerable.
If the bucket is available, we insert $e$ into the bucket and completed the insertion.
Otherwise, $e$ is at higher risk of losing control, we keep finding an available bucket in the following layers until the last one.
In a few cases, the bucket in the last layer is unavailable and the insertion fails, which rarely ($<0.00001\%$) happens under our recommended parameters.
If the insertion failure really happens, we can use our emergency solution (\cref{extension:emergency}) to solve the problem.
% The insertion in the data plane is failed. 
% and we insert $e$ to a small stash to handle these flows. We will detail the stash later.
 



\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{Weighted Insertion.}
    \label{alg:pseudo:Insertion:all:Weighted}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$\langle e, f\rangle$}}{
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
            
            \If{$B_i[j].id==e$}{
                
                
                $B_i[j].YES\gets B_i[j].YES + f$
                
                \textbf{break} 
            }
            \eIf{$B_i[j].YES>\lambda_i$ \textbf{and} $B_i[j].NO+f>\lambda_i$}{
                $B_i[j].NO\gets \lambda_i$
                
                $f\gets B_i[j].NO+f-\lambda_i$
                
            }{
                \eIf{$B_i[j].NO+f>=B_i[j].YES$}{
                    $B_i[j].id\gets e$
                    
                    $NEW\_YES\gets B_i[j].NO+f$
                    
                    $B_i[j].NO\gets B_i[j].YES$
                    
                    $B_i[j].YES\gets NEW\_YES$
                }{
                    $B_i[j].NO\gets B_i[j].NO+f$
                }
                \textbf{break} 
            }
        }
    }
\end{algorithm}
Next, introduce how we insert a packet $e$ with frequency $f$.
The naive approach is to run basic insertion of $e$ by $f$ times, which is time consuming. Actually, we can do it at once (Algorithm \ref{alg:pseudo:Insertion:all:Weighted}). Similarly, from the first layer, we find the mapped bucket $B_i[j]$ by hashing and try to insert the packet into it.
First, if the recorded ID $B_i[j].id$ matches $e$, we just increase the $YES$ by $f$ and finish the insertion.
Otherwise, we know $B_i[j].id$ is not $e$.
Then, we check whether $B_i[j].NO$ can reach the layer error threshold $\lambda_i$. It has two conditions:
\begin{itemize}[leftmargin=*]
    \item $B_i[j].YES>\lambda_i$: No replacement will happen before the bucket is locked.
    \item $B_i[j].NO+f>\lambda_i$: The bucket can be locked if no replacement happens.
\end{itemize}
If so, we set $B_i[j].NO$ to threshold $\lambda_i$, and we save the frequency not inserted for later layers.
Otherwise, $B_i[j].NO$ will not reach $\lambda_i$.
We check whether the replacement will happen. If so, we just perform the replacement and update the counters. Otherwise, we just increase $B_i[j].NO$.


\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Query.}
    \label{alg:pseudo:query:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{QueryFrequency}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $ \widehat{f_e}\gets 0$  \Comment{Flow Size Estimator}
        
        % $ Ub\gets 0$ \Comment{Unbiased Estimator}
        
        $ MPE\gets 0$ \Comment{Maximum Possible Error}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the bucket}
            
            \eIf{$B_i[j].ID=e$}{
                $\widehat{f_e}\gets \widehat{f_e} + B_i[j].\hit{}$
                
                % $Ub\gets Ub+B_i[j].unbias$
            }{
                $\widehat{f_e}\gets \widehat{f_e} + B_i[j].\miss{}$
                
                % $Ub\gets Ub+B_i[j].unbias-B_i[j].low\cdot S(B_i[j].ID)$
            }
            
            
            $ MPE\gets MPE + B_i[j].\miss{}$
            
                        
            \If{ ($B_i[j].\miss{}  < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].\hit{} \leqslant B_i[j].\miss{}$)}{
                \textbf{break} \Comment{Stop collecting flow sizes}
            }
        }
        
        \Return{$\langle \widehat{f_e}, MPE\rangle$}
    }
\end{algorithm}

% \vspace{-0.3cm}

% \ppp{Query (Algorithm \ref{alg:pseudo:query:all}).} 

\subsubsection{\textbf{Query}} $\ $

\noindent{}When query the flow size of a flow $e$, \anamelong{} reports an over-estimated flow size $\widehat{f_e}$ with its MPE.
The pseudo-code is shown in Algorithm \ref{alg:pseudo:query:all}.
As every time inserting a flow, we only insert it into one bucket of a specific layer.
When querying, we just sum up its flow sizes in different layers. 
Starting from the first layer, we access the mapped bucket $B_i[j], j=h_i(e)$ layer by layer. 
We add up the estimated flow sizes and MPE, respectively. 
We can stop when the mapped bucket in layer $i$ is still available for $e$. Because in this case, $e$ must never be inserted to those later layers. 
Finally, we get the $\widehat{f_e}$ with its MPE.
We also get an interval that the true flow size $f_e$ must be in, \ie, $f_e \in \left[\widehat{f_e}-MPE, \widehat{f_e}\right]$.

\ppp{Key Technique II: Double Exponential Composition.}
To control the error of all flows reliably, we need to prevent insertion fails of breaking through the last layer. 
% An ideal goal is to insert all flows into the first few layers, not into the later layers.
In practice, it is critical for every layer to reduce the number of flows entering its next layers.
Under common parameters, each layer may stop half flows and the probability $\mathcal{P}$ that a flow fails to be inserted is $\frac{1}{2^d}$.
We found that, only when both the width $w_i$ and the layer threshold $\lambda_i$ decrease exponentially (\eg, $w_{i+1}=w_i/2, \lambda_{i+1}=\floor{\lambda_i/2}$), the failure probability $\mathcal{P}$ decreases at double exponential speed (\eg, $\frac{1}{2^{2^{d}}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$.}), which can overwhelm the number of flows and eliminate the insertion failure with extremely high probability.


% the effect is best only when we reduce the width and error threshold exponentially. Specifically, the rate of decline is double exponential.......

% We do not access all layers because if a mapped bucket in layer $B_i$ is available for $e$, $e$ must never be inserted to its following layers and we stop at the $i$-th layer.
% In a few cases, we do not stop at the last layer. We estimate the frequency in the stash and add it to the total frequency.


% \presub
% \subsection{Extensions} \postsub

% \subsubsection{Freely turning the accuracy of priority flows.}


% The extended Priority TrustySketch (\anamesum{} for short) can adjust the estimation accuracy of any flow. We can improve the accuracy of a high-priority flow (\eg, a flow with high SLA requirement) by giving it a weight. The weight of flow $e_i$, denoted as $w_i$, is an user-defined positive integer and it can improve the guaranteed accuracy from the old $\Lambda$ to $\lfloor \frac{\Lambda}{w_i} \rfloor$. Therefore, when $w_i$ is set to $\lfloor w_i \rfloor$, the estimation of flow $e_i$ must be correct.
% The key idea of inserting a packet $e_i$ with weight $w_i$ is to insert a packet for $w_i$ times by common insert operation. 
% Instead of spending $w_i$ times of time, we can achieve the same insertion speed as usual by some reasonable modifications. 
% Increasing the accuracy of partial flow will consume more memory. For example, if we reduce the error of 10\% flow by 50\%, we need 10\% more memory. 
% % The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 
% % The new \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. 

% % The extended priority TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% % \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 


% \subsubsection{Improving the overall accuracy by a mice filter.}
% After achieving good theoretical results, the memory efficiency of \anamelong{} can be further optimized in practice.
% % In a switch, the memory reserved for the measurement function is scarce 
% The first layer of \anamelong{} is the largest layer and it takes more than $50\%$ space of the whole \anamelong{}. But the first layer is in efficient when there are quite a few mice flows in the traffic. The mice flows will increment the 'miss' counters sharply and lock most buckets in the first layers. In this case, many buckets are wasted to record the mice flows. 

% To tackle the mice flows, we replace the first layer with a small mice-flow filter and still controlling the error well. Specifically, inspired by CU \cite{estan2002cusketch}, the filter consists of two arrays ($F_1[]$ and $F_2[]$) and each array has $\frac{1}{2} w_1$ $L$-bit counters. For every flow ID $e$, we use two hash functions $h_1^{(1)}(.)$ and $h_1^{(2)}(.)$ to select two mapped counters $C_1=F_1[h_1^{(1)}(e)]$ and $C_2=F_1[h_1^{(1)}(e)]$. To insert a packet with flow ID $e$, if 
% any of its two mapped counters is less than $\lambda_1$, we regard it as a mice flow. For a mice flow, we drop it and increment the minimal mapped counter(s) less than $\lambda_1$ by one. Otherwise, when both mapped counters equal to $\lambda_1$, we regard it as a non-mice flow, and pass the packet to the second layer.
% In practice, 8-bit counters are sufficient for the filter. Compared to a layer composed of 72-bit Error-Sensible buckets, the filter can reduce the space cost of layer-1 nearly $10$ times while incurring small controllable errors. The overall accuracy will be significantly improved when we move the space saved by the filter to the other layers. But we cannot replace other layers by the filter because the filter cannot estimate elephant flows well.

% \presub
% \subsection{More Functions of \anamelong{}} \postsub
% \label{extend}


% Our \anamelong{} has good versatility for various scenarios. We take the two most concernful tasks as examples, weighted counting and unbiased frequency estimation. We only introduce the key idea of how to achieve them.

% \ppp{Weighted Counting.} The extended Weighted TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 

% \presub
% \subsection{Discussions} \postsub
% \label{subsec:alg:discussion}

% We shortly review the design and discuss the design choices.
% In \anamelong{}, we devise Error-Sensible buckets that can sense the error of both mice and elephant flows, and combine them into a multi-layer structure to eliminate the flows at the risk of losing control.

% \noindent\textbf{How we design the Error-Sensible bucket?} We try to design the most simple error-sensible structure so that it can implemented in various platforms, especially the programmable switch. The bucket has only two counters and one ID, which can hardly be further simplified.

% \noindent\textbf{Compared with a simple counter, what is the disadvantage of the Error-Sensible bucket as a basic unit?} The recorded ID consumes a lot of space, and the insertion becomes more complex and time-consuming. These costs are worth paying, in order to get the ability to sense the error. The time consumption is not significant because the main cost lies in memory access and hash calculation, rather than the insertion within the basic unit. 
% Based on the ability to sense the error, we devise the Double Exponential Composition technique, which not only covers the disadvantages of the Error-Sensible bucket but also performs much better than existing sketches.

% \noindent\textbf{What is the difference of the multi-layer structure of \anamelong{} and the traditional multi-layer structure?} The key difference is that we have no copy and can quickly reduce flows layer by layer.
% Existing sketches, including CM, CU, and Count, have multi-layers and may update multiple counters when inserting one packet, which is called copy. We only update one counter for each packet, which makes \anamelong{} accurate and memory-efficient.
% Our multi-layer buckets can reduce both elephant flows and mice flows. In contrast, traditional methods \cite{coldfilter,lu2008counterbraids} insert all remaining flows to the next layer when a counter is large, which method will insert most elephant flows to the next layer and cannot reduce elephant flows effectively.
% Thanks to efficiently reducing flows, every packet only needs to access $1\sim 2$ layers in average, which makes \anamelong{} fast. Never seen before, \anamelong{} can reduce flows at the double exponential speed (proved mathematically in \cref{sec:math} and experimentally in \cref{subsubsec:exp:control}).


% Before a bucket is locked, we have the following theorem:
% \begin{theorem} 
%     \label{alg:theorem:\miss{}}
%     $B_i[j].\miss{}$ is no greater than the total frequency of all flows except for the most frequent flow.
% \end{theorem}
% \ppp{Bounded lock probability for any flow.} Base on Theorem \ref{alg:theorem:\miss{}}, the bucket can ensure that, when we know that an arbitrarily frequent flow will be inserted to the bucket, whatever its arriving time, the probability of the bucket being locked is small and bounded.
% This is the key point that our algorithm can achieve better theoretical complexity in both time and space (detailed in Section \ref{sec:math}).
% When we lock the bucket, some flows will be inserted into the next layer. We use the next technique to handle these flows.




% \wyh{ Due to space limitations, we leave the detailed \anamesum{} algorithm to the reader, which is not the primary focus of this paper.}

% \ppp{Unbiased Frequency Estimation.} 
% Rather than guaranteeing one-side error\footnote{The estimations from \anamelong{} must be no less than the true frequency}, we can extend \anamelong{} to provide the unbiased estimated frequency whose expected value is the true frequency.
% We only introduce how to provide unbiased frequencies in one Error-Sensible bucket.
% It can be directly extended to the entire algorithm.
% To provide unbiased estimation, for each Error-Sensible bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. Initially, $B_i[j].unbias$ is $0$. For each flow $e$ to be inserted, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. 
% When queried flow $e$, a simple but correct approach is to report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency. That is because $E[S(e)\cdot B_i[j].unbias]=E[f(e)]+\sum_{x\in U \setminus {e}} E[S(x)]\cdot E[S(e)f(x)]=f(e)$, where $U$ is the universe of all flows. But in this case, we cannot sense the error and control it below $B_i[j].\miss{}$.
% Actually, we can subtract the frequency of $B_i[j].ID$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{ID}\big)$, where $F_{ID}=S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})$.
% In this case, the error boundary is $2\cdot B_i[j].\miss{}$.


% \ppp{Insertion (Algorithm \ref{?}).}
% In the task of SUM (Defined in Section \ref{??}), each inserted flow includes an identifier $e$ and weight $w_e (w_e>0)$.
% The insertion of \anamesum{} is similar to inserting $e$ by \anamecount{} for $w_e$ times.
% Let variable $W$ represent the remaining weight to be inserted. Its initial value is $w_e$. Every time we find an available bucket, we try to insert into it. First, we calculate how much weight (denoted as $W_0$) can be inserted into the current bucket at most. The $W_0$ is the minimum value of the remaining weight ($W$) and the maximum weight that the bucket can hold $\lambda_i-B_i[j].\miss{}$ before being locked. 
% Next, we insert $e$ with weight $W_0$ to the bucket directly.
% We add up the total flows by $W_0$ and then add up the \miss{} number if needed.
% If the flow replacement is triggered, we replace the flow and correct the number of \miss{}es to $B_i[j].\hit{}$.

% % similar to xxx to insert w0 into the bucket. Next, continue to find the next feasible bucket for insertion until the frequency W to be inserted is equal to 0.

% \ppp{Query.}
% The query asks the total weight of an given flow identifier $e$. 
% The query of \anamesum{} is the same as that of \anamecount{}.

    % \begin{algorithm}[!h]
    %     \SetAlgoNoLine
    %     \caption{Insertion in Sum Task}
    %     \KwIn{a flow $e$ and its weight $w_e$}
    %     \SetKwFunction{FMain}{Insert???}
    %     % \SetKwProg{Fn}{Procedure}{:}{}
    %     % \Fn{\FMain{$e, w_e$}}{
                
    %         $W\gets w_e$ \Comment{The total amount to be inserted}
            
    %         \For{Layer $i=1,2,\dots, d$}
    %         {
    %             $j\gets h_i(e)$  \Comment{Locate the bucket $B_i[j]$}
                            
    %             \If{$(B_i[j].\miss{} < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].\hit{} \leqslant B_i[j].\miss{})$}{
                    
    %                 \If{$B_i[j].ID = null$}{ 
    %                     $B_i[j].ID\gets e$ 
    %                 }
    %                                             \Comment{The amount to be inserted into this bucket}
                                                
    %                 $W_0\gets min(W, \lambda_i-B_i[j].\miss{})$
                    
    %                 $W\gets W-W_0$
                    
    %                 $B_i[j].total\gets B_i[j].total+W_0$ 
                    
    %                 \If{$B_i[j].ID\neq e$}{
    %                     $B_i[j].\miss{}\gets B_i[j].\miss{}+W_0$
    %                 }
                    
    %                 \If{$B_i[j].\hit{} = B_i[j].\miss{}$}{
    %                     $B_i[j].ID\gets e$ \Comment{flow replacement}
                        
    %                     $B_i[j].\miss{}\gets B_i[j].\hit{}$
    %                 }
    %                 \If{$W = 0$}{
    %                     \textbf{break}
    %                 }
    %             }
    %         }
            
    %     % }
    % \end{algorithm}



% \presub
% \subsection{\anamelong{} for Unbiased Estimation} \postsub
% \label{}


% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Unbiased Estimation in Error-Sensible bucket}
%     \label{alg:pseudo:bucketinsert}
%     % \KwIn{a flow $e$}
%     \SetKwFunction{FMain}{InsertToBucket}
%     \SetKwProg{Fn}{Procedure}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         $B_i[j].unbias\gets B_i[j].unbias+S(e)$
        
%         \If{$B_i[j].\hit{} = B_i[j].\miss{}$}{ 
%             $B_i[j].ID\gets e$ \Comment{flow replacement}
%         }
%                             % \Comment{Update counters}
%         \If{$B_i[j].ID\neq e$}{
%             $B_i[j].\miss{}\gets B_i[j].\miss{}+1$
%         }
%         $B_i[j].total\gets B_i[j].total+1$
%     }
    
%     \SetKwFunction{FMain}{QueryBucket}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         % $InsertionSuccess\gets False$
            
%             \eIf{$B_i[j].ID=e$}{
%                 $Ub\widehat{f_e}\gets  S(e)\cdot B_i[j].unbias$
                
%             }{
%                 $Ub\widehat{f_e}\gets   S(e)\cdot \big(B_i[j].unbias-S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})\big)$
                
%             }
            
%             $MaxError\gets 2\cdot B_i[j].\miss{}$
            
%         \Return{$\langle UbFreq, MaxError\rangle $}
%     }
% \end{algorithm}


% The \anamelong{} introduced above provides an estimated frequency that must be greater than the true frequency. In this part, we provide an unbiased frequency whose expected value is equal to the true frequency. We only introduce how to provide unbiased frequencies in one Error-Sensible bucket. It can be directly extended to the entire algorithm. To provide unbiased estimation, for each Error-Sensible bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. The initial value of $B_i[j].unbias$ is $0$.

% \ppp{Insertion.} For each flow $e$, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. Then we update the bucket in the same way as the basic version.

% \ppp{Query.} Given the queried flow $e$. If it is $B_i[j].ID$, we report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency ($UbFreq$). Otherwise, we subtract the frequency of $B_i[j].ID$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{ID}\big)$, where $F_{ID}=S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].\miss{})$.
% Here we explain why the result is unbiased. Let $U$ be all flows that are inserted to this bucket, and let $f(\cdot)$ denote the frequency in this bucket.
% The $B_i[j].unbias$ equals to $\sum_{x\in U} S(x)f(x)$. 
% For the first case that $B_i[j].ID=e$, we have $E[S(e)\cdot B_i[j].unbias]=E[S^2(e)f(e)]+\sum_{x\in U \setminus {e}} E[S(e)S(x)f(x)]$. As $E[S(e)S(x)f(x)]=E[S(x)]E[S(s)f(x)]$ and $E[S(x)]=0$, we have $E[S(e)\cdot B_i[j].unbias]= f(e)$. Similarly, we can proof that the result in the second case ($e\neq B_i[j].ID$) is unbiased. In this case, we substract $F_{ID}$ from $B_i[j].unbias$ is to reduce the variance. 
% Particularly, the maximum possible error is $2\cdot B_i[j].\miss{}$, which is slightly different from the basic algorithm with one-side error.

% \presub
% \subsection{Protective Measure for Emergency} \postsub




% \presub
% \subsection{Practical Configurations and Discussions} \postsub

% Given a goal, we estimate the resources required.

% Given resources, we estimate the best performance.

% strength and weakness?


==> vldb/Body/algo_v6.tex <==

\newcommand\floor[1]{{\lfloor #1 \rfloor}}

\newcommand{\hit}{YES}
\newcommand{\miss}{NO}

% \begin{table} [!ht]
% \begin{center}
% \vspace{-0.3cm}
% \caption{Symbols.}
% \vspace{-0.2cm}
% \label{table:symbol}
% \begin{tabular}{c|l}
% \hline
% \textbf{Notation}&\textbf{Meaning}\\
% \hline
% % $\mathcal{S}$&a data stream\\
% % \hline
% $N$ & the total number of packets\\
% % \hline
% % $e_t$& $t^{th}$ flow in $\mathcal{S}$\\
% % \hline
% % $f_t$&frequency of $e_t$\\
% % \hline
% $d$&the number of layers\\
% % \hline
% % $B_i$&the $i$-th layer\\
% % \hline
% $w_i$&the number of buckets in the $i$-th layer\\
% % \hline
% $R_w$& the proportion that $w_i$ decreases\\
% % \hline
% $\Lambda$& the user-defined error threshold\\
% % \hline
% $\Lambda_i$&the warning threshold in the $i$-th layer\\
% % \hline
% $\lambda_i$&the error threshold in the $i$-th layer\\
% % \hline
% $R_\lambda$& the proportion that $\lambda_i$ decreases\\
% % \hline
% $h_i(.)$& hash function in the $i$-th layer\\
% % \hline
% % $S(.)$& sign hash function\\
% % \hline
% $B_i[j]$& the $j$-th bucket of the $i$-th layer\\
% % \hline
% $B_i[j].\hit $& the number of hits in $B_i[j]$\\
% % \hline
% % $B_i[j].unbias$ & the unbiased estimator in $B_i[j]$\\
% % \hline
% $B_i[j].NO$\;\,& the number of NOes in $B_i[j]$\\
% % \hline
% $B_i[j].ID$\;\;& the recorded frequent flow in $B_i[j]$\\
% \hline
% \end{tabular}
% \vspace{-0.05in}
% \end{center}
% \end{table}
%\vspace{-0.05in}


% 3.1 Rationale
% 3.2 key 
%  data
%  insertion
%  query
% 3.3 key techniques
%  1.
%  2.
% 3.4 dis

% 3.1 rationale
% 3.2 key technique1: NO sensible bucket
%     过渡
% 3.3 key technique2: double exp.. control
% 3.4 Weighted counting version
% 3.5 Unbiased version
% 3.6 handling the worst case


% \presec
\section{The Reliable Sketch} \postsec
\label{SEC:Algorithm}

In this section, we present \anamelong{}. We start from a new alternative to the counter of counter-based sketches, termed an 'Error-Sensible bucket'. This allows every basic counting unit within \anamelong{} to perceive the magnitude of its error, as discussed in \cref{subsec:alg:onebucket}. Then, we demonstrate how to organize these buckets and set appropriate thresholds to control the error of every key within the user-defined threshold, as discussed in \cref{subsec:alg:formal:tech2}.


\begin{figure}[tbp]
    % \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/algo_graph2V2.pdf}
    \vspace{-0.15in}
    \caption{Operation Workflow.}
    \label{fig:operations:bucket}
    \postfig
\end{figure}



\presub
\subsection{Basic Unit: the Error-Sensible Bucket } \postsub
\label{subsec:alg:onebucket}

basic unit被定义为sketch中完成计数功能的最小功能单元。在counter-based的sketch中，basic unit是一个普通的counter。
我们\anamelong{}的基本单元是'Error-Sensible bucket'的结构，它可以主动感知发生了何种程度的哈希碰撞，并且对最大可能误差MPE进行估计。
The bucket supports two operations: (1) Insert a key-value pair; (2) Query the value sum of a key $\widehat{f_e}$ with its MPE.

The workflow is shown in Figure \ref{fig:operations:bucket}.

\ppp{Structure:}
Specifically, the bucket has three fields, one ID field recording the key of a candidate, and two counters recording the positive votes and negative votes, denoted as $ID$, $YES$ and $NO$, respectively. Initially, $ID$ is $null$ and both counters are $0$. 

\ppp{Insert a packet.}
When inserting a packet with flow ID $e$, there are two phases: replacement and voting.
First, we check whether $YES \leqslant NO$.
If so, we believe there are too many $NO$ votes, replace the recorded flow $ID$ with $e$.
In this case, $ID$ is not frequent enough to be kept and we can give other flows a chance to enter.
Then, we vote whether the recorded flow $ID$ is $e$ or not. 
If so, we vote YES by incrementing $YES$ by $1$.
Otherwise, we vote NO by incrementing the number of $NO$ by $1$.


\ppp{Query a flow.}
To query the flow size of $e$ in a bucket, we first check whether the recorded ID is flow $e$. If so, our estimation of the flow size $\widehat{f_e}$ is $YES$. Otherwise, $\widehat{f_e}$ is $NO$. The estimation is guaranteed to be no less than the true flow size (Proved by induction).
In both cases, MPE is $NO$. In other words, the bucket tells that the size of $ID$ is in range $[YES-NO, YES]$ and $[0, NO]$.
At a high level, $NO$ works because it can reflect the intensity of collisions between different flows.



\begin{figure}[tbp]
    % \prefig
    \centering  
    \includegraphics[width=0.98\linewidth]{vldb/Figures/algo/algo_graph1V2.pdf}
    \vspace{-0.15in}
    \caption{An Overview of \anamelong{}.}
    \vspace{-0.1in}
    \label{fig:algo:structure}
    \postfig
\end{figure}









\presub
\subsection{Formal \aname{}} \postsub
\label{subsec:alg:formal:tech2}



% The \anamelong{} consists of multiple layers, and each layer has an increasing warning threshold. These thresholds are at most $\Lambda$.
% When a flow’s error boundary (\ie, the maximum possible error) reaches the warning threshold in one layer, it will be inserted to the next layer. 



In this part, we show how to organize Error-Sensible buckets and assemble them into a \anamelong{}, in order to control per-flow error. The overview of \anamelong{} is shown in Figure \ref{fig:algo:structure}.
First, we introduce a new mechanism called ``lock'' to the bucket in order to control the error in the bucket.
Then, we show the data structure of the \anamelong{}, followed by the operations of insertion and query.



% \subsubsection{\textbf{Lock Mechanism}} $\ $

% \tex{Lock a bucket to control the error when necessary.}
\ppp{Lock Mechanism.}
When MPE of a bucket reaches a threshold, \ie, $B.NO=\lambda$, in order to stop the growth of MPE, we lock the bucket.
When we lock the bucket, only two cases of insertion are allowed, and they will not increase MPE (\ie, $B.NO$) :
\begin{itemize}[leftmargin=*]
    \item $B.ID=e$, which only increment $B.\hit$
    \item $B.YES\leqslant B.NO$, where a replacement happens and we increment $B.\hit$.
\end{itemize}
In other cases, packets cannot be inserted to the locked bucket. These packets are at higher risk of losing control and we will find other buckets for them.


\ppp{Data structure of \anamelong{}:}
As shown in Figure \ref{fig:algo:structure}, \anamelong{} has $d$ layers and each layer has many Error-Sensible buckets. The $j$-th bucket in the $i$-th layer is denoted as $B_i[j]$.
The width of the $i$-th layer (denoted as $w_i$) decreases as $i$ increases.
Each layer has a layer threshold to determine whether to lock the bucket, denoted as $\lambda_i$. 
$\lambda_i$ also decreases as $i$ increases and their sum does not exceed the user-defined error threshold, \ie, $\sum_i \lambda_i \leqslant \Lambda$.
Each layer has a independent hash function $h_i(\cdot)$, which uniformly maps each flow to one bucket in the layer. Detailed parameter settings are in \cref{subsec:math:parametersetting}.

% The warning threshold in layer $B_i$, denoted as $\Lambda_i$, is the sum of the layer thresholds of the first $i$ layers, \ie, $\Lambda_i=\sum_{k=1}^{i}\lambda_k$, and $\Lambda_i$.
% Each layer is associated with a pair-wisely independent hash function $h_i(\cdot)$, which maps each flow (denoted by $e$) into a random bucket (the $j$-th bucket $B_i[j], j=h_i(e)$) uniformly.




% The \anamelong{} consists of multiple layers, and each layer has many buckets.
% % \wyh{Then, we show how to combine these buckets and set thresholds to control the error of every flow to the user-defined threshold in Section.}
% % We present Double Exponential Control technique to handle all flows with large error boundaries.
% As mentioned in Section \ref{subsec:alg:struct}, \anamelong{} has multiple layers, and each layer has a number of buckets.
% Every Error-Sensible bucket in layer $i$ will not be locked until the error boundary reaches $\lambda_i$.
% The size of each layer decreases $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and the error threshold of each layer also decreases $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$.
% An ideal case is that the amount of flows entering each layer decreases much faster than $w_i$ and $\lambda_i$. But it is not easy to reach the ideal case.
% Now, we fully introduce the Double Exponential Control starting from the operations of \anamelong{}: Insertion and Query.






\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Insertion.}
    \label{alg:pseudo:Insertion:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$e$}}{
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
                        
            \If{($B_i[j].NO  < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].YES \leqslant B_i[j].NO$)}{
                \Comment{Insert to the first available bucket}
                % \Comment{}
                
                \If{$B_i[j].\hit \leqslant B_i[j].NO$}{ 
                    $B_i[j].ID\gets e$ \Comment{flow replacement}
                }
                                    % \Comment{Update counters}
                                    
                \eIf{$B_i[j].ID=  e$}{
                    $B_i[j].\hit\gets B_i[j].\hit+1$
                }{
                    $B_i[j].NO\gets B_i[j].NO+1$
                }
                % $InsertToBucket(e, B_i[j])$
                
                \textbf{break} \Comment{Succeed and Stop.}
            }
            % $i\gets i+1$ 
            % \Comment{Go to next layer}
        }
    
    }
\end{algorithm}

\subsubsection{\textbf{Insertion}} $\ $

\noindent{}We insert a packet $e$ to \anamelong{} by two steps, finding an available bucket and insert the packet to it. The pseudo-code is shown in Algorithm \ref{alg:pseudo:Insertion:all}.
For the first step, we start from the first layer and hash $e$ to a bucket of this layer, called \textit{mapped bucket} ($B_i[j], j=h_i(e), i=1$). 
Then we check whether $B_i[j]$ is an available bucket that can be inserted by $e$.
% where $e$ will not incur NOes to make the error greater than $\lambda_i$ (\ie, the error threshold of this layer).
The bucket is available in any of the following three cases: 
\vspace{-0.1cm}
\begin{itemize}[leftmargin=*]
    \item $B_i[j].NO < \lambda_i$: The bucket is not locked.
    \item $B_i[j].ID=e$: Only increment $B_i[j].\hit$
    \item $B_i[j].YES\leqslant B_i[j].NO$: A replacement happens and we increment $B_i[j].\hit$.
    % \item $B_i[j].ID=e$, which means $e$ will not incur NO.
    % \item $B_i[j].YES = B_i[j].NO$, which means we can replace the $B_i[j].ID$ by $e$.
\end{itemize}
\vspace{-0.1cm}
% \textit{(i)} $B_i[j].ID=e$, which means $e$ is an unlimited flow in this bucket; 
% 2) $B_i[j].low=0$, which means the new flow $e$ can replace the old flow $B_i[j].ID$; 
% \textit{(ii)} $\frac{1}{2}(B_i[j].total-B_i[j].low)< \lambda_i$, which means the error of this bucket is tolerable.
If the bucket is available, we insert $e$ into the bucket and completed the insertion.
Otherwise, $e$ is at higher risk of losing control, we keep finding an available bucket in the following layers until the last one.
In a few cases, the bucket in the last layer is unavailable and the insertion fails, which rarely ($<0.00001\%$) happens under our recommended parameters.
If the insertion failure really happens, we can use our emergency solution (\cref{extension:emergency}) to solve the problem.
% The insertion in the data plane is failed. 
% and we insert $e$ to a small stash to handle these flows. We will detail the stash later.
 



\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{Weighted Insertion.}
    \label{alg:pseudo:Insertion:all:Weighted}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{Insert}
    \SetKwProg{Fn}{Procedure}{:}{}
    \Fn{\FMain{$\langle e, w\rangle$}}{
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the $j$-th bucket by hashing}
            
            \If{$B_i[j].id==e$}{
                
                
                $B_i[j].YES\gets B_i[j].YES + w$
                
                \textbf{break} 
            }
            \eIf{$B_i[j].YES>\lambda_i$ \textbf{and} $B_i[j].NO+w>\lambda_i$}{
                $B_i[j].NO\gets \lambda_i$
                
                $f\gets B_i[j].NO+w-\lambda_i$
                
            }{
                \eIf{$B_i[j].NO+w>=B_i[j].YES$}{
                    $B_i[j].id\gets e$
                    
                    $NEW\_YES\gets B_i[j].NO+w$
                    
                    $B_i[j].NO\gets B_i[j].YES$
                    
                    $B_i[j].YES\gets NEW\_YES$
                }{
                    $B_i[j].NO\gets B_i[j].NO+w$
                }
                \textbf{break} 
            }
        }
    }
\end{algorithm}
Next, introduce how we insert a packet $e$ with weight $w$, where the weight can be the packet size in bytes.
The naive approach is to run basic insertion of $e$ by $w$ times, which is time consuming. Actually, we can do it at once (Algorithm \ref{alg:pseudo:Insertion:all:Weighted}). Similarly, from the first layer, we find the mapped bucket $B_i[j]$ by hashing and try to insert the packet into it.
First, if the recorded ID $B_i[j].id$ matches $e$, we just increase the $YES$ by $w$ and finish the insertion.
Otherwise, we know $B_i[j].id$ is not $e$.
Then, we check whether $B_i[j].NO$ can reach the layer error threshold $\lambda_i$. It has two conditions:
\begin{itemize}[leftmargin=*]
    \item $B_i[j].YES>\lambda_i$: No replacement will happen before the bucket is locked.
    \item $B_i[j].NO+w>\lambda_i$: The bucket can be locked if no replacement happens.
\end{itemize}
If so, we set $B_i[j].NO$ to threshold $\lambda_i$, and we save the frequency not inserted for later layers.
Otherwise, $B_i[j].NO$ will not reach $\lambda_i$.
We check whether the replacement will happen. If so, we just perform the replacement and update the counters. Otherwise, we just increase $B_i[j].NO$.


\begin{algorithm}[!h]
\renewcommand\baselinestretch{0.9}\selectfont
    \SetAlgoNoLine
    \caption{\anamelong{} Query.}
    \label{alg:pseudo:query:all}
    % \KwIn{a flow $e$}
    \SetKwFunction{FMain}{QueryFrequency}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$e$}}{
        % $InsertionSuccess\gets False$
        
        $ \widehat{f_e}\gets 0$  \Comment{Flow Size Estimator}
        
        % $ Ub\gets 0$ \Comment{Unbiased Estimator}
        
        $ MPE\gets 0$ \Comment{Maximum Possible Error}
    
        \For{Layer $i=1,2,\dots, d$}{
            $j\gets h_i(e)$  \Comment{Locate the bucket}
            
            \eIf{$B_i[j].ID=e$}{
                $\widehat{f_e}\gets \widehat{f_e} + B_i[j].YES$
                
                % $Ub\gets Ub+B_i[j].unbias$
            }{
                $\widehat{f_e}\gets \widehat{f_e} + B_i[j].NO$
                
                % $Ub\gets Ub+B_i[j].unbias-B_i[j].low\cdot S(B_i[j].ID)$
            }
            
            
            $ MPE\gets MPE + B_i[j].NO$
            
                        
            \If{ ($B_i[j].NO  < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].YES \leqslant B_i[j].NO$)}{
                \textbf{break} \Comment{Stop collecting flow sizes}
            }
        }
        $\widetilde{f_e}\gets \widehat{f_e} - MPE$
        
        \Return{$\langle \widehat{f_e}, \widetilde{f_e} , MPE\rangle$}
    }
\end{algorithm}

% \vspace{-0.3cm}

% \ppp{Query (Algorithm \ref{alg:pseudo:query:all}).} 

\subsubsection{\textbf{Query}} $\ $

\noindent{}When query the flow size of a flow $e$, \anamelong{} reports an over-estimated flow size $\widehat{f_e}$ with its MPE.
The pseudo-code is shown in Algorithm \ref{alg:pseudo:query:all}.
At every time inserting a flow, we only insert it into one bucket of a specific layer.
When querying, we just sum up its flow sizes in different layers. 
Starting from the first layer, we access the mapped bucket $B_i[j], j=h_i(e)$ layer by layer. 
We add up the estimated flow sizes and MPE, respectively. 
We can stop when the mapped bucket in layer $i$ is still available for $e$. Because in this case, $e$ must never be inserted to those later layers. 
Finally, we get the $\widehat{f_e}$ with its MPE.
We also get an interval that the true flow size $f_e$ must be in, \ie, $f_e \in \left[\widehat{f_e}-MPE, \widehat{f_e}\right]$.


\subsubsection{\textbf{Discussion}} $\ $

\ppp{Key Technique I (Error-Sensing).} 
To provide bilateral bounds, our approach is to replace the common counter of sketches with the Error-Sensible bucket as the basic unit.
The bucket uses voting that has been used by many algorithms \cite{frequent,tang2019mvsketch, yang2018elastic}, but we are the first to further analyze the negative votes to show MPE. 
% Based on the ability to sense the error, we devise the Double Exponential Composition technique, which not only covers the Error-Sensible bucket's disadvantages in both time and space but also performs much better than existing sketches.
% Compared with a simple counter, the bucket seems 
% The recorded ID is space-consuming and the insertion becomes more complex and time-consuming. These costs are worth paying, in order to get the ability to sense the error. 
% The time consumption is not significant because the main cost lies in memory access and hash calculation, rather than the insertion within the basic unit. 

\ppp{Key Technique II (Double Exponential Composition).}
To control the error of all flows reliably, we need to prevent insertion fails of breaking through the last layer. 
% An ideal goal is to insert all flows into the first few layers, not into the later layers.
In practice, it is critical for every layer to reduce the number of flows entering its next layers.
Under common parameters, each layer may stop half flows and the probability $\mathcal{P}$ that a flow fails to be inserted is $\frac{1}{2^d}$.
We found that, only when both the width $w_i$ and the layer threshold $\lambda_i$ decrease exponentially (\eg, $w_{i+1}=w_i/2, \lambda_{i+1}=\floor{\lambda_i/2}$), the failure probability $\mathcal{P}$ decreases at double exponential speed (\eg, $\frac{1}{2^{2^{d}}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$.}), which can overwhelm the number of flows and eliminate the insertion failure with extremely high probability.




% the effect is best only when we reduce the width and error threshold exponentially. Specifically, the rate of decline is double exponential.......

% We do not access all layers because if a mapped bucket in layer $B_i$ is available for $e$, $e$ must never be inserted to its following layers and we stop at the $i$-th layer.
% In a few cases, we do not stop at the last layer. We estimate the frequency in the stash and add it to the total frequency.


% \presub
% \subsection{Extensions} \postsub

% \subsubsection{Freely turning the accuracy of priority flows.}


% The extended Priority TrustySketch (\anamesum{} for short) can adjust the estimation accuracy of any flow. We can improve the accuracy of a high-priority flow (\eg, a flow with high SLA requirement) by giving it a weight. The weight of flow $e_i$, denoted as $w_i$, is an user-defined positive integer and it can improve the guaranteed accuracy from the old $\Lambda$ to $\lfloor \frac{\Lambda}{w_i} \rfloor$. Therefore, when $w_i$ is set to $\lfloor w_i \rfloor$, the estimation of flow $e_i$ must be correct.
% The key idea of inserting a packet $e_i$ with weight $w_i$ is to insert a packet for $w_i$ times by common insert operation. 
% Instead of spending $w_i$ times of time, we can achieve the same insertion speed as usual by some reasonable modifications. 
% Increasing the accuracy of partial flow will consume more memory. For example, if we reduce the error of 10\% flow by 50\%, we need 10\% more memory. 
% % The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 
% % The new \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. 

% % The extended priority TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% % \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 


% \subsubsection{Improving the overall accuracy by a mice filter.}
% After achieving good theoretical results, the memory efficiency of \anamelong{} can be further optimized in practice.
% % In a switch, the memory reserved for the measurement function is scarce 
% The first layer of \anamelong{} is the largest layer and it takes more than $50\%$ space of the whole \anamelong{}. But the first layer is in efficient when there are quite a few mice flows in the traffic. The mice flows will increment the 'miss' counters sharply and lock most buckets in the first layers. In this case, many buckets are wasted to record the mice flows. 

% To tackle the mice flows, we replace the first layer with a small mice-flow filter and still controlling the error well. Specifically, inspired by CU \cite{estan2002cusketch}, the filter consists of two arrays ($F_1[]$ and $F_2[]$) and each array has $\frac{1}{2} w_1$ $L$-bit counters. For every flow ID $e$, we use two hash functions $h_1^{(1)}(.)$ and $h_1^{(2)}(.)$ to select two mapped counters $C_1=F_1[h_1^{(1)}(e)]$ and $C_2=F_1[h_1^{(1)}(e)]$. To insert a packet with flow ID $e$, if 
% any of its two mapped counters is less than $\lambda_1$, we regard it as a mice flow. For a mice flow, we drop it and increment the minimal mapped counter(s) less than $\lambda_1$ by one. Otherwise, when both mapped counters equal to $\lambda_1$, we regard it as a non-mice flow, and pass the packet to the second layer.
% In practice, 8-bit counters are sufficient for the filter. Compared to a layer composed of 72-bit Error-Sensible buckets, the filter can reduce the space cost of layer-1 nearly $10$ times while incurring small controllable errors. The overall accuracy will be significantly improved when we move the space saved by the filter to the other layers. But we cannot replace other layers by the filter because the filter cannot estimate elephant flows well.

% \presub
% \subsection{More Functions of \anamelong{}} \postsub
% \label{extend}


% Our \anamelong{} has good versatility for various scenarios. We take the two most concernful tasks as examples, weighted counting and unbiased frequency estimation. We only introduce the key idea of how to achieve them.

% \ppp{Weighted Counting.} The extended Weighted TrustySketch (\anamesum{} for short) can achieve the same accuracy performance as \anamelong{} without visible loss of time and space. The operation of inserting a flow $e$ with weight $w_e$ in \anamesum{} has the same effect as inserting flow $e$ for $w_e$ times in \anamelong{}. 
% \anamesum{} has comparable insertion time cost as \anamelong{}, instead of $w_e$ times. The additional space consumption of \anamesum{} is due to the increase in the value range of the counter. 

% \presub
% \subsection{Discussions} \postsub
% \label{subsec:alg:discussion}

% We shortly review the design and discuss the design choices.
% In \anamelong{}, we devise Error-Sensible buckets that can sense the error of both mice and elephant flows, and combine them into a multi-layer structure to eliminate the flows at the risk of losing control.

% \noindent\textbf{How we design the Error-Sensible bucket?} We try to design the most simple error-sensible structure so that it can implemented in various platforms, especially the programmable switch. The bucket has only two counters and one ID, which can hardly be further simplified.

% \noindent\textbf{Compared with a simple counter, what is the disadvantage of the Error-Sensible bucket as a basic unit?} The recorded ID consumes a lot of space, and the insertion becomes more complex and time-consuming. These costs are worth paying, in order to get the ability to sense the error. The time consumption is not significant because the main cost lies in memory access and hash calculation, rather than the insertion within the basic unit. 
% Based on the ability to sense the error, we devise the Double Exponential Composition technique, which not only covers the disadvantages of the Error-Sensible bucket but also performs much better than existing sketches.

% \noindent\textbf{What is the difference of the multi-layer structure of \anamelong{} and the traditional multi-layer structure?} The key difference is that we have no copy and can quickly reduce flows layer by layer.
% Existing sketches, including CM, CU, and Count, have multi-layers and may update multiple counters when inserting one packet, which is called copy. We only update one counter for each packet, which makes \anamelong{} accurate and memory-efficient.
% Our multi-layer buckets can reduce both elephant flows and mice flows. In contrast, traditional methods \cite{coldfilter,lu2008counterbraids} insert all remaining flows to the next layer when a counter is large, which method will insert most elephant flows to the next layer and cannot reduce elephant flows effectively.
% Thanks to efficiently reducing flows, every packet only needs to access $1\sim 2$ layers in average, which makes \anamelong{} fast. Never seen before, \anamelong{} can reduce flows at the double exponential speed (proved mathematically in \cref{sec:math} and experimentally in \cref{subsubsec:exp:control}).


% Before a bucket is locked, we have the following theorem:
% \begin{theorem} 
%     \label{alg:theorem:NO}
%     $B_i[j].NO$ is no greater than the total frequency of all flows except for the most frequent flow.
% \end{theorem}
% \ppp{Bounded lock probability for any flow.} Base on Theorem \ref{alg:theorem:NO}, the bucket can ensure that, when we know that an arbitrarily frequent flow will be inserted to the bucket, whatever its arriving time, the probability of the bucket being locked is small and bounded.
% This is the key point that our algorithm can achieve better theoretical complexity in both time and space (detailed in Section \ref{sec:math}).
% When we lock the bucket, some flows will be inserted into the next layer. We use the next technique to handle these flows.




% \wyh{ Due to space limitations, we leave the detailed \anamesum{} algorithm to the reader, which is not the primary focus of this paper.}

% \ppp{Unbiased Frequency Estimation.} 
% Rather than guaranteeing one-side error\footnote{The estimations from \anamelong{} must be no less than the true frequency}, we can extend \anamelong{} to provide the unbiased estimated frequency whose expected value is the true frequency.
% We only introduce how to provide unbiased frequencies in one Error-Sensible bucket.
% It can be directly extended to the entire algorithm.
% To provide unbiased estimation, for each Error-Sensible bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. Initially, $B_i[j].unbias$ is $0$. For each flow $e$ to be inserted, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. 
% When queried flow $e$, a simple but correct approach is to report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency. That is because $E[S(e)\cdot B_i[j].unbias]=E[f(e)]+\sum_{x\in U \setminus {e}} E[S(x)]\cdot E[S(e)f(x)]=f(e)$, where $U$ is the universe of all flows. But in this case, we cannot sense the error and control it below $B_i[j].NO$.
% Actually, we can subtract the frequency of $B_i[j].ID$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{ID}\big)$, where $F_{ID}=S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].NO)$.
% In this case, the error boundary is $2\cdot B_i[j].NO$.


% \ppp{Insertion (Algorithm \ref{?}).}
% In the task of SUM (Defined in Section \ref{??}), each inserted flow includes an identifier $e$ and weight $w_e (w_e>0)$.
% The insertion of \anamesum{} is similar to inserting $e$ by \anamecount{} for $w_e$ times.
% Let variable $W$ represent the remaining weight to be inserted. Its initial value is $w_e$. Every time we find an available bucket, we try to insert into it. First, we calculate how much weight (denoted as $W_0$) can be inserted into the current bucket at most. The $W_0$ is the minimum value of the remaining weight ($W$) and the maximum weight that the bucket can hold $\lambda_i-B_i[j].NO$ before being locked. 
% Next, we insert $e$ with weight $W_0$ to the bucket directly.
% We add up the total flows by $W_0$ and then add up the NO number if needed.
% If the flow replacement is triggered, we replace the flow and correct the number of NOes to $B_i[j].YES$.

% % similar to xxx to insert w0 into the bucket. Next, continue to find the next feasible bucket for insertion until the frequency W to be inserted is equal to 0.

% \ppp{Query.}
% The query asks the total weight of an given flow identifier $e$. 
% The query of \anamesum{} is the same as that of \anamecount{}.

    % \begin{algorithm}[!h]
    %     \SetAlgoNoLine
    %     \caption{Insertion in Sum Task}
    %     \KwIn{a flow $e$ and its weight $w_e$}
    %     \SetKwFunction{FMain}{Insert???}
    %     % \SetKwProg{Fn}{Procedure}{:}{}
    %     % \Fn{\FMain{$e, w_e$}}{
                
    %         $W\gets w_e$ \Comment{The total amount to be inserted}
            
    %         \For{Layer $i=1,2,\dots, d$}
    %         {
    %             $j\gets h_i(e)$  \Comment{Locate the bucket $B_i[j]$}
                            
    %             \If{$(B_i[j].NO < \lambda_i$ \textbf{or} $B_i[j].ID=e$ \textbf{or} $B_i[j].YES \leqslant B_i[j].NO)$}{
                    
    %                 \If{$B_i[j].ID = null$}{ 
    %                     $B_i[j].ID\gets e$ 
    %                 }
    %                                             \Comment{The amount to be inserted into this bucket}
                                                
    %                 $W_0\gets min(W, \lambda_i-B_i[j].NO)$
                    
    %                 $W\gets W-W_0$
                    
    %                 $B_i[j].total\gets B_i[j].total+W_0$ 
                    
    %                 \If{$B_i[j].ID\neq e$}{
    %                     $B_i[j].NO\gets B_i[j].NO+W_0$
    %                 }
                    
    %                 \If{$B_i[j].YES = B_i[j].NO$}{
    %                     $B_i[j].ID\gets e$ \Comment{flow replacement}
                        
    %                     $B_i[j].NO\gets B_i[j].YES$
    %                 }
    %                 \If{$W = 0$}{
    %                     \textbf{break}
    %                 }
    %             }
    %         }
            
    %     % }
    % \end{algorithm}



% \presub
% \subsection{\anamelong{} for Unbiased Estimation} \postsub
% \label{}


% \begin{algorithm}[!h]
%     \SetAlgoNoLine
%     \caption{Unbiased Estimation in Error-Sensible bucket}
%     \label{alg:pseudo:bucketinsert}
%     % \KwIn{a flow $e$}
%     \SetKwFunction{FMain}{InsertToBucket}
%     \SetKwProg{Fn}{Procedure}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         $B_i[j].unbias\gets B_i[j].unbias+S(e)$
        
%         \If{$B_i[j].YES = B_i[j].NO$}{ 
%             $B_i[j].ID\gets e$ \Comment{flow replacement}
%         }
%                             % \Comment{Update counters}
%         \If{$B_i[j].ID\neq e$}{
%             $B_i[j].NO\gets B_i[j].NO+1$
%         }
%         $B_i[j].total\gets B_i[j].total+1$
%     }
    
%     \SetKwFunction{FMain}{QueryBucket}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Fn{\FMain{$e, B_i[j]$}}{
%         % $InsertionSuccess\gets False$
            
%             \eIf{$B_i[j].ID=e$}{
%                 $Ub\widehat{f_e}\gets  S(e)\cdot B_i[j].unbias$
                
%             }{
%                 $Ub\widehat{f_e}\gets   S(e)\cdot \big(B_i[j].unbias-S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].NO)\big)$
                
%             }
            
%             $MaxError\gets 2\cdot B_i[j].NO$
            
%         \Return{$\langle UbFreq, MaxError\rangle $}
%     }
% \end{algorithm}


% The \anamelong{} introduced above provides an estimated frequency that must be greater than the true frequency. In this part, we provide an unbiased frequency whose expected value is equal to the true frequency. We only introduce how to provide unbiased frequencies in one Error-Sensible bucket. It can be directly extended to the entire algorithm. To provide unbiased estimation, for each Error-Sensible bucket, we need to add one counter to it, denoted as $B_i[j].unbias$. The initial value of $B_i[j].unbias$ is $0$.

% \ppp{Insertion.} For each flow $e$, we add $S(e)$ to $B_i[j].unbias$, where $S(\cdot)$ is a hash function mapping flows to $\{+1, -1\}$ randomly. Then we update the bucket in the same way as the basic version.

% \ppp{Query.} Given the queried flow $e$. If it is $B_i[j].ID$, we report $S(e)\cdot B_i[j].unbias$ as its unbiased frequency ($UbFreq$). Otherwise, we subtract the frequency of $B_i[j].ID$ from $B_i[j].unbias$, and report the result. $UbFreq=S(e)\cdot \big(B_i[j].unbias-F_{ID}\big)$, where $F_{ID}=S(B_i[j].ID)\cdot(B_i[j].total-2\cdot B_i[j].NO)$.
% Here we explain why the result is unbiased. Let $U$ be all flows that are inserted to this bucket, and let $f(\cdot)$ denote the frequency in this bucket.
% The $B_i[j].unbias$ equals to $\sum_{x\in U} S(x)f(x)$. 
% For the first case that $B_i[j].ID=e$, we have $E[S(e)\cdot B_i[j].unbias]=E[S^2(e)f(e)]+\sum_{x\in U \setminus {e}} E[S(e)S(x)f(x)]$. As $E[S(e)S(x)f(x)]=E[S(x)]E[S(s)f(x)]$ and $E[S(x)]=0$, we have $E[S(e)\cdot B_i[j].unbias]= f(e)$. Similarly, we can proof that the result in the second case ($e\neq B_i[j].ID$) is unbiased. In this case, we substract $F_{ID}$ from $B_i[j].unbias$ is to reduce the variance. 
% Particularly, the maximum possible error is $2\cdot B_i[j].NO$, which is slightly different from the basic algorithm with one-side error.

% \presub
% \subsection{Protective Measure for Emergency} \postsub




% \presub
% \subsection{Practical Configurations and Discussions} \postsub

% Given a goal, we estimate the resources required.

% Given resources, we estimate the best performance.

% strength and weakness?


==> vldb/Body/application.tex <==
% \begin{table*}
% \caption{Settings of \aname{} for different applications.}
% \label{table:extend}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% Applications&Input&Remove Duplicates&Input of \aname{}&Report\\
% % & &Duplicates&\aname{}&Report\\
% \hline
% Frequent Items&Item $e_i$&$\times$&$e_i$&top-$k$ largest $f_i$\\
% \hline
% Heavy Changes&Item $e_i$&$\times$&$e_i$&top-$k$ largest $\Delta f_i$\\
% \hline
% Persistent Items&Item $e_i$&$\checkmark$&$e_i$&top-$k$ largest $f_i$\\
% \hline
% Super-Spreaders&Pair $<\!e_i, e_j\!>$&$\checkmark$&$e_i$&top-$k$ largest $f_i$\\
% \hline
% \end{tabular}
% \end{table*}

\presec
\section{Applications} \postsec
\label{SEC:app}

We apply \aname{} to six data stream processing tasks: frequency estimation (Section \ref{subsec:alg:Standard}),
finding top-k frequent items (Section \ref{subsec:app:frequent}), finding heavy changes (Section \ref{subsec:app:change}), cardinality, frequency distribution, and entropy estimation (Section \ref{subsec:app:distribution}). 
%For each application, we describe the problem  addressed, the data structure, the insertion process, and the report process. 
%Note that we focus only on the variations of the approaches in the specific subsections.
% The settings of each application are shown in Table \ref{table:extend}.


\presub
\subsection{Finding Top-k Frequent Items} \postsub
\label{subsec:app:frequent}

%In this section, as an case study, we illustrate how to use \aname{} to find frequent items.
%First, we provide the formal definition of finding frequent items.

\ppp{Problem Statement:}
%Given a data stream $\mathcal{S}$ with $N$ distinct items $(e_1,e_2...,e_N)$, find all items $e_i$ whose frequency $f_i$ exceed a predefined threshold $\mathcal{T}$.
% a data stream $\mathcal{S}=\{e_1,e_2,e_3,\dots\}$ is a sequence of items, each of which could appear more than once. The number that an item $e$ appears is $e$'s
For a finite data stream $\mathcal{S}$ with $N$ distinct items, $e_1,e_2...,e_N$, find the items that have top-$k$ largest frequencies.

\ppp{Data Structure and Insertion:}
The \aname{} can be directly used to find frequent items, so we do not need any additional structure.
%Because \aname{} can be directly used to find frequent items, the insertion and report process are the same as presented in Section \ref{subsec:alg:vote}.

\ppp{Report:} 
We scan the bucket array, estimate the upper bound (Formula \ref{equation:upperbound}) of the frequencies of all recorded item IDs, and report the IDs that have top-$k$ largest frequencies.


% \ppp{Analysis:}
% \aname{} has the following advantages. 
% First, this data structure has high memory efficiency, since it uses no pointer and almost has no empty cells. 
% Second, each insertion only need to access one bucket. 
% %the time complexity for the insertion of each item is $O(d)$, because each item only needs to search in the Heavy Part of its corresponding bucket. 
% And this insertion can be accelerated through SIMD instructions \cite{simd}. After using SIMD, the access time of a bucket is similar to the time of one memory access.
% %
% %Third, \aname{} only needs one memory access per insertion, which can increase its speed because memory accesses often take much time.
% Third, \aname{} can achieve significantly smaller error than the unilateral accumulation of SS \cite{spacesaving} and USS \cite{unbiasedsketch}, which is proved in theory (see Appendix \ref{subsec:appen:error}) and experiments (see Section \ref{sec:experiments}).

%and the estimated frequency of \aname{} is unbiased, which is proved in Section \ref{subsec:math:unbiased}.


\presub
\subsection{Finding Heavy Changes} \postsub
\label{subsec:app:change}
\ppp{Problem Statement:}
A data stream $\mathcal{S}$ is divided into two equal-sized periods: $S_1$ and $S_2$.
Let $f_i^{'},f_i^{''}$ be the frequency of item $e_i$ in $S_1$ and $S_2$ respectively.
The frequency change $\Delta f_i$ was defined as $\left|f_i^{'}-f_i^{''}\right|$.
Finding Heavy Changes is to find the items that have top-$k$ largest $\Delta f_i$.


\ppp{Data Structure:}
We build an \aname{} for every period to record frequent items, and compare the frequent items in adjacent periods to find heavy changes.

\ppp{Insertion:} 
For each input $e_i$, we insert $e_i$ to the \aname{} according to its period. The insertion process is the same as that in Section \ref{subsec:alg:Standard}.

\ppp{Report:} 
For two adjacent periods, we traverse all items whose IDs are recorded in the two corresponding \aname{}es.
For each item $e_i$, we query its frequency in the two \aname{}es, and get two frequencies, \ie $f_i^{'}$ and $f_i^{''}$.
%If the difference between the two frequencies is larger than a predefined threshold $\mathcal{T}$, then the item is reported as a heavy change. 
We calculate $\Delta f_i$ for each item, and report the items with top-$k$ largest $\Delta f_i$.

\presub
\subsection{Real time Cardinality \& Frequency Distribution \& Entropy Estimation} \postsub
\label{subsec:app:distribution}
\ppp{Problem Statement:} For a finite data stream $\mathcal{S}$, suppose that it is a sequence of $M$ items and it consists of $N$ distinct items, $e_{i_1},e_{i_2}...,e_{i_N}$. 
Let $n_f$ denotes the number of distinct items whose frequencies in $\mathcal{S}$ are equal to $f$. 
Cardinality estimation is to estimate the number of distinct items, \ie, $N$.
Frequency distribution estimation is to estimate $\phi=\left\{\frac{n_1}{N}, \frac{n_2}{N}, \dots, \frac{n_M}{N}\right\}$.
Entropy estimation is to estimate $H=-\sum{\frac{n_i}{N} ln\left(\frac{n_i}{N}\right)}$.

\ppp{Data Structure and Insertion:}
The structure and the method of insertion are the same as the standard version. 
We use an auxiliary array $C[f]$ to records the number of distinct items whose frequencies in $\mathcal{S}$ is equal to $f$.
The array $C[]$ is initialized by $0$.
When inserting an item $e_i$, we calculate its frequency $\widehat{f^{up}_i}$ and increase $C[\widehat{f^{up}_i}]$ by $1$. Then we decrease $C[\widehat{f^{up}_i}-1]$ by $1$ if both $\widehat{f^{up}_i}-1$ and $C[\widehat{f^{up}_i}-1]$ not equals to $0$.

\ppp{Report Cardinality:} We report the sum of auxiliary array $C[]$, \ie, $\widehat{N}=\sum_f{C[f]}$.

\ppp{Report Frequency Distribution:} We report the distribution \\ $\widehat{\phi}=\left\{\frac{C[1]}{N}, \frac{C[2]}{N}, \dots, \frac{C[M]}{N}\right\}$.

\ppp{Report Entropy:} We report the entropy $\widehat{H}=-\sum{\frac{C[i]}{N} ln\left(\frac{C[i]}{N}\right)}$.


% We estimate the distribution of frequent items and that of infrequent items respectively in order to get the total result of frequency distribution.
% For frequent items, we scan the bucket array and estimate the frequencies (by Formula \ref{equation:upperbound}) of all recorded item IDs. 
% For infrequent items, we generate the Light \aname{} (by Formula \ref{formula:light}) and implement MRAC algorithm \cite{MRACkumar2004data} on the Light \aname{}. The MRAC algorithm is an Expectation Maximization algorithm to iteratively compute the maximum likelihood distribution to result in the Light \aname{}. We sum the distribution of the frequent items and infrequent items to get the result.



% \presub
% \subsection{Entropy Estimation} \postsub
% \label{subsec:app:entropy}

% \ppp{Problem Statement:} For a finite data stream $\mathcal{S}$, suppose that it is a sequence of $M$ items and it consists of $N$ distinct items, $e_{i_1},e_{i_2}...,e_{i_N}$. 
% Let $n_f$ denotes the number of distinct items whose frequencies in $\mathcal{S}$ are equal to $f$. 
% Estimating the entropy is to estimate $H=-\sum{\frac{n_i}{N} ln\left(\frac{n_i}{N}\right)}$.


% \ppp{Data Structure:}
% We build an additional hash table $C[f]$ which records the number of distinct items whose frequencies in $\mathcal{S}$ is equal to $f$.

% \ppp{Insertion:} 
% For each input $e_i$, we insert $e_i$ to the \aname{}. The insertion process is the same as that in Section \ref{subsec:alg:vote}.

% \ppp{Report:} We compute the entropy based on the frequency distribution (Section \ref{subsec:app:distribution}) directly.

==> vldb/Body/applivationV2.tex <==

\presec
\section{Applications} \postsec
\label{SEC:app}

We apply \aname{} to four network measurement tasks: finding top-k frequent flows, cardinality estimation,  flow size distribution estimation, and entropy estimation.



\presub
\subsection{Finding Top-k Frequent Flows} \postsub
\label{subsec:app:frequent}

%In this section, as an case study, we illustrate how to use \aname{} to find frequent items.
%First, we provide the formal definition of finding frequent items.

\ppp{Problem Statement:}
%Given a packet stream $\mathcal{S}$ with $N$ distinct items $(e_1,e_2...,e_N)$, find all items $e_i$ whose frequency $f_i$ exceed a predefined threshold $\mathcal{T}$.
% a packet stream $\mathcal{S}=\{e_1,e_2,e_3,\dots\}$ is a sequence of items, each of which could appear more than once. The number that an item $e$ appears is $e$'s
For a finite packet stream $\mathcal{S}$ with $N$ flows, $e_1,e_2...,e_N$, the flows with top-$k$ largest sizes are top-$k$ frequent flows.
% Heavy hitters are the flows whose sizes are greater than a threshold $T$.

\ppp{Data Structure and Insertion:}
The \aname{} can be directly used to find frequent flows, so we do not need any additional structure.
%Because \aname{} can be directly used to find frequent items, the insertion and report process are the same as presented in Section \ref{subsec:alg:vote}.

\ppp{Report with no missing (100\% recall rate):} 
We scan the bucket array, estimate the flow size interval of all recorded flows. We sort these flow by their lower bound and choose the $k$-th largest lower bound (denoted by $L$). The true size of the $k$-th largest flow is at least $L$. Then we report all flows whose upper bounds are at least $L$. If the $k$-th largest flow is not too small (smaller than our error threshold $\Lambda$), we can actively report to the user that we definitely not miss any top-$k$ flow.

\ppp{Report with no false frequent flow (100\% precision rate):} 
We scan the bucket array, estimate the flow size interval of all recorded flows. We sort these flow by their upper bound and choose the $k$-th largest upper bound (denoted by $L$). The true size of the $k$-th largest flow is at most $L$. Then we report all flows whose upper bounds are at least $L$. If the $k$-th largest flow is not too small (smaller than our error threshold $\Lambda$), we can actively report to the user that all our reported flows are true top-$k$ flows.



% \ppp{Analysis:}
% \aname{} has the following advantages. 
% First, this data structure has high memory efficiency, since it uses no pointer and almost has no empty cells. 
% Second, each insertion only need to access one bucket. 
% %the time complexity for the insertion of each item is $O(d)$, because each item only needs to search in the Heavy Part of its corresponding bucket. 
% And this insertion can be accelerated through SIMD instructions \cite{simd}. After using SIMD, the access time of a bucket is similar to the time of one memory access.
% %
% %Third, \aname{} only needs one memory access per insertion, which can increase its speed because memory accesses often take much time.
% Third, \aname{} can achieve significantly smaller error than the unilateral accumulation of SS \cite{spacesaving} and USS \cite{unbiasedsketch}, which is proved in theory (see Appendix \ref{subsec:appen:error}) and experiments (see Section \ref{sec:experiments}).

%and the estimated frequency of \aname{} is unbiased, which is proved in Section \ref{subsec:math:unbiased}.



% A packet stream $\mathcal{S}$ is divided into two equal-sized periods: $S_1$ and $S_2$.
% Let $f_i^{'},f_i^{''}$ be the frequency of flow $e_i$ in $S_1$ and $S_2$ respectively.
% If the frequency change $\Delta f_i$ was defined as $\left|f_i^{'}-f_i^{''}\right|$. Finding Heavy Changes is to find the items that have top-$k$ largest $\Delta f_i$.



% \ppp{Data Structure:}
% ???

% \ppp{Insertion:} 
% For each input $e_i$, we insert $e_i$ to the \aname{} according to its period. The insertion process is the same as that in Section \ref{subsec:alg:Standard}.

% \ppp{Report:} 
% For two adjacent periods, we traverse all items whose IDs are recorded in the two corresponding \aname{}es.
% For each item $e_i$, we query its frequency in the two \aname{}es, and get two frequencies, \ie $f_i^{'}$ and $f_i^{''}$.
% %If the difference between the two frequencies is larger than a predefined threshold $\mathcal{T}$, then the item is reported as a heavy change. 
% We calculate $\Delta f_i$ for each item, and report the items with top-$k$ largest $\Delta f_i$.

\presub
\subsection{Other Tasks} \postsub
\label{subsec:app:distribution}
\ppp{Problem Statement:} For a finite packet stream $\mathcal{S}$, suppose that it is a sequence of $M$ items and it consists of $N$ distinct items, $e_{i_1},e_{i_2}...,e_{i_N}$. 
Let $n_f$ denotes the number of distinct items whose frequencies in $\mathcal{S}$ are equal to $f$. 
Cardinality estimation is to estimate the number of distinct items, \ie, $N$.
Frequency distribution estimation is to estimate $\phi=\left\{\frac{n_1}{N}, \frac{n_2}{N}, \dots, \frac{n_M}{N}\right\}$.
Entropy estimation is to estimate $H=-\sum{\frac{n_i}{N} ln\left(\frac{n_i}{N}\right)}$.

\ppp{Data Structure and Insertion:}
The structure and the method of insertion are the same as the standard version. 
We use an auxiliary array $C[f]$ to records the number of distinct items whose frequencies in $\mathcal{S}$ is equal to $f$.
The array $C[]$ is initialized by $0$.
When inserting an item $e_i$, we calculate its frequency $\widehat{f^{up}_i}$ and increase $C[\widehat{f^{up}_i}]$ by $1$. Then we decrease $C[\widehat{f^{up}_i}-1]$ by $1$ if both $\widehat{f^{up}_i}-1$ and $C[\widehat{f^{up}_i}-1]$ not equals to $0$.

\ppp{Report Cardinality:} We report the sum of auxiliary array $C[]$, \ie, $\widehat{N}=\sum_f{C[f]}$.

\ppp{Report Flow Size Distribution:} We report the distribution \\ $\widehat{\phi}=\left\{\frac{C[1]}{N}, \frac{C[2]}{N}, \dots, \frac{C[M]}{N}\right\}$.

\ppp{Report Entropy:} We report the entropy $\widehat{H}=-\sum{\frac{C[i]}{N} ln\left(\frac{C[i]}{N}\right)}$.


% We estimate the distribution of frequent items and that of infrequent items respectively in order to get the total result of frequency distribution.
% For frequent items, we scan the bucket array and estimate the frequencies (by Formula \ref{equation:upperbound}) of all recorded item IDs. 
% For infrequent items, we generate the Light \aname{} (by Formula \ref{formula:light}) and implement MRAC algorithm \cite{MRACkumar2004data} on the Light \aname{}. The MRAC algorithm is an Expectation Maximization algorithm to iteratively compute the maximum likelihood distribution to result in the Light \aname{}. We sum the distribution of the frequent items and infrequent items to get the result.



% \presub
% \subsection{Entropy Estimation} \postsub
% \label{subsec:app:entropy}

% \ppp{Problem Statement:} For a finite packet stream $\mathcal{S}$, suppose that it is a sequence of $M$ items and it consists of $N$ distinct items, $e_{i_1},e_{i_2}...,e_{i_N}$. 
% Let $n_f$ denotes the number of distinct items whose frequencies in $\mathcal{S}$ are equal to $f$. 
% Estimating the entropy is to estimate $H=-\sum{\frac{n_i}{N} ln\left(\frac{n_i}{N}\right)}$.


% \ppp{Data Structure:}
% We build an additional hash table $C[f]$ which records the number of distinct items whose frequencies in $\mathcal{S}$ is equal to $f$.

% \ppp{Insertion:} 
% For each input $e_i$, we insert $e_i$ to the \aname{}. The insertion process is the same as that in Section \ref{subsec:alg:vote}.

% \ppp{Report:} We compute the entropy based on the frequency distribution (Section \ref{subsec:app:distribution}) directly.

==> vldb/Body/conclusion.tex <==
\presec
\section{Conclusion and Future Work} \postsec
\label{sec:conclusion}

Frequency estimation is an important issue that has been studied for a long period. We define the ErrorSensible ability of sensing and controlling the errors of all estimations.
We propose \anamelong{} algorithm to achieve ErrorSensible. 
In theory, \anamelong{} achieves better time and space complexity than existing results, which has not been improved since 2005.
In practice, \anamelong{} outperforms the others in accuracy, memory consumption, and throughput. 

In the future, we plan to deploying \anamelong{} in industrial scenarios, and derive more refined mathematical analysis to provide guidance for practice. 
This work does not raise any ethical issues.

==> vldb/Body/conclusionV2.tex <==

\vspace{-0.1in}
\presec
\section{Conclusion} \postsec
\label{sec:conclusion}

We devise ReliableSketch that can eliminate the outlier by bilateral tight error bounds and control the error of all flows below a small threshold $\Lambda$.
% at line rate
% define the problem of sensing and controlling per-flow error, aiming at reliable measurement results and visible per-flow error in practice.
Our ReliableSketch can work on the data plane of programmable switches at line rate under limited memory with ignorable failure probability (\eg, less than $ 0.1^{70}$).
We reduce space complexity of sketches from $O\left(\frac{N}{\Lambda} \times \ln(\frac{1}{\delta})\right)$ to $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$. 
We implement ReliableSketch on multiple platforms including CPU, FPGA and P4, and conduct experiments on a testbed and an event-level simulation platform.
Experimental results show that ReliableSketch outperforms existing sketches: under the same small memory, ReliableSketch can control all flows with nearly the best throughput, while its competitors have thousands of out-of-control flows. The source codes are released at Github \cite{opensource} anonymously.


This work does not raise any ethical issues.

==> vldb/Body/exp_app.tex <==
\presec
\section{Additional Experiments} \postsec
\label{sec:appendix:exp}

\subsection{Experiments on Parameters}
\postsub
\label{app:exp:param}

We conduct several experiments to explore how the parameters $R_w$, $R_\lambda$ and the error threshold $\Lambda$ affect the performance of \aname{}. 
% \wyh{delete}
% based on two applications: error guarantee and frequency estimation.


\subsubsection{Impact of Parameter $R_w$. }
\label{subsubsec:exp:r_w}

When adjusting $R_w$ (\ie, the parameter of the decreasing speed of array size), we find \aname{} performs best when $R_w=2$.
% Considered the trade-off between the performance of error guarantee and frequency estimation, we find that it is relatively better to set the parameter $R_w$ to 2, which denotes the decrease speed of array size. Therefore, we finally set $R_w$ to 2 for the most of following experiments. 
% denotation: layer? decrease speed of array size

\input{vldb/Figures/nature/rw_range.tex}


\ppp{Memory Usage under Zero Outlier (Figure  \ref{subfig:nature:rw_range_caida}, \ref{subfig:nature:rw_range_webpage}):} 
%$\ppp{$R_w$ vs. Error Guarantee (Figure  \ref{subfig:nature:rw_range_caida}, \ref{subfig:nature:rw_range_webpage}):} 
We conduct experiments on IP Trace and Web Stream datasets. We set the user-defined threshold $\Lambda$ to 25, and compare the minimum memory consumption achieving zero outlier under different $R_w$.
It is shown that \aname{} with $R_w=2 \sim 2.5$ requires less memory than the ones with other $R_w$. When $R_w$ is lower than 1.6 or higher than 3, the memory consumption increases rapidly.

\input{vldb/Figures/nature/rw_freq.tex}

\ppp{Memory Usage under the Same Average Error (Figure  \ref{subfig:nature:rw_freq_caida}, \ref{subfig:nature:rw_freq_webpage}):} 
We conduct experiments on IP Trace and Web Stream datasets, set the target estimation AAE to 5, and compare the memory consumption when $R_w$ varies. The figures show that the higher $R_w$ goes with less memory usage. However, the memory consumption is quite close to the minimum value when $R_w= 2 \sim 6$. 

\subsubsection{impact of Parameter $R_\lambda$. }
\label{subsubsec:exp:r_l}
When adjusting $R_\lambda$ (\ie, the parameter of the decreasing speed of error threshold), we find \aname{} performs best when we set $R_\lambda=2.5$.
% We find that it is relatively better to set the parameter $R_\lambda$ to 2.5, which denotes the decreasing speed of error threshold. 

\input{vldb/Figures/nature/rl_range.tex}

\ppp{Memory Usage under Zero Outlier (Figure  \ref{subfig:nature:rl_range_caida}, \ref{subfig:nature:rl_range_webpage}):} 
We conduct experiments and set the target $\Lambda$ to 25. As the figures show, memory consumption drops down rapidly when $R_\lambda$ grows from 1.2 to 2 and finally achieve the minimum when $R_\lambda = 2$. There is no significant change when $R_\lambda$ is higher than 2.5, only some jitters due to the randomness of \aname{}. 

\input{vldb/Figures/nature/rl_freq.tex}

\ppp{Memory Usage under the Same Average Error (Figure  \ref{subfig:nature:rl_freq_caida}, \ref{subfig:nature:rl_freq_webpage}):} 
To explore the impact of parameter $R_\lambda$ on average error, we set the target estimation AAE to 5 and compare the memory consumption when $R_\lambda$ varies. It is shown that when $R_w$ is low, the higher $R_\lambda$ is, the less memory \aname{} uses. When $R_w$ is greater than 4, $R_\lambda$ affects little.

\subsubsection{Error Threshold $\Lambda$. }
\label{subsubsec:exp:eps}

We find that the user-defined error threshold $\Lambda$, which denotes the maximum estimated error \aname{} guaranteed, is almost inversely proportional to the memory consumption. In real tasks, we can implement \aname{} in a proper $\Lambda$ to meet our actual need better.

\input{vldb/Figures/nature/eps_range}

\ppp{Memory Usage under Zero Outlier (Figure \ref{subfig:nature:eps_range_caida}):} In this experiment, we fix the parameter $R_w$ to 2,  $R_\lambda$ to 2.5, and conduct it on three different datasets. 
It is shown that memory usage monotonically decreases, which means the optimal $\Lambda$ is exactly the maximum tolerable error.
% It is shown that memory usage monotonically decreases, which means the optimal $\Lambda$ is exactly the target guarantee range.
On the other hand, reducing $\Lambda$ blindly will lead to an extremely high memory cost.

\ppp{Memory Usage under the Same Average Error (Figure \ref{subfig:nature:eps_freq_caida}):} In this experiment, we fix the parameter $R_w$ to 2,  $R_\lambda$ to 2.5, and conduct it on IP Trace dataset. The figure shows that optimal $\Lambda$ increases as target AAE increases, and optimal $\Lambda$ is about 2 $\sim$ 3 times greater than target AAE. For target AAE=5/10/15/20, the optimums are 15/25/35/50, requiring 1.43/1.05/0.85/0.75MB memory respectively.


\subsection{Experiments on Datasets}
\postsub
\label{app:exp:datset}
We further conducts experiments on additional datasets.

\subsubsection{Additional Datasets. }
\begin{itemize}[leftmargin=0.15in]
    \item \ppp{ Cache Stream: } A  dataset built from real-world traffic distribution of CACHE. The first 10M packets of the whole trace are used to conduct experiments, including about 0.2M distinct flows.
    \item \ppp{ DCTCP Stream: } A  dataset built from real-world traffic distribution of DCTCP \cite{DCTCP}. The first 10M packets of the whole trace are used to conduct experiments, including about 1K distinct flows.
    % \item \ppp{ Click Stream: } A click stream dataset built from a hungarian online news portal  \cite{webpage}. We fetch the all 8M packets of the dataset for our experiments, containing about 41K distinct flows.
    \item \ppp{University Data Center: } An anonymized packet trace from university data center \cite{benson2010network}. We fetch 10M packets of the dataset, containing about 1M distinct flows.
    \item \ppp{Synthetic Datasets:} We generate \cite{webpoly} several synthetic datasets according to a Zipf distribution with different skewness for experiments, each of them consists of 32M packets.
\end{itemize}

\subsubsection{The Number of Outliers. } We conduct experiments on four additional datasets to explore the relation between the memory size and the number of outliers.

\input{vldb/Figures/app_new2/outlier_dataset}

\ppp{Impact of Dataset (Figure \ref{subfig:app:range25:webpage},\ref{subfig:app:range25:kosarak},\ref{subfig:app:range25:syn003},\ref{subfig:app:range25:syn030}):} We fix $\Lambda$ to 25 and change the dataset. The figures illustrate that \aname{} has the least memory requirement regardless of the dataset. 
% Space-Saving requires 2 $\sim$ 4 times more memory to achieve zero outlier than \aname{}.
% HeavyGuardian achieves stable performance on Web Stream and Click Stream datasets, because there are relatively less infrequent items than IP Trace. However, it still requires comparable amount of memory as Space-Saving.
% CU (accurate) requires 4 $\sim$ 8 times more memory and performs unstably in different datasets.
For synthetic dataset with skewness=0.3, no algorithm achieves zero outlier within 4MB memory, while the number of outliers of \aname{} is over 50 times less than others. 


\subsubsection{Average Error. }
We conduct experiments on two additional datasets to show the accuracy of \aname{} in average error by ARE and AAE.

\input{vldb/Figures/app_new2/avg_err_app}

\ppp{ARE \emph{vs.} Memory Size (Figure \ref{subfig:app:fe_are:webpage}, \ref{subfig:app:fe_are:syn030}):}
% It is shown that under-estimating \aname{} can keep an extremely low ARE even with limited memory consumption. This is because that most items are infrequent, and the under-estimating sketches often offer less error than the over-estimating ones when estimating their frequencies. 
It is shown that when memory size is up to 4MB, \aname{} achieves a comparable ARE with Elastic in two datasets, and is $1.63 \sim 2.75$ times lower than CU, $2.78 \sim 5.23$ times lower than CM, $2.76 \sim 5.05$ times lower than Coco, and $18.07 \sim 36.67$ times lower than Space-Saving.
% Note that ARE of \aname{} is about 2 times higher than CU Sketch when memory size is 200KB, because the derived $\Lambda$ is too large and the bottom layers are totally wasted. Under such a circumstance, we recommend to increase $R_w$ or decrease $d$ appropriately to enlarge the size of top layers.

% Indeed, \aname{} with higher $R_w$ can get better performance, but also results in more outliers. For the trade-off, extreme parameters are not recommended in common use.

\ppp{AAE \emph{vs.} Memory Size (Figure \ref{subfig:app:fe_aae:webpage}, \ref{subfig:app:fe_aae:syn030}):}
It is shown that when memory size is up to 4MB, \aname{} has a comparable AAE with Elastic and CU in two datasets, is about $1.59 \sim 2.01$ times lower than CM, $1.34 \sim 1.69$ times lower than Coco, and $9.10 \sim 11.48$ times lower than Space-Saving.

\subsection{Experiments on Throughput}
\postsub
\label{app:exp:throughput}

% \subsubsection{Hash Function Call. }

In common sketch algorithms, hash function always has higher computation complexity than other parts and affects the throughput a lot. Differed from prior sketches, \aname{} has a multi-layer structure. Hence the number of hash function calls is dynamic varied when performing insertions and queries. 
We conduct experiments on the IP Trace dataset to explore the relation between memory size and average number of hash function calls.

\input{vldb/Figures/tp_new2/tp_hash}

\ppp{\# Function Calls \emph{vs.} Memory Size (Figure \ref{subfig:tp:hash_insert},\ref{subfig:tp:hash_query}):} The figures show that average hash function calls of the raw version \aname{} goes down rapidly as memory grows, and finally converges to 1.  \aname{} with 2-array mice fitler finally converges to 3 for 2 extra calls in the filter.
% CM Sketch calls hash function 3 times per operation
% The figures show that the throughput of CM Sketch and CU Sketch is almost independent from the load rate, while the throughput of \aname{} goes down as load rate grows.
% can be easily found
Smaller \aname{} records more early-arrived but infrequent flows in the top layers, resulting in more hash function calls and poor throughput.
For this reason, as long as the memory is not particularly precious, we recommend offering more space in exchange for faster processing speed.

==> vldb/Body/experiments.tex <==
\presec
\section{Experiment Results} \postsec
\label{sec:experiments}

% In this section, we provide experimental results of \aname{}.
% We first introduce the experimental setup in \cref{subsec:exp:setup}. The performance of \aname{} depends on several factors, in \cref{subsec:exp:nature} we show how the parameters and data distribution affect it. In \cref{subsec:exp:app}, we apply \aname{} to five common applications and compare it with other prior algorithms. Benefited by the versatility, \aname{} has five extra operations, we measure the accuracy of them in \cref{subsec:exp:exop}. Finally in \cref{subsec:exp:throughput}, we make a comparison of the processing speed between \aname{} and prior algorithms. The source codes of \aname{} are  released at Github \cite{opensource} anonymously.
%     \input{vldb/Experiment/setup_2.tex}
% \input{vldb/Experiment/nature.tex}
% \input{vldb/Experiment/app.tex}
% \input{vldb/Experiment/exop.tex}
% \input{vldb/Experiment/throughput.tex}

In this section, we provide experiment results of \aname{}.
First, we introduce the experiment setup in \cref{subsec:exp:setup}.
Second, we show our performance on \goal{} in \cref{subsec:exp:sense_ctrl_err}. 
Third, we apply \aname{} to several network-wide applications by simulation in \cref{subsec:exp:sim}.
Finally, we implement \aname{} on the Tofino switch and evaluate the accuracy in \cref{subsec:exp:testbed}.
The source codes are released at Github \cite{opensource} anonymously.
\input{vldb/Experiment/setup_V3.tex}
\input{vldb/Experiment/sense_ctrl_err.tex}
\input{vldb/Experiment/sim.tex}
\input{vldb/Experiment/testbed.tex}



% \input{vldb/Experiment/nature_new.tex}
% \input{vldb/Experiment/nature_V3.tex}
% \input{vldb/Experiment/app_V3.tex}
% \input{vldb/Experiment/exop.tex}
% \input{vldb/Experiment/throughput_V3.tex}
% \input{vldb/Experiment/prior.tex}


==> vldb/Body/intro_backup.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub


%sketch方法
Accurate network measurement is often the first and fundamental step in many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, anomaly detection \cite{chen2020beaucoup,subsketchIMC}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}. 
These tasks benefit from precisely and timely network flow metrics including per-flow sizes, heavy hitters, heavy changes, or flow size distribution \cite{yang2018elastic}. 
Recently, the sketch algorithm \cite{zhang2021cocosketch,chen2021precise,liu2019nitrosketch,liu2016UnivMon, huang2021toward,huang2020omnimon,huang2017sketchvisor,huang2018sketchlearn,yang2018elastic}, which is compact and fast with small error, becomes the most promising solution.

% 第二段 现有工作：1、sketch的核心指标是误差。2、优化平均误差（部分、所有）。
% sketch在工业界部署的时候会遇到问题：如何感知和控制误差小于L。
% 现有sketch无法解决：1、理论无法解决。2、实践无法解决。来一个包希望感知误差。
% 重要性：放在sec2 也可以在下一段%计费 误差保证提供证据
% 第三段：重要性 design goal 
The core function of the sketch is to approximate/estimate per-flow size\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}, which enables a sketch to measure multiple network metrics in one small data structure \cite{liu2016UnivMon,yang2018elastic}.
In the simulation with known ground-truth\footnote{The true flow sizes.}, existing sketches show a small average error of flow sizes by directly comparing the estimated sizes with the ground-truth.
But in practice without the ground-truth, sketch users know nothing about the range/boundary
\footnote{The error refers to the absolute error of the flow size estimation: $AbsoluteError=|\hat{f_i}-f_i|$, where $\hat{f_i}$ is the estimated size and $f_i$ is the true flow size of flow $i$. The range of error is an interval. We mainly focus on its upper bound, \ie, the maximum possible error, which is also called the error boundary} of the error: 
When a sketch reports that the estimated flow size is $1000$, the true flow size/ground-truth can be 0 (Error=1000) or 5000 (Error=4000).
Naturally, we ask: For each estimation, can we know the upper bound of the error (\ie, maximum possible error or the error boundary) without the ground-truth (called Error-Sensing)?
If we know that the error is at most $10$, the true flow size must be in range $[990,1010]$. We will elaborate the benefits later.

%但是现有sketch都无法感知误差
While recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, they are neither concerned nor able to sense the error for all flows, let alone control the error.
In theory, without prior knowledge of the flow distribution, the error bound is too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. In addition, existing error bound is a bound of error distribution rather than a personalized feedback of the error for each estimation. 
For example, when a 3000-size flow is estimated to be 3010, what we hope to know is not "the error of 3010 is less than 200 with 90 probability", but "the error of 3010 must be less than 20".
In practice, existing sketches cannot sense the error. At a high level, they \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} use one counter to count the sizes of many flows, which method has no ability to sense the error. The errors of these sketches vary widely: from 0 to the largest flow size. This means that the estimated size of a mice flow may be larger than the size of the largest elephant flow, but sketches cannot sense the error and know whether each result is accurate enough.


Our goal is to sense the error for every flow and then control the worst-case error of all flows. 
% We name this the \textit{ErrorSensible} ability.
Specifically, for each flow, we find a dynamic error boundary that must be no less than the possible true error and changes as the true error changes. 
Each flow has its own independent and tight error boundary to show its maximum possible error with 100\% confidence.
Leveraging the error boundary, we aim to devise new strategy to control the error of all flows under the pre-defined user requirement. 
In this way, we can provide reliable estimations with visible error boundaries.



% (1) Hidden inaccurate reports. The inaccurate reports are always mixed with accurate reports and cannot be distinguished.% 随机隐藏
% When the user analyses the reports further, he/she must carefully consider the possibility that the reports are not accurate, even if they are of small amount.
% (2) Huge error of inaccurate reports. The errors of inaccurate reports are unbounded. In the worst case, the estimated frequency of a mice flow could be greater than the largest elephant flow. 
% The uncontrolled error deepens the user's concerns further.
% While recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, they cannot identify or eliminate inaccurate estimations.
% In other words, existing sketches can neither help users distinguish which flows are with inaccurate estimations, nor provide reliable per-flow statistics with the worst-case accuracy guarantee.


%我们的motivation，要做什么 感知和控制误差
Our goal is to sense the error for every flow and control the worst-case error of all flows. 
%这个名字感觉还是不行？因为没有包含控制。

% The accuracy of a sketch depends on its performance in per-flow size estimation. 





% Generally, under strict resource limitations, the sketch achieves high accuracy by compromising the reliability.

Not surprisingly, a sketch can estimate the size of most flows accurately, \eg, 95\% reported flow sizes are with error less than 10 (packets).


% 
% Generally, under strict resource limitations, the sketch achieves high average accuracy by compromising the reliability of every estimation report.
% Generally, under strict resource limitations, the sketch achieves high accuracy by compromising the reliability.
% 原理是啥
% 不知道误差是啥
% 实验测、理论bound
% 理论感知误差 实际感知误差
% per flow visibility
% 工业：这么大规模的网络流 能否让每个流误差都小于20。
%sketch error在给定memory下是最重要的，1、优化平均误差。minimize average error 通过和ground truth比较得到average error来证明误差的减小。但是实际中不实际，因为没有全流的ground truth。但现有算法无法感知每一条流有多大。
%2、没有感知误差 
%
% 能否让每个流误差都小于20。
% per

% 第二段：现有sketch优化平均误差，但无法控制每一个流误差小于L。认可sketch可以有小误差。工业界实现的时候，希望所有误差小于L。容忍小误差，不容忍大误差。零误差付出的代价太大了。重要性 有xxx收益，具体见xxx
% 第三段 goal：设计一个sketch算法，保证所有误差小于L 强调L是一个小值比如20 10
% 
% 每个流的误差大小-》超过我们的界-》控制     上做不到
% 第四段：
% 
% 100% 小于20  小于1000 99.99%
% handle xxx practical
% 问题：希望感知和控制流的误差小于20
% 相关工作：
% CM控制大部分流小于 
% 目标：感知控制每流误差小于L
% 
% 新问题
% 现有做不到新问题
% 做到新问题重要性
% 

% 完全掌控整个工具
% 第二段 现有工作：1、sketch的核心指标是误差。2、优化平均误差（部分、所有）。
% sketch在工业界部署的时候会遇到问题：如何感知和控制误差小于L。
% 现有sketch无法解决：1、理论无法解决。2、实践无法解决。来一个包希望感知误差。
% 重要性：放在sec2 也可以在下一段%计费 误差保证提供证据

% 第三段：重要性 design goal 


% Generally, under strict resource limitations, the sketch achieves high accuracy by compromising the reliability.
% The basic function of the sketch is to estimate the size of every flow\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}.
% Not surprisingly, a sketch can estimate the size of most flows accurately, \eg, 95\% reported flow sizes are with error less than 10 (packets).

% However, every report lacks reliability:
% (1) Hidden inaccurate reports\footnote{A reported frequency is accurate if its absolute error is no greater than a pre-defined threshold $\Lambda$. Otherwise, the report is inaccurate.}. The inaccurate reports are always mixed with accurate reports and cannot be distinguished.% 随机隐藏
% When the user analyses the reports further, he/she must carefully consider the possibility that the reports are not accurate, even if they are of small amount.
% % When the user analyses a reported frequency further, he/she must carefully consider the possibility that the report is not accurate, even if it happens with a small probability.
% % (2) Huge Worst-Case Error. In the worst case, the estimated frequency of a mice flow could be greater than the largest elephant flow. 
% (2) Huge error of inaccurate reports. The errors of inaccurate reports are unbounded. In the worst case, the estimated frequency of a mice flow could be greater than the largest elephant flow. 
% The uncontrolled error deepens the user's concerns further.
% % The completely uncontrolled worst-case deepens the user's concerns further.
% While recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, they cannot identify or eliminate inaccurate estimations.
% In other words, existing sketches can neither help users distinguish which flows are with inaccurate estimations, nor provide reliable per-flow statistics with the worst-case accuracy guarantee.


%我们的motivation，要做什么 感知和控制误差
Our goal is to sense the error for every flow and control the worst-case error of all flows. 
%这个名字感觉还是不行？因为没有包含控制。
% 控制可以不用controll manage管理 或者 steer掌舵领航？
% 叫AccuracyManage？
We name this the \textit{ErrorSensible} ability.
Specifically, for each flow, we find a dynamic error boundary that changes as the true error changes and must be no less than the true error. 
Each flow has its own independent error boundary to show its maximum possible error with 100\% confidence.
Then we can find hidden inaccurate reports out because their error boundaries must be larger than the requirement.
Leveraging the error boundary, we aim to devise new strategy to control the worst-case error of all flows under the user requirement. 
In this way, we can totally eliminate user concerns about inaccurate estimates.
We list four use cases as follows:


%目前的4个case：
%1、“资源调优”：现有sketch没有考虑实际分布，给的memory很大。我们可以通过感知的误差大小知道memory是分多了还是少了。进行可能的调整。
%2、不用为少量元素牺牲整体精度。计费场景使用CM sketch，整体减小20%来避免高估。知道每一个流的精度以后可以避免这个问题。
%3、不会把小流误分类为大流。拥塞时随机丢包不丢小流（控制信号）。
%4、方便故障定位。现有sketch算法允许存在严重误差，此时无法判定sketch算法的实现是否正确、参数配置是否合适。一个误差全可控的sketch可以快速的发现sketch是否时故障原因，进而排除故障。

%是否可以把1和4合并？合并成“方便故障定位+参数配置”。感觉单独去讲“sketch没有考虑实际分布，给的memory很大” 偏离了我们文章的重点。


% \textbf{Case IV:} Reliable fault diagnosis.
% Existing sketches often significantly over-estimates a few flows.
% %sketch运行 测试运行结果，当我们查看少数几个流
% When one flow is obviously over-estimated based on user knowledge, users cannot distinguish whether it is an accident in a normal sketch, or a malfunction caused by an incorrect configuration of the sketch. 
% When achieving ErrorSensible that can sense and control the error, user can affirm that the algorithm is misconfigured if there is one large error.
% % If we can achieve ErrorSensible, which senses and controls the error, we will make sure that the algorithm is misconfigured if there is one larger error.



% 这一段相关工作是不是删掉呢？因为前面讲了。
% 另外一个选择是，在这里讲space saving一类的确定性算法为什么不行。之前讲的都是带“失败”概率的sketch算法，比如CM sketch count sketch。


% \begin{comment}
% \vspace{-0.05in}
% \presec
% \subsection{Prior Art and Their Limitations} \postsec


\subsection{Our Proposed Approach}



We propose two techniques to address our goal of sensing and controlling the error.
First, we devise the \textit{Error-Sensing} technique that can estimate personalized error boundaries for every flow.
This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
Second, for those flows with risk, we devise the \textit{Double Exponential Composition} technique to control their error and eliminate inaccurate estimate.



%Double Exponential Composition
%Exponential Composition、superposition
%Composition比较好，有复合函数的“复合”，叠加的意思

\ppp{Key Technique I: Error-Sensing.} 
We argue that existing sketches cannot perceive the error because their basic unit is too weak.
% The basic unit of the data structure is the key to sense the error. 
For the well-known Count-Min sketch, its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
To replace the counter, we devise an Error-Sensible bucket, whose key idea is to bound the error by the number of "nay" when electing one frequent flow.
The bucket has three fields, including a candidate frequent flow, a counter of "yea", and a counter of "nay".
For each incoming packet, if it differs from the candidate, we increment "nay". Otherwise, we increment "yea". When there are too many nays, the recorded candidate item will probably be replaced.
\textbf{Our key novelty} is that \textit{we find and prove that the error is at most "nay"}, and thereafter we can build a sketch by properly organizing these buckets.
Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.


%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double Exponential Composition
\ppp{Key Technique II: Double Exponential Composition.} 
This technique aims to control the error of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the uncontrollable flows sharply by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
Using a straightforward solution, the probability can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}
Owing to the propose of double Exponential parameters, we strictly derive that \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space.

%and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 

\begin{figure}[htbp]
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
    \vspace{-0.15in}
    \caption{Paper Outline.}
    \label{fig:intro}
    \postfig
\end{figure}
% evaluation
%TBD ： new problem不准确
%

As shown in Figure \ref{fig:intro}, our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We define ErrorSensible and devise \anamelong{} that can sense and control the accuracy for every item.
    \item In theory, we prove that \anamelong{} outperforms state-of-the-art in both time complexity and space complexity.
    % There has been no breakthrough since 2005 \cite{cmsketch}.
    % And \aname{} can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We implement \anamelong{} in multiple platforms (\ie, CPU, FPGA, and Programmable Switch).
    Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double Exponential Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v1.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub

In high-speed data stream processing, counting the frequency of each data item and summing up the numeric attribute of each item are two critical statistic tasks with many applications \cite{?}.
%
For example, enterprise cloud service providers process the network traffic, where each data item is a packet with many attributes, including its size (Bytes), source IP address, and destination IP address, and they estimate the total size of the packets with the same source IP. 
Instead of estimating the results exactly, enterprises choose approximate algorithms like sampling \cite{?} and sketches \cite{?}, because only these algorithms can handle high-speed data ($100$ Million packets per second per switch) with low time and space cost.
In these scenarios, given an accuracy requirement (\ie, an error threshold) from the enterprise, approximate algorithms try to make all estimation results meet the requirement.
Unfortunately, there is always some estimations cannot meet the requirement.
If the absolute error of an estimation is greater than the error threshold, the estimation is called \textit{uncontrollable}.
% But a few results will deviate a lot.

% However, these approximate algorithms relying on probabilistic statistics cannot guarantee that all results meet the accuracy requirement, 
% 
These uncontrollable estimations that deviate a lot from the ground truths will lead to concernful problems in the following two real cases. 
%
%误差感知
%
\ppp{Case 1:} Hurt all estimations in accounting. The cloud service provider needs to monitor how much data traffic an user/service uses and send a bill. However, approximate algorithm may lead to significant over-estimation for a few users, but any seriously over-estimated bill is never tolerated.
These users are unknown for the enterprise. Therefore, a well-known enterprise has to reduce the estimated results of all users by $20\%$, which hurts the profit.
%
\ppp{Case 2:} Misclassification of frequent items. An infrequent item may have a large estimated frequency, and then it is mistaken for frequent items. In machine learning, existing works such misclassifications can seriously hurt many applications \cite{agument,a1,a2,a36} . In networking, an infrequent item (\eg, a flow identified by source IP and destination IP) is often a control signal packet, which are more important than frequent item. If the control signal is mistaken for frequent items, it may suffers packet loss or long latency.

\subsection{Prior Art and Their Limitations}

Unfortunately, existing approximate algorithms rely on probabilistic statistics and therefore they are always with uncontrollable estimations. 
The Count-Min (CM) sketch \cite{cmsketch} is a milestone with the best theoretical result.
A CM sketch consists of multiple arrays of counters. when counting frequency, for each incoming item, CM picks one counter (called \textit{mapped counters}) in every array by calculating hash value of the item's identifier, and then increment these mapped counters by one.
When querying the frequency of an item, CM reports the minimal counter among the mapped counters.
Given a data stream with $N$ items, when the absolute error of an estimation is smaller than $\epsilon N$ with high probability $1-\delta$ (\eg, $1-\delta=95\%$), CM needs $O(\ln(\delta)\frac{1}{\epsilon})$ space and can be built in real time by $O(\ln(\delta)N)$ totally.
Its followers \cite{???} improve the algorithms in many aspects, but none of them eliminates uncontrollable estimation or achieves better theoretical result.
\textbf{Our goal is eliminating uncontrollable estimations while achieving better performance in both time and space than state-of-the-art. }
% There are two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} If we solve challenge 1 that the maximum possible error is visible, we need a reliable control strategy to control every estimations that may be uncontrollable, and it still needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\subsection{Our Proposed Approach}

Our key idea is to perceive the error of each estimation and control the estimations with large errors. It raises two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} After the maximum possible error is visible, we need a reliable control strategy to control every estimations that may be uncontrollable (\ie, the absolute error is greater than given threshold), and it needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\ppp{Key technique 1: Error-visible unit.} The basic unit of the data structure is the key to know and control the error. For CM sketch, its basic unit is a counter, which estimate the frequency by the total number of items that mapped/hashed to it, no matter these items are the same or not. So CM cannot estimate the error. 
Our basic unit consists of a pair of counters and a identifier recorder.
The key idea is that we elect the frequent item and count different votes to bound the error. 
Together with artful update strategy and report approach, our basic unit can provide a maximum possible error feedback for any items mapped to it. 
When inserting a new item, if its maximum possible error is close to the error threshold, it is dangerous and we use the next technique to control its error.

%
\ppp{Key technique 2: ??-control structure.} To control all estimations under a threshold $\lambda$, we design a stair like structure consists of multiple layers, where each layer is an array of error-visible units and each layer has an increasing error warning threshold (\eg, $\lambda-\lfoor\frac{\lambda}{2^i}\rfoor$ for the $i$-th level).
To insert an item, we first pick one unit from the first layer by hashing, and then check whether the maximum possible error of the unit is smaller than the warning threshold. If so, we insert the item to the unit. Otherwise, we try to insert the item to the next layer.
Only a small portion of items will be insert to the next layer and the size of each layer (\ie, the number of units) decreases exponentially. 
It is notable that in most cases ($> 100\%-10^{-1000}$) there is no item can reach the last layer, because the number of items that enter each level decreases in double exponential speed, \ie, only $\frac{1}{2^{(2^{i})}}$ of items can enter the $(i+1)$-th level ($\frac{1}{2^{(2^{5})}}=2.3e-10$).


\ppp{Key contributions:}
\begin{itemize}
    \item We define .... propose a data stream sketching algorithm, called \aname{}, that can reliably control the estimation accuracy for all items.
    \item \aname{} outperforms state-of-the-art in both time complexity and space complexity, where has been no breakthrough since 2005 \cite{cmsketch}. And it can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We perform rigorous mathematical proofs and conducted comprehensive experiments on four datasets to verify the effectiveness of our algorithm.
\end{itemize}



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---Visible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\epsilon$, \ie, $|\hat{f}-f|<\epsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\epsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to invisible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become visible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \epsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v2.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub

In high-speed data stream processing, counting the frequency of each data item and summing up the numeric attribute of each item are two fundamental statistic tasks with many applications \cite{?}.
%
For example, enterprise cloud service providers process the network traffic, where each data item is a packet with many attributes, including its size (Bytes), source IP address, and destination IP address, and each query estimates the total size of the packets with the same source IP. 
Instead of estimating the results exactly, enterprises choose approximate algorithms like sampling \cite{?} and sketches \cite{?}, because only these algorithms can handle high-speed data ($100$ Million packets per second per switch) with low time and space cost.
In these scenarios, given an accuracy requirement (\ie, an absolute error threshold) from the enterprise, approximate algorithms try to make all estimations meet the requirement.
Unfortunately, there always exists some estimations (\eg, 5\% of the total) cannot meet the requirement, called \textit{uncontrollable estimations}. 
Moreover, these uncontrollable estimations are hard to detect and identify. Both the algorithm and the user cannot identify which estimations are uncontrollable.


% 
The unidentified uncontrollable estimations will lead to concernful problems in the following two aspects. 
%
\ppp{Aspect 1:} Hurt the accuracy of all estimations. In order to reduce the impact of uncontrolled estimations, the algorithm has to sacrifice the accuracy of all estimations. In a real case, a cloud service provider needs to monitor how much data traffic an user/service uses and send a bill. The approximate algorithm leads to significant over-estimation for a few unknown users. However, any seriously over-estimated bill is never tolerated. Therefore, a well-known enterprise has to reduce the estimated results of all users by $20\%$, which seriously hurts the profit of the enterprise.
%
\ppp{Aspect 2:} Misclassification of frequent items. An infrequent item may have a large estimated frequency, and then it is mistaken for frequent items. In machine learning, such misclassifications can seriously hurt many models \cite{agument,a1,a2,a36}. In networking, an infrequent item (\eg, a flow identified by source IP and destination IP) is often a control signal, which are more important than other items. If the control signal is mistaken for frequent items, it may suffers packet loss or long latency.

\subsection{Prior Art and Their Limitations}

Unfortunately, existing approximate algorithms rely on probabilistic statistics and therefore they are always with unidentified uncontrollable estimations. 
The Count-Min (CM) sketch \cite{cmsketch} is a milestone with the best theoretical result.
A CM sketch consists of multiple arrays of counters. when counting frequency, for each incoming item, CM picks one counter (called \textit{mapped counters}) in every array by calculating hash value of the item's identifier, and then increment these mapped counters by one.
When querying the frequency of an item, CM reports the minimal counter among the mapped counters.
Given a data stream with $N$ items, when the absolute error of an estimation is smaller than $\epsilon N$ with high probability $1-\delta$ (\eg, $1-\delta=95\%$), CM needs $O(\ln(\delta)\frac{1}{\epsilon})$ space and can be built in real time by $O(\ln(\delta)N)$ totally.
Its followers \cite{???} improve the algorithms in many aspects, but none of them eliminates uncontrollable estimation or achieves better theoretical result.
\textbf{Our goal is eliminating uncontrollable estimations while achieving better performance in both time and space than state-of-the-art. }
% There are two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} If we solve challenge 1 that the maximum possible error is visible, we need a reliable control strategy to control every estimations that may be uncontrollable, and it still needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\subsection{Our Proposed Approach}

Our idea is to perceive the error of each estimation and control the estimations with large errors. First, we perceive the maximum possible error of each estimation. Second, if the the maximum possible error becomes large and is close to the error threshold, we take actions to control the error. 
We propose two key techniques for the two steps.


% It raises two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} After the maximum possible error is visible, we need a reliable control strategy to control every estimations that may be uncontrollable (\ie, the absolute error is greater than given threshold), and it needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\ppp{Key technique 1: Error-visible unit.} The basic unit of the data structure is the key to know and control the error. For CM sketch, its basic unit is a counter, which estimate the frequency by the total number of items that mapped/hashed to it, no matter these items are the same or not. So CM cannot estimate the error. 
Our idea is to bound the error by the number of hash collisions during electing the frequent item.
Our error-visible unit has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
For each insertion of new item, if it is different from the candidate, a collision happens. When there is too many collisions, the new item can take place of the old candidate item.
We prove that the error is at most the number of collisions, so that we provide visible error feedback. 
In addition, the unit separates the most frequent flow from other infrequent flows, which is basis of our better time and space complexity.
% Our basic unit consists of a pair of counters and a identifier recorder.
% Together with artful update strategy and report approach, our basic unit can provide a maximum possible error feedback for any items mapped to it. 
When inserting a new item, if its maximum possible error is close to the error threshold, it is dangerous and we use the next technique to control its error.

%
\ppp{Key technique 2: Double exponential control.} We design a stair like structure consists of multiple layers, where each layer is an array of error-visible units and each layer has an increasing error warning threshold.
To control all estimations under a threshold $\lambda$, the warning threshold for the first level is $\frac{1}{2}\lambda$, $\frac{3}{4}\lambda$ for the second level, and $(1-\frac{1}{2^i})\lambda$ for the $i$-th level.
To insert an item, we first pick one unit from the first layer by hashing, and then check whether the maximum possible error of the unit is smaller than the warning threshold. If so, we insert the item to the unit. Otherwise, we try to insert the item to the next layer.
Only a small portion of items will be insert to the next layer and the size of each layer (\ie, the number of units) decreases exponentially. 
It is notable that in most cases ($> 100\%-10^{-100}$) there is no item can reach the last layer, because the number of items that enter each level decreases in double exponential speed, \ie, only $\frac{1}{2^{(2^{i})}}$ of items can enter the $(i+1)$-th level (\eg, $\frac{1}{2^{(2^{6})}}=5.4\cdot10^{-20}$). That is why this technique is called double exponential control.


\ppp{Key contributions:}
\begin{itemize}
    \item We define .... propose a data stream sketching algorithm, called \aname{}, that can reliably control the estimation accuracy for all items.
    \item \aname{} outperforms state-of-the-art in both time complexity and space complexity, where has been no breakthrough since 2005 \cite{cmsketch}. And it can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We perform rigorous mathematical proofs and conducted comprehensive experiments on four datasets to verify the effectiveness of our algorithm.
\end{itemize}



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---Visible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\epsilon$, \ie, $|\hat{f}-f|<\epsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\epsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to invisible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become visible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \epsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v3.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub


%sketch方法
Accurate network measurement is often the first and fundamental step in many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, anomaly detection \cite{chen2020beaucoup,subsketchIMC}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}. 
These tasks benefit from precisely and timely network flow metrics including per-flow sizes, heavy hitters, heavy changes, or flow size distribution \cite{yang2018elastic}. 
Recently, the sketch algorithm \cite{zhang2021cocosketch,chen2021precise,liu2019nitrosketch,liu2016UnivMon, huang2021toward,huang2020omnimon,huang2017sketchvisor,huang2018sketchlearn,yang2018elastic}, which is compact and fast with small error, becomes the most promising solution.

wyh to Prof. Yang: Please see following comments.
% 上次讨论的框架：
% 第二段 现有工作：1、sketch的核心指标是误差。2、优化平均误差（部分、所有）。
% sketch在工业界部署的时候会遇到问题：如何感知和控制误差小于L。
% 现有sketch无法解决：1、理论无法解决。2、实践无法解决。来一个包希望感知误差。
% 重要性：放在sec2 也可以在下一段%计费 误差保证提供证据
% 第三段：重要性 design goal 

%目前的框架：
% 第二段：现有sketch的核心功能是估计频数。但是现有sketch在没有ground-truth的情况下，无法知道误差。因此我们要知道error bound。（这里是初步提出我们的目标，不会显得太晚或者突兀）
% 第三段：现有sketch无法解决误差感知和控制。1、理论上无法解决（理论的bound很松不可用，理论的bound是分布的bound，而不是每一个估计值的bound）。2、实践上无法解决。现有sketch盲目地把多个流的混合在一个counter内，无法感知误差。
% 第四段：描绘我们的具体目标。并且描述重要性。

%现有写作的问题（我自己觉得还没解决好）
%1、误差感知过度到误差控制似乎不够自然
%2、之前计费的那个例子没有直接写在intro里，担心不够solid（因为实际上的计费并不是直接数总的包数量）。感觉是不是不写比较好？
The core function of the sketch is to estimate per-flow size\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}, which enables a sketch to measure multiple network metrics in one small data structure \cite{liu2016UnivMon,yang2018elastic}.
In the simulation with known ground-truth\footnote{The true flow sizes.}, existing sketches show a small average error of flow sizes by directly comparing the estimated sizes with the ground-truth.
\textbf{existing sketches compete for the small average error of flow sizes by directly comparing the estimated sizes with the ground-truth.}
But in practice without the ground-truth, sketch users know nothing about the range/boundary
\footnote{The error refers to the absolute error of the flow size estimation: $AbsoluteError=|\hat{f_i}-f_i|$, where $\hat{f_i}$ is the estimated size and $f_i$ is the true flow size of flow $i$. The range of error is an interval. We mainly focus on its upper bound, \ie, the maximum possible error, which is also called the error boundary} of the error: 
When a sketch reports that the estimated flow size is $1000$, the true flow size/ground-truth can be 0 (Error=1000) or 5000 (Error=4000).
Naturally, we ask: For each estimation, can we know the upper bound of the error (\ie, maximum possible error or the error boundary) without the ground-truth (called Error-Sensing)?
If we know that the error is at most $10$, the true flow size must be in range $[990,1010]$. We will elaborate the benefits later.


%但是现有sketch都无法感知误差
While recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, they are neither concerned nor able to sense the error for all flows, let alone control the error.
In theory, without prior knowledge of the flow distribution, the error bound is too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. In addition, existing error bound is a bound of error distribution rather than a personalized feedback of the error for each estimation. 
For example, when a 3000-size flow is estimated to be 3010, what we hope to know is not "the error of 3010 is less than 200 with 90 probability", but "the error of 3010 must be less than 20".
In practice, existing sketches cannot sense the error. The errors of these sketches vary widely: from 0 to the largest flow size. This means that the estimated size of a mice flow may be larger than the size of the largest elephant flow. The reason behind is that they \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} use one counter to count the sizes of many flows, which method has no enough ability to sense the error. 


Our goal is to sense the error for every flow and then control the worst-case error of all flows. 
% We name this the \textit{ErrorSensible} ability.
\textbf{We believe that making progresses in this direction can significantly accelerate the application of sketching algorithm into practices.}
Specifically, for each flow, we find a dynamic error boundary that must be no less than the possible true error and changes as the true error changes. 
Each flow has its own independent and tight error boundary to show its maximum possible error with 100\% confidence.
Leveraging the error boundary, we devise new strategy to control the error of all flows under a small user-defined threshold. 
The sensing and controlling the error will greatly improve the reliability and usability of sketch estimation results.



\subsection{Our Proposed Approach}



We propose two techniques to address our goal of sensing and controlling the error.
First, we devise the \textit{Error-Sensing} technique that can estimate personalized error boundaries for every flow.
This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
Second, for those flows with risk, we devise the \textit{Double Exponential Composition} technique to control their error and eliminate inaccurate estimate.


%老师，agree和disagree是不是可以考虑写成yea和nay, 这个是投票表决时候的专业术语，显得比较高级https://www.zhihu.com/question/36433186，分别表示赞同和反对。
%Double Exponential Composition
%Exponential Composition、superposition
%Composition比较好，有复合函数的“复合”，叠加的意思

\ppp{Key Technique I: Error-Sensing.} 
We argue that existing sketches cannot perceive the error because their basic unit is too weak.
For the well-known Count-Min sketch, its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
To replace the counter, we devise an Error-Sensible bucket, whose key idea is to bound the error by the number of "nay" when electing one frequent flow.
The bucket has three fields, including a candidate frequent flow, a counter of "yea", and a counter of "nay".
For each incoming packet, if it differs from the candidate, we increment "nay". Otherwise, we increment "yea". When there are too many nays, the recorded candidate item will probably be replaced.
\textbf{Our key novelty} is that \textit{we find and prove that the error is at most "nay"}, and thereafter we can build a sketch by properly organizing these buckets.
Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.


%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double Exponential Composition
\ppp{Key Technique II: Double Exponential Composition.} 
This technique aims to control the error of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the uncontrollable flows sharply by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
Using a straightforward solution, the probability can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}
Owing to the propose of double Exponential parameters, we strictly derive that \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space.

%and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 

\begin{figure}[htbp]
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
    \vspace{-0.15in}
    \caption{Paper Outline.}
    \label{fig:intro}
    \postfig
\end{figure}
% evaluation
%TBD ： new problem不准确
%

As shown in Figure \ref{fig:intro}, our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We define ErrorSensible and devise \anamelong{} that can sense and control the accuracy for every item.
    \item In theory, we prove that \anamelong{} outperforms state-of-the-art in both time complexity and space complexity.
    % There has been no breakthrough since 2005 \cite{cmsketch}.
    % And \aname{} can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We implement \anamelong{} in multiple platforms (\ie, CPU, FPGA, and Programmable Switch).
    Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double Exponential Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v4.tex <==


% 1、测量重要 sketch是重要手段
% 2、当前最典型的CMsketch被使用时遇到了一系列问题：
% 3、总结出缺陷背后的原因是无法误差感知和控制 
% 4、当前学界提出了很多sketch，但是这些sketch没有关注且无法解决这个问题。因此这个问题很重要急切。。。。

% 1 网络测量重要
% 2 部署的时候是没有truth的
% 3 感知并且控制误差
% 4 （讲challenge）
% 5 现有解决不了

% 1 背景
% 2 现有sketch 都是和truth比 聚焦在误差如何感知和控制
% 3 

% 相关工作 
% sub1、定义问题、讲例子重要性
% sub2 相关工作

\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub


%sketch方法
Accurate network measurement is often the first and fundamental step in many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, anomaly detection \cite{chen2020beaucoup,subsketchIMC}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}. 
These tasks benefit from precise and timely network flow metrics including per-flow sizes, heavy hitters, heavy changes, or flow size distribution \cite{yang2018elastic}. 
Recently, the sketch algorithm \cite{zhang2021cocosketch,chen2021precise,liu2019nitrosketch,liu2016UnivMon, huang2021toward,huang2020omnimon,huang2017sketchvisor,huang2018sketchlearn,yang2018elastic,mitzenmacher2017probability} becomes the most promising solution owing to its small memory usage and fast speed.
The main concern of using sketches is the error of flow size estimation\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}. 
% \sout{The main overhead of sketches is the introduce of error of flow size estimation}\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}. 
% 感觉sketch改成using sketch会更好一点？老师是想表达使用sketch的代价吗？
%  estimation似乎自带error，introduce 用在这里有一些奇怪？

%which is compact and fast with small error, 


%\wyh{Current sketches have a variety of functions, most of which are based on one fundamental function: estimating per-flow size


%第一段：测量背景、sketch和引入频数估计

%第二段：讲述我们遇到的实践困难
%中文意思：
%在实际使用中，我们遇到了一系列由频数估计误差导致的问题。
%例子1、误分类问题。当我们用sketch划分大小流的时候（根据阈值T=1000）。我们发现许多实际频数远小于T的小流的估计值大于T，被划分为大流。
% 后续的拥塞控制模块模块本想根据测量分类，来进行对大流进行随机丢包。但是由于测量模块的误差，部分作为控制信号的小流被误丢包了，可能产生严重的问题。因此我们只能给sketch成被地过量地分配空间以减缓这个现象。类似地，一些机器学习应用也不允许误分类。
%例子2、精度可信问题。给定误差阈值，用户要求每流误差小于阈值，这样才可以相信测量结果，并把它们进一步使用。（不用说具体怎么用，丢给用户）

%第三段：问题归因，无法感知控制误差。定义新问题：感知控制误差。解释感知和控制以后如何解决第二段提到的两个问题。

%第四段：为什么现有sketch方案无法感知控制误差（距离这个目标很远）。理论上bound不准也不好，实践上设计不行。
When taking sketches to practice, we encountered many problems caused by the error of flow size estimation.
The first is the problem of \textit{misclassification}. When using a sketch (\eg, the well-known Count-Min \cite{cmsketch}) to classify elephant and mice flows according to the estimated flow size, many mice flows are overestimated by tens of or hundreds of times, and consequently classified as elephant flows.
%which lead to their misclassification as elephant flows. 
These misclassifications may cause congestion control policies \cite{lin1997dynamics} to mistake control signals (mice flows) for elephant flows, and consequently drops the packets of critical control signals. 
%
These misclassifications can also cause other problems \cite{asketch}. The current available solution is to expand the sketch size many times to alleviate this problem, which is often unacceptable due to the very limited size of on-chip memory.
%In response, we expanded the sketch size many times to alleviate this problem.
%
The second is the problem of \textit{accuracy certainty}. Although under limited memory size, the user requires that the estimated size must be credible enough: the absolute error of each flow cannot exceed a pre-defined threshold $\Lambda$.
In this case, the user can trust the estimated sizes, and use them for anomaly detection \cite{chen2020beaucoup,subsketchIMC} and more \cite{yu2019dshark,guo2015pingmesh,geng2019simon}. 
More details are provided in \cref{subsec:related:problem}. 
%\wyh{\textbf{It seems to be a dilemma that the error cannot be eliminated under limited resources.}
%}

%As many sketches compete for smaller average error, 
We realize the cause behind above problems is that sketches cannot \textit{sense and control per-flow error}, which is ignored by the existing studies. Sensing the error is to \textit{find the Maximum Possible Error (MPE) of each estimated flow size}. 
For example, when the absolute error of an estimation is 20, it is desired for a sketch to report a MPE closing to 20. 
With sensing per-flow error, the first problem can be tackled by excluding false elephant flows whose estimated sizes are close to their MPE.
Controlling per-flow error is to \textit{control the MPE of all flows to be lower than the user-defined threshold $\Lambda$.} After that, the actual error must also be less than $\Lambda$ and the second problem is solved.
It is expected that sensing and controlling per-flow error should be performed at line rate, because some network operations (\eg, congestion control, flow scheduling) need the estimation of flow size at exactly the current time.


%  \wyh{\sout{such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian},}}
While sketches have made significant progresses in many aspects, they do not handle the problem of \textit{Sensing and controlling per-flow error}.
(1) In theory, without prior knowledge of the flow distribution, existing error bounds are too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. 
In addition, existing error bounds are bounds of error distribution rather than per-flow error bound, \ie, a personalized feedback of the error for each flow. 
% In addition, existing error bound is a bound of error distribution rather than per-flow error: a personalized feedback of the error for each estimation. 
For example, when a flow with size of 3000 is estimated to be 3010, what we hope to know is ``the error of 3010 must be less than 20'' rather than ``the error of 3010 is less than 200 with $90\%$ probability''.
%On the other hand in practice, groundtruth\footnote{All existing sketches claim they have a small error on given datasets by comparing the estimation value to groundtruth.} cannot be obtained due to the high speed of network traffic. Existing sketches cannot sense the error, and have to report that their error could vary widely: from 0 to a very large value.
%
In evaluation, existing sketches claim they have a small error on the given datasets by comparing the estimation value to groundtruth.
However, (2) in practice, groundtruth cannot be entirely obtained due to the high speed of network traffic. Therefore, existing sketches cannot claim a small error without groundtruth any more, and have to report that their error could vary widely: from 0 to a very large value.
%On the other hand in practice, existing sketches cannot sense the error when without groundtruth: their error could vary widely: from 0 to a very large value.
The reason behind is that their designs \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} let all hash collision happen naturally, and do not observe whether each collision is intensive.



% \wyh{old}.The most well known Count-Min sketch (\cite{cmsketch}) derives the bound for the absolute error, and then a great many sketches compete for smaller absolute error which is calculated by comparing the estimated sizes with the ground-truth (the true flow sizes).
% However, the ground-truth is unknown due to the high speed of network traffic in practice, and the error cannot be calculated by comparison.
% In practice, the error may vary a lot but users know nothing about the error of each flow. 
% For example, when a Count-Min sketch \cite{cmsketch} reports that an estimated flow size is $10000$, the estimation error could be 0, 10, or even 10000.
% %
% It is highly desired to answer such a question: for each incoming packet of flow $f$, \textit{can we sense its error and elegantly control it at line rate}? In other words, for each incoming flow, can we give an estimation value additionally with an acceptable maximum error?
% For the same example, one satisfactory report is that the estimation is 10000 and the maximum error is 20, which means that the true flow size is definitely in the range $[10000,10020]$. 
% We believe that making progresses in this direction can significantly accelerate the application of sketching algorithm into practices.
% \textit{Sensing and controlling per-flow error} have many benefits which are details in Section \ref{....}. 



% \wyh{old.}Based on the classic sketches including Count-Min, recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, but they still do not handle the problem of \textit{Sensing and controlling per-flow error}.
% On the one hand in theory, without prior knowledge of the flow distribution, the error bound is too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. In addition, existing error bound is a bound of error distribution rather than per-flow error: a personalized feedback of the error for each estimation. 
% For example, when a flow with size of 3000 is estimated to be 3010, what we hope to know is ``the error of 3010 must be less than 20'' rather than ``the error of 3010 is less than 200 with $90\%$ probability''.
% On the other hand in practice, existing sketches cannot sense the error when without groundtruth: their error could vary widely: from 0 to a very large value.  
% The reason behind is that they \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} let all hash collision happen naturally, and do not observe whether each collision is intensive.






\subsection{Our Proposed Approach}

This paper proposes the \aname{}, the first sketch to sense and control per-flow error at line rate. 
%We propose two techniques to address our goal of sensing and controlling the error.\aname{}
\aname{} has two key techniques: \textit{Error-Sensing} and \textit{Double Exponential Composition}.
\textit{Error-Sensing} helps us sense the error and distinguish which flows are at risk of losing control.
% This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
For those flows at risk, \textit{Double Exponential Composition} controls their error at great efficiency.
%
%\wyh{at great efficiency.}\sout{and achieves the best theoretical results.}
%
In theory, \aname{} achieves the smallest space complexity among all sketches working at line rate.
%\sout{The theoretical proofs of \aname{} is strictly tighter than existing proofs. }
% proof不能比较是否更紧（tighter），只有bound可以。
We implement \aname{} on three platforms, and conduct experiments on testbed and event-level simulation to verify the function and theoretical results of \aname{}. 
%Implementations on three platforms and evaluation on a test-bed and simulations verify the function and theoretical results of \aname{}. 





\ppp{Key Technique I: Error-Sensing.} 
We argue that existing sketches cannot sense the error because their basic unit does not observe the collision, where collisions are closely related to error.
Take the well-known Count-Min \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
Differently, we aim at an Error-Sensible bucket instead of a counter to observe whether the collision is intensive.
Inspired by existing election algorithms, we find that the negative vote in an election is an ideal approach to observe the collision and sense the error.
In order to study the error sensing in elections, we devise a comprehensive framework that covers many election designs from Elastic, Majority, SpaceSaving and more \cite{tang2019mvsketch,frequent}.
The framework answers how to sense the error in one bucket.
Thereafter we can find out high-risk buckets where can handle those buckets in which the error is about to out of control. How to elegantly control the error is addressed by our second key technique.

% \ppp{Key Technique I: Error-Sensing.} 
% We argue that existing sketches cannot sense the error because their basic unit does not observe the collision, where collisions are closely related to error.
% Take the well-known Count-Min \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
% Differently, we devise an Error-Sensible bucket instead of a counter to observe whether the collision is intensive.
% The bucket has three fields: a ID for a candidate flow, a counter for ``YES'', and a counter for ``NO''.
% For each incoming packet, if its ID is same as the candidate, we increment ``YES''. Otherwise, we increment ``NO''. 
% When there are too many ``NO'', the recorded candidate flow will be replaced.
% Interestingly, \textit{we find and prove that the error is at most ``NO''}, and thereafter \wyh{we can find out high-risk buckets where} \sout{can handle those buckets in which }the error is about to out of control. How to elegantly control the error is addressed by our second key technique.




%by properly organizing these buckets.
%Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.

%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double Exponential Composition
\ppp{Key Technique II: Double Exponential Composition.} 
This technique aims to control the error of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the number of out-of-control flows sharply to zero by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
If one flow is about to out of control, we send it to the next array, and in total we have $d$ arrays.
The key is how to reduce the probability $\mathcal{P}$ of failure (\ie, a flow is sent out from the last array) sharply to nearly-zero.
%the flows entering the next array as sharply as possible.
Using a straightforward solution, the probability $\mathcal{P}$ can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}, overwhelming the number of flows easily.
Owing to the setting of double Exponential parameters, we strictly derive that \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space to control the error below $\Lambda$ with high probability $1-\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space.

%and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 


\begin{table} [h]
\begin{center}
\vspace{-0.3cm}
\caption{Paper Outline.}
\vspace{-0.3cm}
\label{table:outline}
\begin{tabular}{m{0.35\columnwidth}|m{0.55\columnwidth}}
% \hline
\bottomrule[1pt]
\textbf{Section}&\textbf{Contents}\\
\hline
% $\mathcal{S}$&a data stream\\
% \hline
\cref{sec:relate} New Problem  & Sense and Control the Error\\
\cref{SEC:Algorithm} New Algorithm  & \anamelong{}\\
\cref{sec:math} New Theory  & $O\left(\frac{N}{\Lambda}\times\ln(\frac{1}{\delta})\right) \rightarrow O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$\\
\cref{sec:extensions} Extensions  & Priority and Network-wide\\
\cref{sec:Implementations} Platforms  & CPU, FPGA, and P4 Switch\\
\cref{sec:experiments} Evaluation  & Benchmarks, NS2, Testbed\\
\toprule[1pt]
\end{tabular}
\vspace{-0.05in}
\end{center}
\end{table}
% \begin{figure}[htbp]
%     \prefig
%     \centering  
%     \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
%     \vspace{-0.15in}
%     \caption{Contribution Outline.}
%     \label{fig:intro}
%     \postfig
% \end{figure}
% % evaluation
%TBD ： new problem不准确
%
As shown in Table \ref{table:outline}, %Figure \ref{fig:intro},
our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We define SenseCtrlErr and devise \textbf{ReliableSketch} that can sense and control the accuracy for every flow.
    \item We theoretically prove that \anamelong{} outperforms state-of-the-art in both space and time complexity.
    \item We implement \anamelong{} in multiple platforms including CPU, FPGA, and Programmable Switch. Under the same small memory, ReliableSketch not only controls all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows.
    % Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double Exponential Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v5.tex <==

\begin{comment}

% 确定区间heavy hitter 理想情况 猜想无错不可能用单侧完成。   区间宽度为0就是ideal，但是不可能。现有算法也做不了区间。区间确定性heavy hitter?
problem: finding heavy hitter in network measurement 
heavy hitter define .
heavy application

现有工作分类

ideal goal

1、heavy hitter重要性
2、衡量指标 precision recall ideal goal两个都是100%    证明不可达
3、现有工作 尝试逼近，但是离目标很远。单方面有bound，两面没有。都在朝向ideal goal前进。现有 adhoc heavy hitter（逼近），我们双向保证？


optimal heavy hitter 没有误报漏报
我们做到大部分范围没有漏报误报。
两头无错

near optimal heavy hitter
memory越大区间越小越接近






准确地heavy hitter识别

由于测量资源的限制，完全准确的
ideal的测量

\end{comment}





\presec
\section{Introduction} \postsec
\label{sec:intro}

% \subsection{Background and Motivation}\postsub




% P1：
% heavy hitter重要性：在哪些方面有应用
% heavy hitter定义，给定一个阈值，高于xx的是heavy hitter，低于的不是。
% (\eg, total bytes received by a IP)
% Accurate network measurement is often the first and fundamental step in many network functions.
Among all measurement tasks, finding heavy hitter flows, that have flow sizes greater than a threshold $T$, is a classic and important topic.
It can benefit many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}.
Besides, network operator can leverage heavy hitters to detect anomalies including worms, port scans, DDoS attacks and SYN floods \cite{chen2020beaucoup,subsketchIMC}.
Since the subsequent network functions (\eg, congestion control, flow scheduling) need the results at exactly the current time, the solutions are desired to be performed at line rate on the switch data plane,
%(\eg, a destination IP receiving more than a certain portion of the traffic in a short time interval)
% 假阳性和阴性的定义，对应的后果


\wyh{Recently, sketch-based solutions become one of the most promising approach for finding heavy hitters, because they can achieve high accuracy using small memory and work at line rate on the data plane.}
% To find heavy hitters, one of the most promising approach is using sketches and other similar approximation algorithms, because they can achieve highest accuracy using small memory and work at line rate on the data plane.
Typical solutions include Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, Elastic \cite{yang2018elastic}, and more \cite{basat2020Precision, liu2016UnivMon, hashpipe, chen2020beaucoup, namkung2022sketchlib}. We call them sketches for short. 
Existing sketches identify the heavy hitter according to whether its estimated flow size is greater than the threshold $T$.
In this process, the misidentifications of heavy hitters are inevitable\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.} and sketches tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.
Meanwhile, the other misidentifications are serious ones and called outliers, including false positives (\ie, mistaking a non-heavy flow with sizes $< T-\Lambda$ for a heavy one) and false negatives (\ie, mistaking a heavy flow with sizes $> T+\Lambda$ for a non-heavy one). We show them in Figure \ref{fig:intro:hh}. 
These outliers will cause numerous problems. For example, in anomaly detection, the false positives are false alarms of attacks \cite{hashpipe} and the false negatives result in that the operator cannot find out all anomalies. Besides, the outliers will degrade the performance of its follow-up network functions including load balancing and traffic engineering, and could further lead to network congestion and service level agreement (SLA) violation.
Although sketches have high confidence that each misidentification is mild with high probability, they cannot completely eliminate the outliers when the total number of flows is large. 
When a network failure occurs, the non fully confident results having outliers will always be suspected in the diagnosis process.
In response, our design goal is to reliably eliminate the outlier at line rate, so as to avoid problems caused by outliers and the suspicion about the results.


% and the solution has always been eager for reliable results to prove itself innocence.



% Since the zero-error solution with no misidentification of heavy hitters will cost too much memory\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.}, sketches tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.
% Existing sketches identify the heavy hitter if the estimated  size of  with the threshold $T$.
% If the estimated value is greater than the threshold value, it is considered as a large flow. Otherwise, it is not.

% but the flow size may be seriously overestimated or underestimated, resulting in outliers.

% Since a zero-erroreliminating all misidentifications of heavy hitters will cost too much memory\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.}, the consensus of the existing solutions represented by sketches (\eg, Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, Elastic \cite{yang2018elastic}, and more \cite{basat2020Precision, liu2016UnivMon, hashpipe, chen2020beaucoup, namkung2022sketchlib}) is to tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.

% P2
% 理想情况是消除假阳性和阴性，但理想状况不可能实现。依赖无错的频数估计。
% The ideal goal is to eliminate all misidentifications with certain design guarantees or mathematical proofs, but it cannot be achieved over large amount of flows due to its high memory cost.
% Meanwhile, the other misidentifications, including false positives with real flow sizes $< T-\Lambda$ and false negatives with real flow sizes $> T+\Lambda$, are serious ones and called outliers. We show them in Figure \ref{fig:intro:hh}.
% not acceptable, 
% and we call them false positive outlier and false negative outlier, respectively.
% % However, the other misidentifications are serious and they have not been completely eliminated in practice. 





% In response, our design goal is to reliably eliminate the outlier on the switch data plane, so as to avoid the suspicion about the results.



\begin{figure}[tbp]
    \prefig
    \centering  
    \includegraphics[width=0.98\linewidth]{vldb/GraphPPT/introFig.pdf}
    \vspace{-0.15in}
    \caption{The error type of heavy hitter detection.}
    \label{fig:intro:hh}
    \postfig
\end{figure}


%对于这类错误分类，其中大部分错误是可接受的，但总有无法被接受的。
% For the other kind of outliers, Elastic and other sketches provide a bound showing that most misidentified flows are tolerable misidentifications, but since the total number of flows is large there are always many misidentifications are not tolerable.
% P4
% 现有工作无法实现，本质原因是它们的频数bound是概率bound，缺少直接的保证。


% P3
% 我们退一步，设定一个允许的误差区间，为双阈值 HH。
% 我们的目标是消除xx的假阳性和阴性，将影响降低到最小。

% P5
% 我们提出的方案。


% When taking sketches to practice, we encountered many problems caused by the error of flow size estimation.
% The first is the problem of \textit{misclassification}. When using a sketch (\eg, the well-known Count-Min \cite{cmsketch}) to classify elephant and mice flows according to the estimated flow size, many mice flows are overestimated by tens of or hundreds of times, and consequently classified as elephant flows.
% These misclassifications may cause congestion control policies \cite{lin1997dynamics} to mistake control signals (mice flows) for elephant flows, and consequently drops the packets of critical control signals. 
% These misclassifications can also cause other problems \cite{asketch}. The current available solution is to expand the sketch size many times to alleviate this problem, which is often unacceptable due to the very limited size of on-chip memory.
% The second is the problem of \textit{accuracy certainty}. Although under limited memory size, the user requires that the estimated size must be credible enough: the absolute error of each flow cannot exceed a pre-defined threshold $\Lambda$.
% In this case, the user can trust the estimated sizes, and use them for anomaly detection \cite{chen2020beaucoup,subsketchIMC} and more \cite{yu2019dshark,guo2015pingmesh,geng2019simon}. 
% More details are provided in \cref{subsec:related:problem}. 

% We realize the cause behind above problems is that sketches cannot \textit{sense and control per-flow error}, which is ignored by the existing studies. Sensing the error is to \textit{find the Maximum Possible Error (MPE) of each estimated flow size}. 
% For example, when the absolute error of an estimation is 20, it is desired for a sketch to report a MPE closing to 20. 
% With sensing per-flow error, the first problem can be tackled by excluding false elephant flows whose estimated sizes are close to their MPE.
% Controlling per-flow error is to \textit{control the MPE of all flows to be lower than the user-defined threshold $\Lambda$.} After that, the actual error must also be less than $\Lambda$ and the second problem is solved.
% It is expected that sensing and controlling per-flow error should be performed at line rate, because some network operations (\eg, congestion control, flow scheduling) need the estimation of flow size at exactly the current time.


% While sketches have made significant progresses in many aspects, they do not handle the problem of \textit{Sensing and controlling per-flow error}.
% (1) In theory, without prior knowledge of the flow distribution, existing error bounds are too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. 
% In addition, existing error bounds are bounds of error distribution rather than per-flow error bound, \ie, a personalized feedback of the error for each flow. 
% For example, when a flow with size of 3000 is estimated to be 3010, what we hope to know is ``the error of 3010 must be less than 20'' rather than ``the error of 3010 is less than 200 with $90\%$ probability''.
% In evaluation, existing sketches claim they have a small error on the given datasets by comparing the estimation value to groundtruth.
% However, (2) in practice, groundtruth cannot be entirely obtained due to the high speed of network traffic. Therefore, existing sketches cannot claim a small error without groundtruth any more, and have to report that their error could vary widely: from 0 to a very large value.
% The reason behind is that their designs \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} let all hash collision happen naturally, and do not observe whether each collision is intensive.

% \subsection{Our Proposed Approach}

% Some solutions have a one-side certain bound of flow sizes that definitely avoids one of overestimation or underestimation for the flow size, and thus eliminate one of the false negative or the false positive, but they cannot eliminate both simultaneously.


In this paper, we propose \aname{} having bilateral tight error bounds for every flow, so as to eliminate all outliers:
When estimating the size of each flow ($f$), \aname{} can provide both an upper estimate/bound ($\widehat{f}\geqslant f$) that must be greater than or equal to the flow size and a lower estimate/bound ($\widetilde{f}\leqslant f$). 
The difference between the two estimates is the Maximum Possible Error (MPE) of each estimate, \ie, $MPE=\widehat{f}-\widetilde{f}$, $MPE\geqslant |\widehat{f}-f|$ and $MPE\geqslant |\widetilde{f}-f|$.
Further, for every flow, \aname{} controls that the MPE is less than or equal to $\Lambda$.
Finally, when comparing any estimate with $T$ to identify heavy hitters, only mild misclassification may occur instead of outlier\footnote{When comparing $\widehat{f}$ with $T$ to identify heavy hitters, there is no false negative because their $\widehat{f}$ must be no less than $T$, and there is no false positive because the $\widehat{f}$ of the flow with size $< T - \Lambda$ must be less than $T$.}.

\aname{} has two key techniques: \textit{Error-Sensing} and \textit{Double-Exponential-Control}.
Error-Sensing can build the two bound by calculating MPE, where MPE comes from observing the amount of hash collisions.
% calculate MPE by observing the amount of hash collisions
% builds the two bound by observing the amount of hash collisions and calculating MPE.
Then, Double-Exponential-Control looks for the flows with potential large MPE to control them, and therefore the two bounds are close enough.

% the error of every flow to be lower than the user-defined threshold $\Lambda$
% not only provide bilateral certain error bounds for every flow, but also control the distance between two bounds for all flows under threshold $\Lambda$.
% \aname{} has two key techniques: \textit{Bound-Setup} and \textit{Double-Exponential-Control}.
% \textit{Bound-Setup} builds the two bound by observing the amount of hash collisions. Then, the Double-Exponential-Control looks for the flows with large distance between bounds and control their distance.
% helps us sense the error and distinguish which flows are at risk of losing control.
% This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
% For those flows at risk, \textit{Double-Exponential-Control} controls their error at great efficiency.
%
%\wyh{at great efficiency.}\sout{and achieves the best theoretical results.}
%
%Implementations on three platforms and evaluation on a test-bed and simulations verify the function and theoretical results of \aname{}. 




% Towards the design goal, we propose \aname{} that can not only provide bilateral certain error bounds for every flow, but also control the distance between two bounds for all flows under threshold $\Lambda$.
% \aname{} has two key techniques: \textit{Bound-Setup} and \textit{Double-Exponential-Control}.
% \textit{Bound-Setup} builds the two bound by observing the amount of hash collisions. Then, the Double-Exponential-Control looks for the flows with large distance between bounds and control their distance.
% helps us sense the error and distinguish which flows are at risk of losing control.
% This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
% For those flows at risk, \textit{Double-Exponential-Control} controls their error at great efficiency.
%
%\wyh{at great efficiency.}\sout{and achieves the best theoretical results.}
%
%\sout{The theoretical proofs of \aname{} is strictly tighter than existing proofs. }
% proof不能比较是否更紧（tighter），只有bound可以。
% In theory, \aname{} achieves the smallest space complexity among all sketches working at line rate.
% We implement \aname{} on three platforms, and conduct experiments on testbed and event-level simulation to verify the function and theoretical results of \aname{}. 
%Implementations on three platforms and evaluation on a test-bed and simulations verify the function and theoretical results of \aname{}. 



\ppp{Key Technique I: Error-Sensing.} 
We can build the two bounds if we can acquire the upper bound and the MPE, \ie, $\widetilde{f}=\widehat{f}-MPE$.
To find MPE, our idea is to observe the hash collision of the upper bound, where the amount of collision can reflect the error.
Take the well-known Count-Min (CM) \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
The total number is an upper bound/estimate no less than the actual flow size.
If a flow and many other flows are mapped to a same counter, its error will be large. Otherwise, its error is small.
Inspired by existing election algorithms \cite{tang2019mvsketch,frequent}, we find that the negative vote in an election is an ideal approach to observe the collision and calculate the MPE.
We replace the counter by an Error-Sensible bucket, so as to observe whether the collision is intensive. 
We will detail the Error-Sensible bucket in Section \ref{subsec:alg:onebucket}.
After observing the collision and getting the MPE, we use our second key technique to control the MPE.

% We  many election designs from Elastic, Majority, SpaceSaving and more \cite{tang2019mvsketch,frequent}.
% Thereafter we can find out high-risk buckets where can handle those buckets in which the error is about to out of control. 
% How to elegantly control the error is addressed by our second key technique.

% \ppp{Key Technique I: Bound-Setup.} 
% We argue that existing sketches cannot sense the error because their basic unit does not observe the collision, where collisions are closely related to error.
% Take the well-known Count-Min \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
% Differently, we devise an Error-Sensible bucket instead of a counter to observe whether the collision is intensive.
% The bucket has three fields: a ID for a candidate flow, a counter for ``YES'', and a counter for ``NO''.
% For each incoming packet, if its ID is same as the candidate, we increment ``YES''. Otherwise, we increment ``NO''. 
% When there are too many ``NO'', the recorded candidate flow will be replaced.
% Interestingly, \textit{we find and prove that the error is at most ``NO''}, and thereafter \wyh{we can find out high-risk buckets where} \sout{can handle those buckets in which }the error is about to out of control. How to elegantly control the error is addressed by our second key technique.




%by properly organizing these buckets.
%Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.

%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double-Exponential-Control
\ppp{Key Technique II: Double-Exponential-Control.} 
This technique aims to control the MPE of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the number of out-of-control flows sharply to zero by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
If one flow is about to out of control, we send it to the next array, and in total we have $d$ arrays.
The key is how to reduce the probability $\mathcal{P}$ of failure (\ie, a flow is sent out from the last array) sharply to nearly-zero.
%the flows entering the next array as sharply as possible.
Using a straightforward solution, the probability $\mathcal{P}$ can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}, overwhelming the number of flows easily.
Owing to the setting of double Exponential parameters, we strictly derive that, for $N$ packets, \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space to control the error of all flows below $\Lambda$ with failure probability $\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space.


%and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 

Our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We devise \textbf{ReliableSketch} to eliminate the outlier by bilateral tight bounds and control the error of all flows under threshold $\Lambda$.
    \item We theoretically prove that \anamelong{} outperforms state-of-the-art in both space and time complexity.
    \item We implement \anamelong{} on multiple platforms including CPU, FPGA, and Programmable Switch. Under the same small memory, ReliableSketch not only controls all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows.
    % Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}

% \begin{table} [h]
% \begin{center}
% \vspace{-0.3cm}
% \caption{Paper Outline.}
% \vspace{-0.3cm}
% \label{table:outline}
% \begin{tabular}{m{0.35\columnwidth}|m{0.55\columnwidth}}
% % \hline
% \bottomrule[1pt]
% \textbf{Section}&\textbf{Contents}\\
% \hline
% % $\mathcal{S}$&a data stream\\
% % \hline
% \cref{sec:relate} New Problem  & Sense and Control the Error\\
% \cref{SEC:Algorithm} New Algorithm  & \anamelong{}\\
% \cref{sec:math} New Theory  & $O\left(\frac{N}{\Lambda}\times\ln(\frac{1}{\delta})\right) \rightarrow O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$\\
% \cref{sec:extensions} Extensions  & Priority and Network-wide\\
% \cref{sec:Implementations} Platforms  & CPU, FPGA, and P4 Switch\\
% \cref{sec:experiments} Evaluation  & Benchmarks, NS2, Testbed\\
% \toprule[1pt]
% \end{tabular}
% \vspace{-0.05in}
% \end{center}
% \end{table}
% \begin{figure}[htbp]
%     \prefig
%     \centering  
%     \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
%     \vspace{-0.15in}
%     \caption{Contribution Outline.}
%     \label{fig:intro}
%     \postfig
% \end{figure}
% % evaluation
%TBD ： new problem不准确
%
% As shown in Table \ref{table:outline}, 


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double-Exponential-Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_v6.tex <==

\begin{comment}

% 确定区间heavy hitter 理想情况 猜想无错不可能用单侧完成。   区间宽度为0就是ideal，但是不可能。现有算法也做不了区间。区间确定性heavy hitter?
problem: finding heavy hitter in network measurement 
heavy hitter define .
heavy application

现有工作分类

ideal goal

1、heavy hitter重要性
2、衡量指标 precision recall ideal goal两个都是100%    证明不可达
3、现有工作 尝试逼近，但是离目标很远。单方面有bound，两面没有。都在朝向ideal goal前进。现有 adhoc heavy hitter（逼近），我们双向保证？


optimal heavy hitter 没有误报漏报
我们做到大部分范围没有漏报误报。
两头无错

near optimal heavy hitter
memory越大区间越小越接近






准确地heavy hitter识别

由于测量资源的限制，完全准确的
ideal的测量

\end{comment}





\presec
\section{Introduction} \postsec
\label{sec:intro}

% \subsection{Background and Motivation}\postsub




% P1：
% heavy hitter重要性：在哪些方面有应用
% heavy hitter定义，给定一个阈值，高于xx的是heavy hitter，低于的不是。
% (\eg, total bytes received by a IP)
% Accurate network measurement is often the first and fundamental step in many network functions.
Among all measurement tasks, finding heavy hitter flows that have flow sizes\footnote{\wyh{flow size}} greater than a threshold $T$, is a classic and important \wyh{task}.
It can benefit many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}.
Besides, network operator can leverage heavy hitters to detect anomalies including worms, port scans, DDoS attacks and SYN floods \cite{chen2020beaucoup,subsketchIMC}.
Since the subsequent network functions (\eg, congestion control, flow scheduling) need the results at exactly the current time, the solutions are desired to be performed at line rate on the switch data plane.
%(\eg, a destination IP receiving more than a certain portion of the traffic in a short time interval)
% 假阳性和阴性的定义，对应的后果



\begin{figure}[tbp]
    \prefig
    \centering  
    \includegraphics[width=0.98\linewidth]{vldb/GraphPPT/introfig3.pdf}
    \vspace{-0.15in}
    \caption{The error types of finding heavy hitters.}
    \label{fig:intro:hh}
    \postfig
\end{figure}


\wyh{Recently, sketch-based solutions become one of the most promising approach for finding heavy hitters, because they can achieve high accuracy under tight memory limitation and work at line rate on the data plane.}
% To find heavy hitters, one of the most promising approach is using sketches and other similar approximation algorithms, because they can achieve highest accuracy using small memory and work at line rate on the data plane.
Typical solutions (called sketches for short) include Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, Elastic \cite{yang2018elastic}, and more \cite{basat2020Precision, liu2016UnivMon, hashpipe, chen2020beaucoup, namkung2022sketchlib}. 
% These sketches identify the heavy hitter according to whether its estimated flow size is greater than the threshold $T$.
\wyh{When finding heavy hitters, the sketch first estimates the size of each flow and report the flows with estimated size greater than the threshold $T$ as heavy hitters.
%
Since the estimated sizes are not (and cannot be?) error-free, the reported heavy hitters based them include misclassifications.}
%
\wyh{Among all misclassifications, those with actual sizes close enough to $T$ (in range $[T-\Lambda, T+\Lambda]$) are tolerable, where $\Lambda$ is a user-defined tolerance parameter?/limit.}
Meanwhile, the other misclassifications are serious ones and called outliers.
We show them in Figure \ref{fig:intro:hh}.
\wyh{On the surface, every time when estimating the size of a flow, existing sketches ensure that the error is tolerable with a somewhat large probability. Formally, sketches can estimate a size with an absolute error less than $\Lambda$ with a probability at least $1-\delta$, where $\delta$ is a hyper parameter of the sketch. 
But in fact, due to the large number of total flows (denoted as $M$), it is too expensive and almost impossible to make $\delta$ far less than $M$ to eliminate the outlier.}

\wyh{OLD:} To find heavy hitters, one of the most promising approach is using sketches and other similar approximation algorithms, because they can achieve highest accuracy using small memory and work at line rate on the data plane.
Typical solutions include Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, Elastic \cite{yang2018elastic}, and more \cite{basat2020Precision, liu2016UnivMon, hashpipe, chen2020beaucoup, namkung2022sketchlib}. We call them sketches for short. 
Existing sketches identify the heavy hitter according to whether its estimated flow size is greater than the threshold $T$.
In this process, the misidentifications of heavy hitters are inevitable\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.} and sketches tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.
Meanwhile, the other misidentifications are serious ones and called outliers, including false positives (\ie, mistaking a non-heavy flow with sizes $< T-\Lambda$ for a heavy one) and false negatives (\ie, mistaking a heavy flow with sizes $> T+\Lambda$ for a non-heavy one). We show them in Figure \ref{fig:intro:hh}. 
These outliers will cause numerous problems. For example, in anomaly detection, the false positives are false alarms of attacks \cite{hashpipe} and the false negatives result in that the operator cannot find out all anomalies. Besides, the outliers will degrade the performance of its follow-up network functions including load balancing and traffic engineering, and could further lead to network congestion and service level agreement (SLA) violation.
Although sketches have high confidence that each misidentification is mild with high probability, they cannot completely eliminate the outliers when the total number of flows is large. 
When a network failure occurs, the non fully confident results having outliers will always be suspected in the diagnosis process.
In response, our design goal is to reliably eliminate the outlier at line rate, so as to avoid problems caused by outliers and the suspicion about the results.



These outliers will cause numerous problems. For example, in anomaly detection, the false positives are false alarms of attacks \cite{hashpipe} and the false negatives result in that the operator cannot find out all anomalies. Besides, the outliers will degrade the performance of its follow-up network functions including load balancing and traffic engineering, and could further lead to network congestion and service level agreement (SLA) violation.
When a network failure occurs, the non fully confident results including outliers will always be suspected in the diagnosis process.
In response, our design goal is to reliably eliminate the outlier at line rate, so as to avoid problems caused by outliers and the suspicion about the results.


% and the solution has always been eager for reliable results to prove itself innocence.



% Since the zero-error solution with no misidentification of heavy hitters will cost too much memory\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.}, sketches tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.
% Existing sketches identify the heavy hitter if the estimated  size of  with the threshold $T$.
% If the estimated value is greater than the threshold value, it is considered as a large flow. Otherwise, it is not.

% but the flow size may be seriously overestimated or underestimated, resulting in outliers.

% Since a zero-erroreliminating all misidentifications of heavy hitters will cost too much memory\footnote{Eliminating all misidentifications requires to estimate the flow sizes of all flows exactly, whose memory cost is proportional to the number of all flows and is too large for a switch.}, the consensus of the existing solutions represented by sketches (\eg, Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, Elastic \cite{yang2018elastic}, and more \cite{basat2020Precision, liu2016UnivMon, hashpipe, chen2020beaucoup, namkung2022sketchlib}) is to tolerate the mild misidentifications whose true flow sizes are close to the threshold $T$, \ie, the difference is less than $\Lambda$.

% P2
% 理想情况是消除假阳性和阴性，但理想状况不可能实现。依赖无错的频数估计。
% The ideal goal is to eliminate all misidentifications with certain design guarantees or mathematical proofs, but it cannot be achieved over large amount of flows due to its high memory cost.
% Meanwhile, the other misidentifications, including false positives with real flow sizes $< T-\Lambda$ and false negatives with real flow sizes $> T+\Lambda$, are serious ones and called outliers. We show them in Figure \ref{fig:intro:hh}.
% not acceptable, 
% and we call them false positive outlier and false negative outlier, respectively.
% % However, the other misidentifications are serious and they have not been completely eliminated in practice. 





% In response, our design goal is to reliably eliminate the outlier on the switch data plane, so as to avoid the suspicion about the results.



%对于这类错误分类，其中大部分错误是可接受的，但总有无法被接受的。
% For the other kind of outliers, Elastic and other sketches provide a bound showing that most misidentified flows are tolerable misidentifications, but since the total number of flows is large there are always many misidentifications are not tolerable.
% P4
% 现有工作无法实现，本质原因是它们的频数bound是概率bound，缺少直接的保证。


% P3
% 我们退一步，设定一个允许的误差区间，为双阈值 HH。
% 我们的目标是消除xx的假阳性和阴性，将影响降低到最小。

% P5
% 我们提出的方案。


% When taking sketches to practice, we encountered many problems caused by the error of flow size estimation.
% The first is the problem of \textit{misclassification}. When using a sketch (\eg, the well-known Count-Min \cite{cmsketch}) to classify elephant and mice flows according to the estimated flow size, many mice flows are overestimated by tens of or hundreds of times, and consequently classified as elephant flows.
% These misclassifications may cause congestion control policies \cite{lin1997dynamics} to mistake control signals (mice flows) for elephant flows, and consequently drops the packets of critical control signals. 
% These misclassifications can also cause other problems \cite{asketch}. The current available solution is to expand the sketch size many times to alleviate this problem, which is often unacceptable due to the very limited size of on-chip memory.
% The second is the problem of \textit{accuracy certainty}. Although under limited memory size, the user requires that the estimated size must be credible enough: the absolute error of each flow cannot exceed a pre-defined threshold $\Lambda$.
% In this case, the user can trust the estimated sizes, and use them for anomaly detection \cite{chen2020beaucoup,subsketchIMC} and more \cite{yu2019dshark,guo2015pingmesh,geng2019simon}. 
% More details are provided in \cref{subsec:related:problem}. 

% We realize the cause behind above problems is that sketches cannot \textit{sense and control per-flow error}, which is ignored by the existing studies. Sensing the error is to \textit{find the Maximum Possible Error (MPE) of each estimated flow size}. 
% For example, when the absolute error of an estimation is 20, it is desired for a sketch to report a MPE closing to 20. 
% With sensing per-flow error, the first problem can be tackled by excluding false elephant flows whose estimated sizes are close to their MPE.
% Controlling per-flow error is to \textit{control the MPE of all flows to be lower than the user-defined threshold $\Lambda$.} After that, the actual error must also be less than $\Lambda$ and the second problem is solved.
% It is expected that sensing and controlling per-flow error should be performed at line rate, because some network operations (\eg, congestion control, flow scheduling) need the estimation of flow size at exactly the current time.


% While sketches have made significant progresses in many aspects, they do not handle the problem of \textit{Sensing and controlling per-flow error}.
% (1) In theory, without prior knowledge of the flow distribution, existing error bounds are too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. 
% In addition, existing error bounds are bounds of error distribution rather than per-flow error bound, \ie, a personalized feedback of the error for each flow. 
% For example, when a flow with size of 3000 is estimated to be 3010, what we hope to know is ``the error of 3010 must be less than 20'' rather than ``the error of 3010 is less than 200 with $90\%$ probability''.
% In evaluation, existing sketches claim they have a small error on the given datasets by comparing the estimation value to groundtruth.
% However, (2) in practice, groundtruth cannot be entirely obtained due to the high speed of network traffic. Therefore, existing sketches cannot claim a small error without groundtruth any more, and have to report that their error could vary widely: from 0 to a very large value.
% The reason behind is that their designs \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} let all hash collision happen naturally, and do not observe whether each collision is intensive.

% \subsection{Our Proposed Approach}

% Some solutions have a one-side certain bound of flow sizes that definitely avoids one of overestimation or underestimation for the flow size, and thus eliminate one of the false negative or the false positive, but they cannot eliminate both simultaneously.


In this paper, we propose \aname{} having bilateral tight error bounds for every flow, so as to eliminate all outliers:
When estimating the size of each flow ($f$), \aname{} can provide both an upper estimate/bound ($\widehat{f}\geqslant f$) that must be greater than or equal to the flow size and a lower estimate/bound ($\widetilde{f}\leqslant f$). 
The difference between the two estimates is the Maximum Possible Error (MPE) of each estimate, \ie, $MPE=\widehat{f}-\widetilde{f}$, $MPE\geqslant |\widehat{f}-f|$ and $MPE\geqslant |\widetilde{f}-f|$.
Further, for every flow, \aname{} controls that the MPE is less than or equal to $\Lambda$.
Finally, when comparing any estimate with $T$ to identify heavy hitters, only mild misclassification may occur instead of outlier\footnote{When comparing $\widehat{f}$ with $T$ to identify heavy hitters, there is no false negative because their $\widehat{f}$ must be no less than $T$, and there is no false positive because the $\widehat{f}$ of the flow with size $< T - \Lambda$ must be less than $T$.}.

\aname{} has two key techniques: \textit{Error-Sensing} and \textit{Double-Exponential-Control}.
Error-Sensing can build the two bound by calculating MPE, where MPE comes from observing the amount of hash collisions.
% calculate MPE by observing the amount of hash collisions
% builds the two bound by observing the amount of hash collisions and calculating MPE.
Then, Double-Exponential-Control looks for the flows with potential large MPE to control them, and therefore the two bounds are close enough.

% the error of every flow to be lower than the user-defined threshold $\Lambda$
% not only provide bilateral certain error bounds for every flow, but also control the distance between two bounds for all flows under threshold $\Lambda$.
% \aname{} has two key techniques: \textit{Bound-Setup} and \textit{Double-Exponential-Control}.
% \textit{Bound-Setup} builds the two bound by observing the amount of hash collisions. Then, the Double-Exponential-Control looks for the flows with large distance between bounds and control their distance.
% helps us sense the error and distinguish which flows are at risk of losing control.
% This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
% For those flows at risk, \textit{Double-Exponential-Control} controls their error at great efficiency.
%
%\wyh{at great efficiency.}\sout{and achieves the best theoretical results.}
%
%Implementations on three platforms and evaluation on a test-bed and simulations verify the function and theoretical results of \aname{}. 




% Towards the design goal, we propose \aname{} that can not only provide bilateral certain error bounds for every flow, but also control the distance between two bounds for all flows under threshold $\Lambda$.
% \aname{} has two key techniques: \textit{Bound-Setup} and \textit{Double-Exponential-Control}.
% \textit{Bound-Setup} builds the two bound by observing the amount of hash collisions. Then, the Double-Exponential-Control looks for the flows with large distance between bounds and control their distance.
% helps us sense the error and distinguish which flows are at risk of losing control.
% This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
% For those flows at risk, \textit{Double-Exponential-Control} controls their error at great efficiency.
%
%\wyh{at great efficiency.}\sout{and achieves the best theoretical results.}
%
%\sout{The theoretical proofs of \aname{} is strictly tighter than existing proofs. }
% proof不能比较是否更紧（tighter），只有bound可以。
% In theory, \aname{} achieves the smallest space complexity among all sketches working at line rate.
% We implement \aname{} on three platforms, and conduct experiments on testbed and event-level simulation to verify the function and theoretical results of \aname{}. 
%Implementations on three platforms and evaluation on a test-bed and simulations verify the function and theoretical results of \aname{}. 



\ppp{Key Technique I: Error-Sensing.} 
We can build the two bounds if we can acquire the upper bound and the MPE, \ie, $\widetilde{f}=\widehat{f}-MPE$.
To find MPE, our idea is to observe the hash collision of the upper bound, where the amount of collision can reflect the error.
Take the well-known Count-Min (CM) \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
The total number is an upper bound/estimate no less than the actual flow size.
If a flow and many other flows are mapped to a same counter, its error will be large. Otherwise, its error is small.
Inspired by existing election algorithms \cite{tang2019mvsketch,frequent}, we find that the negative vote in an election is an ideal approach to observe the collision and calculate the MPE.
We replace the counter by an Error-Sensible bucket, so as to observe whether the collision is intensive. 
We will detail the Error-Sensible bucket in Section \ref{subsec:alg:onebucket}.
After observing the collision and getting the MPE, we use our second key technique to control the MPE.

% We  many election designs from Elastic, Majority, SpaceSaving and more \cite{tang2019mvsketch,frequent}.
% Thereafter we can find out high-risk buckets where can handle those buckets in which the error is about to out of control. 
% How to elegantly control the error is addressed by our second key technique.

% \ppp{Key Technique I: Bound-Setup.} 
% We argue that existing sketches cannot sense the error because their basic unit does not observe the collision, where collisions are closely related to error.
% Take the well-known Count-Min \cite{cmsketch} sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
% Differently, we devise an Error-Sensible bucket instead of a counter to observe whether the collision is intensive.
% The bucket has three fields: a ID for a candidate flow, a counter for ``YES'', and a counter for ``NO''.
% For each incoming packet, if its ID is same as the candidate, we increment ``YES''. Otherwise, we increment ``NO''. 
% When there are too many ``NO'', the recorded candidate flow will be replaced.
% Interestingly, \textit{we find and prove that the error is at most ``NO''}, and thereafter \wyh{we can find out high-risk buckets where} \sout{can handle those buckets in which }the error is about to out of control. How to elegantly control the error is addressed by our second key technique.




%by properly organizing these buckets.
%Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.

%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double-Exponential-Control
\ppp{Key Technique II: Double-Exponential-Control.} 
This technique aims to control the MPE of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the number of out-of-control flows sharply to zero by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
If one flow is about to out of control, we send it to the next array, and in total we have $d$ arrays.
The key is how to reduce the probability $\mathcal{P}$ of failure (\ie, a flow is sent out from the last array) sharply to nearly-zero.
%the flows entering the next array as sharply as possible.
Using a straightforward solution, the probability $\mathcal{P}$ can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}, overwhelming the number of flows easily.
Owing to the setting of double Exponential parameters, we strictly derive that, for $N$ packets, \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space to control the error of all flows below $\Lambda$ with failure probability $\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space.


%and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 

Our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We devise \textbf{ReliableSketch} to eliminate the outlier by bilateral tight bounds and control the error of all flows under threshold $\Lambda$.
    \item We theoretically prove that \anamelong{} outperforms state-of-the-art in both space and time complexity.
    \item We implement \anamelong{} on multiple platforms including CPU, FPGA, and Programmable Switch. Under the same small memory, ReliableSketch not only controls all flows, but also achieves near the best throughput, while its five competitors have thousands of out-of-control flows.
    % Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}

% \begin{table} [h]
% \begin{center}
% \vspace{-0.3cm}
% \caption{Paper Outline.}
% \vspace{-0.3cm}
% \label{table:outline}
% \begin{tabular}{m{0.35\columnwidth}|m{0.55\columnwidth}}
% % \hline
% \bottomrule[1pt]
% \textbf{Section}&\textbf{Contents}\\
% \hline
% % $\mathcal{S}$&a data stream\\
% % \hline
% \cref{sec:relate} New Problem  & Sense and Control the Error\\
% \cref{SEC:Algorithm} New Algorithm  & \anamelong{}\\
% \cref{sec:math} New Theory  & $O\left(\frac{N}{\Lambda}\times\ln(\frac{1}{\delta})\right) \rightarrow O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$\\
% \cref{sec:extensions} Extensions  & Priority and Network-wide\\
% \cref{sec:Implementations} Platforms  & CPU, FPGA, and P4 Switch\\
% \cref{sec:experiments} Evaluation  & Benchmarks, NS2, Testbed\\
% \toprule[1pt]
% \end{tabular}
% \vspace{-0.05in}
% \end{center}
% \end{table}
% \begin{figure}[htbp]
%     \prefig
%     \centering  
%     \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
%     \vspace{-0.15in}
%     \caption{Contribution Outline.}
%     \label{fig:intro}
%     \postfig
% \end{figure}
% % evaluation
%TBD ： new problem不准确
%
% As shown in Table \ref{table:outline}, 


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double-Exponential-Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$ space and $O\left(N+\delta\ln(\ln(\frac{N}{\Lambda}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_yt.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub

Approximately recording the frequency of items\footnote{In a data stream, an item could occur more than once, the frequency of an item refers to the number of occurrences of the item.} in high-speed data streams is a hot topic in recent years.
The most promising solution is using sketches, which are compact and fast with small error. 
%
% Typical sketch solutions include AugmentedSketch \cite{asketch}, UnbiasedSpaceSaving \cite{unbiasedsketch}, and HeavyGuardian \cite{heavyguardian}, CountMinSketch \cite{cmsketch}, CountSketch \cite{cmsketch}, SpaceSaving \cite{spacesaving}, and more \cite{???}.
Typical sketch algorithms include Augmented \cite{asketch}, HeavyGuardian \cite{yang2018heavyguardian}, Count-Min \cite{cmsketch}, Count \cite{countsketch},  SpaceSaving \cite{spacesaving}, UnbiasedSpaceSaving \cite{unbiasedsketch}, and more \cite{cusketch, coldfilter}.
% \wyh{"and more" is ok with "Typical sketch solutions include"?}
%\wyh{Comment: No more sketch estimates the frequency in recent years. The following sketches are not for frequency estimation.  COMPASS \cite{2021Online} (SIGMOD'21), CSC \cite{li2021building} (SIGMOD'21), and Correlation \cite{santos2021correlation} (SIGMOD'21).}
% Old: While most existing sketches manage to achieve smaller average error for different application scenarios or different measurement tasks, no existing work studies how to be aware of error for every n item (ErrorAware for short).
%\wyh{The sketch estimates most items accurately, but the other items are with large errors. While most existing sketches manage to achieve smaller average error, no existing work studies how to sense the error for every estimation (\ie, what is the maximum possible error of an estimation, namely error boundary) and control the estimations with large error (ErrorSensible for short).}
%
% Given any item, when we query its frequency using existing sketches, the error may be very small, but also may be very large.
%
Given any item, when we query its frequency using existing sketches, the error may be small, but may also be quite large.
% No existing work studies how to sense the error for each estimation (\ie, what is the maximum possible error of an estimation, namely error boundary) and limit the error of any element to the user-defined range (ErrorSensible for short). 
% No existing work studies how to sense the error for each estimation (\ie, what is the maximum possible error of \wyh{each} estimation, namely error bound) and control \wyh{the errors} of all items below a user-defined error threshold (ErrorSensible \wyh{problem} for short).
No existing work studies how to sense differentiated/personalized error boundary\footnote{For an item $e$ with its true frequency $f(e)$ and estimated frequency $\hat{f}(e)$, the error boundary of item $e$ is no less than the absolute error $AE=|\hat{f}(e)-f(e)|$. We aim to find different tight error boundaries for different items. The boundary is small when $AE$ is small and it large when $AE$ is large. } (\ie, the 
upper bound of the error) for each estimation and control the errors of all items below a user-defined error threshold.
We name this the \textit{ErrorSensible} ability.
We argue that ErrorSensible is critical in practice, and below we list four use cases:

\textbf{Case I:} Providing feedback for resource allocation. 
% As it is difficult to take account of the data distribution in sketch theory study, the required amount of memory advised by theory is not accurate in practice. 
% In other words, sketches need much less memory to achieve the user-defined accuracy.
As it is difficult to take account of the data distribution in sketch theory study, when achieving user-defined accuracy in practice, sketches need much less memory than that advised by theory.
However, existing sketches cannot sense the error. Users cannot know whether the allocated memory is too much or too little. 
%
ErrorSensible will be helpful for users to adjust the memory size to achieve the user-defined accuracy.

\textbf{Case II:} No longer sacrificing all estimates for large errors. 
In a real case, a cloud service provider uses the Count-Min sketch \cite{cmsketch} to monitor how much network traffic a user/service uses.
The most widely used Count-Min sketch achieves small average error.
But it often significantly over-estimates the frequencies of a few items. 
In business, any seriously over-estimated item/bill could incur legal issues, which is hardly tolerable.
But the service provider has no idea which items are significantly over-estimated using existing sketches. 
Therefore, the service provider reduces the estimated results of all items by $20\%$ before sending the bill to users, which seriously hurts the profit. 
The desired sketch should be error-sensible to avoid seriously over-estimated items/bills so that it can protect the profit.


\textbf{Case III:} Eliminating misclassification of frequent items.
As existing sketches often significantly over-estimate a few items, it is usual that an infrequent item is misclassified as a frequent item. 
In machine learning, such misclassifications can seriously hurt many models \cite{asketch,aggarwal2012event,aggarwal2010classification,yu2004false}. In networking, an infrequent item (\eg, a flow identified by source IP and destination IP) is often a control signal, which is more important than other items. When a link is congested, the congestion control policy often discards a part of frequent items to alleviate the congestion. If control signals are mistakenly considered as frequent items and discarded, the congestion will oppositely deteriorate.


\textbf{Case IV:} Reliable fault diagnosis.
Existing sketches often significantly over-estimates a few items.
%sketch运行 测试运行结果，当我们查看少数几个流
When one item is obviously over-estimated based on user knowledge, users cannot distinguish whether it is an accident in a normal sketch, or a malfunction caused by an incorrect configuration of the sketch. 
When achieving ErrorSensible that can sense and control the error, user can affirm that the algorithm is misconfigured if there is one large error.
% If we can achieve ErrorSensible, which senses and controls the error, we will make sure that the algorithm is misconfigured if there is one larger error.



% \ppp{Use Case I:} Memory allocation for sketches. 
% most sketches works in the fixed-window model. For example, one can divide a data stream into many sub-streams. Each sub-stream lasts for the same time interval, \eg, 1 minute. One can build a sketch for each sub-stream, and sends these sketches periodically to a remote collector.
% It is highly desired that each sketch has the similar error.
% \wyh{???}
% However, in practice, different sub-streams has different frequency distribution, different number of items and distinct items, and thus the accuracy of these sketches could vary a lot.
% If the sketch achieves ErrorSensible, we can use large size of memory and bandwidth for the current sketch if the error is large, and use small size of memory and bandwidth otherwise.


% \ppp{Use Case II:} a real case of a cloud service provider. The provider uses the Count-Min sketch \cite{cmsketch} to monitor how much network traffic an user/service uses.
% The most wide used Count-Min sketch has only over-estimation error, and could significantly over-estimates frequency in some cases. 
% Unfortunately, any seriously over-estimated bill could incur legal issues, which is hardly tolerable.
% However, we have no idea which item is significantly over-estimated using existing sketches. 
% Therefore, the provider reduces the estimated results of all items by $20\%$ before sending the bill to users, which seriously hurts the profit.

%
% \ppp{Use Case III:} Misclassification of items. As most sketch has over-estimation errors.
% \wyh{??}
% Therefore, it is usual that an infrequent item is over-estimated to be a frequent item. In machine learning, such misclassifications can seriously hurt many models \cite{agument,a1,a2,a36}. In networking, an infrequent item (\eg, a flow identified by source IP and destination IP) is often a control signal, which are more important than other items. When a link is congested, the congestion control policy often discards a part of frequent items to alleviate the congestion. If control signals are mistakenly considered as frequent items and discarded, the congestion will oppositely deteriorate.
\vspace{-0.05in}
\presec
\subsection{Prior Art and Their Limitations} \postsec

No existing sketch is ErrorSensible: Existing sketches can neither report tight error bound for every estimation nor control the errors of all estimations below the user-defined error threshold.
% Existing algorithms rely on probabilistic approaches without the accuracy feedback.
The most typical solution Count-Min (CM) sketch \cite{cmsketch} is a milestone with the best theoretical result.
% A CM sketch consists of multiple arrays of counters. When counting frequency, for each incoming item, CM picks one counter (called \textit{mapped counters}) in every array by calculating a hash value of the item's identifier, and then increments these mapped counters by one.
% When querying the frequency of an item, CM reports the minimal counter among all the mapped counters.
Given a data stream with $N$ items, when the absolute error of each estimation is smaller than $\varepsilon N$ in high probability $1-\delta$ (\eg, $1-\delta=95\%$), CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space.
% and can be built in real time by $O(\ln(\delta)N)$ totally.
For example, when CM reports that the frequency of an item is 1000, its true frequency may be 1 or 1000.
The sketch user only knows that true frequency is probably close to 1000 instead of complete certainty.
Further, it is impossible to control the error.
The followers of CM \cite{asketch, coldfilter} improve the algorithms in many aspects, but none of them is error-sensible.
% \textbf{Our goal is a sketch that is error-sensible and can achieve better performance in both time and space than non-error-sensible sketches.}
\textbf{Our goal is to devise a new sketch which is error-sensible and can achieve better performance in both time and space than existing sketches.}

% There are two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} If we solve challenge 1 that the maximum possible error is sensible, we need a reliable control strategy to control every estimations that may be uncontrollable, and it still needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\subsection{Our Proposed Approach}
%  technique to count the frequency and sense the error by counting the
We propose two key techniques to achieve ErrorSensible.
First, we devise the \textit{Collision-Sensing} technique that can estimate personalized error boundaries for distinct items.
Second, we devise the \textit{Double Exponential Control} technique to control the error of every estimation.

% This strategy can 
% This strategy can control the error with double exponential speed so that we can control the errors of all items.

% First, we perceive the maximum possible error of each estimation. Second, if the the maximum possible error becomes large and is close to the error threshold, we take actions to control the error. 
% We propose two key techniques for the two steps.


% It raises two key challenges. \textbf{Challenge 1 --- Error visibility.} Existing algorithms cannot report which estimations are uncontrollable. If we can know the maximum possible error of each estimation, we can find which estimations may become uncontrollable and try to control them by other strategies. \textbf{Challenge 2 --- Control strategy.} After the maximum possible error is sensible, we need a reliable control strategy to control every estimations that may be uncontrollable (\ie, the absolute error is greater than given threshold), and it needs to be fast, space-efficient, and easy to implement. No existing work can achieve it.

\ppp{Key Technique I: Collision-Sensing.} 
% Our idea is to bound the error by the number of hash collisions when electing the frequent item. 
% Sketches based on hashing consist of many identical units/buckets. 
We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
\textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.
% In addition, the bucket separates the most frequent flow from other infrequent flows, which is basis of our better time and space complexity.
% When inserting a new item, if its error bound is close to the error threshold, it is dangerous and we use the next technique to control its error.

%
\ppp{Key Technique II: Double Exponential Control.} 
% Given fixed amount of memory, 
This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
In our design, each layer has an increasing warning threshold.
% when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% We want fewer items to be inserted into the next layer.
This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 

% Specifically, whether an item is frequent or not, its probability of reaching the warning threshold should be smaller than a small constant.

%$R=\frac{1}{R_{\lambda} R_{w}}$ (detailed later).
% Our collision-sensible buckets can guarantee it. 
% In contrast, the frequent items in existing sketches often go to a deep layer in high probability \cite{coldfilter, yang2017pyramid}.


Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
\anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.
Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.

% To control all estimations under a threshold $\Lambda$, the warning thresholds are $\frac{1}{2}\Lambda$ (1st layer), $(1-\frac{1}{4})\Lambda$ (2nd layer), $(1-\frac{1}{8})\Lambda$ (3rd layer), $\dots$, and $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer.
% To insert an item, we first pick one bucket from the first layer by hashing, and then check whether the error bound is smaller than the warning threshold. If so, we insert the item to the bucket. Otherwise, we try to insert the item to the next layer.
% Only a small portion of items will be insert to the next layer and the size of each layer (\ie, the number of buckets) decreases exponentially. 
% It is notable that in most cases ($> 100\%-10^{-100}$) there is no item can reach the last layer, because the number of items that enter each layer decreases in double exponential speed, \ie, only $\frac{1}{2^{(2^{i})}}$ of items can enter the $(i+1)$-th layer (\eg, $\frac{1}{2^{(2^{6})}}=5.4\cdot10^{-20}$). That is why this technique is called double exponential control.
%嵌套 叠加 起名字
\ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We define ErrorSensible and devise \anamelong{} that can sense and control the accuracy for every item.
    \item In theory, we prove that \anamelong{} outperforms state-of-the-art in both time complexity and space complexity.
    There has been no breakthrough since 2005 \cite{cmsketch}.
    % And \aname{} can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We conduct comprehensive experiments on four datasets. 
     
     The \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intro_yt2.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub


%sketch方法
Accurate network measurement is often the first and fundamental step in many network management tasks, including accounting \cite{estan2002cusketch,sekar2008csamp,gupta2018sonata,zhou2020flow}, traffic engineering \cite{benson2011microte,yu2019dshark,guo2015pingmesh,geng2019simon,benson2010network}, load balancing \cite{miao2017silkroad,liu2019distcache,alizadeh2014conga,vanini2017let}, anomaly detection \cite{chen2020beaucoup,subsketchIMC}, and flow scheduling \cite{sharma2018approximating,li2019hpcc,bai2014pias}. 
These tasks benefit from precisely and timely network flow metrics including per-flow sizes, heavy hitters, heavy changes, or flow size distribution \cite{yang2018elastic}. 
Recently, the sketch algorithm \cite{zhang2021cocosketch,chen2021precise,liu2019nitrosketch,liu2016UnivMon, huang2021toward,huang2020omnimon,huang2017sketchvisor,huang2018sketchlearn,yang2018elastic}, which is compact and fast with small error, becomes the most promising solution.

% 1、测量重要 sketch是重要手段
% 2、当前最典型的CMsketch被使用时遇到了一系列问题：
% 3、总结出缺陷背后的原因是无法误差感知和控制 
% 4、当前学界提出了很多sketch，但是这些sketch没有关注且无法解决这个问题。因此这个问题很重要急切。。。。

% 1 网络测量重要
% 2 部署的时候是没有truth的
% 3 感知并且控制误差
% 4 （讲challenge）
% 5 现有解决不了

% 1 背景
% 2 现有sketch 都是和truth比 聚焦在误差如何感知和控制
% 3 

% 相关工作 
% sub1、定义问题、讲例子重要性
% sub2 相关工作



%wyh to Prof. Yang: Please see following comments.
% 上次讨论的框架：
% 第二段 现有工作：1、sketch的核心指标是误差。2、优化平均误差（部分、所有）。
% sketch在工业界部署的时候会遇到问题：如何感知和控制误差小于L。
% 现有sketch无法解决：1、理论无法解决。2、实践无法解决。来一个包希望感知误差。
% 重要性：放在sec2 也可以在下一段%计费 误差保证提供证据
% 第三段：重要性 design goal 

%目前的框架：
% 第二段：现有sketch的核心功能是估计频数。但是现有sketch在没有ground-truth的情况下，无法知道误差。因此我们要知道error bound。（这里是初步提出我们的目标，不会显得太晚或者突兀）
% 第三段：现有sketch无法解决误差感知和控制。1、理论上无法解决（理论的bound很松不可用，理论的bound是分布的bound，而不是每一个估计值的bound）。2、实践上无法解决。现有sketch盲目地把多个流的混合在一个counter内，无法感知误差。
% 第四段：描绘我们的具体目标。并且描述重要性。

%现有写作的问题（我自己觉得还没解决好）
%1、误差感知过度到误差控制似乎不够自然
%2、之前计费的那个例子没有直接写在intro里，担心不够solid（因为实际上的计费并不是直接数总的包数量）。感觉是不是不写比较好？

Current sketches have a variety of functions, most of which are based on one fundamental function: estimating per-flow size\footnote{In a packet stream, packets with the same flow ID (\eg, five tuples) are of a same flow. The size/frequency of a flow is the number of packets it contains. The flow size can generate many more advance metrics \cite{liu2016UnivMon}, and therefore estimating the per-flow size is the basic function.}. 
% 这个里有个转折，现在的研究是“平均误差”，为什么我们要转到最大误差。担心读者会想在没有ground-truth的时候测平均误差。所以我把平均误差改成了绝对误差。
% The core metric of per-flow size is the average error, and many sketches compete for the average error which is calculated by comparing the estimated sizes with the ground-truth (the true flow sizes).
The most well known Count-Min sketch (\cite{cmsketch}) derives the bound for the absolute error, and then a great many sketches compete for smaller absolute error which is calculated by comparing the estimated sizes with the ground-truth (the true flow sizes).
%The core metric of per-flow size is the absolute error, and many sketches compete for the absolute error which is calculated by comparing the estimated sizes with the truth (the true flow sizes).
%
% However, the ground-truth is unknown due to the high speed of network traffic in practice, and user known nothing about the error, such as the average error and the maximum error.
% 
However, the ground-truth is unknown due to the high speed of network traffic in practice, and the error cannot be calculated by comparison.
%TYPE A: However, the truth is unknown due to the high speed of network traffic in practice, and the error cannot be calculated as before.
%TYPE B: But when the user is finding the truth by a sketch in practice, the truth is unknown and the error cannot be calculated as before.
%
In practice, the error may vary a lot but users know nothing about the error of each flow. %之间讲average error不太严谨，因为average error可以通过采样计算或者理论保证。但是最大误差不行。
For example, when a Count-Min sketch \cite{cmsketch} reports that an estimated flow size is $10000$, the estimation error could be 0, 10, or even 10000.
%
It is highly desired to answer such a question: for each incoming packet of flow $f$, \textit{can we sense its error and elegantly control it at line rate}? In other words, for each incoming flow, can we give an estimation value additionally with an acceptable maximum error?
For the same example, one satisfactory report is that the estimation is 10000 and the maximum error is 20, which means that the true flow size is definitely in the range $[10000,10020]$. 
We believe that making progresses in this direction can significantly accelerate the application of sketching algorithm into practices.
\textit{Sensing and controlling per-flow error} have many benefits which are details in Section \ref{....}. 




%但是现有sketch都无法感知误差
Based on the classic sketches including Count-Min, recent sketches have made significant progresses in many aspects, such as the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian}, but they still do not handle the problem of \textit{Sensing and controlling per-flow error}.
%are neither concerned nor able to sense the error for all flows, let alone control the error.
On the one hand in theory, without prior knowledge of the flow distribution, the error bound is too loose (\eg, >10 times looser \cite{chen2021precise}) to be practical. In addition, existing error bound is a bound of error distribution rather than per-flow error: a personalized feedback of the error for each estimation. 
For example, when a flow with size of 3000 is estimated to be 3010, what we hope to know is ``the error of 3010 must be less than 20'' rather than ``the error of 3010 is less than 200 with $90\%$ probability''.
On the other hand in practice, existing sketches cannot sense the error when without groundtruth: their error could vary widely: from 0 to a very large value. 
%This means that the estimated size of a mice flow may be larger than the size of the largest elephant flow. 
The reason behind is that they \cite{liu2016UnivMon,yang2018elastic,liu2019nitrosketch,zhang2021cocosketch} let all hash collision happen naturally, and do not observe whether each collision is intensive.



%The design goal is to sense the error for every flow and then control the error of all flows. 
% We name this the \textit{ErrorSensible} ability.




\subsection{Our Proposed Approach}

As shown in Figure 1, this paper proposes the AgreeSketch, the first sketch to sense and control per-flow error. 
%We propose two techniques to address our goal of sensing and controlling the error.AgreeSketch
AgreeSketch has two key techniques: \textit{Error-Sensing} and \textit{Double Exponential Composition}.
\textit{Error-Sensing} can estimate personalized error boundaries for every flow.
This technique helps us sense the error and distinguish which flows are at risk of becoming inaccurate estimates.
For those flows with risk, \textit{Double Exponential Composition} controls their error and eliminates inaccurate estimate. 
The theoretical proofs of AgreeSketch is strictly tighter than existing proofs. 
Implementations on four platforms and evaluation on a test-bed and simulations verify the function and theoretical proofs of AgreeSketch. 

%老师，agree和disagree是不是可以考虑写成yea和nay, 这个是投票表决时候的专业术语，显得比较高级https://www.zhihu.com/question/36433186，分别表示赞同和反对。
%Double Exponential Composition
%Exponential Composition、superposition
%Composition比较好，有复合函数的“复合”，叠加的意思

\ppp{Key Technique I: Error-Sensing.} 
We argue that existing sketches cannot sense the error because their basic unit does not observe the collision, where collisions is closely related to error.
Take the well-known Count-Min sketch as example: its basic unit is a counter, which can only estimate the flow sizes by the total number of packets that mapped/hashed to it, no matter these packets are of the same flow or not. 
Differently, we devise an Error-Sensible bucket instead of a counter to observe whether the collision is intensive.
%, whose key idea is to bound the error by the number of "nay" when electing one frequent flow.
The bucket has three fields: a candidate frequent flow, a counter of "yea", and a counter of "nay".
For each incoming packet, if it differs from the candidate, we increment "nay". Otherwise, we increment "yea". When there are too many nays, the recorded candidate item will probably be replaced.
Interestingly, \textit{we find and prove that the error is at most "nay"}, and thereafter can handle those buckets in which the error is about to out of control. How to elegantly control the error is addressed by our second key technique.

%by properly organizing these buckets.
%Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.

%巧妙的理论推导，漂亮的理论技巧
%嵌套 叠加
%Double Exponential Composition
\ppp{Key Technique II: Double Exponential Composition.} 
This technique aims to control the error of all flows below a pre-defined threshold $\Lambda$.
Our key idea is reducing the number of uncontrollable flows sharply by careful parameter setting and smart theoretical techniques.
% Specifically, our sketch consists of multiple layers, we need to make the elements entering to next layer as few as possible.
% Specifically, our sketch consists of $d$ layers, we need to reduce the  as few as possible.
If one flow is about to out of control, we send it to the next array, and in total we have $d$ arrays. The key is how to reduce the probability $\mathcal{P}$ that a flow is sent to next array sharply.
%the flows entering to the next array as sharply as possible.
Using a straightforward solution, the probability $\mathcal{P}$ can be small as $2^{-d}$. Using our double Exponential parameters, we strictly prove that the probability can be reduced to $\frac{1}{2^{(2^d)}}$\footnote{When $d=8$, the probability is $8.6*0.1^{78}$, which is much smaller than $2^{-8}\approx 0.003$.}
Owing to the setting of double Exponential parameters, we strictly derive that \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
This is strictly better than the state-of-the-art theoretical result: CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space.

%and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time   and $O\left(N\ln(\frac{1}{\delta})\right)$ time 

\begin{figure}[htbp]
    \prefig
    \centering  
    \includegraphics[width=0.96\linewidth]{vldb/Figures/algo/introOutline.pdf}
    \vspace{-0.15in}
    \caption{Contribution Outline.}
    \label{fig:intro}
    \postfig
\end{figure}
% evaluation
%TBD ： new problem不准确
%

As shown in Figure \ref{fig:intro}, our key contributions are as follows:
% \ppp{Key Contributions:}
\begin{itemize}[leftmargin=*]
    \item We define ErrorSensible??? and devise \anamelong{} that can sense and control the accuracy for every flow.
    \item We theoretically prove that \anamelong{} outperforms state-of-the-art in both time complexity and space complexity.
    % There has been no breakthrough since 2005 \cite{cmsketch}.
    % And \aname{} can be easily deployed without pointers and dynamic memory allocation.
    % Its pipeline structure makes it easy to be implement in FPGA.
    \item We implement \anamelong{} in multiple platforms (\ie, CPU, FPGA, and Programmable Switch).
    Our evaluation shows that \anamelong{} is up to 300 times more accurate than others with the same memory consumption and faster processing speed.
    %现有算法需要2.5-100倍的memory。
    % \aname{} is easy to deploy without pointers and dynamic memory allocation.
\end{itemize}


% Given fixed amount of memory, 


% Specifically, the \anamelong{} consists of multiple layers, where each layer is an array of collision-sensible buckets.
% The insertion operation of each incoming packet starts from the first layer, and will enter the next layer only when it is out of control in the current layer, \ie, the collision-sensible bucket reports a large error.
% As the number of layers increases, the uncontrollable packets decrease to 0 sharply.
% In a common design, the uncontrollable packets decrease exponentially, \eg, $\frac{N}{2^d}$ packets enters the $d+1$-th layer, where $N$ is the total number of packets. 
% It is not fast enough when $N$ is large.
% Our new theorem shows that we can achieve double exponential decreasing speed (\eg, $\frac{N}{2^{(2^d)}}$) with sophisticated designs.
% As a result, \anamelong{} outperforms other sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.


% \ppp{Key Technique I: Collision-Sensing.} 
% We devise \textit{Collision-Sensing} technique to count the frequency and sense the error by counting the collisions when electing the most frequent item.
% Below, we show how Collision-Sensing works by using one bucket to sense collisions and error.
% The bucket has three fields, including a candidate frequent item, a counter recording the number of collisions, and a counter recording the total number of items.
% For each insertion of new item, if it is different from the candidate, a collision happens. When there are too many collisions, the recorded candidate item will probably be replaced.
% \textbf{Our key novelty} is that \textit{we find and prove that the error is at most the number of collisions}, and therefore the number of collisions is the error bound in this bucket (called collision-sensible bucket).
% Under strict mathematical guarantees, the error bound is often small, and we will use the next key technique to control the error if the error bound is going to get larger.



%
%wyh：把1/eps 改成 n/Lambda?
%

% \ppp{Key Technique II: Double Exponential Control.} 
% % Given fixed amount of memory, 
% This technique aims to control the errors of all items below a user-defined threshold $\Lambda$.
% The \anamelong{} has $d$ layers where each layer is an array of collision-sensible buckets.
% Not satisfied with controlling the errors of $2^d$ items with $d$ layers, we aim to control $2^{(2^d)}$ (\eg, $2^{(2^{6})}\approx 1.8\cdot 10^{19}$) items with $d$ layers, called Double Exponential.
% In our design, each layer has an increasing warning threshold.
% % when an item's error bound reaches the warning threshold in one layer, it will be inserted to the next layer with less density of stored items.
% When an item's error boundary reaches the warning threshold in one layer, we have to insert it into the next layer with higher warning threshold.
% % We want fewer items to be inserted into the next layer.
% This multi-layer design seems ordinary, but it can achieve Double Exponential only when three conditions are satisfied: 
% First, the warning thresholds must increase with exponentially decreased speed, \eg, $(1-\frac{1}{2^i})\Lambda$ for the $i$-th layer, where $\Lambda$ is the user-defined error threshold.
% Second, the number of buckets in each layer must decrease exponentially so that the total memory size is near optimal.
% Last but not least, each bucket should sense the error boundary accurately and the error boundaries of items are less likely to reach the warning threshold. 


% Further, \anamelong{} significantly outperforms existing non error-sensible sketches in both time and space complexity.
% The state-of-the-art theoretical result from CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to control the error of one estimation less than $\varepsilon N$ in high probability $1-\delta$. 
% \anamelong{} only needs $O\left(\ln(\frac{1}{\delta})+\frac{1}{\varepsilon}\right)$ space and $O\left(N+\delta\ln(\ln(\frac{1}{\varepsilon}))N\right)$ average time to achieve the same goal.
% Compared with seven competitors, our \anamelong{} can control the error of all items with $2.1 \sim 100 $ times less memory and $15\%\sim500\%$ faster speed. We release our source code at GitHub anonymously \cite{opensource}.



% There are three types of existing work, sampling \cite{?}, sketching \cite{?}, and top-k mining algorithms \cite{?}. The sampling and sketching algorithm cannot control all estimations ........????how?





% As the demand for high-speed data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information in one pass, have attracted wide interests.
% Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
% Owning to its efficiency, sketches \cite{asketch} have performed well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
% %
% When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
% Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
% Therefore, frequency estimation is
% the core of sketching a data stream.


% In this paper, we study a new problem---sensible Accuracy in data sketching.
% However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
% This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
% In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\varepsilon$, \ie, $|\hat{f}-f|<\varepsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
% As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
% Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\varepsilon$), but does not know whether each answer is accurate or how accurate each answer is.
% The reliability problem due to insensible accuracy undermines the sketch algorithm. 

% Our goal is to make the accuracy become sensible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \varepsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.






==> vldb/Body/intronotes.tex <==

Shortcomings of sketch:
1) not support range estimation
2) not support expansion
3) cannot separate infrequent items from frequent items, a never inserted item may report a large frequency. How to proof it by experiments?

Shortcomings of top k algorithms: SS USS       hash pipe CSS?
1) heap structure is not friendly for the pipeline

Arena Sketch:
1)a sketch that can accurately estimate the frequent item.
2)an accurate sketch that can be easily implemented on hardware.
3)a sketch that has a much higher no-error possibility.
4)a sketch that can report both an accurate lower bound and an accurate upper bound, while other sketches can only report upper bound.
5)a sketch that can support expansion.
6)a sketch that can separate infrequent items from frequent items.
7)%频数估计一定连续增加，不会跳变
8)%熵变化实时


==> vldb/Body/introv0.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\subsection{Background and Motivation}\postsub



% As the data volume increases everyday, the data preprocessing and reduction become 
% complete raw data is often unnecessary and inefficient in many applications due to . 
% Sketch algorithms are known for describing high-volume data streams with high efficiency. The data stream is a 
% As the demand for high-volume data stream processing grows, sketches \cite{cmsketch}, a type of probabilistic data structures, have attracted wide interests owing to the efficiency in terms of both time and space.
As the demand for high-volume data stream processing grows, sketches \cite{cmsketch}, a type of algorithms that profile the data stream and summarize key information from raw data, have attracted wide interests.
Sketches have efficient data structures with small (sub-linear) space, supporting fast update or lookup in constant time.
Owning to the high efficiency in terms of both time and space, sketches \cite{asketch} have perform well in many applications, including online machine learning \cite{Sketchingclassifiers}, graph stream processing \cite{gsketch,graphstream1,graphstream2}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, and complex aggregate queries \cite{complexaggre}. 
%
When sketching a data stream, \ie, a sequence of items ordered by time, a common function of all kinds of sketches is to count the number of occurrences of each item, called frequency estimation. 
Based on frequency estimation, a sketch can process many significant tasks, including finding frequent items, changed items, estimating cardinality, frequency distribution, and entropy\footnote{1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}. 
Therefore, frequency estimation is
the core of sketching a data stream.
% The performance of frequency estimation directly affects the sketch in many aspects, including its generality for various tasks, adaptability for different platforms, accuracy, space cost, and time cost. There are many works focus on improving the accuracy of frequency estimation \cite{pyramid,?}.

In this paper, we study a new problem---Visible Accuracy in data sketching.
However, existing sketches are not reliable enough, because the user can hardly know the accuracy of each estimation output.
This problem has two aspects. First, there is a giant gap (around 10 times) between the accuracy in theory and the real accuracy.
In theory, existing sketches guarantee: with high probability $1-\delta$ (\eg, $1-\delta=95\%$), the absolute error of each estimation is smaller than a small threshold $\epsilon$, \ie, $|\hat{f}-f|<\epsilon$, where $\hat{f}$ is the estimate value and $f$ is the true frequency.
As shown in figure \ref{?}, in real datasets, the real absolute error is about 10 times smaller than the theory. Reducing the gap between the theory and real performance is quite challenging \cite{siam14?,cmbound?}, because there are many practical factors that affect the performance of sketches, including the frequency distribution of the real dataset and the order of item arrival.
Second, existing sketches guarantee the overall accuracy (\ie, the average performance), but the accuracy of each single output is still unknown. In other words, the user only knows that the estimation answer is likely to be accurate (defined as $|\hat{f}-f|<\epsilon$), but does not know whether each answer is accurate or how accurate each answer is.
The reliability problem due to invisible accuracy undermines the sketch algorithm. 

Our goal is to make the accuracy become visible for every estimation. If a sketch can report the accuracy of every estimation (\eg, the absolute error is smaller than $0.1 \epsilon$ in this estimation), it will address the above reliability problem from both of the two aspects. First, whatever the scenario changes, the sketch will report as much as the actual accuracy is, with perfect robustness. Second, the estimation answer is no longer likely to be accurate, but to clearly show how accurate it is.



% 1) \textit{Generality} for various tasks.
% It can be applied to many approximate data stream processing tasks\footnote{A data stream is defined as a sequence of items ordered by time.
% \\1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding top-k frequent items is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time windows vary a lot.\\~4) Cardinality estimation is to estimate the number of distinct items in the data stream.\\~5) Frequency distribution estimation is to estimate the ratio of the item whose frequencies are equal to a given value\\~6) Entropy estimation is to estimate the entropy of item frequencies.}, 
% including finding top-k frequent items, finding heavy change, cardinality, frequency distribution, and entropy estimation.
% These are fundamental tasks in database query optimization \cite{schweller2004reversible}, information retrieval \cite{chowdhury2010introduction}, data mining \cite{cheng1999entropy}, data quality estimation \cite{li2012truth}, and more \cite{flowradar}.
%vldb sigmod topic搜关键词+sketch
% These tasks are important in database query optimization \cite{schweller2004reversible}, information retrieval \cite{chowdhury2010introduction}, data mining \cite{?}, data quality estimation \cite{?}, and more \cite{?}.
%information retrieval 是本书，要不要加页码？
% network measurement and management, web search engines [31], anomalies detection [32, 33], time series forecasting and outlier analysis [34]. [41, 42], network measurement and monitoring [43]. 
%
% Capability for two-sided estimation.
% % Double Bound
% Capability for interval estimation.
% both over-estimation and under-estimation.



\presub
\subsection{Our Proposed Approach} \postsub

% Our key idea of achieving versatility is to design a bucket structure including at least an ID field and a pair of counters.
Our key idea of achieving versatility is to append more kinds of fields, including at least an ID field and a pair of counters, to each bucket.
Specifically, each bucket's structure is $\langle ID, pair counter, \dots\rangle$.
With only a pair of counters, we can already achieve much flexibility for estimation and processing tasks.
% When only have a pair of counters for each ID, we can already achieve much flexibility for estimation and processing tasks.
% Typically, each bucket has three fields: $ID$, $C1$, and $C2$.
% As we have two counters for each ID, we can achieve much flexibility for estimation and processing tasks. 
For example, we can use the pair counter to get the upper bound and lower bound of frequencies of the recorded ID, and can also estimate the frequency of items whose IDs are not recorded.
%算法里说明为了实现dominant 所以选的某种替换方案
We can have more choices and flexibility to determine which item should be kept when two distinct items collide in one bucket.
%
Further, we can add more fields in each bucket to achieve more processing tasks, such as finding DDoS attacks \cite{ddos}, data attributes summary, and data aging. The details are provided in Section \ref{subsec:alg:scalability}.

Based on <ID, pair counter> structure, our \aname{} achieves the above five aspects simultaneously.
1) Generality for various tasks (Section \ref{SEC:app}): We implement five processing tasks in one versatile sketch. Moreover, we show that our versatile sketch can process many more tasks with more fields in Section \ref{subsec:alg:scalability}.
2) Capability for interval estimation (Section \ref{subsec:alg:Standard}): The pair counters can provide both the upper bound and lower bound of item frequencies. Furthermore, we prove that both bounds are tight and are accurate for frequency estimation.
3) Adaptability for distributed systems (Section \ref{subsec:alg:extra}): \aname{} is flexible, easy for expansion, compression, and aggregation.
4) Flexibility for incremental deployment (Section \ref{subsec:alg:extra}): \aname{} can compress the pair counter into one counter, aiming to be compatible with the most widely used CM/CU sketch.
5) Certainty for dominant items (Section \ref{subsec:math:dominant}): \aname{} can keep the dominant item (frequency larger than 50\%) in each bucket relying on the pair counters.



2) \textit{Capability} for interval estimation\footnote{The interval estimator reports both an over-estimated value and an under-estimated value at the same time.}.
% it is the first sketch for two-sided boundary estimation. 
A common function of sketches is the frequency estimation, which is to query the number of times that a given item appears in the data stream. 
Our \aname{} can report a pair of integers $\langle a,b\rangle$ for any given item, and we make sure that the exact answer must be in interval $[a,b]$. 
The length of the interval is small bounded in theory.
Interval estimation is useful in practice.
For example, when finding frequent items whose frequency is larger than $\mathcal{T}$, we can select the items whose over-estimated values are greater than $\mathcal{T}$ to avoid False Negative\footnote{A result that the algorithm indicates negative but it should be positive.}, \ie, no item whose frequency is larger than $\mathcal{T}$ is left out. Also, we can select the items whose under-estimated values are greater than $\mathcal{T}$ to avoid False Positive\footnote{A result that the algorithm indicates positive but it should be negative.}. 
For another example, when finding items whose frequency is in a given range $[l,r]$, we can make sure the reported item must be in $[l,r]$ as long as the estimated interval is contained in the given range.
%


\vspace{0.05in}
\ppp{Key contributions:}
\begin{enumerate}[1)]
    \item  We define the five aspects of versatility and propose a versatile sketch, which is generic for various tasks, capable for interval estimation, adaptable for distributed systems, flexible for incremental deployment, and certain for dominant items.
    \item  We derived analytical performance guarantees and conducted extensive experiments to verify the versatility of our \aname{}.
\end{enumerate}



% mathmatic l....
% Experimental results, 
% Open source ..
%代办：1、算法部分添加discussion，关于多field。双counter的替换策略选取
% pair counter单复数统一


% Our key idea of achieving versatility is to add more fields for each bucket: ID field, $counter_1$ field, $counter_2$ field, $counter_3$ field\dots.
% The more fields it uses, the more functions could be achieved.
% % Typically, we find using two counters are already to achieve many functions.
% Typically, we find using two counters can achieve many functions already.
% % \ref{...sliding window, timestamp, aging.  flag, used to be a large flow, flowlet... flag, eviction, totall correct, freezing counter, ... }.

%para 3
% This paper mainly focuses on how to use two counters to achieve many functions.
% In our design, we give a simple case study, using a high counter and a low counter, aiming to achieve the above design goal.
% %
% For simplicity, we designing the 3-tuple $<ID, freq1, freq2>$, meeting the following requirement:
% First, for the recorded item, we can estimate its upper bound and lower bound of its frequency.
% Second, for the cold items (whose IDs are not recorded in buckets), we need to give a upper bound of their frequency.
% % Third, when two distinct items are mapped into one bucket, we use to use this two counter to decide the eviction policy.
% Third, when two different items are inserted into a same bucket, we use this two counter to decide the eviction policy.
% % To satisfy these three requirements, we have several choice.
% We have many design choices of the 3-tuple, including 1) \textit{high and low}; 2) total and pure; 3) positive and native counters.
% These choices can achieve the similar results, different functions, and we show how to use \textit{high and low}. 
% The descriptions of \textit{high and low} are provided in section \ref{?} and we show how other two choices achieve different functions in section \ref{}. We provide through mathematical analysis in section \ref{sec:math} and experiments in \ref{sec:experiments}.



% para 5
% math,,, experiment ....



% %Sketch, Buckets, ideal
% A typical sketch distributes a data stream to large amounts of buckets, and each bucket processes a subset of the data stream independently. The key design of a sketch is its buckets, each of which receives incoming items and reports the frequency of a given item. We will focus on designing a bucket in the following parts.
% %
% We should record two kinds of information, \ie, item IDs and frequencies, because we need them in \textit{finding Top-k frequent items} and we can indirectly estimate the distribution and entropy through frequency.
% Besides, we are more concerned about high-frequency items, because they are the core factors of error and they get more attention in applications.
% %
% As the space is limited, we should make a trade-off between memory efficiency and recording all items.
% A straightforward approach is to abandon the IDs of infrequent items. In other words, an \textbf{ideal bucket} can maintain both IDs and frequencies of the top x items and maintain the total frequencies of all other items.
% However, it is hard to maintain these information in practice. Because the bucket not only can hardly identify which items are the most frequent but also can hardly find true frequencies of the frequent items.
% Therefore, we relax the requirement of ideal bucket from two aspects. First, we only require maintaining the ID of the most frequent item instead of top x frequent items, because the second-largest frequency is often much smaller than the largest frequency.%需不需要更详细地讨论？
% Second, we require both an over-estimated frequency and an under-estimated frequency instead of an exact frequency.

% We design a new bucket, called \textbf{versatile bucket}, to meet the requirement. 
% In the bucket, we use a counteraction strategy to find the most frequent item, where the item whose frequency is larger than half must be found. 
% A versatile bucket has three fields, a \textit{high} counter, a \textit{low} counter, and an \textit{ID} recorder. The counteraction strategy only uses the \textit{low} counter and the \textit{ID} recorder.
% When a new item $e$ comes, if the \textit{ID} recorder is empty or the same as new item $e$, we set the \textit{ID} recorder to $e$ and increase the \textit{low} counter by $1$. Otherwise, we decrease the \textit{low} counter by $1$. After that, if the \textit{low} counter equals to $0$, we replace the item in \textit{ID} recorder with $e$.
% The \textit{ID} recorder can find the most frequent item approximately.
% Besides, the high counter increases by $1$ when a new item $e$ comes.
% When querying the frequency of the item recorded in the \textit{ID} recorder, we can get its over-estimated/under-estimated frequency by $(high+low)/2$ and $low$ respectively. And we can estimate the over-estimated frequencies of other items by $(high-low)/2$.
% As a sketch, \aname{} inserts an incoming item into multiple buckets and summaries all mapped buckets when querying.
% We devise a conservative update strategy to reduce unnecessary insertions and prove its correctness rigorously.





% 1、sketch算法的核心思想是把所有的item通过哈希插入到N个桶中的d个。查询时每个桶分别给出对频数的估计。因此设计一个合适的桶结构是设计sketch算法的关键点。要设计合适的桶结构，就要先回归到我们的5个目标，了解清楚我们究竟要存储哪些信息。从“通用性”支持的任务来看，我们需要保存元素的频数信息和ID。由于我们更关注高频元素，一个理想的情况是：忽略低频元素的ID，保存桶内最高频的k个元素的频数和id，以及其余元素的频数之和。这样的情况是 存储信息与内存占用之间最好的trade off。但是做不到理想情况。

% 2、几乎没有算法可以做到上述理想情况。我们从实验/理论分析可以看出，在常见分布下，第二大的元素频数往往远效于第一大的元素。因此我们仅保存最高频的元素，令k=1。另一方面，很难有算法可以在亚线性memory下精确求出某个元素的频数（可以构造算法证明没有，需要数学吗？）。因此，我们选择为最高频的元素提供尽可能准确的高估/低估估计。此外，我们的算法还要能够求出最高频的元素，但这也是不可能办到的。因此我们引入了dominant item的概念，即我们能保证求出频数大于50\%的元素，而且元素频数越高，留下来的概率越大。

% 3、具体的做法。相比于现有sketch，我们提供的一个新功能是interval。因此我们从interval入手来讨论我们对桶结构的设计。因为我们要给出高估/低估值与高频元素id，我们至少需要两个counter field和一个ID field。首先设计求高频元素的算法。有多种办法，“一样加，不一样不加”。“一样就加，不一样概率减”。概率替换/减到0替换。我们选择了“一样加，不一样不加，减到0替换”。这个算法能保证求出频数大于50\%的元素。同时，我们利用剩下的一个counter来记录元素总数。这时我们可以发现一个有趣的结论: (high+low)/2 是高频元素高估值， (high-low)/2是剩余元素之和的高估值。 除了桶设计以外，我们还引入了保守更新的策略。

% 4、这样的结构为啥versatile。


% Based on the Counter-Key-Counter structure, \aname{} achieves five functions.
% 1) It can report the possible range of the frequency of the recorded item by $[low, (high+low)/2]$ and that of the unrecorded item by $[0,(high-low)/2]$.
% 2) The recorded items and their frequencies can be applied to finding heavy hitters and heavy change. Further, the function of estimating frequency can be used for estimating item size distribution and entropy. 
% 3) A CKC bucket is flexible for splitting into two buckets, merging two buckets. Therefore, \aname{} is flexible for expansion, compression, and merging.
% 4) \aname{} can replace each CKC bucket with a counter whose value is $(high+low)/2$ to get an accurate sketch for frequent item. %light 没写
% 5) The dominant item in each bucket will be recorded in the ID field and its frequency can be estimated accurately.

% 5、并且做了数学证明、实验、开源。文章结构的overview。



% We propose a new sketch, namely \textit{Versatile Sketch}, in this paper. 
% It is based on Counter-Key-Counter (CKC) array structure and achieves versatility of five properties.
% %2、
% Our key idea of Counter-Key-Counter is to preserve both IDs and frequency upper/lower bounds for frequent items, which are more important than infrequent items for which we only preserve the upper bound.
% Specifically, the \aname{} is an array of Counter-Key-Counter buckets, and the devised bucket has three fields, a \textit{high} counter, an \textit{ID} recorder, and a \textit{low} counter.
% The \textit{ID} recorder can approximately record the most frequent item mapped to the bucket, and the item can be recorded for certain if the frequency of the item is larger than half of the total frequency of the items mapped to the bucket. The items whose frequencies are larger than half are called \textit{dominant item}.
% In a bucket, we can get the upper/lower bound of the frequency of the dominant item by $(high+low)/2$ and $low$ respectively. And we can estimate the upper bound of frequencies of infrequent items by $(high-low)/2$.
% As a sketch, \aname{} inserts an incoming item into multiple buckets to reduce hash collisions, and summaries all mapped buckets when querying.
% We devise a conservative update strategy to reduce unnecessary insertions and prove its correctness by rigorous analysis because the correctness is unintuitive.

% %3、
% Based on the Counter-Key-Counter structure, \aname{} achieves five functions.
% 1) It can report the possible range of the frequency of the recorded item by $[low, (high+low)/2]$ and that of the unrecorded item by $[0,(high-low)/2]$.
% 2) The recorded items and their frequencies can be applied to finding heavy hitters and heavy change. Further, the function of estimating frequency can be used for estimating item size distribution and entropy. 
% 3) A CKC bucket is flexible for splitting into two buckets, merging two buckets. Therefore, \aname{} is flexible for expansion, compression, and merging.
% 4) \aname{} can replace each CKC bucket with a counter whose value is $(high+low)/2$ to get an accurate sketch for frequent item. %light 没写
% 5) The dominant item in each bucket will be recorded in the ID field and its frequency can be estimated accurately.

% %4 
% The key novelty of \aname{} is our Counter-Key-Counter structure which is quite different from existing works.






%%%%%%%%%%%%%%%
%data stream frequency estimation重要性 挑战
% In data stream scenarios, huge volumes of high-velocity data are being produced continuously in real time, such as sensor data from the Internet of Things (IoT), graph streams, video streams, web Interactions, network traffics, and twitter posts \cite{?}.
% In these scenarios, data is organized as a sequence of items. Some common statistical analyzes, such as item frequencies \footnote{?}, heavy hitter \cite{?}, heavy change \cite{changedetection}, flow size distribution \cite{flowsizedistribution}, and entropy \cite{estimatingentropy}, are often require to process. And the analyzes are often being processed on the fly \cite{?}, which means the incoming items should be taken in real time and the statistical results could be fetched at anytime. 



% \textbf{The high-speed and high-volume data makes the data stream processing quite challenging.} First, the memory usage of the processing is limited in order to be implemented in high-speed medium (\eg, SRAM, ASIC \cite{?}??) whose footprints are expensive and limited.
% Second, the stream data should be processed on the fly. Finally, the accuracy of the analyze should be accurate enough.


%介绍sketch
% %sketch分类 讲不同
% Sketches, a kind of compact probabilistic data structure(s?), has become popular in recent years for stream data processing \cite{?}. Sketches are designed for estimating the frequency of items \cite{?} and the estimated frequency would be used for other statistical analyzes, including heavy hitter, heavy change, item size distribution, and entropy. 
% To explain the key idea of sketches, we choose the Count-Min (CM) sketch as an example. The CM sketch is a two-dimensional array counters with depth $d$ and width $w$. There are $d$ independent hash functions associated with $d$ rows. To insert item $e_i$, the CM sketch maps $e_i$ to \textit{the mapping counters} by the hash functions in each row, and increment each mapping counter by 1. To estimate the frequency of $e_j$ the CM sketch returns the minimum mapping counters.
% The key idea of sketches is to solve collision by mixing and answer the minimum collision.
% Compare with the hash table\cite{?}, sketches has the following three advantages. First, sketch is a sub-linear memory algorithm \cite{?} which is much more memory efficient than the per-item-state techniques (hash tables) \cite{?}. Second, the time for sketches to insert per item is constant while that for the hash table is not.
% Third, sketches is friendly for the hardware with the pipeline/multistage structure\cite{?} and is friendly for parallel processing because all units of sketches are independent.

% %需要同时测量多个任务，需要多样性
% %sketch功能缺乏，需要额外的数据结构补充，但是不能被视为完整结构。
% However, the weakness of sketches is the functional diversity. The ordinary sketches can only record the frequencies of items. The users can only resort to different kinds of additional special-designed structures if they needs any other information, such as the identification (ID) of frequent items, the average/latest arriving time of an item, or the average/maximum size of the packet load for a flow in network traffics scenario. Most additional structures only utilize the output frequency from sketches but cannot improve the performance of the sketches, which \textit{can hardly be regarded as an integral structure}.

% To add functions to the sketches, one straight forward idea is to add a new ID field to store items along with each counter. As sketches mixes all the frequency of the items mapped to the same counter, a serious error might happen when the queried infrequent item collides with a frequent item. It would be quite useful if we can record the most frequent items in every counter and separate their frequencies apart.




    %
% We propose a new sketch, namely \textit{Versatile Sketch}, in this paper.
% Our key idea comes from the open contest that the competitor whose ability exceeds the sum of all other competitors must be the winner on the stage, regardless of the order of the competitors.
% Instead of the counter, the basic unit of \aname{} is a bucket. Each bucket has three fields, a \textit{high} counter, a \textit{low} counter, and an \textit{ID} recorder. The high counter increments by $1$ when an item is inserted to the bucket, which is the same as the CM sketch.
% The item in the \textit{ID} recorder is the defender and the \textit{low} counter represents the health point of the defender. For an incoming item $e$ mapped to current bucket, we first check the ID recorder. If it is empty, we store item $e$ in the recorder and set the low counter to $1$. Otherwise, we check whether the defender item in ID recorder is $e$. If so, we increment the low counter by $1$. Otherwise, $e$ is an attacker so we decrement the low counter by $1$. If the low counter equals to $0$, the defender was defeated and we set the ID recorder to $null$.

% Among all items mapped to current bucket, the item whose frequency is larger than the sum of the others must be a defender left in the ID recorder and the item is called \textit{the dominant item}.
% We can estimate the frequency $f$ of the defender by $low$ and $(high+low)/2$, where $low\leq f \leq (high+low)/2$. And we can estimate the frequency $f'$ of other items mapped to current bucket by $(high-low)/2$, where $0\leq f' \leq (high-low)/2$.
% It is trivial that $low$ is the underestimated frequency of the defender but the overestimation $(high+low)/2$ is not straightforward. Suppose the defender is $e$. At the latest time $t_0$ that the ID recorder was set to $e$, the $low$ equaled to $0$. Before , the $e$ must appears no more than $high/2$ ( equals to $(high+low)/2$) times, because the dominant item, if exists, must be left in the ID recorder. After time $t_0$, $e$ remained in the recorder. In this period, every incoming $e$ will increased $(high+low)/2$ by $1$ and other items 
% did not change $(high+low)/2$. Therefore, $(high+low)/2$ is the overestimation. 
% Suppose the defender is $e$. For the item $e'$ ($e'\neq e$), $(high-low)/2$ is the overestimation of the frequency of $e'$. Because we can extract $low$ item $e$ from $high$ total items and it is impossible to occupy half of the rest because of the property of the dominant item.
% Additionally, if all collisions (\ie, the case that the incoming item is not the recorded item) happen between the final defender $e$ and other items, $(high+low)/2$ is the no-error estimation of $e$.

% The \aname{} has the following seven novel functions.
% \begin{itemize}
%     \item it can mining out the dominant item in each buckets and has higher accuracy for the dominant item.
%     %
%     \item it is the first sketch for two-sided boundary estimation while the other sketches can only do one-side estimation.
%     %
%     \item it can be applied to four applications, including heavy hitter, heavy change, item size distribution and entropy.
%     %
%     % \item it is hardware-friendly because it can be easily implemented in pipeline structured hardware and it do not need heap or pointer.
%     %
%     \item its structure is flexible for expansion, compression, and merging, which are important operations for distributed systems.
%     %
%     \item it can refine itself to get Heavy \aname{} which is more accurate than CM/CU sketch and it can refine itself to get Light \aname{} which can estimate infrequent items accurately.
%     %
%     % \item it supports conservative update which can improve the accuracy.
%     %
%     % \item KV store??
% \end{itemize}



% the dominant item %重要性。

% \old{One of the most fundamental problems in approximate data stream mining is finding top-$k$ items. }
% %
% Top-$k$ is defined in terms of various metrics. Four kinds of top-$k$ items under different metrics have attracted wide attention by researchers: 1) top-$k$ \textit{frequent items} \cite{frequent, frequent2, frequentstream, countsketch, persistentsketch}, 2) top-$k$ \textit{heavy changes} \cite{revsketch, kary, flowradar}, 3) top-$k$ \textit{persistent items} \cite{persistentsketch, persisitem}, and 4) top-$k$ \textit{Super-Spreaders} \cite{superspreader}. 
% %
% \textit{Frequent items} refer to items whose numbers of appearances exceed a predefined threshold. \textit{Heavy changes} refer to items whose frequencies change drastically over two adjacent time windows. \textit{Persistent items} are items which appear in more time windows than others. \textit{Super-Spreaders} refer to sources that connect to a large number of distinct destinations. 
% %
% Although these four kinds of tasks have different metrics, we find that if an algorithm does well in finding frequent items, it can also well handle the other three tasks.
% %
% The reason behind is discussed below. 
% %
% To find heavy changes in two adjacent time windows, we can first find all frequent items in both time windows respectively since heavy changes must be frequent items in at least one time window.
% %
% Then heavy changes can be detected through calculate the absolute change in frequencies of those frequent items in the two time windows.
% %
% Persistent items and frequent items are equivalent if the frequency of an item is defined as the number of time windows in which it appears.
% Similarly, for finding Super-Spreaders, we only need to view the number of destinations an item connects to as its frequency.
% %
% %As to finding Super-Spreaders, we can view the number of destinations an item connects to as its frequency, then the task is transformed to finding frequent items. 
% %In conclusion, algorithms for finding frequent items can deal with the above tasks, and if it performs well in finding frequent items, it will probably also achieve good performance in these tasks.
% %
% %Sketches, a kind of probabilistic data structure, have attracted wide interests in recent years, due to their memory efficiency and small error for .....
% In summary, if a data structure can accurately find frequent items, it can also well handle other three tasks. Therefore, we only consider finding frequent items in this section below.
% %
% In practice, sketches, a kind of probabilistic data structure, have been widely used in finding top-$k$ items, due to their memory efficiency and small error for estimating item frequencies.


% %
% \textit{Unbiased estimation} is well acknowledged as a theoretically elegant and pragmatic property.
% %Therefore, we aim at devising a sketch which can report unbiased estimation of item's frequency.
% %
% % for frequency estimation
% %Frequency estimation is the key technique in finding frequent items. of a frequency estimation algorithm.
% %
% Unbiased estimation of item frequencies is beneficial for several global estimation problems, such as global heavy hitters, global distribution, global entropy, \etc For example, to measure distributed data streams, one data structure is deployed for each data stream. If their estimations are biased, the error will accumulate when the data structures are aggregated.
% %
% Further, unbiased approaches could stimulate theoretical progress in sketches. Although numerous sketches have been proposed, only a very few of them (Count-Min Sketch \cite{cmsketch}, Count Sketch \cite{countsketch}) have explicit and concise theory bounds and proofs, and most of the others show error bounds and proofs that are fairly complicated. One of the primary reasons for this is that their estimations are biased.


% Among a large number of algorithms for finding frequent items \cite{cmsketch, cusketch, countsketch, spacesaving, frequent, losscounting, unbiasedsketch}, one recent work, Unbiased SpaceSaving (USS) \cite{unbiasedsketch}, achieves unbiased estimation. 
% %
% While USS makes a great contribution in terms of unbiased estimation, its accuracy is relatively low, \ie, its variance of estimation is large. As a result, when it is applied to other tasks (\eg, finding heavy changes, persistent items, or Super-Spreaders), the inaccuracy of frequency estimation will incur large error for other tasks, which may be the reason why USS was only used for frequent items in the paper \cite{unbiasedsketch}.
% %the shortcomings brought by its inaccuracy grow disturbing, which makes it inappropriate for USS to be deployed in these task. 
% %
% %In summary, prior unbiased algorithms, such as USS, are too inaccurate to be generic, this is why no prior algorithm achieves both unbiased estimation and generality.
% %
% The goal of our study is to devise an algorithm which is unbiased, and accurate enough to be generic for other tasks.



% %The goal of our study is to devise an algorithm which is unbiased as well as accurate in the task of finding frequent items and is capable of handling the other three tasks mentioned above. 
% %In processing high-rate data streams, finding \textit{frequent items} has long been a crucial problem and an active topic \cite{frequent, frequent2, frequentstream, countsketch, persistentsketch}.
% %
% %A lot of applications involve finding \textit{frequent items}, such as congestion control \cite{usagefrequent1} and caching of forward table entries \cite{usagefrequent3}.
% %应用需要改

% %Items with other special characteristics are also of general interest. Some of the most interested among them are heavy changes \cite{revsketch, kary, flowradar}, persistent items \cite{persistentsketch, persisitem}, and Super-Spreaders \cite{superspreader}.
% %

% %
% %These items are especially important in the field of security \cite{usageother2, usageother3}. Existing algorithms are often utilized to detect denial of service attacks \cite{usageother2}, and worms \cite{usageother3}.

% %

% \presub
% \subsection{Our Proposed Approach} \postsub

% \paragraph{rationale:}eliminate the error of minor flows.
% \paragraph{arena game}
% \paragraph{properties}

% In this paper, we propose a new sketch, namely \aname{}, which is unbiased, accurate, and generic for finding top-$k$ items. 
% %
% We use a simple example to show the key idea of \aname{}. We use a counter and a list. The counter, namely the Waving Counter, provides an unbiased estimation of item frequencies and the list is used to store $k'$ $(k'>k)$ frequent items.
% %
% For each incoming item $e$, we use a hash function $s(e)$ to hash $e$ to $+1$ or $-1$, and then increase or decrease the Waving Counter by 1. Afterwards, we estimate $e$'s frequency using the Waving Counter. 
% %
% %We have proved that the counter can provide an unbiased estimation of frequency for any item appeared before.
% If its frequency is larger than the smallest frequency in the list, we exchange them.  
% %
% Based on this idea, we use a group of Waving Counters and lists, and add additional fields in the list to achieve higher accuracy (see details in Section \ref{subsec:alg:struct}).
% %



% Below we explain the rationale of \aname.
% The value of the Waving Counter fluctuates over time, and it is quite analogous to the waves in the sea. 
% %
% Where there is a heavy swell, there is probably a strong flow driving it.
% %
% Therefore, we expect to catch a frequent item when the absolute value of the counter is fairly high.
% %
% %This idea is quite reasonable. 
% %
% Specifically, given an incoming item, we use the Waving Counter to unbiasedly estimate its frequency.
% %provide unbiased estimation for its frequency.
% %The value of the Waving counter can provide an unbiased estimation to the incoming item.
% If the estimated frequency is large enough, it is with high probability that the incoming item is frequent enough to replace the least frequent item in the list.


% \aname{} has four advantages. First, it is unbiased, and we theoretically prove that the estimated frequency of \aname{} is unbiased in Section \ref{subsec:math:unbiased}. 
% %
% Second, our theoretical and experimental results show that the error of \aname{} is much smaller than SpaceSaving and Unbiased SpaceSaving.
% %
% Third, \aname{} is generic. To verify this, we apply \aname{} to four applications: finding frequent items, finding heavy changes, finding persistent items, and finding Super-Spreaders.
% %
% Fourth, \aname{} is fast. For each insertion or query, we only need to access one bucket and it often requires only one memory access.
% %1次连续访存

% \ppp{Main Experimental Results:}
% In finding frequent items, compared with USS, \aname{} achieves $4.50$ times higher insertion speed and up to $9 \times 10^6$ times ($2 \times 10^4$ times in average) smaller error rate.
% % reduces the error up to $9 \times 10^6$ times ($66$ times in average) and improves the insertion throughput by $4.50$ times in average.
% %
% In finding heavy changes, \aname{} improves the F1 Score \cite{f1score} by $8$ times in average when using only $1/10$ of the memory size of other algorithms and improves the insertion speed by up to $1.9$ times. 
% %
% In finding persistent items, \aname{} achieves up to $7.5$ times higher insertion speed and up to $286$ times smaller error rate.
% % the error by up to $56$ times and improves the insertion throughput up to $7.5$ times.
% %
% In finding Super-Spreaders, \aname{} achieves up to $14$ times lower error rate. 
% %
% All related codes are open-sourced and available at Github anonymously \cite{opensource}.

% \presub
% \subsection{Contributions} \postsub
% \begin{itemize}
%     \item We propose the \aname{}, which provides unbiased and accurate estimation of items in data streams.
%     \item We theoretically prove that \aname{} achieves unbiased estimation, and show that its error is often much smaller than the state-of-the-art, USS \cite{unbiasedsketch}. 
%     \item We apply \aname{} to four applications: finding frequent items, finding heavy changes, finding persistent items, and finding Super-Spreaders.
%     \item We conduct extensive experiments, and the results show that \aname{} achieves up to two orders of magnitude smaller error than the state-of-the-art.
% \end{itemize}



==> vldb/Body/math_v0old.tex <==
\presec
\section{Mathematical Analysis} \postsec
\label{sec:math}

In this section, we provide theoretical analysis for TrustySketch.
First, we show the time complexity and space complexity of TrustySketch in Section \ref{key}, \wyh{and prove them in the following Sections \ref{bucket}-\ref{finalcon}.}
We prove the property of error-sensible buckets in Section \ref{bucket}.
After that, we analyze the filtering property in one level of TrustySketch in Section \ref{filter}.
% 4.4
Finally, we complete the prove of the time complexity and space complexity of TrustySketch in Section \ref{finalcon}.

\subsection{Key Results}
\label{key}
\begin{theorem}
The time complexity of the algorithm is O$(N)$.
\end{theorem}

\begin{theorem}
When the probability that the absolute error of all estimation is smaller than $\epsilon |F|_1$ is greater than $1-\gamma$, the space complexity of the algorithm is O$\left(\ln(\gamma)+\frac{1}{\epsilon}\right)$.
\end{theorem}

\begin{theorem}
When the probability that the absolute error of an estimation is smaller than $\epsilon |F|_1$ is greater than $1-\delta$, the space complexity of the algorithm is O$\left(\ln(\delta)+\frac{1}{\epsilon}\right)$.
\end{theorem}

\subsection{Property of Error-Sensible Buckets}
\label{bucket}
\begin{theorem}
\label{t1}
    The majority item that with a frequency more than half of $B_i[j].total$ must be the winner $B_i[j].winner$.
\end{theorem}
\begin{proof}
Consider the moments when item replacement happens.
These moments divide the timeline into several parts.
Inside each part, the winner of this part remains unchanged.
If the inserting item $e$ is equal to $B_i[j].winner$, $B_i[j].total - 2\cdot B_i[j].collision$ increases by 1.
Otherwise, $B_i[j].total - 2\cdot B_i[j].collision$ decreases by 1.
In every part except for the last part, $B_i[j].total - 2\cdot B_i[j].collision$ is initially 0 when item replacement happens, and $B_i[j].total - 2\cdot B_i[j].collision$ returns to 0 when the next replacement happens.
Therefore, $B_i[j].winner$ of the part has a frequency equals to the half of the frequency of the part.
In the last part, $B_i[j].total - 2\cdot B_i[j].collision$ is non-negative in the end.
Thus, $B_i[j].winner$ of the last part has a frequency no less than the half of the frequency of the part.
If $B_i[j].winner$ of the last part is not the majority item,
then the majority item should be no more than half in every part.
This contradicts the definition of the majority item.
Therefore, $B_i[j].winner$ of the last part must be the majority item.
\end{proof}

\begin{theorem}
\label{t2}
The frequency of the winner is at most $B_i[j].total-B_i[j].collision$ and it is at least $B_i[j].total-2\cdot B_i[j].collision$. The frequency of any item other than the winner is at most $B_i[j].collision$.
\end{theorem}

\begin{proof}
In the above proof, we divide the timeline into several parts.
In every part, the number of collisions in the part is the total frequency of any item other than the winner of the part.
Therefore, in each part, the total frequency of any item except the winner of the last part is no less than the number of collisions in the part.
Because the sum of the number of collisions in each part is $B_i[j].collision$,
we come to a conclusion that the total frequency of any item except the winner of the last part is no less than $B_i[j].collision$.
In other words, the frequency of the winner is at most $B_i[j].total - B_i[j].collision$.

Consider the last part, $B_i[j].total - 2\cdot B_i[j].collision$ is initially 0.
the inserting item $e$ is equal to $B_i[j].winner$, $B_i[j].total - 2\cdot B_i[j].collision$ increases by 1.
Therefore, the frequency of the winner is at least $B_i[j].total - 2\cdot B_i[j].collision$.

In every part except for the last part, the frequency of the winner of the part is equal to the frequency of any item other than the winner of the part.
And they all equal to the number of collisions in the part.
In the last part, the frequency of any item other than the winner is equal to the number of collisions in the last part.
Thus, for a item which is not the winner, its frequency is at most $B_i[j].collision$.

\end{proof}

\begin{theorem} 
    \label{alg:theorem:collision}
    $B_i[j].collision$ is no greater than the total frequency of all items except for the most frequent item.
\end{theorem}

\begin{proof}
If the most frequent item is the majority item, then it must be the winner.
According to the conclusions of Theorem \ref{t2}, the frequency of other items is at least $B_i[j].collision$.
Otherwise, the frequency of the most frequent item is no more than $\frac{1}{2}B_i[j].total$.
Because $B_i[j].total - 2\cdot B_i[j].collision$ is non-negative,
we have $B_i[j].collision \leqslant \frac{1}{2}B_i[j].total$.
Thus, the frequency of other items is at least $\frac{1}{2}B_i[j].total \geqslant B_i[j].collision$.

\end{proof}

\subsection{Filtering in One Level}
\label{filter}
In this section, we analyze the filtering property of TrustySketch.
Let $S^{i}=\{e_1, e_2, \dots, e_n\}$ denote all flows that enters the $i^{th}$ level.
Let $f_i(e)$ denotes the frequency of flow $e$ that enters the $i^{th}$ level. 
We divide flows into two types according to their flow sizes.
Let $F_i$ be the total frequency of all small flows in $S^{i}$, $F_i\coloneqq \sum_{e\in S^{i}\land f_i(e)\leqslant \frac{1}{2}\lambda_i}f_i(e)$,
and $C_i$ be the number of distinct large flows, $C_i\coloneqq |\{e\in S^{i}\land f_i(e)> \frac{1}{2}\lambda_i\}|$.
Let $F_{i,k}$ denote the total frequency of the small flows satisfies: \textit{i)} in set $\{e_1, e_2, \dots, e_{k-1}\}$ and \textit{ii)} map into the same bucket as $e_k$. $F_{i,k}=\sum_{l \in [1,k-1]}f_i(e_l)*[h_i(e_l)=h_i(e_k) \land f_i(e_l) \leqslant \frac{1}{2}\lambda_i]$. 
Let $C_{i,k}$ denote the number of distinct large flows map into the same bucket as $e_k$. $C_{i,k}=\sum_{l \in [1,k-1]}1*[h_i(e_l)=h_i(e_k) \land f_i(e_l) > \frac{1}{2}\lambda_i]$. 
For bucket $B_i[j]$, let $S^{i,j}_0$ denote all small flows inserted into bucket $B_i[j]$, and $S^{i,j}_1$ denote the large flows.
$ S^{i,j}_0 \coloneqq \{e_k | f_i(e_k)\leqslant \frac{1}{2}\lambda_i \land e_k\in S_i\}$, $ S^{i,j}_1 \coloneqq \{e| f_i(e)> \frac{1}{2}\lambda_i  \land e_k\in S_i\}$.
Let $f_{i,j}$ be the total frequency of the small flows, $f_{i,j}\coloneqq \sum_{e\in S^{i,j}_0}f_i(e)$, and $c_{i,j}$ be the number of distinct large flows, $c_{i,j}\coloneqq |S^{i,j}_1|$. 
Suppose $S^{i}_0=\bigcup_{j=1}^{w_i}S^{i,j}_0=\{e_{a_1}, e_{a_2}, \dots, e_{a_{n_0}}\}, a_{l}<a_{l+1}, l\in [1,n-1]$.
Suppose $S^{i}_1=\bigcup_{j=1}^{w_i}S^{i,j}_1=\{e_{b_1}, e_{b_2}, \dots, e_{b_{n_1}}\}, b_{l}<b_{l+1}, l\in [1,n-1]$.

\begin{lemma}
    
    We define that:
    \begin{align}
        &x_{i,k}=
            \begin{cases}
              0, & \text{if } c_{i, h_i(e_k)}=0\land F_{i,k}\leqslant \frac{1}{2}\lambda_i,
            \\
              f_i(e_k), & \text{if } c_{i, h_i(e_k)}=0\land F_{i,k} > \frac{1}{2}\lambda_i,
            \\
              f_i(e_k), & \text{otherwise, } c_{i, h_i(e_k)}>0.
            \end{cases}\\
        &X^{(i)}=\sum_{l=1}^{n_0} x_{i,a_l}
    \end{align}
    For any fixed $h_i()$, the $X^{(i)}$ is an upper bound of the total frequency of small flows that enters the next level:
    \begin{align}
        F_{i+1}\leqslant X^{(i)}
    \end{align}
\end{lemma}


\begin{proof}
    We consider every bucket respectively. 
    For small flows, their total frequencies that enter the next level is denoted by $f'_{i,j}\coloneqq \sum_{e\in S^{i,j}_0}f_{i+1}(e)$.
    
    Because: ......
    We have:
    \begin{align}
        f'_{i,j}\leqslant g_{i,j}=
            \begin{cases}
              0, & \text{if } c_{i,j}=0\land f_{i,j}\leqslant \lambda_i,
            \\
              f_{i,j}-\lambda_i, & \text{if } c_{i,j}=0\land f_{i,j}> \lambda_i,
            \\
              f_{i,j}, & \text{otherwise, } c_{i,j}>0.
            \end{cases}
    \end{align}
    
    Because: ..... We have:
    \begin{align*}
        % &g_{i,j} \leqslant q_{i,j}=\sum_{\forall e_k, h_i(e_k)=j} x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]\\
        &g_{i,j} \leqslant q_{i,j}=\sum_{\forall k, e_k\in S^{i,j}_0} x_{i,k}\\
        &X^{(i)}=\sum_{k=1}^n x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]\\
        &=\sum_{j=1}^{w_i}\sum_{\forall e_k, h_i(e_k)=j} x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]=\sum_{j=1}^{w_i}q_{i,j}\\
        &F_{i+1}=\sum_{j=1}^{w_i}f'_{i,j}\leqslant \sum_{j=1}^{w_i}q_{i,j}=X^{(i)}
    \end{align*}


\end{proof}


Similarly, we have the following lemma.
\begin{lemma}
%   $C_{i,j,k}=\sum_{l \in [1,k-1]}1*[h_i(e_l)=j \land f_i(e_l) > \frac{1}{2}\lambda_i]$. 
   Let 
    \begin{align}
        &y_{i,k}=
            \begin{cases}
              0, & \text{if } C_{i,k}=0\land f_{i,h_i(e_k)}\leqslant \lambda_i,
            \\
              1, & \text{if } C_{i,k}=0\land f_{i,h_i(e_k)}> \lambda_i
            \\
              2, & \text{otherwise, } C_{i,k}>0.
            \end{cases}\\
        &Y^{(i)}=\sum_{l=1}^{n_1} y_{i,b_l}
    \end{align}
    For any fixed $h_i()$, the $Y^{(i)}$ is an upper bound of the number of distinct large flows that enters the next level:
    \begin{align}
        C_{i+1}\leqslant Y^{(i)}
    \end{align}
\end{lemma}

\begin{proof}
    proof
    For large flows, the total number of distinct large flows that enter the next level is denoted by $c'_{i,j}\coloneqq |\{e| f'_i(e)>0, e\in S^{i,j}_1\}|$. We have
    \begin{align}
        c'_{i,j}\leqslant c_{i,j}
    \end{align}
        $$\sum_{j=1}^{w_i}g_{i,j}\leqslant\sum_{j=1}^{w_i}q_{i,j}= X^{(i)}$$
\end{proof}




\begin{theorem}
    Consider the $i^{th}$ level, $P_{k}=h_i(e_k)$ are independent random variables.
    \begin{align}
        & \Pr_{P_{a_l}}[x_{i,a_l}>0]\leqslant  \frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i} \forall P_{1}, P_2,\dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}
    \end{align}
    
    \begin{align}
        & \Pr_{P_{b_l}}[y_{i,b_l}>0]\leqslant  \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \forall P_{1}, P_2,\dots, P_{b_l-1},  P_{b_l+1},\dots, P_{b_{n_1}}
    \end{align}
        
\end{theorem}




\begin{theorem}
    For any $S$ satisfies:
    \begin{align}
        & \frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S}\\
        & \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S} 
    \end{align}
    We construct random variables $X'^{(i)}$, $Y'^{(i)}$:\\
    $\forall P_{1}, P_{2}, \dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}$, 
    For $P_{a_l}$ that $x_{i,a_l}>0$, let $X_l=f_i(e_{a_l})$. For random $P_{a_l}$ that $x_{i,a_l}=0$, let $X_l=f_i(e_{a_l})$ to make $\Pr[X_l=f_i(e_{a_l})]=\frac{1}{S}$. Otherwise, for other $P_{a_l}$,  $x_{i,a_l}=0$ and $X_l=0$. $\Pr[X_l=0]=1-\frac{1}{S}$.
    \begin{align}
        &X'^{(i)}=\sum_{l=1}^{n_0} X_l, X_l\leqslant f_i(e_{a_l})\\
        % &\Pr[Y_l=2]=\frac{1}{S}, \Pr[Y_l=0]=1-\frac{1}{S}\\
        &Y'^{(i)}=\sum_{l=1}^{n_1} Y_l, Y_l\leqslant 2
    \end{align}
    For given $P_{1}, P_2,\dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}$, $P_{a_l}$ decides the value of $X_l$. $X_l$ is an independent variable from $X_1,\dots, X_{l-1},X_{l+1},\dots, X_{n_0}$.\\
    $\forall\ given\ P_{...}$, $X_l\geqslant x_{i,a_l}$ and therefore $X'^{(i)}\geqslant X^{(i)}$.
    So, We have:
    \begin{align}
        &\forall t \Pr[X'^{(i)}>t] \geqslant \Pr[X^{(i)}>t]\\
        &\forall t \Pr[Y'^{(i)}>t] \geqslant \Pr[Y^{(i)}>t] 
    \end{align}
        
\end{theorem}

    
    % \begin{align}
    %     &\Pr[X_l=f_i(e_{a_l})]=\frac{1}{S}, \Pr[X_l=0]=1-\frac{1}{S}\\
    %     &\forall t \Pr[X_l>t]\geqslant \Pr[x_{i,a_l}>t]\\
    %     &X'^{(i)}=\sum_{l=1}^{n_0} X_l, X_l\leqslant f_i(e_{a_l})\\
    %     &\forall t \Pr[X'^{(i)}>t] \geqslant \Pr[X^{(i)}>t]\\
    %     & \Pr_{P_{b_l}}[y_{i,b_l}>0]\leqslant  \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S} \forall P_{1}, P_2,\dots, P_{b_l-1},  P_{b_l+1},\dots, P_{b_{n_1}}\\
    %     &\Pr[Y_l=2]=\frac{1}{S}, \Pr[Y_l=0]=1-\frac{1}{S}\\
    %     &\forall t \Pr[Y_l>t]\geqslant \Pr[y_{i,b_l}>t]\\
    %     &Y'^{(i)}=\sum_{l=1}^{n_1} Y_l, Y_l\leqslant 2\\
    %     &\forall t \Pr[Y'^{(i)}>t] \geqslant \Pr[Y^{(i)}>t] 
    % \end{align}


\begin{lemma}
\label{basic}
Let $X_1,\dots, X_n$ be a set of $n$ independent random variables satisfying $Pr(X_i=s_i(0\leqslant s_i \leqslant 1) )=p$, $Pr(X_i=0)=1-p$, $\frac{1}{n}\sum_{i=1}^n s_i=m$, $\mu=E[X=\sum_{i=1}^n x_i]=nmp$.
\begin{equation}
    Pr[X>(1+\delta)\mu] \leqslant e^{-(\delta-0.75)nmp}
\end{equation}
\end{lemma}
\begin{proof}
For any $t > 0$, Using the Markov inequality:
$$\Pr[X>(1+\delta)\mu] = \Pr[e^{tX}>e^{t(1+\delta)\mu}] \leqslant \frac{E[e^{tX}]}{e^{t(1+\delta)\mu}}$$
Note that $X_1,\dots, X_n$ are independent, 
$$E[e^{tX}]=\prod_{i=1}^n{E[e^{t X_i}]}=\prod_{i=1}^n\left (e^{t s_i}-1\right )p+1$$
Because $1+x < e ^x$, we have:
$$E[e^{tX}]\leqslant\prod_{i=1}^n e^{\left(e^{t s_i}-1\right) p}$$
Noticed that when $t\leqslant 1$, $x = t s_i\leqslant 1$, $e^x \leqslant 1 + 1.75x$, therefore:
$$E[e^{tX}]\leqslant\prod_{i=1}^n e^{\left(e^{t s_i}-1\right) p}\leqslant e^{\sum_{i=1}^n 1.75 t s_i p} = e^{1.75mnpt}$$
Thus, let $t = 1$:
$$Pr[X>(1+\delta)\mu] \leqslant \frac{e^{1.75nmp}}{e^{(1+\delta)nmp}}=e^{-(\delta-0.75)nmp}$$

\end{proof}

\begin{comment}
\begin{theorem}
Hoeffding's inequality: Let $X_1,\cdots, X_n$ be independent random variables, $X_i$ are strictly bounded by interval $[a_i, b_i]$. Let $S_n$ be the sum of the random variables:
\begin{align}
    & \Pr\left[ S_n - E[S_n]\geqslant t\right]\leqslant \exp\left( -\frac{2t^2}{\sum_{i=1}^n(b_i-a_i)^2}\right)
\end{align}
\end{theorem}
\end{comment}

We set $w_i=\lceil\frac{W (R_{w}-1)}{R_{w}^i}\rceil$, and $\lambda_i= \frac{\Lambda (R_\lambda-1)}{R_\lambda^i} = \frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i}$.
therefore, $w_i$ satisfy $\sum_{i=1}^d w_i \leqslant W+d$, and $\lambda_i$ satisfy $\sum \lambda_i\leqslant \Lambda$.

Let $ R=R_w R_\lambda$, 
$\alpha_i= \frac{\Vert F\Vert_1}{R^{i-1}}$, 
$\beta_i= \frac{2 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)}$,
we have:
$$\frac{\alpha_i}{max(1, \frac{1}{2}\lambda_i)}\leqslant \frac{2 \alpha_i}{\lambda_i}=  \frac{2 \frac{\Vert F\Vert_1}{(R_{w}R_{\lambda})^{i-1}} R_\lambda^i}{ \epsilon \Vert F\Vert_1 (R_\lambda-1)} = \frac{2 R_\lambda}{\epsilon R_{w}^{i-1}(R_\lambda-1)}=\beta_i$$

Let $D_i$ be the number of flows whose flow size is in $(\frac{1}{2}\lambda_{i+1}, \frac{1}{2}\lambda_{i}]$, and these flows enters $i+1$ level.
$D_i\leqslant F_{i+1}/max(1,\frac{1}{2}\lambda_{i+1})$
Let $E_i$ be the number flows whose flow size is greater than $\frac{1}{2}\lambda_{i}$, and these flows enters $i+1$ level.
$C_{i+1}=D_{i}+E_{i}$. 

\begin{comment}
\begin{theorem}
    When $T_i=\alpha_i$, and $U_i=\beta_i$, 
    \begin{align}
         &\text{From :}\frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i}
         \leqslant \frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i} \leqslant \frac{2 U_i}{w_i}\leqslant\frac{1}{S} \\
        &\text{We have :} \\
        &\Pr[F_{i+1}>\frac{(1+\delta)}{S}T_i] \leqslant
        \Pr[X^{(i)}>\frac{(1+\delta)}{S}T_i]\leqslant e^{(0.75-\delta)\frac{1}{S}\frac{T_i}{\frac{1}{2}\lambda_i}}\\
        & \Pr[C_{i+1}>\frac{(1+\delta)}{S}U_i] \leqslant
        \Pr[Y^{(i)}>\frac{(1+\delta)}{S} U_i ]\leqslant e^{(0.75-\delta)\frac{1}{S}\frac{U_i}{2}}
    \end{align}
    \label{math:smallprob}
\end{theorem}
\end{comment}

\begin{theorem}
\label{math:smallprob}
When $T_i=\alpha_i, U_i=\beta_i$,
if $\frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i} \leqslant \frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i} \leqslant \frac{2 U_i}{w_i}\leqslant\frac{1}{S_i}$, 
then we have:
\begin{equation}
    \Pr[F_{i+1}>\frac{(1+\delta)}{S_i}T_i] \leqslant
        \exp\left(-\frac{2(\delta - 0.75)F_i}{\lambda_i S_i}\right)
\end{equation}

\begin{equation}
    \Pr[E_i > \frac{(1+\delta)}{S_i}U_i]
    \leqslant \exp\left( -\frac{(\delta - 0.75)U_i}{2S_i}\right)
\end{equation}

\end{theorem}
\begin{proof}
Using Lemma \ref{basic}.
\end{proof}


\begin{theorem}
When $T_i=\frac{\alpha_i}{\gamma_i}$, $U_i=\frac{\beta_i}{\gamma_i}$, $S_i=S_0 \gamma_i$.
Let $W=\frac{4 S_0 R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) } $.
Then we have:
\begin{equation}
\frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i}\leqslant\frac{1}{S_i}=\frac{1}{S_0\gamma_i}    
\end{equation}
\end{theorem}

\begin{proof}
Noticed that $\frac{\alpha_i}{max(1, \frac{1}{2}\lambda_i)}\leqslant \beta_i$, therefore:
$$\frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i} = \frac{\frac{\alpha_i}{\gamma_i}}{\frac{1}{2}\lambda_i w_i} + \frac{\frac{\beta_i}{\gamma_i}}{w_i}
\leqslant \frac{2\frac{\beta_i}{\gamma_i}}{w_i} = \frac{2\frac{\beta_i}{\gamma_i}}{\frac{W (R_{w}-1)}{R_{w}^i}} = \frac{1}{S_0\gamma_i}$$
\end{proof}

\begin{theorem}
Suppose $\gamma_i=R^{a_i}$, $S_0=R^k$, $T_i = \frac{\alpha_i}{\gamma_i}$, $U_i = \frac{\beta_i}{\gamma_i}$, then $S = S_0\gamma_i = R^{k+a_i}$. If $a_i$ and $k$ satisfy $a_i + k = 2^{i-1}(k-2) + 2\ (k\geqslant2)$, and $R\geqslant 2(1+\delta)$, then we have
\begin{equation}
    T_{i}\frac{1+\delta}{S}\leqslant \frac{1}{2}T_{i+1}
\end{equation}
\end{theorem}

\begin{proof}
$$T_i\frac{1+\delta}{S} = \frac{\Vert F\Vert_1}{R^{i-1+a_i}}\frac{1+\delta}{R^{a_i+k}}$$
Because $R\geqslant 2(1+\delta)$, we have
$$T_i\frac{1+\delta}{S}\leqslant \frac{\Vert F\Vert_1}{2R^{2a_i + k + i - 2}}$$
Note that $2a_i + k - 2 = a_{i+1}$, we can write as:
$$T_i\frac{1+\delta}{S}\leqslant \frac{\Vert F\Vert_1}{2R^{a_{i+1} + i }} = \frac{1}{2}T_{i+1}$$
\end{proof}

\begin{theorem}
\label{next}
Suppose $\gamma_i=R^{a_i}$, $S_0=R^k$, $T_i = \frac{\alpha_i}{\gamma_i}$, $U_i = \frac{\beta_i}{\gamma_i}$, $a_i$ and $k$ satisfy $a_i + k = 2^{i-1}(k-2) + 2\ (k\geqslant2)$, and $R\geqslant 2(1+\delta)$, $F_{i+1}\leqslant \frac{1+\delta}{S_i}T_{i}$, $E_{i}\leqslant \frac{1+\delta}{S_i}U_{i}$, then we have
\begin{align}
    &F_{i+1}\leqslant \frac{1+\delta}{S_i}T_{i}
     \leqslant \frac{1}{2}T_{i+1}\leqslant T_{i+1}\\
    &D_{i}\leqslant \frac{F_{i+1}}{max(1,\frac{1}{2}\lambda_{i+1})}
    \leqslant \frac{\frac{1}{2}T_{i+1}}{\frac{1}{2}\lambda_{i+1}}
    \leqslant \frac{1}{2}U_{i+1}\\
    &E_{i}\leqslant \frac{1+\delta}{S_i}U_{i}\leqslant \frac{1}{2 R_\lambda} U_{i+1}\leqslant \frac{1}{2} U_{i+1}\\
    &C_{i+1}=E_i+D_i\leqslant U_{i+1}
\end{align}
\end{theorem}

Theorem \ref{math:smallprob} prove that $F_{i+1} \leqslant \frac{(1+\delta)}{S_i}T_i$ and $E_{i} \leqslant \frac{(1+\delta)}{S_i}U_i$ are high probability events.
If one of these events does not happen, we consider it to be a failure in level i.
Theorem \ref{next} show that if the above events happen, the restriction of the next level $F_{i+1}\leqslant T_{i+1}$ and $C_{i+1}\leqslant U_{i+1}$ holds.
Thus, we can apply the theorems on next level.

\subsection{Time and Space Complexity}
\label{finalcon}
\begin{theorem}
The time complexity of the algorithm is O$(N)$.
\end{theorem}
\begin{proof}
In Section \ref{filter}, we prove that every flow entering level i passes through level i with a probability not exceeding $\frac{1}{S_i}$.
Therefore, the time complexity of the algorithm is
$$N\left (1 + \frac{1}{S_1} + \frac{1}{S_1S_2} + \dots + \frac{1}{S_1S_2\dots S_d}\right) = O(N)$$
\end{proof}

\begin{theorem}
When the probability that the absolute error of all estimation is smaller than $\epsilon |F|_1$ is greater than $1-\gamma$, the space complexity of the algorithm is O$\left(\ln(\gamma)+\frac{1}{\epsilon}\right)$.
\end{theorem}
\begin{proof}
Noticed that if every level does not fail, the absolute error of all estimation is smaller than $\epsilon |F|_1$. Thus, we need:
$$\Pr[\exists i,\ s.t.\ level\ i\ fails]\leqslant\gamma$$
Using union bound, we need:
$$\Pr[\exists i,\ s.t.\ level\ i\ fails]\leqslant \sum_{i=1}^d\Pr[level\ i\ fails]\leqslant\gamma$$
Noticed that the probability that level i fails increases when i becomes larger, thus, we need:
$$\sum_{i=1}^d\Pr[level\ i\ fails]\leqslant d\Pr[level\ d\ fails]\leqslant \gamma$$
We can write:
$$d\left( \exp\left(-\frac{2(\delta - 0.75)F_d}{\lambda_d S_d}\right) + \exp\left( -\frac{(\delta - 0.75)U_d}{2S_d}\right) \right)\leqslant \gamma$$
Note that in the above inequality, $\frac{F_d}{S_d}$ and $\frac{U_d}{S_d}$ should be $O\left(\ln (\gamma)\right)$.
Therefore, the total frequencies of the flows passing through level $d$ is $O\left(\ln (\gamma)\right)$.
Thus, the size of the SpaceSaving structure is $O\left(\ln (\gamma)\right)$.
Integrating the size of all levels and the SpaceSaving structure, the space complexity of the algorithm is O$\left(\ln(\gamma)+W\right) = $ O$\left(\ln(\gamma)+\frac{1}{\epsilon}\right)$.
\end{proof}

\begin{theorem}
When the probability that the absolute error of an estimation is smaller than $\epsilon |F|_1$ is greater than $1-\delta$, the space complexity of the algorithm is O$\left(\ln(\delta)+\frac{1}{\epsilon}\right)$.
\end{theorem}
\begin{proof}
Noticed that if the absolute error of all estimation is smaller than $\epsilon |F|_1$ is greater than $1-\delta$, then we have the probability that the absolute error of an estimation is smaller than $\epsilon |F|_1$ is greater than $1-\delta$.
\end{proof}



%\input{vldb/Math/newmath}

% In this section, we provide a theoretical analysis for \aname{}.
% % Due to space limitation, we show the variance and the error bound of \aname{} in Appendix \ref{subsec:math:error}, and how the parameter of \aname{} influences its performance in Appendix \ref{subsec:math:para}.
% First, we prove that \aname{} outputs an upper bound and a lower bound of the frequency in Section \ref{subsec:math:cuoverestimation}.
% Then, we demonstrate the certainty for dominant items in Section \ref{subsec:math:dominant}.
% After that, we show the error bound of \aname{} in Section \ref{subsec:math:expectationerror}.
% % Finally, we show the probability of \aname{} to output an error-free estimation in Section \ref{subsec:math:errorfree}.
% %First, we prove that our algorithm can provide an unbiased estimated frequency in Section \ref{subsec:math:unbiased}.
% %Then, we show the variance and the error bound of \aname{} in Section \ref{subsec:math:error}.
% %Due to space limitation, we show how the parameter of \aname{} influences its performance in Appendix \ref{subsec:appen:para}.

% % \input{vldb/Math/unbiased.tex}
% \input{vldb/Math/overestimation.tex}
% \input{vldb/Math/zipf}
% \input{vldb/Math/expectationerror.tex}
% % \input{vldb/Math/errorfree.tex}
% %\input{vldb/Math/para.tex}



==> vldb/Body/math_v1zyk.tex <==
\presec
\section{Mathematical Analysis} \postsec
\label{sec:math}

\vspace{0.2cm}

% In this section, we drive the error bounds, the time complexity, and the space complexity of the algorithm.

\subsection{Key Results}
\label{key}

The key results of this section is to prove the following two claims. 



\ppp{Claim 1:}
%
The algorithm can achieve the following two properties by using $O\left(\frac{1}{\epsilon}+\ln(\frac{1}{\delta})\right)$  space:

%
\begin{align*}
    \Pr\left(\forall \textit{ item } e, \left|\hat{f}(e)-f(e)\right|\leqslant\varepsilon\Vert F\Vert_1\right)\geqslant 1-\delta
\end{align*}
and 
\begin{align*}
    \forall \textit{ item } e, \Pr\left(\left|\hat{f}(e)-f(e)\right|\leqslant\varepsilon\Vert F\Vert_1\right)\geqslant 1-\delta
\end{align*}

\ppp{Claim 2:}
%
The algorithm can achieve the above two properties with $O\left(N+\delta\ln\ln(\frac{1}{\varepsilon})N\right)$ time complexity.

\subsection{Preliminaries}
\postsub

\pretheo\begin{lemma}
\label{basic}
Let $X_1,\dots, X_n$ be $n$ random variables such that
\begin{align*}
    X_i\in\{0,s_i\}, &&
    \Pr(X_i=s_i~|~X_1,\cdots,X_{i-1})\leqslant p,
\end{align*}
where $0\leqslant s_i \leqslant 1$.
%
Let $X=\sum_{i=1}^n X_i$, and $\mu=\sum_{i=1}^n ps_i=nmp$.
\begin{align*}
    Pr\left(X>(1+\delta)\mu\right) \leqslant e^{-(\delta-(e-2))nmp}
\end{align*}
\end{lemma}\posttheo

\preprof\begin{proof}
For any $t > 0$, by using the Markov inequality we have
%
\begin{align*}
    \Pr(X>(1+\delta)\mu) 
    =
    \Pr(e^{X}>e^{(1+\delta)\mu}) 
    \leqslant
    \frac{E(e^{X})}{e^{(1+\delta)\mu}}.
\end{align*}
%
According to the conditions, we have
%
\begin{align*}
    &
    E(e^{X}) 
    = 
    E\left(E(e^{\sum_{i=1}^n{X_i}}~|~X_1,\cdots,X_{n-1})\right)
    \\
    =&
    E\left(
    \begin{aligned}
    e^{\sum_{i=1}^{n-1}{X_i}}
    \cdot \Pr(X_n=0~|~X_1,\cdots,X_{n-1})
    \\+
    e^{s_n+\sum_{i=1}^{n-1}{X_i}}
    \cdot \Pr(X_n=s_n~|~X_1,\cdots,X_{n-1})
    \end{aligned}
    \right)
    \\
    \leqslant&
    E\left(
    e^{\sum_{i=1}^{n-1}{X_i}}
    \right)
    \cdot
    \left(1+p\left(e^{s_n}-1\right)\right)
    \leqslant
    \cdots
    \leqslant 
    \prod_{i=1}^n  \left(1+p\left(e^{s_i}-1\right)\right)
\end{align*}
%
Because of $1+x < e ^x$, we have
\begin{align*}
    E(e^{X})
    \leqslant
    \prod_{i=1}^n e^{p\left(e^{s_i}-1\right)}.
\end{align*}
%
Since for $s_i\leqslant 1$, there is $e^{s_i}-1 \leqslant (e-1)s_i$, so there is
\begin{align*}
    E(e^{X})
    \leqslant
    e^{\sum_{i=1}^n p(e-1) s_i} = e^{(e-1)mnp}.
\end{align*}
That is
\begin{align*}
    Pr(X>(1+\delta)\mu)
    \leqslant
    \frac{e^{(e-1)nmp}}{e^{(1+\delta)nmp}}
    =
    e^{-(\delta-(e-2))nmp}
\end{align*}

\end{proof}\postprof

\vspace{-0.4cm}

\presub
\subsection{Definition of Symbols}
\postsub

\begin{enumerate}[leftmargin=*]
    \item $\mathcal{S}_{i}$: $\{e_1,\cdots,e_{N_i}\}$, the set of items entering the $i$-th layer, where $N_i=|\mathcal{S}_i|$.

    \item $f_i(e)$: the number of times that item $e$ enters the $i$-th layer.
    
    \vspace{0.2cm}
    
    \item $\mathcal{S}^{0}_{i}$: $\{e~|~e\in\mathcal{S}_i\land \forall i'\leqslant i, f_{i'}(e)\leqslant \frac{\lambda_{i'}}{2}\}$, the set of small items.
    
    \item $\mathcal{S}^{1}_{i}$:  $\{e~|~e\in\mathcal{S}_i\land \exists i'\leqslant i, f_{i'}(e) > \frac{\lambda_{i'}}{2}\}$, the set of large items.
    
    \item $F_i$: $\sum_{\{e\in\mathcal{S}^{0}_i\}} f_i(e)$, the total frequency of small items in $\mathcal{S}^{0}_{i}$.
    
    \item $C_i$: $|\mathcal{S}^{1}_i|$, the number of large items in $\mathcal{S}^{1}_{i}$.
    
    \vspace{0.2cm}
    
    \item $\mathcal{S}^{0}_{i,j}$: $\{e~|~e\in\mathcal{S}^{0}_{i}\land h(e)=j\}$, the set of small items that are mapped to the $j$-th bucket.
    
    \item $\mathcal{S}^{1}_{i,j}$: $\{e~|~e\in\mathcal{S}^{1}_{i}\land h(e)=j\}$, the set of large items that are mapped to the $j$-th bucket.
    
    \item $F_{i,j}$: $\sum_{\{e\in\mathcal{S}^{0}_{i,j}\}} f_i(e)$, the total frequency of small items in $\mathcal{S}^{0}_{i,j}$.
    
    \item $C_{i,j}$: $|\mathcal{S}^{1}_{i,j}|$, the number of large items in $\mathcal{S}^{1}_{i,j}$.
    
    \vspace{0.2cm}
        
    \item $\mathcal{P}_{i,k}$: $\{e_1,\cdots,e_{k}\}$, a subset of $\mathcal{S}_i$ composed of the first $k$ items.
    
    \item $f^{P}_{i,k}$: $\sum_{\{e\in\mathcal{P}_{i,k-1}\cap\mathcal{S}^{0}_{i,h(e_k)}\}} f_i(e)$, the total frequency of small items with a smaller index that conflicts with item $e_k$.
    
    \item $c^{P}_{i,k}$: $\left|\{e~|~e\in\mathcal{P}_{i,k-1}\cap\mathcal{S}^{1}_{i,h(e_k)}\}\right|$, the number of large items with a smaller index that conflicts with item $e_k$.
\end{enumerate}


\subsection{Properties in One Layer}
\label{filter}


This section aims to prove that only a small proportion of the items inserted into the $i$-th layer will be inserted into the (i+1)-th layer.
% In this section, we analyze the filtering property of TrustySketch.


\pretheo\begin{lemma}
\label{lem:x}    
    Let
    \begin{align*}
        X_{i,k}=
            \begin{cases}
              0 & C_{i, h(e_k)}=0 \land f^{P}_{i,k}\leqslant \frac{\lambda_i}{2}
            \\
              f_i(e_k) &  C_{i, h(e_k)}=0\land f^{P}_{i,k} > \frac{\lambda_i}{2}
            \\
              f_i(e_k) & C_{i, h(e_k)}>0
            \end{cases},
        &&
        X_i=\sum_{\{e_k\in\mathcal{S}^{0}_{i}\}} X_{i,k}.
    \end{align*}
    The total frequency of the small items in the $i$-th layer entering the $(i+1)$-th layer does not exceed $X_i$, \ie,
    \begin{align*}
        F_{i+1}
        \leqslant
        \sum_{\{e\in\mathcal{S}^{0}_i\cap\mathcal{S}_{i+1}\}} f_{i+1}(e) \leqslant X_{i}.
    \end{align*}
\end{lemma}\posttheo


\preprof\begin{proof}
    For the small items in the $j$-th bucket of the $i$-th layer, let the number of times they enter the $(i+1)$-th layer be
    $F'_{i,j}=\sum_{\{e\in\mathcal{S}^{0}_{i,j}\cap\mathcal{S}^{0}_{i+1}\}} f_{i+1}(e).$
    %
    Since a bucket can hold at least $\lambda_i$ occurrences of the item, we have:
    \begin{align*}
    \begin{cases}
        F'_{i,j}=0 & C_{i,j}=0 \land F_{i,j} \leqslant \lambda_i
        \\
        F'_{i,j}\leqslant F_{i,j}-\lambda_i & C_{i,j}=0 \land F_{i,j} > \lambda_i
        \\
        F'_{i,j}\leqslant F_{i,j} & C_{i,j}>0
    \end{cases}.
    \end{align*}
    %
    When $C_{i,j}=0 \land F_{i,j} > \lambda_i$, exists $k'$ satisfies
    \begin{align*}
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k< k'\}} f_{i}(e_k)
        \leqslant \frac{\lambda_i}{2}
        \leqslant
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k\leqslant k'\}} f_{i}(e_k)
        \leqslant \lambda_i.
    \end{align*}
    Then for and only for any $e_k\in\mathcal{S}^{0}_{i,j}\land k\leqslant k'$, there is $X_{i,k}=0$, and
    \begin{align*}
        F'_{i,j}
        &\leqslant
        \left(
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k\leqslant k'\}} f_{i}(e_k)
        +
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k> k'\}} f_{i}(e_k)
        \right)
        -
        \lambda_i
        \\
        &\leqslant
        0 + \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k> k'\}} f_{i}(e_k)
        \\
        &\leqslant
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k\leqslant k'\}} X_{i, k}
        +
        \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\land k> k'\}} X_{i,k}.
    \end{align*}
    %
    Then we have $F'_{i,j}\leqslant \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\}} X_{i,k}$, and
    \begin{align*}
        \sum_{\{e\in\mathcal{S}^{0}_i\cap\mathcal{S}_{i+1}\}} f_{i+1}(e)
        =
        \sum_{j=1}^{w_i} F'_{i,j}
        \leqslant
        \sum_{j=1}^{w_i} \sum_{\{e_k\in\mathcal{S}^{0}_{i,j}\}} X_{i,k}
        =
        X_{i}.
    \end{align*}


\end{proof}\postprof

\vspace{-0.3cm}


Similarly, we have the following lemma.
\pretheo\begin{lemma}
\label{lem:y}
   Let 
    \begin{align*}
        &Y_{i,k}=
            \begin{cases}
              0 &  c^{P}_{i,k}=0\land F_{i,h(e_k)}\leqslant \lambda_i,
            \\
              2 & c^{P}_{i,k}=0\land F_{i,h(e_k)}> \lambda_i
            \\
              2 & c^{P}_{i,k}>0.
            \end{cases},
        &&
        Y_{i}=\sum_{e_k\in\mathcal{S}^{1}_{i}} Y_{i,k}.
    \end{align*}
    The number of distinct large items in the $i$-th layer entering the $i$-th layer does not exceed $Y_i$, \ie,
    \begin{align*}
        \left|\mathcal{S}^{1}_{i}\cap\mathcal{S}^{1}_{i+1}\right|\leqslant Y_{i}.
    \end{align*}
\end{lemma}\posttheo

\preprof\begin{proof}
    For the large items in the $j$-th bucket of the $i$-th layer, 
    $\sum_{\{e_k\in\mathcal{S}^{1}_{i,j}\}} Y_{i,k}<C_{i,j}$
    if and only if
    $C_{i,j}=1\land F_{i,j}\leqslant \lambda_i$.
    %
    In this case, the number of collisions in the bucket does not exceed $\lambda_i$, and no item enters the $(i+1)$-th layer.
    %
    Thus we have $|\mathcal{S}^{1}_{i,j}\cap\mathcal{S}^{1}_{i+1}|\leqslant \sum_{\{e_k\in\mathcal{S}^{1}_{i,j}\}} Y_{i,j}$, and
    \begin{align*}
        \left|\mathcal{S}^{1}_{i}\cap\mathcal{S}^{1}_{i+1}\right|
        =
        \sum_{j=1}^{w_i} |\mathcal{S}^{1}_{i,j}\cap\mathcal{S}^{1}_{i+1}|
        \leqslant
        \sum_{j=1}^{w_i} \sum_{\{e_k\in\mathcal{S}^{1}_{i,j}\}} Y_{i,j}
        =
        Y_{i}.
    \end{align*}
\end{proof}\postprof

\vspace{-0.2cm}

\pretheo\begin{theorem}
    For the $i$-th layer, the following inequalities hold.
    \begin{align*}
        \Pr\left(X_{i,k}>0~|~X_{i,1},\cdots,X_{i,k-1}\right)
        \leqslant
        \frac{2F_i}{\lambda_i w_i}+ \frac{C_i}{w_i},
        && \forall e_k\in\mathcal{S}^{0}_{i}.
        \\
        \Pr\left(Y_{i,k}>0~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
        \leqslant 
        \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i},
        && \forall e_k\in\mathcal{S}^{1}_{i}.
    \end{align*}
\label{theo:markov}
\end{theorem}\posttheo

\preprof\begin{proof}
By using Markov's inequality, we have
\begin{align*}
    &
    \Pr\left(X_{i,k}>0~|~X_{i,1},\cdots,X_{i,k-1}\right)
    \\
    =&
    \Pr\left(\left(C_{i, h(e_k)}=0\land f^{P}_{i,k} > \frac{\lambda_i}{2}\right)\lor C_{i, h(e_k)}>0~|~X_{i,1},\cdots,X_{i,k-1}\right)
    \\
    \leqslant&
    \begin{aligned}
    \Pr\left(C_{i, h(e_k)}>0~|~X_{i,1},\cdots,X_{i,k-1}\right)
    \\+\quad
    \Pr\left(F_{i,h(e_k)} - f_i(e_k)> \frac{\lambda_i}{2}~|~X_{i,1},\cdots,X_{i,k-1}\right)
    \end{aligned}
    \\
    \leqslant&
    \frac{E(C_{i, h(e_k)}~|~X_{i,1},\cdots,X_{i,k-1})}{1}+\frac{E(F_{i,h(e_k)}-f_i(e_k)~|~X_{i,1},\cdots,X_{i,k-1})}{\frac{\lambda_i}{2}}
    \\
    \leqslant&
    \frac{C_i}{w_i} + \frac{2F_i}{\lambda_i w_i}
\end{align*}
\begin{align*}
    &
    \Pr\left(Y_{i,k}>0~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
    \\
    =&
    \Pr\left(\left(c^{P}_{i,k}=0\land F_{i,h(e_k)}> \lambda_i\right)\lor c^{P}_{i,k}>0~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
    \\
    \leqslant&
    \begin{aligned}
    \Pr\left(C_{i, h(e_k)}-1>0~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
    \\+\quad
    \Pr\left(F_{i,h(e_k)} > \lambda_i~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
    \end{aligned}
    \\
    \leqslant&
    \frac{E(C_{i, h(e_k)}-1~|~Y_{i,1},\cdots,Y_{i,k-1})}{1}+\frac{E(F_{i,h(e_k)}~|~Y_{i,1},\cdots,Y_{i,k-1})}{\lambda_i}
    \\
    \leqslant&
    \frac{C_i}{w_i} + \frac{F_i}{\lambda_i w_i}.
\end{align*}
\end{proof}\postprof




\pretheo\begin{theorem}
\label{theo:exp_1}
Let
$W=\frac{4(R_wR_\lambda)^{6}}{\varepsilon(R_w-1)(R_\lambda-1)}$,
$\alpha_i= \frac{\Vert F\Vert_1}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
%
Under the conditions of
    $F_i\leqslant\frac{\alpha_i}{\gamma_i}$ and
    $C_i\leqslant\frac{\beta_i}{\gamma_i}$,
we have
\begin{align*}
    \Pr\left(X_{i}>(1+\delta)\frac{p_i\alpha_i}{\gamma_i}\right)
    \leqslant
    \exp\left(-(\delta-(e-2))\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
\end{align*}
and
\begin{align*}
    \Pr\left(Y_{i}>(1+\delta)\frac{3}{2}\frac{p_i\beta_i}{\gamma_i}\right)
    \leqslant
    \exp\left(-(\delta-(e-2))\frac{3p_i\beta_i}{4\gamma_i}\right).
\end{align*}
\end{theorem}\posttheo

\preprof\begin{proof}
Recall that
%
$w_i=\lceil\frac{W (R_{w}-1)}{R_{w}^i}\rceil$ and
$\lambda_i = \frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i}$
,
according to Theorem \ref{theo:markov},
\begin{align*}
    &
    \Pr\left(
    \frac{X_{i,k}}{\frac{\lambda_i}{2}}=\frac{f_i(e_k)}{\frac{\lambda_i}{2}}
    ~|~
    \frac{X_{i,1}}{\frac{\lambda_i}{2}},\cdots,\frac{X_{i,k-1}}{\frac{\lambda_i}{2}}
    \right)
    \\
    \leqslant&
    \frac{\beta_i}{\gamma_i w_i} + \frac{2\alpha_i}{\gamma_i \lambda_i w_i}
    =
    \frac{4\alpha_i}{\gamma_i \lambda_i w_i}
    \leqslant
    \frac{1}{(R_wR_\lambda)^{2^{i-1}+4}}=p_i.
    \\
    &
    \Pr\left(\frac{Y_{i,k}}{2}=1
    ~|~
    \frac{Y_{i,1}}{2}, \cdots, \frac{Y_{i,k-1}}{2}
    \right)
    \\
    \leqslant&
    \frac{\beta_i}{\gamma_i w_i} + \frac{\alpha_i}{\gamma_i \lambda_i w_i}
    =
    \frac{3\alpha_i}{\gamma_i \lambda_i w_i}
    \leqslant
    \frac{3}{4(R_wR_\lambda)^{2^{i-1}+4}}\leqslant \frac{3}{4}p_i.
\end{align*}
According to Lemma \ref{basic},
\begin{align*}
    &
    \Pr\left(
    X_i>(1+\delta)\frac{p_i\alpha_i}{\gamma_i}
    \right)
    \leqslant
    \Pr\left(
    X_i>(1+\delta)p_iF_i
    ~|~F_i=\frac{\alpha_i}{\gamma_i}
    \right)
    \\
    =&
    \Pr\left(
    \sum_{\{e_k\in\mathcal{S}^{0}_{i}\}} \frac{X_{i,k}}{\frac{\lambda_i}{2}}>(1+\delta)p_i\sum_{\{e_k\in\mathcal{S}^{0}_{i}\}}\frac{f_i(e_k)}{\frac{\lambda_i}{2}}
    ~|~F_i=\frac{\alpha_i}{\gamma_i}
    \right)
    \\
    \leqslant&
    \exp\left(-(\delta-(e-2))\frac{\alpha_i}{\gamma_i\frac{\lambda_i}{2}}p_i\right)
    =
    \exp\left(-(\delta-(e-2))\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
    \\
    &
    \Pr\left(
    Y_i>(1+\delta)\frac{3}{2}\frac{p_i\beta_i}{\gamma_i}
    \right)
    \leqslant
    \Pr\left(
    Y_i>(1+\delta)\frac{3}{2}p_iC_i
    ~|~ C_i=\frac{\beta_i}{\gamma_i}
    \right)
    \\
    =&
    \Pr\left(
    \sum_{\{e_k\in\mathcal{S}^{1}_{i}\}} \frac{Y_{i,k}}{2}>(1+\delta)\frac{3}{4} p_i\sum_{\{e_k\in\mathcal{S}^{1}_{i}\}}\frac{2}{2}
    ~|~ C_i=\frac{\beta_i}{\gamma_i}
    \right)
    \\
    \leqslant&
    \exp\left(-(\delta-(e-2))\frac{\beta_i}{\gamma_i}\frac{3}{4}p_i\right)
    =
    \exp\left(-(\delta-(e-2))\frac{3p_i\beta_i}{4\gamma_i}\right).
\end{align*}

\end{proof}\postprof

\pretheo\begin{theorem}
\label{theo:gamma}
Let
$R_wR_\lambda\geqslant2$,
$W=\frac{4(R_wR_\lambda)^{6}}{\varepsilon(R_w-1)(R_\lambda-1)}$,
$\alpha_i= \frac{\Vert F\Vert_1}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
%
We have
%
\begin{align*}
&    
    \Pr\left(F_{i+1}>\frac{\alpha_{i+1}}{\gamma_{i+1}}
    ~|~
    F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)
    \leqslant
    \exp\left(-(9-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
    \\
&
    \Pr\left(C_{i+1}>\frac{\beta_{i+1}}{\gamma_{i+1}}
    ~|~
    F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land
    C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)
    \\
    \leqslant&
    \exp\left(-(5-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right)
    +
    \exp\left(-(\frac{11}{3}-e)\frac{3p_i\beta_i}{4\gamma_i}\right).
\end{align*}
\end{theorem}\posttheo

\preprof\begin{proof}
According to settings, we have
\begin{align*}
    p_i\frac{\alpha_i}{\gamma_i}
    &=
    \frac{\Vert F\Vert_1}{(R_wR_\lambda)^{(2^{i}+i+2)}}
    \leqslant
    \frac{1}{8}\frac{\alpha_{i+1}}{\gamma_{i+1}}
    \\
    p_i\frac{\beta_i}{\gamma_i}
    &=
    p_i\frac{\alpha_i}{\gamma_i\frac{\lambda_i}{2}}
    \leqslant
    \frac{1}{8}\frac{\alpha_{i+1}}{\gamma_{i+1}\frac{\lambda_{i+1}}{2}}
    =
    \frac{1}{8}\frac{\beta_{i+1}}{\gamma_{i+1}}.
\end{align*}
%
Recall that $C_{i+1}=|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{0}_i|+|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{1}_i|$, and
\begin{align*}
|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{0}_i|
\leqslant
\frac{\sum_{\{e\in\mathcal{S}^{0}_i\cap\mathcal{S}_{i+1}\}} f_i(e)}{\frac{\lambda_{i+1}}{2}}
\leqslant
\frac{X_i}{\frac{\lambda_{i+1}}{2}}
\end{align*}
%
Let $\Gamma_i=\left(F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land
    C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)$, according to Lemma \ref{lem:x} and Theorem \ref{theo:exp_1}, 
\begin{align*}
    \Pr(F_{i+1}>\frac{\alpha_{i+1}}{\gamma_{i+1}}
    ~|~\Gamma_i)
    \leqslant
    \Pr\left(X_{i}>8 p_i\frac{\alpha_i}{\gamma_i} ~|~\Gamma_i\right)
    \leqslant
    \exp\left(-(9-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
\end{align*}
%
According to Lemma \ref{lem:y} and Theorem \ref{theo:exp_1}, 
\begin{align*}
    &
    \Pr(C_{i+1}>\frac{\beta_{i+1}}{\gamma_{i+1}}~|~\Gamma_i)
    \\
    =&
    \Pr(|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{0}_i|+|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{1}_i|>\frac{\beta_{i+1}}{\gamma_{i+1}}~|~\Gamma_i)
    \\
    \leqslant&
    \Pr(|\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{0}_i|>\frac{\beta_{i+1}}{2\gamma_{i+1}}
    \lor
    |\mathcal{S}^{1}_{i+1}\cap\mathcal{S}^{1}_i|>\frac{\beta_{i+1}}{2\gamma_{i+1}}~|~\Gamma_i)
    \\
    \leqslant&
    \Pr(\frac{X_i}{\frac{\lambda_{i+1}}{2}}>\frac{\beta_{i+1}}{2\gamma_{i+1}}~|~\Gamma_i)
    +
    \Pr(Y_i>\frac{\beta_{i+1}}{2\gamma_{i+1}}~|~\Gamma_i)
    \\
    \leqslant&
    \Pr(X_i > 4p_i\frac{\alpha_i}{\gamma_i}~|~\Gamma_i)
    +
    \Pr(Y_i>4p_i\frac{\beta_i}{\gamma_i}
    ~|~\Gamma_i)
    \\
    \leqslant&
    \exp\left(-(5-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right)
    +
    \exp\left(-(\frac{11}{3}-e)\frac{3p_i\beta_i}{4\gamma_i}\right)
    .
\end{align*}
\end{proof}\postprof

\subsection{Space and Time Complexity}
\label{finalcon}

\pretheo\begin{theorem}
\label{theo:main}
Let
$R_wR_\lambda\geqslant 2$,
$W=\frac{4(R_wR_\lambda)^{6}}{\varepsilon(R_w-1)(R_\lambda-1)}$,
$\alpha_i= \frac{\Vert F\Vert_1}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
For given $\varepsilon$ and $\delta<\frac{1}{4}$, 
%
let $d$ be the root of the following equation
\begin{align*}
    \frac{R_\lambda^{d}}{(R_wR_\lambda)^{(2^{d}+d)}}=\Delta_1\varepsilon\ln(\frac{1}{\delta}).
\end{align*}
And use an SpaceSaving of size $\Delta_2\ln(\frac{1}{\delta})$ (as the $(d+1)$-layer), then 
\begin{align*}
    \Pr\left(\forall \textit{ item } e, \left|\hat{f}(e)-f(e)\right|\leqslant\varepsilon\Vert F\Vert_1\right)\geqslant 1-\delta,
\end{align*}
where
\begin{align*}
    \Delta_1=2R_w^2R_\lambda^2(R_\lambda-1),
    &&
    \Delta_2=3\left(\frac{R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1=6R_w^3R_\lambda^4.
\end{align*}
\end{theorem}\posttheo

\preprof\begin{proof}
Recall that 
$\Gamma_i=\left(F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)$,
When all conditions $\Gamma_i$ (including $\Gamma_{d+1}$) are true, we have
\begin{align*}
    C_{d+1}
    \leqslant&
    \frac{\beta_{d+1}}{\gamma_{d+1}}
    =
    \frac{2R_\lambda^{d+1}}{(R_wR_\lambda)^{(2^{d}+d-1)}(R_\lambda-1)\varepsilon}
    =
    \left(\frac{2R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1\ln(\frac{1}{\delta}).
    \\
    F_{d+1}
    \leqslant&
    \frac{\alpha_{d+1}}{\gamma_{d+1}}
    =
    \frac{\lambda_{d+1}}{2}\frac{\beta_{d+1}}{\gamma_{d+1}}
    =
    \lambda_{d+1}\left(\frac{R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1\ln(\frac{1}{\delta}).
\end{align*}
Since we use an SpaceSaving of size $\Delta_2\ln(\frac{1}{\delta})>C_{d+1}$, it can record all large items without error, and the estimation error for small items does not exceed
\begin{align*}
    \frac{F_{d+1}}{\Delta_2\ln(\frac{1}{\delta})-C_{d+1}}
    \leqslant
    \frac{\lambda_{d+1}\left(\frac{R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1\ln(\frac{1}{\delta})}{\Delta_2\ln(\frac{1}{\delta})-\left(\frac{2R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1\ln(\frac{1}{\delta})}
    =\lambda_{d+1}
\end{align*}
Therefore, for any item $e$,
\begin{align*}
    \left|\hat{f}(e)-f(e)\right|
    =
    \sum_{i=1}^{d} \lambda_i
    \leqslant
    \sum_{i=1}^{\infty} \frac{\varepsilon\Vert F\Vert_1(R_\lambda -1)}{R_\lambda^{i}}
    =
    \varepsilon\Vert F\Vert_1
\end{align*}
Next, we deduce the probability that at least one condition $\Gamma_i$ is false.
%
Note that
\begin{align*}
    \left.
    \begin{aligned}
    & (\frac{11}{3}-e)\frac{3p_i\beta_i}{4\gamma_i}
    \\
    & (9-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}
    \\
    & (5-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}
    \end{aligned}
    \right\}
    \geqslant\frac{p_i\alpha_i}{\lambda_i\gamma_i}.
\end{align*}
Then According to Theorem \ref{theo:gamma}, we have
\begin{align*}
    &
    \Pr\left(\lnot\left(\bigwedge_{i=1}^{d}\Gamma_{i+1}\right)\right)
    =
    \Pr\left(\bigvee_{i=1}^{d} \lnot\Gamma_{i+1}\right)
    =
    \Pr\left(\bigvee_{i=1}^{d}\left(\bigwedge_{j=1}^{i}\Gamma_j\land\lnot\Gamma_{i+1}\right)\right)
    \\
    \leqslant&
    \sum_{i=1}^{d}\Pr\left(\Gamma_{i}\land\lnot\Gamma_{i+1}\right)
    \leqslant
    \sum_{i=1}^{d}\Pr\left(\lnot\Gamma_{i+1}~|~\Gamma_{i}\right)
    \\
    \leqslant&
    \sum_{i=1}^{d}
    \left(
    \begin{aligned}
    \exp\left(-(\frac{11}{3}-e)\frac{3p_i\beta_i}{4\gamma_i}\right)
    \\+
    \exp\left(-(9-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right)
    +
    \exp\left(-(5-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right)
    \end{aligned}
    \right)
    \\
    \leqslant&
    \sum_{i=1}^{d} 3\exp\left(-\frac{p_i\alpha_i}{\lambda_i\gamma_i}\right).
\end{align*}
Note that
\begin{align*}
    \exp\left(-\frac{p_d\alpha_d}{\lambda_d\gamma_d}\right)
    =&
    \exp\left(-\frac{R_\lambda^{d}}{(R_wR_\lambda)^{(2^{d}+d+2)}\varepsilon(R_\lambda-1)}\right)
    \\
    =&
    \exp\left(-\frac{1}{R_w^2R_\lambda^2(R_\lambda-1)}\Delta_1\ln(\frac{1}{\delta})\right)
    \\
    =&
    \delta^{\left(\frac{1}{R_w^2R_\lambda^2(R_\lambda-1)}\Delta_1\right)}
    =\delta^{2}.
\end{align*}
Since $\delta\leqslant1$, and the monotonicty of $\exp\left(-\frac{p_d\alpha_d}{\lambda_d\gamma_d}\right)$, we have
\begin{align*}
    \exp\left(-\frac{p_i\alpha_i}{\lambda_i\gamma_i}\right)
    =&
    \exp\left(-\frac{p_{i+1}\alpha_{i+1}}{\lambda_{i+1}\gamma_{i+1}}\cdot R_w^{(2^{i}+1)}R_\lambda^{(2^{i})}\right)
    \\
    \leqslant&
    \exp\left(-\frac{p_{i+1}\alpha_{i+1}}{\lambda_{i+1}\gamma_{i+1}}\right)^{R_wR_\lambda}
    \leqslant
    \exp\left(-\frac{p_{i+1}\alpha_{i+1}}{\lambda_{i+1}\gamma_{i+1}}\right)^{2}
    \\
    \leqslant&
    \delta^2\exp\left(-\frac{p_{i+1}\alpha_{i+1}}{\lambda_{i+1}\gamma_{i+1}}\right)
\end{align*}
Therefore, we have
\begin{align*}
    \sum_{i=1}^{d} 3\exp\left(-\frac{p_i\alpha_i}{\lambda_i\gamma_i}\right)
    \leqslant
    3\sum_{i=1}^{d} \delta^{2i}
    \leqslant
    \left(\frac{3\delta}{1-\delta^2}\right)\delta
    \leqslant\delta.
\end{align*}
%
In other words,
\begin{align*}
    \Pr\left(\forall \textit{ item } e, \left|\hat{f}(e)-f(e)\right|\leqslant\varepsilon\Vert F\Vert_1\right)\geqslant 1-\delta,
\end{align*}
which leads to a weaker conclusion,
\begin{align*}
    \forall \textit{ item } e, \Pr\left(\left|\hat{f}(e)-f(e)\right|\leqslant\varepsilon\Vert F\Vert_1\right)\geqslant 1-\delta.
\end{align*}
\end{proof}\postprof

\pretheo\begin{theorem}
Using the same settings as Theorem \ref{theo:main}, the space complexity of the algorithm is $O(\frac{1}{\varepsilon}+\ln(\frac{1}{\delta}))$, and the time complexity of the algorithm is $O(N+\delta\ln\ln(\frac{1}{\varepsilon}) N)$.
\end{theorem}\posttheo

\preprof\begin{proof}
Recall that $d$ is the root of the equation
\begin{align*}
    \frac{R_\lambda^{d}}{(R_wR_\lambda)^{(2^{d}+d)}}=\Delta_1\varepsilon\ln(\frac{1}{\delta}),
\end{align*}
which means $d=O\left(\ln\ln(\frac{1}{\varepsilon})\right)$.
%
Therefore, total space used by the data structure is
\begin{align*}
    \sum_{i=1}^{d} w_i+\Delta_1\ln(\frac{1}{\delta})
    =&
    \sum_{i=1}^{d} \lceil\frac{W (R_{w}-1)}{R_{w}^i}\rceil
    +O(\ln(\frac{1}{\delta}))
    \\
    \leqslant&
    \frac{4(R_wR_\lambda)^{6}}{\varepsilon(R_w-1)(R_\lambda-1)}+d+O(\ln(\frac{1}{\delta}))
    \\
    =&
    O(\frac{1}{\varepsilon}+\ln(\frac{1}{\delta}))
\end{align*}
%
Next, we analyze the time complexity.
%
When all condition $\Gamma_i$ are true, for a new item $e\not\in\mathcal{S}_{1}$, the probability that it enters the $(i+1)$-th layer from the $i$-th layer is
$\frac{\frac{F_i}{\frac{\lambda_2}{2}}+C_i}{w_i}\leqslant p_i$.
%
Thus the time complexity of insert item $e$ does noes exceed
\begin{align*}
    (1-\delta)\cdot(1+\sum_{i=1}^{d} p_i)
    +
    \delta\cdot d
    =
    O(1+\delta\ln\ln(\frac{1}{\varepsilon})).
\end{align*}
%
Since the time complexity of inserting each item does noes exceed the time complexity of inserting it as a new item, the time complexity of the algorithm is
\begin{align*}
    O(N+\delta\ln\ln(\frac{1}{\varepsilon})N).
\end{align*}
\end{proof}\postprof

==> vldb/Body/math_v2.tex <==
\presec
\section{Mathematical Analysis} \postsec
\label{sec:math}

\vspace{0.2cm}

% In this section, we drive the error bounds, the time complexity, and the space complexity of the algorithm.

\subsection{Key Results}
\label{subsec:math:parametersetting}
\label{key}

The key results of this section are to prove the following two claims. 



\ppp{Claim 1:}
%
The algorithm can achieve the following two properties by using $O\left(\frac{N}{\Lambda}+\ln(\frac{1}{\delta})\right)$  space:

%
\begin{align*}
    \Pr\left[\forall \textit{ flow } e, \left|\hat{f}(e)-f(e)\right|\leqslant\Lambda\right]\geqslant 1-\delta
\end{align*}
and 
\begin{align*}
    \forall \textit{ flow } e, \Pr\left[\left|\hat{f}(e)-f(e)\right|\leqslant\Lambda\right]\geqslant 1-\delta
\end{align*}

\ppp{Claim 2:}
%
The algorithm can achieve the above two properties with $O\left(N+\delta\ln\ln(\frac{N}{\Lambda})N\right)$ time complexity.


\ppp{Parameter Configurations:} 
Let $W$ denote the total number of buckets. We set $w_i=\left\lceil\frac{W (R_{w}-1)}{R_{w}^i}\right\rceil$ and $\lambda_i = \left\lfloor\frac{\Lambda (R_\lambda-1)}{R_\lambda^i}\right\rfloor$. 
In our proofs (Theorem \ref{theo:main}), we set $W=\frac{4(R_w R_\lambda)^{6}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, which is with large constant.
But based on our experiment results, we recommend to set $W=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{\Lambda}$, $R_w\in[2, 10]$, $R_l\in[2, 10]$, and $d\geqslant 7$.
When then memory size is given without given $\Lambda$, we set 
\begin{align}
    \Lambda=\frac{(R_w R_\lambda)^{2}}{(R_w-1)(R_\lambda-1)}\cdot \frac{N}{W}
    \label{formula:setLambda}
\end{align}

\subsection{Key Steps}


In this section, we show the following conclusion: by using an \aname{} in $O(\frac{N}{\Lambda})$, we can ensure that the number of packets that cannot find an available bucket in \aname{} is controlled at $O(\ln(\frac{1}{\delta}))$ with a high probability $1-\delta$.
%
In our proof, we classify all flows entering the $i$-th layer into two types:
1) Elephant flows: flows with more than $\frac{\lambda_i}{2}$ ($\lambda_i$ is the error threshold of the $i$-th layer) packets entering the $i$-th layer.
2) Mice flows: flows other than elephant flows. Below we first give a proof sketch because the detailed mathematical analysis is too complex.
%



\ppp{Proof sketch:}
%
The proof consists of the following four steps.
The first three steps focus on a single layer (the $i$-th layer), and analyze the relationship between the $i$-th layer and the $(i+1)$-th layer.
%
The fourth step traverses all layers to draw a final conclusion.
%
\begin{itemize}[leftmargin=*]
    \item Step 1:
    The random process of the $i$-th layer depends on not only the set of packets entering this layer, but also on the arrival order of these packets.
    %
    Based on step 1, to remove the influence of packet arrival order, we construct two random variable $X_i$ and $Y_i$, where $X_i$ bounds the total frequency of the mice flows in the $i$-th layer entering the $(i+1)$-th layer (Lemma \ref{lem:x}), and $Y_i$ bounds the number of distinct elephant flows in the $i$-th layer entering $(i+1)$ layer (Lemma \ref{lem:y}).
    %
    \item Step 2:
    %
    $X_i$ (and $Y_i$) is the sum of a series of random variable $X_{i,k}$ (and $Y_{i,k}$).
    %
    In this step, by using Markov's inequality, we prove that for each random variable $X_{i,k}$ (and $Y_{i,k}$), the probability that it is not zero is controlled by a small number $p_i$ (and $\frac{3}{4} p_i$) (Theorem \ref{theo:markov}).
    \item Step 3:
    %
    If the total frequency of mice flows entering the $i$-th layer and the number of distinct elephant flows entering the $i$-th layer are both controlled, we claim that the $i$-th layer is successfully controlled.
    %
    Based on step 2, by using a Concentration inequality (\ie, a variant of Chernoff bound), we prove that if the $i$-th layer is successfully controlled, then the $(i+1)$-th layer also has a high probability of being controlled (Theorem \ref{theo:gamma}).
    %
    \item Step 4:
    If each layer of \aname{} is successfully controlled, the number of packets that cannot find an available bucket in \aname{} can also be controlled.
    %
    Based on step 3, by using Boole's inequality, we prove that there is a high probability ($1-\delta$) that each layer is successfully controlled, and then the final conclusion holds (Theorem \ref{theo:main}). 
\end{itemize}
%
Due to space constraints, we only show the results of each step below.
%
Below we first list some symbols commonly used in proof, and then give our specific theorems.
We show the detailed proof in Appendix \ref{app:math:pre}-\ref{app:finalcon}.

\ppp{Common symbols.}
%
\begin{enumerate}[leftmargin=*]
    % \setlength{\itemsep}{0.05cm}
    % \item $\mathcal{S}_{i}$: $\{e_1,\cdots,e_{N_i}\}$, the set of items entering the $i$-th layer, where $N_i=|\mathcal{S}_i|$.

    \item $f_i(e)$: the number of times that flow $e$ enters the $i$-th layer.
    
    % \item $\mathcal{S}^{0}_{i}$: $\{e~|~e\in\mathcal{S}_i\land \forall i'\leqslant i, f_{i'}(e)\leqslant \frac{\lambda_{i'}}{2}\}$, the set of mice flows.
    \item $\mathcal{S}^{0}_{i}$: $\{e~|~e\in\mathcal{S}_i\land  f_{i}(e)\leqslant \frac{\lambda_{i}}{2}\}$, the set of mice flows.
    
    % \item $\mathcal{S}^{1}_{i}$:  $\{e~|~e\in\mathcal{S}_i\land \exists i'\leqslant i, f_{i'}(e) > \frac{\lambda_{i'}}{2}\}$, the set of elephant flows.
    \item $\mathcal{S}^{1}_{i}$:  $\{e~|~e\in\mathcal{S}_i\land f_{i}(e) > \frac{\lambda_{i}}{2}\}$, the set of elephant flows.
    
    \item $F_i$: $\sum_{\{e\in\mathcal{S}^{0}_i\}} f_i(e)$, the total frequency of mice flows in $\mathcal{S}^{0}_{i}$.
    
    \item $C_i$: $|\mathcal{S}^{1}_i|$, the number of elephant flows in $\mathcal{S}^{1}_{i}$.
    
    \item $\mathcal{S}^{0}_{i,j}$: $\{e~|~e\in\mathcal{S}^{0}_{i}\land h(e)=j\}$, the set of mice flows that are mapped to the $j$-th bucket.
    
    \item $\mathcal{S}^{1}_{i,j}$: $\{e~|~e\in\mathcal{S}^{1}_{i}\land h(e)=j\}$, the set of elephant flows that are mapped to the $j$-th bucket.
    
    \item $F_{i,j}$: $\sum_{\{e\in\mathcal{S}^{0}_{i,j}\}} f_i(e)$, the total frequency of mice flows in $\mathcal{S}^{0}_{i,j}$.
    
    \item $C_{i,j}$: $|\mathcal{S}^{1}_{i,j}|$, the number of elephant flows in $\mathcal{S}^{1}_{i,j}$.
    
    \item $\mathcal{P}_{i,k}$: $\{e_1,\cdots,e_{k}\}$, a subset of $\mathcal{S}_i$ composed of the first $k$ flows.
    
    \item $f^{P}_{i,k}$: $\sum_{\{e\in\mathcal{P}_{i,k-1}\cap\mathcal{S}^{0}_{i,h(e_k)}\}} f_i(e)$, the total frequency of mice flows with a smaller index that conflicts with flow $e_k$.
    
    \item $c^{P}_{i,k}$: $\left|\{e~|~e\in\mathcal{P}_{i,k-1}\cap\mathcal{S}^{1}_{i,h(e_k)}\}\right|$, the number of elephant flows with a smaller index that conflicts with flow $e_k$.
\end{enumerate}

\ppp{The results of step 1.}

% \subsubsection{Step 1: Separate the elephant flows and the mice flows.}
% For each layer $i$, according to the frequency, we separate the flows into the elephant flows and the mice flows.
% For the elephant flows, we focus on and will control the number of distinct elephant flows. For the mice flows, we will control the total frequency of mice flows.
% Specifically, if the number of packets that flow $e$ enters the $i$-th layer ($f_i(e)$) is greater than half of the error threshold $\lambda_i$, it is an elephant flow. Otherwise, it is a mice flow.
%wyh：我想在这里大概交代一下使用的符号

% \subsubsection{Step 2: Remove the influence of packet arrival order.}
%wyh：这部分介绍我们构造了一个变量来移除考察顺序的影响。来说明我们计算Xi和Yi就可以控制住误差。
% We construct a more regular random variable sequence Xi and Yi as the bounds of small flow and large flow respectively.
\pretheo\begin{lemma}
\label{lem:x}    
    Let
    \begin{align*}
        X_{i,k}=
            \begin{cases}
              0 & C_{i, h(e_k)}=0 \land f^{P}_{i,k}\leqslant \frac{\lambda_i}{2}
            \\
              f_i(e_k) &  C_{i, h(e_k)}=0\land f^{P}_{i,k} > \frac{\lambda_i}{2}
            \\
              f_i(e_k) & C_{i, h(e_k)}>0
            \end{cases},
        &&
        X_i=\sum_{\{e_k\in\mathcal{S}^{0}_{i}\}} X_{i,k}.
    \end{align*}
    The total frequency of the mice flows in the $i$-th layer entering the $(i+1)$-th layer does not exceed $X_i$, \ie,
    \begin{align*}
        F_{i+1}
        \leqslant
        \sum_{\{e\in\mathcal{S}^{0}_i\cap\mathcal{S}_{i+1}\}} f_{i+1}(e) \leqslant X_{i}.
    \end{align*}
\end{lemma}\posttheo


% Similarly, we have the following lemma.
\pretheo\begin{lemma}
\label{lem:y}
   Let 
    \begin{align*}
        &Y_{i,k}=
            \begin{cases}
              0 &  c^{P}_{i,k}=0\land F_{i,h(e_k)}\leqslant \lambda_i,
            \\
              2 & c^{P}_{i,k}=0\land F_{i,h(e_k)}> \lambda_i
            \\
              2 & c^{P}_{i,k}>0.
            \end{cases},
        &&
        Y_{i}=\sum_{e_k\in\mathcal{S}^{1}_{i}} Y_{i,k}.
    \end{align*}
    The number of distinct elephant flows in the $i$-th layer entering the $(i+1)$-th layer does not exceed $Y_i$, \ie,
    \begin{align*}
        \left|\mathcal{S}^{1}_{i}\cap\mathcal{S}^{1}_{i+1}\right|\leqslant Y_{i}.
    \end{align*}
\end{lemma}\posttheo


\ppp{The results of step 2.}

% \subsubsection{Step 3: Control the probability of any flow entering the next level.}
%wyh：这部分改了一下，把原来不等号右边的表达式改成了pi，这样方便理解。
\pretheo\begin{theorem}
Let
$W=\frac{4N(R_wR_\lambda)^{6}}{\Lambda(R_w-1)(R_\lambda-1)}$,
$\lambda_i = \frac{\Lambda (R_\lambda-1)}{R_\lambda^i}$,
$\alpha_i= \frac{N}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
%
Under the conditions of
    $F_i\leqslant\frac{\alpha_i}{\gamma_i}$ and
    $C_i\leqslant\frac{\beta_i}{\gamma_i}$,
we have
    \begin{align*}
        \Pr\left(X_{i,k}>0~|~X_{i,1},\cdots,X_{i,k-1}\right)
        \leqslant
        p_i,
        && \forall e_k\in\mathcal{S}^{0}_{i}.
        \\
        \Pr\left(Y_{i,k}>0~|~Y_{i,1},\cdots,Y_{i,k-1}\right)
        \leqslant 
        \frac{3}{4} p_i,
        && \forall e_k\in\mathcal{S}^{1}_{i}.
    \end{align*}
\label{theo:markov}
\end{theorem}\posttheo


\ppp{The results of step 3.}

% \pretheo\begin{theorem}
% \label{theo:exp_1}
% Let
% $W=\frac{4(R_wR_\lambda)^{6}}{\varepsilon(R_w-1)(R_\lambda-1)}$,
% $\alpha_i= \frac{N}{(R_wR_\lambda)^{i-1}}$,
% $\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
% $\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
% $p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
% %
% Under the conditions of
%     $F_i\leqslant\frac{\alpha_i}{\gamma_i}$ and
%     $C_i\leqslant\frac{\beta_i}{\gamma_i}$,
% we have
% \begin{align*}
%     \Pr\left(X_{i}>(1+\delta)\frac{p_i\alpha_i}{\gamma_i}\right)
%     \leqslant
%     \exp\left(-(\delta-(e-2))\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
% \end{align*}
% and
% \begin{align*}
%     \Pr\left(Y_{i}>(1+\delta)\frac{3}{2}\frac{p_i\beta_i}{\gamma_i}\right)
%     \leqslant
%     \exp\left(-(\delta-(e-2))\frac{3p_i\beta_i}{4\gamma_i}\right).
% \end{align*}
% \end{theorem}\posttheo




% \subsubsection{Step 4: merge all layers.}
% wyh：归纳法，希望能写得更易读一点？用文字解释一下定理的结果。是不是可以把式子右边的概率用变量来替换比如exp(-G_i),然后把G_i写在普通的参数里？

\pretheo\begin{theorem}
\label{theo:gamma}
Let
$R_wR_\lambda\geqslant2$,
$W=\frac{4N(R_wR_\lambda)^{6}}{\Lambda(R_w-1)(R_\lambda-1)}$,
$\lambda_i = \frac{\Lambda (R_\lambda-1)}{R_\lambda^i}$,
$\alpha_i= \frac{N}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
%
We have
%
\begin{align*}
&    
    \Pr\left(F_{i+1}>\frac{\alpha_{i+1}}{\gamma_{i+1}}
    ~|~
    F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)
    \leqslant
    \exp\left(-(9-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right).
    \\
&
    \Pr\left(C_{i+1}>\frac{\beta_{i+1}}{\gamma_{i+1}}
    ~|~
    F_{i}\leqslant\frac{\alpha_{i}}{\gamma_{i}} \land
    C_{i}\leqslant\frac{\beta_{i}}{\gamma_{i}}\right)
    \\
    \leqslant&
    \exp\left(-(5-e)\frac{2p_i\alpha_i}{\lambda_i\gamma_i}\right)
    +
    \exp\left(-(\frac{11}{3}-e)\frac{3p_i\beta_i}{4\gamma_i}\right).
\end{align*}
\end{theorem}\posttheo

% \subsubsection{Step 5: Handle small remaining traffic.}
% 这部分能不能最好不提space saving，就直接说上送？空间消耗就是原始数据结构+上送量？应该还是ln(1/delta) ?

\ppp{The results of step 4.}

\pretheo\begin{theorem}
\label{theo:main}
Let
$R_wR_\lambda\geqslant 2$,
$W=\frac{4N(R_wR_\lambda)^{6}}{\Lambda(R_w-1)(R_\lambda-1)}$,
$\lambda_i = \frac{\Lambda (R_\lambda-1)}{R_\lambda^i}$,
$\alpha_i= \frac{N}{(R_wR_\lambda)^{i-1}}$,
$\beta_i= \frac{\alpha_i}{\frac{\lambda_i}{2}}$,
$\gamma_i=(R_wR_\lambda)^{(2^{i-1}-1)}$, and
$p_i = (R_wR_\lambda)^{-(2^{i-1}+4)}$.
For given $\Lambda$ and $\delta<\frac{1}{4}$, 
%
let $d$ be the root of the following equation
\begin{align*}
    \frac{R_\lambda^{d}}{(R_wR_\lambda)^{(2^{d}+d)}}=\Delta_1\frac{\Lambda}{N}\ln(\frac{1}{\delta}).
\end{align*}
And use an SpaceSaving of size $\Delta_2\ln(\frac{1}{\delta})$ (as the $(d+1)$-layer), then 
\begin{align*}
    \Pr\left(\forall \textit{ flow } e, \left|\hat{f}(e)-f(e)\right|\leqslant\Lambda\right)\geqslant 1-\delta,
\end{align*}
where
\begin{align*}
    \Delta_1=2R_w^2R_\lambda^2(R_\lambda-1),
    &&
    \Delta_2=3\left(\frac{R_wR_\lambda^2}{R_\lambda-1}\right)
    \Delta_1=6R_w^3R_\lambda^4.
\end{align*}
\end{theorem}\posttheo

% \subsubsection{Final results.}

\ppp{Complexity of \aname{}.}

\pretheo\begin{theorem}
Using the same settings as Theorem \ref{theo:main}, the space complexity of the algorithm is $O(\frac{N}{\Lambda}+\ln(\frac{1}{\delta}))$, and the time complexity of the algorithm is $O(N+\delta\ln\ln(\frac{N}{\Lambda}) N)$.
\end{theorem}\posttheo


==> vldb/Body/relate.tex <==
\presec
\section{Related Work} \postsec
\label{sec:relate}

In this section, we introduce existing sketches from three aspects: 1) the tasks they support, 2) the type of their error, and 3) their operations for distributed systems and incremental deployment.


\presub
\subsection{Sketches for Various Tasks} \postsub
\label{subsec:relate:}
We introduce common data stream processing tasks and their corresponding algorithms.

\ppp{Frequency estimation} refers to estimating the frequency of an item in a data stream. 
A great many solutions use sketches. 
Sketches are a series of memory-efficient data structure for frequency estimation and other applications.
Some typical sketches include Count-Min (CM) sketches \cite{cmsketch}, CU sketches \cite{cusketch}, Count sketches \cite{countsketch} and more \cite{coldfilter,Sketchingclassifiers,persistent-bf,persistentsketch,complexaggre,pyramid,ada-sketch}.
CM sketches, CU sketches and Count sketches use a two-dimensional array of counters to record items' frequencies.
They also use pairwise-independent hash functions to map items into several mapping counters.


\ppp{Finding frequent items} refers to finding items whose frequencies exceed a user-specified threshold.
Existing works can be classified into two kinds of algorithms: counters-only algorithms and ID-frequency pair algorithms.
counters-only algorithms have only one counter in each bucket.
Typical counters-only algorithms include Count-Min (CM) sketches \cite{cmsketch}, CU sketches \cite{cusketch} and Count sketches \cite{countsketch}.
Since they do not record ID for each counter, all items are updated into the counters.
Instead of recording only the counter, ID-frequency pair algorithms also have a field to record the ID/key of the counter.
Typical ID-frequency pair algorithms include Space-Saving \cite{spacesaving}, Unbaised Spave-Saving \cite{ting2018data} and Frequent \cite{frequent}.
Because recording all IDs is memory consumption, these algorithms only keep a monitored set to record.

\ppp{Heavy change detection} refers to finding items whose frequencies in two adjacent time windows vary a lot.
Several algorithms based on sketches are designed for heavy change detection.
Sketches are used to summarize the frequency during each window.
Typical algorithms for heavy change detection are based on the CM sketch \cite{cmsketch}, the $k-ary$ sketch \cite{changedetection}, and HeavyGuardian \cite{heavyguardian}.

\ppp{Cardinality Estimation} refers to estimating the number of different items in a data stream.
Bitmap \cite{bitmap} and HyperLogLog \cite{hyperloglog} are two typical algorithms for this task.
The Bitmap is a n-bit vector with all bits set to 0 initially. When inserting item $e$, it maps $e$ to a mapping bit according to the hash value $h(e)$, and set the mapping bit to 1. To output a cardinality estimation, it calculates the number of 0s in it, denoted as $u$, and output an estimation as: $-n\ln{\frac{u}{n}}$.
The HyperLogLog uses a counter array, and achieve higher accuracy through more complex calculation. 



\ppp{Frequency distribution estimation} refers to estimating the frequency distribution in a data stream.
FlowRadar \cite{flowradar}, MRAC \cite{kumar2004data} are two representative algorithms for the task.
The shortcoming of these algorithms is that they do not support real-time query.
HeavyGuardian \cite{heavyguardian} can support real-time frequency distribution estimation, which is important for some applications.



\ppp{Entropy Estimation} refers to estimating the entropy of item frequencies. Entropy of a data stream reflects its uncertainty. Mathematically, it is defined as $\sum_{i}\frac{f_i}{M}log_2 \frac{f_i}{M}$, where $M$ is total number of items in the data stream, $f_i$ is the frequency of item $e_i$. \citet{lall2006data} proposed an algorithm to estimate entropy using sampling and mathematical derivation.
But it can not support real-time query.
HeavyGuardian \cite{heavyguardian} uses an auxiliary array that maintains the frequency distribution of the data stream to support real-time entropy estimation.


\presub
\subsection{Sketch Estimation Types } \postsub
\label{subsec:relate:}
Frequency estimation is one of the most common tasks. Therefore, there have been scores of algorithms for it. The frequencies estimated by these algorithms have different properties. We classify these algorithms into three types, according to the property of estimated frequency.

\ppp{Over estimation: }Many algorithms output an answer without an under-estimation error. Typical algorithms in this category include CM sketches \cite{cmsketch}, CU sketches \cite{cusketch}, and SpaceSaving \cite{spacesaving}.

\ppp{Under estimation: }On the contrary, some algorithms have no over-estimation error, which means the output is always equal or less to the ground truth. Representative algorithms like HeavyKeeper \cite{heavykeeper}, the heavy part of HeavyGuardian \cite{heavyguardian}.

\ppp{Unbiased estimation: }Many algorithms pursuit for providing unbiased frequency estimation for items. The state-of-the-art algorithms in this category include Count sketches \cite{countsketch}, Unbiased Space-Saving \cite{ting2018data}, Waving Sketch \cite{li2020wavingsketch}.

To the best of our knowledge, we are the first sketch that outputs both over estimation and under estimation.


\presub
\subsection{Sketch for Distributed Systems and Incremental Deployment.} \postsub
\label{subsec:relate:}

In distributed data stream scenarios, the data stream processors in the remote sites are often required to adjust the precision, transmit the query results, and aggregate the answer from different sites \cite{olston2003adaptive, cormode2008approximate}.
Three sketch operations, \ie, compression, expansion, and aggregation, support the above three requirements.
For adjusting the precision, there are some filters/sketches that can adapt to both the precision constraints and drastically changing data volume by resizing---compression/expansion \cite{pandey2017general,yang2018elastic}.
When processing distributed streams, we need to aggregate the answer, but only a few existing sketches consider it \cite{ECMsketch}.
Therefore, the operations are crucial for a sketch in distributed scenarios.
As the remote sites may be heterogeneous, the incremental deployment should be considered.
When one site constructs a new kind of sketch, it is satisfying if the new sketch can be compatible with some standard sketches (\eg, CM \cite{cmsketch}, and CU \cite{cusketch}), which means the new sketch can be transformed into standard sketches and can be merged with standard sketches.
To the best of our knowledge, no existing sketch work has focused on this issue.

% compression expansion aggregation 哪些sketch能做哪些不能做
% 这部分可能不好写。参照elastic sketch。




%In this section, we first show the related work on finding frequent items in Section \ref{subsec:relate:frequent}.
%Then we will show the related work on other applications in Section \ref{subsec:relate:other}.

%In this section, we only show the related algorithms for the four typical top-$k$ tasks, for other related work please refer to \cite{sketchsurvey, maxloghash, sketchml}. 

%Besides the tasks mentioned so far, sketch-based techniques have also attracted attention in other applications, such as estimating set similarity\cite{maxloghash}
%, accelerating distributed machine learning\cite{sketchml}, 
%, \etc. 

%\presub
%\subsection{Finding Frequent Items} \postsub
%\label{subsec:relate:frequent}

%To find frequent items, two types of solutions exist.
%The first, \textit{sketch-based algorithms}, records the frequencies of all items through linear projections. The second, \textit{KV-based algorithms}, records $<ID, frequency>$ pairs of a subset of items that have a large frequency. %Then we will show the related work of these two types in detail.

%\ppp{Sketch-based Algorithms:}
%Typical sketches include the CM~\cite{cmsketch}, CU~\cite{cusketch}, Count~\cite{countsketch}, and ASketch~\cite{asketch}.
%These sketches often consist of multiple arrays, each containing many counters.
%Each array is associated with a hash function that maps items to the counters. 
%Hash collision may lower their accuracy, so they use some methods to reduce the error, however these methods are usually memory inefficient. 
%This is because they also record relatively unimportant small items. 
%Furthermore, sometimes multiple memory accesses per insertion decrease their throughput.


%\ppp{KV-based Algorithms:}
%Typical KV-based algorithms include SpaceSaving~\cite{spacesaving, finding2008}, Unbiased SpaceSaving~\cite{unbiasedsketch}, Lossy Counting \cite{losscounting}, HeavyGuardian \cite{heavyguardian}, and Cold filter~\cite{coldfilter}.
%SpaceSaving and Unbiased SpaceSaving use a data structure called Stream-Summary to record frequent items. When the data structure is full, the frequency of the least frequent item is incremented by one whenever a new item arrives. 
%In this way, the frequencies are over-estimated.
%Unbiased SpaceSaving achieves unbiased estimation by \textit{considering the frequencies of all non-recorded items as $0$}.
%Below we use an example to illustrate the low accuracy of Unbiased SpaceSaving. 
%For example, given a data stream with $10^6$ distinct items, each appearing $10$ times, only one bucket is used to choose the most frequent item. For Unbiased SpaceSaving, the estimated frequency of the item recorded in the bucket is $10^7$, while the estimated frequencies of all other items are $0$. 
%Although the average estimated frequency is unbiased, the relative error of the recorded items is very large, \ie, $10^6$.
%Also, for each insertion, many pointer operations reduce the throughput of SpaceSaving and Unbiased SpaceSaving.


%\vspace{-0.05in}
%\subsection{old-Other Applications}
%\label{subsec:relate:other}

%\presub
%\subsection{Frequency estimation} \postsub
%To find heavy changes, there are two kinds of algorithms.
%One is \textit{record all}. This kind of algorithms build a data structure to record all items in each period, and then decode and report heavy changes. 
%Typical algorithms include k-ary \cite{kary}, the reversible sketch \cite{revsketch}, and FlowRadar \cite{flowradar}. 
%FlowRadar \cite{flowradar} uses a Bloom filter to remove duplicates, and records each item in a modified Invertible Bloom Lookup Table (IBLT) \cite{iblt}. 
%When IBLT uses the appropriate parameters, FlowRadar can successfully decode all the items with high probability. 
%As FlowRadar records and decodes all items, it is not memory efficient.
%The other kind of solutions only records frequent items. A typical algorithm is Cold filter \cite{coldfilter}. 
%Based on FlowRadar, Cold filter \cite{coldfilter} uses an additional filter to filter infrequent items, and only inserts frequent ones into FlowRadar, achieving higher accuracy.
%However, as FlowRadar is inherently not a compact data structure, it is still not memory efficient even with Cold filter.
%Both solutions are not memory efficient because their data structures are not compact.


==> vldb/Body/related_end.tex <==

\vspace{-0.1in}
\presec
\section{Related Work} \postsec
\label{sec:relatedend}

\vspace{-0.1in}

% \wyh{In addition to sec. \ref{}, we introduce more measurement solutions in this section.}





\ppp{Sampling Solutions.} Many measurement systems monitor the traffic by sampling packets. Typical solutions include NetFlow \cite{netflow}, sFlow \cite{sflow}, Everflow \cite{zhu2015packet}, OpenSketch \cite{yu2013OpenSketch}, OpenSample \cite{suh2014opensample}, NitroSketch \cite{liu2019nitrosketch}, and more \cite{duffield2001trajectory,sekar2008csamp,sekar2010revisiting,li2019large}.
Although sampling can directly reduce both time and space overhead, it misses most packets. So it cannot sense and control the error certainly.

%sampling 丢失了很多包，无法感知和控制误差。
% \ppp{Probing Solutions.} By actively sending packets, probing solutions can monitor large-scale network effectively. However, they cannot obtain measurement statistics at per-flow level.
% Typical solutions include AM-PM \cite{}, Pingmesh \cite{} NetBoncer, NetSonar, NetNorad, and more.
%我们关注的是全流策略，probing无法做到每流的粒度
\ppp{Sketch-based Solutions.}
The sketch is a kind of probabilistic data structure \cite{cmsketch,mitzenmacher2002compressed,mitzenmacher2001power,sketchsurvey} and a great many of sketch-based measurement solutions have emerged recently, including UnivMon \cite{liu2016UnivMon}, SketchLib \cite{namkung2022sketchlib}, Coco \cite{zhang2021cocosketch}, Hetero \cite{nsdi2022HeteroSketch}, SketchVisor \cite{huang2017sketchvisor} and SeqSketch \cite{huang2021toward}.
% Sketches \cite{Sketchlib?} have attracted extensive attention recently. 
The most relevant work is the Elastic sketch\cite{yang2018elastic}. They aims at adapting to dynamic traffic and devise the data structure of Elastic based on the idea of election.
Many existing work uses the idea of election, including Elastic, CoCo, Majority \cite{boyer1991majority}, and SpaceSaving \cite{spacesaving}.
Our design benefit from them, but our way and goal are different. 
Their design goal is not to perceive errors, and they do not further use perceived errors in data structures. Our Error-Sensible bucket is not exactly the same as any of them. 
% Specifically, the most similar Elastic uses election to find frequent flow in order to estimate them more accurately.
% In contrast, our approach is to sense the error by the number of "NO", which is not directly applicable to Elastic because Elastic clears the number of "NO" everytime a replacement happens. 
% More solutions are detailed in sec \ref{?}.
% Many sketch-based systems that have made progress in various aspects. 
% Our work can be combined with and benefit from many of them.
Univmon is a general sketch with multiple functions. 
BeauCoup \cite{chen2020beaucoup} can perform measurement over many keys simultaneously, and 
CoCo supports the measurement over arbitrary partial key.
HeteroSketch, Trumpet \cite{trumpet}, DREAM \cite{dream} and SCREAM \cite{moshref2015scream} manage the resource for measurement wisely. 
SketchVisor and SeqSketch improve the accuracy via compressive sensing to nearly zero, which works well when the resource is sufficient but cannot address our design goal under scarce resource or at line rate.

\ppp{In-band Telemetry Solutions.} These solutions append packet-level measurement statistics to each packet, which provides a lot of information. Typical solutions include INT and PINT. Recently, LightGuardian \cite{zhao2021lightguardian} shows that sketch can be cleverly combined with in-band telemetry to achieve a win-win situation.
%每包资源消耗太大，我们研究的是单点的sketch，可以和INT结合进行传输。

\ppp{Recovery Schemes.} These solutions often achieve very high accuracy by recovery approaches, including solving equations and compressive sensing.
But they cannot provide estimations at line rate because they need recovery and aggregation. 
Typical schemes include CounterBraids \cite{lu2008counterbraids}, Omnimon \cite{huang2020omnimon}, FlowRadar \cite{flowradar} and more \cite{li2016lossradar,iblt}. 

% They are deployed in network-wide mostly and can achieve Zero-Error or Nearly-Zero-Error when the resource is sufficient. However, they cannot provide measurement results in real-time but \anamelong{} can. And Zero-Error means that the algorithm is an exact one, whose space complexity is as large as using one hash table to count all flows exactly.
% We mainly focus on, when the error exists, how to make the function and overhead best while meeting the error limit.
% We can also benefit from recovery schemes. For example, we can establish inequalities in network-wide deployment to optimize the accuracy. We leave it for future work.

\ppp{Top-K Algorithms.}
Many algorithms aim to find top-k frequent flows and heavy hitters, including Frequent \cite{demaine2002frequency}, Space Saving \cite{spacesaving}, Unbiased Space Saving \cite{unbiasedsketch}, and more \cite{boyer1991majority}.
They estimate the flow size by appending one counter for every top-k frequent flow. For other flows, they do not provide estimation value. 
Our basic Error-Sensible buckets benefit from some of these algorithms.
These algorithms, relying on heaps and linked lists, are too complex to be implemented on programmable switches. They cannot achieve our design goal at line rate.


% CM sketches, CU sketches and Count sketches use a two-dimensional array of counters to record items' frequencies.
% They also use pairwise-independent hash functions to map items into several mapping counters.



% Frequency estimation is one of the most common tasks. Therefore, there have been scores of algorithms for it. The frequencies estimated by these algorithms have different properties. We classify these algorithms into three types, according to the property of estimated frequency.

% \ppp{Over estimation: } Many algorithms output an answer without an under-estimation error. Typical algorithms in this category include CM sketches \cite{cmsketch}, CU sketches \cite{cusketch}, and SpaceSaving \cite{spacesaving}.

% \ppp{Under estimation: } On the contrary, some algorithms have no over-estimation error, which means the output is always equal or less to the ground truth. Representative algorithms like HeavyKeeper \cite{heavykeeper}, the heavy part of HeavyGuardian \cite{heavyguardian}.

% \ppp{Unbiased estimation: }Many algorithms pursuit for providing unbiased frequency estimation for items. The state-of-the-art algorithms in this category include Count sketches \cite{countsketch}, Unbiased Space-Saving \cite{ting2018data}, Waving Sketch \cite{li2020wavingsketch}.

% To the best of our knowledge, we are the first sketch that outputs both over estimation and under estimation.



% \ppp{Finding frequent items} refers to finding items whose frequencies exceed a user-specified threshold.
% Existing works can be classified into two kinds of algorithms: counters-only algorithms and ID-frequency pair algorithms.
% counters-only algorithms have only one counter in each bucket.
% Typical counters-only algorithms include Count-Min (CM) sketches \cite{cmsketch}, CU sketches \cite{cusketch} and Count sketches \cite{countsketch}.
% Since they do not record ID for each counter, all items are updated into the counters.
% Instead of recording only the counter, ID-frequency pair algorithms also have a field to record the ID/key of the counter.
% Typical ID-frequency pair algorithms include Space-Saving \cite{spacesaving}, Unbaised Spave-Saving \cite{ting2018data} and Frequent \cite{frequent}.
% Because recording all IDs is memory consumption, these algorithms only keep a monitored set to record.



% The CM sketch can estimate most flow sizes accurately. Specifically, given a data stream with $N$ items, with $1-\delta$ probability, the absolute error of the query is smaller than $\Lambda$, \ie, $\Pr\big[Absolute Error$\footnote{The absolute error is $|\hat{f}(e)-f(e)|$, where $\hat{f}(e)$ is the estimated flow size of $e$ and $f(e)$ is the true flow size.}$\leqslant \Lambda]\geqslant 1-\delta$.
% When $\Lambda=10, \delta=0.05$, there is a 95\% probability that the absolute error is less than or equal to 10 (packets).
% Toward the above accuracy, CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time.

==> vldb/Body/related_v1.tex <==
\presec
\section{Background and Related Work} \postsec
\label{sec:relate}

% In this section, we introduce existing sketches from three aspects: 1) the tasks they support, 2) the type of their error, and 3) their operations for distributed systems and incremental deployment.
% In this section, we introduce the frequency estimation problem, existing sketches, and other related work.
In this section, we first introduce the background of frequency estimation problem. Then we introduce existing sketches that can estimate the frequency of all items, and other related work.

\presub
\subsection{Preliminaries} \postsub
% \label{??}

\ppp{ Stream:} A data stream $\mathcal{S}=\{\langle e_1, w_1\rangle,$ $ \langle e_2, w_2\rangle,$ $ \dots$, $\langle e_t, w_t\rangle,$ $ \dots,$ $ \langle e_N, w_N\rangle\}$ is a sequence of $N$ items following time order. Each item is a pair of identifier $e_t$ and weight $w_t$ ($w_t>0$). 
An identifier $e$ may appear more than once in different pairs. 
The statistic algorithm should process each data item in real time to support online queries.
% The data stream should be processed in one pass.

\ppp{Frequency Estimation Problem:} There are two types of frequency estimation, Occurrence Counting and Weighted Counting. 

\noindent\textit{Type I: Occurrence Counting.} Given a queried item identifier $e$, we count the number of times that it appears, \ie, $f(e)\coloneqq \sum_{\forall e_t=e} 1$. If $e$ never appears in the data stream, its frequency is $0$. 
We pay more attention to type I, but we also support type II well.

\noindent\textit{Type II: Weighted Counting.} Given a queried item identifier $e$, we sum up all its weights and report the result, \ie, $f(e)\coloneqq \sum_{\forall e_t=e} w_t$.

% The weighted frequency of item $e$ is the total weight, \ie, $w(e)\coloneqq \sum_{\forall e_t=e} w_t$. 
% A data streaming algorithm (\eg, sketches) can only process the data stream in single pass. Our \aname{} is to estimate $f(e)$ and $w(e)$ for arbitrary queried item $e$ ($e$ may not appear in the data stream).

\presub
\subsection{Sketches for Frequency Estimation} \postsub
% \label{??}
%\wyh{Comment: No more sketch estimates the frequency in recent years. The following sketches are not for frequency estimation.  COMPASS \cite{2021Online} (SIGMOD'21), CSC \cite{li2021building} (SIGMOD'21), and Correlation \cite{santos2021correlation} (SIGMOD'21).}
The sketch is a kind of approximate algorithm for frequency estimation and many other tasks \cite{yang2019gb,yang2017sf,indyk2000identifying,garofalakis2013sketch,ting2018count,schweller2007reversible,xie2016topicsketch,shan2016cvs,shrivastava2016time,tai2018sketching,wei2015persistent,cmsketch,csmsketch,izenov2021compass,shi2021time, li2021building, santos2021correlation,pyramid,countsketch,jia2021bidirectionally,dai2021active,zhao2021learned}. In this section, we focus on sketches that can estimate frequency for all items.
% including Count-Min (CM) sketch \cite{cmsketch} and Count sketch \cite{countsketch}. These two sketches
% are two milestones in the theory of frequency estimation. A great many of followers have made a lot of contributions in many aspects, but none of them outperforms CM and Count in theoretical complexity \cite{coldfilter,Sketchingclassifiers,persistent-bf,persistentsketch,complexaggre,pyramid,ada-sketch}.
We classify these sketches into two categories according to the error type, \ie, one-side estimation and unbiased estimation. 
All these sketches can neither sense the error of every estimation, nor control all errors below user-defined threshold.

\ppp{One-Side Estimation.} The sketches for one-sided frequency estimation guarantee the estimated frequency must be no less than the truth. The Count-Min (CM) sketch \cite{cmsketch} is the milestone with the best theoretical result.
A CM sketch consists of $d$ counter arrays, $A_1[], A_2[], \dots, A_d[]$. When counting frequency, for each incoming item $e$, CM picks one counter (called \textit{mapped counters}) in every array by independent hashing $A_i[h_i(e)]$, where $h_i(\cdot)$ is a hash function, and then increment these mapped counters by one.
When querying the frequency of an item, CM reports the minimal counter among these mapped counters.
Given a data stream with $N$ items, when the probability that the absolute error of an estimation is smaller than $\varepsilon \Vert F \Vert _1$ ($\Vert F \Vert _1=\sum_e f(e)$) is greater than $1-\delta$, \ie, $\Pr\big[Absolute Error$\footnote{The absolute error is $|\hat{f}(e)-f(e)|$, where $\hat{f}(e)$ is the estimated frequency of item $e$ and $f(e)$ is the true frequency.}$\leqslant \varepsilon \Vert F \Vert _1\big]\geqslant 1-\delta$, CM needs $O\left(\frac{1}{\varepsilon}\ln(\frac{1}{\delta})\right)$ space and can be built in real time by $O\left(N\ln(\frac{1}{\delta})\right)$ total time.
Many studies improves the performance of sketches, including Conservative Update \cite{cusketch}, Augmented \cite{asketch}, and Cold Filter \cite{coldfilter}. They greatly reduce the average error in practice, but none of them outperforms CM in theoretical complexity.


\ppp{Unbiased Estimation.} The sketches for unbiased frequency estimation guarantee the expectation of the estimated frequency is the true frequency. Unbiased estimation is useful in estimating the sum of a set of items and estimating the average frequency of a set of items.
The Count sketch \cite{countsketch} is the milestone with the best theoretical result in unbiased estimation. Given a data stream $\mathcal{S}$, its L2-norm is $\Vert F \Vert _2=\sqrt{\sum_e f^2(e)}$. When $\Pr[Absolute Error\leqslant \varepsilon \Vert F \Vert _2]\geqslant 1-\delta$, Count needs $O\left(\frac{1}{\varepsilon^2}\ln(\frac{1}{\delta})\right)$ space and can be built in real time by $O\left(\ln(\frac{1}{\delta})\Vert F \Vert _1\right)$ total time.
Other sketches \cite{deng2007new} also provides unbiased estimation. But none of them outperforms Count in theory.
The theoretical results of CM (one-size estimation) and Count (unbiased estimation) are not comparable because they are based on L1-norm and L2-norm, respectively. In our theory study, we focus on one-size estimation.


\presub
\subsection{Other Algorithms} \postsub

\ppp{Finding Top-k Frequent Items.}
Many algorithms aim to find top-k frequent item in the data streams, including Frequent \cite{demaine2002frequency}, Space Saving \cite{spacesaving}, Unbiased Space Saving \cite{unbiasedsketch} and more \cite{yang2018heavyguardian,manku2002approximate,yang2019heavykeeper}.
They estimate the frequencies of top-k items by appending one counter for every top-k frequent item. 
For other items other than the top-k, they do not provide estimation value.
In contrast, we need to sense and control the errors of all items.
% But they cannot estimate other items accurately.
%核心不一样，是不一样问题。
In addition, they cannot support the weighted counting efficiently. They need a heap or a priority queue to order the top-k frequent items, which consumes $O\left(log(k)\right)$ time for each new item. 

% CM sketches, CU sketches and Count sketches use a two-dimensional array of counters to record items' frequencies.
% They also use pairwise-independent hash functions to map items into several mapping counters.



% Frequency estimation is one of the most common tasks. Therefore, there have been scores of algorithms for it. The frequencies estimated by these algorithms have different properties. We classify these algorithms into three types, according to the property of estimated frequency.

% \ppp{Over estimation: } Many algorithms output an answer without an under-estimation error. Typical algorithms in this category include CM sketches \cite{cmsketch}, CU sketches \cite{cusketch}, and SpaceSaving \cite{spacesaving}.

% \ppp{Under estimation: } On the contrary, some algorithms have no over-estimation error, which means the output is always equal or less to the ground truth. Representative algorithms like HeavyKeeper \cite{heavykeeper}, the heavy part of HeavyGuardian \cite{heavyguardian}.

% \ppp{Unbiased estimation: }Many algorithms pursuit for providing unbiased frequency estimation for items. The state-of-the-art algorithms in this category include Count sketches \cite{countsketch}, Unbiased Space-Saving \cite{ting2018data}, Waving Sketch \cite{li2020wavingsketch}.

% To the best of our knowledge, we are the first sketch that outputs both over estimation and under estimation.



% \ppp{Finding frequent items} refers to finding items whose frequencies exceed a user-specified threshold.
% Existing works can be classified into two kinds of algorithms: counters-only algorithms and ID-frequency pair algorithms.
% counters-only algorithms have only one counter in each bucket.
% Typical counters-only algorithms include Count-Min (CM) sketches \cite{cmsketch}, CU sketches \cite{cusketch} and Count sketches \cite{countsketch}.
% Since they do not record ID for each counter, all items are updated into the counters.
% Instead of recording only the counter, ID-frequency pair algorithms also have a field to record the ID/key of the counter.
% Typical ID-frequency pair algorithms include Space-Saving \cite{spacesaving}, Unbaised Spave-Saving \cite{ting2018data} and Frequent \cite{frequent}.
% Because recording all IDs is memory consumption, these algorithms only keep a monitored set to record.


==> vldb/Body/related_v2.tex <==
\presec
\section{Background and Motivation} \postsec
\label{sec:relate}
In this section, we begin with the problem definition, followed by their use cases. Then we discuss the limitations of existing sketches through the typical CM Sketch. 
We introduce more measurement solutions in \cref{sec:relatedend}.
% , and introduce more sketch-based measurement solutions. 
% For more measurement solutions, \wyh{we introduce them in Sec end\ref{??}}.
% In this section, we begin with the background of sketch algorithms, followed by their limitations. Then we discuss the potential use cases of sensing and controlling the error. Finally, we discuss other related work in measurement.

\presub
\subsection{Problem Definition and Use Cases} \postsub
\label{subsec:related:problem}
\label{subsec:related:usecase}
% \presub
% \subsection{Sketches and Their Limitations} \postsub

% \presub
% \subsection{Limitations of Sketches For ErrorControl } \postsub

% including CM (CM) sketch \cite{cmsketch} and Count sketch \cite{countsketch}. These two sketches
% are two milestones in the theory of frequency estimation. A great many of followers have made a lot of contributions in many aspects, but none of them outperforms CM and Count in theoretical complexity \cite{coldfilter,Sketchingclassifiers,persistent-bf,persistentsketch,complexaggre,pyramid,ada-sketch}.

%\wyh{Define the problem.}
%\wyh{
% We define a new problem called \textit{Sensing-and-Controlling Per-flow Error at line rate}, \goal{} for short. When estimating the flow size of each flow\footnote{The flow ID is a combination of packet fields (\eg, 5-tuple).
% The size of a flow is the number packets having the flow ID.}, sensing the error is to find the Maximum Possible Error (MPE)\footnote{The maximum possible error must be non-trivial, \eg, not the estimation result itself.} of each flow's estimation. 
% For example, when the absolute error of an estimation is 10, it is desired for a sketch to report the MPE close to 10, such as 11, 13 or 16. 
% %
% We try to find the MPE instead of the exact error because exact error per flow can never be guaranteed under limited memory at line rate.
% %
% Controlling per-flow error is to control that the MPE of all flows is lower than a user-defined threshold $\Lambda$ at line rate. 
% Formally, we define the problem as follows:
%}




% In this paper, we propose \aname{} to eliminate the outlier by bilateral tight error bounds for every flow:
% When estimating the size of each flow ($f$), \aname{} can provide both a high estimate/bound ($\widehat{f}\geqslant f$) that must be greater than or equal to the flow size and a low estimate/bound ($\widetilde{f}\leqslant f$). 
% The difference between the two estimates is the Maximum Possible Error (MPE) of each estimate, \ie, $MPE=\widehat{f}-\widetilde{f}$, $MPE\geqslant |\widehat{f}-f|$ and $MPE\geqslant |\widetilde{f}-f|$.
% Further, for every flow, \aname{} controls MPE is less than or equal to $\Lambda$.
% Finally, when comparing any estimate with $T$ to identify heavy hitters, only mild misclassification may occur instead of outlier \footnote{...??explain why}.


% \ppp{Definition:}
% \ppp{}
Here we define the problem of flow size estimation with bilateral tight bounds:
Given a small error threshold $\Lambda$ defined by users, for arbitrary flow $e$ with true flow size $f_e$, the algorithm should report both an upper estimate/bound ($\widehat{f_e}\geqslant f$) and a lower estimate/bound ($\widetilde{f_e}\leqslant f_e$).
The difference of the two bounds is the Maximum Possible Error (MPE) that must be less than or equal to $\Lambda$:
\begin{align*}
        \begin{cases}
          \widetilde{f_e} \leqslant f_e\leqslant \widehat{f_e}
        \\
          MPE=\widehat{f_e}-\widetilde{f}\leqslant\Lambda
        \end{cases} \forall\ flow\ e
\end{align*}

% \ppp{Definition:}
% Given a small error threshold $\Lambda$ defined by users, for arbitrary flow $e$ with true flow size $f_e$, the algorithm should report both an estimated flow size $\widehat{f_e}$ and the corresponding Maximum Possible Error (MPE). They satisfy:

% \begin{align*}
%         \begin{cases}
%           \widehat{f_e}-MPE\leqslant f_e\leqslant \widehat{f_e}
%         \\
%           m_e\leqslant\Lambda
%         \end{cases} \forall\ flow\ e
% \end{align*}



% \presub
% \subsection{Use Cases of ErrorControl} \postsub
%\wyh{Importance of the problem.}
%\wyh{
The algorithm can produce visible error and reliable estimation, so as to improve the user's trust in sketch and accelerate the application of sketches in practices.
We give three potential use cases in the following.
%Case I is a misclassification problem due to the uncontrollable error.
%Case II is an accounting scenario that users actively sacrifice the accuracy in order to improve reliability. Case III shows that reliable error feedback can help resource allocation.
%}
% We believe that making progresses in this direction can significantly accelerate the application of sketching algorithm into practices.
% Specifically, for each flow, we find a dynamic error boundary that must be no less than the possible true error and changes as the true error changes. 
% Each flow has its own independent and tight error boundary to show its maximum possible error with 100\% confidence.
% Leveraging the error boundary, we devise new strategy to control the error of all flows under a small user-defined threshold. 
% The sensing and controlling the error will greatly improve the reliability and usability of sketch estimation results.
 


\textbf{Case I:} 
\textit{Eliminating misidentifications of heavy hitters.}
As existing sketches often significantly over-estimate a few flows, it is usual that a mice flow is misidentified as a heavy hitter. 
In anomaly detection, the false positives are false alarms of attacks \cite{hashpipe} and the false negatives result in that the operator cannot find out all anomalies. Besides, the outliers will degrade the performance of its follow-up network functions including load balancing and traffic engineering, and could further lead to network congestion and service level agreement (SLA) violation.
For example, a mice flow (\eg, a flow identified by source IP and destination IP) is often a control signal, which is more important than other flows. When a link is congested, the congestion control policy often discards a part of heavy flows to alleviate the congestion. If control signals are mistakenly considered as heavy flows and discarded, the congestion will oppositely deteriorate. In machine learning, such misidentifications can seriously hurt many models \cite{asketch,aggarwal2012event,aggarwal2010classification,yu2004false}. 


\textbf{Case II:} 
\textit{No longer sacrificing all estimates for large errors.}
In a real case, a cloud service provider uses CM sketch to monitor how much network traffic a user/service uses.
The most widely used CM sketch achieves small average error.
But it often significantly over-estimates the flow sizes of a few flows. 
In business, any seriously over-estimated flow/bill could incur legal issues, which are hardly tolerable \cite{estan2002new}.
But the service provider has no idea which flows are significantly over-estimated using existing sketches. 
Therefore, the service provider reduces the estimated results of all flows by $10\%$ before sending the bill to users.
The desired sketch should be error-sensible to avoid seriously over-estimated flows/bills so that it can protect the profit.


\textbf{Case III:} 
\textit{Providing feedback for resource allocation.}
In practice, most sketches need much less memory than the memory size recommended by the theory, because their theory can hardly take account of the flow size distribution.
Our MPE is calculated based on actual data and it will change with the real flow size distribution.
By comparing the MPE with $\Lambda$, the user of \aname{} can find smaller memory sizes to achieve the user-defined accuracy.


% \wyh{Overview. } Although recent sketches have made significant progresses in many aspects including the average accuracy \cite{huang2021toward,yang2018elastic}, throughput \cite{liu2019nitrosketch}, versatility \cite{liu2016UnivMon}, or flexibility \cite{zhang2021cocosketch, zhao2021lightguardian},  they cannot handle the problem of \textit{Sensing-and-Controlling Per-flow Error}.
% \wyh{An example of CM.}To make a concrete discussion, we take CM (CM) sketch \cite{cmsketch} as an example to show how sketches work and their limitations.
% CM is the milestone with the best theoretical result.




\presub
\subsection{Limitation of Sketches for \goal{} } \postsub

%\wyh{Overview. In network measurement, sketches can provide various statistics (\eg, heavy hitters, heavy changes, and cardinality) based on the estimation of per-flow size. 
% Working on a stream of packets, sketches provide approximate estimation for the size of every flow, \ie, the number of packets with the same flow ID. 
%Compared with traditional solutions \cite{sampling?}, sketches, a series of probabilistic data structures based on hashing, show great effectiveness in the trade-offs between accuracy, memory, and throughput.
%To make a concrete discussion, we take CM (CM) sketch \cite{cmsketch} as an example to show how sketches work, and discuss their limitations in Sensing-and-Controlling Per-flow Error from two aspects: Design and Theory.}

%Although there are a great many
%For our defined problem \goal{}, we find that no e

While existing works have made many great contributions and proposed various sketches, we find that no existing sketch can provide bilateral tight bounds.
% handles the problem of \goal{}. Further, we find they cannot address this problem. 
Below we take CM sketch as an example to explain their limitations for \goal{} from two aspects: algorithm design and error theory. 
%To make a concrete discussion, we take CM (CM) sketch \cite{cmsketch} as an example to show how sketches work, and discuss their limitations in Sensing-and-Controlling Per-flow Error from two aspects: Design and Theory.

\ppp{Limitation in Algorithm Design.} CM is the most typical work for showing the design idea of most sketches.
CM consists of $d$ arrays, $A_i[.]$, and each array has $w$ counters. For each incoming packet $e$ to be inserted, CM picks $d$ \textit{mapped counters} by independent hashing.
% CM picks $d$ counters (called \textit{mapped counters}) from the $d$ arrays by independent hashing, respectively.
The $i$-th mapped counter is $A_i[h_i(e)]$, where $h_i(\cdot)$ is the hash function.
Then, CM increments these mapped counters by one.
When querying the flow size of $e$, CM reports the minimal counter among $e$'s mapped counters as the estimation.
When other flows are mapped to the same counter of $e$ (called collision), they will add their frequency to the counter, resulting in error.
The insight is that the minimal mapped counter is the most accurate because it has the least collisions. 
However, although the minimal counter is with the least error, CM still has no way to know the error or the lower bound.
Similarly, other sketches, including Count \cite{countsketch}, CU \cite{estan2002cusketch}, Univmon \cite{liu2016UnivMon} and more \cite{zhang2021cocosketch,liu2019nitrosketch,nsdi2022HeteroSketch}, suffer from the same limitation in design.


\ppp{Limitation in Error Theory.} In theory, CM achieves the best theoretical result but we argue that its result can be further improved.
Given a stream with $N$ packets, CM needs $O\left(\frac{N}{\Lambda}\ln(\frac{1}{\delta})\right)$ space and $O\left(N\ln(\frac{1}{\delta})\right)$ time to achieve its goal: With $1-\delta$ probability, the absolute error is smaller than $\Lambda$, where $\Lambda$ is a small user-defined threshold and $\delta$ is the failure probability.
We find it may be redundant to increment multiple counters when inserting, and we try to reduce it to only once. As desired, we have improved the space and time complexity of CM. Our results are detailed in \cref{sec:math}.
The theoretical results of Count and CM are not comparable because they are based on L1-norm\footnote{The total number of packets, \ie, $\sum{f_i}$.} and L2-norm\footnote{The sum of squares of flow sizes, \ie, $\sum{f_i^2}$.}, respectively. In our theory study, we focus on L1-norm. 




% \presub
% \subsection{Sophisticated Sketches} \postsub

% A great many of sketch-based measurement solutions have emerged, including UnivMon\cite{liu2016UnivMon}, OpenSketch \cite{opensketch}, SketchLib\cite{Sketchlib?}, OnimMon...
% % Sketches \cite{Sketchlib?} have attracted extensive attention recently. 
% The most relevant work is the Elastic sketch\cite{yang2018elastic}. They aims at adapting to dynamic traffic and devise the data structure of Elastic based on the idea of election.
% Many existing work uses the idea of election, including Elastic, CoCo\cite{zhang2021cocosketch}, Majority\cite{majority????}, and SpaceSaving\cite{spacesaving}.
% Our data structure also utilizes election, but our way and goal are completely different from all of them. Specifically, the most similar Elastic uses election to find frequent flow in order to estimate them more accurately.
% In contrast, our approach is to sense the error by the number of "NO", which is not directly applicable to Elastic because Elastic clears the number of "NO" everytime a replacement happens. 
% More solutions are detailed in sec \ref{?}.


==> vldb/Experiment/app.tex <==
\presub
\subsection{Experiments on Applications} \postsub
\label{subsec:exp:app}

In this section, we apply \aname{} to six common applications: frequency estimation, top-k item detection, heavy change detection, cardinality, frequency distribution, and entropy estimation. We compare the accuracy between \aname{} and other standard algorithms for all the applications.     

\subsubsection{Frequency Estimation.}
We find that \aname{} achieves comparable accuracy with other algorithms in frequency estimation.
We conduct experiments to compare the performance of two version \aname{}es (over-estimating and under-estimating) with that of CM Sketch\cite{cmsketch}, CU Sketch\cite{cusketch} and ASketch\cite{asketch}.
We use $2$ arrays for \aname{} because it is illustrated in Section \ref{subsubsec:exp:num_ary} that $d=2$ can achieve the most balanced performance. 
% Similarly, we use $4$ arrays for CM and CU Sketch to achieve best performance.
Specifically, for ASketch, we set the size of filter to $256$ for overall balance. We vary the memory usage from $50$KB to $2$MB, using ARE and AAE to measure the performance of above five algorithms.

% should we cite here?
% how to explain we set d of CM and CU to 4?

\input{vldb/Figures/application/fe_are.tex}

% 颠倒倍率的表示表现反比关系？

\ppp{ARE vs. memory size (Figure \ref{subfig:app:fe_are:caida},\ref{subfig:app:fe_are:webpage}):} It is shown that under-estimating \aname{} can keep an extremely low ARE even with limited memory consumption. This is because that most items are infrequent, and the under-estimating sketches often offer less error than the over-estimating ones when estimating their frequencies. For over-estimating \aname{}, ARE is $1.7 \sim 2.3$ times lower than the ones of CM Sketch and ASketch in both two datasets. Over-estimating \aname{} also achieves a comparable ARE with CU Sketch. 

\ppp{AAE vs. memory size (Figure \ref{subfig:app:fe_aae:caida},\ref{subfig:app:fe_aae:webpage}):} It is shown that under-estimating \aname{} has a great performance in AAE with low memory size. Compared with CU Sketch, AAE of under-estimating \aname{} is $1.6 \sim 32.5$ times smaller when we vary the memory size from $50$KB to $1$MB. For over-estimating \aname{}, AAE is $1.8 \sim 2.9$ times lower than CM Sketch and ASketch in both two datasets. And it has a small advantage in AAE compared with CU Sketch. Moreover, a fact is that \aname{} will become more and more accurate than others as the memory size grows since the capacity of dominant item grows together, and the result in Section \ref{subsec:exp:dom_acc} shows that just a slight or even no over-estimation error for those dominant items.

% 需要对所有dominant斜体？
% 改成ARE

\subsubsection{Top-k Item Detection.} We find that \aname{} can always achieve better performance than other algorithms in top-k item detection. For this application, we conduct experiments to compare the performance of \aname{} with that of CM Heap, ASketch, and SpaceSaving\cite{spacesaving}. CM Heap consists of a simple CM Sketch and an independent min-heap to record most frequent items, where we fix the heap size to 10KB. For \aname{}, we use the over-estimating one since it has lower estimation error for frequent items. We vary the memory usage and calculate the PR and ARE for top 200 items.
% PR and ARE are used to evaluate the accuracy of the task.
% It is unnecessary to compare the RR, because applied algorithms all report exactly $k$ items for a top-k query.
% 需要这句话吗？

\input{vldb/Figures/application/topk.tex}

\ppp{PR vs. memory size (Figure \ref{subfig:app:topk_pr:caida},\ref{subfig:app:topk_pr:webpage}):} For the CAIDA dataset, when we only use 20KB memory, the PRs of CM Sketch, ASketch and SpaceSaving are $38\%$, $39\%$ and $42\%$ respectively, while that of \aname{} is $92.5\%$. When the memory usage is up to 60KB, \aname{} offers almost $100\%$ PR. For the Web Page dataset and with 20KB memory consumption, the PRs of CM Sketch, ASketch and SpaceSaving are $36\%$, $39.5\%$ and $62\%$ respectively, while that of \aname{} is $98\%$.

\ppp{AAE vs. memory size (Figure \ref{subfig:app:topk_aae:caida},\ref{subfig:app:topk_aae:webpage}):} For the CAIDA dataset, the AAE of \aname{} is $39 \sim 63$ times smaller than the one of CM Sketch, $9 \sim 51$ times smaller than the one of ASketch and $11 \sim 29$ times smaller than the one of SpaceSaving.
For the Web Page dataset, the AAE of \aname{} is $16162 \sim 65651$ times smaller than the one of CM Sketch, $1621 \sim 12494$ times smaller than the one of ASketch and $6 \sim 6659$ times smaller than the one of SpaceSaving.

% 数字不用这么具体

\subsubsection{Heavy Change Detection.} We find that \aname{} can offer higher accuracy than the other three algorithms in heavy change detection. Heavy change detection is to find items with relatively big frequency change between two different time periods. Hence we separate the whole stream into two parts with the same number of items, representing two adjacent time periods. We compare \aname{} with CM Heap, ASketch, and SpaceSaving, the settings of parameters are as the same as top-k item detection. We use F1-score and ARE to measure the performance.

\input{vldb/Figures/application/hc.tex}

\ppp{F1 score vs. memory size (Figure \ref{subfig:app:hc_f1:caida},\ref{subfig:app:hc_f1:webpage}):} For the CAIDA dataset, \aname{} achieves $0.908$ F1 score when the memory usage is up to 70KB. However, the F1 scores of CM Heap, ASketch and SpaceSaving are $0.55$, $0.522$ and $0.523$ respectively with the same memory usage. For the Web Page dataset, \aname{} achieves $0.907$ F1 score when the memory size is 40KB, while the F1 scores of CM Heap, ASketch and SpaceSaving are $0.464$, $0.406$ and $0.522$, respectively. 

% for the three tasks below, we use an auxiliary ... ? 

\ppp{AAE vs. memory size (Figure \ref{subfig:app:hc_aae:caida},\ref{subfig:app:hc_aae:webpage}):} For the CAIDA dataset, AAE of \aname{} is $ 2.0 \sim 5.0$ times smaller than that of CM Heap and ASketch, and is $3.1 \sim 7.7$ times smaller than that of SpaceSaving. For the Web Page dataset, AAE of \aname{} is extremely low even with tight memory, $13.2 \sim 23.7$ and $6.1 \sim 39.9$ times smaller than that of ASketch and CM Heap.

\subsubsection{Real time Cardinality \& Frequency Distribution \& Entropy Estimation.}
In these three applications, we compare \aname{} with CM Sketch and CU Sketch, and implement auxiliary arrays for all algorithms to record the real time estimation of the frequency distribution.

\input{vldb/Figures/application/cd_fd_etp}
% \input{vldb/Figures/application/cd.tex}

\ppp{Cardinality Estimation (Figure \ref{subfig:app:cd}):} We find that \aname{} achieves comparable accuracy with CM Sketch and CU Sketch in cardinality estimation. Notice that with high memory consumption, benefitted by ID field, \aname{} performs slightly better than others.

% \input{vldb/Figures/application/fd.tex}

\ppp{Frequency Distribution Estimation (Figure \ref{subfig:app:fd}):} We find that \aname{} performs more accurate slightly than CM Sketch and CU Sketch in frequency distribution estimation. When the memory consumption is 2MB, WMRE of \aname{} is about $1.41$ times lower than CM Sketch and $1.40$ times lower than CU Sketch.

%For the CAIDA dataset, WMRE of \aname{} is about $0.41$ times lower than CM sketch and $0.40$ times lower than CU sketch when the memory consumption is 2MB.
% For the Web Page dataset, WMRE of \aname{} is about $0.72$ times lower than CM sketch and $0.70$ times lower than CU sketch when the memory consumption is 2MB. 


% \input{vldb/Figures/application/etp.tex}

\ppp{Entropy Estimation (Figure\ref{subfig:app:etp_real},\ref{subfig:app:etp_re}):}
% \subsubsection{Entropy Estimation.}
We find that \aname{} can offer a relatively accurate estimation for real-time entropy. To show entropy change clearly, we select three stream segments of the CAIDA dataset and combine them as the integral input stream. Each segment is not adjacent to any of the others and consists of exactly 80K items.
%We compare \aname{} with CM Sketch and CU Sketch, both implement an array to record frequency distribution and update global entropy in real-time. The metric RE is used to measure the accuracy of the estimation.

Figure \ref{subfig:app:etp_real} shows that \aname{} gives an estimation closer than real entropy compared with CM Sketch and CU Sketch when the memory consumption is 1MB. As shown in Figure \ref{subfig:app:etp_re}, RE of \aname{} is about $1.86 \times 10^{-4}$, while the ones of CM Sketch and CU Sketch are $12.44 \times 10^{-4}$, $4.16 \times 10^{-4}$ respectively, when the memory consumption is 1MB.
%As the memory size varied, \aname{} achieves $1.6 \sim 34.8$ times smaller error than CM sketch and $1.3 \sim 28.2$ times smaller error than CU sketch.

% \subsubsection{Frequency Distribution Estimation.} For this task, we conduct experiments to compare with CM Sketch and CU Sketch. As the same as entropy estimation, we use an auxiliary array to record the real-time estimation of the frequency distribution. We vary the memory size from 50KB to 2MB to show the change of accuracy. 

% \input{vldb/Figures/application/fd.tex}

% \ppp{WMRE vs. memory size (Figure \ref{subfig:app:fd:caida},\ref{subfig:app:fd:webpage}):} We find that \aname{} performs better than CM-sketch and CU-sketch on the metric WMRE. For the CAIDA dataset, WMRE of \aname{} is about 4.5 times lower than CM sketch and 4.2 times lower than CU sketch when the memory size is 1MB. For the Web Page dataset, WMRE of \aname{} is about 5.5 times lower than CM sketch and 4.7 times lower than CU sketch when the memory size is 1MB. 

==> vldb/Experiment/app_V3.tex <==
\presub
\subsection{Experiments on \aname{}} \postsub
\label{subsec:exp:app}
In this section, we apply \aname{} to frequency estimation and compare \aname{} with prior algorithms using two metrics, the number of outliers and average error.

%In this section, we apply \aname{} to two applications with different orientations: frequency estimation and error guarantee. 
%We compare the accuracy between \aname{} and other standard algorithms for these applications.
%We compare the accuracy between \aname{}es in different threshold $\Lambda$ and other standard algorithms for these applications.     

\subsubsection{\# Outliers.}
\label{subsubsec:exp:range}
We find that \aname{} achieves the best performance compared with other algorithms in metric the number of outliers.
We vary the threshold $\Lambda$ and conduct experiments to compare the performance of \aname{} ("Ours" in the legends) with that of CM Sketch \cite{cmsketch}, CU Sketch \cite{cusketch}, Space-Saving (SS) \cite{spacesaving}, ElasticSketch (Elastic) \cite{yang2018elastic} and CocoSketch (Coco) \cite{zhang2021cocosketch}. \whb{!!!cite the appendix talking about parameters} For \aname{}, according to the study in Section \ref{subsec:exp:nature}, we set $R_w$ to 2 and $R_\lambda$ to 2.5 as default. For CM Sketch and CU Sketch, we provide fast (CM\_fast/CU\_fast) and accurate (CM\_acc/CU\_acc) two versions, implementing 3 and 16 arrays respectively.
% Considered the trade-off between processing speed and accuracy, we use $3$ arrays for CM and CU Sketch to achieve better performance.
% Specifically for Augmented Sketch, we set the filter size to $256$ for overall balance.
Specifically for Elastic Sketch, the memory ratio between the light part and the heavy part is fixed to 3.
And for CocoSketch, we set the number of arrays $d$ to 2.
% And for HeavyGuardian, we set $\lambda_h$ to 8, $\lambda_l$ to 64 and $b$ to 1.08.
% We use the number of fails as the metric to measure the performance.
% 更改metric

\input{vldb/Figures/app_new2/outlier_eps}

\ppp{Impact of Threshold $\Lambda$ (Figure \ref{subfig:app:range5:caida},\ref{subfig:app:range10:caida},\ref{subfig:app:range25:caida},\ref{subfig:app:range50:caida}):}
We first choose IP Trace as the experimental dataset and vary the threshold $\Lambda$.
As the figures show, \aname{} takes the lead position regardless of $\Lambda$. For $\Lambda$=$25$, \aname{} achieves zero outlier with only 0.76 MB memory, while Space-Saving requires nearly 1.98 MB memory.
% HeavyGuardian performs as well as \aname{} in low memory, yet it cannot offer a stable report as \aname{} does when memory grows.
For CM Sketch (fast), CU Sketch (fast), ElasticSketch, and CocoSketch, there are still over 100 outliers when memory size is 4 MB.
Compared with the fast versions, despite the fact that CM Sketch (accurate) and CU Sketch (accurate) perform worse with insufficient memory, the number of outliers drops down rapidly when memory grows. However, the accurate versions also suffer low throughput.

\input{vldb/Figures/app_new2/outlier_dataset}

\ppp{Impact of Dataset (Figure \ref{subfig:app:range25:caida},\ref{subfig:app:range25:webpage},\ref{subfig:app:range25:kosarak},\ref{subfig:app:range25:syn003},\ref{subfig:app:range25:syn030}):} We fix $\Lambda$ to 25 and change the dataset. The figures illustrate that \aname{} has the least memory requirement regardless of the dataset. Space-Saving requires 2 $\sim$ 4 times more memory to achieve zero outlier than \aname{}. % HeavyGuardian achieves stable performance on Web Stream and Click Stream datasets, because there are relatively less infrequent items than IP Trace. However, it still requires comparable amount of memory as Space-Saving.
CU Sketch(accurate) requires 4 $\sim$ 8 times more memory and performs unstably in different datasets.
For synthetic dataset with skewness=0.3, no algorithm achieves zero outlier within 4MB memory, while the number of outliers of \aname{} is over 100 times less than others. 

% 柱状图

% \input{vldb/Figures/app_new/range_mem}
\input{vldb/Figures/app_new2/outlier_minmem}

\ppp{Memory Consumption (Figure \ref{fig:app:outlier_minmem}):} We further explore the precise minimum memory consumption to achieve zero outlier for all algorithms, $\Lambda$ is fixed to 25 and experiments are conducted on different datasets. CM Sketch (fast), CU Sketch (fast) and CocoSketch cannot achieve zero outlier within 10MB memory. For the IP Trace dataset, memory consumption of \aname{} is 0.77MB, about 7.33, 3.25, 2.43, 11.25 times less than CM Sketch (accurate), CU Sketch (accurate), Space-Saving, and ElasticSketch respectively. For the Web Stream dataset, memory consumption of \aname{} is 0.44MB, about 7.79, 3.90, 2.59, 7.79 times less than them, respectively. Besides, CM Sketch, CU Sketch and ElasticSketch usually require more memory than the minimum value, otherwise there is still a high probability of outliers.

\subsubsection{Average Error.}
\label{subsubsec:exp:fe}
We find that \aname{} achieves comparable accuracy than other algorithms in average error. We conduct experiments to compare the performance of \aname{} with that of above competitors. 
% except HeavyGuardian, %because HeavyGuardian is bilateral-estimating while others are all over-estimating.
% because its estimation is neither one-side error nor unbiased estimation.
% Noticed that competitors are all over-estimating, while \aname{} may return an under-estimated value when all mapped buckets are locked. For fairness, we set the error threshold of last layer $\lambda_d$ to positive infinite specially, so that returned value is always an over-estimation.
$\Lambda$ of \aname{} is derived from Formula \ref{formula:setLambda}.
% , and $R_w$ is set to 6 for more precise estimation. 
For CM Sketch and CU Sketch, we only compare \aname{} with the 3 arrays versions because more arrays cannot decrease the average error significantly.
Other settings of algorithms are as the same as Section \ref{subsubsec:exp:range}.
% It is had to say that though we still call the CM Sketch and CU Sketch with 16 arrays the accurate version, they are not accurate at average error actually.
We vary the memory usage from $200$KB to $4$MB, using ARE and AAE to measure the accuracy of above algorithms.
% We use $2$ arrays for \aname{} because it is illustrated in Section \ref{subsubsec:exp:num_ary} that $d=2$ can achieve the most balanced performance. 


% how to explain we set d of CM and CU to 4?
% 注明frequency会随着R_w的增加而增加，这个task不是mvs的优化目标

% \input{vldb/Figures/app_new/freq_aae}
\input{vldb/Figures/app_new2/avg_err}

% 颠倒倍率的表示表现反比关系？

\ppp{ARE vs. Memory Size (Figure \ref{subfig:app:fe_are:caida}, \ref{subfig:app:fe_are:webpage}):}
% It is shown that under-estimating \aname{} can keep an extremely low ARE even with limited memory consumption. This is because that most items are infrequent, and the under-estimating sketches often offer less error than the over-estimating ones when estimating their frequencies. 
It is shown that when memory size grows to 4MB, \aname{} achieves a comparable ARE with ElasticSketch, and is $2.62$ times lower than CU Sketch, $4.35$ times lower than CM Sketch, $7.37 \sim 30.37$ times lower than others in two datasets.
Note that ARE of \aname{} is about 2 times higher than CU Sketch when memory size is 200KB, because the derived $\Lambda$ is too large and the bottom layers are totally wasted. Under such a circumstance, we recommend to increase $R_w$ or decrease $d$ appropriately to enlarge the size of top layers.

% Indeed, \aname{} with higher $R_w$ can get better performance, but also results in more outliers. For the trade-off, extreme parameters are not recommended in common use.

\ppp{AAE vs. Memory Size (Figure \ref{subfig:app:fe_aae:caida}, \ref{subfig:app:fe_aae:webpage}):}
It is shown that \aname{} also has a comparable AAE with ElasticSketch and CU Sketch，and is $1.96$ times lower than CM Sketch, $4.25$ times lower than CocoSketch, $11.07$ times lower than Space-Saving in two datasets when memory size is up to 4MB.
% The increasing speed of accuracy slows down when memory size grows high enough for \aname{}.

% The fact is that most of the items are recorded in the top layers of \aname{}, and the remaining layers are totally wasted. Under such a circumstance, we can increase $R_w$ appropriately to enlarge the size of top layers.

% figure two datasets & different threshold
% 高threshold: 
% 低threshold: 最快到达0且稳定
% 不同dataset的相对表现无明显差别

% 需要对所有dominant斜体？
% 改成ARE

% \subsubsection{Top-k Item Detection.} We find that \aname{} can always achieve better performance than other algorithms in top-k item detection. For this application, we conduct experiments to compare the performance of \aname{} with that of CM Heap, Augmented Sketch, and SpaceSaving\cite{spacesaving}. CM Heap consists of a simple CM Sketch and an independent min-heap to record most frequent items, where we fix the heap size to 10KB. For \aname{}, we use the over-estimating one since it has lower estimation error for frequent items. We vary the memory usage and calculate the PR and ARE for top 200 items.
% % PR and ARE are used to evaluate the accuracy of the task.
% % It is unnecessary to compare the RR, because applied algorithms all report exactly $k$ items for a top-k query.
% % 需要这句话吗？

% \input{vldb/Figures/application/topk.tex}

% \ppp{PR vs. memory size (Figure \ref{subfig:app:topk_pr:caida},\ref{subfig:app:topk_pr:webpage}):} For the CAIDA dataset, when we only use 20KB memory, the PRs of CM Sketch, Augmented Sketch and SpaceSaving are $38\%$, $39\%$ and $42\%$ respectively, while that of \aname{} is $92.5\%$. When the memory usage is up to 60KB, \aname{} offers almost $100\%$ PR. For the Web Page dataset and with 20KB memory consumption, the PRs of CM Sketch, Augmented Sketch and SpaceSaving are $36\%$, $39.5\%$ and $62\%$ respectively, while that of \aname{} is $98\%$.

% \ppp{AAE vs. memory size (Figure \ref{subfig:app:topk_aae:caida},\ref{subfig:app:topk_aae:webpage}):} For the CAIDA dataset, the AAE of \aname{} is $39 \sim 63$ times smaller than the one of CM Sketch, $9 \sim 51$ times smaller than the one of Augmented Sketch and $11 \sim 29$ times smaller than the one of SpaceSaving.
% For the Web Page dataset, the AAE of \aname{} is $16162 \sim 65651$ times smaller than the one of CM Sketch, $1621 \sim 12494$ times smaller than the one of Augmented Sketch and $6 \sim 6659$ times smaller than the one of SpaceSaving.

% % 数字不用这么具体

% \subsubsection{Heavy Change Detection.} We find that \aname{} can offer higher accuracy than the other three algorithms in heavy change detection. Heavy change detection is to find items with relatively big frequency change between two different time periods. Hence we separate the whole stream into two parts with the same number of items, representing two adjacent time periods. We compare \aname{} with CM Heap, Augmented Sketch, and SpaceSaving, the settings of parameters are as the same as top-k item detection. We use F1-score and ARE to measure the performance.

% \input{vldb/Figures/application/hc.tex}

% \ppp{F1 score vs. memory size (Figure \ref{subfig:app:hc_f1:caida},\ref{subfig:app:hc_f1:webpage}):} For the CAIDA dataset, \aname{} achieves $0.908$ F1 score when the memory usage is up to 70KB. However, the F1 scores of CM Heap, Augmented Sketch and SpaceSaving are $0.55$, $0.522$ and $0.523$ respectively with the same memory usage. For the Web Page dataset, \aname{} achieves $0.907$ F1 score when the memory size is 40KB, while the F1 scores of CM Heap, Augmented Sketch and SpaceSaving are $0.464$, $0.406$ and $0.522$, respectively. 

% % for the three tasks below, we use an auxiliary ... ? 

% \ppp{AAE vs. memory size (Figure \ref{subfig:app:hc_aae:caida},\ref{subfig:app:hc_aae:webpage}):} For the CAIDA dataset, AAE of \aname{} is $ 2.0 \sim 5.0$ times smaller than that of CM Heap and Augmented Sketch, and is $3.1 \sim 7.7$ times smaller than that of SpaceSaving. For the Web Page dataset, AAE of \aname{} is extremely low even with tight memory, $13.2 \sim 23.7$ and $6.1 \sim 39.9$ times smaller than that of Augmented Sketch and CM Heap.

% \subsubsection{Real time Cardinality \& Frequency Distribution \& Entropy Estimation.}
% In these three applications, we compare \aname{} with CM Sketch and CU Sketch, and implement auxiliary arrays for all algorithms to record the real time estimation of the frequency distribution.

% \input{vldb/Figures/application/cd_fd_etp}
% % \input{vldb/Figures/application/cd.tex}

% \ppp{Cardinality Estimation (Figure \ref{subfig:app:cd}):} We find that \aname{} achieves comparable accuracy with CM Sketch and CU Sketch in cardinality estimation. Notice that with high memory consumption, benefitted by ID field, \aname{} performs slightly better than others.

% % \input{vldb/Figures/application/fd.tex}

% \ppp{Frequency Distribution Estimation (Figure \ref{subfig:app:fd}):} We find that \aname{} performs more accurate slightly than CM Sketch and CU Sketch in frequency distribution estimation. When the memory consumption is 2MB, WMRE of \aname{} is about $1.41$ times lower than CM Sketch and $1.40$ times lower than CU Sketch.

% %For the CAIDA dataset, WMRE of \aname{} is about $0.41$ times lower than CM sketch and $0.40$ times lower than CU sketch when the memory consumption is 2MB.
% % For the Web Page dataset, WMRE of \aname{} is about $0.72$ times lower than CM sketch and $0.70$ times lower than CU sketch when the memory consumption is 2MB. 


% % \input{vldb/Figures/application/etp.tex}

% \ppp{Entropy Estimation (Figure\ref{subfig:app:etp_real},\ref{subfig:app:etp_re}):}
% % \subsubsection{Entropy Estimation.}
% We find that \aname{} can offer a relatively accurate estimation for real-time entropy. To show entropy change clearly, we select three stream segments of the CAIDA dataset and combine them as the integral input stream. Each segment is not adjacent to any of the others and consists of exactly 80K items.
% %We compare \aname{} with CM Sketch and CU Sketch, both implement an array to record frequency distribution and update global entropy in real-time. The metric RE is used to measure the accuracy of the estimation.

% Figure \ref{subfig:app:etp_real} shows that \aname{} gives an estimation closer than real entropy compared with CM Sketch and CU Sketch when the memory consumption is 1MB. As shown in Figure \ref{subfig:app:etp_re}, RE of \aname{} is about $1.86 \times 10^{-4}$, while the ones of CM Sketch and CU Sketch are $12.44 \times 10^{-4}$, $4.16 \times 10^{-4}$ respectively, when the memory consumption is 1MB.
% %As the memory size varied, \aname{} achieves $1.6 \sim 34.8$ times smaller error than CM sketch and $1.3 \sim 28.2$ times smaller error than CU sketch.

% % \subsubsection{Frequency Distribution Estimation.} For this task, we conduct experiments to compare with CM Sketch and CU Sketch. As the same as entropy estimation, we use an auxiliary array to record the real-time estimation of the frequency distribution. We vary the memory size from 50KB to 2MB to show the change of accuracy. 

% % \input{vldb/Figures/application/fd.tex}

% % \ppp{WMRE vs. memory size (Figure \ref{subfig:app:fd:caida},\ref{subfig:app:fd:webpage}):} We find that \aname{} performs better than CM-sketch and CU-sketch on the metric WMRE. For the CAIDA dataset, WMRE of \aname{} is about 4.5 times lower than CM sketch and 4.2 times lower than CU sketch when the memory size is 1MB. For the Web Page dataset, WMRE of \aname{} is about 5.5 times lower than CM sketch and 4.7 times lower than CU sketch when the memory size is 1MB. 



% \subsubsection{Performance in P4 testbed.}
% We also carried out experiments on 1M flow packets in the hardware testbed. On the P4 device, we tested the accuracy of \aname{} based on memory size changes, and measured its time under the network-wide performance.
% As shown in Figure\ref{}, we can see that the AAE and ARE of \aname{} perform well in the case of sufficient memory, and rise in an approximately linear proportion in the case of insufficient memory. In addition, we find that outliers begin to appear when the memory is compressed to only a quarter.
% In Figure\ref{}, we can see that in the environment of maximum memory, it takes about one second to synchronize the data plane, and the time decreases linearly with the decrease of memory. In addition, the time required for network transmission is much less than that required for synchronization. 


==> vldb/Experiment/app_new.tex <==
\presub
\subsection{Comparison on Accuracy} \postsub
\label{subsec:exp:app}
In this section, we apply \aname{} to frequency estimation and compare \aname{} with prior algorithms using two metrics, the number of outliers and average error.

%In this section, we apply \aname{} to two applications with different orientations: frequency estimation and error guarantee. 
%We compare the accuracy between \aname{} and other standard algorithms for these applications.
%We compare the accuracy between \aname{}es in different threshold $\Lambda$ and other standard algorithms for these applications.     

\subsubsection{\# Outliers.}
\label{subsubsec:exp:range}
We find that \aname{} achieves the best performance compared with other algorithms in metric the number of outliers.
We vary the threshold $\Lambda$ and conduct experiments to compare the performance of \aname{} with that of CM Sketch \cite{cmsketch}, CU Sketch \cite{cusketch}, Augmented Sketch (AS) \cite{asketch}, Space-Saving (SS) \cite{spacesaving} and HeavyGuardian (HG) \cite{yang2018heavyguardian}. For \aname{}, according to the study in Section \ref{subsec:exp:nature}, we set $R_w$ to 2 and $R_\lambda$ to 2.5 as default. For CM Sketch and CU Sketch, we provide fast (CM\_fast/CU\_fast) and accurate (CM\_acc/CU\_acc) two versions, implementing 3 and 16 arrays respectively.
% Considered the trade-off between processing speed and accuracy, we use $3$ arrays for CM and CU Sketch to achieve better performance.
Specifically for Augmented Sketch, we set the filter size to $256$ for overall balance. And for HeavyGuardian, we set $\lambda_h$ to 8, $\lambda_l$ to 64 and $b$ to 1.08.
% We use the number of fails as the metric to measure the performance.
% 更改metric

\input{vldb/Figures/app_new/range_eps}

\ppp{Impact of Threshold $\Lambda$ (Figure \ref{subfig:app:range5:caida},\ref{subfig:app:range10:caida},\ref{subfig:app:range25:caida},\ref{subfig:app:range50:caida}):} We first choose IP Trace as the experimental dataset and vary the threshold $\Lambda$. As the figures show, \aname{} takes the lead position regardless of $\Lambda$. For $\Lambda$=$25$, \aname{} achieves zero outlier with only 1.14 MB memory, while Space-Saving requires nearly 2.48 MB memory. HeavyGuardian performs as well as \aname{} in low memory, yet it cannot offer a stable report as \aname{} does when memory grows. For CM Sketch (fast), CU Sketch (fast) and Augmented Sketch, there are still over 100 outliers when memory size is 4 MB. Compared with the fast versions, despite the fact that CM Sketch (accurate) and CU Sketch (accurate) perform worse with insufficient memory, the number of outliers drops down rapidly when memory grows. However, the accurate versions also suffer low throughput.

\input{vldb/Figures/app_new/range_dataset}

\ppp{Impact of Dataset (Figure \ref{subfig:app:range25:caida},\ref{subfig:app:range25:webpage},\ref{subfig:app:range25:kosarak},\ref{subfig:app:range25:syn003},\ref{subfig:app:range25:syn030}):} We fix $\Lambda$ to 25 and change the dataset. The figures illustrate that \aname{} has the least memory requirement regardless of the dataset. Space-Saving requires 2 $\sim$ 4 times more memory to achieve zero outlier than \aname{}. HeavyGuardian achieves stable performance on Web Stream and Click Stream datasets, because there are relatively less infrequent items than IP Trace. However, it still requires comparable amount of memory as Space-Saving. For synthetic dataset with skewness=0.3, no algorithm achieves zero outlier within 4MB memory, while the number of outliers of \aname{} is over 100 times less than others. 

% 柱状图

\input{vldb/Figures/app_new/range_mem}

\ppp{Memory Consumption (Figure \ref{fig:app:range_mem}):} We further explore the precise minimum memory consumption to achieve zero outlier for all algorithms, $\Lambda$ is fixed to 25 and experiments are conducted on different datasets. CM Sketch (fast), CU Sketch (fast) and Augmented Sketch cannot achieve zero outlier within 10MB memory. For the IP Trace dataset, memory consumption of \aname{} is 1.04MB, about 6.17, 3.38, 2.24, 2.23 times less than CM Sketch (accurate), CU Sketch (accurate), Space-Saving, and HeavyGuardian respectively. For the Web Stream dataset, memory consumption of \aname{} is 0.44MB, about 5.68, 3.94, 2.57, 2.13 times less than them, respectively. Besides, CM Sketch, CU Sketch and HeavyGuardian usually require more memory than the minimum value, otherwise there is still a high probability of outliers.

\subsubsection{Average Error.}
\label{subsubsec:exp:fe}
We find that \aname{} achieves comparable accuracy than other algorithms in average error. We conduct experiments to compare the performance of \aname{} with that of above competitors except HeavyGuardian, %because HeavyGuardian is bilateral-estimating while others are all over-estimating.
because its estimation is neither one-side error nor unbiased estimation.
% Noticed that competitors are all over-estimating, while \aname{} may return an under-estimated value when all mapped buckets are locked. For fairness, we set the error threshold of last layer $\lambda_d$ to positive infinite specially, so that returned value is always an over-estimation.
$\Lambda$ of \aname{} is derived from Formula \ref{formula:setLambda}, and $R_w$ is set to 6 for more precise estimation. 
Other settings of algorithms are as the same as Section \ref{subsubsec:exp:range}.
It is worth nothing that though we still call the CM Sketch and CU Sketch with 16 arrays the accurate version, they are not accurate at average error actually.
We vary the memory usage from $200$KB to $4$MB, using ARE and AAE to measure the accuracy of above algorithms.
% We use $2$ arrays for \aname{} because it is illustrated in Section \ref{subsubsec:exp:num_ary} that $d=2$ can achieve the most balanced performance. 


% how to explain we set d of CM and CU to 4?
% 注明frequency会随着R_w的增加而增加，这个task不是mvs的优化目标

\input{vldb/Figures/app_new/freq_aae}

% 颠倒倍率的表示表现反比关系？

\ppp{ARE vs. Memory Size (Figure \ref{subfig:app:fe_are:caida}, \ref{subfig:app:fe_are:webpage}):}
% It is shown that under-estimating \aname{} can keep an extremely low ARE even with limited memory consumption. This is because that most items are infrequent, and the under-estimating sketches often offer less error than the over-estimating ones when estimating their frequencies. 
It is shown that ARE of \aname{} achieves a comparable ARE with CU Sketch (fast), and is $1.38 \sim 1.83$ times lower than CM Sketch (fast), $1.40 \sim 2.15$ times lower than Augmented, $2.52 \sim 8.97$ times lower than others in two datasets. Indeed, \aname{} with higher $R_w$ can get better performance, but also results in more outliers. For the trade-off, extreme parameters are not recommended in common use.

\ppp{AAE vs. Memory Size (Figure \ref{subfig:app:fe_aae:caida}, \ref{subfig:app:fe_aae:webpage}):}
It is shown that AAE of \aname{} also has a comparable AAE with CU Sketch (fast)，and is $1.39 \sim 1.88$ times lower than CM Sketch (fast), $1.41 \sim 2.31$ times lower than Augmented Sketch, $2.17 \sim 9.01$ times lower than others in two datasets. The increasing speed of accuracy slows down when memory size grows high enough for \aname{}. The fact is that most of the items are recorded in the top layers of \aname{}, and the remaining layers are totally wasted. Under such a circumstance, we can increase $R_w$ appropriately to enlarge the size of top layers.

% figure two datasets & different threshold
% 高threshold: 
% 低threshold: 最快到达0且稳定
% 不同dataset的相对表现无明显差别

% 需要对所有dominant斜体？
% 改成ARE

% \subsubsection{Top-k Item Detection.} We find that \aname{} can always achieve better performance than other algorithms in top-k item detection. For this application, we conduct experiments to compare the performance of \aname{} with that of CM Heap, Augmented Sketch, and SpaceSaving\cite{spacesaving}. CM Heap consists of a simple CM Sketch and an independent min-heap to record most frequent items, where we fix the heap size to 10KB. For \aname{}, we use the over-estimating one since it has lower estimation error for frequent items. We vary the memory usage and calculate the PR and ARE for top 200 items.
% % PR and ARE are used to evaluate the accuracy of the task.
% % It is unnecessary to compare the RR, because applied algorithms all report exactly $k$ items for a top-k query.
% % 需要这句话吗？

% \input{vldb/Figures/application/topk.tex}

% \ppp{PR vs. memory size (Figure \ref{subfig:app:topk_pr:caida},\ref{subfig:app:topk_pr:webpage}):} For the CAIDA dataset, when we only use 20KB memory, the PRs of CM Sketch, Augmented Sketch and SpaceSaving are $38\%$, $39\%$ and $42\%$ respectively, while that of \aname{} is $92.5\%$. When the memory usage is up to 60KB, \aname{} offers almost $100\%$ PR. For the Web Page dataset and with 20KB memory consumption, the PRs of CM Sketch, Augmented Sketch and SpaceSaving are $36\%$, $39.5\%$ and $62\%$ respectively, while that of \aname{} is $98\%$.

% \ppp{AAE vs. memory size (Figure \ref{subfig:app:topk_aae:caida},\ref{subfig:app:topk_aae:webpage}):} For the CAIDA dataset, the AAE of \aname{} is $39 \sim 63$ times smaller than the one of CM Sketch, $9 \sim 51$ times smaller than the one of Augmented Sketch and $11 \sim 29$ times smaller than the one of SpaceSaving.
% For the Web Page dataset, the AAE of \aname{} is $16162 \sim 65651$ times smaller than the one of CM Sketch, $1621 \sim 12494$ times smaller than the one of Augmented Sketch and $6 \sim 6659$ times smaller than the one of SpaceSaving.

% % 数字不用这么具体

% \subsubsection{Heavy Change Detection.} We find that \aname{} can offer higher accuracy than the other three algorithms in heavy change detection. Heavy change detection is to find items with relatively big frequency change between two different time periods. Hence we separate the whole stream into two parts with the same number of items, representing two adjacent time periods. We compare \aname{} with CM Heap, Augmented Sketch, and SpaceSaving, the settings of parameters are as the same as top-k item detection. We use F1-score and ARE to measure the performance.

% \input{vldb/Figures/application/hc.tex}

% \ppp{F1 score vs. memory size (Figure \ref{subfig:app:hc_f1:caida},\ref{subfig:app:hc_f1:webpage}):} For the CAIDA dataset, \aname{} achieves $0.908$ F1 score when the memory usage is up to 70KB. However, the F1 scores of CM Heap, Augmented Sketch and SpaceSaving are $0.55$, $0.522$ and $0.523$ respectively with the same memory usage. For the Web Page dataset, \aname{} achieves $0.907$ F1 score when the memory size is 40KB, while the F1 scores of CM Heap, Augmented Sketch and SpaceSaving are $0.464$, $0.406$ and $0.522$, respectively. 

% % for the three tasks below, we use an auxiliary ... ? 

% \ppp{AAE vs. memory size (Figure \ref{subfig:app:hc_aae:caida},\ref{subfig:app:hc_aae:webpage}):} For the CAIDA dataset, AAE of \aname{} is $ 2.0 \sim 5.0$ times smaller than that of CM Heap and Augmented Sketch, and is $3.1 \sim 7.7$ times smaller than that of SpaceSaving. For the Web Page dataset, AAE of \aname{} is extremely low even with tight memory, $13.2 \sim 23.7$ and $6.1 \sim 39.9$ times smaller than that of Augmented Sketch and CM Heap.

% \subsubsection{Real time Cardinality \& Frequency Distribution \& Entropy Estimation.}
% In these three applications, we compare \aname{} with CM Sketch and CU Sketch, and implement auxiliary arrays for all algorithms to record the real time estimation of the frequency distribution.

% \input{vldb/Figures/application/cd_fd_etp}
% % \input{vldb/Figures/application/cd.tex}

% \ppp{Cardinality Estimation (Figure \ref{subfig:app:cd}):} We find that \aname{} achieves comparable accuracy with CM Sketch and CU Sketch in cardinality estimation. Notice that with high memory consumption, benefitted by ID field, \aname{} performs slightly better than others.

% % \input{vldb/Figures/application/fd.tex}

% \ppp{Frequency Distribution Estimation (Figure \ref{subfig:app:fd}):} We find that \aname{} performs more accurate slightly than CM Sketch and CU Sketch in frequency distribution estimation. When the memory consumption is 2MB, WMRE of \aname{} is about $1.41$ times lower than CM Sketch and $1.40$ times lower than CU Sketch.

% %For the CAIDA dataset, WMRE of \aname{} is about $0.41$ times lower than CM sketch and $0.40$ times lower than CU sketch when the memory consumption is 2MB.
% % For the Web Page dataset, WMRE of \aname{} is about $0.72$ times lower than CM sketch and $0.70$ times lower than CU sketch when the memory consumption is 2MB. 


% % \input{vldb/Figures/application/etp.tex}

% \ppp{Entropy Estimation (Figure\ref{subfig:app:etp_real},\ref{subfig:app:etp_re}):}
% % \subsubsection{Entropy Estimation.}
% We find that \aname{} can offer a relatively accurate estimation for real-time entropy. To show entropy change clearly, we select three stream segments of the CAIDA dataset and combine them as the integral input stream. Each segment is not adjacent to any of the others and consists of exactly 80K items.
% %We compare \aname{} with CM Sketch and CU Sketch, both implement an array to record frequency distribution and update global entropy in real-time. The metric RE is used to measure the accuracy of the estimation.

% Figure \ref{subfig:app:etp_real} shows that \aname{} gives an estimation closer than real entropy compared with CM Sketch and CU Sketch when the memory consumption is 1MB. As shown in Figure \ref{subfig:app:etp_re}, RE of \aname{} is about $1.86 \times 10^{-4}$, while the ones of CM Sketch and CU Sketch are $12.44 \times 10^{-4}$, $4.16 \times 10^{-4}$ respectively, when the memory consumption is 1MB.
% %As the memory size varied, \aname{} achieves $1.6 \sim 34.8$ times smaller error than CM sketch and $1.3 \sim 28.2$ times smaller error than CU sketch.

% % \subsubsection{Frequency Distribution Estimation.} For this task, we conduct experiments to compare with CM Sketch and CU Sketch. As the same as entropy estimation, we use an auxiliary array to record the real-time estimation of the frequency distribution. We vary the memory size from 50KB to 2MB to show the change of accuracy. 

% % \input{vldb/Figures/application/fd.tex}

% % \ppp{WMRE vs. memory size (Figure \ref{subfig:app:fd:caida},\ref{subfig:app:fd:webpage}):} We find that \aname{} performs better than CM-sketch and CU-sketch on the metric WMRE. For the CAIDA dataset, WMRE of \aname{} is about 4.5 times lower than CM sketch and 4.2 times lower than CU sketch when the memory size is 1MB. For the Web Page dataset, WMRE of \aname{} is about 5.5 times lower than CM sketch and 4.7 times lower than CU sketch when the memory size is 1MB. 

==> vldb/Experiment/application.tex <==
\presub
\subsection{Experiments on other applications} \postsub
\label{subsec:exp:application}

\ppp{Comparison with prior algorithms:}
For finding heavy changes, we compare \aname\_C with 2 other algorithms: FR\cite{flowradar} and FR with CF\cite{coldfilter}.
For finding persistent items, we compare \aname\_P with 2 other algorithms: PIE\cite{persisitem} and Small-Space\cite{smallspace}.
For finding Super-Spreaders, we compare \aname\_S with 3 other algorithms: OLF\cite{superspreader}, TLF\cite{superspreader}, and OpenSketch\cite{opensketch}.

\ppp{Parameter settings:}
See details in appendix \ref{appendix:para:app}.

\input{vldb/Figures/app/change.tex}

\ppp{Finding Heavy Changes (Figure~\ref{subfig:app:change:f1}-\ref{subfig:app:change:thp}):}
We find that the F1 Score of \aname{}\_C is around $10$ times and $6$ times higher than FR and FR with CF, respectively.
The throughput of \aname{}\_C is around $1.35$ and $1.92$ times higher than FR and FR with CF, respectively.

\input{vldb/Figures/app/persist.tex}

\ppp{Finding Persistent Items (Figure~\ref{subfig:app:persist:f1}-\ref{subfig:app:persist:thp}):}
We find that 
%the ARE of \aname{}\_P is around $16$ times and $72$ times lower than PIE and Small-Space, respectively.
the F1 Score of \aname{}\_P is around $3.71$ and $4.35$ times higher than PIE and Small-Space, respectively.
%The CR of \aname{}\_P is $6.58$ times and $2.02$ times higher than PIE and Small-Space, respectively.
%The PR of \aname{}\_P is almost the same with PIE and is around $6.27$ times higher Small-Space, 
The throughput of \aname{}\_P is close to Small-Space, and is around $7.55$ times higher than PIE.
%There is little difference between the throughput of \aname{}\_P and Small-Space, and the throughput of \aname{}\_P is $7.55$ times higher than PIE.

\input{vldb/Figures/app/super.tex}

\ppp{Finding Super-Spreaders (Figure~\ref{subfig:app:super:f1}-\ref{subfig:app:super:thp}):}
We find that 
%the ARE of \aname{}\_S is around $16$, $17$, and $8$ times lower than OLF, TLF, and OpenSketch, respectively.
the F1 Score of \aname{}\_S is around $22.18$, $17.73$, and $1.21$ times higher than OLF, TLF, and OpenSketch, respectively.
%The CR of \aname{}\_S is around $1.38$, $1.59$, and $1.15$ times higher than OLF, TLF, and OpenSketch, respectively.
%The PR of \aname{}\_S is around $44.47$, $35.00$, and $1.27$ times higher than OLF, TLF, and OpenSketch, respectively.
The throughput of \aname{}\_S is lower than OLF and TLF, but higher than OpenSketch.

\ppp{Analysis.}
1)
The F1 Score shows that \aname{}\_C greatly outperforms FR and FR+CF while using merely $\frac{1}{10}$ memory they use.
%The F1 Score of \aname{}\_C is much better than the considered algorithms. 
This is because finding heavy changes requires frequency of items.
Since \aname{} provides more accurate estimation, it also performs better in this task. 
%If we can get a more accurate estimated frequency, we can also do better in finding heavy changes.
%As a result, \aname{} outperforms FR and FR+CF while using merely $\frac{1}{10}$ memory they use.
2) On finding persistent items, the F1 Score of \aname{}\_P is much better than prior algorithms.
For Small-Space, sampling can enhance the throughput, but the low sample rate under small memory magnifies the error.
For PIE, though it uses $200$ times memory as \aname{}\_P, hash collisions still lower its accuracy seriously.
%For PIE, though it uses $200$ times more memory as \aname{}\_P, there are still many hash collisions making its accuracy low.
3) On finding Super-Spreaders, though the Bloom filter requires a lot of memory, \aname{}\_C still greatly outperforms prior algorithms.
The reason for this is the significant amount of memory required by prior algorithms to remove duplicates. For example, OpenSketch uses bitmaps, and OLF uses a hash-table. In contrast, Bloom filter is more effective.

==> vldb/Experiment/distri.tex <==
\presub
\subsection{Experiments on Distributions} \postsub
\label{subsec:exp:distri}

%\input{vldb/Figures/distri/distri.tex}

\ppp{Parameter Setting:}
See details in appendix \ref{appendix:para:dis}.\\
\ppp{ARE (Figure~\ref{subfig:distri:are}):}
We find that the ARE of a skewness of $0.3$ is around 3.0 and 4.0 times higher than that of a skewness of $0.6$ and $3$ respectively.

\ppp{F1 Score (Figure~\ref{subfig:distri:f1}):}
We find that the F1 Score of a skewness of $0.3$ is around 1.03 and 1.04 times lower than that of a skewness of $0.6$ and $3$ respectively.

\ppp{Analysis:} 
According to the results, \aname{} can achieve higher accuracy under high skewness of the dataset. However, even when the skewness is limited, e.g., 0.3, \aname{} with 60KB memory can still achieve an ARE lower than 0.003, and a PR higher than 0.99.
Furthermore, when the skewness is larger than 1.2, the influence brought by the skewness of the dataset is limited.


==> vldb/Experiment/exop.tex <==
\presub
\subsection{Experiments on Extra Operations} \postsub
\label{subsec:exp:exop}

% TODO: operation name of heavy & light?   5 or 4 ops?

In this section, we conduct experiments to illustrate the performance of the extra operations of \aname{} and show more versatility of \aname{}. The operations are: expansion, compression, mergence, and refinement(two kinds of generated sketch: Heavy \aname{} and Light \aname{}). For different operations, we choose appropriate metrics and approaches to compare the performance.

% load factor not mentioned ?

\input{vldb/Figures/application/exopfig}


\subsubsection{Expansion.} We find that we can expand \aname{} to get higher accuracy anytime. According to Formula \ref{formula:expand}, we can double the size of \aname{} when load factor grows. For this experiment, we  separate the CAIDA dataset into three parts with the same number of items and expand \aname{} after inserting one part of the three, so the size of \aname{} is quadrupled in the end. We set the initial size of \aname{} to 50KB and compare the performance between expanded \aname{} and another \aname{} without any expansions.

%\input{vldb/Figures/application/epd.tex}

% 改图：更大的内存获得更小的ARE 

% \ppp{Accuracy vs. memory size (Figure \ref{subfig:epd:high_are:caida},\ref{subfig:epd:high_aae:caida}):}
\ppp{ARE vs. memory size (Figure \ref{subfig:exop:epd}):}
As figures show, we find that the slope of ARE becomes lower evidently after two expansions. %, as well as the one of AAE.
After we finish all insertions, ARE of expanded \aname{} is approximately $1.94$ times lower than the original one.
% After we finish all insertions, ARE and AAE of expanded \aname{} are both approximately $1.94$ times lower than the original one.

\subsubsection{Compression.} We find that compression can significantly improve the accuracy of \aname{} when memory is tight. By using Formula \ref{formula:compress}, \aname{} can be compressed to halve the memory consumption. We measure the accuracy of compressed \aname{} based on the CAIDA dataset.

% TODO: enlarge this paragraph
% 需不需要删掉一组图

%\input{vldb/Figures/application/cpr.tex}
% \input{vldb/Figures/application/cpr_low.tex}

%\ppp{Accuracy vs. memory size (Figure \ref{subfig:cpr:high_are:caida},\ref{subfig:cpr:high_aae:caida}):}
\ppp{ARE vs. memory size (Figure \ref{subfig:exop:cpr}):}
As the figures show, when the memory usage is 400KB, ARE of compressed \aname{} is about $2.04$ times smaller than basic \aname{}. When the memory usage is up to 4MB, the accuracy of the basic one exceed the compressed one because it can record most of the items. In contrast, the compressed \aname{} loses its accuracy by compression operation further.
% For compressed under-estimating \aname{}, Figure \ref{subfig:cpr:low_are:caida} and \ref{subfig:cpr:low_aae:caida} show that ARE and AAE of it is $1.07 \sim 1.30$ times, and is between $1.08 \sim 1.27$ times smaller than that of basic \aname{}, respectively.


\subsubsection{Mergence.} We find that merged \aname{} has almost the same performance compared with basic \aname{}. We can merge two \aname{} with the same sizes and hash functions using Formula \ref{formula:merge}. To conduct experiments, we select two different segments of the CAIDA dataset and use two \aname{}es to process them, respectively. Finally, the merger of the \aname{}es is compared with another \aname{}, which has processed both the two segments.

%\input{vldb/Figures/application/mrg.tex}

% \ppp{Accuracy vs. memory size (Figure \ref{subfig:mrg:high_are:caida},\ref{subfig:mrg:high_aae:caida}):}
\ppp{ARE vs. memory size (Figure \ref{subfig:exop:mrg}):} The figures illustrate that the curves of two \aname{}es are almost the same. So it is feasible to gather distributed information together by merging different \aname{}es into a new one, with extremely low accuracy loss.

\subsubsection{Heavy \aname{}.} We find that corresponding Heavy \aname{} generated by Formula \ref{formula:heavy} can achieve higher performance than basic \aname{} with the same memory usage. By discarding ID records and merging the two counters into a new one, nearly $2/3$ of the memory consumption can be saved. We compared Heavy \aname{} with CM Sketch, CU Sketch, ASketch, and basic \aname{} in frequency estimation using CAIDA dataset.

%\input{vldb/Figures/application/gen_heavy.tex}

\ppp{ARE vs. memory size (Figure \ref{subfig:exop:heavy}):}  As figures show, Heavy \aname{} offers higher accuracy than basic \aname{}, as well as CM Sketch, CU Sketch and ASketch when memory is tight. Notice that the performance of basic \aname{} approaches that of Heavy \aname{} when the memory size grows to 2MB or larger. This is because most of the frequent items have become a dominant item of at least one bucket.
%And indeed, to generate a Heavy \aname with size $N$, we need a \aname{} with size $3N$ to perform insertions firstly.

% 需不需要指出这个盲区：refined sketch需要更大的sketch来运行一段时间

\subsubsection{Light \aname{}. } We find that Light \aname{} generated by Formula \ref{formula:light} can estimate the frequency of the infrequent items more accurately. We measure its performance by comparing the ARE based on the infrequent items whose real frequency is lower than $0.005\%$ of the total. 

%\input{vldb/Figures/application/gen_light.tex}

% \ppp{Accuracy vs. memory size (Figure \ref{subfig:gen:light_are:caida},\ref{subfig:gen:light_aae:caida}):}
\ppp{ARE vs. memory size (Figure \ref{subfig:exop:light}):}
As figures show, Light \aname{} indeed provides a more accurate estimation for infrequent items compared with the other four sketches when the memory usage is less than 100KB. As the memory size increases, the performance of Light \aname{} is exceeded by that of basic \aname{} and CU Sketch. This is because more collisions can be avoided as the number of buckets increases. 
And the contents of most counters in Light \aname{}, which are calculated by $high - low$, become 0.



==> vldb/Experiment/frequent.tex <==
%\vspace{-0.15in}
\presub
\subsection{Experiments on Finding Frequent Items} \postsub
\label{subsec:exp:frequent}

%\input{vldb/Figures/fre/fre_aae.tex}
%\input{vldb/Figures/fre/fre_are.tex}
%\input{vldb/Figures/fre/fre_cr.tex}
%\input{vldb/Figures/fre/fre_pr.tex}
%\input{vldb/Figures/fre/fre_thp.tex}

    
    
    
\ppp{Parameter settings:}
See details in appendix \ref{appendix:para:fre}.



\ppp{Comparison with prior algorithms:}
We compare \aname{} with $3$ algorithms: Count+Heap\cite{countsketch}, USS\cite{unbiasedsketch}, and SS\cite{spacesaving}.
We choose Count+Heap because it is a typical unbiased sketch-based algorithm.
We choose USS because it is a typical unbiased KV-based algorithm.
And we choose SS because it is classic and has been shown in \cite{finding2008} to be better than many algorithms, like Lossy Counting\cite{losscounting} and Frequent\cite{frequent}.
%不知道这个理由是否充分




\ppp{AAE (Figure~\ref{subfig:fre:aae:syn}-\ref{subfig:fre:aae:net}):}
We find that, on the synthetic dataset, the AAE of \aname{} is lower than $0.001$ under a memory of 400KB. On the three real-world datasets, the AAE of \aname{} is on average $651$, $8599$, and $7420$ times lower than Count+Heap, USS, and SS, respectively.

\ppp{ARE (Figure~\ref{subfig:fre:are:syn}-\ref{subfig:fre:are:net}):}
We find that, on the synthetic dataset, the ARE of \aname{} is around $7 \times 10^{-5}$ under a memory of 200KB.
On the three real-world datasets, the ARE of \aname{} is around $1565$, $21737$, and $19802$ times lower than Count+Heap, USS, and SS, respectively.

\ppp{CR (Figure~\ref{subfig:fre:cr:syn}-\ref{subfig:fre:cr:net}):}
We find that, on the synthetic dataset, the CR of \aname{} is around $1.31$, $1.39$, and $1.38$ times higher than Count+Heap, USS, and SS, respectively. On the three real-world datasets, the CR of \aname{} is around $1.25$, $1.35$, and $1.41$ times higher than Count+Heap, USS, and SS, respectively.

\ppp{PR (Figure~\ref{subfig:fre:pr:syn}-\ref{subfig:fre:pr:net}):}
On the synthetic dataset, the PR of \aname{} is around $1.61$, $3.68$, and $3.67$ times higher than Count+Heap, USS, and SS, respectively.
On the three real-world datasets, the PR of \aname{} is around $1.54$, $2.33$, and $2.39$ times higher than Count+Heap, USS, and SS, respectively.	

\ppp{Throughput (Figure~\ref{subfig:fre:thp:syn}-\ref{subfig:fre:thp:net}):}
On the synthetic dataset and the three real-world datasets, the insertion throughput of \aname{} is around $4.05$, $4.50$, and $2.50$ times higher than Count+Heap, USS, and SS, respectively.


\ppp{Analysis.} 
1) The ARE and the AAE of SS and USS are much higher than \aname{}, because the recorded items' frequency tends to be greatly overestimated in SS and USS.
%The reason is that SS and USS often overestimate the frequency of items recorded in the data structure. 
%For example, if the frequency of an item is 1000, the estimated frequency of that item in SS and USS may be 5000, and the ARE may be 4.
The ARE and the AAE of Count+Heap are higher than \aname{} because Count+Heap needs to keep a large Count Sketch to ensure the accuracy.
So when the memory is very limited, its accuracy will be much worse than \aname{}.
2) The throughput of \aname{} is much higher than that of prior algorithms, because \aname{} only needs one memory access for each insertion. 
In SS and USS, the pointer operations will lead to cache misses and make the throughput much lower.
In Count+Heap, multiple accesses to memory and the $O(\log k)$ time complexity of the heap operations slow down the insertion throughput. 
3) We find that the PR of SS and USS sometimes decreases as memory consumption increases. 
This is common for algorithms that overestimate the frequency. 
For example, if the only 200 items are recorded, there are at most 200 items whose estimated frequency exceeds the predefined threshold. However, if 2000 items are recorded, there may be 1000 items whose estimated frequency exceeds the predefined threshold due to overestimation, which leads to a decrease in PR.

==> vldb/Experiment/nature.tex <==
\presub
\subsection{Experiments on \aname{}} \postsub
\label{subsec:exp:nature}

In this section, we conduct several experiments on CAIDA dataset to explore how the number of arrays $d$ and the skewness of a dataset affect the accuracy of \aname{}, for both ordinary and dominant items.     

\subsubsection{Number of Arrays. }
\label{subsubsec:exp:num_ary}
We find that it is relatively better to set the parameter $d$ to 2, which denotes the number of arrays and affects accuracy and parallel efficiency. Therefore, we finally set $d$ to 2 for most following experiments.

\input{vldb/Figures/nature/hashnum.tex}

\ppp{$d$ vs. memory size (Figure  \ref{subfig:nature:hash_are}, \ref{subfig:nature:hash_aae}):} 
%The parameter $d$, denoting the number of arrays, affects the accuracy and parallel efficiency.
It is shown that \aname{}es with $d=1 \sim 2$ perform better than the ones with bigger $d$ in accuracy when memory is tight since the number of buckets is the bottleneck. As the memory size increases, \aname{} with $d=2$ estimates the frequency more accurately than others because of fewer hash collisions and an adequate size. 


\subsubsection{Accuracy of Dominant Item.}
\label{subsec:exp:dom_acc}
% If the frequency of a item is greater than 50\% of the total frequency in the same bucket, we call it as the \emph{dominant item}.
We find that \aname{} offers particularly high accuracy on dominant items. %the frequency of which is greater than 50\% of the total frequency in the same bucket. 
We vary the memory size from 200KB to 4MB and measure the accuracy of \aname{}es with different $d$ (the number of arrays). The metrics PR and AAE show how accurate the estimations of dominant items are.

\input{vldb/Figures/nature/dom.tex}

\ppp{Accuracy vs. memory size (Figure \ref{subfig:nature:dom_pr},\ref{subfig:nature:dom_aae}):} Figure \ref{subfig:nature:dom_pr} shows that \aname{} with $d=1$ takes the leading position when the memory size is less than 4MB. There are two main reasons why $d=1$ performs best: \textbf{1)} A frequent item will occupy at most $d$ buckets so that when memory is tight, bigger the $d$ is, greater the waste of space is. \textbf{2)} An infrequent item will affect $d$ buckets, leading to more error. When the memory size grows to 4MB, the PR of \aname{} with $d=1$ is $94.9\%$, and the ones of $d=2, 3, 4$ are $93.5\%$, $89.4\%$ and $83.4\%$ respectively. Figure \ref{subfig:nature:dom_aae} shows that AAE of \aname{} with $d=2$ is lower than that of \aname{} with $d=1$, which suggests hash collisions become the bottleneck.

\subsubsection{Proportion of Dominant Items} We find that it is common to become a dominant item of one bucket, since a large number of items are extremely infrequent (only appear several times). When the memory size is fixed, there are two main factors affecting the difficulty to be a dominant item: the skewness on dataset and the parameter $d$, representing the number of arrays of \aname{}.   

\ppp{The skewness of datasets (Figure \ref{subfig:nature:dompro_skew}):} We conduct experiments on segments of synthetic datasets specially, which consist of 0.5M items respectively, to control the skewness. We fix the memory size to 1MB and set $d$ to 2. We find that there should be a positive correlation between the proportion of dominant items and the skewness on the dataset as shown in the figure. The results also show that even on the dataset with 0.6 skewness, $99\%$ of the items with frequency greater than 15,  about $0.003\%$ of the stream, become dominant items.

\input{vldb/Figures/nature/dompro.tex}

\ppp{The number of arrays $d$ (Figure \ref{subfig:nature:dompro_d}):} For the parameter $d$, we fix the memory size to 1MB and conduct experiments. As the figure shows, the more arrays we use, the greater probability of becoming a dominant  item with the same frequency is. For $d$ from 2 to 4, $99\%$ of the items with frequency greater than 13, about $0.002\%$ of the stream, become dominant items. 




% \ppp{Skewness of Dataset:} \emph{placeholder}.

==> vldb/Experiment/nature_V3.tex <==
\presub
\subsection{Experiments on \aname{}} \postsub
\label{subsec:exp:nature}

In this section, we conduct several experiments to explore how \aname{} performs in two key techniques, error-sensing and error-controlling. 

\subsubsection{Error-sensing Technique. }
\label{subsubsec:exp:sense}
We find that \aname{} performs well in error-sensing with sufficient memory. For default parameters, we fix the memory size to 1000KB, $\Lambda$ to 25, and conduct experiments on IP Trace dataset. 

\input{vldb/Figures/nature3/nature_7.2.1.1.tex}

\ppp{Sensed Interval (Figure  \ref{subfig:nature:7.2.1.1}, \ref{subfig:nature:7.2.1.1_2}):}
We sample flows with different flow sizes and illustrate the intervals sensed by \aname{}. The results show that sensed error is well-controlled within preconfigured $\Lambda$ regardless of the flow size. And a larger flow always has less error.
% 区间被严格控制在lambda内，并且大流拥有更小的感知误差

\input{vldb/Figures/nature3/nature_7.2.1.2.tex}

\ppp{Actual Error vs. Sensed Error (Figure  \ref{subfig:nature:7.2.1.2}):}
We divide flows by the actual error \aname{} reports, and calculate the average sensed error respectively.
The result shows that sensed error increases with actual error in almost the same speed, which means \aname{} can sense error accurately and stably in current circumstances.
% 无论实际误差为多少，感知区间与实际误差差的不远

\ppp{Memory Size vs. Sensed Error (Figure  \ref{subfig:nature:7.2.1.3}):}
We further vary the memory size from 1000KB to 2500KB, and study how errors change.
The figure shows that sensed error decreased rapidly when memory grows, and it is about 2.03 $\sim$ 5.34 times the actual error. Note that sensed error would never be lower than the error threshold of mice filter, which is set to 3 in this experiment.

% \ppp{Priority Weight vs. Error (Figure  \ref{subfig:nature:7.2.1.4}):}


\subsubsection{Error-controlling Technique. }
\label{subsubsec:exp:control}
We find that \aname{} controls error as our expectation. All experiments are conducted on IP Trace dataset. 

\input{vldb/Figures/nature3/nature_7.2.2.tex}

\ppp{Flow Distribution (Figure  \ref{subfig:nature:7.2.2.1}):}
When the insertion of a flow ends in a certain layer, we call the flow belongs to the layer. We do repeated experiments and compute the flow distribution \wyh{across} layers. The figures show that the number of flows belonging to each level decays faster than exponentially, which means \aname{} can control errors well with few layers and the remains are more often functionless. 
% We can technically reduce the number of layers $d$ to enlarge the size of top layers when memory is excessive.

\ppp{Error Distribution (Figure  \ref{subfig:nature:7.2.2.2}):}
We count absolute errors of all flows, sort them in descending order, and illustrate in percentiles. It shows that errors of \aname{} are controlled within $\Lambda$ completely, while most traditional sketches such as CM Sketch cannot guarantee the expected error.

==> vldb/Experiment/nature_new.tex <==
\presub
\subsection{Parameters of \anamelong{}} \postsub
\label{subsec:exp:nature}

In this section, we conduct several experiments to explore how the parameters $R_w$, $R_\lambda$ and the error threshold $\Lambda$ affect the performance of \aname{}. 
% \wyh{delete}
% based on two applications: error guarantee and frequency estimation.


\subsubsection{Impact of Parameter $R_w$. }
\label{subsubsec:exp:r_w}

When adjusting $R_w$ (\ie, the parameter of the decreasing speed of array size), we find \aname{} performs best when $R_w=2$.
% Considered the trade-off between the performance of error guarantee and frequency estimation, we find that it is relatively better to set the parameter $R_w$ to 2, which denotes the decrease speed of array size. Therefore, we finally set $R_w$ to 2 for the most of following experiments. 
% denotation: layer? decrease speed of array size

\input{vldb/Figures/nature/rw_range.tex}


\ppp{Memory Usage under Zero Outlier (Figure  \ref{subfig:nature:rw_range_caida}, \ref{subfig:nature:rw_range_webpage}):} 
%$\ppp{$R_w$ vs. Error Guarantee (Figure  \ref{subfig:nature:rw_range_caida}, \ref{subfig:nature:rw_range_webpage}):} 
We conduct experiments on IP Trace and Web Stream datasets. We set the user-defined threshold $\Lambda$ to 25, and compare the minimum memory consumption achieving zero outlier under different $R_w$.
It is shown that \aname{} with $R_w=2 \sim 2.5$ requires less memory than the ones with other $R_w$. When $R_w$ is lower than 1.6 or higher than 3, the memory consumption increases rapidly.

\input{vldb/Figures/nature/rw_freq.tex}

\ppp{Memory Usage under the Same Average Error (Figure  \ref{subfig:nature:rw_freq_caida}, \ref{subfig:nature:rw_freq_webpage}):} 
We conduct experiments on IP Trace and Web Stream datasets, set the target estimation AAE to 5, and compare the memory consumption when $R_w$ varies. The figures show that the higher $R_w$ goes with less memory usage. However, the memory consumption is quite close to the minimum value when $R_w= 2 \sim 6$. 

\subsubsection{impact of Parameter $R_\lambda$. }
\label{subsubsec:exp:r_l}
When adjusting $R_\lambda$ (\ie, the parameter of the decreasing speed of error threshold), we find \aname{} performs best when we set $R_\lambda=2.5$.
% We find that it is relatively better to set the parameter $R_\lambda$ to 2.5, which denotes the decreasing speed of error threshold. 

\input{vldb/Figures/nature/rl_range.tex}

\ppp{Memory Usage under Zero Outlier (Figure  \ref{subfig:nature:rl_range_caida}, \ref{subfig:nature:rl_range_webpage}):} 
We conduct experiments and set the target $\Lambda$ to 25. As the figures show, memory consumption drops down rapidly when $R_\lambda$ grows from 1.2 to 2 and finally achieve the minimum when $R_\lambda = 2$. There is no significant change when $R_\lambda$ is higher than 2.5, only some jitters due to the randomness of \aname{}. 

\input{vldb/Figures/nature/rl_freq.tex}

\ppp{Memory Usage under the Same Average Error (Figure  \ref{subfig:nature:rl_freq_caida}, \ref{subfig:nature:rl_freq_webpage}):} 
To explore the impact of parameter $R_\lambda$ on average error, we set the target estimation AAE to 5 and compare the memory consumption when $R_\lambda$ varies. It is shown that when $R_w$ is low, the higher $R_\lambda$ is, the less memory \aname{} uses. When $R_w$ is greater than 4, $R_\lambda$ affects little.

\subsubsection{Error Threshold $\Lambda$. }
\label{subsubsec:exp:eps}

We find that the user-defined error threshold $\Lambda$, which denotes the maximum estimated error \aname{} guaranteed, is almost inversely proportional to the memory consumption. In real tasks, we can implement \aname{} in a proper $\Lambda$ to meet our actual need better.

\input{vldb/Figures/nature/eps_range}

\ppp{Memory Usage under Zero Outlier (Figure \ref{subfig:nature:eps_range_caida}):} In this experiment, we fix the parameter $R_w$ to 2,  $R_\lambda$ to 2.5, and conduct it on three different datasets. 
It is shown that memory usage monotonically decreases, which means the optimal $\Lambda$ is exactly the maximum tolerable error.
% It is shown that memory usage monotonically decreases, which means the optimal $\Lambda$ is exactly the target guarantee range.
On the other hand, reducing $\Lambda$ blindly will lead to an extremely high memory cost.

\ppp{Memory Usage under the Same Average Error (Figure \ref{subfig:nature:eps_freq_caida}):} In this experiment, we fix the parameter $R_w$ to 2,  $R_\lambda$ to 2.5, and conduct it on IP Trace dataset. The figure shows that optimal $\Lambda$ increases as target AAE increases, and optimal $\Lambda$ is about 2 $\sim$ 3 times greater than target AAE. For target AAE=5/10/15/20, the optimums are 15/25/35/50, requiring 1.43/1.05/0.85/0.75MB memory respectively.

% 改成四个数据集

% \subsubsection{Accuracy of Dominant Item.}
% \label{subsec:exp:dom_acc}
% % If the frequency of a item is greater than 50\% of the total frequency in the same bucket, we call it as the \emph{dominant item}.
% We find that \aname{} offers particularly high accuracy on dominant items. %the frequency of which is greater than 50\% of the total frequency in the same bucket. 
% We vary the memory size from 200KB to 4MB and measure the accuracy of \aname{}es with different $d$ (the number of arrays). The metrics PR and AAE show how accurate the estimations of dominant items are.

% \input{vldb/Figures/nature/dom.tex}

% \ppp{Accuracy vs. memory size (Figure \ref{subfig:nature:dom_pr},\ref{subfig:nature:dom_aae}):} Figure \ref{subfig:nature:dom_pr} shows that \aname{} with $d=1$ takes the leading position when the memory size is less than 4MB. There are two main reasons why $d=1$ performs best: \textbf{1)} A frequent item will occupy at most $d$ buckets so that when memory is tight, bigger the $d$ is, greater the waste of space is. \textbf{2)} An infrequent item will affect $d$ buckets, leading to more error. When the memory size grows to 4MB, the PR of \aname{} with $d=1$ is $94.9\%$, and the ones of $d=2, 3, 4$ are $93.5\%$, $89.4\%$ and $83.4\%$ respectively. Figure \ref{subfig:nature:dom_aae} shows that AAE of \aname{} with $d=2$ is lower than that of \aname{} with $d=1$, which suggests hash collisions become the bottleneck.

% \subsubsection{Proportion of Dominant Items} We find that it is common to become a dominant item of one bucket, since a large number of items are extremely infrequent (only appear several times). When the memory size is fixed, there are two main factors affecting the difficulty to be a dominant item: the skewness on dataset and the parameter $d$, representing the number of arrays of \aname{}.   

% \ppp{The skewness of datasets (Figure \ref{subfig:nature:dompro_skew}):} We conduct experiments on segments of synthetic datasets specially, which consist of 0.5M items respectively, to control the skewness. We fix the memory size to 1MB and set $d$ to 2. We find that there should be a positive correlation between the proportion of dominant items and the skewness on the dataset as shown in the figure. The results also show that even on the dataset with 0.6 skewness, $99\%$ of the items with frequency greater than 15,  about $0.003\%$ of the stream, become dominant items.

% \input{vldb/Figures/nature/dompro.tex}

% \ppp{The number of arrays $d$ (Figure \ref{subfig:nature:dompro_d}):} For the parameter $d$, we fix the memory size to 1MB and conduct experiments. As the figure shows, the more arrays we use, the greater probability of becoming a dominant  item with the same frequency is. For $d$ from 2 to 4, $99\%$ of the items with frequency greater than 13, about $0.002\%$ of the stream, become dominant items. 




% \ppp{Skewness of Dataset:} \emph{placeholder}.

==> vldb/Experiment/order.tex <==
\subsection{Experiments on Arrival Orders}
\label{subsec:exp:order}

\input{Figures/order/order_are/order_are.tex}
\input{Figures/order/order_f1/order_f1.tex}

In this section, we analyze how the order of arrival of items influences the performance of the following 4 algorithms: \aname, Count+Heap\cite{countsketch}, USS\cite{unbiasedsketch}, and SS\cite{spacesaving}. 

\ppp{Parameter Setting:}
For \aname{}, we set $d=16$, which means there are 16 cells in the counting part. For other sketches, the parameters are set according to their authors' recommendations.
As in Section \ref{subsec:exp:frequent}, the memory size ranges from 0.2MB to 1MB. For the datasets, we use the synthetic datasets whose skewness is 1.5 with three different item orders. The original order which stands for the i.i.d. stream is called "i.i.d.". Then we sort the synthetic dataset by frequency. The dataset which is sorted by ascending order is called "Ascend", and the dataset which is sorted by descending order is called "Descend".

\ppp{\aname (Figure~\ref{subfig:order:are:aname}\&\ref{subfig:order:f1:aname}):
}
We find that the ARE of \aname{} under i.i.d. order is often lower than the ARE under ascending order. In addition, the F1 Score of \aname{} under i.i.d. order is often higher than the F1 Score under ascending order.
The F1 Score of \aname{} under descending order is often 1, and the ARE of \aname{} under descending order is often 0.


\ppp{Count+Heap (Figure~\ref{subfig:order:are:count}\&\ref{subfig:order:f1:count}):
}
We find that the ARE of Count+Heap under i.i.d. order is around $2.58$ times lower and $1.51$ times higher than the ARE under ascending order and the ARE under descending order. In addition, the F1 Score of Count+Heap under i.i.d. order is around $1.39$ times lower than the F1 Score under ascending order and around $1.15$ times higher than the F1 Score under descending order.

\ppp{USS (Figure~\ref{subfig:order:are:uss}\&\ref{subfig:order:f1:uss}):
}
We find that the ARE of USS under i.i.d. order is around $1.45$ times lower and $1.01$ times higher than the ARE under ascending order and the ARE under descending order. In addition, the F1 Score of USS under i.i.d. order is around $1.15$ times higher than the F1 Score under ascending order and is almost the same with the F1 Score under descending order.

\ppp{SS (Figure~\ref{subfig:order:are:ss}\&\ref{subfig:order:f1:ss}):
}
we find that the ARE of SS under i.i.d. order is around $1.99$ times lower than the ARE under ascending order.
In addition, the F1 Score of SS under i.i.d. order is around $1.60$ times lower than the F1 Score under ascending order and around $1.89$ times higher than the F1 Score under descending order. The ARE of SS under descending order is often 0.

\ppp{Analysis:} 
1) The ARE of all algorithms is often the worst under ascending order.
This is because the frequent items that arrive later will be highly influenced by the earlier part of the data stream. As a result, the estimated frequency of items that arrive later will have a larger error in all these 4 algorithms.

2) We find that though the ARE of SS is often the worst under ascending order, the F1 Score of SS is often the best under ascending order.
On the contrary, the ARE of SS is often the best under descending order, and the F1 Score of SS is often the worst under descending order.
This is because SS often reports the last $k$ items as the frequent items.
However, as shown above, the estimated frequency of the items which arrive last will have the largest error. Therefore, if the frequent items arrive later, their estimated frequency will be inaccurate, but they can be reported. If the frequent items arrive earlier, their estimated frequency will be accurate, but they can hardly be reported.

==> vldb/Experiment/para.tex <==
\presub
\subsection{Experiments on Parameter Settings} \postsub
\label{subsec:exp:para}

%\input{vldb/Figures/para/para.tex}

As shown in Section \ref{SEC:Algorithm}, we have two parameters in \aname{}: $l$ and $d$. To evaluate the influence of parameter setting, we fix the memory usage of \aname{} and vary the value of $d$.
We use finding frequent items as the considered application in this section to avoid the influence brought by the Bloom filter. The memory size ranges from 20KB to 100KB, because such little memory better exposes the differences between different values of $d$. As shown in Section \ref{subsec:exp:frequent}, \aname{} performs better than prior algorithms with only 200KB memory. We vary $d$ from $8$ to $64$ and use the synthetic dataset to evaluate the influence of the parameter setting.


\ppp{ARE (Figure~\ref{subfig:para:are}):}
We find that the ARE of $d=8$ is around 1.6, 3.3, and 3.7 times higher than that of $d=16$, $d=32$, and $d=64$, respectively.
			
\ppp{CR (Figure~\ref{subfig:para:cr}):}
We find that the CR of $d=8$ is around 1.03, 1.04, and 1.04 times lower than that of $d=16$, $d=32$, and $d=64$, respectively.

\ppp{PR (Figure~\ref{subfig:para:pr}):}
We find that the PR of $d=8$ is around 1.004, 1.022, and 1.034 times lower than that of $d=16$, $d=32$, and $d=64$, respectively.
			
\ppp{Throughput (Figure~\ref{subfig:para:thp}):}
We find that the throughput of $d=8$ is around 1.04, 1.11, and 1.21 times higher than that of $d=16$, $d=32$, and $d=64$, respectively.


\ppp{Analysis:} 
According to the results, given an amount of memory, a higher value of $d$ typically goes with a higher accuracy of \aname{}, while the throughput is often lower.
%In other words, deciding the most appropriate value of $d$ will involve balancing accuracy and throughput.
In other words, the value of $d$ is selected based on a trade-off between accuracy and throughput.
If the application requires a higher speed, we can use a smaller value of $d$. If the application requires a higher accuracy, we can use a larger value of $d$. Furthermore, the results confirm that \aname{} works well with only 20KB of memory.

==> vldb/Experiment/prior.tex <==
\presub
\subsection{Performance on Priority} \postsub
\label{subsec:exp:prior}

As Section ?? claims, \aname{} can handle different priority packets in a succinct way. In this section, we further conduct experiments to study the performance in this case.

% \subsubsection{Impact of Parameter $R_w$. }
% \label{subsubsec:exp:r_w}

==> vldb/Experiment/sense_ctrl_err.tex <==
\presub
\subsection{Experiments on \goal{}} \postsub
\label{subsec:exp:sense_ctrl_err}

We show how \aname{} performs in \goal{} comprehensively, and compare it with prior algorithms. 
% In this section, we conduct several experiments to explore how \aname{} performs in \goal{} and compare with prior algorithms. 
% In this section, we apply \aname{} to frequency estimation and compare \aname{} with prior algorithms using two metrics, the number of outliers and average error.

\presubsub
\subsubsection{Error-Sensing Ability. }
\label{subsubsec:exp:sense}
\aname{} can sense the error confidently and accurately with default parameters.
% We find that \aname{} performs well in error-sensing with default parameters (\cref{?}).
% We fix the memory size to 1000KB, $\Lambda$ to 25, and conduct experiments on IP Trace dataset.

\input{vldb/Figures/nature3/nature_7.2.1.1.tex}

\ppp{Sensed Interval (Figure  \ref{subfig:nature:7.2.1.1}, \ref{subfig:nature:7.2.1.1_2}):}
We sample flows with different flow sizes and illustrate the intervals of possible flow sizes sensed by \aname{}. The results show that the interval must contain the actual flow size and sensed error (\ie, interval length) is well-controlled within user-defined $\Lambda$ regardless of the flow size. 
% And a larger flow tends to have less error.
% 区间被严格控制在lambda内，并且大流拥有更小的感知误差

\input{vldb/Figures/nature3/nature_7.2.1.2.tex}

\ppp{Actual Error \emph{vs.} Sensed Error (Figure  \ref{subfig:nature:7.2.1.2}):}
As we query the sizes of all flows in \aname{}, we classify these flows by their actual absolute error, and calculate the average sensed error respectively.
% We divide flows by the actual error \aname{} reports, and calculate the average sensed error respectively.
The result shows that sensed error keeps close to the actual error no matter how it changes, which means \aname{} can sense error accurately and stably.
% The result shows that sensed error increases with actual error in almost the same speed, which means \aname{} can sense error accurately and stably in current circumstances.
% 无论实际误差为多少，感知区间与实际误差差的不远

\ppp{Sensed Error \emph{vs.} Memory Size  (Figure  \ref{subfig:nature:7.2.1.3}):}
We further vary the memory size from 1000KB to 2500KB, and study how errors change.
The figure shows that sensed error decreased rapidly when memory grows, and it is about 2.03 $\sim$ 5.34 times the actual error. 
% Note that sensed error would never be lower than the error threshold of mice filter, which is set to 3 in this experiment. 没必要

% \ppp{Priority Weight vs. Error (Figure  \ref{subfig:nature:7.2.1.4}):}

\presubsub
\subsubsection{Error-Controlling Ability. }
\label{subsubsec:exp:control}
\aname{} controls error efficiently as our expectation and achieves the best performance compared with competitors.
% in metric the number of outliers.
% \whb{!!! here is too messive, find a proper way to handle them.}
 
% And for HeavyGuardian, we set $\lambda_h$ to 8, $\lambda_l$ to 64 and $b$ to 1.08.
% We use the number of fails as the metric to measure the performance.
% 更改metric


\input{vldb/Figures/nature3/nature_7.2.2.tex}

\ppp{Flow Distribution (Figure  \ref{subfig:nature:7.2.2.1}):}
When the insertion of a flow's last packet ends in a specific layer, we call the flow belongs to the layer. We do repeated experiments and compute the flow distribution across layers. The figure shows that the number of flows belonging to each level decays faster than exponentially, which means \aname{} can control errors well with few layers and the remains can reduce potential accidents.
% are more often functionless. 
% We can technically reduce the number of layers $d$ to enlarge the size of top layers when memory is excessive.

\ppp{Error Distribution (Figure  \ref{subfig:nature:7.2.2.2}):}
We count absolute errors of all flows, and sort them in descending order. %, and illustrate in percentiles. 
The figure shows that errors of \aname{} are controlled within $\Lambda$ completely, while most traditional sketch algorithms cannot control the error of all flows, such as CM.


% \presub
% \subsection{Experiments on \aname{}} \postsub
% \label{subsec:exp:app}



%In this section, we apply \aname{} to two applications with different orientations: frequency estimation and error guarantee. 
%We compare the accuracy between \aname{} and other standard algorithms for these applications.
%We compare the accuracy between \aname{}es in different threshold $\Lambda$ and other standard algorithms for these applications.     

% \subsubsection{\# Outliers.}
% \label{subsubsec:exp:range}
% We find that \aname{} achieves the best performance compared with other algorithms in metric the number of outliers.

\input{vldb/Figures/app_new2/outlier_lambda}

\ppp{Impact of Threshold $\Lambda$ (Figure \ref{subfig:app:range5:caida}, \ref{subfig:app:range25:caida}):}
We vary $\Lambda$ and count the number of outliers (\ie, out-of-control flows).
%不用所有都写error threshold，第一次出现的时候写完整就行。
As the figures show, \aname{} takes the lead position regardless of $\Lambda$.
When $\Lambda$=$25$, \aname{} achieves zero outlier within 1MB memory, while the others still report over 5000 outliers. 
% , while Space-Saving requires nearly 1.98 MB memory.
% HeavyGuardian performs as well as \aname{} in low memory, yet it cannot offer a stable report as \aname{} does when memory grows.
% Other competitors still report over 100 outliers when memory size is 4 MB.
% Compared with the fast versions, despite the fact that CM Sketch (accurate) and CU Sketch (accurate) perform worse with insufficient memory, the number of outliers drops down rapidly when memory grows. However, the accurate versions also suffer low throughput.

% \input{vldb/Figures/app_new2/outlier_dataset}

% \ppp{Impact of Dataset (Figure \ref{subfig:app:range25:caida},\ref{subfig:app:range25:webpage},\ref{subfig:app:range25:kosarak},\ref{subfig:app:range25:syn003},\ref{subfig:app:range25:syn030}):} We fix $\Lambda$ to 25 and change the dataset. The figures illustrate that \aname{} has the least memory requirement regardless of the dataset. Space-Saving requires 2 $\sim$ 4 times more memory to achieve zero outlier than \aname{}. % HeavyGuardian achieves stable performance on Web Stream and Click Stream datasets, because there are relatively less infrequent items than IP Trace. However, it still requires comparable amount of memory as Space-Saving.
% CU Sketch(accurate) requires 4 $\sim$ 8 times more memory and performs unstably in different datasets.
% For synthetic dataset with skewness=0.3, no algorithm achieves zero outlier within 4MB memory, while the number of outliers of \aname{} is over 100 times less than others. 

% 柱状图

% \input{vldb/Figures/app_new/range_mem}
\input{vldb/Figures/app_new2/outlier_minmem}

\ppp{Memory Consumption (Figure \ref{fig:app:outlier_minmem}):} We further explore the precise minimum memory consumption to achieve zero outlier for all algorithms, $\Lambda$ is fixed to 25 and experiments are conducted on different datasets. 
For the IP Trace dataset, memory consumption of \aname{} is 0.91MB, about 6.07, 2.69, 2.01, 9.32 times less than CM (accurate), CU (accurate), Space-Saving, and Elastic respectively.
CM (fast), CU (fast) and Coco cannot achieve zero outlier within 10MB memory.
% For the Web Stream dataset, memory consumption of \aname{} is 0.44MB, about 7.79, 3.90, 2.59, 7.79 times less than them, respectively.
Besides, CM, CU and Elastic usually require more memory than the minimum value, otherwise they cannot achieve zero outlier stably.
% there is still a high probability of outliers.

% \subsubsection{Average Error.}
% \label{subsubsec:exp:fe}
% We find that \aname{} achieves comparable accuracy with competitors in the average error.
% % We conduct experiments to compare the performance of \aname{} with that of above competitors. 
% % except HeavyGuardian, %because HeavyGuardian is bilateral-estimating while others are all over-estimating.
% % because its estimation is neither one-side error nor unbiased estimation.
% % Noticed that competitors are all over-estimating, while \aname{} may return an under-estimated value when all mapped buckets are locked. For fairness, we set the error threshold of last layer $\lambda_d$ to positive infinite specially, so that returned value is always an over-estimation.
% % \whb{clarify why not use a fixed $\Lambda$.} 
% Although different from others, our \aname{} does not target to small average error, we still perform well.
% The threshold $\Lambda$ varies under different memory size according to Formula \ref{formula:setLambda}.
% % $\Lambda$ of \aname{}  Formula \ref{formula:setLambda}.
% % , and $R_w$ is set to 6 for more precise estimation. 
% For CM and CU, we only compare \aname{} with the 3 arrays versions because more arrays cannot decrease the average error significantly.
% % Other settings of algorithms are as the same as Section \cref{subsubsec:exp:control}.
% % It is had to say that though we still call the CM Sketch and CU Sketch with 16 arrays the accurate version, they are not accurate at average error actually.
% We vary the memory usage from $200$KB to $4$MB, using ARE and AAE to measure the accuracy of  above algorithms.
% % We use $2$ arrays for \aname{} because it is illustrated in Section \ref{subsubsec:exp:num_ary} that $d=2$ can achieve the most balanced performance. 


% % how to explain we set d of CM and CU to 4?
% % 注明frequency会随着R_w的增加而增加，这个task不是mvs的优化目标

% % \input{vldb/Figures/app_new/freq_aae}
% % \input{vldb/Figures/app_new2/avg_err_v2}

% % 颠倒倍率的表示表现反比关系？

% \ppp{ARE \emph{vs.} Memory Size (Figure \ref{subfig:app:fe_are:caida}):}
% % It is shown that under-estimating \aname{} can keep an extremely low ARE even with limited memory consumption. This is because that most items are infrequent, and the under-estimating sketches often offer less error than the over-estimating ones when estimating their frequencies. 
% It is shown that when memory size grows to 4MB, \aname{} achieves a comparable ARE with Elastic, and is $1.90$ times lower than CU, $3.19$ times lower than CM, $3.46$ times lower than Coco, and $22.05$ times lower than Space-Saving.
% % Note that ARE of \aname{} is about 2 times higher than CU Sketch when memory size is 200KB, because the derived $\Lambda$ is too large and the bottom layers are totally wasted. Under such a circumstance, we recommend to increase $R_w$ or decrease $d$ appropriately to enlarge the size of top layers.

% % Indeed, \aname{} with higher $R_w$ can get better performance, but also results in more outliers. For the trade-off, extreme parameters are not recommended in common use.

% \ppp{AAE \emph{vs.} Memory Size (Figure \ref{subfig:app:fe_aae:caida}):}
% It is shown that \aname{} also has a comparable AAE with Elastic and CU, is about $1.36$ times lower than CM, $1.28$ times lower than Coco, and $7.54$ times lower than Space-Saving when memory size is up to 4MB.
\presubsub
\subsubsection{Heavy Hitter Detection.}
\label{subsubsec:exp:hh}
We find that \aname{} achieves the highest fidelity and stability in eliminating outliers, compared with other schemes for heavy hitter detection. 
When the flow size is larger than a predefined threshold $T$, we report it as a heavy hitter.
The user-defined $\Lambda$ is fixed to 25.
As Figure \ref{fig:intro:hh} shows, we count intolerable error as a heavy hitter outlier, which means a false positive with flow size smaller than $T - \Lambda$ or a false negative with flow size larger than $T + \Lambda$.
We vary the memory usage from $200$KB to $4$MB, using the number of outliers to measure the accuracy of above algorithms.
For a specific setting, we change hash seed, conduct 100 repeated experiments, and illustrate the worst case.

\input{vldb/Figures/app_new2/hh}

\ppp{Worst Accuracy (Figure \ref{fig:app:hh}):}
It is shown that \aname{} requires least memory to achieve zero outliers with stable performance.
For $T = 100$, there are totally 12718 heavy hitters.
Space-Saving requires about $1.8$ times larger memory than \aname{}, and others cannot provide no-error estimation stably within 4MB.
For $T = 1000$, there are 1625 heavy hitters.
\aname{} achieves comparable performance with Space-Saving, but it is worth noting that the Space-Saving cannot be implemented on the hardware platforms including programmable switches and FPGA.
% Others perform well when memory is restricted. 
Even when memory is quite large, the other competitors cannot completely eliminate the outlier.

\presubsub
\subsubsection{Throughput.}
We find that \aname{} is not only accurate but also fast.
We perform 10M insertions and 10M queries, compare the throughput among \aname{} and the competitors. 
An alternative version of \aname{} without mice filter ("Raw" in the figures) is provided in addition, which sacrifices tolerable accuracy for significant speed boost.

\input{vldb/Figures/tp_new2/tp_mix}

\ppp{Performance on Throughput (Figure \ref{fig:app:tp}):} The figure shows that the insertion throughput of \aname{} and \aname{} (Raw) are 25.40Mpps and 51.29Mpps respectively. The raw version has comparable throughput with CM (fast), Coco and HashPipe, 1.42 times faster than CU (fast), 1.43 times faster than Elastic, 1.56 times faster than PRECISION, 3.40 $\sim$ 6.65 times faster than others.
The query throughput of two \aname{}es are 31.29Mpps and 66.89Mpps respectively. The raw version is about 1.22 times faster than CM (fast), CU (fast) and Coco, 1.81 times faster than PRECISION, 2.14 times faster than Elastic, and 2.22 $\sim$ 5.62 times faster than others. More conducted experiments in \cref{app:exp:throughput}.
% For the Web Stream dataset, two version \aname{}es perform 30.41Mips and 64.70Mips throughput respectively, the raw version is about 1.17 times faster than CM Sketch (fast), 1.64 times faster than CU Sketch (fast), 1.89 times faster than ElasticSketch, and 3.58 $\sim$ 7.72 times faster than others.

% \ppp{Query (Figure \ref{fig:tp}):} 
% For the Web Stream dataset, two \aname{}es provide 34.49Mips and 84.79Mips throughput respectively, the raw one is comparable with CocoSketch, about 1.57 times faster than CM Sketch (fast) and CU Sketch (fast), 1.51 times faster than ElasticSketch, and 2.68 $\sim$ 7.22 times faster than others.










==> vldb/Experiment/setup.tex <==
\presub

\begin{table}
\caption{Abbreviations in experiments.}
\label{table:abbr}
\begin{tabular}{|c|l|}
\hline
Abbreviation&Full name\\
\hline
Count+Heap&Count Sketch\cite{countsketch} with a heap\\
\hline
SS&SpaceSaving\cite{spacesaving}\\
\hline
USS&Unbiased SpaceSaving\cite{unbiasedsketch}\\
\hline
FR&FlowRadar\cite{flowradar}\\
\hline
CF&Cold Filter\cite{coldfilter}\\
\hline
OLF&One-level Filtering\cite{superspreader}\\  
\hline
TLF&Two-level Filtering\cite{superspreader}\\
\hline
\aname&The \aname{} in Section \ref{SEC:Algorithm}\\
\hline
\aname\_C&\aname{} for heavy changes\\
\hline
\aname\_P&\aname{} for persistent items\\
\hline
\aname\_S&\aname{} for Super-Spreaders\\
\hline
\end{tabular}
\end{table}

\subsection{Experimental Setup} \postsub
\label{subsec:exp:setup}

See details of the implementation, datasets and computation platform in appendix \ref{exp:imp}, appendix \ref{exp:dat}, appendix \ref{compute}, respectively.
%\ppp{Implementation:}
%We have implemented \aname{} and all other algorithms in C++.
%The hash functions are implemented using the 32-bit Bob Hash (obtained from the open-source website \cite{bobhash}) with different initial seeds.


%\ppp{Datasets:}
%Shown in appendix \ref{exp:dat}.


%\ppp{Computation Platform:}
%See details in appendix \ref{compute}.
%We conducted all the experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory. 
%Each processor has three levels of cache memory: one 32KB L1 data caches and one 32KB L1 instruction cache for each core, one 256KB L2 cache for each core, and one 15MB L3 cache shared by all cores.

\ppp{Metrics:}
\label{subsec:eva:metric}

\ppp{1) Average Absolute Error (AAE):} $\frac{1}{|\mathbf{\Psi}|} \sum_{e_i \in \mathbf{\Psi}}|f_i-\hat{f_i}| $,
where $f_i$ is the real frequency of item $e_i$, $\hat{f_i}$ is its estimated frequency, and $\mathbf{\Psi}$ is the query set. 
Here, we query the dataset by querying each actually frequent item once in the sketch.
% Steve: the "each truly/actually frequent reported item" is not clear to me. I think it's worth rewording more precisely.

\ppp{2) Average Relative Error (ARE):} $\frac{1}{|\mathbf{\Psi}|} \sum_{e_i \in \mathbf{\Psi}}|f_i-\hat{f_i}|/ f_i $,
where $f_i$ is the real frequency of item $e_i$, $\widehat{f_i}$ is its estimated frequency, and $\mathbf{\Psi}$ is the query set. 
Here, we query the dataset by querying each actually frequent item once in the sketch.

\ppp{3) Recall Rate (CR):}
The ratio of the number of correctly reported items to the number of correct items.

\ppp{4) Precision Rate (PR):}
The ratio of the number of correctly reported items to the number of reported items.

\ppp{5) F1 Score:}
$\frac{2 * CR * PR}{CR + PR}$

\ppp{6) Throughput:}
Million operations (insertions) per second (Mops).
%We only focus on the insertion throughput in our experiments.
% Steve: Why only insertion throughput?
All the experiments about throughput are repeated 10 times and the average throughput is reported.

==> vldb/Experiment/setup_2.tex <==

\presub
\subsection{Experimental Setup} \postsub
\label{subsec:exp:setup}

\ppp{Datasets:}

\ppp{1) CAIDA: } An anonymized dataset from \cite{caida}, comprised of IP packets. We can identify an item by the IP addresses of the source and destination. The first 10M items out of the whole trace are used to conduct experiments, including about 4.2M distinct items.

\ppp{2) Web Page: } A transactional dataset built from a spidered collection of web HTML documents \cite{webpage}. We use 10M items of the dataset, containing about 0.4M distinct items.

\ppp{3) Synthetic Datasets:} We generate \cite{webpoly} several synthetic datasets according to a Zipf distribution with different skewness for experiments, each of them consists of 32M items.
%\ppp{Implementation:}
%We have implemented \aname{} and all other algorithms in C++.
%The hash functions are implemented using the 32-bit Bob Hash (obtained from the open-source website \cite{bobhash}) with different initial seeds.


%\ppp{Datasets:}
%Shown in appendix \ref{exp:dat}.

\ppp{Implementation:}
We have implemented \aname{} and related algorithms in C++. Here we use the 32-bit Bob Hash \cite{bobhash}, where different hash functions affect performance little. A bucket of \aname{} consists of two 32-bit counters and a 16-bit ID field. All experiments are conducted on a server with dual 6-core processors(12 threads, Intel Xeon CPU E5-2620 @ 2.00GHz) and 16x8 GB memory. 

%\ppp{Computation Platform:}
%See details in appendix \ref{compute}.
%We conducted all the experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory. 
%Each processor has three levels of cache memory: one 32KB L1 data caches and one 32KB L1 instruction cache for each core, one 256KB L2 cache for each core, and one 15MB L3 cache shared by all cores.

\ppp{Metrics:}
\label{subsec:exp:metric}

\ppp{1) AAE (Average Absolute Error):} $\frac{1}{|\mathbf{\Psi}|} \sum_{e_i \in \mathbf{\Psi}}|f_i-\hat{f_i}| $,
where $\Psi$ is the set of items in the dataset, $f_i$ is the correct frequency of item $e_i$, and $\hat{f_i}$ is the estimated frequency. 
% AAE evaluates the accuracy of the estimated frequency.
% Steve: the "each truly/actually frequent reported item" is not clear to me. I think it's worth rewording more precisely.

\ppp{2) ARE (Average Relative Error):} $\frac{1}{|\mathbf{\Psi}|} \sum_{e_i \in \mathbf{\Psi}}|f_i-\hat{f_i}|/ f_i $,
where $\Psi$ is the set of items in the experimental dataset, $f_i$ is the correct frequency of item $e_i$, and $\hat{f_i}$ is the estimated frequency. 
% ARE evaluates the accuracy of the estimated frequency. 
% We use it in most of the tasks.

\ppp{3) PR (Precision Rate):} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Omega}|}$, where $\Omega$ is the answer set reported by our algorithm.
% PR refers to the ratio of the number of correctly reported answers to the number of all reported answers.

\ppp{4) RR (Recall Rate):} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Psi}|}$.
% RR refers to the ratio of the number of correctly reported answers to the number of all correct items.

\ppp{5) F1 Score:} $\frac{2 \times PR \times RR}{PR + RR}$. F1 Score is the harmonic mean of PR and RR, which are mentioned above. 

\ppp{6) RE (Relative Error):} $\sum_{e_i \in \mathbf{\Psi}} |d_i - \hat{d_i}| / d_i$, where $d_i$ is the real value and $\hat{d_i}$ is the estimated value. % We use it to evaluate the performance of cardinality and entropy estimation.

\ppp{7) WMRE (Weighted Mean Relative Error) \cite{kumar2004data}:} $\frac{\sum_{i=1}^{z}{|d_i - \hat{d_i}|}}{\sum_{i=1}^{z}\frac{d_i + \hat{d_i}}{2}}$, where $d_i$ and $\hat{d_i}$ are the real and estimated number of items with frequency $i$.
% We use it to evaluate the performance of frequency distribution estimation.

\ppp{8) Throughput:} $\frac{N}{T}$, where $N$ is the number of operations and $T$ is the time spent. Throughput describes the processing speed of an algorithm, and we use Million of items per second(Mips) to measure  throughput.


==> vldb/Experiment/setup_V3.tex <==

\presub
\subsection{Experimental Setup} \postsub
\label{subsec:exp:setup}

%\ppp{Implementation:}
%We have implemented \aname{} and all other algorithms in C++.
%The hash functions are implemented using the 32-bit Bob Hash (obtained from the open-source website \cite{bobhash}) with different initial seeds.


%\ppp{Datasets:}
%Shown in appendix \ref{exp:dat}.

\subsubsection{Implementation}
We have implemented \aname{} and related algorithms in C++. Here we use fast 32-bit Murmur Hashing \cite{murmur}, and different hash functions that affect accuracy little. Each bucket of \aname{} consists of a 32-bit $YES$ counter, a 16-bit $NO$ counter, and a 32-bit $ID$ field. Mice filter occupies 20\% of total memory, and bucket size of it is fixed to 2 bits without notes. 
% \whb{!!!cite the appendix talking about parameters}
According to the study in \cref{app:exp:param}, we set $R_w$ to 2 and $R_\lambda$ to 2.5 by default. The memory size is 1MB and the user-defined threshold $\Lambda$ is 25 by default.
All the experiments are conducted on a server with 18-core CPU (36 threads, Intel CPU i9-10980XE @3.00 GHz), which has 128GB memory. Programs are compiled with O2 optimization. 


% \subsubsection{Testbed}
% We have implemented P4 prototype \aname{} on a Tofino switch, with xxxxx. 
% % need Tofino configuration
% Our testbed has one host as the data plane directly connected through 40Gbps link. The control is connected through a 1Gbps link.
% The switch is configured with two forwarding rules for bidirectional packet forwarding.



\subsubsection{Datasets}
% We mainly use IP Trace dataset as our experimental dataset, which is an anonymized dataset collected from \cite{caida} and comprised of IP packets. We identify an flow by its source and destination IP addresses. The first 10M packets of the whole trace are used to conduct experiments, including about 0.4M distinct flows. 
% three real datasets and one synthetic dataset.
\begin{itemize}[leftmargin=0.15in]
    \item \ppp{ IP Trace: } An anonymized dataset collected from \cite{caida}, comprised of IP packets. We identify a flow by its source and destination IP addresses. The first 10M packets of the whole trace are used to conduct experiments, including about 0.4M distinct flows.
    \item \ppp{ Web Stream: } A dataset built from a spidered collection of web HTML documents \cite{webpage}. The first 10M packets of the entire trace are used to conduct experiments, including about 0.3M distinct flows.
    \item \ppp{ Hadoop Stream: } A  dataset built from real-world traffic distribution of HADOOP. The first 10M packets of the whole trace are used to conduct experiments, including about 20K distinct flows.
    % \item \ppp{Synthetic Datasets:} We generate \cite{webpoly} several synthetic datasets according to a Zipf distribution with different skewness for experiments, each of them consists of 32M items.
\end{itemize}

We use the IP Trace dataset as our experimental dataset by default. Experiments on more datasets can be found in \cref{app:exp:datset}.

% 与webpage同网站可下载
% The skewness of the dataset is about 1.0.


%\ppp{Computation Platform:}
%See details in appendix \ref{compute}.
%We conducted all the experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory. 
%Each processor has three levels of cache memory: one 32KB L1 data caches and one 32KB L1 instruction cache for each core, one 256KB L2 cache for each core, and one 15MB L3 cache shared by all cores.

\subsubsection{Evaluation Metrics}
\label{subsec:exp:metric}
\begin{itemize}[leftmargin=0.15in]
    \item \ppp{The Number of Outliers (\# Outliers):} 
    The number of flows whose absolute error of estimation is greater than the user-defined threshold $\Lambda$.
    We use it to evaluate the error-controlling accuracy.
    % The number of items for which we give a frequency estimation out of the provided range. 
    % We use it to evaluate the performance of error guarantee.
    \item \ppp{Average Absolute Error (AAE):} $\frac{1}{|U|} \sum\limits_{e_i \in U}|f(e_i)-\hat{f}(e_i)| $,
where $U$ is the set of the flows in the dataset, $f(e_i)$ is the true size of flow $e_i$, and $\hat{f}(e_i)$ is the estimated flow size. 
    % \item \ppp{Average Relative Error (ARE):} $\frac{1}{|U|} \sum\limits_{e_i \in U}\frac{|f(e_i)-\hat{f}(e_i)|}{f(e_i)} $.
% where $U$ is the set of flows in the dataset, $f(e_i)$ is the true frequency of flow $e_i$, and $\hat{f}(e_i)$ is the estimated frequency. 
    \item \ppp{Recall Rate:} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Psi}|}$, where $\Psi$ is the set of correct flows and $\Omega$ is the set of reported flows.
% It refers to the ratio of the number of correctly reported answers to that of all correct flows.
    \item \ppp{Throughput:} $\frac{N}{T}$, where $N$ is the number of operations and $T$ is the elapsed time. Throughput describes the processing speed of an algorithm, and we use Million of packets per second (Mpps) to measure the throughput.
\end{itemize}

We evaluate the performance of \aname{} and its competitors by above four metrics. As our goal is to control all errors below the user-defined threshold, when evaluating the accuracy, we \textit{pay more attention to the first metric \# Outliers than other metrics that evaluates the average error (\ie, AAE).}


\subsubsection{Implementation of Competitor}
We conduct experiments to compare the performance of \aname{} ("Ours" in figures) with seven competitors, including Count-Min (CM) \cite{cmsketch}, CU \cite{estan2002cusketch}, Space-Saving (SS) \cite{spacesaving}, Elastic \cite{yang2018elastic}, Coco \cite{zhang2021cocosketch}, HashPipe \cite{hashpipe}, and PRECISION\cite{ben2018efficient}. 
For CM and CU, we provide fast (CM\_fast/CU\_fast) and accurate (CM\_acc/CU\_acc) two versions, implementing 3 and 16 arrays respectively.
For Elastic, its light/heavy memory ratio is 3 as recommended \cite{yang2018elastic}.
For Coco, we set the number of arrays $d$ to 2 as recommended \cite{zhang2021cocosketch}.
For HashPipe, we set the number of pipeline stages $d$ to 6 as recommended \cite{hashpipe}.
And for PRECISION, we set the number of pipeline stages $d$ to 3 for best performance \cite{ben2018efficient}.
% All experiments are conducted on IP Trace dataset by default.

% AAE evaluates the accuracy of the estimated frequency.
% Steve: the "each truly/actually frequent reported item" is not clear to me. I think it's worth rewording more precisely.


% ARE evaluates the accuracy of the estimated frequency. 
% We use it in most of the tasks.

%\ppp{3) AE (Absolute Error):} $\sum_{e_i \in \mathbf{\Psi}} |d_i - \hat{d_i}|$, where $d_i$ is the real value and $\hat{d_i}$ is the estimated value. % We use it to evaluate the performance of cardinality and entropy estimation.



% \ppp{3) PR (Precision Rate):} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Omega}|}$, where $\Omega$ is the answer set reported by our algorithm.
% % PR refers to the ratio of the number of correctly reported answers to the number of all reported answers.

% \ppp{5) F1 Score:} $\frac{2 \times PR \times RR}{PR + RR}$. F1 Score is the harmonic mean of PR and RR, which are mentioned above. 

% \ppp{6) RE (Relative Error):} $\sum_{e_i \in \mathbf{\Psi}} |d_i - \hat{d_i}| / d_i$, where $d_i$ is the real value and $\hat{d_i}$ is the estimated value. % We use it to evaluate the performance of cardinality and entropy estimation.

% \ppp{7) WMRE (Weighted Mean Relative Error) \cite{kumar2004data}:} $\frac{\sum_{i=1}^{z}{|d_i - \hat{d_i}|}}{\sum_{i=1}^{z}\frac{d_i + \hat{d_i}}{2}}$, where $d_i$ and $\hat{d_i}$ are the real and estimated number of items with frequency $i$.
% % We use it to evaluate the performance of frequency distribution estimation.




==> vldb/Experiment/setup_new.tex <==

\presub
\subsection{Experimental Setup} \postsub
\label{subsec:exp:setup}

%\ppp{Implementation:}
%We have implemented \aname{} and all other algorithms in C++.
%The hash functions are implemented using the 32-bit Bob Hash (obtained from the open-source website \cite{bobhash}) with different initial seeds.


%\ppp{Datasets:}
%Shown in appendix \ref{exp:dat}.

\subsubsection{Implementation}
We have implemented \aname{} and related algorithms in C++. Here we use fast 32-bit Murmur Hashing \cite{murmur}, and different hash functions that affect accuracy little. Each bucket of \aname{} consists of a 32-bit total counter, a 16-bit collision counter, a 16-bit winner ID field, and a 1-bit lock flag. Mice filter occupies 20\% of total memory, and bucket size of it is fixed to 2 bits. All the experiments are conducted on a server with 18-core CPU (36 threads, Intel CPU i9-10980XE @3.00 GHz), which has 128GB memory. Programs are compiled with O2 optimization. 


\subsubsection{Testbed}
We have implemented P4 prototype \aname{} on a Tofino switch, with xxxxx. 
% need Tofino configuration
Our testbed has one host as the data plane directly connected through 40Gbps link. The control is connected through a 1Gbps link.
The switch is configured with two forwarding rules for bidirectional packet forwarding.



\subsubsection{Datasets}  
% three real datasets and one synthetic dataset.
\begin{itemize}[leftmargin=0.15in]
    \item \ppp{ IP Trace: } An anonymized dataset collected from \cite{caida}, comprised of IP packets. We identify an item by its source and destination IP addresses. The first 10M items of the whole trace are used to conduct experiments, including about 0.4M distinct items.
    \item \ppp{ Web Stream: } A transactional dataset built from a spidered collection of web HTML documents \cite{webpage}.The first 10M items of the whole trace are used to conduct experiments, including about 0.3M distinct items.
    \item \ppp{ Click Stream: } A click stream dataset built from a hungarian online news portal \cite{webpage}. We fetch the all 8M items of the dataset for our experiments, containing about 41K distinct items.
    \item \ppp{Synthetic Datasets:} We generate \cite{webpoly} several synthetic datasets according to a Zipf distribution with different skewness for experiments, each of them consists of 32M items.
\end{itemize}

% 与webpage同网站可下载
% The skewness of the dataset is about 1.0.


%\ppp{Computation Platform:}
%See details in appendix \ref{compute}.
%We conducted all the experiments on a machine with two 6-core processors (12 threads, Intel Xeon CPU E5-2620 @2 GHz) and 64 GB DRAM memory. 
%Each processor has three levels of cache memory: one 32KB L1 data caches and one 32KB L1 instruction cache for each core, one 256KB L2 cache for each core, and one 15MB L3 cache shared by all cores.

\subsubsection{Evaluation Metrics}
\label{subsec:exp:metric}
\begin{itemize}[leftmargin=0.15in]
    \item \ppp{The Number of Outliers (\# Outliers):} 
    The number of items whose errors of frequency estimation is greater than the user-defined threshold $\Lambda$.
    We use it to evaluate the accuracy.
    % The number of items for which we give a frequency estimation out of the provided range. 
    % We use it to evaluate the performance of error guarantee.
    \item \ppp{Average Absolute Error (AAE):} $\frac{1}{|U|} \sum\limits_{e_i \in U}|f(e_i)-\hat{f}(e_i)| $,
where $U$ is the set of items in the dataset, $f(e_i)$ is the true frequency of item $e_i$, and $\hat{f}(e_i)$ is the estimated frequency. 
    \item \ppp{Average Relative Error (ARE):} $\frac{1}{|U|} \sum\limits_{e_i \in U}\frac{|f(e_i)-\hat{f}(e_i)|}{f(e_i)} $,
where $U$ is the set of items in the dataset, $f(e_i)$ is the true frequency of item $e_i$, and $\hat{f}(e_i)$ is the estimated frequency. 
    \item \ppp{Throughput:} $\frac{N}{T}$, where $N$ is the number of operations and $T$ is the elapsed time. Throughput describes the processing speed of an algorithm, and we use Million of items per second (Mips) to measure the throughput.
\end{itemize}

We evaluate the performance of \aname{} and its competitors by the above four metrics. As our goal is to control all errors below the user-defined threshold, when evaluating the accuracy, we \textit{pay more attention to the first metric \# Outliers than other metrics that evaluates the average error (\ie, AAE and ARE).}

% AAE evaluates the accuracy of the estimated frequency.
% Steve: the "each truly/actually frequent reported item" is not clear to me. I think it's worth rewording more precisely.


% ARE evaluates the accuracy of the estimated frequency. 
% We use it in most of the tasks.

%\ppp{3) AE (Absolute Error):} $\sum_{e_i \in \mathbf{\Psi}} |d_i - \hat{d_i}|$, where $d_i$ is the real value and $\hat{d_i}$ is the estimated value. % We use it to evaluate the performance of cardinality and entropy estimation.



% \ppp{3) PR (Precision Rate):} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Omega}|}$, where $\Omega$ is the answer set reported by our algorithm.
% % PR refers to the ratio of the number of correctly reported answers to the number of all reported answers.

% \ppp{4) RR (Recall Rate):} $\frac{|\mathbf{\Psi} \cap \mathbf{\Omega}|}{|\mathbf{\Psi}|}$.
% % RR refers to the ratio of the number of correctly reported answers to the number of all correct items.

% \ppp{5) F1 Score:} $\frac{2 \times PR \times RR}{PR + RR}$. F1 Score is the harmonic mean of PR and RR, which are mentioned above. 

% \ppp{6) RE (Relative Error):} $\sum_{e_i \in \mathbf{\Psi}} |d_i - \hat{d_i}| / d_i$, where $d_i$ is the real value and $\hat{d_i}$ is the estimated value. % We use it to evaluate the performance of cardinality and entropy estimation.

% \ppp{7) WMRE (Weighted Mean Relative Error) \cite{kumar2004data}:} $\frac{\sum_{i=1}^{z}{|d_i - \hat{d_i}|}}{\sum_{i=1}^{z}\frac{d_i + \hat{d_i}}{2}}$, where $d_i$ and $\hat{d_i}$ are the real and estimated number of items with frequency $i$.
% % We use it to evaluate the performance of frequency distribution estimation.




==> vldb/Experiment/sim.tex <==
\presub
% \subsection{Experiments on Network-wide Applications} \postsub
\subsection{Experiments on Simulation} \postsub
\label{subsec:exp:sim}

In this section, we apply \aname{} to three common network-wide applications and evaluate the performance. We use NS2 \cite{ns2} to simulate network traffic based on leaf-spine topology, which consists of 16 hosts, 4 aggregation switches, and 4 core switches (32 duplex-links in total).
% Bucket size of filter level is fixed to 2 bits.

\input{vldb/Figures/sim/intersection.tex}

% \subsubsection{Range Intersection. }
\ppp{Accuracy Improvement (Figure  \ref{subfig:sim:intersection:10}, \ref{subfig:sim:intersection:25}):} 
\label{subsubsec:exp:intersec}
We find that accuracy of \aname{} can be improved up to $100\times$ by network-wide information.
We conduct experiments on 0.1M unique flows and 8.7M packets in total, no packet loop or drop occurs.
For each flow, the controller scans all sketches in the forwarding path respectively, and reports the intersection of estimated flow size intervals.
% The figures illustrate how the number of outliers changes by the number of sketches with different $\Lambda$.
The results show that more implemented sketches lead to fewer outliers.
% 利用全网信息有效加快了Outliers下降速度

\input{vldb/Figures/sim/anomaly.tex}




\ppp{Detecting Packet Drops and Loops (Figure  \ref{subfig:sim:anomaly:drop}, Figure \ref{subfig:sim:anomaly:loop}):} 
\label{subsubsec:exp:drop}
% \whb{!!!note: add theoretical parameters setting to Application part}
We find that \aname{} achieves high and stable accuracy in both packet drop detection and loop detection.
For packet drop, we simulate for about 100ms, and randomly shut down a duplex-link in the network for 25ms.
The result shows that when memory usage is about 180KB, \aname{} achieves 99\% recall rate with $\Lambda=10$.
For loop detection, we let 1\% flows loop between two selected adjacent switches for over 20 times and also generate a 100ms trace. 
The result shows that when memory usage is about 180KB, \aname{} achieves 99\% recall rate with $\Lambda=10$.
% 增加内存显著增加 Recall，eps/2时保证100
% Precison维持100
% 调节threshold改变两者的重心





% \ppp{Packet Drop Detection (Figure  \ref{subfig:sim:anomaly:drop}):} 
% \label{subsubsec:exp:drop}
% % \whb{!!!note: add theoretical parameters setting to Application part}
% We find that \aname{} achieves high and stable accuracy in packet drop detection.
% We simulate for about 100ms, and randomly shut down a duplex-link in the network for 25ms.
% % The trace includes about 0.1M flows and 2.6M packets.
% For each flow, we query sketches of two adjacent switches in the forwarding path and compare the estimated flow size intervals.
% We report an abnormal packet drop when the intersection is empty and estimated flow size is smaller than the previous one. 
% % When \aname{} achieves zero outlier, it guarantees 100\% recall rate for flows which drops over $2 \Lambda$ packets. 
% % For a fixed threshold $\Lambda$, we calculate the accuracy over flows which drop over $2\Lambda$ packets.
% The result shows that when memory usage is about 180KB, \aname{} achieves 99\% recall rate with $\Lambda=10$.
% % 增加内存显著增加 Recall，eps/2时保证100
% % Precison维持100
% % 调节threshold改变两者的重心

% \ppp{Packet Loop Detection (Figure  \ref{subfig:sim:anomaly:loop}):} 
% \label{subsubsec:exp:loop}
% % \whb{!!!note: add theoretical parameters setting to Application part}
% We find that \aname{} achieves high and stable accuracy in packet loop detection.
% We let 1\% flows loop between two selected adjacent switches for over 20 times and also generate a 100ms trace. % , including about 0.1M flows and 2.7M packets.
% % For each flow, we query sketches in the same way as packet drop detection, and report an abnormal packet loop when the intersection is empty and estimated flow size is bigger than the previous one. 
% For each flow, we report an abnormal packet loop when the intersection is empty and estimated flow size is bigger than the previous one. 
% % When \aname{} achieves zero outlier, it guarantees 100\% recall rate for flows which drops over $2 \Lambda$ packets. 
% % For a fixed threshold $\Lambda$.
% The accuracy is calculated over flows which loop over $2\Lambda$ times.
% The result shows that when memory usage is about 180KB, \aname{} achieves 99\% recall rate with $\Lambda=10$.
% % 增加内存显著增加 Recall，eps/2时保证100
% % Precison维持100
% % 调节threshold改变两者的重心

==> vldb/Experiment/testbed.tex <==

\vspace{-0.1in}
\presub
\subsection{Experiments on TestBed} \postsub
\label{subsec:exp:testbed}


In this section, we evaluate the accuracy of \aname{} implemented on the Tofino switch.

\input{vldb/Figures/testbed/acc}

\ppp{Accuracy in Different SRAM Size (Figure  \ref{fig:testbed:acc}):}
%
We send 40M packets selected from the IP Trace dataset and Hadoop dataset with 40Gbps link speed on a end-host connected to the Tofino switch, and evaluate the AAE and the number of outliers of \aname{} using SRAM of different sizes.
%
As shown in Figure \ref{fig:testbed:acc}, for IP Trace dataset, when \aname{} uses more than 368KB SRAM, it can ensure that there are no outliers, and its AAE is within 4Kbps. For Hadoop dataset, when \aname{} uses more than 92KB SRAM, it can ensure that there are no outliers, and its AAE is within 10Kbps.


==> vldb/Experiment/throughput.tex <==
\presub
\subsection{Experiments on Throughput} \postsub
\label{subsec:exp:throughput}

We find that \aname{} is not only more accurate and versatile but also faster than other algorithms. Throughput measures the processing speed of an algorithm. In this section, we compare the throughput among \aname{}, CM sketch, and CU sketch. The memory size is fixed to 500KB for all algorithms, and we perform 10M item insertions and 10M frequency queries on the CAIDA and Web Page datasets. Some additional parts for specific tasks are removed in advance, such as auxiliary arrays for recording top-k items and frequency distribution.

\input{vldb/Figures/application/tp.tex}

\ppp{Item Insertion (Figure \ref{subfig:tp:insert}):} The results show that the throughput of \aname{} on the CAIDA dataset is 10.02Mips, 1.12 times faster than CM sketch, 1.52 times faster than CU sketch and 3.93 times faster than ASketch. For the Web Page dataset, \aname{} performs 11.1Mips throughput, which is about 1.28, 1.44 and 2.57 times greater than CM sketch, CU sketch and ASketch, respectively.

\ppp{Frequency Query (Figure \ref{subfig:tp:query}):} For the CAIDA dataset, the throughput of \aname{} is 11.72Mips, which means \aname{} is 1.25, 1.29 and 2.42 times faster than CM Sketch, CU Sketch and ASketch. For the Web Page dataset, \aname{} provides 11.1Mips throughput, which is about 1.44, 1.46 and 1.75 times greater than CM sketch, CU sketch and ASketch, respectively.

==> vldb/Experiment/throughput_V3.tex <==
\presub
\subsection{Experiments on Throughput} \postsub
\label{subsec:exp:throughput}

In this section, we conduct experiments to illustrate the throughput of \aname{} and explore how the throughput changes in different circumstances. For different tasks, we choose different metrics and approaches.

\subsubsection{General Throughput. }

We find that \aname{} is not only accurate but also fast. Throughput measures the processing speed of an algorithm, we compare the throughput among \aname{}, CM Sketch, CU Sketch, Space-Saving, ElasticSketch and CocoSketch. We perform 10M item insertions and 10M queries on the IP Trace and Web Stream datasets.
% The memory size is fixed to 2MB for other algorithms except \aname{} since they are almost unaffected by size without consideration of cache.
The memory size is fixed to 2MB for all algorithms.
Specifically for \aname{}, we set $R_w$ to 2,  $R_\lambda$ to 2.5, $\Lambda$ to 25. And we provide an alternative version of \aname{} without mice filter ("Raw" in the figures), which sacrifice tolerable accuracy for significant speed boost.
% Some additional parts for specific tasks are not implemented, such as the unbiased counter for unbiased estimation.

\input{vldb/Figures/tp_new2/tp_general}

\ppp{Item Insertion (Figure \ref{subfig:tp:insert}):} The figures show that the throughput of \aname{} and \aname{} (Raw) on the IP Trace dataset is 25.40Mips and 51.29Mips respectively. The raw version is comparable with CM Sketch (fast) and CocoSketch, 1.42 times faster than CU Sketch (fast), 1.43 times faster than ElasticSketch, 3.40 $\sim$ 6.65 times faster than CM Sketch (accurate), CU Sketch (accurate) and Space-Saving. For the Web Stream dataset, two version \aname{}es perform 30.41Mips and 64.70Mips throughput respectively, the raw version is about 1.17 times faster than CM Sketch (fast), 1.64 times faster than CU Sketch (fast), 1.89 times faster than ElasticSketch, and 3.58 $\sim$ 7.72 times faster than others.

\ppp{Frequency Query (Figure \ref{subfig:tp:query}):} For the IP Trace dataset, the throughput of two \aname{}es is 31.29Mips and 66.89Mips respectively, which means the raw version is about 1.22 times faster than CM Sketch (fast) and CU Sketch (fast), 2.14 times faster than ElasticSketch, and 2.22 $\sim$ 5.62 times faster than others. For the Web Stream dataset, two \aname{}es provide 34.49Mips and 84.79Mips throughput respectively, the raw one is comparable with CocoSketch, about 1.57 times faster than CM Sketch (fast) and CU Sketch (fast), 1.51 times faster than ElasticSketch, and 2.68 $\sim$ 7.22 times faster than others.

%\input{vldb/Figures/tp_new/tp_acc}

%\ppp{Throughput under Zero Outlier (Figure \ref{subfig:tp_acc:insert},\ref{subfig:tp_acc:query}):} We further study the throughputs of experimental algorithms with their minimum memory to achieve zero outlier (given in Section \ref{subsubsec:exp:range}), respectively. The result shows that \aname{} is still 1.11 $\sim$ 7.83 times faster than others. 

% \subsubsection{Load Factor. }
% \subsubsection{Load Rate. }
% \label{subsubsec:exp:tp_lf}
% % Load factor describes the space utilization of a data structure.
% Load Rate describes the load progress of a experimental dataset.
% Differing from compared algorithms, \aname{} has a multi-layer structure. Hence the throughput also depends on the average number of accessed layers.
% We conduct experiments on the IP Trace dataset to explore the relation between the load rate and throughput of \aname{}.
% For reference, we also plot the throughput of CM Sketch (fast) and CU Sketch (fast) under different load rates.
% % We find that when load factor exceeds xxx, the throughput of \aname{} drops fiercely. As long as the memory is not particularly precious, we recommend using more space in exchange for faster processing speed.

% % figure & analysis

% \input{vldb/Figures/tp_new/tp_lr.tex}

% \ppp{Load Rate vs. Throughput (Figure \ref{subfig:tp_lr:insert},\ref{subfig:tp_lr:query}):}
% % \ppp{Item Insertion (Figure \ref{subfig:tp_lr:insert}):} 
% The figures show that the throughput of \aname{} goes down as load rate grows. The throughput of CM Sketch and CU Sketch is almost independent from the load rate.
% % The figures show that the throughput of CM Sketch and CU Sketch is almost independent from the load rate, while the throughput of \aname{} goes down as load rate grows.
% % can be easily found
% It shows that the 4MB \aname{} has a higher throughput than the 2MB one, because the smaller \aname{} records more early-arrived but infrequent items in the top layers. 
% For this reason, as long as the memory is not particularly precious, we recommend offering more space in exchange for faster processing speed.
% % When load factor is less than 0.4, 2MB \aname{} has a transcendent insertion throughput compared with CM Sketch and CU Sketch.

% \ppp{Frequency Query (Figure \ref{subfig:tp_lr:query}):}
% It is shown that when load factor is less than 0.6, \aname{} has a higher query throughput than that of CM Sketch and CU Sketch. 

%\subsubsection{Parameter $R_w$. }
%$R_w$ depicts the decreasing portion of bucket numbers for adjacent two layers. The higher $R_w$ is, the more buckets top layers include, and therefore it has a considerable influence on the average layer where items recorded. For the same reason explained in section \ref{subsubsec:exp:tp_lf}, throughput can be decided by $R_w$. We conduct experiments on the IP Trace dataset to explore how the parameter $R_w$ of \aname{} affects the throughput.

% figure & analysis
%\input{vldb/Figures/tp_new/tp_rw}

%\ppp{$R_w$ vs. Throughput (Figure %\ref{subfig:tp_rw:insert},\ref{subfig:tp_rw:query}):} 
%As the figure shows, when $R_w$ is less than 4, the throughput of \aname{} is affected by $R_w$ greatly. And when $R_w$ is higher than 4, the average layer of items changes little, since the insertion throughput stops growing at about 60Mips. The query throughput has similar curves, and eventually converges to 65Mips. 

% \ppp{Frequency Query (Figure \ref{subfig:tp_rw:query}):}

\subsubsection{Hash Function Call. }

In common sketch algorithms, hash function always has higher computation complexity than other parts and affects the throughput a lot. Differed from prior sketches, \aname{} has a multi-layer structure. Hence the number of hash function calls is dynamic varied when performing insertions and queries. 
We conduct experiments on the IP Trace dataset to explore the relation between memory size and average number of hash function calls.

\input{vldb/Figures/tp_new2/tp_hash}

\ppp{# Function Calls vs. Memory Size (Figure \ref{subfig:tp:hash_inser},\ref{subfig:tp:hash_query}):} The figures show that average hash function calls of the raw version \aname{} goes down rapidly as memory grows, and finally converges to 1.  \aname{} with 2-array mice fitler finally converges to 3 for 2 extra calls in the filter.
% CM Sketch calls hash function 3 times per operation
% The figures show that the throughput of CM Sketch and CU Sketch is almost independent from the load rate, while the throughput of \aname{} goes down as load rate grows.
% can be easily found
Smaller \aname{} records more early-arrived but infrequent items in the top layers, resulting in more hash function calls and poor throughput.
For this reason, as long as the memory is not particularly precious, we recommend offering more space in exchange for faster processing speed.

% figure & analysis

% We find that ...



==> vldb/Experiment/throughput_new.tex <==
\presub
\subsection{Comparison on Throughput} \postsub
\label{subsec:exp:throughput}

In this section, we conduct experiments to illustrate the throughput of \aname{} and explore how the throughput changes in different circumstances. For different tasks, we choose different metrics and approaches.

\subsubsection{General Throughput. }

We find that \aname{} is not only accurate but also fast. Throughput measures the processing speed of an algorithm, we compare the throughput among \aname{}, CM Sketch, CU Sketch, Augmented Sketch, Space-Saving, and HeavyGuardian. We perform 10M item insertions and 10M queries on the IP Trace and Web Stream datasets. The memory size is fixed to 2MB for other algorithms except \aname{} since they are almost unaffected by size without consideration of cache. Specifically for \aname{}, we set $R_w$ to 2,  $R_\lambda$ to 2.5, $\Lambda$ to 25, and provide two versions with different sizes. Some additional parts for specific tasks are not implemented, such as the unbiased counter for unbiased estimation.

\input{vldb/Figures/tp_new/newtp.tex}

\ppp{Item Insertion (Figure \ref{subfig:tp:insert}):} The figures show that the throughput of 2MB \aname{} and 4MB \aname{} on the IP Trace dataset is 41.56Mips and 50.06Mips respectively, comparable with CM Sketch (fast), 1.23 $\sim$ 1.49 times faster than CU Sketch (fast), 1.37 $\sim$ 1.65 times faster than HeavyGuardian, and 3.49 $\sim$ 8.31 times faster than CM Sketch (accurate), CU Sketch (accurate), Augmented Sketch and Space-Saving. For the Web Stream dataset, 2MB and 4MB \aname{} perform 61.42Mips and 59.36Mips throughput respectively, which is about 1.31 $\sim$ 1.35 times faster than CM Sketch (fast), 1.69 $\sim$ 1.74 times faster than CU Sketch (fast), 1.07 $\sim$ 1.11 times faster than HeavyGuardian, and 4.72 $\sim$ 7.47 times faster than others.

\ppp{Frequency Query (Figure \ref{subfig:tp:query}):} For the IP Trace dataset, the throughput of 2MB and 4MB \aname{} is 53.14Mips and 54.64Mips respectively, which means \aname{} is about 1.06 $\sim$ 1.11 times faster than CM Sketch (fast) and CU Sketch (fast), 1.67 $\sim$ 1.72 times faster than HeavyGuardian, and 2.79 $\sim$ 4.55 times faster than others. For the Web Stream dataset, 2MB and 4MB \aname{} provide 75.16Mips and 71.66Mips throughput respectively, which is about 1.48 $\sim$ 1.60 times faster than CM Sketch (fast) and CU Sketch (fast), 1.25 $\sim$ 1.31 times faster than HeavyGuardian, and 3.18 $\sim$ 6.43 times faster than others.

%\input{vldb/Figures/tp_new/tp_acc}

%\ppp{Throughput under Zero Outlier (Figure \ref{subfig:tp_acc:insert},\ref{subfig:tp_acc:query}):} We further study the throughputs of experimental algorithms with their minimum memory to achieve zero outlier (given in Section \ref{subsubsec:exp:range}), respectively. The result shows that \aname{} is still 1.11 $\sim$ 7.83 times faster than others. 

% \subsubsection{Load Factor. }
\subsubsection{Load Rate. }
\label{subsubsec:exp:tp_lf}
% Load factor describes the space utilization of a data structure.
Load Rate describes the load progress of a experimental dataset.
Differing from compared algorithms, \aname{} has a multi-layer structure. Hence the throughput also depends on the average number of accessed layers.
We conduct experiments on the IP Trace dataset to explore the relation between the load rate and throughput of \aname{}.
For reference, we also plot the throughput of CM Sketch (fast) and CU Sketch (fast) under different load rates.
% We find that when load factor exceeds xxx, the throughput of \aname{} drops fiercely. As long as the memory is not particularly precious, we recommend using more space in exchange for faster processing speed.

% figure & analysis

\input{vldb/Figures/tp_new/tp_lr.tex}

\ppp{Load Rate vs. Throughput (Figure \ref{subfig:tp_lr:insert},\ref{subfig:tp_lr:query}):}
% \ppp{Item Insertion (Figure \ref{subfig:tp_lr:insert}):} 
The figures show that the throughput of \aname{} goes down as load rate grows. The throughput of CM Sketch and CU Sketch is almost independent from the load rate.
% The figures show that the throughput of CM Sketch and CU Sketch is almost independent from the load rate, while the throughput of \aname{} goes down as load rate grows.
% can be easily found
It shows that the 4MB \aname{} has a higher throughput than the 2MB one, because the smaller \aname{} records more early-arrived but infrequent items in the top layers. 
For this reason, as long as the memory is not particularly precious, we recommend offering more space in exchange for faster processing speed.
% When load factor is less than 0.4, 2MB \aname{} has a transcendent insertion throughput compared with CM Sketch and CU Sketch.

% \ppp{Frequency Query (Figure \ref{subfig:tp_lr:query}):}
% It is shown that when load factor is less than 0.6, \aname{} has a higher query throughput than that of CM Sketch and CU Sketch. 

%\subsubsection{Parameter $R_w$. }
%$R_w$ depicts the decreasing portion of bucket numbers for adjacent two layers. The higher $R_w$ is, the more buckets top layers include, and therefore it has a considerable influence on the average layer where items recorded. For the same reason explained in section \ref{subsubsec:exp:tp_lf}, throughput can be decided by $R_w$. We conduct experiments on the IP Trace dataset to explore how the parameter $R_w$ of \aname{} affects the throughput.

% figure & analysis
%\input{vldb/Figures/tp_new/tp_rw}

%\ppp{$R_w$ vs. Throughput (Figure %\ref{subfig:tp_rw:insert},\ref{subfig:tp_rw:query}):} 
%As the figure shows, when $R_w$ is less than 4, the throughput of \aname{} is affected by $R_w$ greatly. And when $R_w$ is higher than 4, the average layer of items changes little, since the insertion throughput stops growing at about 60Mips. The query throughput has similar curves, and eventually converges to 65Mips. 

% \ppp{Frequency Query (Figure \ref{subfig:tp_rw:query}):}


% \subsubsection{Hash Function Call. }

% Hash function has comparably higher computation complexity than other parts of a sketch and affects the throughput a lot. Differed from prior sketches, \aname{} has a multi-layer structure. Hence the number of hash function calls is dynamic when performing insertions and queries for \aname{}. 

% figure & analysis

% We find that ...



==> vldb/Figures/app/change.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/change_f1-crop.pdf}
		\end{center}
		}
		\label{subfig:app:change:f1}
		\end{minipage}
	}
	%
	\subfigure[Throughput]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/change_thp-crop.pdf}
		\end{center}
		}
		\label{subfig:app:change:thp}
		\end{minipage}
	}
	%
    \caption{Evaluation on finding Heavy Changes.}
    \prefig
    %\vspace{-0.1in}
	\label{fig:app:change}
\end{figure}

==> vldb/Figures/app/persist.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/persistent_f1-crop.pdf}
		\end{center}
		}
		\label{subfig:app:persist:f1}
		\end{minipage}
	}
	%
	\subfigure[Throughput]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/persistent_thp-crop.pdf}
		\end{center}
		}
		\label{subfig:app:persist:thp}
		\end{minipage}
	}
	%
    \caption{Evaluation on finding Persistent Items.}
    \postfig
    %\vspace{-0.1in}
	\label{fig:app:persist}
\end{figure}

==> vldb/Figures/app/super.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/super_f1-crop.pdf}
		\end{center}
		}
		\label{subfig:app:super:f1}
		\end{minipage}
	}
	%
	\subfigure[Throughput]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/app/super_thp-crop.pdf}
		\end{center}
		}
		\label{subfig:app:super:thp}
		\end{minipage}
	}
	%
    \caption{Evaluation on finding Super-Spreaders.}
    \postfig
    %\vspace{-0.1in}
	\label{fig:app:super}
\end{figure}

==> vldb/Figures/app_new/freq_aae.tex <==

% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_are:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_are:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{ARE of Frequency Estimation.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newfreq_are_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newfreq_are_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:fe_are:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{ARE of Frequency Estimation.}
	\label{fig:app:fe_are}
\postfig
\end{figure}

\begin{figure}[htbp]
%\vspace{2cm}
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newfreq_aae_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newfreq_aae_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:fe_aae:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE of Frequency Estimation.}
	\label{fig:app:fe_aae}
\postfig
\end{figure}


% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_aae:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_aae:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{AAE of Frequency Estimation.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	%
% 	\postfig
% \end{figure}



==> vldb/Figures/app_new/range_dataset.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps25_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:range25:webpage}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps25_kosarak.pdf}
        \presubfigcaption
        \caption{Click Stream}
		\label{subfig:app:range25:kosarak}
        \end{subfigure}
        
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps25_syn003.pdf}
        \presubfigcaption
        \caption{Synthetic with Skewness=0.3}
		\label{subfig:app:range25:syn003}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps25_syn030.pdf}
        \presubfigcaption
        \caption{Synthetic with Skewness=3.0}
		\label{subfig:app:range25:syn030}
        \end{subfigure}
        
    \prefigcaption
    \caption{\# Outliers for Different Datasets.}
	\label{fig:app:range_dataset}
\postfig
\end{figure}

==> vldb/Figures/app_new/range_eps.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps5_caida.pdf}
        \presubfigcaption
        \caption{$\Lambda$=5}
		\label{subfig:app:range5:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps10_caida.pdf}
        \presubfigcaption
        \caption{$\Lambda$=10}
		\label{subfig:app:range10:caida}
        \end{subfigure}
    
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps25_caida.pdf}
        \presubfigcaption
        \caption{$\Lambda$=25}
		\label{subfig:app:range25:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new/newrange_eps50_caida.pdf}
        \presubfigcaption
        \caption{$\Lambda$=50}
		\label{subfig:app:range50:caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{\# Outliers for Different $\Lambda$.}
	\label{fig:app:range_eps}
\postfig
\end{figure}

==> vldb/Figures/app_new/range_mem.tex <==
\begin{figure}[htbp]
\prefig
    \centering
	\includegraphics[width=0.85\linewidth, ]{vldb/Figures/app_new2/minmem_eps25.pdf}
    \prefigcaption
    \caption{Memory Consumption under Zero Outlier.}
	\label{fig:app:outlier_minmem}
\postfig
\end{figure}

==> vldb/Figures/app_new2/avg_err.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/are_caida_eps25.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/are_webpage_eps25.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:fe_are:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{ARE of Frequency Estimation.}
	\label{fig:app:fe_are}
\postfig
\end{figure}

\begin{figure}[htbp]
%\vspace{2cm}
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/aae_caida_eps25.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/aae_webpage_eps25.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:fe_aae:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE of Frequency Estimation.}
	\label{fig:app:fe_aae}
\postfig
\end{figure}


==> vldb/Figures/app_new2/avg_err_app.tex <==


\begin{figure}[htbp]
%\vspace{2cm}
% \prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/aae_caida_eps25.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/aae_synthesis030_eps25.pdf}
        \presubfigcaption
        \caption{Synthetic (Skewness=3.0)}
		\label{subfig:app:fe_aae:syn030}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE on Different Datasets.}
	\label{fig:exp_app:aae}
\postfig
\end{figure}

\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/are_caida_eps25.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:app:fe_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/are_synthesis030_eps25.pdf}
        \presubfigcaption
        \caption{Synthetic (Skewness=3.0)}
		\label{subfig:app:fe_are:syn030}
        \end{subfigure}
    \prefigcaption
    \caption{ARE on Different Datasets.}
	\label{fig:exp_app:are}
\postfig
\end{figure}

==> vldb/Figures/app_new2/avg_err_v2.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/are_caida_eps25.pdf}
        \presubfigcaption
        \caption{ARE Evaluation}
		\label{subfig:app:fe_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/aae_caida_eps25.pdf}
        \presubfigcaption
        \caption{AAE Evaluation}
		\label{subfig:app:fe_aae:caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{Accuracy of Average Error.}
	\label{fig:app:avg_err}
\postfig
\end{figure}


==> vldb/Figures/app_new2/hh.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/newhh_caida_eps25_100.pdf}
        \presubfigcaption
        \caption{$T = 100$}
		\label{subfig:app:hh100:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/newhh_caida_eps25_1000.pdf}
        \presubfigcaption
        \caption{$T = 1000$}
		\label{subfig:app:hh1000:caida}
        \end{subfigure}
        
    \prefigcaption
% \vspace{-0.1in}
    \caption{Number of Outliers in Elephant Keys.}
	\label{fig:app:hh}
\postfig
\end{figure}


==> vldb/Figures/app_new2/outlier_dataset.tex <==
\begin{figure}[htbp]
% \prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_webpage_eps25.pdf}
        \presubfigcaption
        \caption{Web Stream}
		\label{subfig:app:range25:webpage}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_imc_eps25.pdf}
        \presubfigcaption
        \caption{University Data Center}
		\label{subfig:app:range25:kosarak}
        \end{subfigure}
        
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_synthesis003_eps25.pdf}
        \presubfigcaption
        \caption{Synthetic (Skewness=0.3)}
		\label{subfig:app:range25:syn003}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_synthesis030_eps25.pdf}
        \presubfigcaption
        \caption{Synthetic (Skewness=3.0)}
		\label{subfig:app:range25:syn030}
        \end{subfigure}
        
    \prefigcaption
    \caption{\# Outliers on Different Datasets.}
	\label{fig:app:range_dataset}
\postfig
\end{figure}

==> vldb/Figures/app_new2/outlier_eps.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps5.pdf}
        \presubfigcaption
        \caption{$\Lambda$=5}
		\label{subfig:app:range5:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps10.pdf}
        \presubfigcaption
        \caption{$\Lambda$=10}
		\label{subfig:app:range10:caida}
        \end{subfigure}
    
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps25.pdf}
        \presubfigcaption
        \caption{$\Lambda$=25}
		\label{subfig:app:range25:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps50.pdf}
        \presubfigcaption
        \caption{$\Lambda$=50}
		\label{subfig:app:range50:caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{\# Outliers for Different $\Lambda$.}
	\label{fig:app:range_eps}
\postfig
\end{figure}

==> vldb/Figures/app_new2/outlier_lambda.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps5.pdf}
        \presubfigcaption
        \caption{$\Lambda$=5}
		\label{subfig:app:range5:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/app_new2/outlier_caida_eps25.pdf}
        \presubfigcaption
        \caption{$\Lambda$=25}
		\label{subfig:app:range25:caida}
        \end{subfigure}
        
    \prefigcaption
    % \vspace{-0.1in}
    \caption{\# Outliers in Different $\Lambda$.}
	\label{fig:app:range_eps}
\postfig
\end{figure}

==> vldb/Figures/app_new2/outlier_minmem.tex <==
\begin{figure}[htbp]
\prefig
    \centering
	\includegraphics[width=0.85\linewidth, ]{vldb/Figures/app_new2/minmem_eps25.pdf}
    \prefigcaption
    \caption{Memory Consumption under Zero Outlier.}
	\label{fig:app:outlier_minmem}
\postfig
\end{figure}

==> vldb/Figures/application/cd.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cd_re_caida.pdf}
		\end{center}
		}
		\label{subfig:app:cd:caida}
		\end{minipage}
	}
	%
	\subfigure[WebPage]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cd_re_webpage.pdf}
		\end{center}
		}
		\label{subfig:app:cd:webpage}
		\end{minipage}
	}
	\prefigcaption
    \caption{RE of Cardinality Estimation.}
    %\vspace{-0.1in}
	\label{fig:app:fd}
	\postfig
\end{figure}


==> vldb/Figures/application/cd_fd_etp.tex <==
\begin{figure*}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/cd_re_caida.pdf}
        \presubfigcaption
        \caption{Cardinality}
        \label{subfig:app:cd}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.225\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/fd_wmre_caida.pdf}
        \presubfigcaption
        \caption{Frequency Distribution}
        \label{subfig:app:fd}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.225\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/etp_real_caida.pdf}
        \presubfigcaption
        \caption{Real-time Entropy}
        \label{subfig:app:etp_real}
        \end{subfigure}
    \hfill
        \begin{subfigure}{0.225\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/etp_re_caida.pdf}
        \presubfigcaption
        \caption{RE of Entropy}
        \label{subfig:app:etp_re}
        \end{subfigure}
    \prefigcaption
    \caption{Performance of Cardinality, Frequency Distribution and Entropy Estimation.}
    \label{fig:app:cd_fd_etp}
    \postfig
\end{figure*}
% \begin{figure*}[htbp]
%  \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{-0.3cm}
% \prefig
%     \centering
%  	    \begin{subfigure}{0.225\textwidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/cd_re_caida.pdf}
%         \precaption
%         \caption{Cardinality}
%         \label{subfig:app:cd}
%         \end{subfigure}
%     \hfill
%  	    \begin{subfigure}{0.225\textwidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/fd_wmre_caida.pdf}
%         \precaption
%         \caption{Frequency Distribution}
%         \label{subfig:app:fd}
%         \end{subfigure}
%     \hfill
%  	    \begin{subfigure}{0.225\linewidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/etp_real_caida.pdf}
%         \precaption
%         \caption{Real-time Entropy}
%         \label{subfig:app:etp_real}
%         \end{subfigure}
%     \hfill
%         \begin{subfigure}{0.225\linewidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/etp_re_caida.pdf}
%         \precaption
%         \caption{RE of Entropy}
%         \label{subfig:app:etp_re}
%         \end{subfigure}
%     \precaption
%     \caption{Performance of Cardinality, Frequency Distribution and Entropy Estimation.}
%     \label{fig:app:cd_fd_etp}
% \postfig
% \end{figure*}

==> vldb/Figures/application/cpr.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cpr_are_caida.pdf}
		\end{center}
		}
		\label{subfig:cpr:high_are:caida}
		\end{minipage}
	}
	%
	\subfigure[AAE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cpr_aae_caida.pdf}
		\end{center}
		}
		\label{subfig:cpr:high_aae:caida}
		\end{minipage}
	}
	\prefigcaption
    \caption{Performance of Compressed \aname{}.}
    %\vspace{-0.1in}
	\label{fig:cpr:high:caida}
	\postfig
\end{figure}


==> vldb/Figures/application/cpr_low.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cpr_are_caida_low.pdf}
		\end{center}
		}
		\label{subfig:cpr:low_are:caida}
		\end{minipage}
	}
	%
	\subfigure[AAE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/cpr_aae_caida_low.pdf}
		\end{center}
		}
		\label{subfig:cpr:low_aae:caida}
		\end{minipage}
	}
    \caption{Performance of Compressed Under-estimating \aname{}.}
    %\vspace{-0.1in}
	\label{fig:cpr:low:caida}
	\postfig
\end{figure}


==> vldb/Figures/application/epd.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/epd_are_caida.pdf}
		\end{center}
		}
		\label{subfig:epd:high_are:caida}
		\end{minipage}
	}
	%
	\subfigure[AAE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/epd_aae_caida.pdf}
		\end{center}
		}
		\label{subfig:epd:high_aae:caida}
		\end{minipage}
	}
	\prefigcaption
    \caption{Performance of Expanded \aname{}.}
    %\vspace{-0.1in}
	\label{fig:epd:high:caida}
	\postfig
\end{figure}


==> vldb/Figures/application/etp.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[Real-time Entropy Estimation]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/etp_real_caida.pdf}
		\end{center}
		}
		\label{subfig:app:etp_real:caida}
		\end{minipage}
	}
	%
	\subfigure[RE of Entropy Estimation]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/etp_re_caida.pdf}
		\end{center}
		}
		\label{subfig:app:etp_re:caida}
		\end{minipage}
	}
	\prefigcaption
    \caption{Performance of Entropy Estimation.}
    %\vspace{-0.1in}
	\label{fig:app:etp:caida}
	\postfig
\end{figure}


==> vldb/Figures/application/exopfig.tex <==
\begin{figure*}[htbp]
% \prefig

\vspace{0.1in}
    \centering
 	    \begin{subfigure}{0.195\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/epd_are_caida.pdf}
        \presubfigcaption
        \caption{Expansion}
        \label{subfig:exop:epd}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.197\textwidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/cpr_are_caida.pdf}
        \presubfigcaption
        \caption{Compression}
        \label{subfig:exop:cpr}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.197\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/mrg_are_caida.pdf}
        \presubfigcaption
        \caption{Mergence}
        \label{subfig:exop:mrg}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.197\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/gen_are_caida.pdf}
        \presubfigcaption
        \caption{Heavy \aname{}}
        \label{subfig:exop:heavy}
        \end{subfigure}
    \hfill
        \begin{subfigure}{0.195\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/application/gen2_are_caida.pdf}
        \presubfigcaption
        \caption{Light \aname{}}
        \label{subfig:exop:light}
        \end{subfigure}
    \prefigcaption
    \caption{Performance of Extra Operations.}
    \label{fig:exop}
    \postfig
\end{figure*}
% \begin{figure*}[htbp]
%  \setlength{\abovecaptionskip}{0.2cm}
% \setlength{\belowcaptionskip}{-0.3cm}
% \prefig
%     \centering
%  	    \begin{subfigure}{0.225\textwidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/cd_re_caida.pdf}
%         \precaption
%         \caption{Cardinality}
%         \label{subfig:app:cd}
%         \end{subfigure}
%     \hfill
%  	    \begin{subfigure}{0.225\textwidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/fd_wmre_caida.pdf}
%         \precaption
%         \caption{Frequency Distribution}
%         \label{subfig:app:fd}
%         \end{subfigure}
%     \hfill
%  	    \begin{subfigure}{0.225\linewidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/etp_real_caida.pdf}
%         \precaption
%         \caption{Real-time Entropy}
%         \label{subfig:app:etp_real}
%         \end{subfigure}
%     \hfill
%         \begin{subfigure}{0.225\linewidth}
%  	    \setlength{\abovecaptionskip}{-0.2cm}
%         \setlength{\belowcaptionskip}{-0.2cm}
%         \centering
%         \includegraphics[width=\textwidth]{vldb/Figures/application/etp_re_caida.pdf}
%         \precaption
%         \caption{RE of Entropy}
%         \label{subfig:app:etp_re}
%         \end{subfigure}
%     \precaption
%     \caption{Performance of Cardinality, Frequency Distribution and Entropy Estimation.}
%     \label{fig:app:cd_fd_etp}
% \postfig
% \end{figure*}

==> vldb/Figures/application/fd.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[CAIDA]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fd_wmre_caida.pdf}
		\end{center}
		}
		\label{subfig:app:fd:caida}
		\end{minipage}
	}
	%
	\subfigure[WebPage]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fd_wmre_webpage.pdf}
		\end{center}
		}
		\label{subfig:app:fd:webpage}
		\end{minipage}
	}
	\prefigcaption
    \caption{WMRE of Frequency Distribution Estimation.}
    %\vspace{-0.1in}
	\label{fig:app:fd}
	\postfig
\end{figure}


==> vldb/Figures/application/fe_are.tex <==

% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_are:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_are:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{ARE of Frequency Estimation.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:fe_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_are_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:fe_are:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{ARE of Frequency Estimation.}
	\label{fig:app:fe_are}
\postfig
\end{figure}

\begin{figure}[htbp]
%\vspace{2cm}
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:fe_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:fe_aae:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE of Frequency Estimation.}
	\label{fig:app:fe_aae}
\postfig
\end{figure}


% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_aae:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/fe_aae_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:fe_aae:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{AAE of Frequency Estimation.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	%
% 	\postfig
% \end{figure}



==> vldb/Figures/application/gen_heavy.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen_are_caida.pdf}
		\end{center}
		}
		\label{subfig:gen:heavy_are:caida}
		\end{minipage}
	}
	%
	\subfigure[AAE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen_aae_caida.pdf}
		\end{center}
		}
		\label{subfig:gen:heavy_aae:caida}
		\end{minipage}
	}
	\prefigcaption
    \caption{Performance of Heavy \aname{}.}
    %\vspace{-0.1in}
	\label{fig:gen:heavy}
	\postfig
\end{figure}


==> vldb/Figures/application/gen_light.tex <==
\begin{figure}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen2_are_caida.pdf}
		\end{center}
		}
		\label{subfig:gen:light_are:caida}
		\end{minipage}
	}
	%
	\subfigure[AAE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen2_aae_caida.pdf}
		\end{center}
		}
		\label{subfig:gen:light_aae:caida}
		\end{minipage}
	}
	\prefigcaption
    \caption{Performance of Light \aname{}.}
    %\vspace{-0.1in}
	\label{fig:gen:light}
	\postfig
\end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen2_are_caida.pdf}
        \presubfigcaption
        \caption{ARE}
		\label{subfig:gen:light_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/gen2_aae_caida.pdf}
        \presubfigcaption
        \caption{AAE}
		\label{subfig:gen:light_aae:caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{Performance of Light \aname{}.}
	\label{fig:gen:light}
\postfig
\end{figure}

==> vldb/Figures/application/hc.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_f1_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:hc_f1:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_f1_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:hc_f1:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{F1 Score of Heavy Change Detection.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	\postfig
% 	%
% 	%
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_f1_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:hc_f1:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_f1_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:hc_f1:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{F1 Score of Heavy Change Detection.}
	\label{fig:app:fe_are}
\postfig
\end{figure}


% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:hc_aae:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_aae_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:hc_aae:webpage}
% 		\end{minipage}
% 	}
%     \caption{AAE of Heavy Change Detection.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	%
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_aae_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:hc_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/hc_aae_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:hc_aae:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE of Heavy Change Detection.}
	\label{fig:app:fe_are}
\postfig
\end{figure}

==> vldb/Figures/application/mrg.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[ARE]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]%{vldb/Figures/application/sample.pdf}
% 		{vldb/Figures/application/mrg_are_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:mrg:high_are:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[AAE]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]%{vldb/Figures/application/sample2.pdf}
% 		{vldb/Figures/application/mrg_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:mrg:high_aae:caida}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{Performance of Merged \aname{}.}
%     %\vspace{-0.1in}
% 	\label{fig:mrg:high:caida}
% 	\postfig
% \end{figure}

\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]%{vldb/Figures/application/sample.pdf}
		{vldb/Figures/application/mrg_are_caida.pdf}
        \presubfigcaption
        \caption{ARE}
		\label{subfig:mrg:high_are:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]%{vldb/Figures/application/sample2.pdf}
		{vldb/Figures/application/mrg_aae_caida.pdf}
        \presubfigcaption
        \caption{AAE}
		\label{subfig:mrg:high_aae:caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{Performance of Merged \aname{}.}
	\label{fig:mrg:high:caida}
\postfig
\end{figure}

==> vldb/Figures/application/topk.tex <==


% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
		
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_pr_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:topk_pr:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_pr_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:topk_pr:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{Precision Rate of Top-k Item Detection.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	\postfig
% 	%
% \end{figure}



\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_pr_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:topk_pr:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_pr_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:topk_pr:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{Precision Rate of Top-k Item Detection.}
	\label{fig:app:fe_are}
\postfig
\end{figure}



% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	\subfigure[CAIDA]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:topk_aae:caida}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Web page]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_aae_webpage.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:app:topk_aae:webpage}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{AAE of Top-k Item Detection.}
%     %\vspace{-0.1in}
% 	\label{fig:app:fe_are}
% 	%
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_aae_caida.pdf}
        \presubfigcaption
        \caption{CAIDA}
		\label{subfig:app:topk_aae:caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/topk_aae_webpage.pdf}
        \presubfigcaption
        \caption{Web Page}
		\label{subfig:app:topk_aae:webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{AAE of Top-k Item Detection.}
	\label{fig:app:fe_are}
\postfig
\end{figure}



==> vldb/Figures/application/tp.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[Item Insertion]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/tp_insert.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:tp:insert}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[Frequency Query]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/application/tp_query.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:tp:query}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{Throughput Evaluation.}
%     %\vspace{-0.1in}
% 	\label{fig:tp}
% 	\postfig
% \end{figure}

\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/tp_insert.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp:insert}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/application/tp_query.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput Evaluation.}
	\label{fig:tp}
\postfig
\end{figure}

==> vldb/Figures/distri/distri.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.41\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/distri/skewness_are-crop.pdf}
		\end{center}
		}
		\label{subfig:distri:are}
		\end{minipage}
	}
	%
	\subfigure[F1 Score]{
		\begin{minipage}[t]{0.41\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/distri/skewness_f1-crop.pdf}
		\end{center}
		}
		\label{subfig:distri:f1}
		\end{minipage}
	}
	%
    \caption{Evaluation on Distributions.}
    %\vspace{-0.1in}
	\label{fig:distri}
	\postfig
\end{figure*}

==> vldb/Figures/fre/fre_aae.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[Synthetic]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/aae_syn-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:syn}
		\end{minipage}
	}
	%
	\subfigure[IP trace]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/aae_ip-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:ip}
		\end{minipage}
	}
	%
	\subfigure[Web page]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/aae_web-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:web}
		\end{minipage}
	}
	%
	\subfigure[Network]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/aae_net-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:aae:net}
		\end{minipage}
	}
	%
    \caption{AAE of finding frequent items.}
    %\vspace{-0.1in}
	\label{fig:fre:aae}
	\postfig
\end{figure*}

==> vldb/Figures/fre/fre_are.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[Synthetic]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/are_syn-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:are:syn}
		\end{minipage}
	}
	%
	\subfigure[IP trace]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/are_ip-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:are:ip}
		\end{minipage}
	}
	%
	\subfigure[Web page]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/are_web-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:are:web}
		\end{minipage}
	}
	%
	\subfigure[Network]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/are_net-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:are:net}
		\end{minipage}
	}
	%
    \caption{ARE of finding frequent items.}
    %\vspace{-0.1in}
	\label{fig:fre:are}
	\postfig
\end{figure*}

==> vldb/Figures/fre/fre_cr.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[Synthetic]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/cr_syn-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:cr:syn}
		\end{minipage}
	}
	%
	\subfigure[IP trace]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/cr_ip-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:cr:ip}
		\end{minipage}
	}
	%
	\subfigure[Web page]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/cr_web-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:cr:web}
		\end{minipage}
	}
	%
	\subfigure[Network]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/cr_net-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:cr:net}
		\end{minipage}
	}
	%
    \caption{CR of finding frequent items.}
    %\vspace{-0.1in}
	\label{fig:fre:cr}
	\postfig
\end{figure*}

==> vldb/Figures/fre/fre_pr.tex <==

\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[Synthetic]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/pr_syn-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:pr:syn}
		\end{minipage}
	}
	%
	\subfigure[IP trace]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/pr_ip-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:pr:ip}
		\end{minipage}
	}
	%
	\subfigure[Web page]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/pr_web-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:pr:web}
		\end{minipage}
	}
	%
	\subfigure[Network]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/pr_net-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:pr:net}
		\end{minipage}
	}
	%
    \caption{PR of finding frequent items.}
    %\vspace{-0.1in}
	\label{fig:fre:pr}
	\postfig
\end{figure*}


==> vldb/Figures/fre/fre_thp.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[Synthetic]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/thp_syn-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:thp:syn}
		\end{minipage}
    }
	%
	\subfigure[Synthetic]{
	    \begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/thp_ip-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:thp:ip}
		\end{minipage}
	}
	%
	\subfigure[Synthetic]{
	\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/thp_web-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:thp:web}
		\end{minipage}
	}
	%
	\subfigure[Synthetic]{
    \begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/fre/thp_net-crop.pdf}
		\end{center}
		}
		\label{subfig:fre:thp:net}
		\end{minipage}
	}
	%
	%
    \caption{Throughput of finding frequent items.}
    %\vspace{-0.1in}
	\label{fig:fre:thp}
	\postfig
\end{figure*}

==> vldb/Figures/nature/dom.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[Precision Rate]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/dom_pr_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:nature:dom_pr}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[AAE]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/dom_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:nature:dom_aae}
% 		\end{minipage}
% 	}
	
% 	\prefigcaption
%     \caption{Experiments on Accuracy of Dominant Item.}
% 	\label{fig:nature:dom}
% 	\postfig
% \end{figure}

\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/dom_pr_caida.pdf}
        \presubfigcaption
        \caption{Precision Rate}
        \label{subfig:nature:dom_pr}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/dom_aae_caida.pdf}
        \presubfigcaption
        \caption{AAE}
        \label{subfig:nature:dom_aae}
        \end{subfigure}
        
    \prefigcaption
    \caption{{Experiments on Accuracy of Dominant Item.}}
    \label{fig:nature:dom}
\postfig
\end{figure}


==> vldb/Figures/nature/dompro.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[The Skewness of Dataset]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/dompro_skew.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:nature:dompro_skew}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[The Number of Arrays]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}		
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/dompro_hash.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:nature:dompro_d}
% 		\end{minipage}
% 	}
% 	\prefigcaption
%     \caption{Experiments on Proportion of Dominant Item.}
%     %\vspace{-0.1in}
% 	\label{fig:nature:dompro}
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/dompro_skew.pdf}
        \presubfigcaption
        \caption{The Skewness of Dataset}
        \label{subfig:nature:dompro_skew}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/dompro_hash.pdf}
        \presubfigcaption
        \caption{The Number of Arrays}
		\label{subfig:nature:dompro_d}
        \end{subfigure}
        
    \prefigcaption
    \caption{Experiments on Proportion of Dominant Item.}
    \label{fig:nature:dompro}
\postfig
\end{figure}


==> vldb/Figures/nature/eps_range.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/eps_caida.pdf}
        \presubfigcaption
        \caption{Zero Outlier}
        \label{subfig:nature:eps_range_caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/eps_newfreq_caida.pdf}
        \presubfigcaption
        \caption{Overall AAE=5}
        \label{subfig:nature:eps_freq_caida}
        \end{subfigure}
        
    \prefigcaption
    \caption{{Memory Usage for Different $\Lambda$.}}
    \label{fig:nature:eps_range}
\postfig
\end{figure}


==> vldb/Figures/nature/hashnum.tex <==
% \begin{figure}[!ht]
% 	\centering
% 	\prefig
% 	%
% 	\subfigure[ARE]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/hash_are_caida.pdf}
% 	    \vspace{-0.2in}
% 		\end{center}
% 		}
% 		\label{subfig:nature:hash_are}
% 		\end{minipage}
% 	}
% 	%
% 	\subfigure[AAE]{
% 		\begin{minipage}[t]{0.225\textwidth}{
% 		\begin{center}	
% 		\includegraphics[width=\textwidth, ]{vldb/Figures/nature/hash_aae_caida.pdf}
% 		\end{center}
% 		}
% 		\label{subfig:nature:hash_aae}
% 		\end{minipage}
% 	}	
% 	\prefigcaption
%     \caption{Experiments on The Parameter $d$.}
% 	\label{fig:nature:hash}
% 	\postfig
% \end{figure}


\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/hash_are_caida.pdf}
        \presubfigcaption
        \caption{ARE}
        \label{subfig:nature:hash_are}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/hash_aae_caida.pdf}
        \presubfigcaption
        \caption{AAE}
        \label{subfig:nature:hash_aae}
        \end{subfigure}
        
    \prefigcaption
    \caption{Experiments on The Parameter $d$.}
    \label{fig:nature:hash}
\postfig
\end{figure}


==> vldb/Figures/nature/rl_freq.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rl_eps25_freq_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
        \label{subfig:nature:rl_freq_caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rl_eps25_freq_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
        \label{subfig:nature:rl_freq_webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{{Impact of $R_\lambda$ under the Same Average Error.}}
    \label{fig:nature:rl_freq}
\postfig
\end{figure}


==> vldb/Figures/nature/rl_range.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rl_eps25_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
        \label{subfig:nature:rl_range_caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rl_eps25_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
        \label{subfig:nature:rl_range_webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{{Impact of $R_\lambda$ under Zero Outlier.}}
    \label{fig:nature:rl_range}
\postfig
\end{figure}


==> vldb/Figures/nature/rw_freq.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rw_eps25_freq_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
        \label{subfig:nature:rw_freq_caida}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
        \includegraphics[width=\textwidth]{vldb/Figures/nature/rw_eps25_freq_webpage.pdf}
        \presubfigcaption
        \caption{Web Stream}
        \label{subfig:nature:rw_freq_webpage}
        \end{subfigure}
        
    \prefigcaption
    \caption{{Impact of $R_w$ under the Same Average Error.}}
    \label{fig:nature:rw_freq}
\postfig
\end{figure}


==> vldb/Figures/nature3/nature_7.2.1.1tex.tex <==
% \begin{figure}[!h]
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.1_new.pdf}
        \presubfigcaption
        \caption{Mice Keys}
		\label{subfig:nature:7.2.1.1}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.1_2_new.pdf}
        \presubfigcaption
        \caption{Elephant Keys}
		\label{subfig:nature:7.2.1.1_2}
        \end{subfigure}
    \prefigcaption
    % \vspace{-0.1in}
    \caption{Illustration of Sensed Error and Intervals.}
	\label{fig:nature:overview}
\postfig
\end{figure}

==> vldb/Figures/nature3/nature_7.2.1.2tex.tex <==
% \begin{figure}[!h]
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.2.pdf}
        \presubfigcaption
        \caption{vs. Actual Error}
		\label{subfig:nature:7.2.1.2}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.3.pdf}
        \presubfigcaption
        \caption{vs. Memory Size}
		\label{subfig:nature:7.2.1.3}
        \end{subfigure}
    \prefigcaption
    % \vspace{-0.1in}
    \caption{Experiments on Sensed Error.}
	\label{fig:nature:sensed_error}
\postfig
\end{figure}

==> vldb/Figures/nature3/nature_7.2.1.tex <==
% \begin{figure}[!h]
\begin{figure*}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.19\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.1.pdf}
        \presubfigcaption
        \caption{Overview(1-400)}
		\label{subfig:nature:7.2.1.1}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.19\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.1_2.pdf}
        \presubfigcaption
        \caption{Overview(4000-4400)}
		\label{subfig:nature:7.2.1.1_2}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.19\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.2.pdf}
        \presubfigcaption
        \caption{Sensed Error}
		\label{subfig:nature:7.2.1.2}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.19\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.3.pdf}
        \presubfigcaption
        \caption{Memory vs. Error}
		\label{subfig:nature:7.2.1.3}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.19\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.1.4.pdf}
        \presubfigcaption
        \caption{Priority Weight}
		\label{subfig:nature:7.2.1.4}
        \end{subfigure}
    \prefigcaption
    \caption{Experiments on Error-sensing Technique.}
	\label{fig:nature:error_sense}
\postfig
\end{figure*}

==> vldb/Figures/nature3/nature_7.2.2.tex <==
\begin{figure}[htbp]
% \prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.2.1.pdf}
        \presubfigcaption
        \caption{Layer Distribution }
		\label{subfig:nature:7.2.2.1}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/nature3/nature_7.2.2.2_log.pdf}
        \presubfigcaption
        \caption{Error Distribution}
		\label{subfig:nature:7.2.2.2}
        \end{subfigure}
        
    \prefigcaption
    \caption{ Illustration of Error-Controlling.}
    \vspace{-0.1in}
	\label{fig:nature:error_control}
\postfig
\end{figure}

==> vldb/Figures/order/order_are.tex <==
\begin{figure*}[!ht]
	\centering
	%
	\subfigure[\aname]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{Figures/order/order_are/order_are_ws.pdf}
		\end{center}
		}
		\label{subfig:order:are:aname}
		\end{minipage}
	}
	%
	\subfigure[SS]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{Figures/order/order_are/order_are_ss.pdf}
		\end{center}
		}
		\label{subfig:order:are:ss}
		\end{minipage}
	}
	%
	\subfigure[USS]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{Figures/order/order_are/order_are_uss.pdf}
		\end{center}
		}
		\label{subfig:order:are:uss}
		\end{minipage}
	}
	%
	\subfigure[Count+Heap]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{Figures/order/order_are/order_are_countheap.pdf}
		\end{center}
		}
		\label{subfig:order:are:count}
		\end{minipage}
	}
	%
    \caption{ARE of different arrival orders.}
    \vspace{-0.1in}
	\label{fig:order:are}
\end{figure*}

==> vldb/Figures/order/order_f1.tex <==
\begin{figure*}[!ht]
	\centering
	%
	\subfigure[\aname]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{Figures/order/order_f1/order_f1_ws.pdf}
		\end{center}
		}
		\label{subfig:order:f1:aname}
		\end{minipage}
	}
	%
	\subfigure[SS]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{Figures/order/order_f1/order_f1_ss.pdf}
		\end{center}
		}
		\label{subfig:order:f1:ss}
		\end{minipage}
	}
	%
	\subfigure[USS]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{Figures/order/order_f1/order_f1_uss.pdf}
		\end{center}
		}
		\label{subfig:order:f1:uss}
		\end{minipage}
	}
	%
	\subfigure[Count+Heap]{
		\begin{minipage}[t]{0.235\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{Figures/order/order_f1/order_f1_ch.pdf}
		\end{center}
		}
		\label{subfig:order:f1:count}
		\end{minipage}
	}
	%
    \caption{F1 Score of different arrival orders.}
    \vspace{-0.1in}
	\label{fig:order:f1}
\end{figure*}

==> vldb/Figures/para/para.tex <==
\begin{figure*}[!ht]
	\centering
	\prefig
	%
	\subfigure[ARE]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/para/slot_num_are-crop.pdf}
		\end{center}
		}
		\label{subfig:para:are}
		\end{minipage}
	}
	%
	\subfigure[CR]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}
		\includegraphics[width=\textwidth, ]{vldb/Figures/para/slot_num_cr-crop.pdf}
		\end{center}
		}
		\label{subfig:para:pr}
		\end{minipage}
	}
	%
	\subfigure[PR]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/para/slot_num_pr-crop.pdf}
		\end{center}
		}
		\label{subfig:para:cr}
		\end{minipage}
	}
	%
	\subfigure[Throughput]{
		\begin{minipage}[t]{0.225\textwidth}{
		\begin{center}		
		\includegraphics[width=\textwidth, ]{vldb/Figures/para/slot_num_thp-crop.pdf}
		\end{center}
		}
		\label{subfig:para:thp}
		\end{minipage}
	}
	%
    \caption{Evaluation on Parameter Setting.}
    %\vspace{-0.1in}
	\label{fig:para}
	\postfig
\end{figure*}	

==> vldb/Figures/sim/anomaly.tex <==
\begin{figure}[htbp]
% \prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/sim/drop_recall.pdf}
        \presubfigcaption
        \caption{Packet Drop}
		\label{subfig:sim:anomaly:drop}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/sim/loop_recall.pdf}
        \presubfigcaption
        \caption{Packet Loop}
		\label{subfig:sim:anomaly:loop}
        \end{subfigure}
        
    \prefigcaption
    % \vspace{-0.1in}
    \caption{Network Anomaly Detection.}
    % \vspace{-0.1in}
	\label{fig:sim:anomaly}
\postfig
\end{figure}

==> vldb/Figures/sim/intersection.tex <==
\begin{figure}[htbp]
\prefig
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/sim/intersection_eps10.pdf}
        \presubfigcaption
        \caption{$\Lambda$ = 10}
		\label{subfig:sim:intersection:10}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/sim/intersection_eps25.pdf}
        \presubfigcaption
        \caption{$\Lambda$ = 25}
		\label{subfig:sim:intersection:25}
        \end{subfigure}
        
    \prefigcaption
\vspace{-0.1in}
    \caption{Accuracy Improvement by Multiple Switches.}
	\label{fig:sim:intersection}
\postfig
\end{figure}

==> vldb/Figures/testbed/acc.tex <==
\begin{figure}[htbp]
\prefig
%     \centering
% 	\includegraphics[width=0.85\linewidth, ]{vldb/Figures/testbed/testbed_acc.pdf}
%     \prefigcaption
%     \caption{Accuracy on TestBed.}
% 	\label{fig:testbed:acc}
    \centering
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/testbed/testbed_acc_caida.pdf}
        \presubfigcaption
        \caption{IP Trace}
		\label{subfig:testbed:acc:caida}
        \end{subfigure}
    % \hfill
 	    \begin{subfigure}{0.47\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/testbed/testbed_acc_hadoop.pdf}
        \presubfigcaption
        \caption{Hadoop}
		\label{subfig:testbed:hadoop}
        \end{subfigure}
        
    % \vspace{-0.1in}
    \prefigcaption
    \caption{Accuracy on TestBed Deployment.}
	\label{fig:testbed:acc}
\postfig
\end{figure}


==> vldb/Figures/tp_new/newtp.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/newtp_insert.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp:insert}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/newtp_query.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput Evaluation.}
	\label{fig:tp}
\postfig
\end{figure}

==> vldb/Figures/tp_new/tp.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_insert.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp:insert}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_query.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput Evaluation.}
	\label{fig:tp}
\postfig
\end{figure}

==> vldb/Figures/tp_new/tp_acc.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_acc_insert.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp_acc:insert}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_acc_query.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp_acc:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput Evaluation under Zero Outlier.}
	\label{fig:tp_acc}
\postfig
\end{figure}

==> vldb/Figures/tp_new/tp_lf.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_lf_ist_caida.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp_lf:insert}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_lf_qry_caida.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp_lf:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput for Different Load Factors.}
	\label{fig:tp_lf}
\postfig
\end{figure}

==> vldb/Figures/tp_new/tp_lr.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_lr_ist_caida.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp_lr:insert}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_lr_qry_caida.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp_lr:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput for Different Load Rates.}
	\label{fig:tp_lr}
\postfig
\end{figure}

==> vldb/Figures/tp_new/tp_rw.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_rw_ist_caida.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp_rw:insert}
        \end{subfigure}
    \hfill
 	    \begin{subfigure}{0.49\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new/tp_rw_qry_caida.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp_rw:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput for Different Parameter $R_w$.}
	\label{fig:tp_rw}
\postfig
\end{figure}

==> vldb/Figures/tp_new2/tp_general.tex <==
\begin{figure}[!h]
\prefig
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new2/tp_insert.pdf}
        \presubfigcaption
        \caption{Item Insertion}
		\label{subfig:tp:insert}
        \end{subfigure}
    \centering
 	    \begin{subfigure}{0.85\linewidth}
        \centering
		\includegraphics[width=\textwidth, ]{vldb/Figures/tp_new2/tp_query.pdf}
        \presubfigcaption
        \caption{Frequency Query}
		\label{subfig:tp:query}
        \end{subfigure}
        
    \prefigcaption
    \caption{Throughput Evaluation.}
	\label{fig:tp}
\postfig
\end{figure}

==> vldb/Figures/tp_new2/tp_mixtex.tex <==
\begin{figure}[htbp]
% \prefig
    \centering
	\includegraphics[width=0.85\linewidth, ]{vldb/Figures/tp_new2/tp_mix_new.pdf}
    \prefigcaption
    \caption{Throughput Evaluation.}
	\label{fig:app:tp}
\postfig
% \vspace{-0.1in}
\end{figure}

==> vldb/InputFiles/author_format.tex <==
\author{Tong Yang, Gaogang xie, Yanbiao Li, Qiaobin Fu, Alex X. Liu, Qi Li, Laurent Mathy}

\numberofauthors{6}
\author{
\alignauthor
Tong Yang,Gaogang Xie*\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences (CAS), China.}\\
       \affaddr{ICT, CAS, China.}\\
       \email{yangtongemail@gmail.com, *xie@ict.ac.cn}
\alignauthor
YanBiao Li\\
       %\affaddr{College of Computer Science and Electronic Engineering, Hunan University, China}\\
       \affaddr{Hunan University, China}\\
       \email{lybmath\_cs@hnu.edu.cn}
\alignauthor
Qiaobin Fu\\
       \affaddr{ICT, CAS, China}\\
       \email{fuqiaobin@ict.ac.cn}
\and
\alignauthor Alex X. Liu\\
       \affaddr{Department of Computer Science and Engineering, Michigan State University}\\
       \email{alexliu@cse.msu.edu}
\alignauthor Qi Li\\
       \affaddr{ICT, CAS, China}\\
       \email{liqi19872006@gmail.com}
\alignauthor Laurent Mathy\\
       \affaddr{University of Liege, Belgium}\\
       \email{laurent.mathy@ulg.ac.be}
}


\author{\IEEEauthorblockN{Tong Yang\IEEEauthorrefmark{1},
Xiaoming Li\IEEEauthorrefmark{1},
Alex X. Liu\IEEEauthorrefmark{2},
Qiaobin Fu\IEEEauthorrefmark{3},
Gaogang Xie\IEEEauthorrefmark{4}}
\IEEEauthorblockA{\IEEEauthorrefmark{1}Computer Science Department, Peking University, Beijing, China}
\IEEEauthorblockA{\IEEEauthorrefmark{2}Department of Computer Science and Engineering, Michigan State University}
\IEEEauthorblockA{\IEEEauthorrefmark{3}Computer Science Department, Boston University, USA}
\IEEEauthorblockA{\IEEEauthorrefmark{4}ICT, CAS, China}
}

==> vldb/InputFiles/new-commands.tex <==
\mathchardef\Gamma="0100 \mathchardef\Delta="0101
\mathchardef\Theta="0102 \mathchardef\Lambda="0103
\mathchardef\Xi="0104 \mathchardef\Pi="0105
\mathchardef\Sigma="0106 \mathchardef\Upsilon="0107
\mathchardef\Phi="0108 \mathchardef\Psi="0109
\mathchardef\Omega="010A

\newcommand{\ovspace}[1]{\vspace{#1}}

\newcommand{\outline}[1]{}%{\textbf{#1}}

\newcommand{\dl}{\mbox{$\, [ \hspace*{-1.5pt} [\,$}}
\newcommand{\dr}{\mbox{$\, ] \hspace*{-1.5pt} ]\:$}}
\newcommand{\da}{\mbox{$\, A \hspace*{-6.75pt} A \,$}}
%\newcommand{\drightarrow}{\mbox{$\rightarrow \hspace*{-8pt} \rightarrow$}}

\newcommand{\BA}{\mbox{${\bm{a}}$}}
%\newcommand{\BB}{\mbox{${\bm{c}}$}}
\newcommand{\BC}{\mbox{${\bm{c}}$}}
\newcommand{\BD}{\mbox{${\bm{d}}$}}
\newcommand{\BE}{\mbox{${\bm{e}}$}}
\newcommand{\BO}{\mbox{${\bm{o}}$}}
\newcommand{\BP}{\mbox{${\bm{p}}$}}
\newcommand{\BQ}{\mbox{${\bm{q}}$}}
\newcommand{\BR}{\mbox{${\bm{r}}$}}
\newcommand{\BV}{\mbox{${\bm{v}}$}}
\newcommand{\BL}{\mbox{${\bm{l}}$}}
\newcommand{\BI}{\mbox{${\bm{i}}$}}
\newcommand{\BH}{\mbox{${\bm{h}}$}}
\newcommand{\BS}{\mbox{${\bm{s}}$}}
\newcommand{\BB}{\mbox{${\bm{k}}$}}

\newcommand{\wrapbox}[1]{\framebox{\begin{tabular}{c}#1\end{tabular}}}
\newcommand{\CodeIn}[1]{{\small\texttt{#1}}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\SFigure}[2]{Figure~\ref{fig:#1}(#2)}

%\usepackage{cite}
\usepackage{xspace}
\usepackage{url}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{amsfonts}
%\usepackage{times}
\usepackage{psfrag}
%\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{comment}
%packages for algorithms
%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{alltt}
\usepackage{color}

\newtheorem{defn}{Definition}[section]
\newtheorem{exmp}{Example}[section]
\newtheorem{thrm}{Theorem}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lemm}{Lemma}[section]
\newtheorem{obsv}{Observation}[section]
\newtheorem{corr}{Corollary}[section]

%\addtolength{\textheight}{.23in} \addtolength{\textwidth}{.15in}
%\addtolength{\topmargin}{-.23in}
%\addtolength{\oddsidemargin}{.1in}
%\addtolength{\evensidemargin}{.1in}

\newtheorem{thm}{Theorem}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
%\newcommand{\ie}{\emph{i.e.}\xspace}
%\newcommand{\eg}{\emph{e.g.}\xspace}
\newcommand{\etc}{\emph{etc.}\xspace}
%\newcommand{\etal}{\frenchspacing{}\emph{et al{.}}\xspace}
%\newcommand{\etal}[1]{{\sl et al.{#1}}}

%%\newcommand{\thm}[1]{Theorem~\ref{thm:#1}}
%%\newcommand{\lem}[1]{Lemma~\ref{lemma:#1}}
%\newcommand{cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\fac}[1]{Fact~\ref{fact:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}

%\theoremstyle{plain}
\newtheorem{property}{Property}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{theorem}{Theorem}[section]

%\theoremstyle{definition}
\newtheorem{notation}{Notation}
\newtheorem{Definition}{Definition}[section]

%\theoremstyle{remark}
\newtheorem{fact}{Fact}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{insight}{Insight}[section]

%%\algorithmstyle{definition}
%\algsetup{indent=1em}
%\renewcommand{\algorithmicrequire}{\textbf{Input:  }}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\factorial}{\ensuremath{\mbox{\sc Factorial}}}

% \newcommand{\Comment}[1]{}

\renewcommand\floatpagefraction{0.999}
\renewcommand\topfraction{0.999}
\renewcommand\bottomfraction{0.999}
\renewcommand\textfraction{0.001}
\setcounter{totalnumber}{5}


==> vldb/InputFiles/ref2.tex <==

@article{lossyhash,
	title={Lossy dictionaries},
	author={Pagh, Rasmus and Rodler, Flemming},
	journal={Algorithms—ESA 2001},
	pages={300--311},
	year={2001},
	publisher={Springer}
}


@incollection{hashsurvey,
  title={Hash-based techniques for high-speed packet processing},
  author={Kirsch, Adam and Mitzenmacher, Michael and Varghese, George},
  booktitle={Algorithms for Next Generation Networks},
  pages={181--218},
  year={2010},
  publisher={Springer}
}

@incollection{hashbased,
	title={Hash-based techniques for high-speed packet processing},
	author={Kirsch, Adam and Mitzenmacher, Michael and Varghese, George},
	booktitle={Algorithms for Next Generation Networks},
	pages={181--218},
	year={2010},
	publisher={Springer}
}

@article{perfecthash,
	title={Perfect hashing functions: a single probe retrieving method for static sets},
	author={Sprugnoli, Renzo},
	journal={Communications of the ACM},
	volume={20},
	number={11},
	pages={841--850},
	year={1977},
	publisher={ACM}
}


@inproceedings{robinhood,
	title={Robin hood hashing},
	author={Celis, Pedro and Larson, Per-Ake and Munro, J Ian},
	booktitle={Foundations of Computer Science, 1985, 26th Annual Symposium on},
	pages={281--288},
	year={1985},
	organization={IEEE}
}
@inproceedings{hopscotch,
	title={Hopscotch hashing},
	author={Herlihy, Maurice and Shavit, Nir and Tzafrir, Moran},
	booktitle={International Symposium on Distributed Computing},
	pages={350--364},
	year={2008},
	organization={Springer}
}

@article{cuckoohash,
	title={Cuckoo hashing},
	author={Pagh, Rasmus and Rodler, Flemming Friche},
	journal={Journal of Algorithms},
	volume={51},
	number={2},
	pages={122--144},
	year={2004},
	publisher={Elsevier}
}

@article{dlefthash,
	title={How asymmetry helps load balancing},
	author={V{\"o}cking, Berthold},
	journal={Journal of the ACM (JACM)},
	volume={50},
	number={4},
	pages={568--589},
	year={2003},
	publisher={ACM}
}


@inproceedings{sketchvldb05,
  title={Sketching streams through the net: Distributed approximate query tracking},
  author={Cormode, Graham and Garofalakis, Minos},
  booktitle={\Proc VLDB},
  pages={13--24},
  year={2005}
}


@inproceedings{sketchjoin96,
  title={The space complexity of approximating the frequency moments},
  author={Alon, Noga and Matias, Yossi and Szegedy, Mario},
  booktitle={\Proc ACM symposium on Theory of computing},
  year={1996}
}

@inproceedings{sketchjoin,
  title={Tracking join and self-join sizes in limited storage},
  author={Alon, Noga and Gibbons, Phillip B and Matias, Yossi and Szegedy, Mario},
  booktitle={\Proc ACM SIGMOD},
  pages={10--20},
  year={1999}
}


@inproceedings{tuplegraph,
  title={Graph-based synopses for relational selectivity estimation},
  author={Spiegel, Joshua and Polyzotis, Neoklis},
  booktitle={\Proc ACM SIGMOD},
  year={2006}
}

@inproceedings{birch,
  title={BIRCH: an efficient data clustering method for very large databases},
  author={Zhang, Tian and Ramakrishnan, Raghu and Livny, Miron},
  booktitle={ACM Sigmod Record},
  volume={25},
  number={2},
  pages={103--114},
  year={1996}
}


@inproceedings{treesketch,
  title={Approximate XML query answers},
  author={Polyzotis, Neoklis and Garofalakis, Minos and Ioannidis, Yannis},
  booktitle={\Proc ACM SIGMOD},
  year={2004}
}


@inproceedings{YCSB,
	title = {Benchmarking cloud serving systems with {YCSB}},
	booktitle = {\Proc ACM SOCC},
	author = {Cooper, Brian F. and Silberstein, Adam and et al.},
	year = {2010}
}

@inproceedings{charikar2002finding,
  title={Finding frequent items in data streams},
  author={Charikar, Moses and Chen, Kevin and Farach-Colton, Martin},
  booktitle={International Colloquium on Automata, Languages, and Programming},
  pages={693--703},
  year={2002},
  organization={Springer}
}

@article{cormode2005an,
title={An improved data stream summary: the count-min sketch and its applications},
author={Cormode, Graham and Muthukrishnan, S},
journal={Journal of Algorithms},
volume={55},
number={1},
pages={58--75},
year={2005}}

@article{cormode2011sketch,
  title={Sketch techniques for approximate query processing},
  author={Cormode, Graham},
  journal={Foundations and Trends in Sample. NOW publishers},
  year={2011}
}

@inproceedings{li2009one,
  title={One sketch for all: Theory and application of conditional random sampling},
  author={Li, Ping and Church, Kenneth W and Hastie, Trevor J},
  booktitle={Advances in Neural Information Processing Systems},
  pages={953--960},
  year={2009}
}

@inproceedings{gilbert2007one,
  title={One sketch for all: fast algorithms for compressed sensing},
  author={Gilbert, Anna C and Strauss, Martin J and Tropp, Joel A and Vershynin, Roman},
  booktitle={\Proc ACM STOC},
  year={2007}
}

@inproceedings{cormode2005sketching,
  title={Sketching streams through the net: Distributed approximate query tracking},
  author={Cormode, Graham and Garofalakis, Minos},
  booktitle={\Proc VLDB},
  year={2005}
}

@inproceedings{callegari2009statistical,
  title={Statistical approaches for network anomaly detection},
  author={Callegari, Christian},
  booktitle={\Proc ICIMP},
  year={2009},
  organization={Citeseer}
}

@inproceedings{zhao2006finding,
  title={Finding global icebergs over distributed data sets},
  author={Zhao, Qi George and Ogihara, Mitsunori and Wang, Haixun and Xu, Jun Jim},
  booktitle={\Proc ACM SIGMOD-SIGACT-SIGART},
  year={2006}
}


@inproceedings{superspreader,
  title={New Streaming Algorithms for Fast Detection of Superspreaders},
  author={S. Venkataraman and D. Xiaodong Song and P. B. Gibbons and A. Blum},
  booktitle={NDSS},
  year={2005}
}
@article{smallspace,
  title={Space-efficient tracking of persistent items in a massive data stream},
  author={Bibudh Lahiri and Jaideep Chandrashekar and Srikanta Tirthapura},
  journal={Statistical Analysis and Data Mining},
  year={2011},
  volume={7},
  pages={70-92}
}
@article{raptorcode,
 author = {A.Shokrollahi},
 title = {Raptor Codes},
 journal = {IEEE Transactions Information Theory},
 volume = {52},
 number = {6},
 year = {2006}
} 
@article{twodimensional,
  title={Detection of Super Sources and Destinations in High-Speed Networks: Algorithms, Analysis and Evaluation},
  author={Zhao, Q. and Xu, J. and Kumar, A.},
  journal={IEEE JSAC},
  volume={24},
  number={10},
  pages={1840-1852},
  year={2006},
}


@inproceedings{skimmedsketch,
	title={Processing data-stream join aggregates using skimmed sketches},
	author={Ganguly, Sumit and Garofalakis, Minos and Rastogi, Rajeev},
	booktitle={International Conference on Extending Database Technology},
	pages={569--586},
	year={2004},
	organization={Springer}
}

@inproceedings{parass,
	title={Efficient frequent item counting in multi-core hardware},
	author={Roy, Pratanu and Teubner, Jens and Alonso, Gustavo},
	booktitle={\Proc ACM SIGKDD},
	pages={1451--1459},
	year={2012},
	organization={ACM}
}
@inproceedings{fcmsketch,
	title={On efficient query processing of stream counts on the cell processor},
	author={Thomas, Dina and Bordawekar, Rajesh and Aggarwal, Charu C and Philip, S Yu},
	booktitle={Data Engineering, 2009. ICDE'09. IEEE 25th International Conference on},
	pages={748--759},
	year={2009},
	organization={IEEE}
}
@article{mgalgo,
	title={Finding repeated elements},
	author={Misra, Jayadev and Gries, David},
	journal={Science of computer programming},
	volume={2},
	number={2},
	pages={143--152},
	year={1982},
	publisher={Elsevier}
}


@inproceedings{wavelet,
	title={Wavelet synopses with error guarantees},
	author={Garofalakis, Minos and Gibbons, Phillip B},
	booktitle={\Proc ACM SIGMOD},
	pages={476--487},
	year={2002},
	organization={ACM}
}

@inproceedings{quantiles,
	title={How to summarize the universe: Dynamic maintenance of quantiles},
	author={Gilbert, Anna C and Kotidis, Yannis and Muthukrishnan, S and Strauss, Martin J},
	booktitle={\Proc VLDB},
	pages={454--465},
	year={2002},
	organization={VLDB Endowment}
}


@article{ewma,
	title={Control chart tests based on geometric moving averages},
	author={Roberts, SW},
	journal={Technometrics},
	volume={1},
	number={3},
	pages={239--250},
	year={1959},
	publisher={Taylor \& Francis}
}
@article{keylist,
	title={Algorithmic challenges in web search engines},
	author={Henzinger, Monika R},
	journal={Internet Mathematics},
	volume={1},
	number={1},
	pages={115--123},
	year={2004},
	publisher={Taylor \& Francis}
}

@article{slidingsketch,
	title={Sketch-based querying of distributed sliding-window data streams},
	author={Papapetrou, Odysseas and Garofalakis, Minos and Deligiannakis, Antonios},
	journal={\Proc VLDB},
	volume={5},
	number={10},
	pages={992--1003},
	year={2012},
	publisher={VLDB Endowment}
}

@article{usageother2,
author = {KJ, Houle and GM, Weaver and Long, N and Thomas, R},
year = {2001},
month = {01},
title = {Trends in Denial of Service Attack Technology}
}

@TECHREPORT{usageother3,
    Author = {Moore, D. and Paxson, V. and Savage, S. and Shannon, C. and Staniford, S. and Weaver, N.}, Title = {{The Spread of the Sapphire/Slammer Worm}},
    Institution = {CAIDA, ICSI, Silicon Defense, UCB EECS and UC San Diego CSE},
    Month = {Jan},
    Year = {2003},
}

@inproceedings{kary,
	title={Sketch-based change detection: methods, evaluation, and applications},
	author={K. Balachander and S. Subhabrata and Z. Yin and C. Yan},
	booktitle={Proceedings of the 3rd ACM SIGCOMM conference on Internet measurement},
	pages={234--247},
	year={2003},
	organization={ACM}
}

@inproceedings{usagefrequent1,
 author = {S. Anirudh and S. Suvinay and A. Mohammad and C. Sharad and C. Shang-Tse and A. Anurag and B. Hari and E. Tom and K. Sachin and M. Nick},
 title = {Programmable Packet Scheduling at Line Rate},
 booktitle = {Proceedings of the 2016 ACM SIGCOMM Conference},
 series = {SIGCOMM '16},
 year = {2016},
 pages = {44--57},
 numpages = {14},
 acmid = {2934899},
 publisher = {ACM},
} 

@ARTICLE{usagefrequent2, 
author={A. {Feldmann} and A. {Greenberg} and C. {Lund} and N. {Reingold} and J. {Rexford} and F. {True}}, 
journal={IEEE/ACM Transactions on Networking}, 
title={Deriving traffic demands for operational IP networks: methodology and experience}, 
year={2001}, 
volume={9}, 
number={3}, 
pages={265-279}, 
month={June},}


@ARTICLE{usagefrequent3, 
author={O. {Rottenstreich} and J. {Tapolcai}}, 
journal={IEEE/ACM Transactions on Networking}, 
title={Optimal Rule Caching and Lossy Compression for Longest Prefix Matching}, 
year={2017}, 
volume={25}, 
number={2}, 
pages={864-878}, 
month={April},}

@article{DKEhighratestream,
  title={Frequent items in streaming data: An experimental evaluation of the state-of-the-art},
  author={Manerikar, Nishad and Palpanas, Themis},
  journal={Data \& Knowledge Engineering},
  volume={68},
  number={4},
  pages={415--430},
  year={2009},
  publisher={Elsevier}
}


@article{revsketch,
	title={Reversible sketches: enabling monitoring and analysis over high-speed data streams},
	author={Schweller, Robert and Li, Zhichun and Chen, Yan and others},
	journal={IEEE/ACM Transactions on Networking (ToN)},
	volume={15},
	number={5},
	pages={1059--1072},
	year={2007},
	publisher={IEEE Press}
}
@article{frequent2,
	title={A simple algorithm for finding frequent elements in streams and bags},
	author={Karp, Richard M and Shenker, Scott and Papadimitriou, Christos H},
	journal={ACM Transactions on Database Systems (TODS)},
	volume={28},
	number={1},
	pages={51--55},
	year={2003},
	publisher={ACM}
}

@article{shbf,
	title={A shifting bloom filter framework for set queries},
	author={Yang, Tong and Liu, Alex X and Shahzad, Muhammad and Zhong, Yuankun and Fu, Qiaobin and Li, Zi and Xie, Gaogang and Li, Xiaoming},
	journal={Proceedings of the VLDB Endowment},
	volume={9},
	number={5},
	pages={408--419},
	year={2016},
	publisher={VLDB Endowment}
}


@article{counterbraids,
	title={Counter braids: a novel counter architecture for per-flow measurement},
	author={Lu, Yi and Montanari, Andrea and Prabhakar, Balaji and Dharmapurikar, Sarang and Kabbani, Abdul},
	journal={\Proc ACM SIGMETRICS},
	volume={36},
	number={1},
	pages={121--132},
	year={2008}
}


@article{approximate2000,
	title={Approximate Query Processing Using Wavelets},
	author={Chakrabarti, Kaushik and Garofalakis, Minos and Rastogi, Rajeev and Shim, Kyuseok},
	journal={Very Large Data Bases},
	volume={10},
	number={2-3},
	pages={199--223},
	year={2000}
}

@article{barman2007detecting,
	title={Detecting Attacks in Routers Using Sketches},
	author={Barman, Dhiman and Satapathy, Piyush and Ciardo, Gianfranco},
	journal={High Performance Switching and Routing},
	year={2007}
}

@inproceedings{bu2007fast,
	title={A fast and compact method for unveiling significant patterns in high speed networks},
	author={Bu, Tian and Cao, Jin and Chen, Aiyou and Lee, Patrick PC},
	booktitle={\Proc IEEE INFOCOM},
	pages={1893--1901},
	year={2007}
}

@InProceedings{CallegariCyprus2009,
	author =    {Callegari, Christian and Cyprus, North},
	title =     {Statistical approaches for network anomaly detection},
	booktitle = {\Proc ICIMP},
	year =      {2009}
}

@inproceedings{chen2010tracking,
	title={Tracking long duration flows in network traffic},
	author={Chen, Aiyou and Jin, Yu and Cao, Jin and Li, Li Erran},
	booktitle={\Proc IEEE INFOCOM},
	year={2010}
}
@article{cisco2015cisco,
	title={Cisco visual networking index: Forecast and methodology, 2015--2020},
	journal={CISCO White paper},
}


@article{cmlog,
	title={Count-Min-Log sketch: Approximately counting with approximate counters},
	author={Pitel, Guillaume and Fouquier, Geoffroy},
	journal={arXiv preprint arXiv:1502.04885},
	year={2015}
}

@article{cmlsketch,
	title={Count-Min-Log sketch: Approximately counting with approximate counters},
	author={Pitel, Guillaume and Fouquier, Geoffroy},
	journal={arXiv preprint arXiv:1502.04885},
	year={2015}
}


@article{daq2015,
	title={DAQ: a new paradigm for approximate query processing},
	author={Potti, Navneet and Patel, Jignesh M},
	journal={Proceedings of The Vldb Endowment},
	year={2015}}


@InProceedings{DurmeLall2009,
	author =    {Durme, Benjamin V and Lall, Ashwin},
	title =     {Streaming pointwise mutual information},
	booktitle = {Advances in Neural Information Processing Systems},
	year =      {2009},
	pages =     {1892--1900}
}


@article{dynamicCF,
	title={Dynamic count filters},
	author={Aguilar-Saborit, Josep and Trancoso, Pedro and Muntes-Mulero, Victor and Larriba-Pey, Josep-Lluis},
	journal={ACM SIGMOD Record},
	pages={26--32},
	year={2006}
}

@inproceedings{fan1998summary,
	title={Summary cache: A scalable wide-area web cache sharing protocol},
	author={Fan, Li and Cao, Pei and Almeida, Jussara and Broder, Andrei Z},
	booktitle={\Proc ACM SIGCOMM},
	year={1998}
}


@article{finding2008,
	title={Finding frequent items in data streams},
	author={C. Graham and H. Marios},
	journal={VLDB},
	year={2008}}


@InProceedings{GilbertStraussTroppEtAl2007,
	author =    {Gilbert, Anna C and Strauss, Martin J and Tropp, Joel A and Vershynin, Roman},
	title =     {One sketch for all: fast algorithms for compressed sensing},
	booktitle = {\Proc ACM STOC},
	year =      {2007}
}

@inproceedings{goyalIII,
	title={Approximate scalable bounded space sketch for large data NLP},
	author={Goyal, Amit and Daum{\'e} III, Hal},
	booktitle={\Proc EMNLP},
	year={2011}
}

@inproceedings{GPU-GAMT,
	title={{GAMT}: a Fast and Scalable IP Lookup Engine for GPU-based Software Routers},
	author={Li, Yanbiao and Zhang, Dafang and Liu, Alex X. and Zheng, Jintao},
	booktitle={\Proc IEEE/ACM ANCS},
	year={2013}
}

@inproceedings{GPU-NDN,
	Author = {Yi Wang and Yuan Zu and et al.},
	Booktitle = {\Proc USENIX NSDI},
	Pages = {199-212},
	Title = {Wire Speed Name Lookup: A GPU-based Approach},
	Year = {2013}
}

@INPROCEEDINGS{huaweiSmartMem,
	author = {Bill Lynch and Sailesh Kumar},
	title = {Smart Memory for High Performance Network Packet Forwarding},
	booktitle = {\Proc Hot Chips Symposium},
	year = {2010}
}


@article{kollios2005robust,
	title={Robust Aggregation in Sensor Networks.},
	author={Kollios, George and Byers, John W and Considine, Jeffrey and Hadjieleftheriou, Marios and Li, Feifei},
	journal={IEEE Data Eng. Bull.},
	volume={28},
	number={1},
	pages={26--32},
	year={2005}
}

@inproceedings{li1sketch,
	title={One sketch for all: Theory and application of conditional random sampling},
	author={Li, Ping and Church, Kenneth W and Hastie, Trevor J},
	booktitle={Advances in Neural Information Processing Systems},
	pages={953--960},
	year={2009}
}


@inproceedings{lossyAAAI,
	title={Lossy Conservative Update (LCU) Sketch: Succinct Approximate Count Storage.},
	author={Goyal, Amit and Daum{\'e} III, Hal},
	booktitle={AAAI},
	year={2011}
}

@misc{memcached,
	title = {{M}emcached - a distributed memory object caching system},
	howPublished = {\url{http://memcached.org}}
}
@INPROCEEDINGS{miller2011bandwidth,
	author = {Michael J. Miller},
	title = {Bandwidth Engine Serial Memory Chip Breaks 2 Billion Accesses/sec},
	booktitle = {\Proc Hot Chips Symposium},
	year = {2011}
}



@inproceedings{NLPstreaming,
	title={Streaming for large scale NLP: Language modeling},
	author={Goyal, Amit and Daum{\'e} III, Hal and Venkatasubramanian, Suresh},
	booktitle={\Proc NAACL},
	year={2009},
	organization={Association for Computational Linguistics}
}

@article{pike2005interpreting,
	title={Interpreting the data: Parallel analysis with Sawzall},
	author={Pike, Rob and Dorward, Sean and Griesemer, Robert and Quinlan, Sean},
	journal={Dynamic Grids and Worldwide Computing},
	volume={13},
	number={4},
	pages={277--298},
	year={2005},
	publisher={Hindawi Publishing Corporation}
}

@inproceedings{probacounting,
	title={Probabilistic Counting with Randomized Storage.},
	author={Van Durme, Benjamin and Lall, Ashwin},
	booktitle={IJCAI},
	pages={1574--1579},
	year={2009}
}


@inproceedings{sketch05stream,
	title={Sketching streams through the net: Distributed approximate query tracking},
	author={Cormode, Graham and Garofalakis, Minos},
	booktitle={Proceedings of VLDB Endowment},
	pages={13--24},
	year={2005}
}

@InProceedings{spectralBF,
	Title                    = {{S}pectral bloom filters},
	Author                   = {Cohen, Saar and Matias, Yossi},
	Booktitle                = {\Proc ACM SIGMOD},
	Year                     = {2003},
	Pages                    = {241--252}
}
@article{VLDB1TBMemory,
	title={Instant loading for main memory databases},
	author={M{\"u}hlbauer, Tobias and R{\"o}diger, Wolf and Seilbeck, Robert and Reiser, Angelika and Kemper, Alfons and Neumann, Thomas},
	journal={Proceedings of the VLDB Endowment},
	volume={6},
	number={14},
	pages={1702--1713},
	year={2013}
}


@inproceedings{YCSB,
	title = {Benchmarking cloud serving systems with {YCSB}},
	booktitle = {\Proc ACM SOCC},
	author = {Cooper, Brian F. and Silberstein, Adam and et al.},
	year = {2010}
}
@inproceedings{zhang2004online,
	title={Online identification of hierarchical heavy hitters: algorithms, evaluation, and applications},
	author={Zhang, Yin and Singh, Sumeet and Sen, Subhabrata and Duffield, Nick and Lund, Carsten},
	booktitle={\Proc ACM IMC},
	year={2004}
}

@InProceedings{ZhaoOgiharaWangEtAl2006,
	author =       {Zhao, Qi George and Ogihara, Mitsunori and Wang, Haixun and Xu, Jun Jim},
	title =        {Finding global icebergs over distributed data sets},
	booktitle =    {\Proc ACM PODS},
	year =         {2006},
	organization = {ACM}
}

@inproceedings{goyal2012sketch,
  title={Sketch algorithms for estimating point queries in NLP},
  author={Goyal, Amit and Daume and Iii, Hal and Cormode, Graham},
  booktitle={\Proc EMNLP},
  year={2012}
}

@inproceedings{sdm12social,
  title={Event Detection in Social Streams.},
  author={Aggarwal, Charu C and Subbian, Karthik},
  booktitle={SDM},
  volume={12},
  year={2012},
  organization={SIAM}
}

@inproceedings{sdm10sketch,
  title={On Classification of High-Cardinality Data Streams.},
  author={Aggarwal, Charu C and Philip, S Yu},
  booktitle={SDM},
  volume={10},
  pages={802--813},
  year={2010},
  organization={SIAM}
}

@inproceedings{sigsketch,
  title={One Sketch to Rule Them All: Rethinking Network Flow Monitoring with UnivMon},
  author={Liu, Zaoxing and Manousis, Antonis and et al.},
  booktitle={\Proc ACM SIGCOMM},
  year={2016}
}

@article{summarycache,
  title={Summary cache: a scalable wide-area web cache sharing protocol},
  author={Fan, Li and Cao, Pei and Almeida, Jussara and Broder, Andrei Z},
  journal={IEEE/ACM ToN},
  volume={8},
  number={3},
  pages={281--293},
  year={2000}
}

@inproceedings{probaestima2013,
	title={Exploring sketches for probability estimation with sublinear memory},
	author={Kleerekoper, Anthony and Luj{\'a}n, Mikel and Brown, Gavin},
	booktitle={IEEE International Conference on Big Data},
	year={2013}
}

@inproceedings{fan2008efficient,
title={Efficient and robust sensor data aggregation using linear counting sketches},
author={Fan, Yao-Chung and Chen, Arbee LP},
booktitle={Parallel and Distributed Processing, 2008. IPDPS 2008. IEEE International Symposium on},
pages={1--12},
year={2008},
organization={IEEE}
}

@article{FMCMsensor2004,
	title={Robust Aggregation in Sensor Networks.},
	author={Kollios, George and Byers, John W and et al.},
	journal={IEEE Data Eng. Bull.},
	volume={28},
	number={1},
	pages={26--32},
	year={2005}
}


@inproceedings{FMsensor2004,
	title={Approximate aggregation techniques for sensor databases},
	author={Considine, Jeffrey and Li, Feifei and Kollios, George and Byers, John},
	booktitle={\Proc IEEE ICDE},
	year={2004}
}

@inproceedings{minoutlier2012,
	title={A near-linear time approximation algorithm for angle-based outlier detection in high-dimensional data},
	author={Pham, Ninh and Pagh, Rasmus},
	booktitle={\Proc ACM SIGKDD},
	year={2012},
}


@article{mintopk2010,
	title={Mining top-K frequent itemsets through progressive sampling},
	author={Pietracaprina, Andrea and Riondato, Matteo and Upfal, Eli and Vandin, Fabio},
	journal={Data Mining and Knowledge Discovery},
	volume={21},
	number={2},
	pages={310--326},
	year={2010},
	publisher={Springer}
}


@inproceedings{slidwindow04,
  title={Approximate counts and quantiles over sliding windows},
  author={Arasu, Arvind and Manku, Gurmeet Singh},
  booktitle={\Proc ACM SIGMOD},
  pages={286--296},
  year={2004}
}


@inproceedings{sketchsoda,
  title={Tabulation based 4-universal hashing with applications to second moment estimation.},
  author={Thorup, Mikkel and Zhang, Yin},
  booktitle={SODA},
  volume={4},
  pages={615--624},
  year={2004}
}

@article{pitel2015count,
  title={Count-Min-Log sketch: Approximately counting with approximate counters},
  author={Pitel, Guillaume and Fouquier, Geoffroy},
  journal={arXiv preprint arXiv:1502.04885},
  year={2015}
}

@inproceedings{cohen2003spectral,
  title={Spectral bloom filters},
  author={Cohen, Saar and Matias, Yossi},
  booktitle={\Proc ACM SIGMOD},
  year={2003}
}

@article{aguilar2006dynamic,
  title={Dynamic count filters},
  author={Aguilar-Saborit, Josep and Trancoso, Pedro and et al.},
  journal={ACM SIGMOD},
  year={2006}
}


==> vldb/Math/errorfree.tex <==


\subsection{Probability of Error-free}
\label{subsec:math:errorfree}
%Since the effect of the hash function $w$ on the result is greater than other factors such as the sequence of items,  our \aname{} has a property of stability which ensures that the item with higher frequency is always more likely to be inserted in the positive part or the negative part.
In this section, we analyze the probability of \aname{} to output an estimated frequency without error.

\begin{theorem}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In simplified \aname{}, We have
\begin{equation}
\begin{aligned}
Pr\{ \widetilde{f_{i}^{up}} = f_i\}\geq 1 - \Bigg (1 - \max\limits_{t > 1}\Big \{\Big (1-\frac{f_i}{tf_i + t}\Big )\Big (1 - \frac{(M-f_i)t}{wf_i}\Big )\Big \}\Bigg )^d
\end{aligned}
\end{equation}
\end{theorem}
%overfull

\begin{proof}
For each $j=1,2,\cdots,d$ and $t > 1$, according to lemma \ref{base}, we have
$$Pr\{f_i\geq tF_{i, j}\}\geq 1 - \frac{(M-f_i)t}{wf_i} $$

We then calculate the probability of $\widetilde{f_{i}^{up}} = f_i$ under the condition of $f_i\geq tF_{i, j}$. By the linearity of expectation, we have, 
\begin{equation*}
\begin{array}{ll}
&Pr\{\tilde{f}_{i, j}^{up} = f_i | f_i\geq tF_{i, j}\}\\
&\geq Pr\{ID_{k} = e_i\vee p_{k+1} = e_i,\ \forall k = 1,2,\cdots,F_{i, j} - 1 | f_i\geq tF_{i, j}\}\\
&\geq Pr\{2\sum\limits_{l = 1}^{k}I_{p_l = e_i}\geq k,\ \forall k = 2,\cdots,F_{i, j} | f_i\geq tF_{i, j}\}\\
\end{array}
\end{equation*}


This is a classic combinatorial mathematics problem, we apply its conclusion,
\begin{equation*}
Pr\{\tilde{f}_{i, j}^{up} = f_i | f_i\geq tF_{i, j}\} \geq 1-\frac{f_i}{tf_i + t}
\end{equation*}

Finally, we union different $j$ and different $t$, 
\begin{equation*}
\begin{array}{ll}
&Pr\{ \widetilde{f_{i}^{up}} = f_i\}\\
&= 1 - (1 - Pr\{\tilde{f}_{i, j}^{up} = f_i\})^d\\
&\geq 1 - (1 - Pr\{\tilde{f}_{i, j}^{up} = f_i | f_i\geq tF_{i, j}\}\cdot Pr\{f_i\geq tF_{i, j}\})^d\\
&\geq 1 - \Big (1 - \max \limits_{t > 1}\Big \{\big (1-\frac{f_i}{tf_i + t}\big )\cdot \big (1 - \frac{(M-f_i)t}{wf_i}\big )\Big \}\Big )^d\\
\end{array}
\end{equation*}
%overfull
\end{proof}

\begin{corollary}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In \aname{}, We have
\begin{equation}
\begin{aligned}
Pr\{ \widehat{f_{i}^{up}} = f_i\}\geq 1 - \Bigg (1 - \max\limits_{t > 1}\Big \{\Big (1-\frac{f_i}{tf_i + t}\Big )\Big (1 - \frac{(M-f_i)t}{wf_i}\Big )\Big \}\Bigg )^d
\end{aligned}
\end{equation}
\end{corollary}

==> vldb/Math/expectationerror.tex <==
\subsection{Error Bound of \aname{}}
\label{subsec:math:expectationerror}
Since it is difficult to analyze the error bound of \aname{} directly, we consider a simplified version of \aname{} in which an incoming item $e_i$ is inserted into all hashed buckets. We can prove that the error of \aname{} is definitely no more than the error of simplified \aname{}. Therefore, we derive the error bound of simplified \aname{} and it is also an error bound of \aname{}.
\begin{lemma}
\label{lem1}
Consider we insert a data stream $\mathcal{S}$ into a bucket. Let $low_m$ be the low counter of the bucket, $high_m$ be the high counter of the bucket, $ID_m$ be the ID of the bucket. Consider another circumstance, we insert another data stream $\hat{\mathcal{S}}$ which is a subsequence of $\mathcal{S}$ into the bucket. Let $low_u$, $high_u$, $ID_u$ be the high counter, low counter and ID of the bucket in this circumstance. Thus, we have
\begin{equation}
\begin{aligned}
high_m - high_u \geq \begin{cases} |low_u - low_m|, & \text{$ID_u = ID_m$}\\ |low_u + low_m|, & \text{$ID_u\neq ID_m$} \end{cases}
\end{aligned}
\label{2st}
\end{equation}
\end{lemma}
\begin{proof}
We use mathematical induction to prove this lemma. For all $n \in \mathbb{Z}^+$, after $n^{th}$ insertion, \eqref{2st} is true.

\noindent\textbf{Base case:} The initial values of $high_m$, $low_m$, $high_u$, $low_u$ are all 0. Therefore, it is obvious that \eqref{2st} holds.

\noindent\textbf{Induction Step:} Suppose, \eqref{2st} holds after the $k^{th}$ insertion. We consider the insertion of item $e_{k+1}$. There are four possible cases.

\noindent Case 1: $e_{k+1}$ is not in $\hat{\mathcal{S}}$.

Then, $high_m$ increases by 1, and $high_u$ keeps unchanged, the left side of the inequality increases by 1. $low_m$ increases or decreases by 1, and $low_u$ keeps unchanged, the right side of the inequality at most increases by 1. Therefore, \eqref{2st} still holds.

\noindent Case 2: $e_{k+1}$ is in $\hat{\mathcal{S}}$. Both $low_m$ and $low_u$ are more than 0 before inserting $e_{k+1}$.

In this case, the left side of \eqref{2st} does not change, and both $ID_m$ and $ID_u$ keeps unchanged. If $ID_m = ID_u$, $low_m$ and $low_u$ either increase by 1 or decrease by 1. Therefore, the right side does not change. Otherwise, at least one of $low_m$ and $low_u$ decreases by 1. So the right side will not increase. In both circumstances, \eqref{2st} holds.

\noindent Case 3: $e_{k+1}$ is in $\hat{\mathcal{S}}$. One of $low_m$ and $low_u$ is 0.

Without loss of generality, we assume $low_m = 0$. The right side before insertion is $low_u$. If $ID_u = e_{k+1}$, then $ID_m = ID_u = e_{k+1}$ after insertion. Both $low_m$ and $low_u$ increase by 1, the right side does not change. Otherwise, $ID_u \neq ID_m = e_{k+1}$ after insertion. $low_u$ decreases by 1 and $low_m$ increase by 1, the right side does not change. In both circumstances, \eqref{2st} still holds.

\noindent Case 4: $e_{k+1}$ is in $\hat{\mathcal{S}}$. $low_m$ and $low_u$ are 0.

The right side before insertion is 0. After insertion, $ID_m = ID_u = e_{k+1}$, and $low_m = low_u = 1$. Thus, the right side is still 0, \eqref{2st} holds.

\noindent \textbf{Conclusion: }By the principle of induction, the lemma holds for any data stream $\mathcal{S}$.
\end{proof}


\begin{theorem}
\label{bound}
Given a data stream $\mathcal{S}$, an arbitrary item $e_i$. Let $f_i$ be the real frequency of $e_i$, $\widehat{f_i^{up}}$ be the estimated frequency of \aname{}, $\widetilde{f_i^{up}}$ be the estimated frequency of simplified \aname{}. We have
\begin{equation}
\begin{aligned}
f_i\leq \widehat{f_i^{up}}\leq \widetilde{f_i^{up}}
\end{aligned}
\end{equation}
\end{theorem}
\begin{proof}
For each $j = 1,2,\cdots, d$, we want to prove
\begin{equation*}
f_i\leq \hat{f}_{i,j}^{up} \leq \tilde{f}_{i,j}^{up}
\end{equation*}

Consider bucket $B_j[h_j(e_i)]$, the data stream inserted into the bucket in \aname{} is a subsequence of the data stream inserted into the bucket in simplified \aname{}. Let $low_u$, $high_u$, $ID_u$ be the high counter, low counter and ID of the bucket in \aname{}. Let $low_m$, $high_m$, $ID_m$ be the high counter, low counter and ID of the bucket in simplified version. Then, we separately consider cases to analyze.

\noindent Case 1: $ID_u = ID_m = e_i$.

According to lemma \ref{lem1}, we have $high_m - high_u \geq |low_u - low_m|$. Thus, $2\tilde{f}_{i,j}^{up} = high_m + low_m \geq high_u + low_u = 2\hat{f}_{i,j}^{up}$.

\noindent Case 2: $ID_u = ID_m \neq e_i$.

According to lemma \ref{lem1}, we have $high_m - high_u \geq |low_u - low_m|$. Thus, $2\tilde{f}_{i,j}^{up} = high_m - low_m \geq high_u - low_u = 2\hat{f}_{i,j}^{up}$.

\noindent Case 3: $ID_u \neq ID_m $.

According to lemma \ref{lem1}, we have $high_m - high_u \geq |low_u + low_m| = low_u + low_m$. Thus, $2\tilde{f}_{i,j}^{up} \geq high_m - low_m \geq high_u + low_u \geq 2\hat{f}_{i,j}^{up}$. Therefore, $\hat{f}_{i,j}^{up}\leq \tilde{f}_{i,j}^{up}$.

In all cases, we have $\hat{f}_{i,j}^{up}\leq \tilde{f}_{i,j}^{up}$. Therefore,
\begin{equation*}
\widehat{f_i^{up}} = \min\limits_{j=1}^{d}\{\hat{f}_{i,j}^{up}\}\leq \min\limits_{j=1}^{d}\{\tilde{f}_{i,j}^{up}\} = \widetilde{f_i^{up}}
\end{equation*}
According to theorem \ref{t1}, we have 
\begin{equation*}
f_i\leq \widehat{f_i^{up}}\leq \widetilde{f_i^{up}}
\end{equation*}
\end{proof}


\begin{lemma}
\label{base}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$, in the simplified \aname{}, for each $j = 1,2,\cdots, d$ and $t > 1$, we have
\begin{equation}
\begin{aligned}
Pr\{f_i\geq {t}F_{i, j}\}\geq 1 - \frac{(M-f_i)t}{wf_i} 
\end{aligned}
\end{equation}
\end{lemma}

\begin{proof}
We introduce indicator variables $I_{i,j,k}$, which are 1 if $(e_i\neq e_k)\wedge (h_j(e_i) = h_j(e_k))$, and 0 otherwise. By the pairwise independence of the hash functions, for $e_i\neq e_k$, we have
\begin{equation*}
E[I_{i,j,k}] = Pr\{h_j(e_i) = h_j(e_k)\} = \frac{1}{w}
\end{equation*}
Also, we have $F_{i, j} = \sum\limits_{e_k\neq e_i}f_k I_{i,j,k}$.
By the linearity of expectation,
\begin{equation*}
E[F_{i, j}] = \sum_{k\neq i} f_k E[I_{i,j,k}] = \frac{(M - f_i)}{w}
\end{equation*}
By the Markov inequality,
\begin{equation*}
\begin{aligned}
Pr\{F_{i, j} \leq \frac{1}{t}f_i\} = 1 - Pr\{F_{i,j} > \frac{1}{t}f_i\}
\geq 1 - \frac{(M-f_i)t}{wf_i}
\end{aligned}
\end{equation*}
\end{proof}

\begin{comment}
\begin{lemma}\label{low}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In the simplified \aname{}, for row $j$, if $f_i > F_{i, j}$, we have
\begin{equation}
f_i - F_{i, j} \leq \widehat{f_{i, j}^{lo}}
\end{equation}
and $B_j[h_j(e_i)].ID = e_i$.
\end{lemma}
\begin{proof}
For bucket $B_j[h_j(e_i)]$, there are $f_i$ numbers of item $e_i$ and $F_{i,j}$ other items mapping to it. %
Because each one of the other items at most counterbalances one $e_i$, so there remains at least $f_i - F_{i,j}$ numbers of $e_i$. Thus $B_j[h_j(e_i)].ID$ is bound to be $e_i$.
\end{proof}
\end{comment}

\begin{theorem}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In the simplified \aname, given an error $\epsilon$, we have
\begin{equation}
\begin{aligned}
Pr\{f_i - \widetilde{f_{i}^{lo}} \geq \epsilon\} \leq \frac{(M-f_i)t}{wf_i}
\end{aligned}
\end{equation}
\end{theorem}
\begin{proof}
According to lemma \ref{base}, we have 
\begin{equation*}
Pr\{F_{i, j} \leq \frac{1}{t}f_i\} = 1 - Pr\{F_{i,j} > \frac{1}{t}f_i\}
\geq 1 - \frac{(M-f_i)t}{wf_i}
\end{equation*}
If $f_i > tF_{i,j}$, then we have $\widetilde{f_{i}^{lo}} \geq f_i - F_{i,j}$.
And let $t = \frac{f_i}{\epsilon}$, thus $f_i - \widetilde{f_{i}^{lo}} \leq F_{i,j} < \frac{1}{t}f_i = \epsilon$.
Therefore, we have
\begin{equation*}
Pr\{f_i - \widetilde{f_{i}^{lo}} \geq \epsilon\} \leq \frac{(M-f_i)}{w\epsilon}
\end{equation*}
\end{proof}

\begin{corollary}
Given a stream $\mathcal{S}$ which obeys arbitrary distribution. In the \aname, given an arbitrary item $e_i$ and an error $\epsilon$, 
\begin{equation}
\begin{aligned}
Pr\{f_i - \widehat{f_{i}^{lo}} \geq \epsilon\} \leq \frac{(M-f_i)}{w\epsilon}
\end{aligned}
\end{equation}
\end{corollary}

\begin{theorem}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In the simplified \aname, given an error $\epsilon$, we have
\begin{equation}
\begin{aligned}
Pr\{\widetilde{f_{i}^{up}} - f_i\geq \epsilon\}< \Bigg (\min \limits_{t > 1}\Big \{\frac{(M-f_i)t}{w f_i} + \frac{q^2}{(1-q)\epsilon}\Big \} \Bigg )^d
\end{aligned}
\end{equation}
where
\begin{equation*}
q = e^{-\frac{(t-1)^2}{2(t+1)^2}}
\end{equation*}
\end{theorem}

\begin{proof}
For each $j=1,2,\cdots,d$ and $t>1$, from lemma \ref{base},
\begin{equation*}
Pr\{f_i\geq tF_{i, j}\}\geq 1 - \frac{(M-f_i)t}{w f_i}
\end{equation*}
We calculate the expectation of $\tilde{f}_{i,j}^{up} - f_i$ under the condition of $f_i\geq tF_{i, j}$. Let $p_k$ be the $k^{th}$ item in the data stream which satisfies $h_j(p_k) = h_j(e_i)$, $ID_{k}$ be the value of $B_j[h_j(e_i)].ID$ after the insertion of $p_k$. Then, by the linearity of expectation and the lemma above, we have
\begin{equation*}
\begin{array}{ll}
    &E[\tilde{f}_{i, j}^{up} - f_i | f_i\geq tF_{i, j}]\\
    &= \sum\limits_{k = 2}^{f_i + F_{i,j}}Pr\{p_k\neq e_i\wedge ID_{k}\neq e_i\wedge p_k\neq ID_{k} | f_i\geq tF_{i, j}\}\\
    &\leq \sum\limits_{k = 2}^{f_i + F_{i,j}} Pr\{ID_k\neq e_i| f_i \geq tF_{i,j}\}\\
    &= \sum\limits_{k = 2}^{f_i + F_{i,j}}1 - Pr\{ID_{k} = e_i | f_i\geq tF_{i, j}\}\\
    &\leq \sum\limits_{k = 2}^{f_i + F_{i,j}}1 - Pr\{2\sum\limits_{l = 1}^{k}I_{p_l = e_i}> k | f_i\geq tF_{i, j}\}\\
    &\leq \sum\limits_{k = 2}^{f_i+F_{i, j}}Pr\{2\sum\limits_{l = 1}^{k}I_{p_l = e_i} \leq k | f_i\geq tF_{i, j}\}\\
\end{array}
\end{equation*}
%这一步用了draw without replacement
According to the probability inequalities for the sum in sampling without replacement,
\begin{equation*}
\begin{aligned}
    E[\tilde{f}_{i, j}^{up} - f_i | f_i\geq tF_{i, j}] \leq \sum\limits_{k = 2}^{f_i+F_{i, j}}e^{-\frac{k(t-1)^2}{2(t+1)^2}}
    = \sum\limits_{k = 2}^{f_i+F_{i, j}}q^k
    < \frac{q^2}{1-q}
\end{aligned}
\end{equation*}
By Markov inequality, we have
\begin{equation*}
\begin{array}{ll}
&Pr\{\tilde{f}_{i,j}^{up} - f_i\geq \epsilon\}\\
&\leq Pr\{f_i< tF_{i, j}\} + Pr\{\tilde{f}_{i,j}^{up} - f_i\geq \epsilon | f_i\geq tF_{i, j}\}\\
&\leq \frac{(M-f_i)t}{wf_i} + \frac{q^2}{(1-q)\epsilon}
\end{array}
\end{equation*}

Finally, we union different $j$ and different $t$, 
\begin{align*}
Pr\{\widetilde{f_{i}^{up}} - f_i\geq \epsilon\} &= Pr^{d}\{\tilde{f}_{i, j}^{up} - f_i\geq \epsilon\} \\
&< \Bigg (\min \limits_{t > 1}\Big \{\frac{(M-f_i)t}{w f_i} + \frac{q^2}{(1-q)\epsilon}\Big \} \Bigg )^d
\end{align*}
\end{proof}

\begin{corollary}
Given a stream $\mathcal{S}$ which obeys arbitrary distribution. In the \aname, given an arbitrary item $e_i$ and an error $\epsilon$, 
\begin{equation}
\begin{aligned}
Pr\{\widehat{f_{i}^{up}} - f_i\geq \epsilon\}< \Bigg (\min \limits_{t > 1}\Big \{\frac{(M-f_i)t}{w f_i} + \frac{q^2}{(1-q)\epsilon}\Big \} \Bigg )^d
\end{aligned}
\end{equation}
\end{corollary}

\begin{corollary}
Given a stream $\mathcal{S}$ which obeys arbitrary distribution. In the \aname, given an arbitrary item $e_i$ and an error $\epsilon$, 
\begin{equation}
\begin{aligned}
Pr\{\widehat{f_{i}^{up}} - \widehat{f_{i}^{lo}} \geq 2\epsilon\} \leq \frac{(M-f_i)}{w\epsilon} + \Bigg (\min \limits_{t > 1}\Big \{\frac{(M-f_i)t}{w f_i} + \frac{q^2}{(1-q)\epsilon}\Big \} \Bigg )^d
\end{aligned}
\end{equation}
\end{corollary}


% \begin{proof}
% Let $P_{i}$ denote the probability that the $e_i$'s corresponding part in $B[h(e_i)]$ contains at least $d$ items whose frequency is higher than $e_i$. 
% When $i \leqslant d$, $P_{i} = 1$.
% Therefore, we only need to discuss the situation when $i > d$.
% When $i > d$, we have
% \begin{equation}
% \begin{aligned}
%  P_{i}
%     \leqslant \dbinom{i-1}{d}\cdot\left(\frac{1}{l}\right)^{d} \leqslant \frac{d^d}{d!}\cdot \left(\frac{i-1}{c}\right)^{d}
% \end{aligned}
% \end{equation}
% \end{proof}

% We can find that, when $i$ decreases, $P_i$ decreases sharply, which indicates that the probability that $e_i$ is in the top $d$ item is much higher.
% According to Stirling's approximation,
% \begin{equation}
% \begin{aligned}
% 1 - \frac{d^d}{d!}\cdot \left(\frac{i-1}{c}\right)^{d}
% \approx 
% 1 - \frac{1}{\sqrt{2 \pi d}} \cdot \left(\frac{e (i - 1)}{c}\right)^{d}
% \end{aligned}
% \end{equation}
% We can find that, when $i < \frac{c}{e} + 1$, the probability that $e_i$ is the top $d$ item will increase with $d$ increases.


==> vldb/Math/newmath.tex <==
%\subsection{Relationship between Levels}

In this section, we analyze the relationship of the number of flows between levels.
Let $S^{i}=\{e_1, e_2, \dots, e_n\}$ denote all flows that enters the $i^{th}$ level.
Let $f_i(e)$ denotes the frequency of flow $e$ that enters the $i^{th}$ level. 
We divide flows into two types according to their flow sizes.
Let $F_i$ be the total frequency of all small flows in $S^{i}$, $F_i\coloneqq \sum_{e\in S^{i}\land f_i(e)\leqslant \frac{1}{2}\lambda_i}f_i(e)$,
and $C_i$ be the number of distinct large flows, $C_i\coloneqq |\{e\in S^{i}\land f_i(e)> \frac{1}{2}\lambda_i\}|$.
%$ w_i=\frac{W}{2^i}$,  $\lambda_i=\frac{\Lambda}{2^i}$






Let $F_{i,k}$ denote the total frequency of the small flows satisfies: \textit{i)} in set $\{e_1, e_2, \dots, e_{k-1}\}$ and \textit{ii)} map into the same bucket as $e_k$. $F_{i,k}=\sum_{l \in [1,k-1]}f_i(e_l)*[h_i(e_l)=h_i(e_k) \land f_i(e_l) \leqslant \frac{1}{2}\lambda_i]$. 
Let $C_{i,k}$ denote the number of distinct large flows map into the same bucket as $e_k$. $C_{i,k}=\sum_{l \in [1,k-1]}1*[h_i(e_l)=h_i(e_k) \land f_i(e_l) > \frac{1}{2}\lambda_i]$. 

For bucket $B_i[j]$, let $S^{i,j}_0$ denote all small flows inserted into bucket $B_i[j]$, and $S^{i,j}_1$ denote the large flows.
$ S^{i,j}_0 \coloneqq \{e_k | f_i(e_k)\leqslant \frac{1}{2}\lambda_i \land e_k\in S_i\}$, $ S^{i,j}_1 \coloneqq \{e| f_i(e)> \frac{1}{2}\lambda_i  \land e_k\in S_i\}$.
Let $f_{i,j}$ be the total frequency of the small flows, $f_{i,j}\coloneqq \sum_{e\in S^{i,j}_0}f_i(e)$, and $c_{i,j}$ be the number of distinct large flows, $c_{i,j}\coloneqq |S^{i,j}_1|$. 
Suppose $S^{i}_0=\bigcup_{j=1}^{w_i}S^{i,j}_0=\{e_{a_1}, e_{a_2}, \dots, e_{a_{n_0}}\}, a_{l}<a_{l+1}, l\in [1,n-1]$.
Suppose $S^{i}_1=\bigcup_{j=1}^{w_i}S^{i,j}_1=\{e_{b_1}, e_{b_2}, \dots, e_{b_{n_1}}\}, b_{l}<b_{l+1}, l\in [1,n-1]$.

\begin{lemma}
    
    We define that:
    \begin{align}
        &x_{i,k}=
            \begin{cases}
              0, & \text{if } c_{i, h_i(e_k)}=0\land F_{i,k}\leqslant \frac{1}{2}\lambda_i,
            \\
              f_i(e_k), & \text{if } c_{i, h_i(e_k)}=0\land F_{i,k} > \frac{1}{2}\lambda_i,
            \\
              f_i(e_k), & \text{otherwise, } c_{i, h_i(e_k)}>0.
            \end{cases}\\
        &X^{(i)}=\sum_{l=1}^{n_0} x_{i,a_l}
    \end{align}
    For any fixed $h_i()$, the $X^{(i)}$ is an upper bound of the total frequency of small flows that enters the next level:
    \begin{align}
        F_{i+1}\leqslant X^{(i)}
    \end{align}
\end{lemma}


\begin{proof}
    We consider every bucket respectively. 
    For small flows, their total frequencies that enter the next level is denoted by $f'_{i,j}\coloneqq \sum_{e\in S^{i,j}_0}f_{i+1}(e)$.
    
    Because: ......
    We have:
    \begin{align}
        f'_{i,j}\leqslant g_{i,j}=
            \begin{cases}
              0, & \text{if } c_{i,j}=0\land f_{i,j}\leqslant \lambda_i,
            \\
              f_{i,j}-\lambda_i, & \text{if } c_{i,j}=0\land f_{i,j}> \lambda_i,
            \\
              f_{i,j}, & \text{otherwise, } c_{i,j}>0.
            \end{cases}
    \end{align}
    
    Because: ..... We have:
    \begin{align*}
        % &g_{i,j} \leqslant q_{i,j}=\sum_{\forall e_k, h_i(e_k)=j} x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]\\
        &g_{i,j} \leqslant q_{i,j}=\sum_{\forall k, e_k\in S^{i,j}_0} x_{i,k}\\
        &X^{(i)}=\sum_{k=1}^n x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]\\
        &=\sum_{j=1}^{w_i}\sum_{\forall e_k, h_i(e_k)=j} x_{i,k}*[f_i(e_k) \leqslant \frac{1}{2}\lambda_i]=\sum_{j=1}^{w_i}q_{i,j}\\
        &F_{i+1}=\sum_{j=1}^{w_i}f'_{i,j}\leqslant \sum_{j=1}^{w_i}q_{i,j}=X^{(i)}
    \end{align*}


\end{proof}


Similarly, we have the following lemma.
\begin{lemma}
%   $C_{i,j,k}=\sum_{l \in [1,k-1]}1*[h_i(e_l)=j \land f_i(e_l) > \frac{1}{2}\lambda_i]$. 
   Let 
    \begin{align}
        &y_{i,k}=
            \begin{cases}
              0, & \text{if } C_{i,k}=0\land f_{i,h_i(e_k)}\leqslant \lambda_i,
            \\
              1, & \text{if } C_{i,k}=0\land f_{i,h_i(e_k)}> \lambda_i
            \\
              2, & \text{otherwise, } C_{i,k}>0.
            \end{cases}\\
        &Y^{(i)}=\sum_{l=1}^{n_1} y_{i,b_l}
    \end{align}
    For any fixed $h_i()$, the $Y^{(i)}$ is an upper bound of the number of distinct large flows that enters the next level:
    \begin{align}
        C_{i+1}\leqslant Y^{(i)}
    \end{align}
\end{lemma}

\begin{proof}
    proof
    For large flows, the total number of distinct large flows that enter the next level is denoted by $c'_{i,j}\coloneqq |\{e| f'_i(e)>0, e\in S^{i,j}_1\}|$. We have
    \begin{align}
        c'_{i,j}\leqslant c_{i,j}
    \end{align}
        $$\sum_{j=1}^{w_i}g_{i,j}\leqslant\sum_{j=1}^{w_i}q_{i,j}= X^{(i)}$$
\end{proof}




\begin{theorem}
    Consider the $i^{th}$ level, $P_{k}=h_i(e_k)$ are independent random variables.
    \begin{align}
        & \Pr_{P_{a_l}}[x_{i,a_l}>0]\leqslant  \frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i} \forall P_{1}, P_2,\dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}
    \end{align}
    
    \begin{align}
        & \Pr_{P_{b_l}}[y_{i,b_l}>0]\leqslant  \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \forall P_{1}, P_2,\dots, P_{b_l-1},  P_{b_l+1},\dots, P_{b_{n_1}}
    \end{align}
        
\end{theorem}




\begin{theorem}
    For any $S$ satisfies:
    \begin{align}
        & \frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S}\\
        & \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S} 
    \end{align}
    We construct random variables $X'^{(i)}$, $Y'^{(i)}$:
    $\forall\ given\ or\ ungiven\ P_{1}, P_2,\dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}$:
    For $P_{a_l}$ that $x_{i,a_l}>0$, let $X_l=f_i(e_{a_l})$. For random $P_{a_l}$ that $x_{i,a_l}=0$, let $X_l=f_i(e_{a_l})$ to make $\Pr[X_l=f_i(e_{a_l})]=\frac{1}{S}$. Otherwise, for other $P_{a_l}$, $x_{i,a_l}=0 and X_l=0$. $\Pr[X_l=0]=1-\frac{1}{S}$.
    \begin{align}
        &X'^{(i)}=\sum_{l=1}^{n_0} X_l, X_l\leqslant f_i(e_{a_l})\\
        % &\Pr[Y_l=2]=\frac{1}{S}, \Pr[Y_l=0]=1-\frac{1}{S}\\
        &Y'^{(i)}=\sum_{l=1}^{n_1} Y_l, Y_l\leqslant 2
    \end{align}
    For given $P_{1}, P_2,\dots, P_{a_l-1},  P_{a_l+1},\dots, P_{a_{n_0}}$, $P_{a_l}$ decides the value of $X_l$. $X_l$ is an independent variable from other $X_{...}$.\\
    $\forall\ given\ P_{...}$, $X_l\geqslant x_{i,a_l}$ and therefore $X'^{(i)}\geqslant X^{(i)}$.
    So, We have:
    \begin{align}
        &\forall t \Pr[X'^{(i)}>t] \geqslant \Pr[X^{(i)}>t]\\
        &\forall t \Pr[Y'^{(i)}>t] \geqslant \Pr[Y^{(i)}>t] 
    \end{align}
        
\end{theorem}

\begin{proof}
    
    % \begin{align}
    %     &\Pr[X_l=f_i(e_{a_l})]=\frac{1}{S}, \Pr[X_l=0]=1-\frac{1}{S}\\
    %     &\forall t \Pr[X_l>t]\geqslant \Pr[x_{i,a_l}>t]\\
    %     &X'^{(i)}=\sum_{l=1}^{n_0} X_l, X_l\leqslant f_i(e_{a_l})\\
    %     &\forall t \Pr[X'^{(i)}>t] \geqslant \Pr[X^{(i)}>t]\\
    %     & \Pr_{P_{b_l}}[y_{i,b_l}>0]\leqslant  \frac{F_i}{\lambda_i w_i}+ \frac{C_i}{w_i}  \leqslant \frac{1}{S} \forall P_{1}, P_2,\dots, P_{b_l-1},  P_{b_l+1},\dots, P_{b_{n_1}}\\
    %     &\Pr[Y_l=2]=\frac{1}{S}, \Pr[Y_l=0]=1-\frac{1}{S}\\
    %     &\forall t \Pr[Y_l>t]\geqslant \Pr[y_{i,b_l}>t]\\
    %     &Y'^{(i)}=\sum_{l=1}^{n_1} Y_l, Y_l\leqslant 2\\
    %     &\forall t \Pr[Y'^{(i)}>t] \geqslant \Pr[Y^{(i)}>t] 
    % \end{align}
\end{proof}


\begin{theorem}
General chernoff: There are $n$ independent random variable $X_i$ and $p$. $Pr(X_i=s_i(0\leqslant s_i \leqslant 1) )=p$,$Pr(X_i=0)=1-p$\\ $\sum s_i=m$, $\mu=E[X=\sum x_i]=mp$.
$$Pr[X>(1+\delta)\mu] \leqslant (e^{1.75-(1+\delta)})^{mp}$$
\end{theorem}
\begin{proof}

\begin{align*}
    &Pr[X>(1+\delta)\mu]\leqslant \frac{E[e^{tX}]}{e^{t(1+\delta)\mu}}\\
    &E[e^{tX}]=\prod_i{E[e^{t X_i}]}\\
    &E[e^{t X_i}]=e^{t s_i}p+(1-p)=(e^{t s_i}-1)p+1\\
    &x=(e^{t s_i}-1)p, 1+x<e^x\\
    &E[e^{t X_i}]\leqslant e^{(e^{t s_i}-1) p}\\
    &if 0<t<=1, x=t s_i\leqslant 1, e^x\leqslant 1+1.75x\\
    &E[e^{tX}]=\prod_i{E[e^{t X_i}]}=e^{\sum_i[(e^{t s_i}-1)p]}\leqslant e^{\sum_i[1.75 t s_i p]}=e^{1.75mpt}\\
    &Pr[X>(1+\delta)\mu] \leqslant \frac{e^{1.75mp}}{e^{t(1+\delta)mp}}=(e^{1.75-t(1+\delta)})^{mpt}, t=1
\end{align*}

\end{proof}


\begin{theorem}
Hoeffding's inequality: Let $X_1,\cdots, X_n$ be independent random variables, $X_i$ are strictly bounded by interval $[a_i, b_i]$. Let $S_n$ be the sum of the random variables:
\begin{align}
    & \Pr\left[ S_n - E[S_n]\geqslant t\right]\leqslant \exp\left( -\frac{2t^2}{\sum_{i=1}^n(b_i-a_i)^2}\right)
\end{align}
\end{theorem}
 

$w_i=\lceil\frac{W (R_{w}-1)}{R_{w}^i}\rceil$, $\sum w_i \leqslant W+d$,

$\lambda_i= \frac{\Lambda (R_\lambda-1)}{R_\lambda^i} $, $\sum \lambda_i\leqslant \Lambda$, 
$\Lambda=\epsilon \Vert F\Vert_1$, $\lambda_i=\frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i} $

Let $ R=R_w R_\lambda$.

$\alpha_i= \frac{\Vert F\Vert_1}{R^{i-1}}$,

$\beta_i= \frac{2 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)}$,

$\frac{\alpha_i}{max(1, \frac{1}{2}\lambda_i)}\leqslant \frac{2 \alpha_i}{\lambda_i}=  \frac{2 \frac{\Vert F\Vert_1}{(R_{w}R_{\lambda})^{i-1}} R_\lambda^i}{ \epsilon \Vert F\Vert_1 (R_\lambda-1)} = \frac{2 R_\lambda}{\epsilon R_{w}^{i-1}(R_\lambda-1)}=\beta_i$

\begin{comment}
\begin{theorem}
    When $T_i=\alpha_i, U_i=\beta_i$, 
    \begin{align}
         &\text{From :}\frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i}
         \leqslant \frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i} \leqslant \frac{2 U_i}{w_i}\leqslant\frac{1}{S} \\
        &\text{We have :} \\
        &\Pr[F_{i+1}>\frac{(1+\delta)}{S}T_i] \leqslant
        \Pr[X^{(i)}>\frac{(1+\delta)}{S}T_i]\leqslant e^{(0.75-\delta)\frac{1}{S}\frac{T_i}{\frac{1}{2}\lambda_i}}\\
        & \Pr[C_{i+1}>\frac{(1+\delta)}{S}U_i] \leqslant
        \Pr[Y^{(i)}>\frac{(1+\delta)}{S} U_i ]\leqslant e^{(0.75-\delta)\frac{1}{S}\frac{U_i}{2}}
    \end{align}
    \label{math:smallprob}
\end{theorem}
\end{comment}

\begin{theorem}
    When $T_i=\alpha_i, U_i=\beta_i$, 
    \begin{align}
         &\text{From :}\frac{F_i}{\frac{1}{2}\lambda_i w_i}+ \frac{C_i}{w_i}
         \leqslant \frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i} \leqslant \frac{2 U_i}{w_i}\leqslant\frac{1}{S_i} \\
        &\text{We have :} \\
        &\Pr[F_{i+1}>\frac{(1+\delta)}{S_i}T_i] \leqslant
        \Pr[X^{(i)}>\frac{(1+\delta)}{S_i}F_i]\leqslant 
        \exp\left(-\frac{8\delta^2F_i^2}{n_0\lambda_i^2S_i^2}\right)
        %& \Pr[C_{i+1}>\frac{(1+\delta)}{S}U_i] \leqslant
        %\Pr[Y^{(i)}>\frac{(1+\delta)}{S} C_i ]\leqslant e^{(0.75-\delta)\frac{1}{S}\frac{U_i}{2}}
    \end{align}
    \label{math:smallprob}
\end{theorem}


\begin{theorem}
When $T_i=\frac{\alpha_i}{\gamma_i}$, $U_i=\frac{\beta_i}{\gamma_i}$, $S_i=S_0 \gamma_i$
Let $W=\frac{4 S_0 R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) } $.
We have:
$$ \frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i}\leqslant\frac{1}{S_i}=\frac{1}{S_0\gamma_i}$$.
\end{theorem}

\begin{proof}
% \begin{align*}
%     &\frac{T_i}{\lambda_i w_i}\leqslant \frac{T_i}{\lambda_i \frac{W (R_{w}-1)}{R_{w}^i}}\\
%     &\text{Solving the inequality:} \frac{T_i}{\lambda_i \frac{W (R_{w}-1)}{R_{w}^i}} \leqslant \frac{1}{S_1}\\
%     & W\geqslant W^{*}= \frac{T_i S_1}{\lambda_i \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &W^{*}=\frac{\frac{\Vert F\Vert_1}{(R_{w}R_{\lambda})^{i-1}} S_1}{ \frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i} \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &=\frac{S_1(R_{w}R_{\lambda})}{\epsilon  (R_\lambda-1)(R_{w}-1)}\\
% \end{align*}

\begin{align*}
    &\frac{T_i}{\frac{1}{2}\lambda_i w_i}=\frac{\frac{\alpha_i}{\gamma_i}}{\frac{1}{2}\lambda_i w_i}
        \leqslant \frac{\frac{\beta_i}{\gamma_i}}{w_i}\\
    &\frac{T_i}{\frac{1}{2}\lambda_i w_i} + \frac{U_i}{w_i}\leqslant \frac{2\frac{\beta_i}{\gamma_i}}{w_i}\\
    &\frac{2U_i}{w_i}\leqslant \frac{2\frac{\beta_i}{\gamma_i}}{\frac{W (R_{w}-1)}{R_{w}^i}}\\
    &\text{Solving the inequality:} \frac{2\frac{\beta_i}{\gamma_i}}{\frac{W (R_{w}-1)}{R_{w}^i}} \leqslant \frac{1}{S_0\gamma_i}\\
    &W\geqslant W^{*}= \frac{2 \frac{\beta_i}{\gamma_i} S_0\gamma_i}{\frac{(R_{w}-1)}{R_{w}^i}}\\
    & W^{*}= \frac{ 2\frac{2 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)} S_0}{\frac{(R_{w}-1)}{R_{w}^i}}\\
    &=  \frac{4 S_0 R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) }
\end{align*}

% Let $S_2=2 S$.
% \begin{align*}
%     % \frac{T_i}{\lambda_i w_i} + \frac{U_i}{w_i}\leqslant\frac{1}{S_1}+\frac{1}{S_2}=\frac{1}{S}
%     \frac{2 U_i}{w_i}\leqslant\frac{1}{S}
% \end{align*}
\end{proof}




Let $D_i$ be the number of flows whose flow size is in $(\frac{1}{2}\lambda_{i+1}, \frac{1}{2}\lambda_{i}]$, and these flows enters $i+1$ level.
$D_i\leqslant F_{i+1}/max(1,\frac{1}{2}\lambda_{i+1})$
Let $E_i$ be the number flows whose flow size is greater than $\frac{1}{2}\lambda_{i}$, and these flows enters $i+1$ level.
$C_{i+1}=D_{i}+E_{i}$. 


\begin{align*}
    &\gamma_i=R^{a_i}, S_0=R^k\\
    &\frac{1}{S}=\frac{1}{R^{k+a_i}}\\
    &\text{Suppose:} R\geqslant 2(1+\delta)\\
    &\text{We want:} T_{i}\frac{1+\delta}{S}\leqslant \frac{1}{2}T_{i+1}\\
    &\text{We need:} \frac{\Vert F\Vert_1}{R^{i-1+a_i}}\frac{1}{R^{a_i+k}}\leqslant \frac{\Vert F\Vert_1}{R^{i+a_{i+1}+1}}\\
    & a_{i+1} = 2 a_i+k-2\\
    & a_{i+1}+k-2 = 2 (a_i+k-2)\\
    & a_{i}+k = 2^{i-1}(k-2)+2, (k-2\geqslant0)\\
\end{align*}

% \begin{align*}
%     &T'_i=\frac{T_i}{R^{a_i}}=\frac{\Vert F\Vert_1}{R^{i-1+a_i}}, a_1=0\\
%     &U'_i=\frac{U_i}{R^{a_i}}=\frac{4 R_\lambda}{ \epsilon R^{a_i} R_{w}^{i-1}(R_\lambda-1)}\\
%     &\frac{T_i}{max(1, \floor{\frac{1}{2}\lambda_i})}\leqslant U_i, \frac{T'_i}{max(1, \floor{\frac{1}{2}\lambda_i})}\leqslant U'_i,\\
%     &S=R^k\\
%     &Pr[X\geqslant \lambda_i | F_i\leqslant T'_i =\frac{T_i}{R^{a_i}}]\leqslant\frac{1}{S*R^{a_i}}\\
%     &F_{i+1}\leqslant F_{i}\frac{1+\delta}{2*S*R^{a_i}}\\
%     &S=R^k, \delta=1\\
%     &F_{i+1} \leqslant T'_{i}\frac{1}{R^{a_i+k}}\leqslant T'_{i+1}\\
%     & \frac{\Vert F\Vert_1}{R^{i-1+a_i}}\frac{1}{R^{a_i+k}}\leqslant \frac{\Vert F\Vert_1}{R^{i+a_{i+1}}}\\
%     & a_{i+1}\geqslant 2 a_i+k-1\\
%     & a_{i}\geqslant 2^{i-1}, (k-1\geqslant1,i>1)\\
% \end{align*}
When $k=3, S_i=R^{2^{i-1}+2}, a_{i}=2^{i-1}-1, R\geqslant 2(1+\delta), W=\frac{4 S R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) }$, we have:

\begin{align*}
    &F_{i+1}\leqslant \frac{1+\delta}{S_i} F_{i}\leqslant \frac{1+\delta}{S_i}T_{i}=
     \frac{1+\delta}{R^{2^{i-1}+2}} \frac{\frac{\Vert F\Vert_1}{R^{i-1}}}{R^{2^{i-1}-1}}\leqslant
     \frac{1+\delta}{R} \frac{\frac{\Vert F\Vert_1}{R^{i}}}{R^{2^{i}-1}}\leqslant
    \frac{1}{2}T_{i+1}\leqslant T_{i+1}\\
    &D_{i}\leqslant \frac{F_{i+1}}{max(1,\frac{1}{2}\lambda_{i+1})}
    \leqslant \frac{\frac{1}{2}T_{i+1}}{\frac{1}{2}\lambda_{i+1}}
    \leqslant \frac{1}{2}U_{i+1}\\
    &E_{i}\leqslant \frac{1+\delta}{S_i}U_{i}=\frac{1+\delta}{R^{2^{i-1}+2}} \frac{\frac{2 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)}}{R^{2^{i-1}-1}} =\frac{1+\delta}{R} \frac{\frac{2 R_\lambda}{ \epsilon R_{w}^{i}(R_\lambda-1)}}{R^{2^{i}-1}}\frac{1}{R_\lambda}\leqslant \frac{1}{2 R_\lambda} U_{i+1}\leqslant \frac{1}{2} U_{i+1}\\
    &C_{i+1}=E_i+D_i\leqslant U_{i+1}
\end{align*}



We consider $e^{-25}=1.3e-11$ is a sufficient small failure probability that can be ignored.
From theorem \ref{math:smallprob}, we just need to consider one case: Find a largest $i$ satisfies  $(0.75-\delta)\frac{1}{S}\frac{U_{i-1}}{2}=\frac{(0.75-\delta)}{2}\cdot\frac{1}{2(1+\delta)}U_{i}\leqslant -25$. $U_{i}$ is reliable here. Suppose $\lambda=3$, $U_{i}\geqslant 178$
Then $p_{i+t}\leqslant \frac{1}{R^{k+a_{i}-t}}$.
\begin{align*}
    &Pr[fail]\leqslant178*\prod_{t=1} p_{i+t}\\
    &=178*\frac{1}{R^{(k+a_{i})(k+a_{i}-1)/2}}\\
\end{align*}

\begin{align*}
    & U_i>178\\
    &\frac{2 R_\lambda}{ \epsilon R^{a_i} R_{w}^{i-1}(R_\lambda-1)}>178\\
    &\frac{2 R_\lambda}{ \epsilon 178 R_{w}^{i-1}(R_\lambda-1)}>R^{2^{i-1}-1}\\
    &t>R^{2^{i-1}}, t=\frac{2 R_\lambda R }{ \epsilon 178 R_{w}^{i-1}(R_\lambda-1)}\\
    &i-1<\log_2(\log_R(t))\\
    &i^*-1=\floor{\log_2(\log_R(t))}\\
    &>= \log_2(\log_R(t))-1\\
\end{align*}

\begin{align*}
    &Pr[fail]\leqslant 178*\frac{1}{R^{(k+a_{i^*})(k+a_{i^*}-1)/2}}\\
    &Pr[fail]\leqslant 178*\frac{1}{R^{(2^{i^*-1}+2)(2^{i^*-1}+2-1)/2}}\\
    &2^{i^*-1}\geqslant \frac{1}{2}\log_R(t)\\
    &(2^{i^*-1}+2)(2^{i^*-1}+2-1)/2\geqslant \frac{1}{8}\log_R^2(t)\\
    &Pr[fail]\leqslant 178*\frac{1}{t^{\frac{1}{8} \log_R(t) }}\\
    &Pr[fail]\leqslant 178*\frac{1}{(t)^{\frac{1}{8} t }}\\
    &\leqslant 178*t^{-\frac{1}{8} t}, t=\frac{R_\lambda}{ 50 \epsilon (R_\lambda-1)}\\
\end{align*}

$\Lambda =\epsilon_2 \Vert F\Vert_2^{res(k)}=\epsilon_1 \Vert F\Vert_1$
Our Space: $O(1/\epsilon_1)=O(\frac{\Vert F\Vert_1}{\epsilon_2 \Vert F\Vert_2^{res(k)}})$
A common count sketch uses $O(\frac{1}{\epsilon_2})$. When $\frac{\Vert F\Vert_1}{\Vert F\Vert_2^{res(k)}}\leqslant \frac{1}{\epsilon_2}$, our sketch will be better.



 














% Let $X$ denote the total frequency of all other flows that mapped into the same bucket. $X=\sum_{\forall e_j, h_i(e_j)=h_i(e_j)}f_i(e_j)$ 
% If $X\leqslant \lambda_i$, the bucket must not be locked. If a bucket is not locked, all flows in the bucket will not enter the next level. 
% For each flow, we have a random variable $f_j$ that denotes the number of packets that this flow enters the next level.


% Suppose there are $F_i$ packets whose flow size is smaller than $\leqslant \frac{1}{2}\lambda_i$, called small flows, and $B_i$ flows flow size is greater than $>\frac{1}{2}\lambda_i$ enter the $i^{th}$ level, called large flows. We will bound $F_i$ and $B_i$, with high probability, with $T_i, U_i$.


% For one bucket $B[j]$ and those flows (including all flows. small flow total frequency $F$) mapping to it, no matter in what order these flows arrive, if there is no large flow maps to it, the number of packets (of small flows) that enters the next level is no greater than $S[j]= max(F-\lambda_i,0)$. 
% If there is any large flow maps to it, the number is no greater than $S[j]=F$.
% If we sum up $S=S[j]$ for all buckets, we will get the upper bound of the total number of packets of small flows that enter the next level.
% Instead of count $S$ for every bucket, we count the sum $S$ by flow order.
% We count $S$ in a way that we observe each flow one by one. Choose an arbitrary order of flows , $F=\sum f_1...f_k...f_n$. In an arbitrary fixed condition that each flow is mapped to a bucket. We can count $S$ in the following way. We insert each flow by the order. For flow $f_k$, when it is a small flow (otherwise we ignore it in this step) and its mapped bucket already has $f0$ packets mapped into the bucket. If there has any large flow mapped into the bucket, we add $S'[j]$ by $f_k$. Otherwise, if $f0\geqslant \lambda_i$, we add $S'[j]$ by $f_k$. Otherwise, we add $S'[j]$ by $max(0,f0+f_k-\lambda)$. $S'[j]\geqslant S[j]$ will be count correctly. $S'=\sum S'[j]\geqslant S$. If $S'[j]$ increases when inserting $f_k$, we say that $f_k$ enters the next level.
% We consider each flow one by one. Suppose $f_1...f_{k-1}$ are mapped to fixed buckets.
% % Let $X$ be the total number of packets of small flows (from $f_1...f_{k-1}$) that map into the same bucket with $f_{k}$. 


% If a small flow $f1 (0<f1\leqslant \floor{\frac{1}{2}\lambda_i})$ maps into a bucket with $f0 (0\leqslant f0 \leqslant \floor{\frac{1}{2}\lambda_i})$ packets, the flow $f1$ will not enter the next level. When $f0\geqslant \floor{\frac{1}{2}\lambda_i}+1 > \frac{1}{2}\lambda_i $, $f1$ can enter the next level.

% \begin{align*}
% &Pr[f_{k} \text{ enters the next level}|f_{k} is small flow] \\
% &\leqslant Pr[X>\lambda_i| F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j] \\
% \end{align*}
% $X_1$ denotes the event that no large flow maps into the same bucket $B_i[h_i(f_{k})]$ and the total frequency of other flows mapping into the bucket is $>\frac{1}{2}\lambda_i$. $X_2$ denotes the event that at least one large flow is mapped to the same bucket as $f_{k}$.

% \begin{align*}
% &Pr[f_{k} \text{ enters the next level}]\\
% &\leqslant Pr[Union (X_1, X_2)| F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j]\\
% &\leqslant Pr[X_1| F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j]\\
% &+ Pr[X_2 | F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j]\\
% &\leqslant \frac{1}{S}\\
% \end{align*}

 
% \begin{align*}
% &Pr[X_1| F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j]\\
%     &\leqslant \frac{T_i}{\frac{1}{2}\lambda_i w_i}\leqslant \frac{T_i}{\frac{1}{2}\lambda_i \frac{W (R_{w}-1)}{R_{w}^i}}\\
%     &\text{let it smaller than:} \leqslant \frac{1}{S}\\
%     & W\geqslant W^{*}= \frac{T_i S_1}{\frac{1}{2}\lambda_i \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &W^{*}=\frac{\frac{\Vert F\Vert_1}{(R_{w}R_{\lambda})^{i-1}} S_1}{ \frac{1}{2}\frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i} \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &=\frac{2 S_1(R_{w}R_{\lambda})}{\epsilon  (R_\lambda-1)(R_{w}-1)}\\
% \end{align*}


% \begin{align*}
%     &Pr[X_2 | F_i \leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\\
%     &\leqslant \frac{U_i}{w_i}\leqslant \frac{U_i}{\frac{W (R_{w}-1)}{R_{w}^i}}\\
%     &\text{let it smaller than:} \leqslant \frac{1}{S_2}\\
%     &W\geqslant W^{*}= \frac{U_i S_2}{\frac{(R_{w}-1)}{R_{w}^i}}\\
%     & W^{*}= \frac{ \frac{2 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)} S_2}{\frac{(R_{w}-1)}{R_{w}^i}}\\
%     &\leqslant  \frac{2 S_2 R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) }
% \end{align*}



% Let $S_1=S_2=2S$.
% We have:
% \begin{theorem}

% $W=\frac{4 S R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) } $ satisfies $$Pr[f_{k}\ enters\  the\ next\ level|f_{k}\ is\ small\ flow,$$ $$ F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\leqslant \frac{1}{S} $$.
% \end{theorem}


% Next, we count the number of large flows that enters the next level.
% For one bucket $B[j]$, if there is more than one large flows ($t$) mapped into it. We add $S[j]$ by $t$. If there is more than one large flows ($t$) mapped into it, we add $S[j]$ by $t$. If there is one large flow and the total small flow frequency sum $F$ is greater than $\lambda_i$, we add $S[j]$ by $1$.
% We count $S$ in a way that we observe each flow one by one. Choose an arbitrary order of flows , $F=\sum f_1...f_k...f_n$.
% For flow $f_k$ and its mapped bucket $B[j]$, if there is already a large flow mapped to this bucket, we add $S[j]$ by $2$. If the total small flow frequency sum $F$ is greater than $\lambda_i$, we add $S[j]$ by $1$.

% \begin{align*}
%     &Pr[f_k\ enters |f_k\ is\ large, F_i \leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\\
%     &Pr[X_1|...]+Pr[X_2|...]\\
%     &\leqslant \frac{1}{S}
% \end{align*}

% $X_1$ denotes the event that no large flow maps into the same bucket $B_i[h_i(f_{k})]$ and the total frequency of other flows mapping into the bucket is $>\lambda_i$. $X_2$ denotes the event that at least one large flow is mapped to the same bucket as $f_{k}$.


% \begin{align*}
%     &Pr[X_1|f_k\ is\ large, F_i \leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\\
%     &\leqslant \frac{T_i}{\lambda_i w_i}\leqslant \frac{T_i}{\lambda_i \frac{W (R_{w}-1)}{R_{w}^i}}\\
%     &\text{let it smaller than:} \leqslant \frac{1}{S_1}\\
%     & W\geqslant W^{*}= \frac{T_i S_1}{\lambda_i \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &W^{*}=\frac{\frac{\Vert F\Vert_1}{(R_{w}R_{\lambda})^{i-1}} S_1}{ \frac{\epsilon \Vert F\Vert_1 (R_\lambda-1)}{R_\lambda^i} \frac{(R_{w}-1)}{R_{w}^i}}\\
%     &=\frac{S_1(R_{w}R_{\lambda})}{\epsilon  (R_\lambda-1)(R_{w}-1)}\\
% \end{align*}

% \begin{align*}
%     &Pr[X_2|f_k\ is\ large, F_i \leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\\
%     &\leqslant \frac{U_i}{w_i}\leqslant \frac{U_i}{\frac{W (R_{w}-1)}{R_{w}^i}}\\
%     &\text{let it smaller than:} \leqslant \frac{1}{S_2}\\
%     &W\geqslant W^{*}= \frac{U_i S_2}{\frac{(R_{w}-1)}{R_{w}^i}}\\
%     & W^{*}= \frac{ \frac{4 R_\lambda}{ \epsilon R_{w}^{i-1}(R_\lambda-1)} S_2}{\frac{(R_{w}-1)}{R_{w}^i}}\\
%     &\leqslant  \frac{4 S_2 R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) }
% \end{align*}

% Let $S_1=5S, S_2=1.25S$.
% We have:
% \begin{theorem}

% $W=\frac{5 S R_{w}R_\lambda}{\epsilon (R_{w}-1) (R_\lambda-1) } $ satisfies $$Pr[f_{k}\ enters\  the\ next\ level|f_{k}\ is\ large\ flow,$$ $$ F_i\leqslant T_i, B_i\leqslant U_i, \forall_{j< k} f_j=s_j ]\leqslant \frac{1}{S} $$.
% \end{theorem}



==> vldb/Math/overestimation.tex <==
\subsection{Proof of Upper Bound and Lower Bound} \postsub
\label{subsec:math:cuoverestimation}
%Here, we show the variance and the error bound of our estimation for each item $e_i$. Then we compare our error bound with that of SS and USS.
%We show the variance and the error bound of our estimation for each item $e_i$ in Theorem \ref{theo:variance} and \ref{theo:bound2}, and we can prove that error of \aname{} is smaller than that of SS and USS.
%Due to space limitation, the details of proofs are provided in Appendix \ref{subsec:appen:error}. 

\begin{theorem}
\label{t1}
	Given a data stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. Let $f_i$ be the real frequency of $e_i$. In the \aname{}, we have
	\begin{equation}
	\begin{aligned}
    \widehat{f_{i}^{lo}}\leq f_i\leq \widehat{f_{i}^{up}}
    \end{aligned}
    \end{equation}
\end{theorem}

\begin{proof}

For each $j = 1,2,\cdots, d$, we prove by induction that, for all $n \in \mathbb{Z}^+$, after $n^{th}$ insertion, 
\begin{equation}
\begin{aligned}
\hat{f}_{i,j}^{lo}\leq f_i\leq \hat{f}_{i,j}^{up}
\end{aligned}
\label{1st}
\end{equation}

\ppp{Base case:} When $n=1$, if $e_1 = e_i$, we have $\hat{f}_{i,j}^{lo} = f_i = \hat{f}_{i,j}^{up} = 1$. Otherwise, $\hat{f}_{i,j}^{lo} = f_i = \hat{f}_{i,j}^{up} = 0$. In both circumstances, the conclusion holds.

\ppp{Induction Step:} Let $k \in \mathbb{Z}^+$ be given, and suppose \eqref{1st} is true for $n=k$. We will prove that \eqref{1st} is true for $n=k+1$. Let $low_k$, $high_k$ and $ID_k$ be the low counter, high counter and ID of bucket $B[h_j(e_i)]$ after the $k^{th}$ insertion, when we insert $e_{k+1}$ into the bucket $B[h_j(e_i)]$, There are four possible cases.

\noindent Case 1: $e_{k+1}$ is not inserted into $B[h_j(e_i)]$.

In this case, if $e_{k+1} = e_i$, then $\hat{f}_{i,j}^{up} > \min_{j = 1}^d\{\hat{f}_{i,j}^{up}\}$ before inserting $e_{k+1}$. Because $f_i$ increases by 1, we have $f_i \leq \hat{f}_{i,j}^{up}$ after insertion. Since $\hat{f}_{i,j}^{lo}$ does not change, we also have $\hat{f}_{i,j}^{lo}\leq f_i$ after insertion. Otherwise, if $e_{k+1}\neq e_i$, then $f_i$, $\hat{f}_{i,j}^{lo}$, $\hat{f}_{i,j}^{up}$ are all unchanged. Therefore, the conclusion holds.

\noindent Case 2: $e_{k+1}$ is inserted into $B[h_j(e_i)]$ and $ID_k = e_{k+1}$.

In this case, $low_{k+1} = low_{k} + 1$, $high_{k+1} = high_k + 1$. If$e_i = ID_k$, then $f_i$, $\hat{f}_{i,j}^{up}$, $\hat{f}_{i,j}^{lo}$ are all increased by 1. Otherwise,  $f_i$, $\hat{f}_{i,j}^{up}$, $\hat{f}_{i,j}^{lo}$ keep unchanged. Thus, the conclusion still holds.
    
\noindent Case 3:  $e_{k+1}$ is inserted into $B[h_j(e_i)]$, $ID_k \neq e_{k+1}$ and $low_{k} = 0$.

In this case, $low_{k+1} = 1$, $high_{k+1} = high_k+1$, $ID_{k+1} = e_{k+1}$. If $e_i = e_{k+1}$, then $\hat{f}_{i,j}^{lo} = 1$, both $f_i$ and $\hat{f}_{i,j}^{up}$ increase by 1. Otherwise, $\hat{f}_{i,j}^lo = 0$, both $f_i$ and $\hat{f}_{i,j}^{up}$ do not change. For both circumstances, the conclusion holds.
    
\noindent Case 4:  $e_{k+1}$ is inserted into $B[h_j(e_i)]$, $ID \neq e_{k+1}$ and $low_{k} > 0$.

In this case, $low_{k+1} = low_{k} - 1$, $high_{k+1} = high_k + 1$. If$e_i = ID_k$, then $\hat{f}_{i,j}^{lo}$ decreases by 1, while $f_i$ and $\hat{f}_{i,j}^{up}$ do not change. Otherwise, $\hat{f}_{i,j}^{up}$ increases by 1, while $f_i$ and $\hat{f}_{i,j}^{lo}$ keep unchanged. Therefore, the conclusion holds.

\ppp{Conclusion:} By the principle of induction, \eqref{1st} is true for all $n \in \mathbb{Z}^+$. That is to say, in the \aname, we have
\begin{equation*}
	\begin{aligned}
    \widehat{f_{i}^{lo}} = \max\limits_{j=1}^d \{\hat{f}_{i,j}^{lo}\}\leq f_i\leq \min\limits_{j=1}^d \{\hat{f}_{i,j}^{up}\} = \widehat{f_{i}^{up}}
    \end{aligned}
    \end{equation*}
\end{proof}
% \begin{proof}
% If $e_i$ is error-free, then $\hat{f_i} = f_i$. Otherwise, we have$\hat{f_i} = \left(\sum_{e_j \in S_e}f_j\cdot s(e_j)\right)\cdot s(e_i)$, where $S_e$ is the set of the items that are not error-free. According to \ref{subsec:math:unbiased}, $E(\hat{f_i})=f_i$, so we get the variance of $\hat{f_i}$ that 
% $Var(\hat{f_i}) &= E_{s(e_j)\in \{1,-1\}} \left( \left(\sum_{e_j \in S_e,j\neq i}f_j\cdot s(e_j)\right)\cdot s(e_i)\right)^2
% =E_{s(e_j)\in \{1,-1\}}\left(\sum_{e_j \in S_e,j\neq i}f_j\cdot s(e_j)\right)^2$

% From the analysis in \ref{subsec:math:unbiased}, we find that $s(e_i)$ and whether $e_i$ is error-free is independent. Thus, the cross terms have the same chance to be positive and negative, their expectation is $0$. Therefore, we have
% $Var(\hat{f_i}) 
% =E_{s(e_j)\in \{1,-1\}}\left(\sum_{e_j \in S_e, j\neq i} (f_j)^2\right)
% \leqslant  \sum_{e_j \neq e_i} (f_j)^2$
% \end{proof}

% According to the variance, we can derive an error bound for $\left\|f\right\|_2$.


% \begin{proof}
% Based on Chebyshev's theorem, we have
% $P\left(\left|\hat{f_i}-f_i\right| \geqslant \sqrt{e \sum_{e_j \neq e_i} (f_j)^2}\right) 
% \leqslant
% \frac{Var(\hat{f_i})}{\left(\sqrt{e \sum_{e_j \neq e_i} (f_j)^2}\right)^2} 
% \leqslant \frac{1}{e}$. 

% For items in $B[h(e_i)]$, we can have an estimation that
% $\sum_{e_j} {(f_j)^2} = \frac{1}{l}(\left\|f\right\|_2)^2$. 
% Therefore, we can get\\
% $P\left(\left|\hat{f_i}-f_i\right| \geqslant \epsilon \left\|f\right\|_2\right) 
% \leqslant 
% P\left(\left|\hat{f_i}-f_i\right| \geqslant \epsilon \sqrt{l \cdot \sum_{h(e_j)=h(e_i)} f_j^2}\right)
% \leqslant
% P\left(\left|\hat{f_i}-f_i\right| \geqslant \sqrt{e \sum_{e_j \neq e_i} f_j^2}\right)
% \leqslant \frac{1}{e}$
% \end{proof}

% We can find that this bound is relatively loose because it also takes effect on the items which are in the vote part.
% However, for items in the positive or negative parts, $\sqrt{l \cdot \sum_{e_j \neq e_i} (\Delta_i f_j)^2}$ is often much smaller than $\left\|f\right\|_2$. 

% Then we compare the error of \aname{} with that of SS and USS.
% For SS and USS, we can regard the smallest count in the data structure as the voting part and the other bins in the data structure as the counting part.
% Therefore, we can transform SS and USS to one bucket with a voting part and a counting part.
% Similar to \aname, the error of SS and USS comes from the period when the items are in the count.
% The comparison of their error is shown below.


% \begin{proof}
% For our \aname, 
% \begin{equation}
% \begin{aligned}
% \sup\left|\hat{f_i}-f_i\right|_{Waving} = 
% \left|\sum_{e_j \neq e_i}{f_j\cdot s(e_j)}\right|
% \end{aligned}
% \end{equation}
% For SS, 
% \begin{equation}
% \begin{aligned}
% \sup\left|\hat{f_i}-f_i\right|_{SS} = 
% \left|\sum_{e_j \neq e_i}{f_j}\right|
% \end{aligned}
% \end{equation}
% Though the replacement procedure of USS is different from that of SS, they all increment the minimum counter for each item which is not in the list.
% Therefore, the expression of the error of USS is the same as that of SS.
% If  $f_j$ in our \aname{} is same as $f_j$ in SS and USS, we can get that
% \begin{equation}
% \begin{aligned}
% \sup\left|\hat{f_i}-f_i\right|_{Waving} &= 
% \left|\sum_{e_j \neq e_i}{ f_j\cdot s(e_j)}\right|\\
% &\leqslant \left|\sum_{e_j \neq e_i}{f_j}\right|\\
% &=\sup\left|\hat{f_i}-f_i\right|_{SS}\\
% \end{aligned}
% \end{equation}
% We can find that they are equal only when all $s(e_j)$ is $1$ or all $s(e_j)$ is $-1$.
% \end{proof}

% Even though $f_j$ may be different, $\left|\sum_{e_j \neq e_i}{f_j\cdot s(e_j)}\right|$ is often smaller than $\left|\sum_{e_j \neq e_i}{f_j}\right|$.
% It is because that we divide the data stream into $l$ buckets, so each item may accesses different counting parts and the error is also divided.
% On the contrary, there is only one waving counter in SS and USS, so all unilateral accumulations will occur in the same waving counter and the estimated frequency will be highly overestimated.
% In other word, the error of \aname{} is often smaller than that of SS and USS.

% According to the comparison, we can derive an error bound for $\left\|f\right\|_1$.

% \begin{theorem}
% Let $l = \frac{e}{\epsilon}$, we have
% \[
% P\left(\left|\hat{f_i}-f_i\right| \geqslant \epsilon \left\|f\right\|_1 \right) \leqslant \frac{1}{e}
% \]
% \label{theo:bound1}
% \end{theorem}

% \begin{proof}
% According to Theorem \ref{theo:compare}, we have
% \begin{equation}
% \begin{aligned}
% \centering 
% \mathbb{E}\left[\left|\hat{f_i}-f_i\right|\right]
% &=
% \mathbb{E}\left[\left|\sum_{e_j \neq e_i}{ f_j\cdot s(e_j)}\right|\right]\\
% &\leqslant
% \mathbb{E}\left[\left|\sum_{e_j \neq e_i}{ f_j}\right|\right]\\
% &\leqslant
% \frac{\epsilon \left\|f\right\|_1}{e}
% \end{aligned}
% \end{equation}   

% By the Markov inequality,
% \[
% P\left(\left|\hat{f_i}-f_i\right| \geqslant \epsilon \left\|f\right\|_1 \right)
% \leqslant 
% P\left(\left|\hat{f_i}-f_i\right| \geqslant e \mathbb{E}\left[\left|\hat{f_i}-f_i\right|\right]\right)
% \leqslant
% \frac{1}{e}
% \]  
% \end{proof}

% \begin{theorem}
% Assume that $n$ is the number of different items inserted into the waving counter of $B[h(e_i)]$ and $f_1\geq f_2\geq \cdot\cdot\cdot\geq f_n$ is the frequency of the $n$ items that is not error-free. With probability $2\phi(\lambda) - 1$,
% \begin{equation}
% \begin{aligned}
% \left|\hat{f_i}-f_i\right|\leqslant \sum_{k=1}^{l}f_k-\sum_{k=l+1}^{n}f_k
% \end{aligned}
% \end{equation}
% where $\phi(x)$ is the Cumulative distribution function for normal distribution $N(0,1)$, $l = \frac{[\lambda \sqrt{n}]+n}{2}$, 
% $[x]=\max\{y \in \mathbb{Z}:y\leqslant x\}$.
% \end{theorem}

% \begin{proof}
% $s(e_j)$ are independent and identical distributions, which satisfy 
% \[
% E(s(e_j)) = 0,Var(s(e_j)) = 1
% \]

% According to the central limit theorem, 
% \[
% {\lim_{n \to +\infty}}P(-\lambda\leqslant\frac{\sum_ {k=1}^{n}s(e_k)}{\sqrt{n}}\leqslant\lambda) =2\phi(\lambda) - 1
% \]
% So with probability $2\phi(\lambda) - 1$, the number of items with the same $s(e_i)$ is less than $\frac{[\lambda \sqrt{n}]+n}{2}$. Thus,
% \begin{equation}
% \begin{aligned}
% \left|\hat{f_i}-f_i\right|
% &=\sum_{e_j \neq e_i}{f_j\cdot s(e_j)}\cdot s(e_i)\\
% &\leqslant\left|\sum_ {k=1}^{n}s(e_k)\cdot f_k\right|\\
% &\leqslant\sum_{k=1}^{l}f_k-\sum_{k=l+1}^{n}f_k
% \end{aligned}
% \end{equation}
% \end{proof}
\begin{comment}
So the inequality on the right side is proved. Then we prove the inequality on the left side,i.e., the lower bound of estimation of each item after the $k^{th}$ insertion is never overestimated.  

Base: While $k=1$, the estimation of $e_1$ is obviously accurate, i.e., not overestimated.

Inductive hypothesis: We assume that after the $i^{th}$ insertion, the estimation of each item is not overestimated.

Induction Step: After the $(i+1)^{th}$ insertion, $e_{i+1}$ is inserted to k buckets, some of which will be updated if they return the smallest estimation of $e_i$. Obviously, the estimation of those items which are not hashed to the updated buckets remain unchanged, i.e., not overestimated. Consider one of the updated buckets, denoted by $B[p]$. If $B[p].ID=e_i$, then the estimation of $e_i$ from B[p] increments and keeps not overestimated. And the estimation of the other items that hashed to B[p] remain unchanged, i.e., not overestimated. In another case, $B[p].ID \neq e_i$, the result is the same as that when $B[p].ID=e_i$. As a consequence, after the $i^{th}$ insertion, the estimation of each item is not overestimated.

So the theorem is proved
\end{comment}

==> vldb/Math/zipf.tex <==


\subsection{Analysis for Dominant Items}
\label{subsec:math:dominant}
\begin{theorem}
Given a stream $\mathcal{S}$ which obeys an arbitrary distribution. Given an arbitrary item $e_i$. In the \aname{}, for row $j$, let $F_{i,j}$ be the total number of items mapping to bucket $B_j[h_j(e_i)]$ except for item $e_i$. If $f_i > F_{i, j}$, we have $B_j[h_j(e_i)].ID = e_i$.
\end{theorem}
\begin{proof}
Since there are $f_i + F_{i,j}$ items mapping to the bucket, $B_j[h_j(e_i)].high$ is at most $f_i + F_{i,j}$.
If $B_j[h_j(e_i)].ID \neq e_i$, then $f_{i,j}^{up} = \frac{1}{2}\cdot(B_j[h_j(e_i)].high\hspace{-0.3mm}-B_j[h_j(e_i)].low)\leq \frac{1}{2}\cdot(f_i+F_{i,j})< f_i$. This contradicts with theorem \ref{t1}.
\end{proof}



















\begin{comment}
\begin{proof}

Given a stream $\mathcal{S}$. Given an arbitrary item $e_i$.
Given an absolute error $\epsilon$ and an relative error $\gamma$ with probability at least $1-\delta$,
% In the simplified \aname{}, let $F_{i,j}$ be the total number of items mapping to bucket $B_j[h_j(e_i)]$ except for item $e_i$. Then, for each $j = 1,2,\cdots, d$ and $t > 1$, we have

\begin{align*}
    E[I(i,j,k)] & =Pr[h_j(i)=h_j(k)]\leqslant\frac{1}{w}\\
    E[F_{i,j}] & = E\left(\sum\limits_{k=1}^{n}{I(i,j,k)f_i } \right)
    \leqslant \sum\limits_{k=1}^{n}{E[I(i,j,k)]f_i }\notag \leqslant \frac{M}{w} 
\end{align*}
\noindent By the Markov inequality,
\begin{align*}
    &Pr\left[\widehat{f_{i}^{up}}\geq{}f_i+\epsilon\right] \\
    & = Pr\left[\forall j, F_{i,j}\geq{}\epsilon\right]\\
    & \leqslant \left[\frac{E[F_{i,j}]}{\epsilon}\right]^d = \left[\frac{M}{\epsilon w}\right]^d \\
    \intertext{Let $w=\frac{e M}{\epsilon}$ and $d=\lceil ln(1/\delta) \rceil$.}
    & < \textit{e}^{-d}\leqslant \delta\\
    % =Pr[\forall j,F_{i,j}>\epsilon S]\\
\end{align*}

\begin{align*}
    &Pr\left[\widehat{f_{i}^{up}}\geq{}f_i(1+\gamma)\right] \\
    & = Pr\left[\forall j, F_{i,j}\geq{}f_i\gamma\right]\\
    & \leqslant \left[\frac{E[F_{i,j}]}{f_i\gamma}\right]^d = \left[\frac{M}{f_i\gamma w}\right]^d \\
    \intertext{Let $w=\frac{e M}{f_i\gamma}$ and $d=\lceil ln(1/\delta) \rceil$.}
    & < \textit{e}^{-d}\leqslant \delta\\
    % =Pr[\forall j,F_{i,j}>\epsilon S]\\
\end{align*}

\end{proof}
\end{comment}

==> vldb/feedback.tex <==
Common comment for all reviewers - the novelty of this paper.
Both Reviewer 1 and Reviewer 2 believe that our algorithm (Versatile Sketch) is just a combination of existing works. But we do not believe that our algorithm is a simple combination.
The idea of our algorithm is indeed inspired by existing algorithms. But we believe that a general algorithm must combine the advantages of all algorithms whose functions are not general. A general algorithm inevitably has a certain similarity with existing algorithms.
Our algorithm has a novel structure. For example, it first proposed the low counter, which can report under-estimated frequency and can correct the bias of the over-estimated frequency.
Our conservative update strategy not only refers to the high counter, but also refers to the 3 fields. The correctness of our algorithm is not trivial (See section 5.1 in the paper). The success of our general algorithm is quite precious.

Reviewer 1:
O1. Please refet to the common comment.

O2. Thanks for your suggestions. We will add the theoratical analysis for the advanced applications of VSketch.

O3. Indeed, VSketch doesn't have the ability to handle general turnstile streams.

O4. We will double-check the paper and try our best to make it more accurate.

O5.Thank you for your comments. Our claims in the paper are not accurate. We will explain it carefully in the revised paper. Existing sketches are not suitable to expand because they can only copy the content of the original sketch, While VSketch does not copy the content while expanding. Thus, VSketch can maintain more information than existing sketches when doing expansion. Some sketches (e.g., CM sketches, CU sketches, and Count sketches) can support compression.

We propose the Heavy/Light VSketch to estimate frequencies without recording IDs. Heavy VSketch can output an accurate estimation for frequent items, while Light VSketch can output an accurate estimation for infrequent items. Therefore, Light VSketch can estimate the distribution/entropy of all items because most items are infrequent items.

Reviewer 2:

O1. 
Please refer to the common comment for novelty.

O2.
Thanks for your suggestions. We will add these experimental results in the revised paper.

O3.
In fact, Lemma 5.5 suggests the error bound of under-estimation indirectly, we will try to add an independent section to discuss it, as well as the error analyses for extra operations.


O4.
1) CM and CU sketched are not compared in the experiments of expansion, compression and aggregation. We will add the comparison with CM and CU sketch in these distributed system related experiments in the revised version.

2) Since the high estimate field works similar to the CU sketch, there is almost not improvement in frequency estimate compared to CU sketch. Actually, should Versatile Sketch be worse?

For frequency estimation, VSketch actually has a very close performance compared with CU sketch in ARE and AAE.
And when the memory is extremely tight, the result of Versatile Sketch can be worse but not far from CU sketch.
Moreover, the metrics ARE and AAE sum the errors of all items, while VSketch can achieve even higher precision in dominant items which is discussed in Section 5.2 and 6.2.2.
This is also why VSketch performs better in top-k item detection and other frequent item oriented tasks.

3) The experimental results in Section 6.4.2 show that the original sketch does not show advantage over the compressed sketch. Can you explain why this is the case?

We are sorry about the unclear demonstration. Actually, the compressed VSketch in Section 6.4.2 means we use a VSketch with DOUBLE memory initially to perform insertions, and then we compress it to half for offline queries. Hence the compressed VSketch should be more accurate than a VSketch which does not double its memory (this is exactly the "original sketch" in the figure) when performing insertions.
In this section, we are mean to show that compression is a feasible way to get higher query accuracy with same local storage or network bandwidth. We will explain it more clearly in the revised paper, and add a new figure to compare the compressed VSketch with the double-memory one, illustrating the accuracy loss after compression operation. 

Reviewer 3:

Thank you for your constrictive comments. 
O1. We agree with this statement.
O2. We will elaborate on the space-accuracy trade-off in the revised version.
O3. We agree with this statement.

1) What's the fundamental improvement over existing sketch wrt each specific task? In principle, I don't see any fundamental difference in terms of space-accuracy tradeoff wrt each specific task when compared against the state-of-the-art sketch for that task.

The performance of our algorithm is similar to the results of other algorithms on specific tasks. We hope to accomplish more tasks with the same storage and computing overhead.

2) What's the benefit of having a versatile sketch compared to having a different sketch for a different task?

A sketch with multiple functions can reduce the complexity of parameter configuration and reduce deployment costs. But at the same time it also loses the flexibility to adjust the parameters for each task separately. In addition, if our algorithm can achieve similar effects with the state-of-the-art sketch for each task, in a multi-task scenario, the total storage/computation cost of our algorithm will be smaller.

3) how about deletion of streaming element? It doesn't seem the existing design or analysis support this case. Could you please elaborate on this?

Unfortunately, our algorithm does not support deleting elements, which is one of its shortcomings.

We think your understanding of our algorithm is very accurate. Your suggestions to us help us a lot. We will continue to improve our work. Thank you very much.




2. Please provide answers to the following questions for each of the reviews separately, indicating whether:
(a) They were constructive (i.e., helpful to improve your paper);
(b) They were professional (e.g., language was polite).




Reviewer #1

(a) Yes. The reviewer 1 is constructive. 

(b) Yes. The reviewer 1 is professional. 


Reviewer #2

(a) Yes. The reviewer 2 is constructive.

(b) Yes. The reviewer 2 is professional. 

Reviewer #3

(a) Yes. The reviewer 3 is constructive. 

(b) Yes. The reviewer 3 is professional.

==> vldb/yt_revise_new_intro.tex <==
\presec
\section{Introduction} \postsec
\label{sec:intro}

\presub
\subsection{Background and Motivation}\postsub
% 现在几个主要问题；1、如何和现有工作区分，five properties的概况问题。2、five properties具体内容的充实。3、five properties和idea的连结。idea讲故事（打擂台），还是讲留下关键信息呢？
%
%
%
%%Para1:
% 感觉这句最好再改改，完全没讲到sketch是解决什么问题的算法，感觉不太对。
% Approximate data stream processing has been a hot topic in recent years.
% Sketches \cite{cmsketch}, a series of probabilistic data structures, have attracted wide acceptance and interests owing to the efficiency in term of both time and space.
As the demand for high-volume data stream processing grows, sketches \cite{cmsketch}, a series of probabilistic data structures, have attracted wide acceptance and interests owing to the efficiency in term of both time and space.
% Among existing sketches, some aim to elegant theoretical results \cite{countsketch,Sketchingclassifiers}, some aim to achieve high accuracy with small memory size \cite{coldfilter,pyramid}, some aim to achieve high speed \cite{asketch}, some aim to achieve adaptability for distributed data streams \cite{?}, some aim to achieve single-side error \cite{cusketch} or unbiased estimation \cite{countsketch}.
Various sketches \cite{asketch} have emerged in many fields, including graph stream processing \cite{graphsketches,?}, persistent data structures \cite{persistentsketch,persistent-bf,ada-sketch}, complex aggregate queries \cite{complexaggre}, and online machine leaning \cite{Sketchingclassifiers}.....??
%  versatile sketch   functions/properties

%  Generality, Capability, Adaptability, flexibility, and Certainty.

% Task diversity/Generality
% Interval estimation
% Distributed applicability
% Incremental deployment
% Election certainty

% 1) Generality for various tasks.
% 2) Capability for two-sided boundary estimation  interval estimation和confidence interval
% 3) Adaptability for distributed systems.
% 4) Flexibility for incremental deployment.
% 5) Certainty for dominant items.

Existing sketches often focus on one or a few of the following aspects:
some works focus on applying sketches to a specific task \cite{?....};
some focus on achieving one-sided? error \cite{cusketch} or unbiased estimation \cite{countsketch};
some focus on adaptability for distributed data streams \cite{li2020thresholded};
some focus on improving accuracy with small memory size \cite{coldfilter,pyramid};
some focus on accelerating processing speed \cite{asketch};
some focus on elegant theoretical results \cite{countsketch,Sketchingclassifiers}.

%theoretical的引用到底对不对？



% Among existing sketches, some aim to elegant theoretical results \cite{countsketch,Sketchingclassifiers}, some aim to achieve high accuracy with small memory size \cite{coldfilter,pyramid}, some aim to achieve high speed \cite{asketch}, some aim to achieve adaptability for distributed data streams \cite{?}, some aim to achieve single-side error \cite{cusketch} or unbiased estimation \cite{countsketch}.
Different from existing sketches focusing on a few specific aspects, we aim to design a versatile focusing on the following aspects simultaneously: Generality, Capability, Adaptability, Flexibility, and Certainty.

% Different from existing sketches focusing on a few specific aspects, we aim to design a versatile sketch with multiple (promising/attractive/ multifaceted/ xxxadj?) properties: Generality, Capability, Adaptability, Flexibility, and Certainty.


%现有要么只完成目标单一/优化精度/速度/硬件/分布式。
%
%我们研究5个方面：
% : 
% 1) the first sketch for two-sided boundary estimation while the other sketches can only do one-side estimation. 
%全召回 全准确 是不是可能做成 <item,attribute>这样的？

1) \textit{Generality} for various tasks.
It can be applied to four approximate data stream processing tasks\footnote{A data stream is defined as a sequence of items ordered by time.
1) Frequency estimation is to count the appearing number of occurrences of a given item in the data stream.\\~2) Finding Top-k frequent item is to report $k$ items with the largest frequencies.\\~3) Heavy change detection is to find items whose frequencies in two adjacent time window vary a lot.\\~4) Frequency distribution estimation is to estimate the ration of item whose frequencies are equal to a given value\\~5) Entropy Estimation is to estimate the entropy of item frequencies.}, 
including finding Top-k frequent items, finding heavy change, frequency distribution estimation, and entropy estimation.
These are fundamental tasks in database query optimization \cite{schweller2004reversible}, information retrieval \cite{chowdhury2010introduction}, data mining \cite{?}, data quality estimation \cite{?}, and more \cite{?}.
%vldb sigmod topic搜关键词+sketch
% These tasks are important in database query optimization \cite{schweller2004reversible}, information retrieval \cite{chowdhury2010introduction}, data mining \cite{?}, data quality estimation \cite{?}, and more \cite{?}.
%information retrieval 是本书，要不要加页码？
% network measurement and management, web search engines [31], anomalies detection [32, 33], time series forecasting and outlier analysis [34]. [41, 42], network measurement and monitoring [43]. 
%
% Capability for two-sided estimation.
% % Double Bound
% Capability for double-bound estimation.
% both over-estimation and under-estimation.

2) \textit{Capability} for double-bound estimation\footnote{The estimator can report both an over-estimated value and an under-estimated value.}.
% it is the first sketch for two-sided boundary estimation. 
The common function of sketches is the frequency estimation, which is to query the number of times that a given item appears in the data stream. 
Our \aname{} can report a pair of integers? $<a,b>$ for any given item, and we make sure that the exact answer must be in interval $[a,b]$. 
The length of the interval is small bounded in theory.
% and the interval has multiple functions. 
Double-bound estimation is useful in practice.
For example, when finding frequent items whose frequency is larger than $\mathcal{T}$, we can choose the upper bound or the lower bound to avoid False Negative\footnote{?} or False Positive\footnote{?} respectively. 
% When finding heavy changes, we can achieve the upper/lower bound of the frequency change by above interval.
% When finding heavy changes, we can achieve 100\% precision/recall rate by choosing the upper/lower bound
For another example, when finding items whose frequency is in a given range $[l,r]$, we can make sure the reported item must be in $[l,r]$ as long as the estimated interval is contained?? by the given range.
%

3) \textit{Adaptability} for distributed systems.
The designed sketch should be flexible for expansion, compression, and aggregation, which are important for distributed systems. 
To adapt to dynamic changes in data volume, the designed sketch should dynamically adjust its capacity by the expansion/compression operation.
When aggregating the sketches from different data streams, the designed sketch should aggregate them into one sketch for answering global queries over distributed data streams.

% along the way (\eg, a minimal spanning tree) to save bandwidth.
%

4) \textit{Flexibility} for incremental deployment.
In a very large distributed system, there are many data streams, and different data streams could use different sketches.
%
When designing a sketch for a new data stream, if the new sketch can be transformed into a standard sketch, it will be well compatible with existing old sketch.
%
The standard sketches refer to the CM/CU sketch, which are the most widely used and accepted in the academic and industry fields.
For the new data stream, we can inherit existing system functions, such as query language, network transmission mechanism, and compressing algorithms.

% It can refine itself to get Heavy \aname{}, which has the same structure as CM/CU sketch and can collaborate with CM/CU in the same system.
% \wyh{Light \aname{}?}
% It can refine itself to get Heavy \aname{}, which is more accurate than CM/CU sketch, and it can refine itself to get Light \aname{}, which can estimate infrequent items accurately. 
% How?
%

5) \textit{Certainty} for dominant items.
Given a data stream or a subset of the data stream, if the frequency of an item is larger than 50\% of the number of all items, we call it as the \textit{dominant item}.
% The designed sketch should b
It should be certain for the design sketch to keep the dominant items no matter how much memory is used.
Further, the estimated frequency of the dominant item should be more accurate than other items.

% More attention to frequent items.
% It can mining out frequent items directly and has higher accuracy for these items.
% We dispatch all items into $m$ buckets in an uniform distribution. For each bucket, the item with more than half of the frequency is called \textit{dominant item}. \aname{} can mining out dominant item exactly in real time with limited memory. And the dominant items are counted more accurately.





% %放到generality
% Common processing tasks\footnote{1)....5) } include frequency estimation \cite{cmsketch}, finding frequent items \cite{frequentstream}, heavy change detection \cite{changedetection}, flow size distribution \cite{flowsizedistribution} and entropy estimation \cite{estimatingentropy}.
% In practical scenarios, it is often required to perform multiple processing tasks at the same time.
% A straightforward solution is to build multiple \wyh{dedicated} sketches simultaneously to support multiple tasks and consequently incurring the overhead of both time and speed.
% Therefore, it is highly desired to design a versatile sketch to support multiple processing tasks at the same time.



%%Para2:
% There is an inherent contradiction between the versatility and the accuracy when the memory and computing resources are limited.
% As the versatility of the data structure becomes better, its structure becomes more complicated, and the accuracy becomes lower.
% Therefore, it is quite challenging to design a sketch with many properties.


% % It is obviously challenging to design a versatility sketch.
% % new:
% As the dedicated sketches have the best performance in specific tasks, it is challenging to devise a generic sketch and keep comparable accuracy.
% % , which is the design goal of this paper.
% % And it is more challenging to achieve versatility and keep comparable accuracy with existing specific sketches, which is the design goal of this paper.
% Besides the generality, we aim to assign more functions to our designed sketch.




% \presub
% \subsection{Prior Art and Their Limitations} \postsub

% Existing sketches can be divided into two categories:
% Counter-array based sketch and Heap-based sketches.
% Counter-array based sketches use multiple counter arrays, and each array is associated with a hash function. 
% Typical solutions include Count-Min (CM)~\cite{cmsketch}, CU~\cite{cusketch}, Count~\cite{countsketch}, Augmented~\cite{roy2016augmented} and more \cite{coldfilter,persistentsketch}.
% Heap based sketches use a priority-queue or a heap for recording items.
% Typical solutions include Space-Saving\cite{spacesaving}, Unbiased Space-Saving~\cite{unbiasedsketch} and ?Frequent~\cite{frequent}.
% %是不是要讲他们focus on的东西？
% However, these existing do not focus on versatility.






\presub
\subsection{Our Proposed Approach} \postsub


para1: to address, this paper prose ...
Claim:  fast, accurate....


Key idea: rationale


math, application, experimental 


key contribution;

%思想double side estimation至少需要两个counter，一大一小。 double-bound counts。low有多种办法，一样加，不一样不加。一样就加，不一样概率减。4、一样不加，不一样才加。
%本文选择一种最简单实用的形式。
%多了id以后有很多灵活性，替换策略、查询方式。为什么现有工作做不了versatile。有些有ID，但是只有counter，灵活性差，很多做不了。

%1、介绍sketch有啥功能、快、实现的和目标的是不是匹配。
%2、key idea 为啥能做versatile 为啥现有做不了。
%3、做了数学证明、实验、开源。

% 问杨老师：
% a、前面是不是要介绍为什么选择sketch算法，为什么是非精确的。是亚线性的。从sigmod第一轮的review看，似乎并不是所有review都懂非精确的estimate。
% b、如何从double-bound开始说。

point:1
all existing sketches use many buckets to store the summary of a data stream.
THerefore, each bucket is used to process a subset of a data stream.
Then we show how to desgin the data structure of a single bucket.

Among exisitng works, there are two typical desgins:
1) only one coutner in each bucket. such CM,CU, count, etc
advantage: simple, fast. easy to use, easy to implemet, each to depoly
disavataee: functions few
2) ID and frequency. such as spacswaing, frequent....
focus on top-k frequent items. ignore the frequency of cold items.
functions are also limited.

To achieve vasatility, we need add more infomration to each bucket.
Our key idea is to add more counter for each each in each bucket: ID, counter1, counter2, counter 3, counter 3....
THe more counter it uses, the more functions could be achieved.
Typically, we find using two counters are already to achieve many functions.
We will discuss using more counters for more fucntions in Section \ref{...sliding window, timestamp, aging.  flag, used to be a large flow, flowlet... flag, eviction, totall correct, freezing counter, ... }.


This paper mainly focus on how to use two counters to achieve many functions.
In our design, we give a simple case study, using high counter and a low counter, aiming to achieve the above desgin goal.
%
for simplicaty, we desgining the 3-tuple <ID, freq1, freq2>, meeting the following requirement:
First, For the recorded ID, we can estimate its upper bound and lower bound of its frequency.
Second, for the cold items (whose IDs are not recorded in buckets), we need to give a upper bound of their frquency.
Third, when two distinct items are mapped into one bucket, we use to use this two counter to decide the evction policy.
To staify these three requiement, we have several choice.
first, high, low; second, total, pure; third, positive counter, neative counters.
These three choice can achieve the simialr results, differetn fucntions, and we show how to use high and low. the details are poivded in section ....
discussion sections,,,, we show how to use other two counters to achieve different functions.



para:
math,,, experiment ....


%rationale: Sketch, Buckets, ideal
A typical sketch \textbf{distributes} 
a data stream to large amounts of buckets, and each bucket processes a subset of the data stream independently. 
%
The key design of a sketch is its buckets, each of which receives incoming items and reports the frequency of a given item. We will focus on designing a bucket in the following parts.
%
We should record two kinds of information, \ie, item IDs and frequencies, because we need them in \textit{finding Top-k frequent items} and we can indirectly estimate the distribution and entropy through frequency.
Besides, we are more concerned about high-frequency items, because they are the core factors of error and they get more attention in applications.
%
As the space is limited, we should make a trade-off between memory efficiency and recording all items.
A straightforward approach is to abandon the IDs of \textit{infrequent items}. In other words, an \textbf{ideal bucket} can maintain both IDs and frequencies of the top x items and maintain the total frequencies of all other items.
However, it is hard to maintain these information in practice. Because the bucket not only can hardly identify which items are the most frequent but also can hardly find true frequencies of the frequent items.
Therefore, we relax the requirement of ideal bucket from two aspects. First, we only require maintaining the ID of the top \#1 frequent item instead of top x frequent items, 
%
\textbf{because the second-largest frequency is often much smaller than the largest frequency.}%需不需要更详细地讨论？
Second, we require both an over-estimated frequency and an under-estimated frequency instead of an exact frequency.






We design a new bucket, called \textbf{versatile bucket}, to meet the requirement. 
In the bucket, we use a counteraction strategy to find the most frequent item, where the item whose frequency is larger than half must be found. 
A versatile bucket has three fields, a \textit{high} counter, a \textit{low} counter, and an \textit{ID} recorder. The counteraction strategy only uses the \textit{low} counter and the \textit{ID} recorder.
When a new item $e$ comes, if the \textit{ID} recorder is empty or the same as new item $e$, we set the \textit{ID} recorder to $e$ and increase the \textit{low} counter by $1$. Otherwise, we decrease the \textit{low} counter by $1$. After that, if the \textit{low} counter equals to $0$, we replace the item in \textit{ID} recorder with $e$.
The \textit{ID} recorder can find the most frequent item approximately.
Besides, the high counter increases by $1$ when a new item $e$ comes.
When querying the frequency of the item recorded in the \textit{ID} recorder, we can get its over-estimated/under-estimated frequency by $(high+low)/2$ and $low$ respectively. And we can estimate the over-estimated frequencies of other items by $(high-low)/2$.
As a sketch, \aname{} inserts an incoming item into multiple buckets and summaries all mapped buckets when querying.
We devise a conservative update strategy to reduce unnecessary insertions and prove its correctness rigorously.



Key contribution:


% 1、sketch算法的核心思想是把所有的item通过哈希插入到N个桶中的d个。查询时每个桶分别给出对频数的估计。因此设计一个合适的桶结构是设计sketch算法的关键点。要设计合适的桶结构，就要先回归到我们的5个目标，了解清楚我们究竟要存储哪些信息。从“通用性”支持的任务来看，我们需要保存元素的频数信息和ID。由于我们更关注高频元素，一个理想的情况是：忽略低频元素的ID，保存桶内最高频的k个元素的频数和id，以及其余元素的频数之和。这样的情况是 存储信息与内存占用之间最好的trade off。但是做不到理想情况。

% 2、几乎没有算法可以做到上述理想情况。我们从实验/理论分析可以看出，在常见分布下，第二大的元素频数往往远效于第一大的元素。因此我们仅保存最高频的元素，令k=1。另一方面，很难有算法可以在亚线性memory下精确求出某个元素的频数（可以构造算法证明没有，需要数学吗？）。因此，我们选择为最高频的元素提供尽可能准确的高估/低估估计。此外，我们的算法还要能够求出最高频的元素，但这也是不可能办到的。因此我们引入了dominant item的概念，即我们能保证求出频数大于50\%的元素，而且元素频数越高，留下来的概率越大。

% 3、具体的做法。相比于现有sketch，我们提供的一个新功能是double-bound。因此我们从double-bound入手来讨论我们对桶结构的设计。因为我们要给出高估/低估值与高频元素id，我们至少需要两个counter field和一个ID field。首先设计求高频元素的算法。有多种办法，“一样加，不一样不加”。“一样就加，不一样概率减”。概率替换/减到0替换。我们选择了“一样加，不一样不加，减到0替换”。这个算法能保证求出频数大于50\%的元素。同时，我们利用剩下的一个counter来记录元素总数。这时我们可以发现一个有趣的结论: (high+low)/2 是高频元素高估值， (high-low)/2是剩余元素之和的高估值。 除了桶设计以外，我们还引入了保守更新的策略。

% 4、这样的结构为啥versatile。


% Based on the Counter-Key-Counter structure, \aname{} achieves five functions.
% 1) It can report the possible range of the frequency of the recorded item by $[low, (high+low)/2]$ and that of the unrecorded item by $[0,(high-low)/2]$.
% 2) The recorded items and their frequencies can be applied to finding heavy hitters and heavy change. Further, the function of estimating frequency can be used for estimating item size distribution and entropy. 
% 3) A CKC bucket is flexible for splitting into two buckets, merging two buckets. Therefore, \aname{} is flexible for expansion, compression, and merging.
% 4) \aname{} can replace each CKC bucket with a counter whose value is $(high+low)/2$ to get an accurate sketch for frequent item. %light 没写
% 5) The dominant item in each bucket will be recorded in the ID field and its frequency can be estimated accurately.

% 5、并且做了数学证明、实验、开源。文章结构的overview。



% We propose a new sketch, namely \textit{Versatile Sketch}, in this paper. 
% It is based on Counter-Key-Counter (CKC) array structure and achieves versatility of five properties.
% %2、
% Our key idea of Counter-Key-Counter is to preserve both IDs and frequency upper/lower bounds for frequent items, which are more important than infrequent items for which we only preserve the upper bound.
% Specifically, the \aname{} is an array of Counter-Key-Counter buckets, and the devised bucket has three fields, a \textit{high} counter, an \textit{ID} recorder, and a \textit{low} counter.
% The \textit{ID} recorder can approximately record the most frequent item mapped to the bucket, and the item can be recorded for certain if the frequency of the item is larger than half of the total frequency of the items mapped to the bucket. The items whose frequencies are larger than half are called \textit{dominant item}.
% In a bucket, we can get the upper/lower bound of the frequency of the dominant item by $(high+low)/2$ and $low$ respectively. And we can estimate the upper bound of frequencies of infrequent items by $(high-low)/2$.
% As a sketch, \aname{} inserts an incoming item into multiple buckets to reduce hash collisions, and summaries all mapped buckets when querying.
% We devise a conservative update strategy to reduce unnecessary insertions and prove its correctness by rigorous analysis because the correctness is unintuitive.

% %3、
% Based on the Counter-Key-Counter structure, \aname{} achieves five functions.
% 1) It can report the possible range of the frequency of the recorded item by $[low, (high+low)/2]$ and that of the unrecorded item by $[0,(high-low)/2]$.
% 2) The recorded items and their frequencies can be applied to finding heavy hitters and heavy change. Further, the function of estimating frequency can be used for estimating item size distribution and entropy. 
% 3) A CKC bucket is flexible for splitting into two buckets, merging two buckets. Therefore, \aname{} is flexible for expansion, compression, and merging.
% 4) \aname{} can replace each CKC bucket with a counter whose value is $(high+low)/2$ to get an accurate sketch for frequent item. %light 没写
% 5) The dominant item in each bucket will be recorded in the ID field and its frequency can be estimated accurately.

% %4 
% The key novelty of \aname{} is our Counter-Key-Counter structure which is quite different from existing works.






%%%%%%%%%%%%%%%
%data stream frequency estimation重要性 挑战
% In data stream scenarios, huge volumes of high-velocity data are being produced continuously in real time, such as sensor data from the Internet of Things (IoT), graph streams, video streams, web Interactions, network traffics, and twitter posts \cite{?}.
% In these scenarios, data is organized as a sequence of items. Some common statistical analyzes, such as item frequencies \footnote{?}, heavy hitter \cite{?}, heavy change \cite{changedetection}, flow size distribution \cite{flowsizedistribution}, and entropy \cite{estimatingentropy}, are often require to process. And the analyzes are often being processed on the fly \cite{?}, which means the incoming items should be taken in real time and the statistical results could be fetched at anytime. 



% \textbf{The high-speed and high-volume data makes the data stream processing quite challenging.} First, the memory usage of the processing is limited in order to be implemented in high-speed medium (\eg, SRAM, ASIC \cite{?}??) whose footprints are expensive and limited.
% Second, the stream data should be processed on the fly. Finally, the accuracy of the analyze should be accurate enough.


%介绍sketch
% %sketch分类 讲不同
% Sketches, a kind of compact probabilistic data structure(s?), has become popular in recent years for stream data processing \cite{?}. Sketches are designed for estimating the frequency of items \cite{?} and the estimated frequency would be used for other statistical analyzes, including heavy hitter, heavy change, item size distribution, and entropy. 
% To explain the key idea of sketches, we choose the Count-Min (CM) sketch as an example. The CM sketch is a two-dimensional array counters with depth $d$ and width $w$. There are $d$ independent hash functions associated with $d$ rows. To insert item $e_i$, the CM sketch maps $e_i$ to \textit{the mapping counters} by the hash functions in each row, and increment each mapping counter by 1. To estimate the frequency of $e_j$ the CM sketch returns the minimum mapping counters.
% The key idea of sketches is to solve collision by mixing and answer the minimum collision.
% Compare with the hash table\cite{?}, sketches has the following three advantages. First, sketch is a sub-linear memory algorithm \cite{?} which is much more memory efficient than the per-item-state techniques (hash tables) \cite{?}. Second, the time for sketches to insert per item is constant while that for the hash table is not.
% Third, sketches is friendly for the hardware with the pipeline/multistage structure\cite{?} and is friendly for parallel processing because all units of sketches are independent.

% %需要同时测量多个任务，需要多样性
% %sketch功能缺乏，需要额外的数据结构补充，但是不能被视为完整结构。
% However, the weakness of sketches is the functional diversity. The ordinary sketches can only record the frequencies of items. The users can only resort to different kinds of additional special-designed structures if they needs any other information, such as the identification (ID) of frequent items, the average/latest arriving time of an item, or the average/maximum size of the packet load for a flow in network traffics scenario. Most additional structures only utilize the output frequency from sketches but cannot improve the performance of the sketches, which \textit{can hardly be regarded as an integral structure}.

% To add functions to the sketches, one straight forward idea is to add a new ID field to store items along with each counter. As sketches mixes all the frequency of the items mapped to the same counter, a serious error might happen when the queried infrequent item collides with a frequent item. It would be quite useful if we can record the most frequent items in every counter and separate their frequencies apart.




    %
% We propose a new sketch, namely \textit{Versatile Sketch}, in this paper.
% Our key idea comes from the open contest that the competitor whose ability exceeds the sum of all other competitors must be the winner on the stage, regardless of the order of the competitors.
% Instead of the counter, the basic unit of \aname{} is a bucket. Each bucket has three fields, a \textit{high} counter, a \textit{low} counter, and an \textit{ID} recorder. The high counter increments by $1$ when an item is inserted to the bucket, which is the same as the CM sketch.
% The item in the \textit{ID} recorder is the defender and the \textit{low} counter represents the health point of the defender. For an incoming item $e$ mapped to current bucket, we first check the ID recorder. If it is empty, we store item $e$ in the recorder and set the low counter to $1$. Otherwise, we check whether the defender item in ID recorder is $e$. If so, we increment the low counter by $1$. Otherwise, $e$ is an attacker so we decrement the low counter by $1$. If the low counter equals to $0$, the defender was defeated and we set the ID recorder to $null$.

% Among all items mapped to current bucket, the item whose frequency is larger than the sum of the others must be a defender left in the ID recorder and the item is called \textit{the dominant item}.
% We can estimate the frequency $f$ of the defender by $low$ and $(high+low)/2$, where $low\leq f \leq (high+low)/2$. And we can estimate the frequency $f'$ of other items mapped to current bucket by $(high-low)/2$, where $0\leq f' \leq (high-low)/2$.
% It is trivial that $low$ is the underestimated frequency of the defender but the overestimation $(high+low)/2$ is not straightforward. Suppose the defender is $e$. At the latest time $t_0$ that the ID recorder was set to $e$, the $low$ equaled to $0$. Before , the $e$ must appears no more than $high/2$ ( equals to $(high+low)/2$) times, because the dominant item, if exists, must be left in the ID recorder. After time $t_0$, $e$ remained in the recorder. In this period, every incoming $e$ will increased $(high+low)/2$ by $1$ and other items 
% did not change $(high+low)/2$. Therefore, $(high+low)/2$ is the overestimation. 
% Suppose the defender is $e$. For the item $e'$ ($e'\neq e$), $(high-low)/2$ is the overestimation of the frequency of $e'$. Because we can extract $low$ item $e$ from $high$ total items and it is impossible to occupy half of the rest because of the property of the dominant item.
% Additionally, if all collisions (\ie, the case that the incoming item is not the recorded item) happen between the final defender $e$ and other items, $(high+low)/2$ is the no-error estimation of $e$.

% The \aname{} has the following seven novel functions.
% \begin{itemize}
%     \item it can mining out the dominant item in each buckets and has higher accuracy for the dominant item.
%     %
%     \item it is the first sketch for two-sided boundary estimation while the other sketches can only do one-side estimation.
%     %
%     \item it can be applied to four applications, including heavy hitter, heavy change, item size distribution and entropy.
%     %
%     % \item it is hardware-friendly because it can be easily implemented in pipeline structured hardware and it do not need heap or pointer.
%     %
%     \item its structure is flexible for expansion, compression, and merging, which are important operations for distributed systems.
%     %
%     \item it can refine itself to get Heavy \aname{} which is more accurate than CM/CU sketch and it can refine itself to get Light \aname{} which can estimate infrequent items accurately.
%     %
%     % \item it supports conservative update which can improve the accuracy.
%     %
%     % \item KV store??
% \end{itemize}



% the dominant item %重要性。

% \old{One of the most fundamental problems in approximate data stream mining is finding top-$k$ items. }
% %
% Top-$k$ is defined in terms of various metrics. Four kinds of top-$k$ items under different metrics have attracted wide attention by researchers: 1) top-$k$ \textit{frequent items} \cite{frequent, frequent2, frequentstream, countsketch, persistentsketch}, 2) top-$k$ \textit{heavy changes} \cite{revsketch, kary, flowradar}, 3) top-$k$ \textit{persistent items} \cite{persistentsketch, persisitem}, and 4) top-$k$ \textit{Super-Spreaders} \cite{superspreader}. 
% %
% \textit{Frequent items} refer to items whose numbers of appearances exceed a predefined threshold. \textit{Heavy changes} refer to items whose frequencies change drastically over two adjacent time windows. \textit{Persistent items} are items which appear in more time windows than others. \textit{Super-Spreaders} refer to sources that connect to a large number of distinct destinations. 
% %
% Although these four kinds of tasks have different metrics, we find that if an algorithm does well in finding frequent items, it can also well handle the other three tasks.
% %
% The reason behind is discussed below. 
% %
% To find heavy changes in two adjacent time windows, we can first find all frequent items in both time windows respectively since heavy changes must be frequent items in at least one time window.
% %
% Then heavy changes can be detected through calculate the absolute change in frequencies of those frequent items in the two time windows.
% %
% Persistent items and frequent items are equivalent if the frequency of an item is defined as the number of time windows in which it appears.
% Similarly, for finding Super-Spreaders, we only need to view the number of destinations an item connects to as its frequency.
% %
% %As to finding Super-Spreaders, we can view the number of destinations an item connects to as its frequency, then the task is transformed to finding frequent items. 
% %In conclusion, algorithms for finding frequent items can deal with the above tasks, and if it performs well in finding frequent items, it will probably also achieve good performance in these tasks.
% %
% %Sketches, a kind of probabilistic data structure, have attracted wide interests in recent years, due to their memory efficiency and small error for .....
% In summary, if a data structure can accurately find frequent items, it can also well handle other three tasks. Therefore, we only consider finding frequent items in this section below.
% %
% In practice, sketches, a kind of probabilistic data structure, have been widely used in finding top-$k$ items, due to their memory efficiency and small error for estimating item frequencies.


% %
% \textit{Unbiased estimation} is well acknowledged as a theoretically elegant and pragmatic property.
% %Therefore, we aim at devising a sketch which can report unbiased estimation of item's frequency.
% %
% % for frequency estimation
% %Frequency estimation is the key technique in finding frequent items. of a frequency estimation algorithm.
% %
% Unbiased estimation of item frequencies is beneficial for several global estimation problems, such as global heavy hitters, global distribution, global entropy, \etc For example, to measure distributed data streams, one data structure is deployed for each data stream. If their estimations are biased, the error will accumulate when the data structures are aggregated.
% %
% Further, unbiased approaches could stimulate theoretical progress in sketches. Although numerous sketches have been proposed, only a very few of them (Count-Min Sketch \cite{cmsketch}, Count Sketch \cite{countsketch}) have explicit and concise theory bounds and proofs, and most of the others show error bounds and proofs that are fairly complicated. One of the primary reasons for this is that their estimations are biased.


% Among a large number of algorithms for finding frequent items \cite{cmsketch, cusketch, countsketch, spacesaving, frequent, losscounting, unbiasedsketch}, one recent work, Unbiased SpaceSaving (USS) \cite{unbiasedsketch}, achieves unbiased estimation. 
% %
% While USS makes a great contribution in terms of unbiased estimation, its accuracy is relatively low, \ie, its variance of estimation is large. As a result, when it is applied to other tasks (\eg, finding heavy changes, persistent items, or Super-Spreaders), the inaccuracy of frequency estimation will incur large error for other tasks, which may be the reason why USS was only used for frequent items in the paper \cite{unbiasedsketch}.
% %the shortcomings brought by its inaccuracy grow disturbing, which makes it inappropriate for USS to be deployed in these task. 
% %
% %In summary, prior unbiased algorithms, such as USS, are too inaccurate to be generic, this is why no prior algorithm achieves both unbiased estimation and generality.
% %
% The goal of our study is to devise an algorithm which is unbiased, and accurate enough to be generic for other tasks.



% %The goal of our study is to devise an algorithm which is unbiased as well as accurate in the task of finding frequent items and is capable of handling the other three tasks mentioned above. 
% %In processing high-rate data streams, finding \textit{frequent items} has long been a crucial problem and an active topic \cite{frequent, frequent2, frequentstream, countsketch, persistentsketch}.
% %
% %A lot of applications involve finding \textit{frequent items}, such as congestion control \cite{usagefrequent1} and caching of forward table entries \cite{usagefrequent3}.
% %应用需要改

% %Items with other special characteristics are also of general interest. Some of the most interested among them are heavy changes \cite{revsketch, kary, flowradar}, persistent items \cite{persistentsketch, persisitem}, and Super-Spreaders \cite{superspreader}.
% %

% %
% %These items are especially important in the field of security \cite{usageother2, usageother3}. Existing algorithms are often utilized to detect denial of service attacks \cite{usageother2}, and worms \cite{usageother3}.

% %

% \presub
% \subsection{Our Proposed Approach} \postsub

% \paragraph{rationale:}eliminate the error of minor flows.
% \paragraph{arena game}
% \paragraph{properties}

% In this paper, we propose a new sketch, namely \aname{}, which is unbiased, accurate, and generic for finding top-$k$ items. 
% %
% We use a simple example to show the key idea of \aname{}. We use a counter and a list. The counter, namely the Waving Counter, provides an unbiased estimation of item frequencies and the list is used to store $k'$ $(k'>k)$ frequent items.
% %
% For each incoming item $e$, we use a hash function $s(e)$ to hash $e$ to $+1$ or $-1$, and then increase or decrease the Waving Counter by 1. Afterwards, we estimate $e$'s frequency using the Waving Counter. 
% %
% %We have proved that the counter can provide an unbiased estimation of frequency for any item appeared before.
% If its frequency is larger than the smallest frequency in the list, we exchange them.  
% %
% Based on this idea, we use a group of Waving Counters and lists, and add additional fields in the list to achieve higher accuracy (see details in Section \ref{subsec:alg:struct}).
% %



% Below we explain the rationale of \aname.
% The value of the Waving Counter fluctuates over time, and it is quite analogous to the waves in the sea. 
% %
% Where there is a heavy swell, there is probably a strong flow driving it.
% %
% Therefore, we expect to catch a frequent item when the absolute value of the counter is fairly high.
% %
% %This idea is quite reasonable. 
% %
% Specifically, given an incoming item, we use the Waving Counter to unbiasedly estimate its frequency.
% %provide unbiased estimation for its frequency.
% %The value of the Waving counter can provide an unbiased estimation to the incoming item.
% If the estimated frequency is large enough, it is with high probability that the incoming item is frequent enough to replace the least frequent item in the list.


% \aname{} has four advantages. First, it is unbiased, and we theoretically prove that the estimated frequency of \aname{} is unbiased in Section \ref{subsec:math:unbiased}. 
% %
% Second, our theoretical and experimental results show that the error of \aname{} is much smaller than SpaceSaving and Unbiased SpaceSaving.
% %
% Third, \aname{} is generic. To verify this, we apply \aname{} to four applications: finding frequent items, finding heavy changes, finding persistent items, and finding Super-Spreaders.
% %
% Fourth, \aname{} is fast. For each insertion or query, we only need to access one bucket and it often requires only one memory access.
% %1次连续访存

% \ppp{Main Experimental Results:}
% In finding frequent items, compared with USS, \aname{} achieves $4.50$ times higher insertion speed and up to $9 \times 10^6$ times ($2 \times 10^4$ times in average) smaller error rate.
% % reduces the error up to $9 \times 10^6$ times ($66$ times in average) and improves the insertion throughput by $4.50$ times in average.
% %
% In finding heavy changes, \aname{} improves the F1 Score \cite{f1score} by $8$ times in average when using only $1/10$ of the memory size of other algorithms and improves the insertion speed by up to $1.9$ times. 
% %
% In finding persistent items, \aname{} achieves up to $7.5$ times higher insertion speed and up to $286$ times smaller error rate.
% % the error by up to $56$ times and improves the insertion throughput up to $7.5$ times.
% %
% In finding Super-Spreaders, \aname{} achieves up to $14$ times lower error rate. 
% %
% All related codes are open-sourced and available at Github anonymously \cite{opensource}.

% \presub
% \subsection{Contributions} \postsub
% \begin{itemize}
%     \item We propose the \aname{}, which provides unbiased and accurate estimation of items in data streams.
%     \item We theoretically prove that \aname{} achieves unbiased estimation, and show that its error is often much smaller than the state-of-the-art, USS \cite{unbiasedsketch}. 
%     \item We apply \aname{} to four applications: finding frequent items, finding heavy changes, finding persistent items, and finding Super-Spreaders.
%     \item We conduct extensive experiments, and the results show that \aname{} achieves up to two orders of magnitude smaller error than the state-of-the-art.
% \end{itemize}


